Universal linguistic inductive biases via meta-learning

How do learners acquire languages from the limited data available to them? This process must involve some inductive biases - factors that affect how a learner generalizes - but it is unclear which inductive biases can explain observed patterns in language acquisition. To facilitate computational modeling aimed at addressing this question, we introduce a framework for giving particular linguistic inductive biases to a neural network model; such a model can then be used to empirically explore the effects of those inductive biases. This framework disentangles universal inductive biases, which are encoded in the initial values of a neural network's parameters, from non-universal factors, which the neural network must learn from data in a given language. The initial state that encodes the inductive biases is found with meta-learning, a technique through which a model discovers how to acquire new languages more easily via exposure to many possible languages. By controlling the properties of the languages that are used during meta-learning, we can control the inductive biases that meta-learning imparts. We demonstrate this framework with a case study based on syllable structure. First, we specify the inductive biases that we intend to give our model, and then we translate those inductive biases into a space of languages from which a model can meta-learn. Finally, using existing analysis techniques, we verify that our approach has imparted the linguistic inductive biases that it was intended to impart.

==> CHANGES <==
%% The LaTeX package tcolorbox - version 4.30 (2020/04/28)
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2020 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%

(2006-2011): pre publication usage

version 1.00 (2011/12/08): initial public release

version 1.01 (2012/01/26):
- dates amended to \RequirePackage(s)
- provision of the tcolorbox.tds.zip file for easier installation

version 1.02 (2012/02/15)
- documentation language changed from German to English
- small correction of the theorem title line appearance

version 1.10 (2012/03/01)
- tcblatex style for listings changed (nolol added)
- improved hyperref support
- new keys parskip and noparskip
- source code of the documentation added
- new library 'documentation' to support LaTeX documentations
  with several library commands, environments and keys (see documentation)

version 1.20 (2012/03/16)
- new geometry keys:
  'lefttitle', 'leftupper', 'leftlower', 'righttitle', 'rightupper', 'rightlower'
  and implementation changed for 'left' and 'right'
- implementation for tcolorbox changed (adaption to height options)
- new fixed height option keys:
  'natural height', 'height', 'equal height group', 'minimum for equal height group',
  'space', 'space to upper', 'space to lower', 'space to both', 'split',
  'valign', 'valign lower',
  'adjusted title'
- new bounding box option keys:
  'enlarge top by', 'enlarge bottom by', 'enlarge left by', 'enlarge right by',
  'toggle enlargement'
- preparations for a future skin changing option implemented
- commands \brackets and \docAuxCommand added to the documentation library
- documentation rearranged

version 1.30 (2012/04/20)
- several internal code changes to provide a 'skin' exchange mechanism
- new keys for the core package:
  'frame engine', 'interior titled engine', 'interior engine', 'segmentation engine'
  'skin', 'graphical environment', 'geometry nodes', 'colupper', 'collower'
- tcolorbox now defined as 'long' macro
- new keys for the library 'listings':
  'comment', 'listing and comment', 'comment and listing'
- new library 'skins' with the skins
  'standard', 'enhanced', 'freelance', 'bicolor', 'beamer', 'widget'
- keys for the library 'skins':
  'frame style', 'interior style', 'segmentation style'
  'frame code', 'interior titled code', 'interior code', 'segmentation code',
  'colbacklower'

version 2.00 (2013/03/01)
- breaking news: the new library 'breakable' adds breaking support to tcolorbox.
- e-TeX now used instead of calc
- new key 'adjust text' and new implementation for 'adjusted title'
- new geometry keys:
  'toprule', 'toprule at break', 'bottomrule', 'bottomrule at break',
  'leftrule', 'rightrule', 'titlerule', 'outer arc', 'auto outer arc',
  'toptitle', 'bottomtitle'
- new bounding box keys:
  'enlarge top at break by', 'enlarge bottom at break by'
- new overlay keys:
  'overlay', 'no overlay', 'overlay broken', 'overlay unbroken',
  'overlay first', 'overlay middle', 'overlay last',
  'overlay unbroken and first', 'overlay middle and last'
- new key: 'parbox' to change text behaviour
- new library 'breakable' for breakable boxes with the new keys:
  'breakable', 'unbreakable', 'title after break', 'notitle after break',
  'adjusted title after break', 'lines before break', 'shrink break goal'
- new keys for the 'skins' library
  'skin first', 'skin middle', 'skin last', 'title engine', 'pathfirst',
  'pathmiddle', 'pathlast', 'title style', 'title code', 'enhancedfirst',
  'enhancedmiddle', 'enhancedlast', 'enhanced', 'marker', 'bicolor',
  'bicolorfirst', 'bicolormiddle', 'bicolorlast', 'beamer',
  'beamerfirst', 'beamermiddle', 'beamerlast', 'draft', 'freelance', 'standard'
- NOTE: skins 'beamer' and 'widget' changed
  use the new style options 'beamer' and 'widget' to get the old appearance
- new watermark keys:
  'watermark text', 'watermark text on', 'watermark graphics',
  'watermark graphics on', 'watermark tikz', 'watermark tikz on',
  'no watermark', 'watermark opacity', 'watermark color',
  'watermark zoom', 'watermark stretch'

version 2.01 (2013/03/07)
- bug fix: superfluous vertical space for a breakable box which appeared after a page break
- bug fix: height computation error when a broken boxed starts with a segmentation line
- new key for the 'listings' library:
  'listing inputencoding'
- new library 'listingsutf8' as variant of 'listings' with new key
  'listing utf8'
- keys 'toprule at break', 'bottomrule at break',
  'enlarge top at break by', 'enlarge bottom at break by'
  moved from core package to 'breakable' library.
- new keys for the 'breakable' library:
  'topsep at break', 'bottomsep at break', 'pad before break',
  'pad after break', 'pad at break'

version 2.02 (2013/03/13)
- minor bug fix: segmentation line of 'enhanced' now matches 'standard'
- new macro '\tcbox' to draw a colorbox fitted to the content width
- new key 'autoparskip' to detect usage of package parskip automatically
- new key 'nobeforeafter'
- new macro '\tcbline' in the 'skins' library to draw 'just lines'
- new key 'colbacktitle' for the 'skins' library

version 2.10 (2013/04/09)
- bug fix: \tcbox ignored font settings
- outdated documentation in German removed from package
- new core package keys:
  'oversize', 'tcbox raise', 'tcbox raise base',
  'before title', 'after title', 'before upper', 'after upper', 'before lower',
  'after lower', 'center title', 'center upper', 'center lower',
  'tabularx*', 'tabularx', 'tikz upper', 'tikz lower',
  'shrink tight', 'extrude left by', 'extrude right by', 'extrude top by',
  'extrude bottom by', 'extrude by'
- the 'theorems' library now loads 'amsmath'
- new macros for the 'theorems' library:
  '\tcboxmath', '\tcbhighmath'
- new keys for the 'theorems' library:
  'math upper', 'math lower', 'math', 'highlight math', 'highlight math style',
  'ams equation upper', 'ams equation lower', 'ams equation', 'ams equation* upper',
  'ams equation* lower', 'ams equation*', 'ams align upper', 'ams align lower',
  'ams align', 'ams align* upper', 'ams align* lower', 'ams align*',
  'ams gather upper', 'ams gather lower', 'ams gather', 'ams gather* upper',
  'ams gather* lower', 'ams gather*',
  'ams nodisplayskip upper', 'ams nodisplayskip lower', 'ams nodisplayskip'
- new library 'hooks' for hook options with the new keys:
  'before upper app', 'before upper pre', 'after upper app', 'after upper pre',
  'before lower app', 'before lower pre', 'after lower app', 'after lower pre',
  'before title app', 'before title pre', 'after title app', 'after title pre',
  'before app', 'before pre', 'after app', 'after pre',
  'overlay unbroken app', 'overlay unbroken pre', 'overlay first app', 'overlay first pre',
  'overlay middle app', 'overlay middle pre', 'overlay last app', 'overlay last pre',
  'overlay app', 'overlay pre', 'overlay broken app', 'overlay broken pre',
  'overlay unbroken and first app', 'overlay unbroken and first pre',
  'overlay middle and last app', 'overlay middle and last pre',
  'watermark tikz app', 'watermark tikz pre', 'watermark tikz app on', 'watermark tikz pre on',
  'watermark graphics app', 'watermark graphics pre', 'watermark graphics app on', 'watermark graphics pre on',
  'watermark text app', 'watermark text pre', 'watermark text app on', 'watermark text pre on',
  'frame code app', 'frame code pre', 'interior titled code app', 'interior titled code pre',
  'interior code app', 'interior code pre', 'segmentation code app', 'segmentation code pre',
  'title code app', 'title code pre'
- colorization of source code snippets in the documentation

version 2.20 (2013/04/17)
- bug fix: problem with breaking boxes after headings
- new feature: support for boxes with side by side content
- new keys:
  'sidebyside', 'sidebyside align', 'sidebyside gap',
  'lefthand width', 'righthand width', 'lefthand ratio', 'righthand ratio'
- key 'nofloat' documented
- new keys for the 'listings' library:
  'listing side text', 'text side listing'
  'listing outside text', 'text outside listing'
- new keys for the 'skins' library:
  'frame hidden', 'interior hidden', 'segmentation hidden', 'title hidden'
- new environments for the 'documentation' library:
  'dispExample*', 'dispListing*'
- the default style for 'highlight math' is changed to have no title
- minor change of internal width computation
- minor internal fixes
- slight overhaul of the documentation

version 2.21 (2013/04/23)
- bug fix: \tcbox and 'sidebyside' needed 'breakable' library
- bug fix: library 'tcbhooks' relied on etoolbox package
- bug fix: breaking boxes between upper part and box frame
- new macro '\newtcolorbox'
- new macro '\newtcblisting' for the 'listings' library
- new key 'code'
- documentation corrections and extensions

version 2.22 (2013/05/15)
- bug fix: text color bleeded out of the box in some cases
- bug fix: breakable boxes were too large in some cases (leading to blank pages)
- bug fix: breaking boxes produced empty boxes in some cases
- documentation forgot naming package 'colortbl' for the 'tabularx' option
- new feature: breakable boxes allow footnotes now (like minipages)
- new macro '\newtcbox'

version 2.30 (2013/06/04)
- bug fix: handling of 'before' and 'after' for \tcbox corrected
- \tcbline now also works for centered environments
- implementation for \tcbox made more efficient
- new capture mode for automated content fit by font size adjustment
  with the new macros '\tcboxfit' and '\newtcboxfit'
  and the new keys 'fit', 'fit to', 'fit to height', 'fit basedim', 'fit skip',
  'fit maxstep'
- new keys 'baseline', 'capture', 'hbox', 'minipage'
- new stackable borderlines with the 'skins' library:
  'borderline', 'no borderline'
- new keys for the 'skins' library:
  'enhanced standard', 'blank'
- new key 'index format' for the 'documentation' library

version 2.31 (2013/06/18)
- several internal changes
- library loading mechanism revisited
- internal label change for '\tcbmaketheorem'
- new library options 'most' and 'all'
- \tcbline now also works for ragged environments
- new keys:
  'flushleft title', 'flushleft upper', 'flushleft lower',
  'flushright title', 'flushright upper', 'flushright lower'
- new key 'no listing options' for the 'listings' library
- new shadow features for the 'skins' library with the options:
  'shadow', 'fuzzy shadow', 'drop shadow', 'drop fuzzy shadow', 'halo', 'fuzzy halo'
- shadows for the 'beamer' skin changed to fuzzy
- new library 'fitting' for the content fit operations.
  NOTE: '\tcboxfit' and the fit options introduced in version 2.30 are moved
        to this new library
- the fit algorithm is completey revisited and extended
- new macro '\tcbfontsize' ('fitting library') for relative font sizes
- new keys for the 'fitting' library:
  'fit fontsize macros', 'fit height plus', 'fit width plus',
  'fit width from', 'fit height from'

version 2.32 (2013/06/23)
- bug fix: 'ams nodisplayskip lower' was applied to upper.
- new option 'check odd page'
- new environments for the 'skins' library:
  'tcbclipinterior', 'tcbclipframe', 'tcbcliptitle'
- new keys for the 'skins' library:
  'watermark overzoom', 'clip watermark'
  'clip title', 'clip upper', 'clip lower'
- NOTE: watermarks are now clipped by default.
  To get the old behaviour add the option 'clip watermark=false'

version 2.33 (2013/07/04)
- new options 'phantom', 'step and label', 'nophantom',
  'lower separated', 'reset', 'toggle left and right'
- 'highlight math' sets 'notitle,nophantom' automatically
- hyper anchor setting for theorems and LaTeX examples improved
- new key 'shield externalize' for externalization
- additional empty-first-box test for breakable boxes
- new key 'enlargepage' for fine-tuning breakable boxes
- parameter added to option 'oversize'
- option 'toggle enlargement' has a default value 'evenpage' now

version 2.40 (2013/07/15)
- bug fix: wrong footnote text width for breakable boxes
- bug fix: watermarks were influenced by baseline settings
- package etoolbox is now loaded by default
- 'phantom' changed to be stackable (!)
- introducing the new initialization option type for easy
  numbering and list generation. New options:
  'use counter', 'auto counter', 'use counter from',
  'no counter', 'number within', 'number format', 'number freestyle',
  'list inside', 'list type'
- '\newtcolorbox' and 'newtcbox' take initialization options now
- new macros '\tcblistof', '\tcbsetmanagedlayers'
- introducing the layered box concept for boxes in boxes improvement:
  * boxes inside boxes are automatically reset to default values
  * new option 'every box', 'every box on layer x', 'every box on higher layers'
  * support for footnotes for boxes in boxes (default: up to layer 4)
- new options 'step', 'label', 'list entry', 'add to list'
- library 'listings':
  * '\newtcblisting' takes initialization options now
  * new macro '\newtcbinputlisting'
- library 'theorems':
  * '\tcbmaketheorem' takes initialization options now
  * new macro '\newtcbtheorem'
- library 'fitting':
  * 'newtcboxfit' takes initialization options now
- library 'documentation':
  * the \ref... macros suppress the page numbers now if on the same page
  * new macros '\refCom*', '\refEnv*', '\refKey*'
  * docCommand and docEnvironment take options now

version 2.41 (2013/07/23)
- NOTE: The deprecated macro '\tcbmaketheorem' is redefined to its signature
  of v2.33 and before to ensure backward compatibility. This may break code
  written with v2.40 using '\tcbmaketheorem'.
- minor internal improvements
- support for the cleveref package with
  * new initialization options 'crefname', 'Crefname'
  * new options 'label type', 'no label type'
- library 'theorems':
  * new options: 'separator sign', 'separator sign colon', 'separator sign dash'
- library 'listings':
  * capture mode can be changed for 'tcblisting' and '\tcbinputlisting'
  * new option: 'listing remove caption'

version 2.50 (2013/07/29)
- first line indent corrected for 'parbox=false'
- minor internal improvements
- new option keys
  'height plus', 'height from'
- new library 'minted' with support for the minted package (Pygments support)
  * new options 'minted language', 'minted options', 'minted style'
- new library option 'many'
- new common listings options:
  'listing engine'
- library 'documentation':
  * new options 'documentation minted style', 'documentation minted options'

version 2.51 (2013/09/16)
- bug fix: processing of 'initialization option keys' fixed
  for \newtcbox, \newtcbinputlisting, and \newtcboxfit
- bug fix: disturbing horizontal space in \tcboxfix removed
- new macros '\renewtcolorbox', '\renewtcbox'
- library 'skins':
  * implementation for the skin families 'enhanced', 'beamer', and 'bicolor' changed
  * break sequence changed for skin 'freelance'
  * new skins: 'freelancefirst', 'freelancemiddle', 'freelancelast'
  * new options: 'extend freelance', 'extend freelancefirst',
    'extend freelancemiddle', 'extend freelancelast',
    'drop midday shadow', 'drop fuzzy midday shadow'
  * new environment 'tcbinvclipframe'
- library 'listings':
  * new macros '\renewtcblisting', '\renewtcbinputlisting'
- library 'theorems':
  * new macro '\renewtcbtheorem'
- library 'fitting':
  * new macro '\renewtcboxfit'
- library 'documentation':
  * new option 'documentation listing options'

version 2.60 (2013/12/17)
- new 'jigsaw' variants for the skins 'standard' and 'enhanced' for
  advanced transparency and similar effects.
- new package core skin 'standard jigsaw'
- 'tabularx' and 'tabularx*' reset the arrayrulecolor to black after the table now.
- option 'colbacktitle' moved from library 'skins' to package core
- new options:
  'title filled', 'opacityupper', 'opacitylower', 'opacitytitle', 'opacityframe',
  'opacityback', 'opacitybacktitle', 'opacityfill', 'opacitytext','hyphenationfix',
  'standard jigsaw', 'enlarge by', 'grow to left by', 'grow to right by'
- library 'skins':
  * new skin: 'enhanced jigsaw', 'enhancedfirst jigsaw', 'enhancedmidle jigsaw',
    'enhancedlast jigsaw'
  * marker style now based on 'enhancedmiddle jigsaw'
  * new options:
  'enhanced jigsaw', 'tikz', 'tikz reset', 'show bounding box',
  'at begin tikz', 'at begin tikz reset', 'at end tikz', 'at end tikz reset',
  'rotate', 'scale', 'remember', 'remember as',
  'drop shadow southeast', 'drop shadow south', 'drop shadow southwest', 'drop shadow west',
  'drop shadow northwest', 'drop shadow north', 'drop shadow northeast', 'drop shadow east',
  'drop fuzzy shadow southeast', 'drop fuzzy shadow south', 'drop fuzzy shadow southwest',
  'drop fuzzy shadow west', 'drop fuzzy shadow northwest', 'drop fuzzy shadow north',
  'drop fuzzy shadow northeast','drop fuzzy shadow east',
- library 'listings':
  new options 'text above listing' and 'listing above text'
- library 'theorems':
  \newtcbtheorem creates an additional starred theorem environment
- library 'fitting':
  fit algorithm warning switched off by default.
  new options:
  'fit warning'
- library 'documentation': more values for 'index format'
- documentation extended
- major internal implementation changes and optimizations

version 2.61 (2014/01/10)
- bug fix: '@' was set as letter in some situations
- typing error corrections
- new macro \tcbsetforeverylayer
- library 'skins':
  * new macros and environments:
    '\tcbstartdraftmode', '\tcbstopdraftmode', '\tcbinterruptdraftmode', '\tcbcontinuedraftmode'
  * new skin: 'spartan'
  * new options: 'spartan', 'draftmode'
- library 'fitting':
  * alternative fitting algorithms implemented (fontsize, areasize, hybrid, squeeze)
  * new option: 'fit algorithm'

version 2.70 (2014/02/06)
- bug fix: global setting of 'before' or 'after' may produce errors or
           side effects for layered boxes.
- compatibility issue with TikZ 3.00 solved
- new options:
  'detach title', 'attach title', 'attach title to upper',
  'tikznode upper', 'tikznode lower', 'tikznode'
- library 'theorems':
  * new options:
  'separator sign none', 'terminator sign', 'terminator sign colon',
  'terminator sign dash', 'terminator sign none', 'description delimiters',
  'description delimiters parenthesis', 'description delimiters none',
  'theorem name and number', 'theorem number and name', 'theorem name',
  'theorem style'
- library 'documentation':
  * re-implementation of the documenting environments
    (may alter existing documents slightly)
  * new environments:
    'docCommand*', 'docEnvironment*', 'docKey*'
  * new commands:
    '\docAuxCommand*', '\docAuxEnvironment', '\docAuxEnvironment*',
    '\docValue', '\docValue*', '\docAuxKey', '\docAuxKey*',
    '\docColor*', '\refAux', '\refAuxcs'
  * new options:
    'doc left', 'doc right', 'doc left indent', 'doc right indent',
    'doc head', 'doc head command', 'doc head environment', 'doc head key',
    'doc description', 'doc into index', 'value', 'values'

version 2.71 (2014/02/21)
- bug fix: sidebyside setting with empty left hand side caused false positioning
- new options:
  'external', 'remake'
- library 'listings':
  * new options:
    'comment side listing', 'listing side comment', 'comment above listing',
    'listing above comment', 'comment outside listing', 'listing outside comment',
    'image comment',
- library 'documentation':
  * automatic inclusion of the 'skins' library
  * inclusion of 'makeidx' made dependent on the existence of '\printindex'
  * new options:
    'keys', 'index colorize', 'index annotate',
    'color command', 'color environment', 'color key', 'color value', 'color color'

version 2.72 (2014/03/18)
- bug fix: mixing \newtcblisting with 'ams align' and similar options was not possible
- bug fix: footnotes lost for 'listing outside text' and similar options
- sidebyside and outside implementation slightly changed for beamer usage
- bicolor skin respects 'opacityback' for the upper part now
- new TikZ options:
  'fill image opacity', 'fill image options',
  'fill plain image', 'fill plain image*', 'fill stretch image', 'fill stretch image*',
  'fill overzoom image', 'fill overzoom image*', 'fill zoom image', 'fill zoom image*',
  'fill shrink image', 'fill shrink image*', 'fill tile image', 'fill tile image*'
- library 'skins':
  * new options:
    'frame style image', 'frame style tile', 'interior style image', 'interior style tile',
    'title style image', 'title style tile'
- library 'listings':
  * new options:
    'every listing line', 'every listing line*'

version 2.80 (2014/03/31)
- implementation changed for all '\newtcolorbox', '\newtcbox', etc., macros.
- new option:
  'float*'
- new TikZ option:
  'fill image scale'
- library 'skins' new option:
  'watermark shrink'
- new library 'xparse' with new commands:
  '\DeclareTColorBox', '\NewTColorBox', '\RenewTColorBox', '\ProvideTColorBox',
  '\DeclareTotalTColorBox', '\NewTotalTColorBox', '\RenewTotalTColorBox', '\ProvideTotalTColorBox',
  '\DeclareTCBox', '\NewTCBox', '\RenewTCBox', '\ProvideTCBox',
  '\DeclareTotalTCBox', '\NewTotalTCBox', '\RenewTotalTCBox', '\ProvideTotalTCBox',
  '\DeclareTCBListing', '\NewTCBListing', '\RenewTCBListing', '\ProvideTCBListing',
  '\DeclareTCBInputListing', '\NewTCBInputListing', '\RenewTCBInputListing', '\ProvideTCBInputListing',
  '\DeclareTCBoxFit', '\NewTCBoxFit', '\RenewTCBoxFit', '\ProvideTCBoxFit',
  '\DeclareTotalTCBoxFit', '\NewTotalTCBoxFit', '\RenewTotalTCBoxFit', '\ProvideTotalTCBoxFit',
  '\tcboxverb'

version 3.00 (2014/05/08)
- bug fix: 'title code app', 'title code pre' changed wrong code
- documentation corrections
- implementation of graphical engines changed (!)
- note: optical backward compatibility issues with breakable 'freelance' boxes possible
- 'frame code' and similar options are moved from the 'skins' library to the core package
- 'enlarge top at break by' and 'enlarge bottom at break by' moved from 'breakable' library to the core package
- new macros:
  '\tcbnewsubskin'
- new options:
  'skin first is subskin of', 'skin middle is subskin of', 'skin last is subskin of',
  'enlarge top initially by', 'enlarge finally last by', 'overlay unbroken and last'
  'size', 'on line', 'varwidth upper',
  'frame empty', 'interior empty', 'interior titled empty', 'segmentation empty', 'title empty'
- new TikZ options:
  'tcb fill frame', 'tcb fill interior', 'tcb fill title'
  'fill plain picture', 'fill stretch picture', 'fill overzoom picture',
  'fill zoom picture', 'fill shrink picture', 'fill tile picture', 'fill tile picture*'
- library 'skins' new options (concerning 'underlay', 'finish' and 'boxed title'):
  'underlay unbroken', 'underlay first', 'underlay middle', 'underlay last',
  'underlay', 'underlay broken', 'underlay unbroken and first',
  'underlay middle and last', 'underlay unbroken and last',
  'no underlay unbroken', 'no underlay first',
  'no underlay middle', 'no underlay last', 'no underlay',
  'finish unbroken', 'finish first', 'finish middle', 'finish last',
  'finish', 'finish broken', 'finish unbroken and first',
  'finish middle and last', 'finish unbroken and last',
  'no finish unbroken', 'no finish first',
  'no finish middle', 'no finish last', 'no finish',
  'empty', 'blanker',
  'boxed title style', 'varwidth boxed title', 'varwidth boxed title*',
  'minipage boxed title', 'minipage boxed title*', 'tikznode boxed title',
  'hbox boxed title', 'boxtitle/xshift', 'boxtitle/yshift', 'boxtitle/yshifttext',
  'boxtitle/yshift*', 'attach boxed title to top left', 'attach boxed title to top center',
  'attach boxed title to top right', 'attach boxed title to bottom left',
  'attach boxed title to bottom center', 'attach boxed title to bottom right',
- new engine and skin 'empty'
- implementation of 'show bounding box' changed to be a border line.
- library 'hooks' new options:
  'underlay unbroken pre', 'underlay first pre', 'underlay middle pre',
  'underlay last pre', 'underlay pre', 'underlay broken pre',
  'underlay unbroken and first pre', 'underlay middle and last pre',
  'underlay unbroken and last pre'
  'finish unbroken pre', 'finish first pre', 'finish middle pre',
  'finish last pre', 'finish pre', 'finish broken pre',
  'finish unbroken and first pre', 'finish middle and last pre',
  'finish unbroken and last pre'
  'overlay unbroken and last app', 'overlay unbroken and last pre'
- library 'theorems':
  * new options:
  'description color', 'description font', 'description formatter'

version 3.01 (2014/05/13)
- bug fix: 'parbox=false' plus 'breakable' had an unwanted indent
- compatibility fix for tabularx 2014/04/22 v2.09

version 3.02 (2014/05/13)
- compatibility fix for tabularx 2014/04/22 v2.09 (again)

version 3.03 (2014/05/16)
- bug fix: some initialization option keys for \newtcblisting did not operate correctly
- bug fix: boxed title shape 'title' was unknown in underlays
- more boxed title example documented

version 3.04 (2014/05/18)
- compatibility fix for tabularx removed; compatible with tabularx 2014/05/13 v2.10
- boxed title improvements:
  * the 'title' node is accessible now from inside 'frame code' and 'interior code'
  * new keys 'underlay boxed title', 'no underlay boxed title', 'underlay boxed title pre'
  * documentation example updated

version 3.05 (2014/05/28)
- compatibility fix for the upcoming version 2.0 of the package minted
- inner boxes are enforced to be unbreakable now
- library 'breakable':
  new key 'enforce breakable' (for breaking inner boxed deliberately)
- library 'skins':
  * new options:
  'lifted shadow', 'drop small lifted shadow', 'drop lifted shadow', 'drop large lifted shadow'

version 3.10 (2014/07/23)
- box breaking algorithm revised:
  * breakable boxes now always have \noindent
  * distance to preceeding text corrected
  * interaction with floating objects fixed
  * dimensioning of partial boxes improved
  * splitting of an empty closing frame can now be avoided (depending on 'pad at break*')
  * The upper total height limit for breakable boxes is extended from
    about 16384pt to about 65536pt
  * experimental code added (breakable=unlimited) for breakable boxes
    without height limit besides memory
  * splitting boxes inside multicols environments supported (to a certain degree)
  * limited orphan control added ('enlargepage flexible')
- library 'breakable':
  * new options:
  'break at', 'height fixed for', 'enlargepage flexible',
  'pad before break*', 'pad at break*'
- Corners can be set individually now to be 'rounded' or 'sharp'
  for all types of boxes, skins, borders, and shadows:
  * new options:  'sharpish corners', 'sharp corners', and 'rounded corners'
- library 'skins':
  * new macros: '\tcbline*'
  * bug fix: skin families 'bicolor' and 'beamer' did not respect 'colbacktitle'
- pictures 'blueshade.png', 'crinklepaper.png', 'goldshade.png', 'pink_marble.png'
  moved to package folder

version 3.11 (2014/07/25)
- regresssion: vertical space at end of breakable boxes was not removed
- example file updated with new features

version 3.12 (2014/07/29)
- text color implementation changed to circumvent xelatex color problems
- multicol vs. twocolumn detection fixed
- code for breakable boxes without height limit improved
- before box \noindent is replaced by \parindent=0pt (bidi package compatibilty)
- library 'breakable':
  * new option: 'vfill before first'

version 3.20 (2014/09/22)
- bug fix: titles set with 'detach' or 'boxed title' options were not considered
    for lists of tcolorboxes.
- bug fix: 'extrude left by', 'extrude right by' worked only for '\tcbox' but not for 'tcolorbox'
- bug fix: 'pad before break*' and 'pad at break*' were always setting to 0pt
- new options: 'every float', 'list text', 'overlay first and middle',
  'height fill'
- new initialization options:
  'use counter*', 'blend into'
- library 'skins':
  * new macros: '\tcbsettowidthofnode', '\tcbsetmacrotowidthofnode',
    '\tcbsettoheightofnode', '\tcbsetmacrotoheightofnode'
  * new options: 'underlay first and middle', 'finish first and middle'
- library 'hooks':
  * new options: 'underlay first and middle pre',
    'overlay first and middle app', 'overlay first and middle pre',
    'finish first and middle pre'
- library 'documentation':
  * new macros: '\tcbdocmarginnote', '\tcbdocnew', '\tcbdocupdated'
  * The 'docKey' and 'docKey*' environments take tcolorbox options now
  * new options:
    'doclang/new', 'doclang/updated',
    'doc marginnote', 'doc updated', 'doc new', 'doc new and updated'

version 3.21 (2014/10/10)
- bug fix: empty key path handling inside the 'docKey' and 'docKey*' environments was faulty
- bug fix: wrong coloring for '\docAuxCommand' and '\docAuxCommand*'
- bug fix: draft mode for inner boxes deactivated in v3.20
- subtitles added
- new macros:
  '\tcbsubtitle'
- new options:
  'subtitle style', 'before skip', 'after skip', 'beforeafter skip',
- library 'documentation':
  implementation of handling macro and key names changed to accept underscores
  several internal implementation changes

version 3.22 (2014/10/31)
- new macro: '\tcolorboxenvironment'
- new options:
  'text width', 'text height'
- library 'skins':
  * new options: 'borderline north', 'borderline south',
    'borderline east', 'borderline west', 'borderline horizontal', 'borderline vertical'
- library 'breakable':
  * internal change for compatibility with the 'perpage' option of the 'footmisc' package
- library 'theorems':
  * compatibility fix: The 'ams equation' options left too much vertical
    space for the 'fleqn' case
- library 'fitting':
  * new 'fit algorithm' settings: 'fontsize*', 'areasize*', 'hybrid*'

version 3.30 (2014/11/17)
- bug fix: compilation errors using colors like 'red!10' in some skins like 'beamer'
- '\thetcbcounter' can now be used as part of a 'listing file' name for 'tcblisting'
- implementation of 'before skip' and 'after skip' improved
- implementation of 'equal height group' improved to take arbitrary id's
- Quick Reference added
- new options:
  'add to width', 'add to height',
  'box align', 'left skip', 'right skip', 'leftright skip'
- library 'skins':
  * new macros:
  '\tcbincludegraphics', '\tcbincludepdf'
  * new options:
  'graphics options', 'graphics directory', 'graphics pages'
- library 'listings', 'listingsut8', 'minted':
  * 'listing file' now usable inside 'tcblisting' and 'tcbinputlisting'
  * new options:
  'comment only', 'text above* listing', 'listing above* text',
  'comment above* listing', 'listing above* comment',
  'comment style', 'tcbimage comment', 'pdf extension', 'pdf comment',
  'process code', 'no process', 'run system command', 'run pdflatex',
  'run xelatex', 'run lualatex', 'run makeindex', 'run bibtex', 'run biber',
  'run arara', 'run latex', 'run dvips', 'run ps2pdf',
  'compilable listing'
- new library 'raster':
  * new macros and environments:
  'tcbraster', 'tcbitemize', 'tcbitem'
  * new options:
  'raster columns', 'raster rows', 'raster width', 'raster height', 'raster before skip',
  'raster after skip', 'raster left skip', 'raster right skip', 'raster column skip',
  'raster row skip', 'raster halign', 'raster valign', 'raster equal height',
  'raster equal height group', 'raster force size' ,'raster reset',
  'raster odd column', 'raster even column', 'raster column n', 'raster odd row',
  'raster even row', 'raster row m','raster odd number', 'raster even number',
  'raster row m column n', 'raster number n'

version 3.31 (2014/11/28)
- new macros: '\tcbstartrecording', '\tcbrecord', '\tcbstoprecording', '\tcbinputrecords'
- new options: 'squeezed title', 'squeezed title*', 'phantomlabel',
  'record', 'no recording'
- 'savelowerto' changed to need only one run instead of two
- library 'skins':
  * '\imagename' macro can be used in more situations
  * '\tcbincludegraphics' made aware of 'grffile' package
- new library 'raster':
  * tcbraster safeguarded against restricted horizontal mode
  * new option: 'raster every box'

version 3.32 (2014/12/01)
- bug fix for 'crefname' and 'Crefname' options (cleveref support)

version 3.33 (2014/12/11)
- The nobreak settings after a heading are respected now for breakable and
  unbreakable boxes. Use the new option 'ignore nobreak' to restore the old
  behavior.
- vertical skip of two successive tcbraster environments fixed

version 3.34 (2014/12/16)
- 'height fill' now fills gapless and can be overruled by other height options
- 'before skip' and 'after skip' accept glue values now
- library 'breakable':
  * new option 'compress page':
    Use the new option 'compress page=none' to restore the old behavior.
- library 'raster':
  * 'raster before skip' and 'raster after skip' accept glue values now

version 3.35 (2015/01/07)
- fix: 'tcbdocumentation.code.tex' changed to US-ASCII
- text color implementation changed to fix some color problems
- new options: 'upperbox', 'visible', 'invisible'
- documentation complemented

version 3.36 (2015/01/09)
- bug fix: dimension settings with 'em' or 'ex' units were sometimes converted to 0pt
- bug fix: 'boxed title' options and some algorithms of the 'fitting' library were not compatible
- bug fix: 'fit width from' ('fitting' library) may have updated counter too often
- new option: 'only'
- library 'fitting': fit process can now also includes the title
- library 'raster': new option 'raster equal skip'
- library 'documentation':
  * new macros and environments:
    '\docCounter', '\docCounter*', '\docLength', '\docLength*'
  * new options:
    'index command', 'index command name' (for imakeidx),
    'color counter', 'color length',
    'doclang/counter', 'doclang/counters', 'doclang/length', 'doclang/lengths'

version 3.40 (2015/01/14)
- bug fix: list environments had too much leading space if set as first elements in a box
- library 'skins':
  * new option: 'titlerule style'
- library 'breakable':
  algorithm for handling overfull boxes revised; new warnings implemented

version 3.50 (2015/03/16)
- bug fix: \tcbline was broken for \tcboxfit-boxes since 3.36
- text color implementation changed to fix some color problems
- before/after settings changed to detect special situations
- 'sidebyside align': new selections 'top seam', 'center seam', 'bottom seam'
- new options:
  'force nobeforeafter', 'blend before title', 'blend before title code'
- library 'documentation':
  'before example', 'after example' are deprecated; 'docexample' is changed
- new library 'external'
  * new macros and environments:
    'tcbexternal', '\tcbEXTERNALIZE', 'extikzpicture', 'extcolorbox',
    '\tcbifexternal',
    '\newtcbexternalizeenvironment', 'renewtcbexternalizeenvironment',
    'newtcbexternalizetcolorbox', 'renewtcbexternalizetcolorbox'
  * new options:
    'runner', 'externalize', 'force remake', '!',
    'name', 'externalize listing', 'externalize listing!',
    'externalize example', 'externalize example!',
    'prefix', 'environment', 'minipage', 'plain', 'compiler', 'runs',
    'input source on error', 'safety', 'preamble'
- documentation structure revised

version 3.60 (2015/05/07)
- bug fix: dimension settings with 'em' or 'ex' units for 'enlarge .. by' converted to 0pt
- bug fix: 'bicolor' skin sometimes ignored color for lower part when broken
- new macros: '\tcbpatcharcangular', '\tcbpatcharcround'
- implementation of text alignment changed with new options:
  'halign', 'halign upper', 'halign lower', 'halign title', 'valign upper'
- new options:
  'saveto', 'circular arc', 'bean arc', 'arc is angular', 'arc is curved',
  'square', 'tcbox width'
- library 'skins':
  * new option: 'smart shadow arc'
- library 'documentation':
  package 'doc' removed from list of required packages
- library 'external':
  * new options:
    'environment with percent', 'preamble tcbset', 'preclass', 'clear preclass',
    'PassOptionsToPackage', 'PassOptionsToClass'

version 3.61 (2015/06/12)
- bug fix: nobreak settings after a heading were sometimes ignored depending
  on the box content
- library 'external':
  * now throws an error if the same external job name is used twice
  * new option: '-'
- documentation bug fixes

version 3.70 (2015/07/16)
- bug fix: 'attach title to upper' attached also empty titles
- bug fix: library 'raster': blank line after tcbitemize or tcbraster could give an error message
- new options:
  'text fill', 'valign scale bound',
  'valign=scale', 'valigns=scale*', 'valign lower=scale', 'valign lower=scale*'
- library 'breakable':
  * Settings for broken box parts are now shielded by TeX grouping. This may
    break code which used side-effects with unproper skins.
  * new options:
    'extras unbroken', 'extras first', 'extras middle', 'extras last',
    'extras', 'extras broken', 'extras unbroken and first',
    'extras unbroken and last', 'extras middle and last',
    'extras first and middle', 'no extras unbroken', 'no extras first',
    'no extras middle', 'no extras last', 'no extras',
- library 'hooks':
  * new options:
    'extras unbroken pre', 'extras first pre', 'extras middle pre',
    'extras last pre', 'extras pre', 'extras broken pre',
    'extras unbroken and first pre', 'extras unbroken and last pre',
    'extras middle and last pre', 'extras first and middle pre',
- new library 'magazine'
  * new macros and environments:
    '\newboxarray', '\boxarraygetsize', '\boxarrayreset', '\boxarrayclear',
    '\boxarraygetbox', '\boxarraygetwidth', '\boxarraygetheight', '\boxarraygetdepth',
    '\boxarraygettotalheight', '\useboxarray', '\usetcboxarray',
    '\consumeboxarray', '\consumetcboxarray', 'boxarraystore',
  * new options:
    'store to box array', 'reset box array', 'do not store to box array',
    'reset and store to box array'

version 3.71 (2015/07/23)
- bug fix: An error introduced in 3.70 broke all code without 'breakable' library
- bug fix: library 'external': spurious blank in source input removed
- documentation extended

version 3.72 (2015/08/12)
- bug fix: bounding box changes and boxed title additions were not considered
    correctly by 'height fixed for' or 'height fill' (resulting in wrong page breaks)
- library loading made compatible with expl3
- cosmetic documentation changes

version 3.73 (2015/10/16)
- bug fix: '\tcbdocmarginnote' had a spurious blank.
- parbox=false settings adapted for embedded lists
- library 'documentation':
  * new options:
  'before doc body command', 'after doc body command',
  'before doc body environment', 'after doc body environment',
  'before doc body key', 'after doc body key',
  'before doc body', 'after doc body'

version 3.80 (2015/11/27)
- superfluous and sometimes troublesome \unskip's were removed.
  Note that this changed the behavior of 'after upper' and 'after lower'.
  Some user code may need to apply the new 'after upper*' / 'after lower*'
  options or insert an \unskip.
- even/odd page testing completely rewritten.
- some difference formulas were revised.
- new macros:
  '\thetcolorboxnumber', '\thetcolorboxpage',
  '\tcbifoddpage', '\tcbheightfromgroup'
- new options:
  'after upper*', 'after lower*',
  'center', 'flush right', 'flush left',
  'if odd page', 'if odd page*',
  'use height from group'
- library 'xparse':
  * new macro:    '\tcbsidebyside'
  * new options:  'sidebyside adapt', 'sidebyside switch'

version 3.90 (2016/02/29)
- bug fix: 'height fill' after headings (nobreak) produced an error
- implementation for 'before' and 'before skip' changed to avoid spacing
  problems when there is a page break before breakable/unbreakable boxes
- the 'height fill' option can be applied also for boxed inside a tcbraster
- new options:
  'add to natural height', 'space to', 'use height from group' (new default)
- new macros:
  '\tcbheightspace', '\tcbtextwidth', '\tcbtextheight'
- library 'skins':
  * 'halign title' works with 'boxed title' now
  * 'boxed title style' changed to be stackable
  * better support for titles at the bottom of the box
  * new skin: 'tile'
  * new options:
    'blankest', 'tile', 'no boxed title style', 'boxed title size',
    'attach boxed title to bottom', 'attach boxed title to bottom*',
    'attach boxed title to top', 'attach boxed title to top*',
    'flip title'
- library 'raster':
  * new environment:
    'tcboxedraster'
  * new options:
    'raster multicolumn', 'raster multirow'
- library 'documentation':
  removal of some unwanted blanks

version 3.91 (2016/04/27)
- bug fix: '\tcbline' was indented when setting '\parindent' inside a box
- bug fix: 'minimum for equal height group' changed current equal height group
    and settings with 'em' or 'ex' units were converted to 0pt
- bug fix: setting '-output-directory' and 'outputdir=' for the minted package
    broke \tcblisting for 'listing engine=minted'
- documentation: biber problem with latin1 encoding circumvented
- new options:
  'minimum for current equal height group'
- library 'theorems':
  * new option: 'label separator'
- new library 'vignette' for ornamental frames:
  * new fadings: 'semi west', 'semi east', 'semi north', 'semi south'
  * new macros: '\tcbvignette'
  * new options:
    'xmin', 'xmax', 'ymin', 'ymax',
    'lower left corner', 'upper right corner', 'inside node', 'outside node',
    'over node', 'over node offset', 'north size', 'south size', 'east size',
    'west size', 'size', 'north style', 'south style', 'east style', 'west style',
    'draw method', 'fade out', 'semi fade out', 'fade in', 'semi fade in',
    'base color', 'raised color', 'lowered color',
    'underlay vignette', 'underlay raised fading vignette',
    'underlay raised shading vignette', 'underlay shade in vignette',
    'finish vignette', 'finish raised fading vignette', 'finish fading vignette'
- library 'raster':
  * new environment: 'tcboxeditemize'

version 3.92 (2016/05/28)
- bug fix: 'compilable listing' used no '.tex' extension causing problems with minted
- compatibility patch for \vsplit in luatex 0.95 causing problems with breakable boxes
- settings inside \tcbvignette are now inside a group
- library 'vignette': new option 'scope'

version 3.93 (2016/06/01)
- bug fix: compatibility patch for \vsplit in luatex 0.95 was buggy
- system commands are now accessed using the 'shellesc' package for
  compatibility with luatex

version 3.94 (2016/07/14)
- bug fix: '\tcbincludegraphics' for fixed height boxes was broken since v3.90 (2016/02/29)
- new option 'nameref'
- library 'theorems':
  Theorems made nameref-aware
- library 'listings':
  * new options:
  'freeze file', 'freeze none', 'freeze extension',
  'freeze pdf', 'freeze png', 'freeze jpg'
- library 'external':
  * implementation improved for lualatex and xelatex
  * new macro '\tcbiffileprocess'

version 3.95 (2016/10/21)
- The behaviors of 'after upper' and 'after lower' are reverted back to
  prior version 3.80 to have an automatic \unskip inserted.
  Therefore, 'after upper*' and 'after lower*' are deprecated now.
- new option 'void'
- library 'skins':
  '\tcbincludegraphics' made compatible with 'height fill' boxes.
- library 'minted':
  now, included source files are searched for in relation to an optional
  'output-directory' and also locally.
- library 'documentation':
  Language settings are not longer reset to English for embedded boxes.

version 3.96 (2016/11/18)
- bug fix: unprotected definition of the 'nameref' option induced serious errors
- bug fix: nameref package was not detected if loaded after tcolorbox
- new macros:
  '\tcbifoddpageoroneside'
- new options:
  'if odd page or oneside', 'if odd page or oneside*',
- library 'documentation':
  * Documentation options are not longer reset to default values for embedded
    boxes. User code may be affected by this change.
  * marginnotes adapt to twosided documents now

version 4.00 (2017/02/16)
- Code adaptions to support \parfillskip changing packages like KOMA-Script:
  'parskip', 'noparskip', 'after skip', 'breakable', 'raster'
- 'toggle left and right' toggles corners now
- new options:
  'left*', 'right*',
  'spread inwards', 'spread outwards', 'move upwards', 'move upwards*', 'fill downwards',
  'spread sidewards', 'spread upwards', 'spread upwards*', 'spread downwards', 'spread',
  'hypertarget', 'bookmark', 'bookmark*'
- library 'skins':
  * new macro '\tcbhypernode'
  * new options:
  'hyperref', 'hyperref node', 'hyperref interior', 'hyperref title',
  'hyperlink', 'hyperlink node', 'hyperlink interior', 'hyperlink title',
  'hyperurl', 'hyperurl node', 'hyperurl interior', 'hyperurl title',
  'hyperurl*', 'hyperurl* node', 'hyperurl* interior', 'hyperurl* title'

version 4.01 (2017/02/19)
- bug fix: 'raster halign=center' was broken by 4.00 code changes

version 4.02 (2017/02/24)
- Further code adaptions to support \parfillskip changing packages like KOMA-Script
  and to respect center environments
  'parskip', 'noparskip', 'after skip', 'breakable', 'raster'
- new option: 'parfillskip restore'
- bug fix: 'segmentation style' was not applied correctly to breakable boxes with
  'bicolor' skin
- bug fix: '/tcb/external/!' and '/tcb/external/-' were not usable inside \tcbset
- documentation optimizations

version 4.03 (2017/04/25)
- Implementation of 'raster equal height' changed to be more robust e.g. for loops
- Implementation of several fill options like 'fill stretch image' changed
  to be more efficient and to be independent from TikZ node positioning options.
- Bug fix: 'fill plain image' and 'fill plain picture' ignored 'fill image opacity'.
- new macro: '\tcbsegmentstate'
- library 'breakable':
  * new option: 'segmentation at break'
- library 'documentation':
  * new options: 'documentation minted language', 'keywords bold'
- Creation of leaflets documented

version 4.10 (2017/07/05)
- new options:
  'inherit height', 'verbatim ignore percent'
- library 'skins'
  * new style 'enhanced standard jigsaw'
- library 'magazine':
  * new macro: '\ifboxarrayempty'
- library 'breakable':
  * option 'break at' allows negative values now.
  * the algorithm for breaks inside a multicolumn environment was improved
    (user code may be affected by this change).
  * new macro: '\tcbbreak'
- library 'minted':
  * the default settings for 'minted options'
    are supplemented by 'breaklines,autogobble'
- new library 'poster'
  * new macros and environments:
    'tcbposter',  '\tcbposterset', '\posterbox', 'posterboxenv',
    'tcbposterwidth', 'tcbposterheight', 'tcbpostercolspacing', 'tcbposterrowspacing',
    'tcbpostercolumns', 'tcbposterrows', 'tcbpostercolwidth', 'tcbposterrowheight'
  * new options:
    'poster', 'columns', 'rows', 'colspacing', 'rowspacing', 'spacing',
    'showframe', 'width', 'height', 'prefix', 'coverage', 'no coverage',
    'boxes', 'fontsize', 'name', 'column', 'column*', 'span', 'row', 'rowspan',
    'fixed height', 'below', 'above', 'at', 'between', 'sequence',
    'placeholder', 'xshift', 'yshift'
- New example file 'tcolorbox-example-poster'
- New tutorial 'tcolorbox-tutorial-poster' for poster creation

version 4.11 (2017/09/14)
- Standard internal minipage settings changed from 'c' to 'b' which should
  fix some glitches

version 4.12 (2018/01/12)
- color implementation changed to fix problems with expl3 (thanks to Ulrike Fischer)
- Documentation typo corrected ('tcbsetmanagedlayers' instead of 'tcbsetmanagedlayer')
- Bug fix: 'borderline south' and 'borderline north' created 'Missing character'
  messages for breakable boxes
- library 'theorems':
  * new options 'theorem label supplement', 'theorem full label supplement'

version 4.13 (2018/03/22)
- typos in 'tcolorbox-tutorial-poster' corrected
- new options:
  'grow sidewards by'
- library 'breakable':
  * Warning for discarded zero height box content added
- library 'listings':
  * Documentation for 'text side listing', 'listing side text',
    'comment side listing', 'listing side comment' supplemented with notes.
- library 'skins':
  * Options given by '/tcb/graphics options' and '/tikz/fill image options'
    are now fully expanded while applied to underlying '\includegraphics'
  * new option:
    'graphics orientation'

version 4.14 (2018/07/26)
- bug fix (#40): 'tikz lower' and 'tikz upper' failed to take more than one parameter
- '\tcblistof' issues a warning if tocdepth is lower than 1 (#42)
- macro definition of \tcolorbox@label removed from aux file (#47)
- documentation adapted to the changed argument collection of the xparse package (#43)
- new options: 'index', 'index*'
- library 'breakable':
  * (#41) 'title after break' inherits the title alignment now
    (may change output of existing documents!)
  * new options 'extras title after break', 'no extras title after break'

version 4.15 (2018/12/07)
- bug fix (#40): 'tikz upper', 'tikz lower' failed to take more than one parameter (again)
- bug fix: 'tcboxedraster' could not be set to be 'breakable'
- library 'breakable': Implementation of 'pad after break' changed to be
  consistent with a boxed title.
- library 'raster':
  * dimension settings changed to be more robust
  * new options (#52) 'raster width center', 'raster width flush left', 'raster width flush right'
- Example source code of 'tcolorbox-example-poster' and 'tcolorbox-tutorial-poster'
  adapted to be compatible with lipsum package version 2.0

version 4.20 (2019/03/02)
- bug fix (#60): \multicolumn could not be used for first cell with option 'tabularx'
- internal colors names renamend and offially documented (Section 9.5 Color Names):
  'tcbcolframe', 'tcbcolback', 'tcbcolbacktitle', 'tcbcolbacklower',
  'tcbcolupper', 'tcbcollower', 'tcbcoltitle'
- listingsutf8 compatability better documented (#58)
- semantic changed for options: 'after upper*', 'after lower*'
- new options: 'before upper*', 'before lower*', 'titlebox', 'nirvana'
- library 'skins':
  * new options: 'beamer hidden', 'beamer alerted', 'hide', 'alert'
  * option 'only' moved from package to skins library
- new documentation section '13 Beamer Support'

version 4.21 (2019/09/19)
- bug fix (#71): 'shield externalize' should be effective on all tcolorbox layers
- bug fix (#76): 'spread inwards', 'spread outwards', 'spread sidewards' gave
  wrong results for some document geometry settings
- new options (#75): 'tabulars', 'tabulars*'
- library 'extras':
  * bug fix: all 'extras ...' options from library 'hooks' took code instead of options
  * new options (#73): 'minted options app', 'minted options pre',
      'listing options app', 'listing options pre'
- library 'xparse':
  * bug fix: options 'IfNoValueTF', 'IfValueTF', 'IfBooleanTF' failed
      to recognize arguments in some code line breaks situations
- library 'documentation':
  TikZ path operation documentation (#65):
  * new color name: 'Fade'
  * new macros and environments: '\colFade', 'docPathOperation',
      '\refPathOperation', '\refPathOperation*'
  * new options: 'color fade', 'color path', 'doc label', 'doc head path',
      'before doc body path', 'after doc body path'
  * new language string: 'path', 'paths'
- documentation: checkerbox for opacity examples was too dark

version 4.22 (2019/11/15)
- bug fix (#79) in library 'xparse':
  'sidebyside adapt' did not respect color, font, and other options.
- bug fix (#85) in library 'raster':
  'raster before skip' and 'raster after skip' did not accept glue anymore.
- new initialization option (#80): 'reset counter on overlays'

version 4.30 (2020/04/28)
- bug fix (#88): 'parskip' and 'noparskip' had side-effects for the box content
                 in combination with 'height fill' and 'parbox=false'
- bug fix (#90) in library 'documentation':
  initialize 'doc description' for every docXXX to be empty
- Internal box counter renamed to remove warnings when using \includeonly
- library 'documentation':
  * major code overhaul to support simultaneous documentation of
    similar commands, environments, keys, path operations (#89).
  * Note that the new code reserves a small additional amount of vertical space
    for documented macros which may result in changed page breaks.
  * Note that documentation heads are now embedded inside a 'raster'
    which requires other customizations for vertical space (if needed)
  * new macros and environments: 'docCommands', 'docEnvironments',
      'docKeys', '\tcbmakedocSubKeys', 'docPathOperations'
  * new options: 'doc index' (#91), 'doc name', 'doc parameter',
      'doc keypath', 'doc sort index', 'doc no index',
      'doc raster command', 'doc raster environment', 'doc raster key',
      'doc raster path', 'doc raster'
  * additional option setting for: '\docAuxCommand', '\docAuxEnvironment',
      '\docAuxKey', '\docValue', '\docColor', '\docCounter', '\docLength'
  * superfluous and undocumented opton 'color frame' removed (#94)
  * '\refAux' and '\refAuxcs' are not longer colored, if colorlinks=false (#95)
- library 'listingsutf8':
  safeguard against compiling with other engines than pdf(la)tex (#92)
- library 'fitting':
  '\tcbfitdim' is described in more detail (#96)
- library 'poster':
  poster width and height caveats described in more detail (#98)



==> tcbbreakable.code.tex <==
%% The LaTeX package tcolorbox - version 4.30 (2020/04/28)
%% tcbbreakable.code.tex: Code for breakable colorboxes
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2020 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{4.30}

\let\tcb@parboxrestore@true=\tcb@parboxrestore
\let\tcb@parboxrestore@false\tcb@parbox@false@settings

% total height for boxes smaller than 0.4375\maxdimen and 0.4375\maxdimen else (ca 2.5m)
\def\tcb@defToTotalHeightBreakable#1#2{%
  \ifnum\ht#2<0 %
    \edef#1{7168pt}%
  \else\ifnum\ht#2<469762048 %
    \tcbdimto#1{\ht#2+\dp#2}%
  \else%
    \edef#1{7168pt}%
  \fi\fi%
}

\newbox\tcb@testbox

% for oversized boxes height is detected as \textheight or larger
\def\tcb@defToTotalHeightUnlimited#1#2{%
  \tcb@defToTotalHeightBreakable#1#2%
  \ifdim\dimexpr#1<\textheight\relax%
    \edef\tcb@thevfuzz{\the\vfuzz}%
    \edef\tcb@thevbadness{\the\vbadness}%
    \vfuzz=\maxdimen\vbadness=10000%
    \splittopskip=0pt%
    \splitmaxdepth=0pt%
    \savingvdiscards=1%
    \setbox\tcb@testbox=\vsplit#2 to \textheight%
    \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz%
    \ifdim\wd#2=0pt\relax%
      \tcb@swap{#2}{\tcb@testbox}%
      \tcbdimto#1{\ht#2+\dp#2}%
    \else%
      \setbox#2=\vbox{%
        \unvbox\tcb@testbox%
        \splitdiscards%
        \unvbox#2}%
      \edef#1{7168pt}%
    \fi%
    \savingvdiscards=0%
  \fi%
}

\def\tcb@@break{\par\xleaders\vbox{\rule{0pt}{2\textheight}}\vskip 2\textheight\par}

\def\tcb@vbox#1#2{%
  \edef\reserved@a{%
    \endgroup%
    \setbox#1\vbox{\hsize=#2%
      \begingroup\aftergroup}%
      \def\noexpand\@currenvir{\@currenvir}%
      \def\noexpand\@currenvline{\on@line}}%
  \reserved@a%
  \@endpefalse%
  \let\tcbbreak\tcb@@break%
  \color@begingroup%
  \textwidth\hsize%
  \columnwidth\hsize%
  \csname tcb@parboxrestore@\kvtcb@parbox\endcsname%
  \def\@mpfn{mpfootnote}%
  \def\thempfn{\thempfootnote}%
  \c@mpfootnote\z@%
  \let\@footnotetext\@mpfootnotetext%
  \let\@listdepth\@mplistdepth \@mplistdepth\z@%
  \@setminipage\tcb@hyph@fix%
  \let\tcb@drawcolorbox\tcb@drawcolorbox@standalone%
  \let\FN@pp@footnote\@empty% disable perpage mode of 'footmisc' package
  \ignorespaces%
}

\def\endtcb@vbox{%
  \par%
  \unskip%
  \ifvoid\@mpfootins\else%
    \vskip\skip\@mpfootins%
    \normalcolor%
    \footnoterule%
    \unvbox\@mpfootins%
  \fi%
  \@minipagefalse%
  \color@endgroup}

% remaining height
\def\tcb@comp@h@page{%
  \tcb@breakat@next%
  \ifdim\tcb@breakat@dim>0pt\relax%
    \tcbdimto\tcb@h@page{\tcb@breakat@dim-\kvtcb@shrinkbreakgoal}%
  \else%
    \ifx\kvtcb@float\@empty%
      \iftcb@multicol%
        \ifnum\c@tcbbreakpart>1\relax%
          \tcbdimto\tcb@h@page{\@colroom}%
        \else%
          \ifdim\pagegoal=16383.99998pt
            \tcbdimto\tcb@h@page{\@colroom}%
          \else%
            \@tempdima\pagetotal%
            \@whiledim \@tempdima>\@colroom \do{\advance\@tempdima-\@colroom}%
            \tcbdimto\tcb@h@page{\@colroom-\@tempdima}%
          \fi%
        \fi%
      \else%
        \ifdim\pagegoal=16383.99998pt
          \tcbdimto\tcb@h@page{\vsize}% detects floating objects
        \else%
          \tcb@comp@compress%
          \tcbdimto\tcb@h@page{\pagegoal-\pagetotal+\tcb@compress@height}%
        \fi%
      \fi%
    \else%
      \tcbdimto\tcb@h@page{\textheight}%
    \fi%
    \tcbdimto\tcb@h@page{\tcb@h@page+\tcb@breakat@dim-\kvtcb@shrinkbreakgoal}%
  \fi%
}

\def\tcb@comp@h@total@standalone{%
  \tcbdimto\tcb@h@padding{\kvtcb@bbtop@stand+\kvtcb@bbbottom@stand+\kvtcb@top@rule@stand+\kvtcb@bottom@rule@stand+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom}%
  \tcbdimto\tcb@h@total{\tcb@h@padding+\tcb@h@padtitle+\tcb@h@upper+\tcb@h@segment+\tcb@h@lower}%
}


\newif\iftcb@final@box

\def\tcb@check@for@final@box{%
  \ifdim\tcb@h@total>\tcb@h@page\relax%
    \iftcb@multicol%
      \tcb@final@boxfalse%
    \else%
      \ifdim\tcb@h@total>\dimexpr\tcb@h@page+\kvtcb@enlargepage@flex\relax%
        \tcb@final@boxfalse%
      \else%
        \tcbdimto\tcb@temp{\tcb@h@total-\tcb@h@page}%
        \enlargethispage*{\tcb@temp}%
        \tcbdimto\tcb@h@page{\tcb@h@page+\tcb@temp}%
        \tcb@final@boxtrue%
      \fi%
    \fi%
  \else%
    \tcb@final@boxtrue%
  \fi%
}

\def\tcb@following@title{%
  \ifx\kvtcb@followingtitle\@empty%
    \tcb@hasTitlefalse%
    \let\tcb@h@title=\tcb@zpt%
    \let\tcb@h@padtitle=\tcb@zpt%
  \else%
    \tcb@hasTitletrue%
    \tcbdimto\tcb@w@title{\tcb@innerwidth-\kvtcb@boxsep*2-\kvtcb@lefttitle-\kvtcb@righttitle}%
    \begin{tcb@savebox}{\tcb@titlebox}{\tcb@w@title}\tcb@extras@followingtitle\color{tcbcoltitle}\kvtcb@fonttitle\kvtcb@haligntitle\kvtcb@followingtitle\end{tcb@savebox}%
    \tcbdimto\tcb@h@title{\ht\tcb@titlebox+\dp\tcb@titlebox}%
    \tcbdimto\tcb@h@padtitle{\kvtcb@title@rule+\kvtcb@boxsep*2+\kvtcb@toptitle+\kvtcb@bottomtitle+\tcb@h@title}%
  \fi%
}

\newbox\tcb@totalupperbox
\newbox\tcb@totallowerbox
\newif\iftcb@break@allowed

\def\tcb@enlbreak@next@final{%
  \ifdim\dimexpr\tcb@enlbreak@dim=0pt\relax
  \else%
    \iftcb@multicol\else\enlargethispage{\tcb@enlbreak@dim}\fi%
  \fi%
}

\def\tcb@enlbreak@next@scan#1/#2@{%
  \def\temp@a{#2}%
  \tcbdimto\tcb@enlbreak@dim{#1}%
  \ifx\temp@a\@empty%
    \let\tcb@enlbreak@next=\tcb@enlbreak@next@final%
  \else%
     \edef\tcb@enlbreak@seq{\temp@a @}%
  \fi%
  \tcb@enlbreak@next@final%
}

\def\tcb@enlbreak@next@step{%
  \edef\tcb@temp{\noexpand\tcb@enlbreak@next@scan\tcb@enlbreak@seq}%
  \tcb@temp%
}

\def\tcb@enlbreak@init{%
  \edef\tcb@enlbreak@seq{\kvtcb@enlargepage/@}%
  \let\tcb@enlbreak@next=\tcb@enlbreak@next@step%
  \tcb@enlbreak@next%
}


\def\tcb@breakat@next@scan#1/#2@{%
  \def\temp@a{#2}%
  \tcbdimto\tcb@breakat@dim{#1}%
  \ifx\temp@a\@empty%
    \let\tcb@breakat@next=\@empty%
  \else%
     \edef\tcb@breakat@seq{\temp@a @}%
  \fi%
}

\def\tcb@breakat@next@step{%
  \edef\tcb@temp{\noexpand\tcb@breakat@next@scan\tcb@breakat@seq}%
  \tcb@temp%
}

\def\tcb@breakat@init{%
  \edef\tcb@breakat@seq{\kvtcb@breakatdim/@}%
  \let\tcb@breakat@next=\tcb@breakat@next@step%
}


\newif\iftcb@multicol
\newif\iftcb@vfillbeforefirst

\def\tcb@do@nobreak@warning{%
  \iftcb@ignorenobreak%
    \tcb@warning{Using nobreak failed. You should set `ignore nobreak=false' to avoid this}%
  \else%
    \tcb@warning{Using nobreak failed. Try to enlarge `lines before break' or set page breaks manually}%
  \fi%
}

\def\tcb@handle@nobreak{%
  \tcb@enlbreak@init%
  \tcb@breakat@init%
  \tcb@comp@h@page%
  \tcbdimto\tcb@h@page{\tcb@h@page-1.5\baselineskip-\parskip-\lineskip}% security surcharge
  \tcb@comp@h@total@standalone%
  \tcb@check@for@final@box%
  \iftcb@final@box%
  \else%
    \ifdim\dimexpr\tcb@h@page-\tcb@h@padding-\tcb@h@padtitle<\kvtcb@breakminlines\baselineskip\relax%
      \tcbdimto\tcb@h@page{\tcb@h@page+3.5\baselineskip+\parskip+\lineskip}%
      \vspace{\tcb@h@page}%
      {\parskip\z@\nointerlineskip\noindent}%
      \vspace{-\tcb@h@page}%
      \par%
    \fi%
  \fi%
}

\def\tcb@prepare@break@operation{%
  \setcounter{tcbbreakpart}{0}%
  \let\tcb@nobreak@warning\@empty%
  \@ifundefined{columnbreak}{\tcb@multicolfalse}{%
    \ifnum\doublecol@number>\z@ %
      \tcb@multicoltrue%
    \else%
      \tcb@multicolfalse%
    \fi}%
  \ifx\kvtcb@float\@empty%
    \iftcb@nobreak{%
      \let\tcb@nobreak@warning\tcb@do@nobreak@warning%
      \iftcb@ignorenobreak%
        \kvtcb@beforebox%
      \else%
        \tcb@handle@nobreak%
      \fi%
    }{\kvtcb@beforebox}%
    \def\kvtcb@beforebox{\parskip\z@\nointerlineskip\noindent}%
    \noindent% applies parskip
    \vskip\lineskip{\parskip\z@\par\vskip\z@}\bgroup\@nobreakfalse\addpenalty\z@\egroup% force update vertical list
    \tcb@break@allowedtrue%
    \tcb@enlbreak@init%
  \else%
    \tcb@break@allowedfalse%
  \fi%
}

\def\tcb@height@fill@unbroken#1{%
  \ifnum\c@tcblayer<2\relax%
    \tcb@ignorenobreaktrue%
    \tcb@prepare@break@operation%
    \tcb@breakat@init%
    \tcbset{compress page=#1}%
    \tcb@comp@h@page%
    \tcbset{height=\tcb@h@page-\kvtcb@bbtop@stand-\kvtcb@bbbottom@stand}%
  \fi%
}

\def\tcb@height@fill@unbroken@normal{\tcb@height@fill@unbroken{none}}
\def\tcb@height@fill@unbroken@compressed{\tcb@height@fill@unbroken{all}}

\def\tcb@use@after@lastbox{\bgroup\tcb@after@lastbox\egroup}

\def\tcb@drawcolorbox@breakable{%
  \tcbdimto\kvtcb@topsep{\kvtcb@topsep}%
  \tcb@prepare@break@operation%
  \global\let\tcb@after@lastbox=\kvtcb@afterbox%
  \let\kvtcb@afterbox=\@empty%
  \begingroup%
    \parskip\z@skip%
    \parindent\z@%
    \lineskip\z@skip%
    \topskip\z@skip%
    \tcb@parfillskip@check%
    \tcb@split@start%
  \endgroup%
  \color{.}% hack for some special cases
  \ifx\kvtcb@float\@empty%
    \aftergroup\tcb@use@after@lastbox%
  \fi%
}

\def\tcb@split@pagebreak{%
  \tcb@undo@before%
  \iftcb@multicol\columnbreak\else\pagebreak\fi%
  \tcb@nobreak@warning%
  \tcb@enlbreak@init\tcb@break@allowedfalse%
}

\def\tcb@split@start{%
  \tcb@breakat@init%
  \tcb@comp@h@page%
  % height calculation
  \tcb@comp@h@total@standalone%
  %
  \let\tcb@split@next=\relax%
  \tcb@check@for@final@box%
  \iftcb@final@box%
    \tcb@drawcolorbox@standalone%
  \else%
    \iftcb@break@allowed%
      \ifdim\dimexpr\tcb@h@page-\tcb@h@padding-\tcb@h@padtitle<\kvtcb@breakminlines\baselineskip\relax%
        \tcb@split@pagebreak%
        \tcb@comp@h@page%
        \tcb@check@for@final@box%
        \iftcb@final@box%
          \tcb@drawcolorbox@standalone%
        \else%
          \let\tcb@split@next=\tcb@split@first%
        \fi%
      \else%
        \let\tcb@split@next=\tcb@split@first%
      \fi%
    \else%
      \let\tcb@split@next=\tcb@split@first%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@setbox#1#2#3{%
  \setbox#1=\vbox{\unvbox#3}%
  \ifdim\dimexpr\ht#1+\dp#1>#2\relax%
    %\tcb@warning{Splitted box part too large by \the\dimexpr\ht#1+\dp#1-#2\relax}% switched off (99% useless/annoying)
    \setbox#1=\vbox to\the\dimexpr#2-\dp#1\relax{\unvbox#1}%
  \fi%
}


\def\tcb@setbox@upper#1#2{%
  \tcb@setbox\tcb@upperbox{#1}{#2}%
  \tcbdimto\tcb@h@upper{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcb@vsplit@upper{%
  \setbox\tcb@upperbox=\vsplit\tcb@totalupperbox to\tcb@split@dim%
  \edef\tcb@upper@box@badness{\the\badness}%
}

\def\tcb@split@upper@box@and@assemble{%
  \vfuzz=\maxdimen\vbadness=10000\savingvdiscards=1%
  \tcb@vsplit@upper%
  \ifnum\tcb@upper@box@badness=1000000\relax%
    \setbox\tcb@totalupperbox=\vbox{%
      \unvbox\tcb@upperbox%
      \splitdiscards%
      \unvbox\tcb@totalupperbox}%
  \else%
    \tcb@setbox@upper{\tcb@split@dim}{\tcb@upperbox}%
  \fi%
  \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz\savingvdiscards=0%
}

\def\tcb@split@upper@box{%
  \vfuzz=\maxdimen\vbadness=10000%
  \tcb@vsplit@upper%
  \ifnum\tcb@upper@box@badness=1000000\relax%
    \tcb@warning{The upper box part has become overfull}%
  \fi%
  \tcb@setbox@upper{\tcb@split@dim}{\tcb@upperbox}%
  \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz%
}

\def\tcb@setbox@lower#1#2{%
  \tcb@setbox\tcb@lowerbox{#1}{#2}%
  \tcbdimto\tcb@h@lower{\ht\tcb@lowerbox+\dp\tcb@lowerbox}%
}

\def\tcb@vsplit@lower{%
  \setbox\tcb@lowerbox=\vsplit\tcb@totallowerbox to\tcb@split@dim%
  \edef\tcb@lower@box@badness{\the\badness}%
}

\def\tcb@split@lower@box@and@assemble{%
  \vfuzz=\maxdimen\vbadness=10000\savingvdiscards=1%
  \tcb@vsplit@lower%
  \ifnum\tcb@lower@box@badness=1000000\relax%
    \setbox\tcb@totallowerbox=\vbox{%
      \unvbox\tcb@lowerbox%
      \splitdiscards%
      \unvbox\tcb@totallowerbox}%
  \else%
    \tcb@setbox@lower{\tcb@split@dim}{\tcb@lowerbox}%
  \fi%
  \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz\savingvdiscards=0%
}


\def\tcb@split@lower@box{%
  \vfuzz=\maxdimen\vbadness=10000%
  \tcb@vsplit@lower%
  \ifnum\tcb@lower@box@badness=1000000\relax%
    \tcb@warning{The lower box part has become overfull}%
  \fi%
  \tcb@setbox@lower{\tcb@split@dim}{\tcb@lowerbox}%
  \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz%
}

% patch for luatex 0.95 (thanks to Jeremy Engel)
\ifdefined\directlua
  \RequirePackage{ifluatex}
  \ifnum\luatexversion=95\relax
  \def\tcb@vsplit@upper{%
    \directlua{%
      tex.savingvdiscards = 1
      local vlist = tex.splitbox("tcb@totalupperbox", tex.sp("\tcb@split@dim"), "exactly")
      tex.setbox("tcb@upperbox", vlist)
      tex.savingvdiscards = 0
    }%
    \edef\tcb@upper@box@badness{\the\badness}%
  }
  \def\tcb@vsplit@lower{%
    \directlua{%
      tex.savingvdiscards = 1
      local vlist = tex.splitbox("tcb@totallowerbox", tex.sp("\tcb@split@dim"), "exactly")
      tex.setbox("tcb@lowerbox", vlist)
      tex.savingvdiscards = 0
    }%
    \edef\tcb@lower@box@badness{\the\badness}%
  }
\fi\fi

\def\tcb@split@setstate@first{%
  \edef\tcb@split@state{first}%
  \let\kvtcb@top@rule=\kvtcb@top@rule@stand%
  \let\kvtcb@bottom@rule=\kvtcb@bottom@rule@break%
  \let\kvtcb@bbtop=\kvtcb@bbtop@stand%
  \let\kvtcb@bbbottom=\kvtcb@bbbottom@break%
  \let\tcb@break@topsep=\tcb@zpt%
  \let\tcb@break@bottomsep=\kvtcb@bottomsep%
}

\def\tcb@split@setstate@middle{%
  \edef\tcb@split@state{middle}%
  \let\kvtcb@top@rule=\kvtcb@top@rule@break%
  \let\kvtcb@bottom@rule=\kvtcb@bottom@rule@break%
  \let\kvtcb@bbtop=\kvtcb@bbtop@break%
  \let\kvtcb@bbbottom=\kvtcb@bbbottom@break%
  \let\tcb@break@topsep=\kvtcb@topsep%
  \let\tcb@break@bottomsep=\kvtcb@bottomsep%
}

\def\tcb@split@setstate@last{%
  \edef\tcb@split@state{last}%
  \let\kvtcb@top@rule=\kvtcb@top@rule@break%
  \let\kvtcb@bottom@rule=\kvtcb@bottom@rule@stand%
  \let\kvtcb@bbtop=\kvtcb@bbtop@break%
  \let\kvtcb@bbbottom=\kvtcb@bbbottom@stand%
  \let\tcb@break@topsep=\kvtcb@topsep%
  \let\tcb@break@bottomsep=\tcb@zpt%
}


\def\tcb@split@force@standalone{%
  \tcb@comp@h@total@standalone%
  \ifdim\tcb@h@total>\tcb@h@page\relax%
    \tcbdimto\kvtcb@bbbottom@stand{\kvtcb@bbbottom@stand+\tcb@h@page-\tcb@h@total}%
  \fi%
}


\def\tcb@split@break@to@start{%
  \tcb@swap{\tcb@totalupperbox}{\tcb@upperbox}%
  \tcb@swap{\tcb@totallowerbox}{\tcb@lowerbox}%
  \tcbdimto\tcb@h@upper{\ht\tcb@upperbox+\dp\tcb@upperbox}%
  \tcbdimto\tcb@h@lower{\ht\tcb@lowerbox+\dp\tcb@lowerbox}%
  \tcb@split@pagebreak%
  \let\tcb@split@next=\tcb@split@start%
}

\def\tcb@split@first{%
  \setcounter{tcbbreakpart}{1}%
  \ifx\kvtcb@float\@empty%
    \iftcb@vfillbeforefirst%
      \let\tcb@before@first=\vfill%
    \else%
    \let\tcb@before@first=\@empty%
    \fi%
    \let\tcb@before@middle=\@empty%
    \let\tcb@before@last=\@empty%
    \iftcb@multicol%
      \long\def\tcb@after@first{\par}% using \columnbreak here kills multicols' algortihm sometimes
      \long\def\tcb@after@middle{\par\vfill}%
    \else%
      \long\def\tcb@after@first{\par\pagebreak\tcb@enlbreak@next}%
      \long\def\tcb@after@middle{\par\vfill\eject\tcb@enlbreak@next}%
    \fi%
    \let\tcb@after@last=\par%
  \else%
    \edef\tcb@before@first{\noexpand\tcb@float@env@begin{tcbfloat}[\kvtcb@float]\noexpand\kvtcb@everyfloat}%
    \let\tcb@before@middle=\tcb@before@first%
    \let\tcb@before@last=\tcb@before@first%
    \let\tcb@after@first=\tcb@float@env@end%
    \let\tcb@after@middle=\tcb@float@env@end%
    \let\tcb@after@last=\tcb@float@env@end%
  \fi%
  %
  \edef\kvtcb@skin@@first{\kvtcb@skin@first}%
  \edef\kvtcb@skin@@middle{\kvtcb@skin@middle}%
  \edef\kvtcb@skin@@last{\kvtcb@skin@last}%
  %
  \let\tcb@h@breaksep@first=\kvtcb@bottomsep%
  \tcbdimto\tcb@h@breaksep@middle{\kvtcb@bottomsep+\kvtcb@topsep}%
  \let\tcb@h@breaksep@last=\kvtcb@topsep%
  \tcbdimto\tcb@h@padding@first{\kvtcb@bbtop@stand+\kvtcb@bbbottom@break+\kvtcb@top@rule@stand+\kvtcb@bottom@rule@break+\tcb@h@breaksep@first+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom}%
  \tcbdimto\tcb@h@padding@middle{\kvtcb@bbtop@break+\kvtcb@bbbottom@break+\kvtcb@top@rule@break+\kvtcb@bottom@rule@break+\tcb@h@breaksep@middle+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom}%
  \tcbdimto\tcb@h@padding@last{\kvtcb@bbtop@break+\kvtcb@bbbottom@stand+\kvtcb@top@rule@break+\kvtcb@bottom@rule@stand+\tcb@h@breaksep@last+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom}%
  %
  \tcb@split@setstate@first%
  %
  \splittopskip=0pt%
  \splitmaxdepth=0pt%
  \edef\tcb@thevfuzz{\the\vfuzz}%
  \edef\tcb@thevbadness{\the\vbadness}%
  %
  \tcb@swap{\tcb@totalupperbox}{\tcb@upperbox}%
  \tcb@swap{\tcb@totallowerbox}{\tcb@lowerbox}%
  %
  \let\tcb@split@next=\relax%
  \tcbdimto\tcb@split@dim{\tcb@h@page-\tcb@h@padding@first-\tcb@h@padtitle}%
  \ifdim\tcb@split@dim<\tcb@h@upper\relax%
    %
    %
    \iftcb@break@allowed%
      \tcb@split@upper@box@and@assemble%
      \ifnum\tcb@upper@box@badness=1000000\relax%
        \tcb@split@break@to@start%
      \else%
        \ifdim\wd\tcb@totalupperbox=0pt\relax%
          \iftcb@lowerspace%
            \tcb@sdraw@U%
            \let\tcb@split@next=\tcb@split@SL%
          \else%
            \tcb@split@force@standalone%
            \tcb@drawcolorbox@standalone%
          \fi%
        \else%
          \ifdim\dimexpr\tcb@h@upper=0pt\relax%
            \tcb@warning{Discard zero height first box part due to break problems (possible loss of zero height content)}%
            \tcb@split@break@to@start%
          \else%
            \tcb@sdraw@U%
            \let\tcb@split@next=\tcb@split@USL%
          \fi%
        \fi%
      \fi%
    \else%
      \tcb@split@upper@box%
      \ifdim\wd\tcb@totalupperbox=0pt\relax%
        \iftcb@lowerspace%
          \tcb@sdraw@U%
          \let\tcb@split@next=\tcb@split@SL%
        \else%
          \tcb@split@force@standalone%
          \tcb@drawcolorbox@standalone%
        \fi%
      \else%
        \tcb@sdraw@U%
        \let\tcb@split@next=\tcb@split@USL%
      \fi%
    \fi%
  \else%
    \tcb@swap{\tcb@totalupperbox}{\tcb@upperbox}%
    \iftcb@lowerspace%
      \tcbdimto\tcb@split@dim{\tcb@split@dim-\tcb@h@upper-\tcb@h@segment}%
      \ifdim\tcb@split@dim<\kvtcb@breakminlines\baselineskip\relax%
        \tcb@sdraw@U%
        \let\tcb@split@next=\tcb@split@SL%
      \else
        \tcb@split@lower@box@and@assemble%
        \ifnum\tcb@lower@box@badness=1000000\relax%
          \tcb@sdraw@U%
          \let\tcb@split@next=\tcb@split@SL%
        \else%
          \ifdim\wd\tcb@totallowerbox=0pt\relax%
            \tcb@split@force@standalone%
            \tcb@drawcolorbox@standalone%
          \else%
            \tcb@sdraw@USL%
            \let\tcb@split@next=\tcb@split@L%
          \fi%
        \fi%
      \fi%
    \else%
      \tcb@split@force@standalone%
      \tcb@drawcolorbox@standalone%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@split@force@last{%
  \tcb@split@setstate@last%
  \ifdim\tcb@h@total>\tcb@h@page%
    \tcbdimto\kvtcb@bbbottom{\kvtcb@bbbottom+\tcb@h@page-\tcb@h@total}%
  \fi%
}

\def\tcb@nextbreakpart{%
  \stepcounter{tcbbreakpart}%
  \tcb@count@boxes%
  \iftcb@checkpage%
    \tcb@phantom@savepage%
    \tcb@hasPhantomtrue%
    \sbox\tcb@phantombox{\kvtcb@phantom}%
    \let\kvtcb@phantom\@empty%
  \fi%
  \tcb@following@title%
}


\def\tcb@split@USL{%
  \tcb@nextbreakpart%
  \tcb@comp@h@page%
  \tcb@defToTotalHeight\tcb@h@upper{\tcb@totalupperbox}%
  \tcbdimto\tcb@h@total{\tcb@h@padding@last+\tcb@h@padtitle+\tcb@h@upper+\tcb@h@segment+\tcb@h@lower}%
  %
  \let\tcb@split@next=\relax%
  \tcb@check@for@final@box%
  \iftcb@final@box%
    \tcb@split@setstate@last%
    \tcb@setbox@upper{\tcb@h@upper}{\tcb@totalupperbox}%
    \iftcb@lowerspace%
      \tcb@setbox@lower{\tcb@h@lower}{\tcb@totallowerbox}%
      \tcb@sdraw@USL%
    \else
      \tcb@sdraw@U%
    \fi%
  \else
    \tcb@split@setstate@middle%
    \tcbdimto\tcb@split@dim{\tcb@h@page-\tcb@h@padding@middle-\tcb@h@padtitle}%
    \ifdim\tcb@split@dim<\tcb@h@upper\relax%
      \tcb@split@upper@box%
      \ifdim\wd\tcb@totalupperbox=0pt\relax%
        \iftcb@lowerspace%
          \tcb@sdraw@U%
          \let\tcb@split@next=\tcb@split@SL%
        \else%
          \tcb@split@force@last%
          \tcb@sdraw@U%
        \fi%
      \else%
        \tcb@sdraw@U%
        \let\tcb@split@next=\tcb@split@USL%
      \fi%
    \else%
      \tcb@setbox@upper{\tcb@h@upper}{\tcb@totalupperbox}%
      \iftcb@lowerspace%
        \tcbdimto\tcb@split@dim{\tcb@split@dim-\tcb@h@upper-\tcb@h@segment}
        \ifdim\tcb@split@dim<\kvtcb@breakminlines\baselineskip\relax%
          \tcb@sdraw@U%
          \let\tcb@split@next=\tcb@split@SL%
        \else
          \tcb@split@lower@box@and@assemble%
          \ifnum\tcb@lower@box@badness=1000000\relax%
            \tcb@sdraw@U%
            \let\tcb@split@next=\tcb@split@SL%
          \else%
            \ifdim\wd\tcb@totallowerbox=0pt\relax%
              \tcb@split@force@last%
              \tcb@sdraw@USL%
            \else%
              \tcb@sdraw@USL%
              \let\tcb@split@next=\tcb@split@L%
            \fi%
          \fi%
        \fi%
      \else%
        \tcb@split@force@last%
        \tcb@sdraw@U%
      \fi%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@split@SL@displayed{%
  \tcb@nextbreakpart%
  \tcb@comp@h@page%
  \let\tcb@h@upper=\tcb@zpt%
  \tcb@defToTotalHeight\tcb@h@lower{\tcb@totallowerbox}%
  \tcbdimto\tcb@h@total{\tcb@h@padding@last-\kvtcb@top-\kvtcb@boxsep+\tcb@h@padtitle+\tcb@h@segment+\tcb@h@lower}%
  %
  \let\tcb@split@next=\relax%
  \tcb@check@for@final@box%
  \iftcb@final@box%
    \tcb@split@setstate@last%
    \tcb@setbox@lower{\tcb@h@lower}{\tcb@totallowerbox}%
    \tcb@sdraw@SL%
  \else
    \tcb@split@setstate@middle%
    \tcbdimto\tcb@split@dim{\tcb@h@page-\tcb@h@padding@middle+\kvtcb@top+\kvtcb@boxsep-\tcb@h@padtitle-\tcb@h@segment}%
    \tcb@split@lower@box%
    \ifdim\wd\tcb@totallowerbox=0pt\relax%
      \tcb@split@force@last%
      \tcb@sdraw@SL%
    \else
      \tcb@sdraw@SL%
      \let\tcb@split@next=\tcb@split@L%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@split@L{%
  \tcb@nextbreakpart%
  \tcb@comp@h@page%
  \let\tcb@h@upper=\tcb@zpt%
  \tcb@defToTotalHeight\tcb@h@lower{\tcb@totallowerbox}%
  \tcbdimto\tcb@h@total{\tcb@h@padding@last+\tcb@h@padtitle+\tcb@h@lower}%
  %
  \let\tcb@split@next=\relax%
  \tcb@check@for@final@box%
  \iftcb@final@box%
    \tcb@split@setstate@last%
    \tcb@setbox@lower{\tcb@h@lower}{\tcb@totallowerbox}%
    \tcb@sdraw@L%
  \else
    \tcb@split@setstate@middle%
    \tcbdimto\tcb@split@dim{\tcb@h@page-\tcb@h@padding@middle-\tcb@h@padtitle}%
    \tcb@split@lower@box%
    \ifdim\wd\tcb@totallowerbox=0pt\relax%
      \tcb@split@force@last%
      \tcb@sdraw@L%
    \else
      \tcb@sdraw@L%
      \let\tcb@split@next=\tcb@split@L%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@break@ch@fixed{%
  \ifdim\tcb@natheight<\tcb@h@page\relax%
    \tcbdimto\kvtcb@height@fixed{\tcb@h@page-\kvtcb@bbtop-\kvtcb@bbbottom}%
    \tcb@ch@fixed%
  \else%
    \tcb@ch@natural%
  \fi%
}


\def\tcb@sdraw@USL{%
  \begingroup%
  \tcbset{skin=\csname kvtcb@skin@@\tcb@split@state\endcsname}%
  \csuse{tcb@extras@\tcb@split@state}%
  \tcb@afteroptions@hook%
  \def\tcbsegmentstate{1}%
  \tcbdimto\tcb@natheight{\tcb@h@padtitle+\kvtcb@top@rule+\kvtcb@bottom@rule+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom+\tcb@h@upper+\tcb@h@segment+\tcb@h@lower+\csname tcb@h@breaksep@\tcb@split@state\endcsname}%
  \csname tcb@break@ch@\tcb@split@state\endcsname%
  \tcbdimto\tcb@innerheight{\tcb@height-\kvtcb@top@rule-\kvtcb@bottom@rule-\tcb@h@padtitle}%
  \tcbdimto\tcbtextheight{\tcb@innerheight-\kvtcb@boxsep*2-\kvtcb@top-\kvtcb@bottom}%
  \tcb@drawing@env@begin%
    \tcb@extensions@preframe%
     % draw frame and interior
    \tcb@adraw@frame%
    \tcb@adraw@interior%
    \iftcb@lowerseparated%
      \tcb@segmentation@code%
    \fi%
    \tcb@adraw@title%
    \tcb@extensions@postframe%
    % draw text boxes
    \tcb@tdraw@title%
    \tcb@tdraw@upper%
    \tcb@tdraw@lower%
    \tcb@extensions@final%
  \tcb@drawing@env@end%
  \endgroup%
}


\def\tcb@sdraw@U{%
  \begingroup%
  \tcbset{skin=\csname kvtcb@skin@@\tcb@split@state\endcsname}%
  \csuse{tcb@extras@\tcb@split@state}%
  \tcb@afteroptions@hook%
  \def\tcbsegmentstate{0}%
  \tcbdimto\tcb@natheight{\tcb@h@padtitle+\kvtcb@top@rule+\kvtcb@bottom@rule+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom+\tcb@h@upper+\csname tcb@h@breaksep@\tcb@split@state\endcsname}%
  \csname tcb@break@ch@\tcb@split@state\endcsname%
  \tcbdimto\tcb@innerheight{\tcb@height-\kvtcb@top@rule-\kvtcb@bottom@rule-\tcb@h@padtitle}%
  \tcbdimto\tcbtextheight{\tcb@innerheight-\kvtcb@boxsep*2-\kvtcb@top-\kvtcb@bottom}%
  \tcb@drawing@env@begin%
    \tcb@extensions@preframe%
    % draw frame and interior
    \tcb@adraw@frame%
    \tcb@adraw@interior%
    \tcb@adraw@title%
    \tcb@extensions@postframe%
    % draw text boxes
    \tcb@tdraw@title%
    \tcb@tdraw@upper%
    \tcb@extensions@final%
  \tcb@drawing@env@end%
  \endgroup%
}


\def\tcb@sdraw@SL{%
  \begingroup%
  \tcbset{skin=\csname kvtcb@skin@@\tcb@split@state\endcsname}%
  \csuse{tcb@extras@\tcb@split@state}%
  \tcb@afteroptions@hook%
  \def\tcbsegmentstate{1}%
  \tcbdimto\tcb@natheight{\tcb@h@padtitle+\kvtcb@top@rule+\kvtcb@bottom@rule+\kvtcb@bottom+\kvtcb@boxsep+\tcb@h@segment+\tcb@h@lower+\csname tcb@h@breaksep@\tcb@split@state\endcsname}%
  \csname tcb@break@ch@\tcb@split@state\endcsname%
  \tcbdimto\tcb@innerheight{\tcb@height-\kvtcb@top@rule-\kvtcb@bottom@rule-\tcb@h@padtitle}%
  \tcbdimto\tcbtextheight{\tcb@innerheight-\kvtcb@boxsep*2-\kvtcb@top-\kvtcb@bottom}%
  \tcb@drawing@env@begin%
    \tcb@extensions@preframe%
    % draw frame and interior
    \tcb@adraw@frame%
    \tcb@adraw@interior%
    \iftcb@lowerseparated%
      \tcb@segmentation@code%
    \fi%
    \tcb@adraw@title%
    \tcb@extensions@postframe%
    % draw text boxes
    \tcb@tdraw@title%
    \tcb@tdraw@lower%
    \tcb@extensions@final%
  \tcb@drawing@env@end%
  \endgroup%
}


\def\tcb@sdraw@L{%
  \begingroup%
  \tcbset{skin=\csname kvtcb@skin@@\tcb@split@state\endcsname}%
  \csuse{tcb@extras@\tcb@split@state}%
  \tcb@afteroptions@hook%
  \def\tcbsegmentstate{2}%
  \tcbdimto\tcb@natheight{\tcb@h@padtitle+\kvtcb@top@rule+\kvtcb@bottom@rule+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom+\ht\tcb@lowerbox+\dp\tcb@lowerbox+\csname tcb@h@breaksep@\tcb@split@state\endcsname}%
  \csname tcb@break@ch@\tcb@split@state\endcsname%
  \tcbdimto\tcb@innerheight{\tcb@height-\kvtcb@top@rule-\kvtcb@bottom@rule-\tcb@h@padtitle}%
  \tcbdimto\tcbtextheight{\tcb@innerheight-\kvtcb@boxsep*2-\kvtcb@top-\kvtcb@bottom}%
  \tcb@drawing@env@begin%
    \tcb@extensions@preframe%
    % draw frame and interior
    \tcb@adraw@frame%
    \tcb@adraw@interior%
    \tcb@adraw@title%
    \tcb@extensions@postframe%
    % draw text boxes
    \tcb@tdraw@title%
    \tcb@tdraw@lower%
    \tcb@extensions@final%
  \tcb@drawing@env@end%
  \endgroup%
}



\tcbset{%
  breakable@true/.code={%
    \let\tcb@savebox=\tcb@vbox%
    \let\endtcb@savebox=\endtcb@vbox%
    \let\tcb@defToTotalHeight=\tcb@defToTotalHeightBreakable%
    \let\tcb@drawcolorbox=\tcb@drawcolorbox@breakable},
  breakable@unlimited/.code={%
    \let\tcb@savebox=\tcb@vbox%
    \let\endtcb@savebox=\endtcb@vbox%
    \let\tcb@defToTotalHeight=\tcb@defToTotalHeightUnlimited%
    \let\tcb@drawcolorbox=\tcb@drawcolorbox@breakable},
  breakable/.style={breakable@#1},
  breakable/.default=true,%
  unbreakable/.style={breakable=false},%
  enforce breakable/.code={%
    \let\tcb@savebox=\tcb@vbox%
    \let\endtcb@savebox=\endtcb@vbox%
    \let\tcb@defToTotalHeight=\tcb@defToTotalHeightBreakable%
    \let\tcb@drawcolorbox=\tcb@drawcolorbox@breakable},
  title after break/.store in=\kvtcb@followingtitle,%
  notitle after break/.style={title after break=},%
  adjusted title after break/.style={title after break={#1\vphantom{\kvtcb@adjusttext}}},%
  lines before break/.store in=\kvtcb@breakminlines,%
  shrink break goal/.store in=\kvtcb@shrinkbreakgoal,%
  toprule at break/.store in=\kvtcb@top@rule@break,
  bottomrule at break/.store in=\kvtcb@bottom@rule@break,
  topsep at break/.store in=\kvtcb@topsep,%
  bottomsep at break/.store in=\kvtcb@bottomsep,%
  pad before break/.code={\let\kvtcb@bottom@rule@break=\tcb@zpt%
    \tcbdimto\kvtcb@bottomsep{#1-\kvtcb@bottom-\kvtcb@boxsep}},%
  pad before break*/.style={pad before break={#1},%
    code={\tcbdimto\tcb@temp{\kvtcb@bottom@rule@stand-\kvtcb@bottomsep}%
      \ifdim\tcb@temp>0pt\relax%
        \tcbdimto\kvtcb@enlargepage@flex{\kvtcb@enlargepage@flex+\tcb@temp}\fi}},%
  pad after break/.code={\let\kvtcb@top@rule@break=\tcb@zpt%
    \def\kvtcb@topsep{#1-\kvtcb@top-\kvtcb@boxsep}},%
  pad at break/.style={pad before break={#1},pad after break={#1}},%
  pad at break*/.style={pad before break*={#1},pad after break={#1}},%
  enlargepage/.store in=\kvtcb@enlargepage,%
  enlargepage flexible/.store in=\kvtcb@enlargepage@flex,%
  break at/.store in=\kvtcb@breakatdim,%
  height fixed for/.is choice,%
  height fixed for/none/.code={%
    \let\tcb@break@ch@first=\tcb@ch@natural%
    \let\tcb@break@ch@middle=\tcb@ch@natural%
    \let\tcb@break@ch@last=\tcb@ch@natural},%
  height fixed for/first/.code={%
    \let\tcb@break@ch@first=\tcb@break@ch@fixed%
    \let\tcb@break@ch@middle=\tcb@ch@natural%
    \let\tcb@break@ch@last=\tcb@ch@natural},%
  height fixed for/middle/.code={%
    \let\tcb@break@ch@first=\tcb@ch@natural%
    \let\tcb@break@ch@middle=\tcb@break@ch@fixed%
    \let\tcb@break@ch@last=\tcb@ch@natural},%
  height fixed for/last/.code={%
    \let\tcb@break@ch@first=\tcb@ch@natural%
    \let\tcb@break@ch@middle=\tcb@ch@natural%
    \let\tcb@break@ch@last=\tcb@break@ch@fixed},%
  height fixed for/first and middle/.code={%
    \let\tcb@break@ch@first=\tcb@break@ch@fixed%
    \let\tcb@break@ch@middle=\tcb@break@ch@fixed%
    \let\tcb@break@ch@last=\tcb@ch@natural},%
  height fixed for/middle and last/.code={%
    \let\tcb@break@ch@first=\tcb@ch@natural%
    \let\tcb@break@ch@middle=\tcb@break@ch@fixed%
    \let\tcb@break@ch@last=\tcb@break@ch@fixed},%
  height fixed for/all/.code={%
    \let\tcb@break@ch@first=\tcb@break@ch@fixed%
    \let\tcb@break@ch@middle=\tcb@break@ch@fixed%
    \let\tcb@break@ch@last=\tcb@break@ch@fixed},%
  vfill before first/.is if=tcb@vfillbeforefirst,%
  height fill/true/.code={\let\tcb@height@adjust\tcb@height@fill@unbroken@normal},%
  height fill/maximum/.code={\let\tcb@height@adjust\tcb@height@fill@unbroken@compressed},%
  height fill/.default=true,%
  compress page/.is choice,%
  compress page/all/.code={\def\tcb@comp@compress{\def\tcb@compress@height{\pageshrink-1sp}}},%
  compress page/none/.code={\def\tcb@comp@compress{\let\tcb@compress@height\tcb@zpt}},%
  compress page/baselineskip/.code={\def\tcb@comp@compress{%
    \ifdim\pageshrink>\baselineskip%
      \let\tcb@compress@height\baselineskip%
    \else%
      \def\tcb@compress@height{\pageshrink-1sp}%
    \fi}},%
  compress page/.default=all,%
  compress page=baselineskip,% global setting
  extras unbroken/.code={\appto\tcb@extras@unbroken{\tcbset{#1}}},%
  extras first/.code={\appto\tcb@extras@first{\tcbset{#1}}},%
  extras middle/.code={\appto\tcb@extras@middle{\tcbset{#1}}},%
  extras last/.code={\appto\tcb@extras@last{\tcbset{#1}}},%
  extras title after break/.code={\appto\tcb@extras@followingtitle{\tcbset{#1}}},%
  extras/.style={extras unbroken={#1},extras first={#1},extras middle={#1},extras last={#1}},%
  extras broken/.style={extras first={#1},extras middle={#1},extras last={#1}},%
  extras unbroken and first/.style={extras unbroken={#1},extras first={#1}},%
  extras unbroken and last/.style={extras unbroken={#1},extras last={#1}},%
  extras middle and last/.style={extras middle={#1},extras last={#1}},%
  extras first and middle/.style={extras first={#1},extras middle={#1}},%
  no extras unbroken/.code={\let\tcb@extras@unbroken\@empty},%
  no extras first/.code={\let\tcb@extras@first\@empty},%
  no extras middle/.code={\let\tcb@extras@middle\@empty},%
  no extras last/.code={\let\tcb@extras@last\@empty},%
  no extras title after break/.code={\let\tcb@extras@followingtitle\@empty},
  no extras/.code={\let\tcb@extras@unbroken\@empty\let\tcb@extras@first\@empty\let\tcb@extras@middle\@empty\let\tcb@extras@last\@empty\let\tcb@extras@followingtitle\@empty},%
  if odd page*/.style 2 args={check odd page,extras={if odd page={#1}{#2}}},%
  if odd page or oneside*/.style 2 args={check odd page,extras={if odd page or oneside={#1}{#2}}},%
  segmentation at break/.is choice,%
  segmentation at break/true/.code={\let\tcb@split@SL\tcb@split@SL@displayed},
  segmentation at break/false/.code={\let\tcb@split@SL\tcb@split@L},
  segmentation at break/.default=true,
}


\tcbset{%
  reset@breakable/.style={%
    unbreakable,notitle after break,
    shrink break goal=0pt,
    lines before break=2,
    topsep at break=0pt,
    bottomsep at break=0pt,
    enlargepage=0pt,enlargepage flexible=0pt,
    break at=0pt,
    height fixed for=none,
    vfill before first=false,
    no extras,
    segmentation at break
  },
  initialize@reset=reset@breakable,
}


==> tcbdocumentation.code.tex <==
%% The LaTeX package tcolorbox - version 4.30 (2020/04/28)
%% tcbdocumentation.code.tex: Code for LaTeX documentations
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2020 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{4.30}

\tcbuselibrary{listings,skins,xparse,external,raster}

\RequirePackage{pifont}[2005/04/12]
\RequirePackage{marvosym}[2011/07/20]
\ifdefined\printindex\else\RequirePackage{makeidx}[2000/03/29]\fi
\RequirePackage{refcount}[2011/10/16]
\RequirePackage{hyperref}[2012/02/06]
\ifdefined\marginnote\else\RequirePackage{marginnote}[2012/03/29]\fi

\definecolor{Option}{rgb}{0.118,0.546,0.222}
\definecolor{Definition}{rgb}{0.784,0.06,0.176}
\definecolor{ExampleFrame}{rgb}{0.628,0.705,0.942}
\definecolor{ExampleBack}{rgb}{0.963,0.971,0.994}
\definecolor{Hyperlink}{rgb}{0.281,0.275,0.485}
\definecolor{Fade}{rgb}{0.5,0.5,0.5}

\def\colDef#1{\textcolor{\kvtcb@col@command}{#1}}
\def\colOpt#1{\textcolor{\kvtcb@col@opt}{#1}}
\def\colFade#1{\textcolor{\kvtcb@col@fade}{#1}}

\lstdefinestyle{tcbdocumentation}{language={[LaTeX]TeX},
    aboveskip={0\p@ \@plus 6\p@},
    belowskip={0\p@ \@plus 6\p@},
    columns=fullflexible,
    keepspaces=true,
    breaklines=true,
    prebreak={\Righttorque},
    postbreak={\space\Lefttorque},
    breakatwhitespace=true,
    basicstyle=\ttfamily\footnotesize,
    extendedchars=true,
    moredelim={[is][\itshape\rmfamily]{^^a7}{^^a7}},
    nolol,inputencoding=\kvtcb@listingencoding}

% The following macros are taken from ltxdoc
\DeclareRobustCommand\cs[1]{\texttt{\char`\\#1}}
\def\meta@font@select{\rmfamily\itshape}

\AtEndPreamble{%
  \@ifpackageloaded{doc}{%
  }{% code taken from doc.sty
    \ifx\l@nohyphenation\undefined
      \newlanguage\l@nohyphenation
    \fi
    \DeclareRobustCommand\meta[1]{%
         \ensuremath\langle
         \ifmmode \expandafter \nfss@text \fi
         {%
          \meta@font@select
          \edef\meta@hyphen@restore
            {\hyphenchar\the\font\the\hyphenchar\font}%
          \hyphenchar\font\m@ne
          \language\l@nohyphenation
          #1\/%
          \meta@hyphen@restore
         }\ensuremath\rangle
    }%
  }%
}%

\def\marg#1{%
  {\ttfamily\char`\{}\meta{#1}{\ttfamily\char`\}}}
\def\oarg#1{%
  \colOpt{{\ttfamily[}\meta{#1}{\ttfamily]}}}
\def\brackets#1{{\ttfamily\char`\{}#1{\ttfamily\char`\}}}

\newif\iftcb@doc@toindex
\newif\iftcb@doc@colorize
\newif\iftcb@doc@annotate

% language specific texts
\tcbset{
  doclang/.cd,
  color/.store in=\kvtcb@text@color,
  colors/.store in=\kvtcb@text@colors,
  counter/.store in=\kvtcb@text@counter,
  counters/.store in=\kvtcb@text@counters,
  environment content/.store in=\kvtcb@text@envcontent,
  environment/.store in=\kvtcb@text@env,
  environments/.store in=\kvtcb@text@envs,
  index/.store in=\kvtcb@text@index,
  key/.store in=\kvtcb@text@key,
  keys/.store in=\kvtcb@text@keys,
  length/.store in=\kvtcb@text@length,
  lengths/.store in=\kvtcb@text@lengths,
  new/.store in=\kvtcb@text@new,
  path/.store in=\kvtcb@text@path,
  paths/.store in=\kvtcb@text@paths,
  pageshort/.store in=\kvtcb@text@pageshort,
  updated/.store in=\kvtcb@text@updated,
  value/.store in=\kvtcb@text@value,
  values/.store in=\kvtcb@text@values,
}

% documentation options
\tcbset{
  documentation listing options/.store in=\kvtcb@doclistingoptions,%
  documentation listing style/.style={documentation listing options={style=#1}},%
  documentation minted language/.store in=\kvtcb@docminted@language,
  documentation minted style/.store in=\kvtcb@docmintstyle,
  documentation minted options/.store in=\kvtcb@docmintoptions,
  color command/.store in=\kvtcb@col@command,
  color environment/.store in=\kvtcb@col@environment,
  color key/.store in=\kvtcb@col@key,
  color value/.store in=\kvtcb@col@value,
  color counter/.store in=\kvtcb@col@counter,
  color length/.store in=\kvtcb@col@length,
  color color/.store in=\kvtcb@col@color,
  color fade/.store in=\kvtcb@col@fade,
  color path/.store in=\kvtcb@col@path,
  color definition/.style={color command={#1},color environment={#1},color key={#1},
    color value={#1},color color={#1},color counter={#1},color length={#1}, color path={#1}},
  color option/.store in=\kvtcb@col@opt,
  color hyperlink/.store in=\kvtcb@colhyper,
  index actual/.store in=\idx@actual,
  index quote/.store in=\idx@quote,
  index level/.store in=\idx@level,
  index format/.store in=\idx@format,
  index colorize/.is if=tcb@doc@colorize,%
  index annotate/.is if=tcb@doc@annotate,%
  index command/.code={\def\kvtcb@index@command##1{#1{##1}}},%
  index command name/.code={\def\kvtcb@index@command##1{\index[#1]{##1}}},%
  doc left/.dimstore in=\kvtcb@doc@left,
  doc right/.dimstore in=\kvtcb@doc@right,
  doc left indent/.dimstore in=\kvtcb@doc@indentleft,
  doc right indent/.dimstore in=\kvtcb@doc@indentright,
  doc head command/.style={doc@head@command/.style={#1}},
  doc head environment/.style={doc@head@environment/.style={#1}},
  doc head key/.style={doc@head@key/.style={#1}},
  doc head path/.style={doc@head@path/.style={#1}},
  doc head/.style={doc head command={#1},doc head environment={#1},doc head key={#1},
    doc head path={#1}},
  doc raster command/.style={doc@raster@command/.style={#1}},
  doc raster environment/.style={doc@raster@environment/.style={#1}},
  doc raster key/.style={doc@raster@key/.style={#1}},
  doc raster path/.style={doc@raster@path/.style={#1}},
  doc raster/.style={doc raster command={#1},doc raster environment={#1},doc raster key={#1},
    doc raster path={#1}},
  doc label/.store in=\kvtcb@doc@label,
  doc index/.store in=\kvtcb@doc@index,
  doc sort index/.store in=\kvtcb@doc@sortindex,
  doc@name/.store in=\kvtcb@doc@name,
  doc parameter/.store in=\kvtcb@doc@parameter,
  doc name/.style={doc@name={#1},doc label={#1},doc index={#1},doc sort index={#1}},
  doc keypath/.store in=\kvtcb@doc@keypath,
  doc@sub@keypath/.style={doc keypath/.code={
    \ifblank{##1}{\def\kvtcb@doc@keypath{#1}}{\def\kvtcb@doc@keypath{#1/##1}}}},
  before doc body command/.store in=\kvtcb@doc@body@command@before,
  after doc body command/.store in=\kvtcb@doc@body@command@after,
  before doc body environment/.store in=\kvtcb@doc@body@environment@before,
  after doc body environment/.store in=\kvtcb@doc@body@environment@after,
  before doc body key/.store in=\kvtcb@doc@body@key@before,
  after doc body key/.store in=\kvtcb@doc@body@key@after,
  before doc body path/.store in=\kvtcb@doc@body@path@before,
  after doc body path/.store in=\kvtcb@doc@body@path@after,
  before doc body/.style={before doc body command={#1},before doc body environment={#1},
    before doc body key={#1},before doc body path={#1}},
  after doc body/.style={after doc body command={#1},after doc body environment={#1}
    ,after doc body key={#1},after doc body path={#1}},
  doc description/.store in=\kvtcb@doc@description,%
  doc into index/.is if=tcb@doc@toindex,%
  doc no index/.style={doc into index=false},
  doc updated/.style={before upper={\tcbdocmarginnote{\tcbdocupdated{#1}}}},
  doc new/.style={before upper={\tcbdocmarginnote{\tcbdocnew{#1}}}},
  doc new and updated/.style 2 args={before upper={\tcbdocmarginnote{\tcbdocnew{#1}\\\tcbdocupdated{#2}}}},
  doc marginnote/.style={doc@marginnote/.style={#1}},
  keywords bold/.is choice,%
  keywords bold/.default=true,%
  keywords bold/true/.code={\let\tcb@doc@bfseries\bfseries},
  keywords bold/false/.code={\let\tcb@doc@bfseries\mdseries},
}


% styles
\tcbset{
  docexample/.style={colframe=ExampleFrame,colback=ExampleBack,
    before skip=\medskipamount,after skip=\medskipamount,
    fontlower=\footnotesize},
  documentation minted language=latex,
  documentation minted style=,
  documentation minted options={tabsize=2,fontsize=\small},
  index default settings/.style={index actual={@},index quote={"},index level={!}},
  index german settings/.style={index actual={=},index quote={!},index level={>}},
  english language/.code={\tcbset{doclang/.cd,
    color=color,colors=Colors,
    counter=counter,counters=Counters,
    environment content=environment content,
    environment=environment,environments=Environments,
    path=path operation,paths=Path operations,
    index=Index,
    key=key,keys=Keys,
    length=length,lengths=Lengths,
    new=New,
    pageshort={P.},
    updated=Updated,
    value=value,values=Values}},
}

\AtBeginDocument{%
  \csname tcb@doc@index@\idx@format\endcsname%
  \hypersetup{
  citecolor=\kvtcb@colhyper,
  linkcolor=\kvtcb@colhyper,
  urlcolor=\kvtcb@colhyper,
  filecolor=\kvtcb@colhyper,
  menucolor=\kvtcb@colhyper
}}

\def\dispExample{\tcb@layer@pushup\tcbset{docexample}\begingroup\tcbwritetemp}

\def\enddispExample{%
  \endtcbwritetemp\endgroup%
  \begin{tcolorbox}%
  \tcb@doc@usetemplisting%
  \tcblower%
  \tcbusetemp%
  \end{tcolorbox}%
}

\newenvironment{dispExample*}[1]{%
  \tcb@layer@pushup\tcbset{docexample,#1}\begingroup\tcbwritetemp%
  }{\enddispExample}

\def\dispListing{\tcb@layer@pushup\tcbset{docexample}\begingroup\tcbwritetemp}

\def\enddispListing{%
  \endtcbwritetemp\endgroup%
  \begin{tcolorbox}%
  \tcb@doc@usetemplisting%
  \end{tcolorbox}%
}

\newenvironment{dispListing*}[1]{%
  \tcb@layer@pushup\tcbset{docexample,#1}\begingroup\tcbwritetemp%
  }{\enddispListing}

% index auxiliary macros
\def\tcb@Index@Print@CA#1#2#3{%
  \iftcb@doc@colorize\textcolor{#2}{\tcb@scantokens{#1}}\else\tcb@scantokens{#1}\fi%
  \iftcb@doc@annotate\ #3\fi%
}

\def\tcb@Index@Print@C#1#2{%
  \iftcb@doc@colorize\textcolor{#2}{\tcb@scantokens{#1}}\else\tcb@scantokens{#1}\fi%
}

\def\tcb@Index@Print@ComCA#1#2#3{%
  \iftcb@doc@colorize\textcolor{#2}{\tcb@cs{#1}}\else\tcb@cs{#1}\fi%
  \iftcb@doc@annotate\ #3\fi%
}

\def\tcb@Index@Print@ComC#1#2{%
  \iftcb@doc@colorize\textcolor{#2}{\tcb@cs{#1}}\else\tcb@cs{#1}\fi%
}

\newrobustcmd{\tcbIndexPrintComC}[1]{\tcb@Index@Print@ComC{#1}{\kvtcb@col@command}}

\newrobustcmd{\tcbIndexPrintEnvCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@environment}{\kvtcb@text@env}}
\newrobustcmd{\tcbIndexPrintEnvC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@environment}}

\newrobustcmd{\tcbIndexPrintKeyCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@key}{\kvtcb@text@key}}
\newrobustcmd{\tcbIndexPrintKeyC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@key}}

\newrobustcmd{\tcbIndexPrintPathCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@path}{\kvtcb@text@path}}
\newrobustcmd{\tcbIndexPrintPathC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@path}}

\newrobustcmd{\tcbIndexPrintValCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@value}{\kvtcb@text@value}}
\newrobustcmd{\tcbIndexPrintValC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@value}}

\newrobustcmd{\tcbIndexPrintColCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@color}{\kvtcb@text@color}}
\newrobustcmd{\tcbIndexPrintColC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@color}}

\newrobustcmd{\tcbIndexPrintCountCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@counter}{\kvtcb@text@counter}}
\newrobustcmd{\tcbIndexPrintCountC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@counter}}

\newrobustcmd{\tcbIndexPrintLenCA}[1]{\tcb@Index@Print@ComCA{#1}{\kvtcb@col@length}{\kvtcb@text@length}}
\newrobustcmd{\tcbIndexPrintLenC}[1]{\tcb@Index@Print@ComC{#1}{\kvtcb@col@length}}


\newenvironment{tcb@manual@entry}{\begin{list}{}{%
  \setlength{\leftmargin}{\kvtcb@doc@left}%
  \setlength{\itemindent}{0pt}%
  \setlength{\itemsep}{0pt}%
  \setlength{\parsep}{0pt}%
  \setlength{\rightmargin}{\kvtcb@doc@right}%
  }\item}{\end{list}}

\def\tcb@doc@do@description{%
  \ifx\kvtcb@doc@description\@empty\else\tcblower\raggedleft\strut(\kvtcb@doc@description)\strut\fi%
}

\newtcolorbox{tcb@doc@head}[1]{blank,colback=white,colframe=white,
  code={\tcbdimto\tcb@temp@grow@left{-\kvtcb@doc@indentleft}%
        \tcbdimto\tcb@temp@grow@right{-\kvtcb@doc@indentright}},
  grow to left by=\tcb@temp@grow@left,
  grow to right by=\tcb@temp@grow@right,
  sidebyside,sidebyside align=top,
  sidebyside gap=-\tcb@w@upper@real,
  phantom=\phantomsection,#1}


\ExplSyntaxOn


\cs_new_nopar:Npn \__tcobox_sanitize_tl:n #1
  {
    \group_begin:
    \tl_rescan:nn
      {
        \char_set_catcode_letter:N \_
        \char_set_catcode_letter:N \@
      }
      {
        #1
      }
    \group_end:
  }
\cs_generate_variant:Nn \__tcobox_sanitize_tl:n { V }


\cs_new_nopar:Npn \__tcobox_print_docname:
  {
    \texttt{\tcb@doc@bfseries\__tcobox_sanitize_tl:V\kvtcb@doc@name}
  }

\cs_new_nopar:Npn \__tcobox_print_cs_docname:
  {
    \texttt{\tcb@doc@bfseries\c_backslash_str\__tcobox_sanitize_tl:V\kvtcb@doc@name}
  }


\NewDocumentCommand \tcb@scantokens { m }
  {
    \texttt{\__tcobox_sanitize_tl:n{#1}}
  }

\NewDocumentCommand \tcb@cs { m }
  {
    \texttt{\c_backslash_str\__tcobox_sanitize_tl:n{#1}}
  }


% main documentation environments

\seq_new:N \g__tcobox_label_seq


\cs_new:Npn \__tcobox_doc_entry_begin:nnn #1#2#3
  {
    \tcbset{doc~name=, doc~parameter=, doc~description=, #1}
    \begin{tcb@manual@entry}
    \seq_clear:N \g__tcobox_label_seq
    \begin{tcbraster}[raster~columns=1,raster~row~skip=0pt,
      raster~after~skip=4.1pt,raster~force~size=false,doc@raster@#3]
    \seq_set_from_clist:Nn \l_tmpa_seq {#2}
    \seq_if_empty:NT \l_tmpa_seq
    {
      \seq_put_left:Nn \l_tmpa_seq {}
    }
    \seq_map_inline:Nn \l_tmpa_seq
      {
        \group_begin:
        \tcbset{##1}
        \begin{tcb@doc@head}{doc@head@#3}
        \strut
        \use:c { __tcobox_doc_head_#3: }
        \strut
        \end{tcb@doc@head}
        \group_end:
      }
    \end{tcbraster}
    \seq_clear:N \g__tcobox_label_seq
    \nobreak
    \tcbset{before~upper=}
    \use:c { kvtcb@doc@body@#3@before }
    \ignorespaces
  }


\cs_new:Npn \__tcobox_doc_entry_end:n #1
  {
    \ifvmode\else\unskip\fi
    \use:c { kvtcb@doc@body@#1@after }
    \end{tcb@manual@entry}
  }


\cs_new_nopar:Npn \__tcobox_print_command:
  {
    \textcolor{\kvtcb@col@command}{\__tcobox_print_cs_docname:}
  }

\cs_new_nopar:Npn \__tcobox_index_command:
  {
    \iftcb@doc@toindex
      \kvtcb@index@command{\kvtcb@doc@sortindex\idx@actual\tcbIndexPrintComC{\kvtcb@doc@index}}
    \fi
  }

\cs_new:Npn \__tcobox_doc_head_command:
  {
    \__tcobox_print_command:
    \__tcobox_index_command:
    \seq_if_in:NVF \g__tcobox_label_seq \kvtcb@doc@label
      {
        \protected@edef\@currentlabel{\noexpand\tcb@cs{\kvtcb@doc@name}}
        \label{com:\kvtcb@doc@label}
        \seq_gput_left:NV \g__tcobox_label_seq \kvtcb@doc@label
      }
    {\ttfamily\kvtcb@doc@parameter}
    \tcb@doc@do@description
  }


\NewDocumentEnvironment{docCommands}{ +O{} +m }
  {
    \__tcobox_doc_entry_begin:nnn {#1}{#2}{command}
  }
  {
    \__tcobox_doc_entry_end:n { command }
  }


\NewDocumentEnvironment{docCommand}{ +O{} m +m }
  {
    \__tcobox_doc_entry_begin:nnn {doc~name={#2},doc~parameter={#3},#1}{}{command}
  }
  {
    \__tcobox_doc_entry_end:n { command }
  }


\NewDocumentEnvironment{docCommand*}{}
  {
    \group_begin:
    \tcb@doc@toindexfalse
    \begin{docCommand}
  }
  {
    \end{docCommand}
    \group_end:
  }


\cs_new_nopar:Npn \__tcobox_print_environment:
  {
    \textcolor{\kvtcb@col@environment}{\__tcobox_print_docname:}
  }

\cs_new_nopar:Npn \__tcobox_index_environment:
  {
    \iftcb@doc@toindex
      \kvtcb@index@command{\kvtcb@doc@sortindex\idx@actual\tcbIndexPrintEnvCA{\kvtcb@doc@index}}
      \kvtcb@index@command{\kvtcb@text@envs\idx@level\kvtcb@doc@sortindex\idx@actual\tcbIndexPrintEnvC{\kvtcb@doc@index}}
    \fi
  }

\cs_new:Npn \__tcobox_doc_head_environment:
  {
    \strut\cs{begin}\brackets{\__tcobox_print_environment:}
    \__tcobox_index_environment:
    \seq_if_in:NVF \g__tcobox_label_seq \kvtcb@doc@label
      {
        \protected@edef\@currentlabel{\kvtcb@doc@name}
        \label{env:\kvtcb@doc@label}
        \seq_gput_left:NV \g__tcobox_label_seq \kvtcb@doc@label
      }
    {\ttfamily\kvtcb@doc@parameter}\par
    \strut\nobreakspace\nobreakspace\meta{\kvtcb@text@envcontent}\par
    \strut\cs{end}\brackets{\__tcobox_print_environment:}
    \tcb@doc@do@description
  }


\NewDocumentEnvironment{docEnvironments}{ +O{} +m }
  {
    \__tcobox_doc_entry_begin:nnn {#1}{#2}{environment}
  }
  {
    \__tcobox_doc_entry_end:n { environment }
  }


\NewDocumentEnvironment{docEnvironment}{ +O{} m +m }
  {
    \__tcobox_doc_entry_begin:nnn {doc~name={#2},doc~parameter={#3},#1}{}{environment}
  }
  {
    \__tcobox_doc_entry_end:n { environment }
  }


\NewDocumentEnvironment{docEnvironment*}{}
  {
    \group_begin:
    \tcb@doc@toindexfalse
    \begin{docEnvironment}
  }
  {
    \end{docEnvironment}
    \group_end:
  }


\cs_new_nopar:Npn \__tcobox_print_key:
  {
    \textcolor{\kvtcb@col@key}{\tcb@doc@bfseries\ttfamily
    \tl_if_empty:NF \kvtcb@doc@keypath
      {
        /\__tcobox_sanitize_tl:V\kvtcb@doc@keypath/
      }
    \__tcobox_sanitize_tl:V\kvtcb@doc@name}
  }

\cs_new_nopar:Npn \__tcobox_index_key:
  {
    \iftcb@doc@toindex
      \kvtcb@index@command{\kvtcb@doc@sortindex\idx@actual\tcbIndexPrintKeyCA{\kvtcb@doc@index}}
      \tl_if_empty:NTF \kvtcb@doc@keypath
        {
          \kvtcb@index@command{\kvtcb@text@keys\idx@level\kvtcb@doc@sortindex\idx@actual\tcbIndexPrintKeyC{\kvtcb@doc@index}}
        }
        {
          \kvtcb@index@command{\kvtcb@text@keys\idx@level\kvtcb@doc@keypath\idx@actual\tcbIndexPrintKeyC{/\kvtcb@doc@keypath/}
            \idx@level\kvtcb@doc@sortindex\idx@actual\tcbIndexPrintKeyC{\kvtcb@doc@index}}
        }
    \fi
  }

\cs_new:Npn \__tcobox_doc_head_key:
  {
    \__tcobox_print_key:
    \__tcobox_index_key:
    \tl_if_empty:NTF \kvtcb@doc@keypath
      {
        \seq_if_in:NVF \g__tcobox_label_seq \kvtcb@doc@label
          {
            \protected@edef\@currentlabel{\kvtcb@doc@name}
            \label{key:\kvtcb@doc@label}
            \seq_gput_left:NV \g__tcobox_label_seq \kvtcb@doc@label
          }
      }
      {
        \tl_set:Nx \l_tmpa_tl {/\kvtcb@doc@keypath/\kvtcb@doc@label}
        \seq_if_in:NVF \g__tcobox_label_seq \l_tmpa_tl
          {
            \protected@edef\@currentlabel{/\kvtcb@doc@keypath/\kvtcb@doc@name}
            \label{key:/\kvtcb@doc@keypath/\kvtcb@doc@label}
            \seq_gput_left:NV \g__tcobox_label_seq \l_tmpa_tl
          }
      }
    {\ttfamily\kvtcb@doc@parameter}
    \tcb@doc@do@description
  }


\NewDocumentEnvironment{docKeys}{ +O{} +m }
  {
    \__tcobox_doc_entry_begin:nnn {doc~keypath=,#1}{#2}{key}
  }
  {
    \__tcobox_doc_entry_end:n { key }
  }


\NewDocumentEnvironment{docKey}{ O{} +O{} m m +m }
  {
    \__tcobox_doc_entry_begin:nnn
      {
        doc~keypath=#1,doc~name={#3},doc~parameter={#4},doc~description={#5},#2
      }
      {}{key}
  }
  {
    \__tcobox_doc_entry_end:n { key }
  }


\NewDocumentEnvironment{docKey*}{}
  {
    \group_begin:
    \tcb@doc@toindexfalse
    \begin{docKey}
  }
  {
    \end{docKey}
    \group_end:
  }


\NewDocumentCommand \tcbmakedocSubKey { m m }
  {
    \NewDocumentEnvironment{#1}{ O{} +O{} m m +m }
      {
        \__tcobox_doc_entry_begin:nnn
          {
            doc@sub@keypath=#2,
            doc~keypath=##1,
            doc~name={##3},
            doc~parameter={##4},
            doc~description={##5},
            ##2
          }
          {}{key}
      }
      {
        \__tcobox_doc_entry_end:n { key }
      }
    \NewDocumentEnvironment{#1*}{}
      {
        \group_begin:
        \tcb@doc@toindexfalse
        \begin{#1}
      }
      {
        \end{#1}
        \group_end:
      }
  }


\NewDocumentCommand \tcbmakedocSubKeys { m m }
  {
    \NewDocumentEnvironment{#1}{ +O{} +m }
      {
        \__tcobox_doc_entry_begin:nnn
          {
            doc@sub@keypath=#2,
            doc~keypath=,
            ##1
          }
          {##2}{key}
      }
      {
        \__tcobox_doc_entry_end:n { key }
      }
  }


\cs_new_nopar:Npn \__tcobox_print_path:
  {
    \textcolor{\kvtcb@col@path}{\__tcobox_print_docname:}
  }

\cs_new_nopar:Npn \__tcobox_index_path:
  {
    \iftcb@doc@toindex
      \kvtcb@index@command{\kvtcb@doc@sortindex\idx@actual\tcbIndexPrintPathCA{\kvtcb@doc@index}}
      \kvtcb@index@command{\kvtcb@text@paths\idx@level\kvtcb@doc@sortindex\idx@actual\tcbIndexPrintPathC{\kvtcb@doc@index}}
    \fi
  }

\cs_new:Npn \__tcobox_doc_head_path:
  {
    \colFade{\tcb@cs{path~...}}~\__tcobox_print_path:
    \__tcobox_index_path:
    \seq_if_in:NVF \g__tcobox_label_seq \kvtcb@doc@label
      {
        \protected@edef\@currentlabel{\kvtcb@doc@name}
        \label{path:\kvtcb@doc@label}
        \seq_gput_left:NV \g__tcobox_label_seq \kvtcb@doc@label
      }
    {\ttfamily\kvtcb@doc@parameter{}~\colFade{...;}}
    \tcb@doc@do@description
  }


\NewDocumentEnvironment{docPathOperations}{ +O{} +m }
  {
    \__tcobox_doc_entry_begin:nnn {#1}{#2}{path}
  }
  {
    \__tcobox_doc_entry_end:n { path }
  }


\NewDocumentEnvironment{docPathOperation}{ +O{} m +m }
  {
    \__tcobox_doc_entry_begin:nnn {doc~name={#2},doc~parameter={#3},#1}{}{path}
  }
  {
    \__tcobox_doc_entry_end:n { path }
  }


\NewDocumentEnvironment{docPathOperation*}{}
  {
    \group_begin:
    \tcb@doc@toindexfalse
    \begin{docPathOperation}
  }
  {
    \end{docPathOperation}
    \group_end:
  }


\NewDocumentCommand \docAuxCommand { s +O{} m }
  {
    \group_begin:
    \tcbset{doc~name={#3},#2}
    \__tcobox_print_command:
    \IfBooleanF{#1}{\__tcobox_index_command:}
    \group_end:
  }

\NewDocumentCommand \docAuxEnvironment { s +O{} m }
  {
    \group_begin:
    \tcbset{doc~name={#3},#2}
    \__tcobox_print_environment:
    \IfBooleanF{#1}{\__tcobox_index_environment:}
    \group_end:
  }


\NewDocumentCommand \docAuxKey { s O{} +O{} m }
  {
    \group_begin:
    \tcbset{doc~keypath={#2},doc~name={#4},#3}
    \__tcobox_print_key:
    \IfBooleanF{#1}{\__tcobox_index_key:}
    \group_end:
  }


\NewDocumentCommand \docValue { s +O{} m }
  {
    \group_begin:
    \tcbset{doc~name={#3},#2}
    \textcolor{\kvtcb@col@value}{\__tcobox_print_docname:}
    \IfBooleanF{#1}
      {
        \kvtcb@index@command{\kvtcb@doc@sortindex\idx@actual\tcbIndexPrintValCA{\kvtcb@doc@index}}
        \kvtcb@index@command{\kvtcb@text@values\idx@level\kvtcb@doc@sortindex\idx@actual\tcbIndexPrintValC{\kvtcb@doc@index}}
      }
    \group_end:
  }


\NewDocumentCommand \docColor { s +O{} m }
  {
    \group_begin:
    \tcbset{doc~name={#3},#2}
    \textcolor{\kvtcb@col@color}{\__tcobox_print_docname:}
    \IfBooleanF{#1}
      {
        \kvtcb@index@command{\kvtcb@doc@sortindex\idx@actual\tcbIndexPrintColCA{\kvtcb@doc@index}}
        \kvtcb@index@command{\kvtcb@text@colors\idx@level\kvtcb@doc@sortindex\idx@actual\tcbIndexPrintColC{\kvtcb@doc@index}}
      }
    \group_end:
  }


\NewDocumentCommand \docCounter { s +O{} m }
  {
    \group_begin:
    \tcbset{doc~name={#3},#2}
    \textcolor{\kvtcb@col@counter}{\__tcobox_print_docname:}
    \IfBooleanF{#1}
      {
        \kvtcb@index@command{\kvtcb@doc@sortindex\idx@actual\tcbIndexPrintCountCA{\kvtcb@doc@index}}
        \kvtcb@index@command{\kvtcb@text@counters\idx@level\kvtcb@doc@sortindex\idx@actual\tcbIndexPrintCountC{\kvtcb@doc@index}}
      }
    \group_end:
  }


\NewDocumentCommand \docLength { s +O{} m }
  {
    \group_begin:
    \tcbset{doc~name={#3},#2}
    \textcolor{\kvtcb@col@length}{\__tcobox_print_cs_docname:}
    \IfBooleanF{#1}
      {
        \kvtcb@index@command{\kvtcb@doc@sortindex\idx@actual\tcbIndexPrintLenCA{\kvtcb@doc@index}}
        \kvtcb@index@command{\kvtcb@text@lengths\idx@level\kvtcb@doc@sortindex\idx@actual\tcbIndexPrintLenC{\kvtcb@doc@index}}
      }
    \group_end:
  }


\ExplSyntaxOff


\setrefcountdefault{-1}
\NewDocumentCommand\tcb@ref@doc{msm}{%
  \hyperref[#1:#3]{\texttt{\ref*{#1:#3}}%
  \IfBooleanTF{#2}{}{%
    \ifnum\getpagerefnumber{#1:#3}=\thepage%
    \else%
      \textsuperscript{\ding{213}\,\kvtcb@text@pageshort\,\pageref*{#1:#3}}%
    \fi}}%
}

\def\refCom{\tcb@ref@doc{com}}
\def\refEnv{\tcb@ref@doc{env}}
\def\refKey{\tcb@ref@doc{key}}
\def\refPathOperation{\tcb@ref@doc{path}}

\AtBeginDocument{%
  \ifHy@colorlinks
    \def\refAux#1{\textcolor{\kvtcb@colhyper}{\tcb@scantokens{#1}}}%
    \def\refAuxcs#1{\textcolor{\kvtcb@colhyper}{\tcb@cs{#1}}}%
  \else
    \def\refAux#1{\tcb@scantokens{#1}}%
    \def\refAuxcs#1{\tcb@cs{#1}}%
  \fi%
}

\newenvironment{absquote}
               {\list{}{\leftmargin2cm\rightmargin\leftmargin}%
                \item\relax\footnotesize}
               {\endlist}

\newcommand{\tcbdocmarginnote}[2][]{%
  \marginnote{%
  \begin{tcolorbox}[enhanced jigsaw,size=fbox,boxrule=1pt,leftrule=0pt,rightrule=0pt,
    arc=0pt,outer arc=1pt,boxsep=1pt,top=1pt,bottom=1pt,
    nobeforeafter,width=\marginparwidth,
    colframe=red!50!white,colback=red!25!yellow!5!white,fontupper=\scriptsize,
    if odd page or oneside={flushright upper}{flushleft upper},
    doc@marginnote,#1]#2\end{tcolorbox}}}

\newcommand*{\tcbdocnew}[1]{\kvtcb@text@new: #1}
\newcommand*{\tcbdocupdated}[1]{\kvtcb@text@updated: #1}

%--- index macros taken from pgfmanual-en-macros
\def\tcb@doc@index@pgf@{%
  \ifdefined\c@IndexColumns%
    \c@IndexColumns=2%
  \fi%
  \def\theindex{\@restonecoltrue
    \columnseprule \z@  \columnsep 29\p@
    \twocolumn[\index@prologue]%
    \parindent -30pt%
    \columnsep 15pt%
    \parskip 0pt plus 1pt%
    \leftskip 30pt%
    \rightskip 0pt plus 2cm%
    \small%
    \def\@idxitem{\par}%
    \let\item\@idxitem\ignorespaces}
  \def\endtheindex{\onecolumn}%
  \def\noindexing{\let\index=\@gobble}%
}

\def\tcb@doc@index@pgfsection{%
  \def\index@prologue{\section*{\kvtcb@text@index}\addcontentsline{toc}{section}{\kvtcb@text@index}%
    \par\noindent%
  }%
  \tcb@doc@index@pgf@%
}

\def\tcb@doc@index@pgfchapter{%
  \def\index@prologue{\ifdefined\phantomsection\phantomsection\fi\@makeschapterhead{\kvtcb@text@index}\addcontentsline{toc}{chapter}{\kvtcb@text@index}}%
  \tcb@doc@index@pgf@%
}

\let\tcb@doc@index@pgf=\tcb@doc@index@pgfsection%

\def\tcb@doc@index@doc{%
  \ExplSyntaxOn
  \def \__tcobox_index_command:
  {
    \iftcb@doc@toindex
      \SpecialMainIndex{\kvtcb@doc@sortindex\idx@actual\tcbIndexPrintComC{\kvtcb@doc@index}}
    \fi
  }
  \def \__tcobox_index_environment:
  {
    \iftcb@doc@toindex
      SpecialMainEnvIndex{\kvtcb@doc@sortindex\idx@actual\tcbIndexPrintEnvC{\kvtcb@doc@index}}
    \fi
  }
  \ExplSyntaxOff
  \tcbset{index german settings}%
  \EnableCrossrefs%
  \PageIndex%
}

\def\tcb@doc@index@off{}%

\tcbset{%
  reset@documentation/.style={%
  },
  initialize@reset=reset@documentation,
  doc left=2em,
  doc right=0pt,
  doc left indent=-2em,
  doc right indent=0pt,
  doc head=,
  doc raster=,
  before doc body=,
  after doc body=,
  documentation listing style=tcbdocumentation,
  doc into index=true,
  doc marginnote=,
  color option=Option,
  color definition=Definition,
  color hyperlink=Hyperlink,
  color fade=Fade,
  index command=\index,%
  index format=pgf,
  index default settings,
  index colorize=false,
  index annotate=true,
  english language,
  keywords bold,
}

% deprecated
\tcbset{
  before example/.store in=\kvtcb@beforeexample,
  after example/.store in=\kvtcb@afterexample,
    before example=\par\smallskip,
    after example=,
}


==> tcbexternal.code.tex <==
%% The LaTeX package tcolorbox - version 4.30 (2020/04/28)
%% tcbexternal.code.tex: Code for externalization
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2020 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{4.30}

\tcbuselibrary{pro@cessing}

{
\catcode`\"=12
\xdef\tcbexternal@normal@dq{"}
\catcode`\"=13
\gdef\tcbexternal@activate@normal@dq{\let"=\tcbexternal@normal@dq}
}

\long\def\tcbifexternal#1#2{%
  \ifdefined\TCBEXTERNALINPUT%
    #1%
  \else%
    #2%
  \fi%
}

\tcbifexternal{%
  \def\tcbEXTERNALIZE{%
    \RequirePackage{incgraph}%
    \TCBEXTERNALPREAMBLE%
    \begin{document}%
    \begin{inctext}[border=\TCBEXTERNALSAFETY]%
    \input{\TCBEXTERNALINPUT}%
    \end{inctext}%
    \end{document}%
  }%
}{%
  \def\tcbEXTERNALIZE{%
    \tcbset{
      external/.cd,
      externalize/.is if=tcb@externalize,
      externalize=true,
    }%
  }%
}

\@onlypreamble\tcbEXTERNALIZE

\def\tcbexternal@setbasename#1{%
  \edef\tcbexternal@job@name{\expandonce{\tcbexternal@prefix}\expandonce{#1}}%
  \edef\tcbexternal@job@mdfive{\expandonce{\tcbexternal@job@name.md5}}%
  \edef\tcbexternal@job@source{\expandonce{\tcbexternal@job@name.tex}}%
  \edef\tcbexternal@job@pdf{\expandonce{\tcbexternal@job@name.pdf}}%
}

\def\tcbexternal@corecompile{%
  \begingroup%
  \ifnum\the\catcode`\"=13 \tcbexternal@activate@normal@dq\fi%
  \message{=== Compile external '\tcbexternal@job@name': }%
  \immediate\openout\tcb@out="\tcbexternal@run@tex"
  \immediate\write\tcb@out{\string\gdef\string\TCBEXTERNALINPUT{"\tcbexternal@job@source"}}%
  \immediate\write\tcb@out{\string\gdef\string\TCBEXTERNALSAFETY{\tcbexternal@safety}}%
  \immediate\write\tcb@out{\string\gdef\string\TCBEXTERNALPREAMBLE{\expandonce{\tcbexternal@preamble}}}%
  \ifdefempty{\tcbexternal@preclass}{}{\immediate\write\tcb@out{\expandonce{\tcbexternal@preclass}}}%
  \immediate\write\tcb@out{\string\input{"\jobname.tex"}}%
  \immediate\closeout\tcb@out%
  \foreach \n in {1,...,\tcbexternal@runs}
  {%
    \ShellEscape{%
      \tcbexternal@compiler\space
      -shell-escape
      -halt-on-error
      -interaction=batchmode
      -jobname="\tcbexternal@job@name"
      "\tcbexternal@run@tex"
    }%
  }%
  \endgroup%
}

\def\tcbexternal@compile#1{%
  \tcbiffileprocess{#1}%
    {\tcbexternal@job@source}{\tcbexternal@job@mdfive}{\tcbexternal@job@pdf}%
    {\tcbexternal@corecompile}{}%
}

\def\tcbexternal@inputsource{%
  \IfFileExists{\tcbexternal@job@source}%
    {\input{\tcbexternal@job@source}}%
    {\tcb@error{File '\tcbexternal@job@source' missing.}{}}%
}

\def\tcbexternal@pdfmissing@warning{%
  \tcb@warning{File '\tcbexternal@job@pdf' missing.
    Compilation error or shell-escape wasn't enabled or a subdirectory could'nt be generated}%
  \message{Load '\tcbexternal@job@source' instead}%
  \tcbexternal@inputsource%
}

\def\tcbexternal@pdfmissing@error{%
  \tcb@error{File '\tcbexternal@job@pdf' missing.
    Compilation error or shell-escape wasn't enabled or a subdirectory could'nt be generated}{}%
}

\def\tcbexternal@inputpdf{%
  \IfFileExists{\tcbexternal@job@pdf}%
    {%
      \begingroup\edef\x{\endgroup%
        \noexpand\includegraphics[trim=\tcbexternal@safety\space\tcbexternal@safety%
        \space\tcbexternal@safety\space\tcbexternal@safety]{\expandonce{\tcbexternal@job@pdf}}}%
      \x%
    }%
    {\tcbexternal@pdfmissing}%
}

\newif\iftcb@externalize
\tcb@externalizefalse

\def\tcb@useexternal{%
  \iftcb@externalize%
    \tcbexternal@compile{\tcbexternal@condition}%
    \tcbexternal@inputpdf%
  \else%
    \tcbexternal@compile{2}%
    \tcbexternal@inputsource%
  \fi%
}

\newenvironment{tcbexternal}[2][]{%
  \tcbset{external/.cd,#1,name=#2}%
  \@ifundefined{@tcbexternal@JN@\tcbexternal@job@name}{%
      \global\@namedef{@tcbexternal@JN@\tcbexternal@job@name}{}%
    }{%
      \tcb@error{External job name '\tcbexternal@job@name' already used}%
        {Give a new unique name to the current external job.}%
    }%
  \begingroup%
  \let\tcb@verbatim@begin@hook=\tcbexternal@out@begin%
  \let\tcb@verbatim@end@hook=\tcbexternal@out@end%
  \tcbverbatimwrite{\tcbexternal@job@source}}%
{%
  \endtcbverbatimwrite\endgroup%
  \tcb@useexternal%
}

\long\def\new@tcb@externalizeenvironment#1#2#3#4#5{%
  \tcb@newenvironment{#1}[2][]{%
    #4%
    \begingroup%
    \tcbexternal[#3,##1,environment=#2]{##2}%
  }{%
    \endtcbexternal%
    \endgroup%
    #5%
  }%
}

\def\newtcbexternalizeenvironment{%
  \let\tcb@newenvironment\newenvironment%
  \new@tcb@externalizeenvironment%
}

\def\renewtcbexternalizeenvironment{%
  \let\tcb@newenvironment\renewenvironment%
  \new@tcb@externalizeenvironment%
}

\long\def\new@tcb@externalizetcolorbox#1#2#3#4{%
  \new@tcb@externalizeenvironment{#1}{#2}%
    {preamble tcbset={force nobeforeafter},#3}%
    {\tcb@layer@pushup\tcb@apply@box@options{#4}\tcb@set@normal@unbroken@beforeafter\tcb@before@unbroken}%
    {\tcb@after@unbroken}%
}

\def\newtcbexternalizetcolorbox{%
  \let\tcb@newenvironment\newenvironment%
  \new@tcb@externalizetcolorbox%
}

\def\renewtcbexternalizetcolorbox{%
  \let\tcb@newenvironment\renewenvironment%
  \new@tcb@externalizetcolorbox%
}


\newtcbexternalizeenvironment{extikzpicture}{tikzpicture}{}{}{}

\newtcbexternalizetcolorbox{extcolorbox}{tcolorbox}{}{}


\tcbset{
  external/.cd,
  %
  runner/.code={%
    \edef\tcbexternal@run@tex{\expandonce{#1}}%
  },
  %
  prefix/.store in=\tcbexternal@prefix,
  compiler/.store in=\tcbexternal@compiler,
  runs/.code={\numdef\tcbexternal@runs{#1}},
  name/.code={\tcbexternal@setbasename{#1}},
  safety/.store in=\tcbexternal@safety,
  preamble/.code={\appto\tcbexternal@preamble{#1}},
  preamble tcbset/.code={\appto\tcbexternal@preamble{\tcbset{#1}}},
  clear preamble/.code={\def\tcbexternal@preamble{}},
  preclass/.code={\appto\tcbexternal@preclass{#1}},
  clear preclass/.code={\def\tcbexternal@preclass{}},
  PassOptionsToPackage/.code 2 args={\appto\tcbexternal@preclass{\PassOptionsToPackage{#1}{#2}}},
  PassOptionsToClass/.code 2 args={\appto\tcbexternal@preclass{\PassOptionsToClass{#1}{#2}}},
  externalize/.code={},
  -/.style={/tcb/external/externalize=false},
  %
  force remake/.is choice,
  force remake/true/.code={\def\tcbexternal@condition{0}},
  force remake/false/.code={\def\tcbexternal@condition{1}},
  force remake/.default=true,
  !/.style={/tcb/external/force remake},
  %
  input source on error/.is choice,
  input source on error/true/.code={\let\tcbexternal@pdfmissing=\tcbexternal@pdfmissing@warning},
  input source on error/false/.code={\let\tcbexternal@pdfmissing=\tcbexternal@pdfmissing@error},
  input source on error/.default=true,
  %
  plain/.code={%
    \let\tcbexternal@out@begin=\@empty%
    \let\tcbexternal@out@end=\@empty%
  },
  minipage/.code={%
    \appto\tcbexternal@out@begin{\immediate\write\tcb@out{\string\begin{minipage}{\the\dimexpr#1\relax}\string\ignorespaces\@percentchar}}%
    \preto\tcbexternal@out@end{\immediate\write\tcb@out{\string\end{minipage}\@percentchar}}%
  },
  minipage/.default=\linewidth,
  %
  environment with percent/.is choice,
  environment with percent/true/.style={%
    /tcb/external/environment/.code={%
      \appto\tcbexternal@out@begin{\immediate\write\tcb@out{\string\begin{##1}\@percentchar}}%
      \preto\tcbexternal@out@end{\immediate\write\tcb@out{\string\end{##1}\@percentchar}}%
    }
  },
  environment with percent/false/.style={%
    /tcb/external/environment/.code={%
      \appto\tcbexternal@out@begin{\immediate\write\tcb@out{\string\begin{##1}}}%
      \preto\tcbexternal@out@end{\immediate\write\tcb@out{\string\end{##1}}}%
    }
  },
  environment with percent/.default=true,
  %
  runner=\jobname_run.tex,
  prefix={external/},
  compiler=pdflatex,
  runs=1,
  name=unnamed,
  safety=2mm,
  clear preamble,
  clear preclass,
  force remake=false,
  input source on error,
  environment with percent,
  plain
}

\tcbset{%
  externalize example/.style={%
    external/name=#1,tempfile=\tcbexternal@job@source,
    code={\let\tcbusetemp=\tcb@useexternal}%
  },
  externalize example!/.style={externalize example=#1,external/force remake},
  externalize listing/.style={%
    external/name=#1,listing file=\tcbexternal@job@source,
    code={\let\tcbuselistingtext@input=\tcb@useexternal}%
  },
  externalize listing!/.style={externalize listing=#1,external/force remake},
}


==> tcbfitting.code.tex <==
%% The LaTeX package tcolorbox - version 4.30 (2020/04/28)
%% tcbfitting.code.tex: Code for fit boxes
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2020 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{4.30}

\newdimen\tcbfitdim
\newdimen\tcb@lowerfitdim
\newdimen\tcb@upperfitdim
\newif\iftcb@continue

\tcbset{%
  fit/.style={capture=fitbox},%
  fit to/.style args={#1 and #2}{capture=fitbox,width=#1,height=#2},%
  fit to height/.style={capture=fitbox,height=#1},%
  fit basedim/.code={\def\kvtcb@fit@basedim{#1}\tcbfitdim\kvtcb@fit@basedim},%
  fit skip/.store in=\kvtcb@fit@skip,%
  fit fontsize macros/.code={%
    \renewcommand\tiny{\tcb@setfontsize\tiny{0.5}}%
    \renewcommand\scriptsize{\tcb@setfontsize\scriptsize{0.7}}%
    \renewcommand\footnotesize{\tcb@setfontsize\footnotesize{0.8}}%
    \renewcommand\small{\tcb@setfontsize\small{0.9}}%
    \renewcommand\normalsize{\tcb@setfontsize\normalsize{1}}%
    \renewcommand\large{\tcb@setfontsize\large{1.2}}%
    \renewcommand\Large{\tcb@setfontsize\Large{1.44}}%
    \renewcommand\LARGE{\tcb@setfontsize\LARGE{1.728}}%
    \renewcommand\huge{\tcb@setfontsize\huge{2.0736}}%
    \renewcommand\Huge{\tcb@setfontsize\Huge{2.48832}}},%
  fit height plus/.style={fit,height plus=#1},%
  fit width plus/.dimstore in=\kvtcb@fit@plus@width,%
  fit height from/.style args={#1 to #2}{fit,height from={#1} to {#2}},
  fit width from/.style args={#1 to #2}{fit,width={#1},fit width plus={#2-#1}},
  fit maxstep/.store in=\kvtcb@fit@maxstep,%
  fit maxfontdiff/.store in=\kvtcb@fit@maxfontdiff,%
  fit maxfontdiffgap/.store in=\kvtcb@fit@maxfontdiffgap,%
  fit maxwidthdiff/.store in=\kvtcb@fit@maxwidthdiff,%
  fit maxwidthdiffgap/.store in=\kvtcb@fit@maxwidthdiffgap,%
  fit warning/.is choice,
  fit warning/on/.code={\let\tcb@fit@warn@begin=\@empty%
    \let\tcb@fit@warn@end=\@empty},
  fit warning/off/.code={\def\tcb@fit@warn@begin{\hbadness=10000\relax}%
    \let\tcb@fit@warn@end=\@empty},
  fit warning/final/.code={\tcb@cur@hbadness=\hbadness\def\tcb@fit@warn@begin{\hbadness=10000\relax}%
    \def\tcb@fit@warn@end{\hbadness=\tcb@cur@hbadness\relax\tcb@fit@@box}},
  fit algorithm/.is choice,
  fit algorithm/fontsize/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@fontsize},
  fit algorithm/fontsize*/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@fontsize@star},
  fit algorithm/areasize/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@areasize},
  fit algorithm/areasize*/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@areasize@star},
  fit algorithm/hybrid/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@hybrid},
  fit algorithm/hybrid*/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@hybrid@star},
  fit algorithm/squeeze/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@squeeze},
  spartan@fit/.style={fit algorithm=squeeze},
}

\def\tcb@@capture@fitbox{%
  \let\endtcolorbox=\relax%
  \Collect@Body\tcbox@inner@fitbox@collected%
}

\def\tcbfontsize#1{\fontsize{#1\tcbfitdim}{#1\dimexpr\kvtcb@fit@skip\tcbfitdim}\selectfont}

\def\tcb@setfontsize#1#2{\@setfontsize#1{#2\tcbfitdim}{#2\dimexpr\kvtcb@fit@skip\tcbfitdim}}

\long\def\tcbox@inner@fitbox@collected#1{%
  \tcbox@inner@fitbox{#1}%
  \tcb@finalize@environment%
}

\newcount\tcb@cur@hbadness

\def\tcbox@fitalgorithm@fontsize{%
  \tcb@continuetrue%
  \loop%
    \tcbfitdim.5\tcbfitdim%
    \tcb@fit@@box%
    \ifnum\count@=\kvtcb@fit@maxstep\relax%
      \tcb@continuefalse%
    \else%
      \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
        \ifdim\tcbfitdim<18000sp\relax%
          \count@\kvtcb@fit@maxstep\relax%
          \tcb@continuefalse%
        \fi%
      \else%
        \tcb@continuefalse%
      \fi%
    \fi%
  \iftcb@continue \repeat%
  \ifnum\count@<\kvtcb@fit@maxstep\relax%
    \tcbdimto\tcb@fit@@gap{\tcb@fit@@target-\tcb@fit@@h}%
    \tcb@lowerfitdim\tcbfitdim%
    \tcb@upperfitdim2\tcbfitdim%
    \tcbfitdim1.5\tcbfitdim%
    \loop%
      \tcb@fit@@box%
      \tcb@continuetrue%
      \ifnum\count@<\kvtcb@fit@maxstep\relax%
        \ifdim\dimexpr\tcb@upperfitdim-\tcb@lowerfitdim<\kvtcb@fit@maxfontdiff\relax%
          \tcb@continuefalse%
        \else%
          \ifdim\dimexpr\tcb@upperfitdim-\tcb@lowerfitdim<\kvtcb@fit@maxfontdiffgap\relax%
            \ifdim\dimexpr\tcb@fit@@gap<\tcb@fit@@line\relax%
              \tcb@continuefalse%
            \fi%
          \fi%
        \fi%
      \else%
        \tcb@continuefalse%
      \fi%
      \iftcb@continue%
        \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
          \tcb@upperfitdim\tcbfitdim%
          \advance\tcbfitdim\tcb@lowerfitdim%
          \tcbfitdim0.5\tcbfitdim%
        \else%
          \tcbdimto\tcb@fit@@gap{\tcb@fit@@target-\tcb@fit@@h}%
          \tcb@lowerfitdim\tcbfitdim%
          \advance\tcbfitdim\tcb@upperfitdim%
          \tcbfitdim0.5\tcbfitdim%
        \fi%
      \else%
        \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
          \tcbfitdim\tcb@lowerfitdim%
          \tcb@fit@@box%
        \fi%
      \fi%
    \iftcb@continue \repeat%
  \fi%
}

\def\tcbox@fitalgorithm@fontsize@star{%
  \tcbox@fitalgorithm@fontsize%
  \tcb@resize@box{\tcb@upperbox}{\tcb@w@upper}{\tcb@fit@@target}%
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@areasize@core{%
  \pgfmathdivide{\tcb@fit@@h}{\tcb@fit@@target}%
  \pgfmathsqrt{\pgfmathresult}%
  \let\tcb@temp=\pgfmathresult%
  \tcbdimto\tcb@w@upper@temp{\pgfmathresult\dimexpr\tcb@w@upper}%
  \tcb@fit@@boxsave{\tcb@w@upper@temp}%
  %
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
  \pgfmathdivide{\tcb@fit@@h}{\tcb@fit@@target}%
  \pgfmathdivide{\pgfmathresult}{\tcb@temp}%
  \pgfmathsqrt{\pgfmathresult}%
  \ifdim\dimexpr\pgfmathresult pt<0.98pt\relax
    \tcbdimto\tcb@w@upper@temp{\pgfmathresult\dimexpr\tcb@w@upper@temp}%
    \tcb@fit@@boxsave{\tcb@w@upper@temp}%
  \else\ifdim\dimexpr\pgfmathresult pt>1.02pt\relax
    \tcbdimto\tcb@w@upper@temp{\pgfmathresult\dimexpr\tcb@w@upper@temp}%
    \tcb@fit@@boxsave{\tcb@w@upper@temp}%
  \fi\fi%
  %
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@areasize{%
  \tcbox@fitalgorithm@areasize@core%
  \pgfmathdivide{\tcb@w@upper}{\tcb@w@upper@temp}%
  \tcbdimto\tcb@fit@@h{\pgfmathresult\dimexpr\tcb@fit@@h}%
  \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
    \let\tcb@fit@@h=\tcb@fit@@target%
  \fi
  \tcb@resize@box{\tcb@upperbox}{\tcb@w@upper}{\tcb@fit@@h}%
  %
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@areasize@star{%
  \tcbox@fitalgorithm@areasize@core%
  \tcb@resize@box{\tcb@upperbox}{\tcb@w@upper}{\tcb@fit@@target}%
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@squeeze{%
  \tcb@resize@box{\tcb@upperbox}{\tcb@w@upper}{\tcb@fit@@target}%
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@hybrid@core{%
  \pgfmathdivide{\tcb@fit@@target}{\tcb@fit@@h}%
  \pgfmathsqrt{\pgfmathresult}%
  \tcbfitdim=\pgfmathresult\tcbfitdim%
  \tcb@fit@@box%
  %
  \pgfmathdivide{\tcb@fit@@target}{\tcb@fit@@h}%
  \pgfmathsqrt{\pgfmathresult}%
  \ifdim\dimexpr\pgfmathresult pt<0.85pt\relax
    \tcbfitdim=\pgfmathresult\tcbfitdim%
    \tcb@fit@@box%
  \else\ifdim\dimexpr\pgfmathresult pt>1.15pt\relax
    \tcbfitdim=\pgfmathresult\tcbfitdim%
    \tcb@fit@@box%
  \fi\fi%
}

\def\tcbox@fitalgorithm@hybrid{%
  \tcbox@fitalgorithm@hybrid@core%
  \tcbox@fitalgorithm@areasize%
}

\def\tcbox@fitalgorithm@hybrid@star{%
  \tcbox@fitalgorithm@hybrid@core%
  \tcbox@fitalgorithm@areasize@star%
}

\def\tcb@fit@@box{%
  \iftcb@hasTitle%
    \tcbdimto\tcb@w@title{\kvtcb@width-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@lefttitle)-(\kvtcb@righttitle)}%
    \begin{tcb@savebox}{\tcb@titlebox}{\tcb@w@title}\color{tcbcoltitle}\kvtcb@fonttitle\kvtcb@haligntitle\kvtcb@before@title\kvtcb@title\kvtcb@after@title\end{tcb@savebox}%
    \tcbdimto\tcb@h@titletotal{\ht\tcb@titlebox+\dp\tcb@titlebox+\kvtcb@title@rule+(\kvtcb@boxsep)*2+\kvtcb@toptitle+\kvtcb@bottomtitle}%
  \else%
    \let\tcb@h@titletotal=\tcb@zpt%
  \fi%
  \tcbdimto\tcb@fit@@line{\kvtcb@fit@skip\tcbfitdim}%
  \tcbdimto\tcb@w@upper{\kvtcb@width-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@leftupper)-(\kvtcb@rightupper)}%
  \tcb@fit@@boxsave{\tcb@w@upper}%
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
  \tcbdimto\tcb@fit@@target{\kvtcb@height@fixed-(\kvtcb@top@rule@stand)-(\kvtcb@bottom@rule@stand)-(\kvtcb@top)-(\kvtcb@bottom)-(\kvtcb@boxsep)*2-\tcb@h@titletotal}%
}%

\long\def\tcbox@inner@fitbox#1{%
  \tcbset{breakable@false,sidebyside=false}%
  \let\tcb@space\tcb@zpt%
  \let\tcb@val@raisebase=\tcb@zpt%
  \unless\ifdefined\kvtcb@height@fixed%
    \tcbset{height=\kvtcb@width}%
  \fi%
  \tcb@hasLowerfalse%
  %
  \count@\z@%
  \tcbfitdim\kvtcb@fit@basedim%
  \tcb@fit@warn@begin%
  %
  \def\tcb@fit@@boxsave##1{%
    \tcbdimto\tcb@innerwidth{\kvtcb@width-\kvtcb@left@rule-\kvtcb@right@rule}%
    \colorlet{tcbcol@origin}{.}%
    \tcb@set@color{tcbcolupper}%
    \begin{tcb@savebox}{\tcb@upperbox}{##1}%
      \kvtcb@fontupper\fontsize{\tcbfitdim}{\tcb@fit@@line}\selectfont%
      \kvtcb@halignupper\tcb@insert@before@upper#1\tcb@insert@after@upper%
    \end{tcb@savebox}%
    \tcb@reset@color%
    \advance\count@ 1\relax%
  }%
  %
  \tcb@set@@phantom%
  \tcb@set@@title%
  \tcb@fit@@box%
  %
  % height fit
  \ifdim\kvtcb@height@fixed@plus>0pt\relax%
    \let\tcb@fit@@minheight=\kvtcb@height@fixed%
    \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
      \ifdim\dimexpr\tcb@fit@@h>\dimexpr\tcb@fit@@target+\kvtcb@height@fixed@plus\relax%
        \tcbdimto\kvtcb@height@fixed{\kvtcb@height@fixed+\kvtcb@height@fixed@plus}%
        \tcbdimto\tcb@fit@@target{\tcb@fit@@target+\kvtcb@height@fixed@plus}%
      \else%
        \tcbdimto\kvtcb@height@fixed{\kvtcb@height@fixed+\tcb@fit@@h-\tcb@fit@@target}%
        \let\tcb@fit@@target=\tcb@fit@@h%
      \fi%
    \fi%
  \fi%
  %
  % width fit
  \ifdim\kvtcb@fit@plus@width>0pt\relax%
    \ifnum\count@<\kvtcb@fit@maxstep\relax%
      \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
        \tcb@lowerfitdim\dimexpr\kvtcb@width\relax%
        \tcb@upperfitdim\dimexpr\kvtcb@width+\kvtcb@fit@plus@width\relax%
        \tcbdimto\kvtcb@width{\tcb@upperfitdim}%
        \tcb@fit@@box%
        \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
        \else%
          \ifnum\count@<\kvtcb@fit@maxstep\relax%
            \tcbdimto\tcb@fit@@gap{\tcb@fit@@target-\tcb@fit@@h}%
            \tcbdimto\kvtcb@width{(\tcb@lowerfitdim+\tcb@upperfitdim)/2}%
            \loop%
              \tcb@fit@@box%
              \tcb@continuetrue%
              \ifnum\count@<\kvtcb@fit@maxstep\relax%
                \ifdim\dimexpr\tcb@upperfitdim-\tcb@lowerfitdim<\kvtcb@fit@maxwidthdiff\relax%
                  \tcb@continuefalse%
                \else%
                  \ifdim\dimexpr\tcb@upperfitdim-\tcb@lowerfitdim<\kvtcb@fit@maxwidthdiffgap\relax%
                    \ifdim\dimexpr\tcb@fit@@gap<\tcb@fit@@line\relax%
                      \tcb@continuefalse%
                    \fi%
                  \fi%
                \fi%
              \else%
                \tcb@continuefalse%
              \fi%
              \iftcb@continue%
                \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
                  \tcb@lowerfitdim\dimexpr\kvtcb@width\relax%
                  \tcbdimto\kvtcb@width{(\tcb@lowerfitdim+\tcb@upperfitdim)/2}%
                \else%
                  \tcb@upperfitdim\dimexpr\kvtcb@width\relax%
                  \tcbdimto\tcb@fit@@gap{\tcb@fit@@target-\tcb@fit@@h}%
                  \tcbdimto\kvtcb@width{(\tcb@lowerfitdim+\tcb@upperfitdim)/2}%
                \fi%
              \else%
                \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
                  \tcbdimto\kvtcb@width{\tcb@upperfitdim}%
                  \tcb@fit@@box%
                \fi%
              \fi%
            \iftcb@continue \repeat%
          \fi%
        \fi%
      \fi%
    \fi%
  \fi%
  %
  % (font) fit
  \ifnum\count@<\kvtcb@fit@maxstep\relax%
    \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
    \tcbox@fitalgorithm%
    \fi%
  \fi%
  %
  \tcb@fit@warn@end%
  %
  % last height fit
  \ifdim\kvtcb@height@fixed@plus>0pt\relax%
    \ifdim\dimexpr\tcb@fit@@h<\tcb@fit@@target\relax%
      \tcbdimto\tcb@temp{\kvtcb@height@fixed+\tcb@fit@@h-\tcb@fit@@target}%
      \ifdim\dimexpr\tcb@temp<\tcb@fit@@minheight\relax%
      \else%
        \let\kvtcb@height@fixed=\tcb@temp%
      \fi%
    \fi%
  \fi%
  %
  \edef\tcbfitsteps{\the\count@}%
  \tcb@set@@dimensions%
  \tcb@draw@color@box%
}

\newcommand{\tcboxfit}[2][]{%
  \tcb@ox{capture=fitbox,#1}{#2}%
}

\long\def\tcb@newtcboxfit#1#2{\expandafter\tcb@newcommand\csname#1\endcsname{\tcboxfit[#2,options@for=#1]}}

\long\def\tcb@newtcboxfit@#1[#2]#3{\expandafter\tcb@newcommand\csname#1\endcsname[#2]{\tcboxfit[#3,options@for=#1]}}

\long\def\tcb@newtcboxfit@@#1[#2][#3]#4{\expandafter\tcb@newcommand\csname#1\endcsname[#2][#3]{\tcboxfit[#4,options@for=#1]}}

\long\def\tcb@new@tcboxfit@#1[#2]{%
  \@ifnextchar[{\tcb@newtcboxfit@@{#1}[#2]}{\tcb@newtcboxfit@{#1}[#2]}}

\long\def\tcb@new@tcboxfit#1{%
  \@ifnextchar[{\tcb@new@tcboxfit@{#1}}{\tcb@newtcboxfit{#1}}}

\def\newtcboxfit{%
  \let\tcb@newcommand\newcommand%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcboxfit%
  \tcb@process@newcommand}

\def\renewtcboxfit{%
  \let\tcb@newcommand\renewcommand%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcboxfit%
  \tcb@process@newcommand}

\tcbset{%
  reset@fitting/.style={%
    fit algorithm=fontsize,%
    fit basedim=10pt,fit skip=1.2,
    height plus=0pt,fit width plus=0pt,
    fit maxstep=20,fit maxfontdiff=0.1pt,fit maxfontdiffgap=1pt,
    fit maxwidthdiff=1pt,fit maxwidthdiffgap=10pt,
    fit warning=off
  },
  initialize@reset=reset@fitting,
}



==> tcbhooks.code.tex <==
%% The LaTeX package tcolorbox - version 4.30 (2020/04/28)
%% tcbhooks.code.tex: Code for adding hooks
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2020 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{4.30}

\tcbset{%
  before upper app/.code={\appto\kvtcb@before@upper{#1}},%
  before upper pre/.code={\preto\kvtcb@before@upper{#1}},%
  after upper app/.code={\appto\kvtcb@after@upper{#1}},%
  after upper pre/.code={\preto\kvtcb@after@upper{#1}},%
  before lower app/.code={\appto\kvtcb@before@lower{#1}},%
  before lower pre/.code={\preto\kvtcb@before@lower{#1}},%
  after lower app/.code={\appto\kvtcb@after@lower{#1}},%
  after lower pre/.code={\preto\kvtcb@after@lower{#1}},%
  before title app/.code={\appto\kvtcb@before@title{#1}},%
  before title pre/.code={\preto\kvtcb@before@title{#1}},%
  after title app/.code={\appto\kvtcb@after@title{#1}},%
  after title pre/.code={\preto\kvtcb@after@title{#1}},%
  %
  % usable inside the document or in the preamble after setting before / after
  before app/.code={\appto\kvtcb@beforebox{#1}},%
  before pre/.code={\preto\kvtcb@beforebox{#1}},%
  after app/.code={\appto\kvtcb@afterbox{#1}},%
  after pre/.code={\preto\kvtcb@afterbox{#1}},%
  %
  overlay unbroken app/.code={\appto\tcb@overlay@unbroken{#1}},%
  overlay unbroken pre/.code={\preto\tcb@overlay@unbroken{#1}},%
  overlay first app/.code={\appto\tcb@overlay@first{#1}},%
  overlay first pre/.code={\preto\tcb@overlay@first{#1}},%
  overlay middle app/.code={\appto\tcb@overlay@middle{#1}},%
  overlay middle pre/.code={\preto\tcb@overlay@middle{#1}},%
  overlay last app/.code={\appto\tcb@overlay@last{#1}},%
  overlay last pre/.code={\preto\tcb@overlay@last{#1}},%
  %
  overlay app/.style={overlay unbroken app={#1},overlay first app={#1},overlay middle app={#1},overlay last app={#1}},%
  overlay pre/.style={overlay unbroken pre={#1},overlay first pre={#1},overlay middle pre={#1},overlay last pre={#1}},%
  overlay broken app/.style={overlay first app={#1},overlay middle app={#1},overlay last app={#1}},%
  overlay broken pre/.style={overlay first pre={#1},overlay middle pre={#1},overlay last pre={#1}},%
  overlay unbroken and first app/.style={overlay unbroken app={#1},overlay first app={#1}},%
  overlay unbroken and first pre/.style={overlay unbroken pre={#1},overlay first pre={#1}},%
  overlay unbroken and last app/.style={overlay unbroken app={#1},overlay last app={#1}},%
  overlay unbroken and last pre/.style={overlay unbroken pre={#1},overlay last pre={#1}},%
  overlay middle and last app/.style={overlay middle app={#1},overlay last app={#1}},%
  overlay middle and last pre/.style={overlay middle pre={#1},overlay last pre={#1}},%
  overlay first and middle app/.style={overlay first app={#1},overlay middle app={#1}},%
  overlay first and middle pre/.style={overlay first pre={#1},overlay middle pre={#1}},%
  %
  % skins:
  frame code app/.code={\appto\tcb@frame@code{#1}},%
  frame code pre/.code={\preto\tcb@frame@code{#1}},%
  interior titled code app/.code={\appto\tcb@interiortitled@code{#1}},%
  interior titled code pre/.code={\preto\tcb@interiortitled@code{#1}},%
  interior code app/.code={\appto\tcb@interior@code{#1}},%
  interior code pre/.code={\preto\tcb@interior@code{#1}},%
  segmentation code app/.code={\appto\tcb@segmentation@code{#1}},%
  segmentation code pre/.code={\preto\tcb@segmentation@code{#1}},%
  title code app/.code={\appto\tcb@title@code{#1}},%
  title code pre/.code={\preto\tcb@title@code{#1}},%
  %
  extras unbroken pre/.code={\preto\tcb@extras@unbroken{\tcbset{#1}}},%
  extras first pre/.code={\preto\tcb@extras@first{\tcbset{#1}}},%
  extras middle pre/.code={\preto\tcb@extras@middle{\tcbset{#1}}},%
  extras last pre/.code={\preto\tcb@extras@last{\tcbset{#1}}},%
  extras pre/.style={extras unbroken pre={#1},extras first pre={#1},extras middle pre={#1},extras last pre={#1}},%
  extras broken pre/.style={extras first pre={#1},extras middle pre={#1},extras last pre={#1}},%
  extras unbroken and first pre/.style={extras unbroken pre={#1},extras first pre={#1}},%
  extras unbroken and last pre/.style={extras unbroken pre={#1},extras last pre={#1}},%
  extras middle and last pre/.style={extras middle pre={#1},extras last pre={#1}},%
  extras first and middle pre/.style={extras first pre={#1},extras middle pre={#1}},%
  %
  underlay unbroken pre/.code={\preto\tcb@underlay@unbroken{#1}},%
  underlay first pre/.code={\preto\tcb@underlay@first{#1}},%
  underlay middle pre/.code={\preto\tcb@underlay@middle{#1}},%
  underlay last pre/.code={\preto\tcb@underlay@last{#1}},%
  underlay boxed title pre/.code={\preto\tcb@underlay@boxedtitle{#1}},%
  underlay pre/.style={underlay unbroken pre={#1},underlay first pre={#1},underlay middle pre={#1},underlay last pre={#1}},%
  underlay broken pre/.style={underlay first pre={#1},underlay middle pre={#1},underlay last pre={#1}},%
  underlay unbroken and first pre/.style={underlay unbroken pre={#1},underlay first pre={#1}},%
  underlay unbroken and last pre/.style={underlay unbroken pre={#1},underlay last pre={#1}},%
  underlay middle and last pre/.style={underlay middle pre={#1},underlay last pre={#1}},%
  underlay first and middle pre/.style={underlay first pre={#1},underlay middle pre={#1}},%
  finish unbroken pre/.code={\preto\tcb@finish@unbroken{#1}},%
  finish first pre/.code={\preto\tcb@finish@first{#1}},%
  finish middle pre/.code={\preto\tcb@finish@middle{#1}},%
  finish last pre/.code={\preto\tcb@finish@last{#1}},%
  finish pre/.style={finish unbroken pre={#1},finish first pre={#1},finish middle pre={#1},finish last pre={#1}},%
  finish broken pre/.style={finish first pre={#1},finish middle pre={#1},finish last pre={#1}},%
  finish unbroken and first pre/.style={finish unbroken pre={#1},finish first pre={#1}},%
  finish unbroken and last pre/.style={finish unbroken pre={#1},finish last pre={#1}},%
  finish middle and last pre/.style={finish middle pre={#1},finish last pre={#1}},%
  finish first and middle pre/.style={finish first pre={#1},finish middle pre={#1}},%
  %
  watermark tikz app/.style={overlay app={\tcb@drawspec@watermark@tikz{#1}}},
  watermark tikz pre/.style={overlay pre={\tcb@drawspec@watermark@tikz{#1}}},
  watermark tikz app on/.style args={#1 is #2}{overlay #1 app={\tcb@drawspec@watermark@tikz{#2}}},%
  watermark tikz pre on/.style args={#1 is #2}{overlay #1 pre={\tcb@drawspec@watermark@tikz{#2}}},%
  watermark graphics app/.style={overlay app={\tcb@drawspec@watermark@graphics{#1}}},
  watermark graphics pre/.style={overlay pre={\tcb@drawspec@watermark@graphics{#1}}},
  watermark graphics app on/.style args={#1 is #2}{overlay #1 app={\tcb@drawspec@watermark@graphics{#2}}},
  watermark graphics pre on/.style args={#1 is #2}{overlay #1 pre={\tcb@drawspec@watermark@graphics{#2}}},
  watermark text app/.style={overlay app={\tcb@drawspec@watermark@text{#1}}},
  watermark text pre/.style={overlay pre={\tcb@drawspec@watermark@text{#1}}},
  watermark text app on/.style args={#1 is #2}{overlay #1 app={\tcb@drawspec@watermark@text{#2}}},
  watermark text pre on/.style args={#1 is #2}{overlay #1 pre={\tcb@drawspec@watermark@text{#2}}},
  %
  minted options app/.code={\appto\kvtcb@minted@options{,#1}},
  minted options pre/.code={\preto\kvtcb@minted@options{#1,}},
  listing options app/.code={\appto\kvtcb@listingoptions{,#1}},
  listing options pre/.code={\preto\kvtcb@listingoptions{#1,}},
}



==> tcblistings.code.tex <==
%% The LaTeX package tcolorbox - version 4.30 (2020/04/28)
%% tcblistings.code.tex: Code for colorboxes with listings
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2020 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{4.30}

\RequirePackage{listings}[2007/02/22]

\tcbuselibrary{listings@core}

\let\tcb@listing@MakeCaption@org=\lst@MakeCaption

\def\tcb@listing@set@MakeCaption@org{%
  \let\lst@MakeCaption\tcb@listing@MakeCaption@org}
\def\tcb@listing@set@MakeCaption@empty{%
  \lst@HRefStepCounter{lstlisting}%
  \let\lst@MakeCaption\@gobble}

\lstdefinestyle{tcblatex}{language={[LaTeX]TeX},
     aboveskip={0\p@ \@plus 6\p@}, belowskip={0\p@ \@plus 6\p@},
     columns=fullflexible, keepspaces=true,
     breaklines=true, breakatwhitespace=true,
     basicstyle=\ttfamily\small, extendedchars=true, nolol,
     inputencoding=\kvtcb@listingencoding}

\def\tcb@listing@input@listing#1#2{%
  \begingroup%
  \toks@=\expandafter{#1}%
  \edef\tcb@temp{\noexpand\lstinputlisting[nolol,\the\toks@]}%
  \tcb@listing@set@MakeCaption%
  \tcb@temp{#2}%
  \endgroup%
}%


\def\tcb@listing@uselistinglisting{%
  \tcb@listing@input@listing{\kvtcb@listingoptions}{\kvtcb@listingfile}%
}%

\def\tcb@listing@usetemplisting{%
  \tcb@listing@input@listing{\kvtcb@listingoptions}{\kvtcb@tempfile}%
}%

\def\tcb@listing@doc@usetemplisting{%
  \tcb@listing@input@listing{\kvtcb@doclistingoptions}{\kvtcb@tempfile}%
}

\tcbset{%
  listing options/.store in=\kvtcb@listingoptions,%
  listing style/.style={listing options={style=#1}},%
  no listing options/.style={listing options=},%
  listing inputencoding/.store in=\kvtcb@listingencoding,%
  listing remove caption/.is choice,
  listing remove caption/true/.code={\let\tcb@listing@set@MakeCaption\tcb@listing@set@MakeCaption@empty},
  listing remove caption/false/.code={\let\tcb@listing@set@MakeCaption\tcb@listing@set@MakeCaption@org},
  listing remove caption/.default=true,
  listing engine/listings/.code={\let\tcbuselistinglisting\tcb@listing@uselistinglisting%
    \let\tcbusetemplisting\tcb@listing@usetemplisting%
    \let\tcb@doc@usetemplisting\tcb@listing@doc@usetemplisting},
  every listing line/.code={%
    \def\lst@NewLine{%
      \ifx\lst@OutputBox\@gobble\else
          \par\noindent \hbox{}#1%
      \fi
      \global\advance\lst@newlines\m@ne
      \lst@newlinetrue}},%
  every listing line*/.style={every listing line={#1},%
    code={\setbox\z@=\hbox{#1}\tcbdimto\kvtcb@rightupper{\kvtcb@rightupper+\wd\z@}}},%
}


\tcbset{%
  reset@listings/.style={%
    listing style=tcblatex,
    listing inputencoding=\inputencodingname,
    listing remove caption,
    listing engine=listings,
  },
  initialize@reset=reset@listings,
}



==> tcblistingscore.code.tex <==
%% The LaTeX package tcolorbox - version 4.30 (2020/04/28)
%% tcblistingscode.code.tex: Auxiliary code for colorboxes with listings
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2020 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{4.30}

\tcbuselibrary{pro@cessing}

\def\tcbuselistingtext@input{\input{\kvtcb@listingfile}}%
\def\tcbuselistingtext{\tcbuselistingtext@input}%
\def\tcbuselistingcomment{\kvtcb@listingcomment}%
\def\tcb@listing@listing{\tcbuselistinglisting}

\def\tcb@listing@listingAndOther{%
   \tcbuselistinglisting%
   \tcblower%
   \tcb@use@listing@other%
}

\def\tcb@listing@otherAndListing{%
   \tcb@use@listing@other%
   \tcblower%
   \tcbuselistinglisting%
}

\newenvironment{tcb@lower@outside}[1]{%
  \tcbset{savedelimiter=tcb@lower@outside}\tcb@minipage{#1}%
  \color{tcbcollower}\kvtcb@fontlower\kvtcb@halignlower\tcb@insert@before@lower}%
  {\tcb@insert@after@lower\endminipage}

\def\tcb@use@listing@other@reset{%
  \tcbset{every box on layer 1/.style={reset,every box}}%
  \tcb@use@listing@other}

\def\tcb@use@lower@outside#1{%
  \setbox\z@=\hbox{\begin{tcb@lower@outside}{#1}%
    \tcb@use@listing@other@reset%
  \end{tcb@lower@outside}}%
  \tcbdimto{\tcb@temp@wd}{\wd\z@}%
  \unhbox\z@%
}

\def\tcb@inputlisting@out@otherAboveListing{%
  {\kvtcb@beforebox}\noindent%
  \iftcb@lowervisible%
    \tcb@use@lower@outside{\kvtcb@width}%
    \par\vskip-\parskip\vspace*{\kvtcb@middle}\noindent%
  \fi%
  \begin{tcolorbox}[before=,savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
}

\def\tcb@inputlisting@out@otherAboveListing@Decoupled{%
  \iftcb@lowervisible%
    {\par\tcb@use@listing@other@reset\par}%
  \fi%
  \begin{tcolorbox}[savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
}

\def\tcb@inputlisting@out@listingAboveOther{%
  \begin{tcolorbox}[after=,savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
  \iftcb@lowervisible\par\vskip-\parskip\vspace*{\kvtcb@middle}\noindent%
    \tcb@use@lower@outside{\kvtcb@width}%
  \fi%
  {\kvtcb@afterbox}%
}

\def\tcb@inputlisting@out@listingAboveOther@Decoupled{%
  \begin{tcolorbox}[savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
  \iftcb@lowervisible%
    {\par\tcb@use@listing@other@reset\par}%
  \fi%
}


\newenvironment{tcb@outside@environment}{%
  \tcb@before@unbroken%
  \begin{minipage}{\tcb@width}}%
{%
  \end{minipage}%
  \tcb@after@unbroken}

\def\tcb@inputlisting@out@prepare{%
  \tcbdimto\tcb@width{\kvtcb@width}%
  \tcbdimto\tcb@innerwidth{\tcb@width-\kvtcb@left@rule-\kvtcb@right@rule}%
  \tcbdimto\tcb@temp{\tcb@innerwidth-\kvtcb@boxsep*2}%
  \tcbdimto\tcb@w@upper{\tcb@temp-\kvtcb@leftupper-\kvtcb@rightupper}%
  \tcbset{breakable@false}%
  \def\tcb@minipage{\csname tcb@minipage@\kvtcb@sbs@align\endcsname}%
  \tcbdimto\tcb@w@upper@real{\tcb@w@upper}%
  \tcbdimto\tcb@w@sbs{\tcb@w@upper@real-\kvtcb@sbs@gap}%
  \tcb@sbs@quota%
  \ifx\kvtcb@float\@empty%
    \let\tcb@before@unbroken=\kvtcb@beforebox%
    \let\tcb@after@unbroken=\kvtcb@afterbox%
  \else%
    \edef\tcb@before@unbroken{\noexpand\tcb@float@env@begin{tcbfloat}[\kvtcb@float]}%
    \let\tcb@after@unbroken=\tcb@float@env@end%
  \fi%
}

\def\tcb@use@lower@outside@side#1{%
  \setbox\z@=\hbox{\begin{tcb@lower@outside}{#1}%
    \tcb@use@listing@other@reset%
  \end{tcb@lower@outside}}%
  \tcb@box@align\z@%
  \tcbdimto{\tcb@temp@wd}{\wd\z@}%
  \unhbox\z@%
}

\def\tcb@inputlisting@out@listingAndOther{%
  \tcb@inputlisting@out@prepare%
  \tcbdimto\tcb@w@outside{\tcb@w@lower}%
  \tcbdimto\tcb@w@inside{\tcb@width-\tcb@w@lower-\kvtcb@sbs@gap}%
  \begin{tcb@outside@environment}%
  \setbox\z@=\hbox{\tcb@minipage{\tcb@w@inside}%
  \begin{tcolorbox}[width=\tcb@w@inside,nobeforeafter,nofloat,sidebyside=false,savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
  \endminipage}%
  \tcb@box@align\z@%
  \unhbox\z@%
  \kern\kvtcb@sbs@gap%
  \iftcb@lowervisible%
    \tcb@use@lower@outside@side{\tcb@w@outside}%
  \fi%
  \end{tcb@outside@environment}%
}

\def\tcb@inputlisting@out@otherAndListing{%
  \tcb@inputlisting@out@prepare%
  \tcbdimto\tcb@w@outside{\tcb@w@upper}%
  \tcbdimto\tcb@w@inside{\tcb@width-\tcb@w@upper-\kvtcb@sbs@gap}%
  \begin{tcb@outside@environment}%
  \iftcb@lowervisible%
    \tcb@use@lower@outside@side{\tcb@w@outside}%
    \tcbdimto{\tcb@temp@wd}{\tcb@w@outside-\tcb@temp@wd+\kvtcb@sbs@gap}%
  \else%
    \tcbdimto{\tcb@temp@wd}{\tcb@w@outside+\kvtcb@sbs@gap}%
  \fi%
  \kern\tcb@temp@wd%
  \setbox\z@=\hbox{\tcb@minipage{\tcb@w@inside}%
  \begin{tcolorbox}[width=\tcb@w@inside,nobeforeafter,nofloat,sidebyside=false,savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
  \endminipage}%
  \tcb@box@align\z@%
  \unhbox\z@%
  \end{tcb@outside@environment}%
}

\def\tcb@inputlisting@inside{%
  \begin{tcolorbox}[capture=\tcb@listing@capture,savedelimiter=tcolorbox]\tcb@listing@process\end{tcolorbox}%
}

\long\def\tcb@run@system@command#1{%
  \ifcase\pdf@shellescape\relax
    \tcb@error{You must invoke LaTeX with the -shell-escape flag}{Pass the -shell-escape flag to LaTeX.}%
  \or\or
    \tcb@warning{System call with restricted shell escape may fail}%
  \fi%
  \ShellEscape{#1}%
  \relax%
}


\tcbset{%
  listing file/.store in=\kvtcb@listingfile,%
  comment/.store in=\kvtcb@listingcomment,%
  listing@process@inside/.code 2 args={%
    \let\tcb@inputlisting\tcb@inputlisting@inside%
    \let\tcb@listing@process=#1%
    \let\tcb@use@listing@other=#2},%
  listing@process@outside/.code 2 args={%
    \let\tcb@inputlisting=#1%
    \let\tcb@use@listing@other=#2},%
  listing only/.style={listing@process@inside={\tcb@listing@listing}{\tcbuselistingtext}},%
  text only/.style={listing@process@inside={\tcbuselistingtext}{\tcbuselistingtext}},%
  comment only/.style={listing@process@inside={\tcbuselistingcomment}{\tcbuselistingcomment}},%
  listing and text/.style={listing@process@inside={\tcb@listing@listingAndOther}{\tcbuselistingtext}},%
  text and listing/.style={listing@process@inside={\tcb@listing@otherAndListing}{\tcbuselistingtext}},%
  text above listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAboveListing}{\tcbuselistingtext}},%
  text above* listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAboveListing@Decoupled}{\tcbuselistingtext}},%
  listing above text/.style={listing@process@outside={\tcb@inputlisting@out@listingAboveOther}{\tcbuselistingtext}},%
  listing above* text/.style={listing@process@outside={\tcb@inputlisting@out@listingAboveOther@Decoupled}{\tcbuselistingtext}},%
  text outside listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAndListing}{\tcbuselistingtext}},%
  listing outside text/.style={listing@process@outside={\tcb@inputlisting@out@listingAndOther}{\tcbuselistingtext}},%
  text side listing/.style={sidebyside,text and listing},%
  listing side text/.style={sidebyside,listing and text},%
  listing and comment/.style={listing@process@inside={\tcb@listing@listingAndOther}{\tcbuselistingcomment}},%
  comment and listing/.style={listing@process@inside={\tcb@listing@otherAndListing}{\tcbuselistingcomment}},%
  comment above listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAboveListing}{\tcbuselistingcomment}},%
  comment above* listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAboveListing@Decoupled}{\tcbuselistingcomment}},%
  listing above comment/.style={listing@process@outside={\tcb@inputlisting@out@listingAboveOther}{\tcbuselistingcomment}},%
  listing above* comment/.style={listing@process@outside={\tcb@inputlisting@out@listingAboveOther@Decoupled}{\tcbuselistingcomment}},%
  comment outside listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAndListing}{\tcbuselistingcomment}},%
  listing outside comment/.style={listing@process@outside={\tcb@inputlisting@out@listingAndOther}{\tcbuselistingcomment}},%
  comment side listing/.style={sidebyside,comment and listing},%
  listing side comment/.style={sidebyside,listing and comment},%
  listing engine/.is choice,%
  image comment/.style 2 args={comment={\includegraphics[#1]{#2}}},%
  comment style/.store in=\kvtcb@commentstyle,%
  tcbimage comment/.style={comment={\let\tcb@trans@commentstyle\kvtcb@commentstyle\tcbincludegraphics[code={\pgfkeysalsofrom\tcb@trans@commentstyle}]{#1}}},
  pdf extension/.store in=\kvtcb@pdf@extension,%
  pdf comment/.style={comment={\let\tcb@trans@commentstyle\kvtcb@commentstyle\filename@parse{#1}\edef\tcb@trans@commentfile{\filename@area\filename@base.\kvtcb@pdf@extension}%
    \begin{tcbraster}[raster halign=center,sharp corners,size=tight,colback=white,code={\pgfkeysalsofrom\tcb@trans@commentstyle}]\tcbincludepdf{\tcb@trans@commentfile}\end{tcbraster}}},
  pdf comment/.default={\kvtcb@listingfile},
  process code/.code={\appto\tcb@listing@process@hook{#1}},%
  no process/.code={\def\tcb@listing@process@hook{}},%
  compilable listing/.style={listing file={\jobname-listing-\thetcblistingcount.tex}},
  run system command/.style={process code={\tcb@run@system@command{#1}}},%
  run@system@command/.style 2 args={run system command={#1\space#2\space\filename@area\filename@base}},%
  run pdflatex/.style={run@system@command={pdflatex}{#1}},%
  run xelatex/.style={run@system@command={xelatex}{#1}},%
  run lualatex/.style={run@system@command={lualatex}{#1}},%
  run makeindex/.style={run@system@command={makeindex}{#1}},%
  run bibtex/.style={run@system@command={bibtex}{#1}},%
  run biber/.style={run@system@command={biber}{#1}},%
  run arara/.style={run@system@command={arara}{#1}},%
  run latex/.style={run@system@command={latex}{#1}},%
  run dvips/.style={run@system@command={dvips}{#1}},%
  run ps2pdf/.style={run system command={ps2pdf\space#1\space\filename@area\filename@base.ps}},%
  freeze file/.code={\def\tcbprocess@condition{1}\def\tcbprocess@target{#1}},%
  freeze none/.code={\def\tcbprocess@condition{0}\def\tcbprocess@target{}},%
  freeze extension/.style={freeze file={\filename@area\filename@base#1}},%
  freeze pdf/.style={freeze extension={.pdf}},
  freeze png/.style={freeze extension={.png}},
  freeze jpg/.style={freeze extension={.jpg}},
}

\def\tcb@listing@process@core{%
  \filename@parse{\kvtcb@listingfile}%
  \tcbiffileprocess{\tcbprocess@condition}%
    {\kvtcb@listingfile}{\filename@area\filename@base.md5}{\tcbprocess@target}%
    {\tcb@listing@process@hook}{}%
}

\def\tcbinputlisting@core{%
  \ifdefempty\tcb@listing@process@hook{}{\tcb@listing@process@core}%
  \let\tcb@listing@capture=\kvtcb@capture%
  \tcb@inputlisting%
}

\newcounter{tcblisting}

\newenvironment{tcblisting}[1]{%
  \stepcounter{tcblisting}\edef\thetcblistingcount{\thetcblisting}%
  \tcb@layer@pushup%
  \tcb@apply@box@options{capture=minipage,#1}%
  \begingroup\tcbverbatimwrite{\kvtcb@listingfile}%
}{\endtcbverbatimwrite\endgroup%
  \tcbinputlisting@core%
}

\long\def\tcbinputlisting#1{%
  \begingroup%
  \stepcounter{tcblisting}\edef\thetcblistingcount{\thetcblisting}%
  \tcb@layer@pushup%
  \tcb@apply@box@options{capture=minipage,#1}%
  \tcbinputlisting@core%
  \endgroup%
}

\newenvironment{tcboutputlisting}{%
  \begingroup\tcbverbatimwrite{\kvtcb@listingfile}%
}{\endtcbverbatimwrite\endgroup}

\long\def\tcb@newtcblisting#1#2{\tcb@newenvironment{#1}{\tcblisting{#2,options@for=#1}}{\endtcblisting}}

\long\def\tcb@newtcblisting@#1[#2]#3{\tcb@newenvironment{#1}[#2]{\tcblisting{#3,options@for=#1}}{\endtcblisting}}

\long\def\tcb@newtcblisting@@#1[#2][#3]#4{\tcb@newenvironment{#1}[#2][#3]{\tcblisting{#4,options@for=#1}}{\endtcblisting}}

\long\def\tcb@new@tcblisting@#1[#2]{%
  \@ifnextchar[{\tcb@newtcblisting@@{#1}[#2]}{\tcb@newtcblisting@{#1}[#2]}}

\def\tcb@new@tcblisting#1{%
  \@ifnextchar[{\tcb@new@tcblisting@{#1}}{\tcb@newtcblisting{#1}}}

\def\newtcblisting{%
  \let\tcb@newenvironment\newenvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcblisting%
  \tcb@process@newenvironment}

\def\renewtcblisting{%
  \let\tcb@newenvironment\renewenvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcblisting%
  \tcb@process@newenvironment}

\long\def\tcb@newtcbinputlisting#1#2{\expandafter\tcb@newcommand\csname#1\endcsname{\tcbinputlisting{#2,options@for=#1}}}

\long\def\tcb@newtcbinputlisting@#1[#2]#3{\expandafter\tcb@newcommand\csname#1\endcsname[#2]{\tcbinputlisting{#3,options@for=#1}}}

\long\def\tcb@newtcbinputlisting@@#1[#2][#3]#4{\expandafter\tcb@newcommand\csname#1\endcsname[#2][#3]{\tcbinputlisting{#4,options@for=#1}}}

\long\def\tcb@new@tcbinputlisting@#1[#2]{%
  \@ifnextchar[{\tcb@newtcbinputlisting@@{#1}[#2]}{\tcb@newtcbinputlisting@{#1}[#2]}}

\def\tcb@new@tcbinputlisting#1{%
  \@ifnextchar[{\tcb@new@tcbinputlisting@{#1}}{\tcb@newtcbinputlisting{#1}}}

\def\newtcbinputlisting{%
  \let\tcb@newcommand\newcommand%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcbinputlisting%
  \tcb@process@newcommand}

\def\renewtcbinputlisting{%
  \let\tcb@newcommand\renewcommand%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcbinputlisting%
  \tcb@process@newcommand}

\tcbset{%
  reset@listingscore/.style={%
    listing file=\jobname.listing,
    comment=, listing and text,
    no process,freeze none,
    comment style=,pdf extension=pdf,
  },
  initialize@reset=reset@listingscore,
}



==> tcblistingsutf8.code.tex <==
%% The LaTeX package tcolorbox - version 4.30 (2020/04/28)
%% tcblistingsutf8.code.tex: Code for colorboxes with listings in UTF-8
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2020 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{4.30}

\tcbuselibrary{listings}

\RequirePackage{iftex}
\ifpdftex
  \let\tcb@temp\relax%
\else
  \tcb@info{Library `listingsutf8' is compatible with pdftex only.
            Library `listings` is loaded instead.}%
  \let\tcb@temp\endinput
\fi
\tcb@temp

\RequirePackage{listingsutf8}[2011/11/10]

\tcbset{
  listing utf8/.style={listing inputencoding=utf8/#1},
}

\tcbset{%
  reset@listingsutf8/.style={listing utf8=latin1},
  initialize@reset=reset@listingsutf8,
}



==> tcbmagazine.code.tex <==
%% The LaTeX package tcolorbox - version 4.30 (2020/04/28)
%% tcbmagazine.code.tex: Code for box sets and magazine styles
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2020 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{4.30}

\tcbuselibrary{breakable}

\def\newboxarray#1{%
  \ifcsdef{tcb@boxarray@#1@allocated}{%
    \tcb@warning{box array '#1' is allocated again by \string\newboxarray. Memory and registers are wasted}%
  }{}%
  \global\csdef{tcb@boxarray@#1@size}{0}%
  \global\csdef{tcb@boxarray@#1@allocated}{0}%
}

\newboxarray{default}

\newrobustcmd*{\boxarraygetsize}[2][default]{%
  \letcs#2{tcb@boxarray@#1@size}%
  \ifdef{#2}{}{%
    \tcb@error{undefined box array '#1'}%
    {You have to say \string\newboxarray{#1}, before '#1' can be used as box array.}%
  }%
}

\newrobustcmd*{\boxarrayreset}[1][default]{%
  \boxarraygetsize[#1]\tcb@box@array@size%
  \global\csdef{tcb@boxarray@#1@size}{0}%
}

\newrobustcmd*{\boxarrayclear}[1][default]{%
  \boxarraygetsize[#1]\tcb@box@array@size%
  \global\csdef{tcb@boxarray@#1@size}{0}%
  \letcs\tcb@box@array@allocated{tcb@boxarray@#1@allocated}%
  \begingroup%
    \count@=0%
    \loop%
    \ifnum\count@<\tcb@box@array@allocated\relax%
      \advance\count@ 1\relax%
      \letcs\tcb@box@array@box{tcb@boxarray@#1@\number\count@ @box}%
      \setbox0=\box\tcb@box@array@box%
    \repeat%
  \endgroup%
}

\newrobustcmd*{\boxarraygetbox}[3][default]{%
  \boxarraygetsize[#1]\tcb@box@array@size%
  \let#2\@undefined%
  \ifnum\numexpr#3>0\relax%
    \ifnum\numexpr#3>\tcb@box@array@size\relax%
    \else%
      \letcs#2{tcb@boxarray@#1@#3@box}%
    \fi%
  \fi%
}

\newrobustcmd*{\boxarraygetwidth}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#3}%
  \ifdefined\tcb@box@array@box%
    \tcbdimto#2{\wd\tcb@box@array@box}%
  \else%
    \let#2\tcb@zpt%
  \fi%
}

\newrobustcmd*{\boxarraygetheight}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#3}%
  \ifdefined\tcb@box@array@box%
    \tcbdimto#2{\ht\tcb@box@array@box}%
  \else%
    \let#2\tcb@zpt%
  \fi%
}

\newrobustcmd*{\boxarraygetdepth}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#3}%
  \ifdefined\tcb@box@array@box%
    \tcbdimto#2{\dp\tcb@box@array@box}%
  \else%
    \let#2\tcb@zpt%
  \fi%
}

\newrobustcmd*{\boxarraygettotalheight}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#3}%
  \ifdefined\tcb@box@array@box%
    \tcbdimto#2{\ht\tcb@box@array@box+\dp\tcb@box@array@box}%
  \else%
    \let#2\tcb@zpt%
  \fi%
}

\newrobustcmd*{\useboxarray}[2][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#2}%
  \ifdefined\tcb@box@array@box%
    \usebox{\tcb@box@array@box}%
  \fi%
}

\newrobustcmd{\usetcboxarray}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#2}%
  \ifdefined\tcb@box@array@box%
    \tcbox[#3]{\usebox{\tcb@box@array@box}}%
  \fi%
}

\newrobustcmd*{\consumeboxarray}[2][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#2}%
  \ifdefined\tcb@box@array@box%
    \leavevmode\box\tcb@box@array@box\relax%
  \fi%
}

\newrobustcmd{\consumetcboxarray}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#2}%
  \ifdefined\tcb@box@array@box%
    \tcbox[#3]{\leavevmode\box\tcb@box@array@box\relax}%
  \fi%
}

\newrobustcmd{\ifboxarrayempty}[2][default]{%
  \begingroup%
    \boxarraygetbox[#1]{\tcb@box@array@box}{#2}%
    \ifdefined\tcb@box@array@box\relax%
      \aftergroup\@secondoftwo%
    \else%
      \aftergroup\@firstoftwo%
    \fi%
  \endgroup%
}

\def\boxarraystore#1{%
  \boxarraygetsize[#1]\tcb@box@array@size%
  \numdef\tcb@box@array@size{\tcb@box@array@size+1}%
  \global\cslet{tcb@boxarray@#1@size}{\tcb@box@array@size}%
  \letcs\tcb@box@array@allocated{tcb@boxarray@#1@allocated}%
  \ifnum\tcb@box@array@allocated<\tcb@box@array@size\relax%
    \newbox\tcb@box@array@box\csxdef{tcb@boxarray@#1@\tcb@box@array@size @box}{\the\tcb@box@array@box}%
    \global\cslet{tcb@boxarray@#1@allocated}{\tcb@box@array@size}%
  \else%
    \letcs\tcb@box@array@box{tcb@boxarray@#1@\tcb@box@array@size @box}%
  \fi%
  \edef\reserved@a{%
    \endgroup
    \global\setbox\tcb@box@array@box\hbox{%
      \begingroup\aftergroup}%
        \def\noexpand\@currenvir{\@currenvir}%
        \def\noexpand\@currenvline{\on@line}}%
  \reserved@a
    \@endpefalse
    \color@setgroup
      \ignorespaces}

\def\endboxarraystore{\unskip\color@endgroup}

\def\tcb@storetoboxarray@begin#1#2[#3]{\begin{boxarraystore}{#1}}
\def\tcb@storetoboxarray@end{\end{boxarraystore}}

\tcbset{
  store to box array/.code={%
    \def\kvtcb@float{S}\def\tcb@float@env@begin{\tcb@storetoboxarray@begin{#1}}\def\tcb@float@env@end{\tcb@storetoboxarray@end}},
  store to box array/.default=default,
  reset box array/.code={\boxarrayreset[#1]},
  reset box array/.default=default,
  reset and store to box array/.style={reset box array={#1},store to box array={#1}},%
  reset and store to box array/.default=default,
  do not store to box array/.style={nofloat},
}



==> tcbminted.code.tex <==
%% The LaTeX package tcolorbox - version 4.30 (2020/04/28)
%% tcbminted.code.tex: Code for colorboxes with listings
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2020 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{4.30}

\RequirePackage{minted}[2011/09/17]

\tcbuselibrary{listings@core}

\def\tcb@minted@input@listing#1#2#3#4{%
  \edef\temp@a{#4}%
  \ifx\temp@a\@empty%
  \else%
    \toks@=\expandafter{#4}%
    \edef\tcb@temp{\noexpand\usemintedstyle{\the\toks@}}%
    \tcb@temp%
  \fi%
  \toks@=\expandafter{#1}%
  \edef\tcb@temp{\noexpand\inputminted[\the\toks@]}%
  \IfFileExists{\minted@outputdir#3}%
    {\tcb@temp{#2}{\minted@outputdir#3}}%
    {\tcb@temp{#2}{#3}}%
}

\def\tcb@minted@uselistinglisting{%
  \tcb@minted@input@listing{\kvtcb@minted@options}{\kvtcb@minted@language}{\kvtcb@listingfile}{\kvtcb@minted@style}%
}%

\def\tcb@minted@usetemplisting{%
  \tcb@minted@input@listing{\kvtcb@minted@options}{\kvtcb@minted@language}{\kvtcb@tempfile}{\kvtcb@minted@style}%
}%

\def\tcb@minted@doc@usetemplisting{%
  \tcb@minted@input@listing{\kvtcb@docmintoptions}{\kvtcb@docminted@language}{\kvtcb@tempfile}{\kvtcb@docmintstyle}%
}

\tcbset{%
  minted language/.store in=\kvtcb@minted@language,
  minted options/.store in=\kvtcb@minted@options,
  minted style/.store in=\kvtcb@minted@style,
  listing engine/minted/.code={\let\tcbuselistinglisting\tcb@minted@uselistinglisting%
    \let\tcbusetemplisting\tcb@minted@usetemplisting%
    \let\tcb@doc@usetemplisting\tcb@minted@doc@usetemplisting},
}


\tcbset{%
  reset@minted/.style={%
    minted language=latex,
    minted options={tabsize=2,fontsize=\small,breaklines,autogobble},
    minted style=,
    listing engine=minted,
  },
  initialize@reset=reset@minted,
}



==> tcbposter.code.tex <==
%% The LaTeX package tcolorbox - version 4.30 (2020/04/28)
%% tcbposter.code.tex: Code for posters
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2020 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{4.30}

\tcbuselibrary{breakable,magazine,skins,fitting}

\newif\iftcb@poster@showframe
\newif\iftcb@posterbox@sequence
\newboxarray{tcb@poster}

\def\tcb@poster@compute@poster@boxheight#1#2{%
  \pgfpointanchor{\tcb@poster@prefix#1}{south}\unskip%
  \@tempdima\pgf@y%
  \pgfpointanchor{\tcb@poster@prefix#2}{north}\unskip%
  \advance \@tempdima by -\pgf@y\relax%
  \advance \@tempdima by -\tcbposterrowspacing\relax%
  \advance \@tempdima by -\tcbposterrowspacing\relax%
  \edef\tcb@poster@boxheight{\the\@tempdima}%
}

\def\poster@scan@sequence#1 between #2 and #3 then#4\@nil{%
  \tcb@poster@compute@poster@boxheight{#2}{#3}%
  \ifundef{\tcb@poster@firstboxheight}{\edef\tcb@poster@firstboxheight{\tcb@poster@boxheight}}{}%
  \eappto\tcb@poster@breakat{\tcb@poster@boxheight/}%
  \@tempcnta\numexpr#1\relax%
  \listeadd\tcb@poster@list{{\tcb@poster@prefix col\@arabic\@tempcnta.west|-\tcb@poster@prefix#2.south}{\tcb@poster@boxheight}}%
  \ifblank{#4}{}{\poster@scan@sequence#4\@nil}%
}

\newenvironment{tcb@poster@env}{%
  \let\posterbox\tcb@poster@box%
  \let\posterboxenv\tcb@poster@boxenv%
  \let\endposterboxenv\endtcb@poster@boxenv%
  \ifundef\tcb@poster@height{%
    \ifnum\c@tcblayer=0\relax%
      \def\tcb@poster@height{\textheight}%
    \else%
      \ifdim\dimexpr\tcbtextheight>0pt\relax%
        \def\tcb@poster@height{\tcbtextheight}%
      \else%
        \def\tcb@poster@height{0.75\textheight}%
      \fi%
    \fi}{}%
  \tcbset{poster/.cd,poster@poster}%
  \tcbdimto\tcbposterwidth{\tcb@poster@width}%
  \tcbdimto\tcbposterheight{\tcb@poster@height}%
  \tcbdimto\tcbpostercolspacing{\tcb@poster@colspacing}%
  \tcbdimto\tcbposterrowspacing{\tcb@poster@rowspacing}%
  \edef\tcbpostercolumns{\the\numexpr\tcb@poster@columns\relax}%
  \edef\tcbposterrows{\the\numexpr\tcb@poster@rows\relax}%
  \tcbdimto\tcbpostercolwidth{(\tcbposterwidth+\tcbpostercolspacing)/\tcbpostercolumns-\tcbpostercolspacing}%
  \tcbdimto\tcbposterrowheight{(\tcbposterheight+\tcbposterrowspacing)/\tcbposterrows-\tcbposterrowspacing}%
  \begin{tikzpicture}%
  \path[use as bounding box] (0,0) rectangle (\tcbposterwidth,\tcbposterheight);
  \node[name=\tcb@poster@prefix poster,at={(0,0)},line width=0mm,inner sep=0mm,outer sep=0mm,draw=none,fill=none,rectangle,
    above right,minimum width=\tcbposterwidth,minimum height=\tcbposterheight]{};
  \coordinate (\tcb@poster@prefix top) at (0,\tcbposterheight+\tcbposterrowspacing);
  \coordinate (\tcb@poster@prefix bottom) at (0,-\tcbposterrowspacing);
  \coordinate (\tcb@poster@prefix middle) at (0,\the\dimexpr0.5\dimexpr\tcbposterheight\relax);
  \begin{scope}[every node/.style={inner sep=0pt,outer sep=0,above right,minimum height=\tcbposterheight,minimum width=\tcbpostercolwidth}]%
    \node (\tcb@poster@prefix col1) at (0,0) {};
    \@tempcnta 1%
    \@tempcntb\numexpr\tcbpostercolumns\relax%
    \@tempdima\dimexpr\tcbpostercolwidth+\tcbpostercolspacing\relax%
    \@whilenum \@tempcnta<\@tempcntb \do{%
      \edef\tcb@temp{\tcb@poster@prefix col\@arabic\@tempcnta}%
      \advance\@tempcnta 1\relax%
      \node[xshift=\tcbpostercolspacing] (\tcb@poster@prefix col\@arabic\@tempcnta) at (\tcb@temp.south east) {};
    }%
  \end{scope}%
  \begin{scope}[every node/.style={inner sep=0pt,outer sep=0,below right,minimum height=\tcbposterrowheight,minimum width=\tcbposterwidth}]%
    \node (\tcb@poster@prefix row1) at (0,\tcbposterheight) {};
    \@tempcnta 1%
    \@tempcntb\numexpr\tcbposterrows\relax%
    \@tempdima\dimexpr\tcbposterrowheight+\tcbposterrowspacing\relax%
    \@whilenum \@tempcnta<\@tempcntb \do{%
      \edef\tcb@temp{\tcb@poster@prefix row\@arabic\@tempcnta}%
      \advance\@tempcnta 1\relax%
      \node[yshift=-\tcbposterrowspacing] (\tcb@poster@prefix row\@arabic\@tempcnta) at (\tcb@temp.south west) {};
    }%
  \end{scope}%
  \iftcb@poster@showframe%
    \@tempcnta 0%
    \@tempcntb\numexpr\tcbpostercolumns\relax%
    \@whilenum \@tempcnta<\@tempcntb \do{%
      \advance\@tempcnta 1\relax%
      \edef\tcb@temp{\tcb@poster@prefix col\@arabic\@tempcnta}%
      \draw[red] (\tcb@temp.north west) node[above right]{col\@arabic\@tempcnta} rectangle (\tcb@temp.south east);
    }%
    \@tempcnta 0%
    \@tempcntb\numexpr\tcbposterrows\relax%
    \@whilenum \@tempcnta<\@tempcntb \do{%
      \advance\@tempcnta 1\relax%
      \edef\tcb@temp{\tcb@poster@prefix row\@arabic\@tempcnta}%
      \draw[red] (\tcb@temp.north west) node[below left]{row\@arabic\@tempcnta} rectangle (\tcb@temp.south east);
    }%
    \gdef\tcb@poster@framelist{}%
  \fi%
}{%
  \iftcb@poster@showframe%
    \renewcommand*{\do}[1]{%
      \node[red,fill=white,opacity=0.7,font=\Large] at (\tcb@poster@prefix##1) {##1};}%
    \dolistloop{\tcb@poster@framelist}%
    \gdef\tcb@poster@framelist{}%
  \fi%
\end{tikzpicture}}

% #1 tcolorbox options
% #2 position
% #3 Inhalt
\newcommand{\tcb@poster@box}[3][]{%
  \bgroup%
  \tcbset{posterloc/.cd,#2}%
  \tcbdimto\tcb@poster@boxwidth{\tcb@poster@span\dimexpr\tcbpostercolwidth+\tcbpostercolspacing\relax-\tcbpostercolspacing}%
  \iftcb@posterbox@sequence%
    \begin{pgfinterruptpicture}%
      \begin{tcolorbox}[tcb@poster@style,width=\tcb@poster@boxwidth,tcb@poster@boxheight,
        height fixed for=all,#1,
        enforce breakable,reset box array=tcb@poster,store to box array=tcb@poster]#3\end{tcolorbox}%
    \end{pgfinterruptpicture}%
    \def\tcb@poster@boxcount{0}%
    \renewcommand*{\do}[1]{\edef\tcb@poster@boxcount{\the\numexpr\tcb@poster@boxcount+1\relax}%
      \node[inner sep=0pt,outer sep=0,tcb@poster@node,name=\tcb@poster@prefix\tcb@poster@boxname\tcb@poster@boxcount] at (\@firstoftwo##1) {%
        \ifboxarrayempty[tcb@poster]{\tcb@poster@boxcount}%
          {\begin{tcolorbox}[placeholder,width=\tcb@poster@boxwidth,height=\@secondoftwo##1]\end{tcolorbox}}%
          {\consumeboxarray[tcb@poster]{\tcb@poster@boxcount}}%
      };}%
    \dolistloop{\tcb@poster@list}%
    \iftcb@poster@showframe%
      \ifdefstring{\tcb@poster@boxname}{@}{}{%
        \def\tcb@poster@boxcount{0}%
        \renewcommand*{\do}[1]{\edef\tcb@poster@boxcount{\the\numexpr\tcb@poster@boxcount+1\relax}%
          \listxadd\tcb@poster@framelist{\tcb@poster@boxname\tcb@poster@boxcount}}%
        \dolistloop{\tcb@poster@list}%
       }%
    \fi%
  \else%
    \begin{pgfinterruptpicture}%
      \begin{tcolorbox}[tcb@poster@style,width=\tcb@poster@boxwidth,tcb@poster@boxheight,#1,
        reset box array=tcb@poster,store to box array=tcb@poster]#3\end{tcolorbox}%
    \end{pgfinterruptpicture}%
    \node[inner sep=0pt,outer sep=0,tcb@poster@node,name=\tcb@poster@prefix\tcb@poster@boxname] at (\tcb@poster@xpos|-\tcb@poster@ypos)
      {\consumeboxarray[tcb@poster]{1}};%
    \iftcb@poster@showframe%
      \ifdefstring{\tcb@poster@boxname}{@}{}{\listxadd\tcb@poster@framelist{\tcb@poster@boxname}}%
    \fi%
  \fi%
  \egroup%
}

\newenvironment{tcb@poster@boxenv}[2][]{%
  \newcommand{\tcb@poster@box@saved}{\posterbox[#1]{#2}{\tcbusetemp}}%
  \tcbwritetemp}%
  {\endtcbwritetemp\tcb@poster@box@saved}

\newenvironment{tcbposter@coverage}{}{}

\newenvironment{tcbposter}[1][]{%
  \tcbposterset{#1}%
  \begin{tcbposter@coverage}\begin{tcb@poster@env}%
}{\end{tcb@poster@env}\end{tcbposter@coverage}}

\newcommand{\tcbposterset}[1]{\tcbset{posterset/.cd,#1}}

\tcbset{%
  poster/.cd,
  width/.store in=\tcb@poster@width,
  height/.store in=\tcb@poster@height,
  colspacing/.store in=\tcb@poster@colspacing,
  rowspacing/.store in=\tcb@poster@rowspacing,
  spacing/.style={colspacing={#1},rowspacing={#1}},
  columns/.store in=\tcb@poster@columns,
  rows/.store in=\tcb@poster@rows,
  showframe/.is if=tcb@poster@showframe,
  prefix/.store in=\tcb@poster@prefix,
  %
  width=\linewidth,
  spacing=4mm,
  columns=3,
  rows=4,
  showframe=false,
  prefix=TCBPOSTER@,
}

\tcbset{%
  posterloc/.cd,
  name/.store in=\tcb@poster@boxname,
  column/.code={\edef\tcb@poster@xpos{\tcb@poster@prefix col#1.west}\edef\tcb@poster@orientation{right}},%
  column*/.code={\edef\tcb@poster@xpos{\tcb@poster@prefix col#1.east}\edef\tcb@poster@orientation{left}},%
  below/.code={\tcb@posterbox@sequencefalse%
    \tikzset{tcb@poster@node/.style={below \tcb@poster@orientation,yshift=\the\dimexpr\tcb@poster@yshift-\tcbposterrowspacing\relax,xshift=\tcb@poster@xshift}}%
    \tcbset{tcb@poster@boxheight/.style={natural height}}%
    \edef\tcb@poster@ypos{\tcb@poster@prefix#1.south}},
  above/.code={\tcb@posterbox@sequencefalse%
    \tikzset{tcb@poster@node/.style={above \tcb@poster@orientation,yshift=\the\dimexpr\tcb@poster@yshift+\tcbposterrowspacing\relax,xshift=\tcb@poster@xshift}}%
    \tcbset{tcb@poster@boxheight/.style={natural height}}%
    \edef\tcb@poster@ypos{\tcb@poster@prefix#1.north}},
  at/.code={\tcb@posterbox@sequencefalse%
    \tikzset{tcb@poster@node/.style={\tcb@poster@orientation,yshift=\tcb@poster@yshift,xshift=\tcb@poster@xshift}}%
    \tcbset{tcb@poster@boxheight/.style={natural height}}%
    \edef\tcb@poster@ypos{\tcb@poster@prefix#1}},
  between/.code args={#1 and #2}{\tcb@posterbox@sequencefalse%
    \tikzset{tcb@poster@node/.style={below \tcb@poster@orientation,yshift=\the\dimexpr\tcb@poster@yshift-\tcbposterrowspacing\relax,xshift=\tcb@poster@xshift}}%
    \edef\tcb@poster@ypos{\tcb@poster@prefix#1.south}%
    \tcb@poster@compute@poster@boxheight{#1}{#2}%
    \tcbset{tcb@poster@boxheight/.style={height=\tcb@poster@boxheight}}%
  },
  sequence/.code={\tcb@posterbox@sequencetrue%
    \tikzset{tcb@poster@node/.style={below \tcb@poster@orientation,yshift=\the\dimexpr\tcb@poster@yshift-\tcbposterrowspacing\relax,xshift=\tcb@poster@xshift}}%
    \undef\tcb@poster@firstboxheight%
    \def\tcb@poster@breakat{}%
    \def\tcb@poster@list{}%
    \poster@scan@sequence #1 then\@nil%
    \eappto\tcb@poster@breakat{\tcbposterheight}%
    \tcbset{tcb@poster@boxheight/.style={break at=\tcb@poster@breakat,height=\tcb@poster@firstboxheight}}%
    },
  row/.code={\tcb@posterbox@sequencefalse%
    \tikzset{tcb@poster@node/.style={below \tcb@poster@orientation,yshift=\tcb@poster@yshift,xshift=\tcb@poster@xshift}}%
    \tcbset{posterloc/fixed height}%
    \edef\tcb@poster@ypos{\tcb@poster@prefix row#1.north}},
  %
  span/.store in=\tcb@poster@span,%
  row@span/.store in=\tcb@poster@rowspan,%
  rowspan/.style={row@span=#1,fixed height},%
  xshift/.store in=\tcb@poster@xshift,%
  yshift/.store in=\tcb@poster@yshift,%
  fixed height/.code={\tcbset{tcb@poster@boxheight/.style={height=\tcb@poster@rowspan\dimexpr\tcbposterrowheight+\tcbposterrowspacing\relax-\tcbposterrowspacing}}},%
  %
  name=@,
  column=1,
  below=top,
  span=1,
  row@span=1,
  xshift=0pt,
  yshift=0pt,
}

\tcbposterset{%
  coverage/.code={\renewtcolorbox{tcbposter@coverage}{%
    enhanced,frame hidden,sharp corners,boxsep=0pt,boxrule=0pt,
    top=4mm,bottom=4mm,left=4mm,right=4mm,
    toptitle=2mm,bottomtitle=2mm,colback=white,#1}},
  no coverage/.code={\renewenvironment{tcbposter@coverage}{}{}},
  poster/.code={\tcbset{poster/.cd,poster@poster/.style={#1}}},
  boxes/.code={\tcbset{tcb@poster@style/.style={nobeforeafter,enhanced standard,#1}}},
  fontsize/.code={\tcbset{fit fontsize macros}\tcbsetforeverylayer{fit basedim=#1}\normalsize},
  %
  poster,boxes
}

\tcbset{placeholder/.style={enhanced jigsaw,
  size=small,sharp corners,colframe=red!50!black,
  interior style={bottom color=red!15!white,top color=blue!15!white},
  opacityback=0.5,
  underlay={\draw[red!50!black,line cap=round] (interior.south west)--(interior.north east);
    \draw[red!50!black,line cap=round] (interior.south east)--(interior.north west);},
}}%


==> tcbprocessing.code.tex <==
%% The LaTeX package tcolorbox - version 4.30 (2020/04/28)
%% tcbprocessing.code.tex: Code for conditional processing
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2020 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{4.30}

\RequirePackage{pdftexcmds}
\RequirePackage{shellesc}

\ifdefined\pdf@filemdfivesum\else% XeLaTeX presumed ...
  \def\pdf@filemdfivesum#1{\mdfivesum file {#1}}%
\fi
\ifdefined\pdf@filemoddate\else% very poor XeLaTeX bypassing
  \def\pdf@filemoddate#1{}%
\fi

\def\tcbproc@readmdfive#1#2{%
  \edef\tcbprocmdfivesum{\pdf@filemdfivesum{#1}}%
  \IfFileExists{#2}{\input{#2}}{\def\tcbproclastmdfivesum{}}%
}

\def\tcbproc@writemdfive#1{%
  \immediate\openout\tcb@out=#1%
  \immediate\write\tcb@out{\string\def\string\tcbproclastmdfivesum{\tcbprocmdfivesum}\@percentchar}%
  \immediate\closeout\tcb@out%
}

\newrobustcmd{\iftcb@process@on}[3]{%
  \tcbproc@readmdfive{#1}{#2}%
  \ifdefstrequal{\tcbproclastmdfivesum}{\tcbprocmdfivesum}{}{\tcbproc@writemdfive{#2}}%
  \expandafter\@firstoftwo%
}

\newrobustcmd{\iftcb@process@conditional}[3]{%
  \tcbproc@readmdfive{#1}{#2}%
  \ifdefstrequal{\tcbproclastmdfivesum}{\tcbprocmdfivesum}{%
    \IfFileExists{#3}{%
      \ifnum\pdf@strcmp{\pdf@filemoddate{#2}}{\pdf@filemoddate{#3}}>0\relax%
        \expandafter\@firstoftwo%
      \else%
        \expandafter\@secondoftwo%
      \fi%
    }{\expandafter\@firstoftwo}%
  }{%
    \tcbproc@writemdfive{#2}%
    \expandafter\@firstoftwo%
  }%
}

\newrobustcmd{\iftcb@process@off}[3]{%
  \tcbproc@readmdfive{#1}{#2}%
  \ifdefstrequal{\tcbproclastmdfivesum}{\tcbprocmdfivesum}{}{\tcbproc@writemdfive{#2}}%
  \expandafter\@secondoftwo%
}%

\newrobustcmd{\tcbiffileprocess}[1]{%
  \ifcase\numexpr#1\relax%
    \expandafter\iftcb@process@on%
  \or%
    \expandafter\iftcb@process@conditional%
  \else%
    \expandafter\iftcb@process@off%
  \fi%
}


==> tcbraster.code.tex <==
%% The LaTeX package tcolorbox - version 4.30 (2020/04/28)
%% tcbskinsjigsaw.code.tex: Code for colorboxes with different skins
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2020 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{4.30}

\newcounter{tcbrastercolumn}
\newcounter{tcbrasterrow}
\newcounter{tcbraster}

\newrobustcmd{\thetcbrasternum}{\the\numexpr(\c@tcbrasterrow-1)*\kvtcb@raster@columns+\c@tcbrastercolumn\relax}

\def\tcb@raster@ehg@all{%
  \tcbset{equal height group={\kvtcb@raster@ehgid}}%
}

\def\tcb@raster@ehg@row{%
  \tcbset{equal height group={\kvtcb@raster@ehgid @\number\c@tcbrasterrow}}%
}


\tcbset{%
  raster columns/.store in=\kvtcb@raster@columns,
  raster rows/.store in=\kvtcb@raster@rows,
  raster width/.store in=\kvtcb@raster@width,
  raster height/.store in=\kvtcb@raster@height,
  %
  raster before skip/.store in=\kvtcb@raster@skip@before,
  raster after skip/.store in=\kvtcb@raster@skip@after,
  raster left skip/.store in=\kvtcb@raster@skip@left,
  raster right skip/.store in=\kvtcb@raster@skip@right,
  %
  raster column skip/.store in=\kvtcb@raster@xskip,
  raster row skip/.store in=\kvtcb@raster@yskip,
  %
  raster equal skip/.style={raster before skip=#1,raster after skip=#1,
    raster column skip=#1,raster row skip=#1},
  %
  raster@halign/.store in=\kvtcb@raster@halign,
  raster halign/.is choice,
  raster halign/center/.style={raster@halign=\centering},
  raster halign/left/.style={raster@halign=\raggedright},
  raster halign/right/.style={raster@halign=\raggedleft},
  %
  raster valign/.store in=\kvtcb@raster@valign,
  %
  raster equal height group/.store in=\kvtcb@raster@ehgid,%
  raster equal height/.is choice,
  raster equal height/.default=all,
  raster equal height/none/.code={\let\tcb@raster@ehg@set\@empty},%
  raster equal height/rows/.code={\let\tcb@raster@ehg@set\tcb@raster@ehg@row},%
  raster equal height/all/.code={\let\tcb@raster@ehg@set\tcb@raster@ehg@all},%
  %
  raster force size/.is choice,%
  raster force size/.default=true,%
  raster force size/true/.code={\let\tcb@raster@set@size\tcbset@late@options},%
  raster force size/false/.code={\let\tcb@raster@set@size\tcbset},%
  raster multicolumn/.code={%
    \ifnum\numexpr\c@tcbrastercolumn+#1>\numexpr\kvtcb@raster@columns+1\relax
      \tcb@warning{'raster multicolumn' combined too much columns}%
    \else%
      \tcbset@late@options{%
        code={\preto\kvtcb@afterbox{\addtocounter{tcbrastercolumn}{\numexpr#1-1}}},
        width=(\tcb@raster@box@width+\tcb@raster@xskip)*#1-\tcb@raster@xskip}%
    \fi%
  },
  raster multirow/.code={%
    \ifdefined\tcb@raster@box@height%
      \tcbset@late@options{%
        height=(\tcb@raster@box@height+\tcb@raster@yskip)*#1-\tcb@raster@yskip}%
    \else%
      \tcb@warning{'raster multirow' needs a fixed 'raster height'}%
    \fi%
  },
  raster width center/.style={raster width=\linewidth,raster left skip=(\linewidth-(#1))/2,raster right skip=(\linewidth-(#1))/2},
  raster width flush left/.style={raster width=\linewidth,raster left skip=0pt,raster right skip=\linewidth-(#1)},
  raster width flush right/.style={raster width=\linewidth,raster left skip=\linewidth-(#1),raster right skip=0pt},
}

\tcbset{
  raster reset/.style={
    raster width=\linewidth,raster height=0pt,
    raster equal skip=2mm,
    raster columns=2,raster rows=2,
    raster left skip=0pt,raster right skip=0pt,
    raster halign=left,raster valign=center,
    raster equal height=none,
    raster equal height group={REG@\tcb@raster@number},
    raster force size,},
  raster reset
}

\setcounter{tcbraster}{0}

\let\tcb@raster@change@minipage\@empty
\let\tcb@raster@change@fitbox\@empty
\def\tcb@raster@change@hbox{\tcbset{capture=minipage}}

\def\tcb@height@fill@unbroken@raster#1{%
  \ifnum\c@tcblayer<2\relax%
    \kvtcb@beforebox%
    \def\kvtcb@beforebox{}%
    \tcb@breakat@init%
    \tcbset{compress page=#1}%
    \tcb@comp@h@page%
    \ifdim\tcb@h@page<0pt\relax\unkern\pagebreak\tcb@comp@h@page\kern\tcb@raster@skip@left\fi%
    \tcbset{height=\tcb@h@page-\kvtcb@bbtop@stand-\kvtcb@bbbottom@stand}%
  \fi%
}

\newenvironment{tcbraster}[1][]{%
  \tcb@layer@pushup%
  \stepcounter{tcbraster}%
  \edef\tcb@raster@number{\number\c@tcbraster}%
  \edef\tcb@raster@save@column{\number\c@tcbrastercolumn}%
  \edef\tcb@raster@save@row{\number\c@tcbrasterrow}%
  \let\tcb@raster@change@fitbox\@empty%
  \setcounter{tcbrastercolumn}{1}%
  \setcounter{tcbrasterrow}{1}%
  \let\tcb@height@fill@unbroken\tcb@height@fill@unbroken@raster%
  \tcbset{every box on layer \the\numexpr\number\c@tcblayer+1\relax/.code={%
    \tcb@raster@ehg@set%
    \tcbset{raster every box/.try}%
    \ifodd\c@tcbrastercolumn\relax%
      \tcbset{raster odd column/.try}%
    \else%
      \tcbset{raster even column/.try}%
    \fi%
    \tcbset{raster column \number\c@tcbrastercolumn/.try}%
    \ifodd\c@tcbrasterrow\relax%
      \tcbset{raster odd row/.try}%
    \else%
      \tcbset{raster even row/.try}%
    \fi%
    \tcbset{raster row \number\c@tcbrasterrow/.try}%
    \ifodd\thetcbrasternum\relax%
      \tcbset{raster odd number/.try}%
    \else%
      \tcbset{raster even number/.try}%
    \fi%
    \tcbset{raster row \number\c@tcbrasterrow\space column \number\c@tcbrastercolumn/.try}%
    \tcbset{raster number \thetcbrasternum/.try}%
  }}%
  \tcbset{#1}%
  % sanitize
  \tcbdimto\tcb@raster@width{\kvtcb@raster@width}%
  \tcbdimto\tcb@raster@height{\kvtcb@raster@height}%
  \tcbglueto\tcb@raster@skip@before{\kvtcb@raster@skip@before}%
  \tcbglueto\tcb@raster@skip@after{\kvtcb@raster@skip@after}%
  \tcbdimto\tcb@raster@skip@left{\kvtcb@raster@skip@left}%
  \tcbdimto\tcb@raster@skip@right{\kvtcb@raster@skip@right}%
  \tcbdimto\tcb@raster@xskip{\kvtcb@raster@xskip}%
  \tcbdimto\tcb@raster@yskip{\kvtcb@raster@yskip}%
  \tcbset@late@options{%
    before={\ifhmode\unskip\fi\ifnum\c@tcbrastercolumn>1 \kern\tcb@raster@xskip\else%
      \ifnum\c@tcbrasterrow>1 \parindent\z@\parskip\z@\par\nointerlineskip\addvspace{\the\dimexpr\tcb@raster@yskip\relax}\noindent\fi%
      \kern\tcb@raster@skip@left\fi},
    after={%
      \ifnum\c@tcbrastercolumn=\kvtcb@raster@columns\relax%
        \kern\tcb@raster@skip@right%
        \setcounter{tcbrastercolumn}{1}\addtocounter{tcbrasterrow}{1}%
      \else%
        \stepcounter{tcbrastercolumn}%
      \fi},%
    box align=\kvtcb@raster@valign,%
  }%
  \tcbdimto\tcb@raster@box@width{(\tcb@raster@width+\tcb@raster@xskip-\tcb@raster@skip@left-\tcb@raster@skip@right)/\kvtcb@raster@columns-\tcb@raster@xskip}%
  \tcb@raster@set@size{%
    code={\csuse{tcb@raster@change@\kvtcb@capture}},
    width=\tcb@raster@box@width,
  }%
  \ifdim\dimexpr\tcb@raster@height>0pt\relax%
    \tcbdimto\tcb@raster@box@height{(\tcb@raster@height+\tcb@raster@yskip-0.001pt)/\kvtcb@raster@rows-\tcb@raster@yskip}%
    \tcb@raster@set@size{height=\tcb@raster@box@height}%
  \fi%
  \let\tcb@end@raster\@empty%
  \ifinner\ifhmode%
    \color@vbox%
    \hsize=\tcb@raster@width%
    \let\tcb@end@raster\color@endbox%
  \fi\fi%&
  \if@nobreak%
    \iftcb@ignorenobreak%
      {\par\nointerlineskip%
      \addvspace{\glueexpr\tcb@raster@skip@before-\parskip}}%
    \fi%
  \else%
    {\par\nointerlineskip%
    \addvspace{\glueexpr\tcb@raster@skip@before-\parskip}}%
  \fi%
  \tcb@parfillskip@check\kvtcb@raster@halign\noindent%
}{%
  \ifhmode\unskip\fi%
  \ifnum\c@tcbrastercolumn>1 %
    \kern\tcb@raster@skip@right%
  \fi%
  \begingroup%
  \par\nointerlineskip%
  \addvspace{\glueexpr\tcb@raster@skip@after-\parskip}%
  \endgroup%
  \tcb@end@raster%
  \setcounter{tcbrastercolumn}{\tcb@raster@save@column}%
  \setcounter{tcbrasterrow}{\tcb@raster@save@row}%
}

\newcommand{\tcbitem@following}[1][]{%
  \end{tcolorbox}\begin{tcolorbox}[#1]%
}

\newcommand{\tcbitem@first}[1][]{%
  \let\tcbitem=\tcbitem@following%
  \begin{tcolorbox}[#1]%
}

\newenvironment{tcbitemize}[1][]{%
  \begin{tcbraster}[#1]%
  \let\tcb@raster@change@fitbox=\tcb@raster@change@hbox%
  \let\tcbitem=\tcbitem@first%
}{\end{tcolorbox}\end{tcbraster}}

\newenvironment{tcboxedraster}[2][]{%
  \tcolorbox[#2]\begin{tcbraster}[#1]}%
  {\end{tcbraster}\endtcolorbox}

\newenvironment{tcboxeditemize}[2][]{%
  \tcolorbox[#2]\tcbitemize[#1]}%
  {\endtcbitemize\endtcolorbox}


==> tcbskins.code.tex <==
%% The LaTeX package tcolorbox - version 4.30 (2020/04/28)
%% tcbskins.code.tex: Code for colorboxes with different skins
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2020 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{4.30}

\RequirePackage{tikz}[2010/10/13]

\newenvironment{tikzpicture@tcb@hooked}{%
  \edef\tcb@tikzpicture@begin{\noexpand\tikzpicture[\expandonce\tcb@tikz@option@hook]}%
  \tcb@tikzpicture@begin\tcb@tikz@begin@hook}{\tcb@tikz@end@hook\endtikzpicture}

\def\tcb@creategeonodes@true{%
  \begin{scope}[every node/.style={line width=0mm,inner sep=0mm,outer sep=0mm,draw=none,fill=none,rectangle}]
    \node[name=frame,at={(0,0)},above right,minimum width=\tcb@width,minimum height=\tcb@height]{};
    \node[name=interior,at={({\kvtcb@left@rule},{\kvtcb@bottom@rule})},above right,minimum width=\tcb@innerwidth,minimum height=\tcb@innerheight]{};
    \ifnum\tcbsegmentstate=1%
    \node[name=segmentation,at={({\kvtcb@left@rule},{\the\dimexpr\kvtcb@bottom@rule+\kvtcb@boxsep*2+\tcb@break@bottomsep+\kvtcb@bottom+\tcb@height@lower\relax})},above right,
       minimum width=\tcb@innerwidth,minimum height=\the\dimexpr\kvtcb@middle*2\relax]{};
    \else\iftcb@sidebyside%
    \node[name=segmentation,at={({\the\dimexpr\kvtcb@left@rule+\kvtcb@boxsep+\kvtcb@leftupper+\tcb@w@upper\relax},{\the\dimexpr\kvtcb@bottom@rule\relax})},above right,
       minimum width=\the\dimexpr\kvtcb@sbs@gap\relax,minimum height=\tcb@innerheight]{};
    \fi\fi%
    \iftcb@hasTitle%
    \node[name=title,at={({\kvtcb@left@rule},{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule\relax})},above right,
       minimum width=\tcb@innerwidth,minimum height=\the\dimexpr\tcb@h@title+\kvtcb@toptitle+\kvtcb@bottomtitle+\kvtcb@boxsep*2\relax]{};
    \fi%
    \tcb@specialgeonodes@hook%
  \end{scope}%
}

\def\tcbsettowidthofnode#1#2{%
  \pgfpointanchor{#2}{east}\unskip%
  #1\pgf@x%
  \pgfpointanchor{#2}{west}\unskip%
  \advance #1 by -\pgf@x\relax%
}

\def\tcbsetmacrotowidthofnode#1#2{%
  \tcbsettowidthofnode\pgf@xa{#2}%
  \edef#1{\the\pgf@xa}%
}

\def\tcbsettoheightofnode#1#2{%
  \pgfpointanchor{#2}{north}\unskip%
  #1\pgf@y%
  \pgfpointanchor{#2}{south}\unskip%
  \advance #1 by -\pgf@y\relax%
}

\def\tcbsetmacrotoheightofnode#1#2{%
  \tcbsettoheightofnode\pgf@ya{#2}%
  \edef#1{\the\pgf@ya}%
}

\def\tcb@spec#1{\tikzset{tcb@spec/.style={#1}}}

\def\tcb@gettikzxy#1#2#3{%
  \tikz@scan@one@point\pgfutil@firstofone#1\relax%
  \edef#2{\the\pgf@x}%
  \edef#3{\the\pgf@y}%
}

\def\tcb@boundary@tikzbase#1#2#3#4#5#6{%
  \tcb@gettikzxy{(#1)}{\tcb@xa}{\tcb@ya}%
  \tcb@gettikzxy{(#2)}{\tcb@xb}{\tcb@yb}%
  \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  #4\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
  #5\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
  #6\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
  #3\pgfpathclose%
}

\def\tcb@pathboundary#1#2{\path[#1]\pgfextra{#2};}

\def\tcb@pathbase#1#2#3#4#5#6#7{\tcb@pathboundary{#1}{\tcb@boundary@tikzbase{#2}{#3}{#4}{#5}{#6}{#7}}}

\def\tcb@boundaryframe@pathfirst{%
  \tcb@boundary@base{0pt}{0pt}%
    {\tcb@width}{\tcb@height}%
    {\tcb@arc@zpt}{\tcb@arc@out@NW}{\tcb@arc@out@NE}{\tcb@arc@zpt}%
}

\def\tcb@boundaryframe@pathmiddle{%
  \tcb@boundary@base{0pt}{0pt}%
    {\tcb@width}{\tcb@height}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@boundaryframe@pathlast{%
  \tcb@boundary@base{0pt}{0pt}%
    {\tcb@width}{\tcb@height}%
    {\tcb@arc@out@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@out@SE}%
}

\tikzset{%
  tcb fill frame/.style={fill=tcbcolframe,fill opacity=\kvtcb@opacityframe,tcb@spec,frame@style},%
  tcb fill interior/.style={fill=tcbcolback,fill opacity=\kvtcb@opacityback,tcb@spec,interior@style},%
  tcb fill title/.style={fill=tcbcolbacktitle,fill opacity=\kvtcb@opacitybacktitle,tcb@spec,title@style},%
}

% fill frame
\def\tcb@drawframe@path{\tcb@pathboundary{tcb fill frame}{\tcb@outerboundary}}
\let\tcb@drawframe@pathfirst=\tcb@drawframe@path
\let\tcb@drawframe@pathmiddle=\tcb@drawframe@path
\let\tcb@drawframe@pathlast=\tcb@drawframe@path


% fill inner box with title
\def\tcb@drawwithtitle@path{\tcb@pathboundary{tcb fill interior}{\tcb@boundaryinterior@title@standard}}

\def\tcb@drawwithtitle@pathfirst{%
  \tcb@pathbase{tcb fill interior}{interior.west|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\let\tcb@drawwithtitle@pathmiddle=\tcb@drawwithtitle@pathfirst

\let\tcb@drawwithtitle@pathlast=\tcb@drawwithtitle@path

% fill inner box without title
\def\tcb@drawwithouttitle@path{\tcb@pathboundary{tcb fill interior}{\tcb@boundaryinterior@notitle@standard}}

\def\tcb@drawwithouttitle@pathfirst{%
  \tcb@pathbase{tcb fill interior}{interior.west|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@ins@NW}{\tcb@arc@ins@NE}{\tcb@arc@zpt}%
}

\def\tcb@drawwithouttitle@pathmiddle{%
  \tcb@pathbase{tcb fill interior}{interior.west|-frame.south}{interior.east|-frame.north}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawwithouttitle@pathlast{%
  \tcb@pathbase{tcb fill interior}{interior.south west}{interior.east|-frame.north}%
    {\tcb@arc@ins@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

% draw title box
\def\tcb@drawtitle@path{\tcb@pathboundary{tcb fill title}{\tcb@boundarytitle@standard}}

\let\tcb@drawtitle@pathfirst=\tcb@drawtitle@path

\def\tcb@drawtitle@pathmiddle{%
  \tcb@pathbase{tcb fill title}{title.south west}{title.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\let\tcb@drawtitle@pathlast=\tcb@drawtitle@pathmiddle

% draw segmentation line
\def\tcb@drawlower@path{%
  \iftcb@sidebyside%
    \path[draw=tcbcolframe,fill opacity=\kvtcb@opacityframe,dash pattern=on 1mm off 1mm,dash phase=0.5mm,tcb@spec,segmentation@style]
    (segmentation.north)--(segmentation.south);%
  \else%
    \path[draw=tcbcolframe,fill opacity=\kvtcb@opacityframe,dash pattern=on 1mm off 1mm,dash phase=0.5mm,tcb@spec,segmentation@style]
    (segmentation.west)--(segmentation.east);%
  \fi%
}

\def\tcb@draw@pseudo@segmentation#1{%
\begingroup\tcb@shield@externalize\noindent\begin{tikzpicture}%
  \path[use as bounding box] (0,{\the\dimexpr-\kvtcb@middle-\kvtcb@boxsep\relax})
     rectangle (\linewidth,{\the\dimexpr\kvtcb@middle+\kvtcb@boxsep\relax});
  \node[line width=0mm,inner sep=0mm,draw=none,fill=none,rectangle,
        name=segmentation,at={({\the\dimexpr-\kvtcb@boxsep-(#1)\relax},0)},right,%
        minimum width=\tcb@innerwidth,minimum height=\the\dimexpr\kvtcb@middle*2\relax]{};
  \tcb@drawlower@path%
\end{tikzpicture}\endgroup}

\def\tcbline@star#1{%
{\parskip\z@\par\nointerlineskip}%
\xleaders\vbox{\tcb@draw@pseudo@segmentation{#1}}\vskip\dimexpr(\kvtcb@middle+\kvtcb@boxsep)*2\relax%
{\parskip\z@\par\nointerlineskip}}

\def\tcbline@#1{%
{\parskip\z@\par\nointerlineskip}%
\tcb@draw@pseudo@segmentation{#1}%
{\parskip\z@\par\nointerlineskip}}

\def\tcbline{%
  \@ifstar{\iftcb@hasLower\tcbline@star{\kvtcb@leftlower}\else\tcbline@star{\kvtcb@leftupper}\fi}%
  {\iftcb@hasLower\tcbline@{\kvtcb@leftlower+\@totalleftmargin}\else\tcbline@{\kvtcb@leftupper+\@totalleftmargin}\fi}}


% draw special versions
\def\tcb@drawspec@UT{%
  \tcb@pathbase{tcb fill interior}{segmentation.west}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@UR{%
  \tcb@pathbase{tcb fill interior}{segmentation.west}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@ins@NW}{\tcb@arc@ins@NE}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@US{%
  \tcb@pathbase{tcb fill interior}{segmentation.west}{interior.east|-frame.north}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@LR#1{%
  \tcb@pathbase{#1,segmentation@style}{interior.south west}{[yshift=0.1mm]segmentation.east}%
    {\tcb@arc@ins@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@LS#1{%
  \tcb@pathbase{#1,segmentation@style}{interior.west|-frame.south}{[yshift=0.1mm]segmentation.east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@A#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@NE}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@sbs@B#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@sbs@C#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@NE}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@D#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@E#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south|-frame.south}{interior.east|-frame.north}%
  {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@F#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south}{interior.east|-frame.north}%
  {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@T{%
  \tcb@pathbase{top color=tcbcolframe,bottom color=tcbcolback,fill opacity=\kvtcb@opacitybacktitle}{[yshift=-0.01pt]interior.north west}{[yshift=0.01pt]title.south east}%
  {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawframe@freelance{\tcb@frame@code}
\def\tcb@drawwithtitle@freelance{\tcb@interiortitled@code}
\def\tcb@drawwithouttitle@freelance{\tcb@interior@code}
\def\tcb@drawlower@freelance{\tcb@segmentation@code}
\def\tcb@drawtitle@freelance{\tcb@title@code}


\def\tcb@drawframe@spartan{%
  \begin{pgfscope}%
  \pgfpathrectangle{\pgfpointorigin}{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \pgfsetfillcolor{tcbcolframe}%
  \pgfsetfillopacity{\kvtcb@opacityframe}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawwithtitle@spartan{%
  \begin{pgfscope}%
  \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\kvtcb@bottom@rule}}%
   {\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight\relax}}%
  \pgfsetfillcolor{tcbcolback}%
  \pgfsetfillopacity{\kvtcb@opacityback}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawwithouttitle@spartan{%
  \begin{pgfscope}%
  \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\kvtcb@bottom@rule}}%
   {\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\the\dimexpr\tcb@height-\kvtcb@top@rule\relax}}%
  \pgfsetfillcolor{tcbcolback}%
  \pgfsetfillopacity{\kvtcb@opacityback}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawtitle@spartan{%
  \begin{pgfscope}%
  \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule\relax}}%
   {\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\the\dimexpr\tcb@height-\kvtcb@top@rule\relax}}%
  \pgfsetfillcolor{tcbcolbacktitle}%
  \pgfsetfillopacity{\kvtcb@opacitybacktitle}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawlower@spartan{%
  \begin{pgfscope}%
  \iftcb@sidebyside%
  \tcbdimto\tcb@seg@pos{\kvtcb@left@rule+\kvtcb@boxsep+\kvtcb@leftupper+\tcb@w@upper+\kvtcb@sbs@gap/2}%
  \pgfpathmoveto{\pgfqpoint{\tcb@seg@pos}{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight\relax}}%
  \pgfpathlineto{\pgfqpoint{\tcb@seg@pos}{\kvtcb@bottom@rule}}%
  \else%
  \tcbdimto\tcb@seg@pos{\kvtcb@bottom@rule+\kvtcb@boxsep*2+\tcb@break@bottomsep+\kvtcb@middle+\kvtcb@bottom+\tcb@height@lower}%
  \pgfpathmoveto{\pgfqpoint{\kvtcb@left@rule}{\tcb@seg@pos}}%
  \pgfpathlineto{\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\tcb@seg@pos}}%
  \fi%
  \pgfsetcolor{tcbcolframe}%
  \pgfsetstrokeopacity{\kvtcb@opacityframe}%
  \pgfusepath{stroke}%
  \end{pgfscope}%
}


\tcbset{%
  frame style/.code={\tikzset{frame@style/.style={#1}}},%
  frame hidden/.style={frame style={draw=none,fill=none}},
  frame engine/path/.style={frame code=\tcb@drawframe@path},
  frame engine/pathfirst/.style={frame code=\tcb@drawframe@pathfirst},
  frame engine/pathmiddle/.style={frame code=\tcb@drawframe@pathmiddle},
  frame engine/pathlast/.style={frame code=\tcb@drawframe@pathlast},
  frame engine/freelance/.style={frame code=\tcb@drawframe@standard},
  frame engine/spartan/.style={frame code=\tcb@drawframe@spartan},
  frame engine/empty/.style={frame code=},
  %
  interior titled engine/path/.style={interior titled code=\tcb@drawwithtitle@path},
  interior titled engine/pathfirst/.style={interior titled code=\tcb@drawwithtitle@pathfirst},
  interior titled engine/pathmiddle/.style={interior titled code=\tcb@drawwithtitle@pathmiddle},
  interior titled engine/pathlast/.style={interior titled code=\tcb@drawwithtitle@pathlast},
  interior titled engine/freelance/.style={interior titled code=\tcb@drawwithtitle@standard},
  interior titled engine/spartan/.style={interior titled code=\tcb@drawwithtitle@spartan},
  interior titled engine/empty/.style={interior titled code=},
  %
  interior engine/path/.style={interior code=\tcb@drawwithouttitle@path},
  interior engine/pathfirst/.style={interior code=\tcb@drawwithouttitle@pathfirst},
  interior engine/pathmiddle/.style={interior code=\tcb@drawwithouttitle@pathmiddle},
  interior engine/pathlast/.style={interior code=\tcb@drawwithouttitle@pathlast},
  interior engine/freelance/.style={interior code=\tcb@drawwithouttitle@standard},
  interior engine/spartan/.style={interior code=\tcb@drawwithouttitle@spartan},
  interior engine/empty/.style={interior code=},
  %
  segmentation engine/path/.style={segmentation code=\tcb@drawlower@path},
  segmentation engine/freelance/.style={segmentation code=\tcb@drawlower@standard},
  segmentation engine/spartan/.style={segmentation code=\tcb@drawlower@spartan},
  segmentation engine/empty/.style={segmentation code=},
  %
  title engine/path/.style={@title code=\tcb@drawtitle@path},
  title engine/pathfirst/.style={@title code=\tcb@drawtitle@pathfirst},
  title engine/pathmiddle/.style={@title code=\tcb@drawtitle@pathmiddle},
  title engine/pathlast/.style={@title code=\tcb@drawtitle@pathlast},
  title engine/freelance/.style={@title code=\tcb@drawtitle@standard},
  title engine/spartan/.style={@title code=\tcb@drawtitle@spartan},
  title engine/empty/.style={@title code=},
  %
  interior style/.code={\tikzset{interior@style/.style={#1}}},%
  interior hidden/.style={interior style={draw=none,fill=none}},
  segmentation style/.code={\tikzset{segmentation@style/.style={#1}}},%
  segmentation hidden/.style={segmentation style={draw=none,fill=none}},
  @title style/.code={\tikzset{title@style/.style={#1}}},%
  title style/.style={title filled,@title style={#1}},
  title hidden/.style={title style={draw=none,fill=none}},
  titlerule style/.style={%
    underlay={\iftcb@hasTitle%
      \path[draw,line width=\kvtcb@title@rule+1000sp,#1]
        ([yshift=-\kvtcb@title@rule/2]title.south west)--([yshift=-\kvtcb@title@rule/2]title.south east);
    \fi}},%
  colbacklower/.colorlet=tcbcolbacklower,%
  clear@spec/.code={\tcb@spec{}},%
  tikz/.code={\appto\tcb@tikz@option@hook{,#1}},%
  tikz reset/.code={\let\tcb@tikz@option@hook\@empty},%
  at begin tikz/.code={\appto\tcb@tikz@begin@hook{#1}},%
  at begin tikz reset/.code={\let\tcb@tikz@begin@hook\@empty},%
  at end tikz/.code={\appto\tcb@tikz@end@hook{#1}},%
  at end tikz reset/.code={\let\tcb@tikz@end@hook\@empty},%
  rotate/.style={tikz={rotate=#1,transform shape}},%
  scale/.style={tikz={scale=#1,transform shape},%
    at begin tikz={%
    \tcbdimto\kvtcb@arc{#1\dimexpr\kvtcb@arc}%
    \tcbdimto\tcb@outer@arc{#1\dimexpr\tcb@outer@arc}%
    \def\tcb@shadow@comp@arc{%
      \tcbdimto\tcb@shadow@ts{#1\dimexpr\tcb@shadow@ts}%
      \ifdim\dimexpr\tcb@outer@arc>\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax%
        \tcbdimto\tcb@shadow@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax}%
      \else%
        \let\tcb@shadow@arc=\tcb@zpt%
      \fi%
    }%
    }},%
  remember/.style={tikz={remember picture}},%
  remember as/.style={tikz={remember picture},at end tikz={\pgfnodealias{#1}{frame}}},%
}

\tcbset{%
  base@unbroken/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@standard,%
    shape@of@skin=unbroken,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@unbroken\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
  base@first/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@pathfirst,%
    shape@of@skin=first,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@first\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
  base@middle/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@pathmiddle,%
    shape@of@skin=middle,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@middle\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
  base@last/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@pathlast,%
    shape@of@skin=last,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@last\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
}

\tcb@new@skin{enhanced}{base@unbroken,%
  frame engine=path,interior titled engine=path,interior engine=path,segmentation engine=path,title engine=path,%
  skin first=enhancedfirst,skin middle=enhancedmiddle,skin last=enhancedlast}

\tcb@new@skin{enhancedfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=pathfirst,interior engine=pathfirst,segmentation engine=path,title engine=pathfirst,%
  skin first=enhancedfirst,skin middle=enhancedmiddle,skin last=enhancedmiddle}

\tcb@new@skin{enhancedmiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=pathmiddle,interior engine=pathmiddle,segmentation engine=path,title engine=pathmiddle,%
  skin first=enhancedmiddle,skin middle=enhancedmiddle,skin last=enhancedmiddle}

\tcb@new@skin{enhancedlast}{base@last,%
  frame engine=pathlast,interior titled engine=pathlast,interior engine=pathlast,segmentation engine=path,title engine=pathlast,%
  skin first=enhancedmiddle,skin middle=enhancedmiddle,skin last=enhancedlast}

\tcbset{enhanced/.style={skin=enhanced},%
  enhanced standard/.style={skin=enhanced,
    skin first=enhanced,skin middle=enhanced,skin last=enhanced},%
  blank/.style={enhanced,frame hidden,interior hidden,segmentation hidden,%
    arc=0pt,outer arc=0pt,boxsep=0pt,top=0pt,bottom=0pt,left=0pt,right=0pt,boxrule=0pt,%
    bottomtitle=6pt,middle=3pt}}

\tcb@new@skin{empty}{base@unbroken,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptyfirst,skin middle=emptymiddle,skin last=emptylast}

\tcb@new@skin{emptyfirst}{base@first,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptyfirst,skin middle=emptymiddle,skin last=emptymiddle}

\tcb@new@skin{emptymiddle}{base@middle,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptymiddle,skin middle=emptymiddle,skin last=emptymiddle}

\tcb@new@skin{emptylast}{base@last,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptymiddle,skin middle=emptymiddle,skin last=emptylast}

\tcbset{empty/.style={skin=empty},%
  blanker/.style={empty,arc=0pt,outer arc=0pt,boxsep=0pt,top=0pt,bottom=0pt,left=0pt,right=0pt,boxrule=0pt,%
    bottomtitle=6pt,middle=3pt},
  blankest/.style={blanker,notitle,
    no shadow,no underlay,no overlay,no finish,no borderline},
  }

\tcb@new@skin{freelance}{base@unbroken,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancefirst,skin middle=freelancemiddle,skin last=freelancelast}%

\tcb@new@skin{freelancefirst}{base@first,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancefirst,skin middle=freelancemiddle,skin last=freelancemiddle}%

\tcb@new@skin{freelancemiddle}{base@middle,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancemiddle,skin middle=freelancemiddle,skin last=freelancemiddle}%

\tcb@new@skin{freelancelast}{base@last,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancemiddle,skin middle=freelancemiddle,skin last=freelancelast}%

\tcbset{freelance/.style={skin=freelance},
  % for backward compatibility:
  extend freelance/.style={#1},%
  extend freelancefirst/.style={skin first is subskin of={freelancefirst}{#1}},%
  extend freelancemiddle/.style={skin middle is subskin of={freelancemiddle}{#1}},%
  extend freelancelast/.style={skin last is subskin of={freelancelast}{#1}}}

\tcb@new@skin{bicolor}{base@unbroken,%
  frame engine=path,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=path,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcbsegmentstate%
      {\tcb@spec{fill=tcbcolback}\tcb@drawwithtitle@path}%
      \or%
      \tcb@spec{fill=tcbcolback}\tcb@drawspec@UT%
      \else%
      {\tcbset{interior style={fill=tcbcolbacklower,segmentation@style}}\tcb@drawwithtitle@path}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcolback}\tcb@drawwithtitle@path}%
    \fi\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcbsegmentstate%
      {\tcb@spec{fill=tcbcolback}\tcb@drawwithouttitle@path}%
      \or%
      \tcb@spec{fill=tcbcolback}\tcb@drawspec@UR%
      \else%
      {\tcbset{interior style={fill=tcbcolbacklower,segmentation@style}}\tcb@drawwithouttitle@path}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcolback}\tcb@drawwithouttitle@path}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@B{fill=tcbcolbacklower}\else%
    \tcb@drawspec@sbs@A{fill=tcbcolbacklower}\fi\else\tcb@drawspec@LR{fill=tcbcolbacklower}\fi\tcb@spec{}},%
  skin first=bicolorfirst,skin middle=bicolormiddle,skin last=bicolorlast}

\tcbset{bicolor/.style={skin=bicolor}}

\tcb@new@skin{bicolorfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathfirst,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcbsegmentstate%
      {\tcb@spec{fill=tcbcolback}\tcb@drawwithtitle@pathfirst}%
      \or%
      \tcb@spec{fill=tcbcolback}\tcb@drawspec@UT%
      \else%
      {\tcbset{interior style={fill=tcbcolbacklower,segmentation@style}}\tcb@drawwithtitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcolback}\tcb@drawwithtitle@pathfirst}%
    \fi\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcbsegmentstate%
      {\tcb@spec{fill=tcbcolback}\tcb@drawwithouttitle@pathfirst}%
      \or%
      \tcb@spec{fill=tcbcolback}\tcb@drawspec@UR%
      \else%
      {\tcbset{interior style={fill=tcbcolbacklower,segmentation@style}}\tcb@drawwithouttitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcolback}\tcb@drawwithouttitle@pathfirst}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@D{fill=tcbcolbacklower}\else%
    \tcb@drawspec@sbs@C{fill=tcbcolbacklower}\fi\else\tcb@drawspec@LS{fill=tcbcolbacklower}\fi\tcb@spec{}},%
  skin first=bicolorfirst,skin middle=bicolormiddle,skin last=bicolormiddle}

\tcb@new@skin{bicolormiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathmiddle,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcbsegmentstate%
      {\tcb@spec{fill=tcbcolback}\tcb@drawwithtitle@pathmiddle}%
      \or%
      \tcb@spec{fill=tcbcolback}\tcb@drawspec@UT%
      \else%
      {\tcbset{interior style={fill=tcbcolbacklower,segmentation@style}}\tcb@drawwithtitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcolback}\tcb@drawwithtitle@pathmiddle}%
    \fi\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcbsegmentstate%
      {\tcb@spec{fill=tcbcolback}\tcb@drawwithouttitle@pathmiddle}%
      \or%
      \tcb@spec{fill=tcbcolback}\tcb@drawspec@US%
      \else%
      {\tcbset{interior style={fill=tcbcolbacklower,segmentation@style}}\tcb@drawwithouttitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcolback}\tcb@drawwithouttitle@pathmiddle}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@D{fill=tcbcolbacklower}\else%
    \tcb@drawspec@sbs@E{fill=tcbcolbacklower}\fi\else\tcb@drawspec@LS{fill=tcbcolbacklower}\fi\tcb@spec{}},%
  skin first=bicolormiddle,skin middle=bicolormiddle,skin last=bicolormiddle}

\tcb@new@skin{bicolorlast}{base@last,%
  frame engine=pathlast,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathlast,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcbsegmentstate
      {\tcb@spec{fill=tcbcolback}\tcb@drawwithtitle@pathlast}%
      \or%
      \tcb@spec{fill=tcbcolback}\tcb@drawspec@UT%
      \else%
      {\tcbset{interior style={fill=tcbcolbacklower,segmentation@style}}\tcb@drawwithtitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcolback}\tcb@drawwithtitle@pathlast}%
    \fi\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcbsegmentstate%
      {\tcb@spec{fill=tcbcolback}\tcb@drawwithouttitle@pathlast}%
      \or%
      \tcb@spec{fill=tcbcolback}\tcb@drawspec@US%
      \else
      {\tcbset{interior style={fill=tcbcolbacklower,segmentation@style}}\tcb@drawwithouttitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcolback}\tcb@drawwithouttitle@pathlast}%
    \fi\tcb@spec{}},%
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@B{fill=tcbcolbacklower}\else%
    \tcb@drawspec@sbs@F{fill=tcbcolbacklower}\fi\else\tcb@drawspec@LR{fill=tcbcolbacklower}\fi\tcb@spec{}},%
  skin first=bicolormiddle,skin middle=bicolormiddle,skin last=bicolorlast}

\tcb@new@skin{tile}{skin@bicolor,frame engine=empty,%
  skin first=tilefirst,skin middle=tilemiddle,skin last=tilelast}

\tcbset{tile/.style={skin=tile,boxrule=0pt,sharp corners,title filled,fonttitle=\bfseries}}

\tcb@new@skin{tilefirst}{skin@bicolorfirst,frame engine=empty,%
  skin first=tilefirst,skin middle=tilemiddle,skin last=tilemiddle}

\tcb@new@skin{tilemiddle}{skin@bicolormiddle,frame engine=empty,%
  skin first=tilemiddle,skin middle=tilemiddle,skin last=tilemiddle}

\tcb@new@skin{tilelast}{skin@bicolorlast,frame engine=empty,%
  skin first=tilemiddle,skin middle=tilemiddle,skin last=tilelast}

\tikzset{beamer@color/.style={fill=none,top color=tcbcolback,bottom color=tcbcolback!85!black}}

\tcb@new@skin{beamer}{base@unbroken,%
  frame engine=path,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=path,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcbsegmentstate=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@path}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@path}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcbsegmentstate=1
      \tcb@spec{beamer@color}\tcb@drawspec@UR%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@path}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@path}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LR{beamer@color}\fi\tcb@spec{}},%
  skin first=beamerfirst,skin middle=beamermiddle,skin last=beamerlast}

\tcbset{beamer/.style={skin=beamer,boxrule=0mm,titlerule=1mm,toptitle=0.5mm,arc=2mm,fonttitle=\bfseries,drop fuzzy shadow}}

\tcb@new@skin{beamerfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathfirst,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcbsegmentstate=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathfirst}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcbsegmentstate=1
      \tcb@spec{beamer@color}\tcb@drawspec@UR%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathfirst}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LS{beamer@color}\fi\tcb@spec{}},%
  skin first=beamerfirst,skin middle=beamermiddle,skin last=beamermiddle}

\tcb@new@skin{beamermiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathmiddle,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcbsegmentstate=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathmiddle}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcbsegmentstate=1
      \tcb@spec{beamer@color}\tcb@drawspec@US%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathmiddle}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LS{beamer@color}\fi\tcb@spec{}},%
  skin first=beamermiddle,skin middle=beamermiddle,skin last=beamermiddle}

\tcb@new@skin{beamerlast}{base@last,%
  frame engine=pathlast,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathlast,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcbsegmentstate=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathlast}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcbsegmentstate=1
      \tcb@spec{beamer@color}\tcb@drawspec@US%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathlast}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LR{beamer@color}\fi\tcb@spec{}},%
  skin first=beamermiddle,skin middle=beamermiddle,skin last=beamerlast}

\def\tcb@drawspec@widgetsegment{%
  \iftcb@sidebyside%
  \tcb@drawlower@path%
  \else%
  \path[left color=tcbcolframe!75!white,right color=tcbcolframe!75!white!25!tcbcolback,segmentation@style]
    ([yshift={-\kvtcb@middle/4}]segmentation.west) rectangle ([yshift={\kvtcb@middle/4}]segmentation.east);
  \fi%
}

\tikzset{widget@color/.style={left color=tcbcolframe!75!white,right color=tcbcolframe!75!white!25!tcbcolback}}

\tcb@new@skin{widget}{base@unbroken,%
  frame engine=path,interior titled engine=path,interior engine=path,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@path}},
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetfirst,skin middle=widgetmiddle,skin last=widgetlast}

\tcbset{widget/.style={skin=widget,arc=0.5mm,fonttitle=\bfseries,titlerule=0mm,toprule at break=0mm}}

\tcb@new@skin{widgetfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=pathfirst,interior engine=pathfirst,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@pathfirst}},%
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetfirst,skin middle=widgetmiddle,skin last=widgetmiddle}

\tcb@new@skin{widgetmiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=pathmiddle,interior engine=pathmiddle,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@pathmiddle}},%
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetmiddle,skin middle=widgetmiddle,skin last=widgetmiddle}

\tcb@new@skin{widgetlast}{base@last,%
  frame engine=pathlast,interior titled engine=pathlast,interior engine=pathlast,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@pathlast}},
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetmiddle,skin middle=widgetmiddle,skin last=widgetlast}

\tcb@new@skin{spartan}{graphical environment=tikzpicture@tcb@hooked,geometry nodes=true,shape@of@skin=unbroken,%
  set@extensions@preframe=,set@extensions@postframe={\tcb@apply@underlay},set@extensions@final=,%
  frame engine=spartan,interior titled engine=spartan,interior engine=spartan,title engine=spartan,segmentation engine=spartan,%
  set@outerboundary=\tcb@boundaryframe@standard,%
  skin first=spartan,skin middle=spartan,skin last=spartan}

\tcbset{spartan/.style={skin=spartan}}

\tcb@new@skin{draft}{clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,shape@of@skin=unbroken,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=path,title empty,%
  segmentation style={draw=black,dashed},
  set@extensions@postframe=,
  set@extensions@final={\tcb@apply@finish},no finish,%
  colupper=black!50!white,collower=black!50!white,coltitle=black!50!white,
  frame code={%
    \path[draw=blue!10!white,double,line width=1pt,dashed] (current bounding box.south west) rectangle (current bounding box.north east);
    {\tcb@spec{fill=black!15!white,draw=black}\tcb@drawframe@path}%
    \iftcb@hasTitle%
      \path[fill=red!10!white,draw,dotted,rounded corners=\kvtcb@arc]
        ([xshift={\kvtcb@left@rule},yshift={\kvtcb@bottom@rule}]frame.south west) rectangle
        (interior.north east);
      \path[fill=red!10!white,draw,dotted,rounded corners=\kvtcb@arc]
        ([yshift={\kvtcb@title@rule}]interior.north west) rectangle
        ([xshift={-\kvtcb@right@rule},yshift={-\kvtcb@top@rule}]frame.north east);
      \path[fill=white,draw,dotted]
        ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep}]title.south west) rectangle
        ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep}]title.north east);
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@lefttitle},yshift={\kvtcb@boxsep+\kvtcb@bottomtitle}]title.south west)
         rectangle node[font=\scriptsize] {title: w=\tcb@w@title, h=\tcb@h@title}
        +(\tcb@w@title,\tcb@h@title);
      \path[draw=red,opacity=0.5] (title.south west) rectangle (title.north east);
    \else%
      \path[fill=red!10!white,draw,dotted,rounded corners=\kvtcb@arc]
        ([xshift={\kvtcb@left@rule},yshift={\kvtcb@bottom@rule}]frame.south west) rectangle
        ([xshift={-\kvtcb@right@rule},yshift={-\kvtcb@top@rule}]frame.north east);
    \fi%
    \ifcase\tcbsegmentstate
      \path[fill=white,draw,dotted]
        ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
        ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@leftupper},yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]interior.south west)
        rectangle node[font=\scriptsize] {upper: w=\tcb@w@upper, h=\tcb@height@upper}
        +(\tcb@w@upper,\tcb@height@upper);
      \iftcb@sidebyside%
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]segmentation.south east)
        rectangle node[font=\scriptsize] {lower: w=\tcb@w@lower, h=\tcb@height@upper}
        +(\tcb@w@lower,\tcb@height@upper);
      \fi%
    \or%
      \ifdim\wd\tcb@upperbox=0pt\relax
        \path[fill=white,draw,dotted]
          ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
          ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
      \else
        \path[fill=white,draw,dotted]
          ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
          ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep}]segmentation.east);
        \path[fill=white,draw,dotted]
           ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep}]segmentation.west)
           rectangle ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
        \path[fill=green!20!white,draw=green!75!black,dashed]
          ([xshift={\kvtcb@boxsep+\kvtcb@leftupper},yshift={\kvtcb@boxsep}]segmentation.north west)
           rectangle node[font=\scriptsize] {upper: w=\tcb@w@upper, h=\tcb@height@upper}
           +(\tcb@w@upper,\tcb@height@upper);
      \fi%
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@leftlower},yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]interior.south west)
        rectangle  node[font=\scriptsize] {lower: w=\tcb@w@lower, h=\tcb@height@lower}
        +(\tcb@w@lower,\tcb@height@lower);
      \path[draw=red,opacity=0.5] (segmentation.south west) rectangle (segmentation.north east);
    \else
      \path[fill=white,draw,dotted]
        ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
        ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@leftlower},yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]interior.south west)
        rectangle  node[font=\scriptsize] {lower: w=\tcb@w@lower, h=\tcb@height@lower}
        +(\tcb@w@lower,\tcb@height@lower);
    \fi%
    \path[draw=red,opacity=0.5] (interior.south west) rectangle (interior.north east);
    \path[draw=red,opacity=0.5] (frame.south west) rectangle (frame.north east);
    \node[above,font=\scriptsize,red!50!black] at (interior.south) {interior: w=\tcb@innerwidth, h=\tcb@innerheight};
    \node[above,font=\scriptsize,red!50!black] at (frame.north) {frame: w=\the\dimexpr\tcb@width\relax, h=\tcb@height};
    \path[draw=blue!10!white,double,line width=1pt,dashed,opacity=0.3] (current bounding box.south west) rectangle (current bounding box.north east);
    \pgfsetfillopacity{0.3}
  },
  skin first=draft,skin middle=draft,skin last=draft}

\tcbset{draft/.style={skin=draft}}

\tikzset{%
  tcb@forced@clip/.code={\tikz@addmode{\tikz@mode@cliptrue}\let\tikz@options=\pgfutil@empty},%
  tcb@invclip/.style={clip,insert path={{[reset cm]\pgfextra{%
    \pgfpathmoveto{\pgfqpoint{-16383.99999pt}{-16383.99999pt}}%
    \pgfpathlineto{\pgfqpoint{16383.99999pt}{-16383.99999pt}}%
    \pgfpathlineto{\pgfqpoint{16383.99999pt}{16383.99999pt}}%
    \pgfpathlineto{\pgfqpoint{-16383.99999pt}{16383.99999pt}}%
    \pgfpathclose}}}}%
}%

\def\tcb@clip@frame{\tcb@pathboundary{clip}{\tcb@outerboundary}}

\def\tcb@invclip@frame{\tcb@pathboundary{tcb@invclip}{\tcb@outerboundary}}

\def\tcb@clip@interior{%
  \begingroup%
  \tcbset{interior hidden}%
  \tcb@spec{tcb@forced@clip}%
  \def\tcb@spec##1{}%
  \iftcb@hasTitle%
    \tcb@interiortitled@code%
  \else%
    \tcb@interior@code%
  \fi%
  \endgroup%
}

\def\tcb@clip@title{%
  \begingroup%
  \tcbset{title hidden}%
  \tcb@spec{tcb@forced@clip}%
  \def\tcb@spec##1{}%
    \iftcb@hasTitle%
      \tcb@title@code%
    \fi%
  \endgroup%
}

\newenvironment{tcbclipframe}{\begin{scope}\tcb@clip@frame}{\end{scope}}
\newenvironment{tcbinvclipframe}{\begin{scope}\tcb@invclip@frame}{\end{scope}}
\newenvironment{tcbclipinterior}{\begin{scope}\tcb@clip@interior}{\end{scope}}
\newenvironment{tcbcliptitle}{\begin{scope}\tcb@clip@title}{\end{scope}}

\def\tcb@apply@underlay{\csname tcb@underlay@\tcb@split@state\endcsname}%
\def\tcb@apply@finish{\csname tcb@finish@\tcb@split@state\endcsname}%

\tcbset{%
  underlay unbroken/.code={\appto\tcb@underlay@unbroken{#1}},%
  underlay first/.code={\appto\tcb@underlay@first{#1}},%
  underlay middle/.code={\appto\tcb@underlay@middle{#1}},%
  underlay last/.code={\appto\tcb@underlay@last{#1}},%
  underlay boxed title/.code={\appto\tcb@underlay@boxedtitle{#1}},%
  underlay/.style={underlay unbroken={#1},underlay first={#1},underlay middle={#1},underlay last={#1}},%
  underlay broken/.style={underlay first={#1},underlay middle={#1},underlay last={#1}},%
  underlay unbroken and first/.style={underlay unbroken={#1},underlay first={#1}},%
  underlay unbroken and last/.style={underlay unbroken={#1},underlay last={#1}},%
  underlay middle and last/.style={underlay middle={#1},underlay last={#1}},%
  underlay first and middle/.style={underlay first={#1},underlay middle={#1}},%
  no underlay unbroken/.code={\let\tcb@underlay@unbroken\@empty},%
  no underlay first/.code={\let\tcb@underlay@first\@empty},%
  no underlay middle/.code={\let\tcb@underlay@middle\@empty},%
  no underlay last/.code={\let\tcb@underlay@last\@empty},%
  no underlay boxed title/.code={\let\tcb@underlay@boxedtitle\@empty},%
  no underlay/.style={no underlay unbroken,no underlay first,no underlay middle,no underlay last,no underlay boxed title},%
  finish unbroken/.code={\appto\tcb@finish@unbroken{#1}},%
  finish first/.code={\appto\tcb@finish@first{#1}},%
  finish middle/.code={\appto\tcb@finish@middle{#1}},%
  finish last/.code={\appto\tcb@finish@last{#1}},%
  finish/.style={finish unbroken={#1},finish first={#1},finish middle={#1},finish last={#1}},%
  finish broken/.style={finish first={#1},finish middle={#1},finish last={#1}},%
  finish unbroken and first/.style={finish unbroken={#1},finish first={#1}},%
  finish unbroken and last/.style={finish unbroken={#1},finish last={#1}},%
  finish middle and last/.style={finish middle={#1},finish last={#1}},%
  finish first and middle/.style={finish first={#1},finish middle={#1}},%
  no finish unbroken/.code={\let\tcb@finish@unbroken\@empty},%
  no finish first/.code={\let\tcb@finish@first\@empty},%
  no finish middle/.code={\let\tcb@finish@middle\@empty},%
  no finish last/.code={\let\tcb@finish@last\@empty},%
  no finish/.style={no finish unbroken,no finish first,no finish middle,no finish last},%
}

\def\tcb@trans@set@boxedsize@copy@top{%
  \begingroup\edef\x{\endgroup\noexpand\def\noexpand\tcb@trans@boxedsize{%
    leftrule=\kvtcb@left@rule,rightrule=\kvtcb@right@rule,
    toprule=\kvtcb@top@rule@stand,bottomrule=\kvtcb@title@rule,
    boxsep=\kvtcb@boxsep,leftupper=\kvtcb@lefttitle,rightupper=\kvtcb@righttitle,
    top=\kvtcb@toptitle,bottom=\kvtcb@bottomtitle,arc=\kvtcb@arc,
    sharp corners=south,
  }}\x}%
\def\tcb@trans@set@boxedsize@copy@bottom{%
  \begingroup\edef\x{\endgroup\noexpand\def\noexpand\tcb@trans@boxedsize{%
    leftrule=\kvtcb@left@rule,rightrule=\kvtcb@right@rule,
    toprule=\kvtcb@title@rule,bottomrule=\kvtcb@bottom@rule@stand,
    boxsep=\kvtcb@boxsep,leftupper=\kvtcb@lefttitle,rightupper=\kvtcb@righttitle,
    top=\kvtcb@toptitle,bottom=\kvtcb@bottomtitle,arc=\kvtcb@arc,
    sharp corners=north,
  }}\x}%

\tcbset{%
  boxed title size/.is choice,
  boxed title size/standard/.code={\def\tcb@trans@set@boxedsize##1{\let\tcb@trans@boxedsize\@empty}},
  boxed title size/title/.code={\def\tcb@trans@set@boxedsize##1{\def\tcb@trans@boxedsize{size=title}}},
  boxed title size/copy/.code={\def\tcb@trans@set@boxedsize##1{%
    \ifstrequal{##1}{top}{\tcb@trans@set@boxedsize@copy@top}{\tcb@trans@set@boxedsize@copy@bottom}}},
  before@boxed@title/.store in=\kvtcb@before@boxedtitle,%
  after@boxed@title/.store in=\kvtcb@after@boxedtitle,%
  boxed title style/.code={\appto\kvtcb@style@boxedtitle{,#1}},%
  no boxed title style/.code={\let\kvtcb@style@boxedtitle\@empty},%
  %
  varwidth boxed title/.style={before@boxed@title={\tcbdimto\tcb@w@title{#1}\begin{varwidth}{\tcb@w@title}},after@boxed@title={\end{varwidth}}},%
  varwidth boxed title/.default={\kvtcb@width-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@lefttitle)-(\kvtcb@righttitle)},
  varwidth boxed title*/.style={varwidth boxed title={\kvtcb@width+#1}},
  varwidth boxed title*/.default={0pt-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@lefttitle)-(\kvtcb@righttitle)},
  %
  minipage boxed title/.style={before@boxed@title={\tcbdimto\tcb@w@title{#1}\begin{minipage}{\tcb@w@title}},after@boxed@title={\end{minipage}}},%
  minipage boxed title/.default={\kvtcb@width-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@lefttitle)-(\kvtcb@righttitle)},
  minipage boxed title*/.style={minipage boxed title={\kvtcb@width+#1}},
  minipage boxed title*/.default={0pt-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@lefttitle)-(\kvtcb@righttitle)},
  %
  tikznode boxed title/.style={before@boxed@title={\centering\tcb@shield@externalize\begin{tikzpicture}\node[align=center,inner sep=0pt,outer sep=0pt,#1]\bgroup},after@boxed@title={\egroup;\end{tikzpicture}}},%
  hbox boxed title/.style={before@boxed@title=,after@boxed@title=},%
  %
  boxtitle/xshift/.dimstore in=\kvtcb@xshift@boxedtitle,%
  boxtitle/yshift/.dimstore in=\kvtcb@yshift@boxedtitle,%
  boxtitle/yshifttext/.dimstore in=\kvtcb@yinnershift@boxedtitle,%
  %
  boxtitle/yshift*@top/.style={yshift*/.code={%
    \tcbdimto\kvtcb@yshift@boxedtitle{##1}%
    \tcbdimto\kvtcb@yinnershift@boxedtitle{\kvtcb@yshift@boxedtitle+\kvtcb@top@rule@stand}%
    \ifdim\dimexpr\kvtcb@yinnershift@boxedtitle>0pt\relax\let\kvtcb@yinnershift@boxedtitle\tcb@zpt\fi%
  }},
  boxtitle/yshift*@bottom/.style={yshift*/.code={%
    \tcbdimto\kvtcb@yshift@boxedtitle{##1}%
    \tcbdimto\kvtcb@yinnershift@boxedtitle{\kvtcb@yshift@boxedtitle-\kvtcb@bottom@rule@stand}%
    \ifdim\dimexpr\kvtcb@yinnershift@boxedtitle<0pt\relax\let\kvtcb@yinnershift@boxedtitle\tcb@zpt\fi%
  }},
  boxtitle/adapt@top/.code={%
    \ifdim\dimexpr\tcboxedtitleheight+\kvtcb@yshift@boxedtitle>0pt\relax
      \tcbdimto\kvtcb@bbtop@stand{\kvtcb@bbtop@stand+\tcboxedtitleheight+\kvtcb@yshift@boxedtitle}%
    \fi%
    \tcbdimto\kvtcb@top{\kvtcb@top-\kvtcb@yinnershift@boxedtitle}%
  },
  boxtitle/adapt@bottom/.code={%
    \ifdim\dimexpr\tcboxedtitleheight-\kvtcb@yshift@boxedtitle>0pt\relax
      \tcbdimto\kvtcb@bbbottom@stand{\kvtcb@bbbottom@stand+\tcboxedtitleheight-\kvtcb@yshift@boxedtitle}%
    \fi%
    \tcbdimto\kvtcb@bottom{\kvtcb@bottom+\kvtcb@yinnershift@boxedtitle}%
  },
  attach@title@boxed/.style n args={5}{%
    detach title,
    code={\def\tcb@specialtitle@hook{%
      \ifx\tcbtitletext\@empty\else%
      \tcb@trans@set@boxedsize{#2}%
      \colorlet{tcbtranscol@frame}{tcbcolframe}%
      \colorlet{tcbtranscol@back}{tcbcolbacktitle}%
      \let\tcb@trans@skin@current\kvtcb@skin@current%
      \let\tcb@trans@boxedstyle\kvtcb@style@boxedtitle%
      \setbox\tcb@titlebox\color@hbox\bgroup\color{tcbcoltitle}\kvtcb@fonttitle\kvtcb@before@boxedtitle\kvtcb@haligntitle\kvtcb@before@title\tcbtitletext\kvtcb@after@title\kvtcb@after@boxedtitle\egroup\color@endbox%
      \setbox\tcb@titlebox\color@hbox\tcbox[skin=\tcb@trans@skin@current,colframe=tcbtranscol@frame,colback=tcbtranscol@back,%
        code={\pgfkeysalsofrom\tcb@trans@boxedsize\pgfkeysalsofrom\tcb@trans@boxedstyle}]{\box\tcb@titlebox}\color@endbox%
      %
      \tcbdimto\tcboxedtitleheight{\ht\tcb@titlebox+\dp\tcb@titlebox}%
      \tcbdimto\tcboxedtitlewidth{\wd\tcb@titlebox}%
      \tcbset{boxtitle/.cd,xshift=0pt,yshift=0pt,yshifttext=0pt,yshift*@#2,#1,adapt@#2}%
      \let\tcb@specialgeonodes@first\relax%
      \let\tcb@specialgeonodes@middle\relax%
      \let\tcb@specialgeonodes@last\relax%
      \def\tcb@specialgeonodes@unbroken{%
        \node[#4,name=title,at={([xshift=\kvtcb@xshift@boxedtitle,yshift=\kvtcb@yshift@boxedtitle]frame.#5)},
                minimum width=\tcboxedtitlewidth,minimum height=\tcboxedtitleheight]{};}%
      \cslet{tcb@specialgeonodes@#3}{\tcb@specialgeonodes@unbroken}%
      \def\tcb@specialgeonodes@hook{\csname tcb@specialgeonodes@\tcb@split@state\endcsname}%
      \preto\tcb@underlay@unbroken{\tcb@underlay@boxedtitle\pgftext[at={\pgfpointanchor{title}{center}}]{\box\tcb@titlebox}}%
      \cspreto{tcb@underlay@#3}{\tcb@underlay@boxedtitle\pgftext[at={\pgfpointanchor{title}{center}}]{\box\tcb@titlebox}}%
      \fi}}%
    },
  attach@title@boxed@top/.style n args={3}{attach@title@boxed={#1}{top}{first}{#2}{#3}},%
  attach@title@boxed@bottom/.style n args={3}{attach@title@boxed={#1}{bottom}{last}{#2}{#3}},%
  %
  attach boxed title to top left/.style={attach@title@boxed@top={#1}{above right}{north west}},
  attach boxed title to top center/.style={attach@title@boxed@top={#1}{above}{north}},
  attach boxed title to top right/.style={attach@title@boxed@top={#1}{above left}{north east}},
  attach boxed title to bottom left/.style={attach@title@boxed@bottom={#1}{below right}{south west}},
  attach boxed title to bottom center/.style={attach@title@boxed@bottom={#1}{below}{south}},
  attach boxed title to bottom right/.style={attach@title@boxed@bottom={#1}{below left}{south east}},
  reduce@vertical@rules/.code={%
    \ifdim\dimexpr\kvtcb@left@rule<\dimexpr\kvtcb@right@rule\relax%
      \tcbdimto\tcb@temp{\kvtcb@left@rule/2}%
    \else%
      \tcbdimto\tcb@temp{\kvtcb@right@rule/2}%
    \fi%
    \tcbset{leftrule/.expanded=\the\dimexpr\kvtcb@left@rule-\tcb@temp\relax,
      rightrule/.expanded=\the\dimexpr\kvtcb@right@rule-\tcb@temp\relax}%
  },
  attach boxed title to bottom/.style={%
    attach boxed title to bottom center={yshift*=\tcboxedtitleheight,#1},
    minipage boxed title,boxed title size=copy,
  },
  attach boxed title to bottom*/.style={%
    attach boxed title to bottom={#1},
    boxed title style={reduce@vertical@rules},
  },
  attach boxed title to top/.style={%
    attach boxed title to top center={yshift*=-\tcboxedtitleheight,#1},
    minipage boxed title,boxed title size=copy,
  },
  attach boxed title to top*/.style={%
    attach boxed title to top={#1},
    boxed title style={reduce@vertical@rules},
  },
  flip title/.style={attach boxed title to bottom,
    boxed title style={reduce@vertical@rules,#1}},
}


\newbox\tcb@waterbox

\def\tcb@setratio#1#2#3{\edef#1{\strip@pt\dimexpr\number\numexpr\number\dimexpr#2\relax*65536/\number\dimexpr#3\relax\relax sp\relax}}

\def\tcb@setratiorobust#1#2#3{\ifdim\dimexpr#3<1pt\tcb@setratio#1{#2}{1pt}\else\tcb@setratio#1{#2}{#3}\fi}

\def\tcb@comp@waterbox@stretch#1#2#3{%
  \tcb@setratiorobust\tcb@scale@x{#1\dimexpr#2}{\wd\tcb@waterbox}%
  \tcb@setratiorobust\tcb@scale@y{#1\dimexpr#3}{\ht\tcb@waterbox+\dp\tcb@waterbox}%
}

\def\tcb@comp@waterbox@zoom#1#2#3{%
  \tcb@comp@waterbox@stretch{#1}{#2}{#3}%
  \ifdim\dimexpr\tcb@scale@x pt\relax<\dimexpr\tcb@scale@y pt\relax\let\tcb@scale@y=\tcb@scale@x\else\let\tcb@scale@x=\tcb@scale@y\fi%
}

\def\tcb@comp@waterbox@overzoom#1#2#3{%
  \tcb@comp@waterbox@stretch{#1}{#2}{#3}%
  \ifdim\dimexpr\tcb@scale@x pt\relax>\dimexpr\tcb@scale@y pt\relax\let\tcb@scale@y=\tcb@scale@x\else\let\tcb@scale@x=\tcb@scale@y\fi%
}

\def\tcb@comp@waterbox@shrink#1#2#3{%
  \tcb@comp@waterbox@zoom{#1}{#2}{#3}%
  \ifdim\dimexpr\tcb@scale@x pt\relax>1pt\relax%
    \edef\tcb@scale@x{1}\edef\tcb@scale@y{1}%
  \fi%
}

\def\tcb@box@scaled@waterbox{\scalebox{\tcb@scale@x}[\tcb@scale@y]{\box\tcb@waterbox}}

\def\tcb@drawspec@watermark@@noclip{%
  \tcb@comp@wm%
  \node[opacity=\kvtcb@watermark@opacity,anchor=center] at (interior) {\tcb@box@scaled@waterbox};%
}

\def\tcb@drawspec@watermark@@clip{%
  \begin{tcbclipinterior}%
  \tcb@drawspec@watermark@@noclip%
  \end{tcbclipinterior}%
}

\def\tcb@drawspec@watermark@tikz#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\pgfsetbaseline{0pt}\begin{tikzpicture}[color=\kvtcb@watermark@color]#1\end{tikzpicture}}\endpgfinterruptpicture\color@endbox%
  \tcb@drawspec@watermark%
}

\def\tcb@drawspec@watermark@graphics#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\includegraphics{#1}}\endpgfinterruptpicture\color@endbox%
  \tcb@drawspec@watermark%
}

\def\tcb@drawspec@watermark@text#1{%
  \tcb@drawspec@watermark@tikz{\node[inner sep=0pt,align=flush center]{#1};}%
}


\tcbset{%
  watermark opacity/.store in=\kvtcb@watermark@opacity,%
  watermark color/.store in=\kvtcb@watermark@color,%
%
  watermark stretch/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@stretch{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
  watermark zoom/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@zoom{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
  watermark overzoom/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@overzoom{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
  watermark shrink/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@shrink{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
%
  watermark tikz/.style={overlay={\tcb@drawspec@watermark@tikz{#1}}},
  watermark tikz on/.style args={#1 is #2}{overlay #1={\tcb@drawspec@watermark@tikz{#2}}},%
  watermark graphics/.style={overlay={\tcb@drawspec@watermark@graphics{#1}}},
  watermark graphics on/.style args={#1 is #2}{overlay #1={\tcb@drawspec@watermark@graphics{#2}}},
  watermark text/.style={overlay={\tcb@drawspec@watermark@text{#1}}},
  watermark text on/.style args={#1 is #2}{overlay #1={\tcb@drawspec@watermark@text{#2}}},
  no watermark/.style={no overlay},
  clip watermark/.is choice,
  clip watermark/true/.code={\let\tcb@drawspec@watermark=\tcb@drawspec@watermark@@clip},
  clip watermark/false/.code={\let\tcb@drawspec@watermark=\tcb@drawspec@watermark@@noclip},
  clip watermark/.default=true,
  show bounding box/.style={border@line app={%
    \path[preaction={draw,line width=0.1pt,#1},draw,double=white,line width=1pt,dashed,opacity=0.5,#1]
    (current bounding box.south west) rectangle (current bounding box.north east);}},%
  show bounding box/.default={red},%
}

\def\tcb@tdraw@title@clip{%
  \begin{tcbcliptitle}%
  \tcb@tdraw@title@core%
  \end{tcbcliptitle}%
}

\def\tcb@tdraw@upper@clip{%
  \begin{tcbclipinterior}%
  \tcb@tdraw@upper@core%
  \end{tcbclipinterior}%
}

\def\tcb@tdraw@lower@clip{%
  \begin{tcbclipinterior}%
  \tcb@tdraw@lower@core%
  \end{tcbclipinterior}%
}


\def\tcb@process@ppbb{%
  \pgf@process{\pgfpointanchor{path picture bounding box}{south west}}%
  \pgf@xa\pgf@x\pgf@ya\pgf@y%
  \pgf@process{\pgfpointanchor{path picture bounding box}{north east}}%
  \pgf@xb\pgf@x\pgf@yb\pgf@y%
  \pgfsetfillopacity{\tcb@tikz@fill@graphics@opacity}%
  \pgfsetstrokeopacity{\tcb@tikz@fill@graphics@opacity}%
}

\def\tcb@process@ppbb@wh{%
  \tcb@process@ppbb%
  \tcbdimto\tcb@ppbb@width{\pgf@xb-\pgf@xa}%
  \tcbdimto\tcb@ppbb@height{\pgf@yb-\pgf@ya}%
}

\def\tcb@ppbb@textbox#1{\pgftext[x=\the\dimexpr\pgf@xa+\tcb@ppbb@width/2\relax,y=\pgf@ya+\tcb@ppbb@height/2]{#1}}

\def\tcb@set@waterbox@to@graphics#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture%
    \begingroup\edef\x{\endgroup\noexpand\includegraphics[\tcb@tikz@fill@graphics@options]}\x{#1}%
    \endpgfinterruptpicture\color@endbox%
}

\def\tcb@set@waterbox@to@picture#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\pgfsetbaseline{0pt}\begin{tikzpicture}#1\end{tikzpicture}}\endpgfinterruptpicture\color@endbox%
}

\tikzset{%
  fill image opacity/.store in=\tcb@tikz@fill@graphics@opacity,%
  fill image opacity=1,%
  fill image scale/.store in=\tcb@tikz@fill@graphics@scale,%
  fill image scale=1,%
  fill image options/.store in=\tcb@tikz@fill@graphics@options,%
  fill image options=,%
  fill plain image/.style={path picture={%
    \tcb@process@ppbb@wh%
    \tcb@ppbb@textbox{\begingroup\edef\x{\endgroup\noexpand\includegraphics[\tcb@tikz@fill@graphics@options]}\x{#1}}%
  }},
  fill plain picture/.style={path picture={%
    \tcb@process@ppbb@wh%
    \tcb@set@waterbox@to@picture{#1}%
    \tcb@ppbb@textbox{\box\tcb@waterbox}%
  }},
  fill stretch image/.style={path picture={%
    \tcb@process@ppbb@wh%
    \tcb@ppbb@textbox{\begingroup\edef\x{\endgroup\noexpand\includegraphics[\tcb@tikz@fill@graphics@options,%
      width=\the\dimexpr\tcb@tikz@fill@graphics@scale\dimexpr\tcb@ppbb@width\relax,%
      height=\the\dimexpr\tcb@tikz@fill@graphics@scale\dimexpr\tcb@ppbb@height\relax]}\x{#1}}%
  }},
  fill stretch picture/.style={path picture={%
    \tcb@process@ppbb@wh%
    \tcb@set@waterbox@to@picture{#1}%
    \tcb@comp@waterbox@stretch{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \tcb@ppbb@textbox{\tcb@box@scaled@waterbox}%
  }},
  fill@overzoom/.style={path picture={%
    \tcb@process@ppbb@wh%
    #1%
    \tcb@comp@waterbox@overzoom{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \tcb@ppbb@textbox{\tcb@box@scaled@waterbox}%
  }},
  fill overzoom image/.style={fill@overzoom={\tcb@set@waterbox@to@graphics{#1}}},%
  fill overzoom picture/.style={fill@overzoom={\tcb@set@waterbox@to@picture{#1}}},%
  fill@zoom/.style={path picture={%
    \tcb@process@ppbb@wh%
    #1%
    \tcb@comp@waterbox@zoom{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \tcb@ppbb@textbox{\tcb@box@scaled@waterbox}%
  }},
  fill zoom image/.style={fill@zoom={\tcb@set@waterbox@to@graphics{#1}}},%
  fill zoom picture/.style={fill@zoom={\tcb@set@waterbox@to@picture{#1}}},%
  fill@shrink/.style={path picture={%
    \tcb@process@ppbb@wh%
    #1%
    \tcb@comp@waterbox@shrink{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \tcb@ppbb@textbox{\tcb@box@scaled@waterbox}%
  }},
  fill shrink image/.style={fill@shrink={\tcb@set@waterbox@to@graphics{#1}}},%
  fill shrink picture/.style={fill@shrink={\tcb@set@waterbox@to@picture{#1}}},%
  fill@tile/.style={path picture={%
    \tcb@process@ppbb%
    #1%
    \tcbdimto\tcb@ppbb@tilew{\wd\tcb@waterbox}%
    \tcbdimto\tcb@ppbb@tileh{\ht\tcb@waterbox+\dp\tcb@waterbox}%
    \pgf@xc\pgf@xa\pgf@yc\pgf@yb%
    \pgfutil@loop%
      \pgfutil@loop%
        \pgftext[x=\pgf@xc,y=\pgf@yc,left,top]{\copy\tcb@waterbox}%
        \ifdim\pgf@xc<\pgf@xb%
        \advance\pgf@xc\tcb@ppbb@tilew%
      \pgfutil@repeat%
      \ifdim\pgf@yc>\pgf@ya%
      \advance\pgf@yc-\tcb@ppbb@tileh%
      \pgf@xc\pgf@xa%
    \pgfutil@repeat%
  }},%
  fill tile image/.style={fill@tile={\tcb@set@waterbox@to@graphics{#1}}},%
  fill tile picture/.style={fill@tile={\tcb@set@waterbox@to@picture{#1}}},%
  fill tile picture*/.style 2 args={fill@tile={\tcb@set@waterbox@to@picture{#2}%
    \setbox\tcb@waterbox=\color@hbox\scalebox{#1}{\box\tcb@waterbox}\color@endbox}},%
  %
  fill plain image*/.style 2 args={fill image options={#1},fill plain image={#2}},%
  fill stretch image*/.style 2 args={fill image options={#1},fill stretch image={#2}},%
  fill overzoom image*/.style 2 args={fill image options={#1},fill overzoom image={#2}},%
  fill zoom image*/.style 2 args={fill image options={#1},fill zoom image={#2}},%
  fill shrink image*/.style 2 args={fill image options={#1},fill shrink image={#2}},%
  fill tile image*/.style 2 args={fill image options={#1},fill tile image={#2}},%
}

\tcbset{%
  frame style image/.style={frame style={fill=none,fill stretch image={#1}}},
  frame style tile/.style 2 args={frame style={fill=none,fill tile image*={#1}{#2}}},
  interior style image/.style={interior style={fill=none,fill stretch image={#1}}},
  interior style tile/.style 2 args={interior style={fill=none,fill tile image*={#1}{#2}}},
  title style image/.style={title style={fill=none,fill stretch image={#1}}},
  title style tile/.style 2 args={title style={fill=none,fill tile image*={#1}{#2}}},
}

\tcbset{%
  clip title/.is choice,
  clip title/true/.code={\let\tcb@tdraw@title=\tcb@tdraw@title@clip},
  clip title/false/.code={\let\tcb@tdraw@title=\tcb@tdraw@title@core},
  clip title/.default=true,
  clip upper/.is choice,
  clip upper/true/.code={\let\tcb@tdraw@upper=\tcb@tdraw@upper@clip},
  clip upper/false/.code={\let\tcb@tdraw@upper=\tcb@tdraw@upper@core},
  clip upper/.default=true,
  clip lower/.is choice,
  clip lower/true/.code={\let\tcb@tdraw@lower=\tcb@tdraw@lower@clip},
  clip lower/false/.code={\let\tcb@tdraw@lower=\tcb@tdraw@lower@core},
  clip lower/.default=true,
}


\tcbset{marker/.style={%
  skin=enhancedmiddle jigsaw,
  breakable,parbox=false,
  boxrule=0mm,leftrule=5mm,rightrule=5mm,boxsep=0mm,
  left=3mm,right=3mm,top=1mm,bottom=1mm,
  toptitle=1mm,bottomtitle=1mm,fonttitle=\bfseries,
  arc=0mm,outer arc=0mm,
  colback=yellow!10!white,colframe=red,
  watermark color=yellow!75!red!25!white,
  enlarge left by=-8mm,
  enlarge right by=-8mm,
  enlarge top by=0mm,
  enlarge bottom by=0mm,
  width=\the\dimexpr\linewidth+1.6cm\relax,
  frame style={top color=tcbcolframe,bottom color=tcbcolframe,middle color=yellow!75!tcbcolframe},
  title style={left color=tcbcolframe,right color=tcbcolframe,middle color=yellow!75!tcbcolframe},
  watermark tikz={\draw[line width=2mm] circle (1cm) node{\fontfamily{ptm}\fontseries{b}\fontsize{20mm}{20mm}\selectfont!};},
  watermark zoom=0.75,
}}


\def\tcb@arc@bor{\pgfsetcornersarced{\pgfqpoint{\tcb@border@arc}{\tcb@border@arc}}}%

\def\tcb@arc@bor@NW{\csname tcb@arc@bor@NW@\tcb@corner@mode@NW\endcsname}
\def\tcb@arc@bor@NE{\csname tcb@arc@bor@NE@\tcb@corner@mode@NE\endcsname}
\def\tcb@arc@bor@SW{\csname tcb@arc@bor@SW@\tcb@corner@mode@SW\endcsname}
\def\tcb@arc@bor@SE{\csname tcb@arc@bor@SE@\tcb@corner@mode@SE\endcsname}

\let\tcb@arc@bor@NW@sharp\tcb@arc@zpt
\let\tcb@arc@bor@NE@sharp\tcb@arc@zpt
\let\tcb@arc@bor@SW@sharp\tcb@arc@zpt
\let\tcb@arc@bor@SE@sharp\tcb@arc@zpt

\let\tcb@arc@bor@NW@rounded\tcb@arc@bor
\let\tcb@arc@bor@NE@rounded\tcb@arc@bor
\let\tcb@arc@bor@SW@rounded\tcb@arc@bor
\let\tcb@arc@bor@SE@rounded\tcb@arc@bor

\def\tcb@border@prepare#1#2{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \ifdim\dimexpr\tcb@outer@arc>\tcb@arc@scale\dimexpr\tcb@border@ts\relax%
    \tcbdimto\tcb@border@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr\tcb@border@ts\relax}%
  \else%
    \let\tcb@border@arc=\tcb@zpt%
  \fi%
}

\def\tcb@border@unbroken#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \tcb@pathbase{draw,line width=#1,#3}{[xshift=\tcb@border@ts,yshift=\tcb@border@ts]frame.south west}%
    {[xshift=-\tcb@border@ts,yshift=-\tcb@border@ts]frame.north east}%
    {\tcb@arc@bor@SW}{\tcb@arc@bor@NW}{\tcb@arc@bor@NE}{\tcb@arc@bor@SE}%
}

\def\tcb@border@first#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \tcb@pathboundary{draw,line width=#1,#3}{%
    \tcb@gettikzxy{([xshift=\tcb@border@ts]frame.south west)}{\tcb@xa}{\tcb@ya}%
    \tcb@gettikzxy{([xshift=-\tcb@border@ts,yshift=-\tcb@border@ts]frame.north east)}{\tcb@xb}{\tcb@yb}%
    \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
    \tcb@arc@bor@NW\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
    \tcb@arc@bor@NE\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
    \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
  }%
}

\def\tcb@border@middle#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \draw[line width=#1,#3]
    ([xshift=\tcb@border@ts]frame.north west) -- ([xshift=\tcb@border@ts]frame.south west);%
  \draw[line width=#1,#3]
    ([xshift=-\tcb@border@ts]frame.north east) -- ([xshift=-\tcb@border@ts]frame.south east);%
}

\def\tcb@border@last#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \tcb@pathboundary{draw,line width=#1,#3}{%
    \tcb@gettikzxy{([xshift=\tcb@border@ts,yshift=\tcb@border@ts]frame.south west)}{\tcb@xa}{\tcb@ya}%
    \tcb@gettikzxy{([xshift=-\tcb@border@ts]frame.north east)}{\tcb@xb}{\tcb@yb}%
    \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
    \tcb@arc@bor@SW\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
    \tcb@arc@bor@SE\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
    \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
  }%
}

\def\tcb@draw@border@unbroken{%
  \let\tcb@border=\tcb@border@unbroken%
  \kvtcb@borderline%
}

\def\tcb@draw@border@first{%
  \let\tcb@border=\tcb@border@first%
  \kvtcb@borderline%
}

\def\tcb@draw@border@middle{%
  \let\tcb@border=\tcb@border@middle%
  \kvtcb@borderline%
}

\def\tcb@draw@border@last{%
  \let\tcb@border=\tcb@border@last%
  \kvtcb@borderline%
}

\def\tcb@bordernorth@draw#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([yshift=-\tcb@border@ts]frame.north west) -- ([yshift=-\tcb@border@ts]frame.north east);%
}

\def\tcb@bordernorth#1#2#3{%
  \ifdefstring{\tcb@split@state}{unbroken}{\tcb@bordernorth@draw{#1}{#2}{#3}}{%
    \ifdefstring{\tcb@split@state}{first}{\tcb@bordernorth@draw{#1}{#2}{#3}}{}}%
}

\def\tcb@bordersouth@draw#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([yshift=\tcb@border@ts]frame.south west) -- ([yshift=\tcb@border@ts]frame.south east);%
}

\def\tcb@bordersouth#1#2#3{%
  \ifdefstring{\tcb@split@state}{unbroken}{\tcb@bordersouth@draw{#1}{#2}{#3}}{%
    \ifdefstring{\tcb@split@state}{last}{\tcb@bordersouth@draw{#1}{#2}{#3}}{}}%
}

\def\tcb@borderwest#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([xshift=\tcb@border@ts]frame.north west) -- ([xshift=\tcb@border@ts]frame.south west);%
}

\def\tcb@bordereast#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([xshift=-\tcb@border@ts]frame.north east) -- ([xshift=-\tcb@border@ts]frame.south east);%
}

\tcbset{%
  border@line app/.code={\appto\kvtcb@borderline{#1}},%
  borderline/.style args={#1#2#3}{border@line app={\tcb@border{#1}{#2}{#3}}},%
  no borderline/.code={\def\kvtcb@borderline{}},%
  borderline north/.style args={#1#2#3}{border@line app={\tcb@bordernorth{#1}{#2}{#3}}},%
  borderline south/.style args={#1#2#3}{border@line app={\tcb@bordersouth{#1}{#2}{#3}}},%
  borderline west/.style args={#1#2#3}{border@line app={\tcb@borderwest{#1}{#2}{#3}}},%
  borderline east/.style args={#1#2#3}{border@line app={\tcb@bordereast{#1}{#2}{#3}}},%
  borderline horizontal/.style args={#1#2#3}{borderline north={#1}{#2}{#3},borderline south={#1}{#2}{#3}},%
  borderline vertical/.style args={#1#2#3}{borderline west={#1}{#2}{#3},borderline east={#1}{#2}{#3}},%
}


\def\tcb@shadow@comp@ts@smart#1#2{%
  \ifdim#2>0pt\relax\tcbdimto\tcb@shadow@ts{#1-#2/2}%%
  \else\tcbdimto\tcb@shadow@ts{#1+#2/2}\fi%
}

\def\tcb@shadow@comp@ts@copy#1#2{%
  \tcbdimto\tcb@shadow@ts{#1}%
}

\def\tcb@shadow@comp@arc{%
  \ifdim\dimexpr\tcb@outer@arc>\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax%
    \tcbdimto\tcb@shadow@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax}%
  \else%
    \let\tcb@shadow@arc=\tcb@zpt%
  \fi%
}

\def\tcb@arc@sha{\pgfsetcornersarced{\pgfqpoint{\tcb@shadow@arc}{\tcb@shadow@arc}}}%

\def\tcb@arc@sha@NW{\csname tcb@arc@sha@NW@\tcb@corner@mode@NW\endcsname}
\def\tcb@arc@sha@NE{\csname tcb@arc@sha@NE@\tcb@corner@mode@NE\endcsname}
\def\tcb@arc@sha@SW{\csname tcb@arc@sha@SW@\tcb@corner@mode@SW\endcsname}
\def\tcb@arc@sha@SE{\csname tcb@arc@sha@SE@\tcb@corner@mode@SE\endcsname}

\let\tcb@arc@sha@NW@sharp\tcb@arc@zpt
\let\tcb@arc@sha@NE@sharp\tcb@arc@zpt
\let\tcb@arc@sha@SW@sharp\tcb@arc@zpt
\let\tcb@arc@sha@SE@sharp\tcb@arc@zpt

\let\tcb@arc@sha@NW@rounded\tcb@arc@sha
\let\tcb@arc@sha@NE@rounded\tcb@arc@sha
\let\tcb@arc@sha@SW@rounded\tcb@arc@sha
\let\tcb@arc@sha@SE@rounded\tcb@arc@sha

\def\tcb@shadow@unbroken#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@sha@SE}%
}

\def\tcb@shadow@first#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@zpt}%
}

\def\tcb@shadow@middle#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@shadow@last#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@sha@SE}%
}


\tcbset{%
  shad@w app/.code={\appto\kvtcb@shadow{#1}},%
  shadow/.style args={#1#2#3#4}{shad@w app={\csuse{tcb@shadow@\tcb@shapeofskin}{#1}{#2}{#3}{#4}}},%
  no shadow/.code={\def\kvtcb@shadow{}},%
  fuzzy shadow/.style args={#1#2#3#4#5}{shad@w app={%
    \begin{scope}[#5]%
      \letcs\tcb@shadow{tcb@shadow@\tcb@shapeofskin}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-4\dimexpr#4\relax}{opacity=0.01}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-3\dimexpr#4\relax}{opacity=0.02}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-2\dimexpr#4\relax}{opacity=0.04}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-#4\relax}{opacity=0.07}%
      \tcb@shadow{#1}{#2}{#3}{opacity=0.11}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+#4\relax}{opacity=0.11}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+2\dimexpr#4\relax}{opacity=0.07}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+3\dimexpr#4\relax}{opacity=0.04}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+4\dimexpr#4\relax}{opacity=0.02}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+5\dimexpr#4\relax}{opacity=0.01}%
  \end{scope}}},%
  %
  drop shadow/.style={shadow={0.9mm}{-0.9mm}{0mm}{opacity=0.5,#1}},
  drop shadow/.default={black!50!white},%
  drop midday shadow/.style={shadow={0mm}{-0.8mm}{-0.4mm}{opacity=0.5,#1}},
  drop midday shadow/.default={black!50!white},%
  halo/.style args={#1 with #2}{shadow={0mm}{0mm}{-#1}{opacity=0.5,#2}},
  halo/.default={0.9mm with yellow},%
  drop fuzzy shadow/.style={fuzzy shadow={1.0mm}{-1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow/.default={black!50!white},%
  drop fuzzy midday shadow/.style={fuzzy shadow={0mm}{-1.0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy midday shadow/.default={black!50!white},%
  fuzzy halo/.style args={#1 with #2}{fuzzy shadow={0mm}{0mm}{-#1}{0.12mm}{#2}},
  fuzzy halo/.default={1.0mm with yellow},%
  %
  drop shadow southeast/.style={shadow={0.9mm}{-0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow southeast/.default={black!50!white},%
  drop shadow south/.style={shadow={0mm}{-0.8mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow south/.default={black!50!white},%
  drop shadow southwest/.style={shadow={-0.9mm}{-0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow southwest/.default={black!50!white},%
  drop shadow west/.style={shadow={-0.8mm}{0mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow west/.default={black!50!white},%
  drop shadow northwest/.style={shadow={-0.9mm}{0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow northwest/.default={black!50!white},%
  drop shadow north/.style={shadow={0mm}{0.8mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow north/.default={black!50!white},%
  drop shadow northeast/.style={shadow={0.9mm}{0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow northeast/.default={black!50!white},%
  drop shadow east/.style={shadow={0.8mm}{0mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow east/.default={black!50!white},%
  drop fuzzy shadow southeast/.style={fuzzy shadow={1.0mm}{-1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow southeast/.default={black!50!white},%
  drop fuzzy shadow south/.style={fuzzy shadow={0mm}{-1.0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow south/.default={black!50!white},%
  drop fuzzy shadow southwest/.style={fuzzy shadow={-1.0mm}{-1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow southwest/.default={black!50!white},%
  drop fuzzy shadow west/.style={fuzzy shadow={-1.0mm}{0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow west/.default={black!50!white},%
  drop fuzzy shadow northwest/.style={fuzzy shadow={-1.0mm}{1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow northwest/.default={black!50!white},%
  drop fuzzy shadow north/.style={fuzzy shadow={0mm}{1.0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow north/.default={black!50!white},%
  drop fuzzy shadow northeast/.style={fuzzy shadow={1.0mm}{1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow northeast/.default={black!50!white},%
  drop fuzzy shadow east/.style={fuzzy shadow={1.0mm}{0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow east/.default={black!50!white},%
  %
  smart shadow arc/.is choice,
  smart shadow arc/true/.code={\let\tcb@shadow@comp@ts=\tcb@shadow@comp@ts@smart},
  smart shadow arc/false/.code={\let\tcb@shadow@comp@ts=\tcb@shadow@comp@ts@copy},
  smart shadow arc/.default=true,
}

\def\tcb@boundary@tikzbendedbase#1#2#3#4#5#6#7#8{%
  \tcb@gettikzxy{(#1)}{\tcb@xa}{\tcb@ya}%
  \tcb@gettikzxy{(#2)}{\tcb@xb}{\tcb@yb}%
  \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
  #5\pgfpathquadraticcurveto{\pgfqpoint{\dimexpr0.5\dimexpr\tcb@xa+\tcb@xb\relax}{\dimexpr\tcb@yb+#8}}{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
  #6\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
  #3\pgfpathquadraticcurveto{\pgfqpoint{\dimexpr0.5\dimexpr\tcb@xa+\tcb@xb\relax}{\dimexpr\tcb@ya+#7}}{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  #4\pgfpathclose%
}

\def\tcb@pathbendedbase#1#2#3#4#5#6#7#8#9{\tcb@pathboundary{#1}{\tcb@boundary@tikzbendedbase{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}}

\def\tcb@shadowbended@prepare#1{%
  \tcbdimto\tcb@shadow@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr#1\relax}%
  \ifdim\dimexpr\tcb@shadow@arc<0pt\relax%
    \let\tcb@shadow@arc=\tcb@zpt%
  \fi%
}

\def\tcb@shadowlifted@unbroken#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@sha@SE}{#4}{0pt}%
}

\def\tcb@shadowlifted@first#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@zpt}{#4}{0pt}%
}

\def\tcb@shadowlifted@middle#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{#4}{0pt}%
}

\def\tcb@shadowlifted@last#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@sha@SE}{#4}{0pt}%
}

\tcbset{
  lifted shadow/.style n args={5}{shad@w app={%
    \begin{scope}[#5]%
      \letcs\tcb@shadowlifted{tcb@shadowlifted@\tcb@shapeofskin}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-4\dimexpr#4}{#3}{opacity=0.01}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-3\dimexpr#4}{#3}{opacity=0.02}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-2\dimexpr#4}{#3}{opacity=0.04}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-#4}{#3}{opacity=0.07}%
      \tcb@shadowlifted{#1}{#2}{0pt}{#3}{opacity=0.11}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+#4}{#3}{opacity=0.11}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+2\dimexpr#4}{#3}{opacity=0.07}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+3\dimexpr#4}{#3}{opacity=0.04}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+4\dimexpr#4}{#3}{opacity=0.02}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+5\dimexpr#4}{#3}{opacity=0.01}%
  \end{scope}}},%
  drop small lifted shadow/.style={lifted shadow={1mm}{-0.75mm}{1.3mm}{0.1mm}{#1}},
  drop small lifted shadow/.default={black!50!white},%
  drop lifted shadow/.style={lifted shadow={1.5mm}{-1.5mm}{2.7mm}{0.12mm}{#1}},
  drop lifted shadow/.default={black!50!white},%
  drop large lifted shadow/.style={lifted shadow={2mm}{-3mm}{5.7mm}{0.16mm}{#1}},
  drop large lifted shadow/.default={black!50!white},%
}

\newif\iftcb@isindraft
\def\tcb@draftmode{\tcbset{spartan,spartan@fit}}
\def\tcbstartdraftmode{\let\tcb@afteroptions@hook=\tcb@draftmode\tcb@isindrafttrue}
\def\tcbstopdraftmode{\let\tcb@afteroptions@hook=\@empty\tcb@isindraftfalse}

\def\tcbinterruptdraftmode{%
  \iftcb@isindraft%
    \tcbstopdraftmode%
    \let\tcbcontinuedraftmode=\tcbstartdraftmode%
  \else%
    \let\tcbcontinuedraftmode=\@empty%
  \fi}

\tcbset{%
  draftmode/.is choice,%
  draftmode/.default=true,%
  draftmode/true/.code=\tcbstartdraftmode,%
  draftmode/false/.code=\tcbstopdraftmode,%
}


\def\tcb@include@graphics{%
  \let\tcb@graphics@options\kvtcb@graphics@options%
  \ifnum\kvtcb@graphics@orientation>-1\relax%
    \setbox\tcb@waterbox=\color@hbox\begingroup\edef\x{\endgroup\noexpand\includegraphics[\tcb@graphics@options]}\x{\imagepath}\color@endbox%
    \ifcase\kvtcb@graphics@orientation\relax%
      \ifdim\wd\tcb@waterbox<\dimexpr\ht\tcb@waterbox+\dp\tcb@waterbox\relax%
        \appto\tcb@graphics@options{,angle=90}%
      \fi%
    \or%
      \ifdim\wd\tcb@waterbox<\dimexpr\ht\tcb@waterbox+\dp\tcb@waterbox\relax%
        \appto\tcb@graphics@options{,angle=-90}%
      \fi%
    \or%
      \ifdim\wd\tcb@waterbox>\dimexpr\ht\tcb@waterbox+\dp\tcb@waterbox\relax%
        \appto\tcb@graphics@options{,angle=90}%
      \fi%
    \or%
      \ifdim\wd\tcb@waterbox>\dimexpr\ht\tcb@waterbox+\dp\tcb@waterbox\relax%
        \appto\tcb@graphics@options{,angle=-90}%
      \fi%
    \fi%
  \fi%
  \ifdefstring{\kvtcb@capture}{hbox}{%
    \tcbox{%
      \begingroup\edef\x{\endgroup\noexpand\includegraphics[\tcb@graphics@options]}%
      \x{\imagepath}%
    }%
  }{%
    \iftcb@fixedheight%
      \begin{tcolorbox}%
        \begingroup\edef\x{\endgroup\noexpand\includegraphics[\tcb@graphics@options,width=\linewidth,height=\tcbtextheight,keepaspectratio]}%
        \x{\imagepath}%
      \end{tcolorbox}%
    \else%
      \ifdefempty\tcb@height@adjust{%
        \begin{tcolorbox}%
          \begingroup\edef\x{\endgroup\noexpand\includegraphics[\tcb@graphics@options,width=\linewidth]}%
          \x{\imagepath}%
        \end{tcolorbox}%
      }{% height fill
        \begin{tcolorbox}[underlay={%
          \begin{tcbclipinterior}%
          \path[fill zoom image*={\tcb@graphics@options}{\imagepath}]
            ([xshift=\kvtcb@boxsep+\kvtcb@leftupper,yshift=\kvtcb@boxsep+\kvtcb@bottom]interior.south west) rectangle
            ([xshift=-\kvtcb@boxsep-\kvtcb@rightupper,yshift=-\kvtcb@boxsep-\kvtcb@top]interior.north east);
          \end{tcbclipinterior}%
          }]%
        \end{tcolorbox}%
      }%
    \fi%
  }%
}

\def\tcb@scanfilename#1#2{%
  \begingroup%
    \everyeof{\noexpand}%
    \endlinechar -1%
    \catcode`\_=11%
    \catcode`\~=11%
    \edef\x{\scantokens\expandafter{#2}}%
  \expandafter\endgroup%
  \expandafter\def\expandafter #1\expandafter{\x}%
}%


\def\tcb@include@graphics@preparefile#1{%
  \tcb@scanfilename\tcb@temp{#1}%
  \filename@parse{\tcb@temp}%
  \ifx\filename@ext\relax%
    \let\imagename\filename@base%
  \else%
    \def\imagename{\filename@base\Gin@sepdefault\filename@ext}%
  \fi%
  \ifdefined\grffile@Ginclude@graphics%
    % grffile package loaded
    \ifx\kvtcb@graphics@directory\@empty%
      \def\imagepath{#1}%
    \else%
      \def\imagepath{\kvtcb@graphics@directory/#1}%
    \fi%
  \else%
    \ifx\kvtcb@graphics@directory\@empty%
      \edef\imagepath{#1}%
    \else%
      \edef\imagepath{\kvtcb@graphics@directory/#1}%
    \fi%
  \fi%
}

\newcommand{\tcbincludegraphics}[2][]{%
  \begingroup%
  \tcb@layer@pushup%
  \tcb@apply@box@options{enhanced,clip upper=true,valign=center,center upper,#1}%
  \tcb@include@graphics@preparefile{#2}%
  \edef\imagepage{1}%
  \tcb@include@graphics%
  \endgroup%
}

\def\tcb@set@pdfpages#1#2{%
  \IfFileExists{#2}{%
    \ifdef{\pdfximage}{%
      \pdfximage{#2}%
      \edef#1{\the\pdflastximagepages}%
    }{%
      \ifdef{\XeTeXpdfpagecount}{%
        \edef#1{\the\XeTeXpdfpagecount #2 }%
        \ifnum#1=0 %
          \edef#1{1}%
        \fi%
      }{\tcb@error{For PDF support run pdflatex, xelatex, or lualatex}{%
        Your compiler seems not to support PDF include files.}}%
    }%
  }{\tcb@error{PDF file `#2' not found}{The PDF file `#2' was not found}}%
  \relax%
}

\newcommand{\tcbincludepdf}[2][]{%
  \begingroup%
  \tcb@layer@pushup%
  \tcb@apply@box@options{enhanced,clip upper=true,valign=center,center upper,#1}%
  \appto\kvtcb@graphics@options{,page=\imagepage}%
  \tcb@include@graphics@preparefile{#2}%
  \tcb@set@pdfpages\pdfpages{\imagepath}%
  \foreach \imagepage in \kvtcb@graphics@pages%
  {%
    \tcb@include@graphics%
  }%
  \endgroup%
}

\tcbset{%
  graphics options/.store in=\kvtcb@graphics@options,
  graphics pages/.store in=\kvtcb@graphics@pages,
  graphics directory/.store in=\kvtcb@graphics@directory,
  graphics orientation/.is choice,
  graphics orientation/as-is/.code={\def\kvtcb@graphics@orientation{-1}},
  graphics orientation/landscape/.code={\def\kvtcb@graphics@orientation{0}},
  graphics orientation/landscape*/.code={\def\kvtcb@graphics@orientation{1}},
  graphics orientation/portrait/.code={\def\kvtcb@graphics@orientation{2}},
  graphics orientation/portrait*/.code={\def\kvtcb@graphics@orientation{3}},
}

\newcommand{\tcbhypernode}[2]{\ifdefined\hypersetup\@ifundefined{pgf@sh@ns@#2}{}{%
  \node[inner sep=0pt,outer sep=0pt] at (#2.center){%
    \tcbsetmacrotowidthofnode\tcb@w@hn{#2}%
    \tcbsetmacrotoheightofnode\tcb@h@hn{#2}%
    \hypersetup{pdfborder=0 0 0}%
    #1{\vtop to \dimexpr\tcb@h@hn-2bp\relax{\hbox to \dimexpr\tcb@w@hn-2bp\relax{}\vfil}}%
  };%
}\fi}

\tcbset{%
  hyperref node/.style 2 args={finish={\tcbhypernode{\hyperref[#1]}{#2}}},
  hyperref/.style={hyperref node={#1}{frame}},
  hyperref interior/.style={hyperref node={#1}{interior}},
  hyperref title/.style={hyperref node={#1}{title}},
  hyperlink node/.style 2 args={finish={\tcbhypernode{\hyperlink{#1}}{#2}}},
  hyperlink/.style={hyperlink node={#1}{frame}},
  hyperlink interior/.style={hyperlink node={#1}{interior}},
  hyperlink title/.style={hyperlink node={#1}{title}},
  hyperurl node/.style 2 args={finish={\tcbhypernode{\href{#1}}{#2}}},
  hyperurl/.style={hyperurl node={#1}{frame}},
  hyperurl interior/.style={hyperurl node={#1}{interior}},
  hyperurl title/.style={hyperurl node={#1}{title}},
  hyperurl* node/.style n args={3}{finish={\tcbhypernode{\href[#1]{#2}}{#3}}},
  hyperurl*/.style 2 args={hyperurl* node={#1}{#2}{frame}},
  hyperurl* interior/.style 2 args={hyperurl* node={#1}{#2}{interior}},
  hyperurl* title/.style 2 args={hyperurl* node={#1}{#2}{title}},
  beamer hidden/.style={nirvana},
  beamer alerted/.style={fuzzy halo},
  only/.code args={<#1>#2}{\only<#1>{\tcbset{#2}}},%
  hide/.code args={<#1>}{\only<#1>{\tcbset{beamer hidden}}},%
  alert/.code args={<#1>}{\only<#1>{\tcbset{beamer alerted}}},%
}

\tcbset{%
  reset@skins/.style={%
    frame style=,interior style=,segmentation style=,@title style=,%
    colbacklower=black!15!white,%
    extend freelance=,extend freelancefirst=,extend freelancemiddle=,extend freelancelast=,%
    clear@spec,%
    watermark opacity=1.00,watermark color=tcbcolback!85!tcbcolframe,%
    watermark zoom=0.75,clip watermark,%
    clip title=false,clip upper=false,clip lower=false,%
    no borderline,smart shadow arc,no shadow,no underlay,no finish,tikz reset,at begin tikz reset,at end tikz reset,%
    boxed title size=title,no boxed title style,hbox boxed title,code={\let\tcb@specialgeonodes@hook\relax},%
    graphics options=,graphics pages={1,...,\pdfpages},graphics directory=,graphics orientation=as-is,%
  },
  initialize@reset=reset@skins,
}

\tcbuselibrary{skins@jigsaw}


==> tcbskinsjigsaw.code.tex <==
%% The LaTeX package tcolorbox - version 4.30 (2020/04/28)
%% tcbskinsjigsaw.code.tex: Code for colorboxes with different skins
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2020 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{4.30}

\tcbuselibrary{skins}

\def\tcb@drawframe@pathjigsaw{%
  \tcb@pathboundary{tcb fill frame}{\tcb@boundaryframe@standardjigsaw}%
}

\def\tcb@boundary@pathfirstjigsaw@A{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\tcb@height-\kvtcb@top@rule}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@out@NW\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \tcb@arc@out@NE\pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \tcb@arc@ins@NE\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \tcb@arc@ins@NW\pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@boundary@pathfirstjigsaw@B{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@out@NW\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \tcb@arc@out@NE\pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@drawframe@pathfirstjigsaw{%
  \tcb@pathboundary{tcb fill frame}{%
    \pgfseteorule%
    \iftcb@hasTitle%
      \iftcb@titlefilled%
        \ifdim\dimexpr\kvtcb@title@rule>0pt\relax%
          \tcb@boundary@pathfirstjigsaw@B%
          \tcb@boundarytitle@standard%
        \else%
          \tcb@boundary@pathfirstjigsaw@A%
        \fi%
      \else%
        \tcb@boundary@pathfirstjigsaw@B%
      \fi%
    \else%
      \tcb@boundary@pathfirstjigsaw@A%
    \fi%
  }%
}

\def\tcb@boundary@pathmiddlejigsaw@A{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \pgfpathrectangle{\pgfpointorigin}{\pgfqpoint{\kvtcb@left@rule}{\tcb@height}}%
  \pgfpathrectangle{\pgfqpoint{\tcb@xa}{0pt}}{\pgfqpoint{\kvtcb@right@rule}{\tcb@height}}%
}

\def\tcb@boundary@pathmiddlejigsaw@B{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\tcb@height-\kvtcb@top@rule}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@boundary@pathmiddlejigsaw@C{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@drawframe@pathmiddlejigsaw{%
  \tcb@pathboundary{tcb fill frame}{%
    \pgfseteorule%
    \iftcb@hasTitle%
      \iftcb@titlefilled%
        \ifdim\dimexpr\kvtcb@title@rule>0pt\relax%
          \tcb@boundary@pathmiddlejigsaw@C%
          \tcb@arc@zpt%
          \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule}%
          \tcbdimto\tcb@xb{\tcb@width-\kvtcb@right@rule}%
          \tcbdimto\tcb@yb{\tcb@height-\kvtcb@top@rule}%
          \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
        \else%
          \tcb@boundary@pathmiddlejigsaw@B%
        \fi%
      \else%
        \tcb@boundary@pathmiddlejigsaw@C%
      \fi%
    \else%
      \tcb@boundary@pathmiddlejigsaw@A%
    \fi%
  }%
}

\def\tcb@drawframe@pathlastjigsaw{%
  \tcb@pathboundary{tcb fill frame}{%
    \pgfseteorule%
    \iftcb@hasTitle%
      \iftcb@titlefilled%
        \ifdim\dimexpr\kvtcb@title@rule>0pt\relax%
          \tcb@boundaryframe@pathlast%
          \tcb@arc@zpt%
          \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule}%
          \tcbdimto\tcb@xb{\tcb@width-\kvtcb@right@rule}%
          \tcbdimto\tcb@yb{\tcb@height-\kvtcb@top@rule}%
          \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
          \tcb@boundaryinterior@title@standard%
        \else%
          \tcb@boundaryframe@pathlast%
          \tcb@boundary@base{\kvtcb@left@rule}{\kvtcb@bottom@rule}%
            {\tcb@width-\kvtcb@right@rule}{\tcb@height-\kvtcb@top@rule}%
            {\tcb@arc@ins@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
        \fi%
      \else%
        \tcb@boundaryframe@pathlast%
      \fi%
    \else%
      \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
      \pgfpathmoveto{\pgfpointorigin}%
      \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
      \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@height}}%
      \tcb@arc@ins@SW\pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\kvtcb@bottom@rule}}%
      \tcb@arc@ins@SE\pgfpathlineto{\pgfqpoint{\tcb@xa}{\kvtcb@bottom@rule}}%
      \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@height}}%
      \pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
      \tcb@arc@out@SE\pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
      \tcb@arc@out@SW\pgfpathclose%
    \fi%
  }%
}


\def\tcb@draw@shadowjigsaw@unbroken{%
  \let\tcb@shadow=\tcb@shadow@unbroken%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\def\tcb@draw@shadowjigsaw@first{%
  \let\tcb@shadow=\tcb@shadow@first%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\def\tcb@draw@shadowjigsaw@middle{%
  \let\tcb@shadow=\tcb@shadow@middle%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\def\tcb@draw@shadowjigsaw@last{%
  \let\tcb@shadow=\tcb@shadow@last%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\tcb@new@skin{enhanced jigsaw}{base@unbroken,%
  frame engine=pathjigsaw,interior titled engine=path,interior engine=path,segmentation engine=path,title engine=path,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@unbroken},%
  skin first=enhancedfirst jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedlast jigsaw}

\tcb@new@skin{enhancedfirst jigsaw}{base@first,%
  frame engine=pathfirstjigsaw,interior titled engine=pathfirst,interior engine=pathfirst,segmentation engine=path,title engine=pathfirst,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@first},%
  skin first=enhancedfirst jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedmiddle jigsaw}

\tcb@new@skin{enhancedmiddle jigsaw}{base@middle,%
  frame engine=pathmiddlejigsaw,interior titled engine=pathmiddle,interior engine=pathmiddle,segmentation engine=path,title engine=pathmiddle,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@middle},%
  skin first=enhancedmiddle jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedmiddle jigsaw}

\tcb@new@skin{enhancedlast jigsaw}{base@last,%
  frame engine=pathlastjigsaw,interior titled engine=pathlast,interior engine=pathlast,segmentation engine=path,title engine=pathlast,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@last},%
  skin first=enhancedmiddle jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedlast jigsaw}

\tcbset{%
  enhanced jigsaw/.style={skin=enhanced jigsaw},%
  enhanced standard jigsaw/.style={skin=enhanced jigsaw,
    skin first=enhanced jigsaw,skin middle=enhanced jigsaw,skin last=enhanced jigsaw},%
  frame engine/pathjigsaw/.style={frame code=\tcb@drawframe@pathjigsaw},
  frame engine/pathfirstjigsaw/.style={frame code=\tcb@drawframe@pathfirstjigsaw},
  frame engine/pathmiddlejigsaw/.style={frame code=\tcb@drawframe@pathmiddlejigsaw},
  frame engine/pathlastjigsaw/.style={frame code=\tcb@drawframe@pathlastjigsaw},
}



==> tcbtheorems.code.tex <==
%% The LaTeX package tcolorbox - version 4.30 (2020/04/28)
%% tcbtheorems.code.tex: Code for theorems in colorboxes
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2020 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{4.30}

\RequirePackage{amsmath}

\def\tcb@hack@amsmath{\tcb@hack@currenvir\vskip-\abovedisplayskip}

\def\tcb@theo@form@namenumber#1#2{\hbox{#1~#2}}
\def\tcb@theo@form@numbername#1#2{\hbox{#2~#1}}
\def\tcb@theo@form@name#1#2{\hbox{#1}}

\def\tcb@theo@desc@form@std#1{\tcb@desc@col\kvtcb@desc@font\kvtcb@desc@delim@left#1\kvtcb@desc@delim@right}

\def\tcb@theo@title#1#2#3{%
  \ifdefempty{#2}{\setbox\z@=\color@hbox#1\color@endbox}{\setbox\z@=\tcb@theo@form{#1}{#2}}%
  \def\temp@a{#3}%
  \ifx\temp@a\@empty\relax%
    \unhbox\z@\kvtcb@terminatorsign%
  \else%
    \setbox\z@=\hbox{\unhbox\z@\kvtcb@separatorsign\ }%
    \hangindent\wd\z@%
    \hangafter=1%
    \mbox{\unhbox\z@}{\tcb@theo@desc@form{#3}}\kvtcb@terminatorsign%
  \fi%
}

\def\tcb@theo@listentry#1#2#3{%
  \def\kvtcb@listentry{\protect\numberline{#2}#3}%
}

\def\tcb@theo@label#1#2{%
  \def\temp@a{#2}%
  \ifx\temp@a\@empty%
  \else%
    \tcbset{label={#1\kvtcb@label@sep#2},%
      tcb@theo@full@label@supp={#1\kvtcb@label@sep#2},tcb@theo@label@supp={#2}}%
  \fi%
}

\if@fleqn%
\tcbset{%
  ams equation upper/.style={before upper*=\tcb@hack@amsmath\equation,after upper*=\endequation},%
  ams equation lower/.style={before lower*=\tcb@hack@amsmath\equation,after lower*=\endequation},%
  ams equation* upper/.style={before upper*=\tcb@hack@amsmath\csname equation*\endcsname,after upper*=\endequation},%
  ams equation* lower/.style={before lower*=\tcb@hack@amsmath\csname equation*\endcsname,after lower*=\endequation}%
}%
\else%
\tcbset{%
  ams equation upper/.style={before upper*=\tcb@hack@currenvir\equation,after upper*=\endequation},%
  ams equation lower/.style={before lower*=\tcb@hack@currenvir\equation,after lower*=\endequation},%
  ams equation* upper/.style={before upper*=\tcb@hack@currenvir\csname equation*\endcsname,after upper*=\endequation},%
  ams equation* lower/.style={before lower*=\tcb@hack@currenvir\csname equation*\endcsname,after lower*=\endequation},%
}%
\fi

\tcbset{
  theorem/.style args={#1#2#3#4}{%
    step and label={#2}{#4},%
    title={\letcs\tcb@temp{the#2}\tcb@theo@title{#1}{\tcb@temp}{#3}}},%
  math upper/.style={before upper*=$\displaystyle,after upper*=$},%
  math lower/.style={before lower*=$\displaystyle,after lower*=$},%
  math/.style={math upper,math lower},%
  ams equation/.style={ams equation upper,ams equation lower},%
  ams equation*/.style={ams equation* upper,ams equation* lower},%
  ams align upper/.style={before upper*=\tcb@hack@amsmath\align,after upper*=\endalign},%
  ams align lower/.style={before lower*=\tcb@hack@amsmath\align,after lower*=\endalign},%
  ams align/.style={ams align upper,ams align lower},%
  ams align* upper/.style={before upper*=\tcb@hack@amsmath\csname align*\endcsname,after upper*=\endalign},%
  ams align* lower/.style={before lower*=\tcb@hack@amsmath\csname align*\endcsname,after lower*=\endalign},%
  ams align*/.style={ams align* upper,ams align* lower},%
  ams gather upper/.style={before upper*=\tcb@hack@amsmath\gather,after upper*=\endgather},%
  ams gather lower/.style={before lower*=\tcb@hack@amsmath\gather,after lower*=\endgather},%
  ams gather/.style={ams gather upper,ams gather lower},%
  ams gather* upper/.style={before upper*=\tcb@hack@amsmath\csname gather*\endcsname,after upper*=\endgather},%
  ams gather* lower/.style={before lower*=\tcb@hack@amsmath\csname gather*\endcsname,after lower*=\endgather},%
  ams gather*/.style={ams gather* upper,ams gather* lower},%
  ams nodisplayskip upper/.style={before upper=\vskip-\abovedisplayskip},%
  ams nodisplayskip lower/.style={before lower=\vskip-\abovedisplayskip},%
  ams nodisplayskip/.style={ams nodisplayskip upper,ams nodisplayskip lower},%
  highlight math style/.style={highlight math/.style={notitle,nophantom,#1}},%
  separator sign/.store in=\kvtcb@separatorsign,%
  separator sign colon/.style={separator sign={:}},%
  separator sign dash/.style={separator sign={\ --}},%
  separator sign none/.style={separator sign=},%
  terminator sign/.store in=\kvtcb@terminatorsign,%
  terminator sign colon/.style={terminator sign={:}},%
  terminator sign dash/.style={terminator sign={\ --}},%
  terminator sign none/.style={terminator sign=},%
  label separator/.store in=\kvtcb@label@sep,%
  description delimiters/.code 2 args={\def\kvtcb@desc@delim@left{#1}\def\kvtcb@desc@delim@right{#2}},%
  description delimiters parenthesis/.style={description delimiters=()},
  description delimiters none/.style={description delimiters={}{}},
  description color/.code={\def\temp@a{#1}\ifx\temp@a\@empty\relax%
    \def\tcb@desc@col{}\else\def\tcb@desc@col{\color{#1}}\fi},%
  description color/.default=,
  description font/.store in=\kvtcb@desc@font,
  description font/.default=,
  description formatter/.code={\let\tcb@theo@desc@form=#1},%
  description formatter/.default={\tcb@theo@desc@form@std},%
  theorem name and number/.code={\let\tcb@theo@form=\tcb@theo@form@namenumber},
  theorem number and name/.code={\let\tcb@theo@form=\tcb@theo@form@numbername},
  theorem name/.code={\let\tcb@theo@form=\tcb@theo@form@name},
  theorem style/.is choice,
  theorem style/standard/.style={separator sign colon,description delimiters none,
    terminator sign none,theorem name and number,attach title},
  theorem style/change standard/.style={theorem style=standard,theorem number and name},
  theorem style/plain/.style={separator sign none,description delimiters parenthesis,
    terminator sign colon,theorem name and number,attach title to upper={\ }},
  theorem style/plain apart/.style={separator sign none,description delimiters parenthesis,
    terminator sign none,theorem name and number,attach title},
  theorem style/break/.style={theorem style=plain,attach title to upper={\par}},
  theorem style/change/.style={theorem style=plain,theorem number and name},
  theorem style/change apart/.style={theorem style=plain apart,theorem number and name},
  theorem style/change break/.style={theorem style=break,theorem number and name},
  theorem style/margin/.style={theorem style=plain,theorem name,before title=\makebox[0pt][r]{\thetcbcounter\ }},
  theorem style/margin apart/.style={theorem style=margin,attach title,terminator sign none},
  theorem style/margin break/.style={theorem style=margin,attach title to upper={\par}},
  theorem label supplement/.style={tcb@theo@label@supp/.style={#1}},
  theorem full label supplement/.style={tcb@theo@full@label@supp/.style={#1}},
}

\newcommand{\new@tcbtheorem}[5][]{%
  \@@newtcolorbox[auto counter,#1]{#2}[3][]{#4,%
    title={\tcb@theo@title{#3}{\thetcbcounter}{##2}},%
    list entry={\protect\numberline{\thetcbcounter}##2},%
    nameref={##2},%
    code={\tcb@theo@label{#5}{##3}},%
    ##1}%
  \@@newtcolorbox[#1,no counter,list inside=]{#2*}[2][]{#4,%
    title={\tcb@theo@title{#3}{\@empty}{##2}},%
    ##1}%
}

\def\newtcbtheorem{\let\@@newtcolorbox\newtcolorbox%
  \new@tcbtheorem}

\def\renewtcbtheorem{\let\@@newtcolorbox\renewtcolorbox%
  \new@tcbtheorem}

\newtcbox{\tcboxmath}[1][]{nobeforeafter,math upper,tcbox raise base,#1}
\newtcbox{\tcbhighmath}[1][]{highlight math,nobeforeafter,math upper,tcbox raise base,#1}

\tcbset{%
  reset@theorems/.style={%
    description formatter,description color,description font,
    highlight math style={colframe=red,colback=yellow!25!white},%
    theorem style=standard,label separator=:,%
    theorem label supplement=,theorem full label supplement=,%
  },
  initialize@reset=reset@theorems,
}

% DEPRECATED
\newcommand{\tcbmaketheorem}[5]{%
  \newtcolorbox{#1}[3][]{#3,theorem={#2}{#4}{##2}{#5\kvtcb@label@sep##3},##1}%
}


==> tcbvignette.code.tex <==
%% The LaTeX package tcolorbox - version 4.30 (2020/04/28)
%% tcbvignette.code.tex: Code for ornamental frames
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2020 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{4.30}

\tcbuselibrary{skins}

\usetikzlibrary{fadings}

\pgfdeclarehorizontalshading{tcb@fade@east}{100bp}
{color(0bp)=(pgftransparent!50); color(25bp)=(pgftransparent!50);
 color(75bp)=(pgftransparent!100); color(100bp)=(pgftransparent!100)}

\pgfdeclarehorizontalshading{tcb@fade@west}{100bp}
{color(0bp)=(pgftransparent!100); color(25bp)=(pgftransparent!100);
 color(75bp)=(pgftransparent!50); color(100bp)=(pgftransparent!50)}

\pgfdeclareverticalshading{tcb@fade@north}{100bp}
{color(0bp)=(pgftransparent!50); color(25bp)=(pgftransparent!50);
 color(75bp)=(pgftransparent!100); color(100bp)=(pgftransparent!100)}

\pgfdeclareverticalshading{tcb@fade@south}{100bp}
{color(0bp)=(pgftransparent!100); color(25bp)=(pgftransparent!100);
 color(75bp)=(pgftransparent!50); color(100bp)=(pgftransparent!50)}

\pgfdeclarefading{semi east}{\pgfuseshading{tcb@fade@east}}
\pgfdeclarefading{semi west}{\pgfuseshading{tcb@fade@west}}
\pgfdeclarefading{semi north}{\pgfuseshading{tcb@fade@north}}
\pgfdeclarefading{semi south}{\pgfuseshading{tcb@fade@south}}

\def\tcb@vig@draw@north#1{\path[#1]\pgfextra{%
  \pgfpathmoveto{\pgfqpoint{\tcb@vig@xA}{\tcb@vig@yB}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xB}{\tcb@vig@yB}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xb}{\tcb@vig@yb}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xa}{\tcb@vig@yb}}%
  \pgfpathclose};}

\def\tcb@vig@draw@east#1{\path[#1]\pgfextra{%
  \pgfpathmoveto{\pgfqpoint{\tcb@vig@xB}{\tcb@vig@yB}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xB}{\tcb@vig@yA}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xb}{\tcb@vig@ya}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xb}{\tcb@vig@yb}}%
  \pgfpathclose};}

\def\tcb@vig@draw@south#1{\path[#1]\pgfextra{%
  \pgfpathmoveto{\pgfqpoint{\tcb@vig@xB}{\tcb@vig@yA}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xA}{\tcb@vig@yA}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xa}{\tcb@vig@ya}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xb}{\tcb@vig@ya}}%
  \pgfpathclose};}

\def\tcb@vig@draw@west#1{\path[#1]\pgfextra{%
  \pgfpathmoveto{\pgfqpoint{\tcb@vig@xA}{\tcb@vig@yA}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xA}{\tcb@vig@yB}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xa}{\tcb@vig@yb}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xa}{\tcb@vig@ya}}%
  \pgfpathclose};}

\def\tcb@vig@draw@direct{%
  \ifdim\tcb@vig@yB>\tcb@vig@yb\relax%
    \begingroup\edef\x{\endgroup\noexpand\tcb@vig@draw@north{fill,draw=none,\expandonce\tcb@vig@style@north}}\x%
  \fi%
  \ifdim\tcb@vig@xB>\tcb@vig@xb\relax%
    \begingroup\edef\x{\endgroup\noexpand\tcb@vig@draw@east{fill,draw=none,\expandonce\tcb@vig@style@east}}\x%
  \fi%
  \ifdim\tcb@vig@yA<\tcb@vig@ya\relax%
    \begingroup\edef\x{\endgroup\noexpand\tcb@vig@draw@south{fill,draw=none,\expandonce\tcb@vig@style@south}}\x%
  \fi%
  \ifdim\tcb@vig@xA<\tcb@vig@xa\relax%
    \begingroup\edef\x{\endgroup\noexpand\tcb@vig@draw@west{fill,draw=none,\expandonce\tcb@vig@style@west}}\x%
  \fi%
}

\def\tcb@vig@draw@clipped{%
  \ifdim\tcb@vig@yB>\tcb@vig@yb\relax%
    \begin{scope}
    \tcb@vig@draw@north{clip}%
    \begingroup\edef\x{\endgroup\noexpand\path[fill,\expandonce\tcb@vig@style@north]}%
    \x\pgfextra{\pgfpathrectanglecorners{\pgfpoint{\tcb@vig@xA-1mm}{\tcb@vig@yb}}%
        {\pgfpoint{\tcb@vig@xB+1mm}{\tcb@vig@yB}}};
    \end{scope}
  \fi%
  \ifdim\tcb@vig@xB>\tcb@vig@xb\relax%
    \begin{scope}
    \tcb@vig@draw@east{clip}%
    \begingroup\edef\x{\endgroup\noexpand\path[fill,\expandonce\tcb@vig@style@east]}%
    \x\pgfextra{\pgfpathrectanglecorners{\pgfpoint{\tcb@vig@xb}{\tcb@vig@yA-1mm}}%
          {\pgfpoint{\tcb@vig@xB}{\tcb@vig@yB+1mm}}};
    \end{scope}
  \fi%
  \ifdim\tcb@vig@yA<\tcb@vig@ya\relax%
    \begin{scope}
    \tcb@vig@draw@south{clip}%
    \begingroup\edef\x{\endgroup\noexpand\path[fill,\expandonce\tcb@vig@style@south]}%
    \x\pgfextra{\pgfpathrectanglecorners{\pgfpoint{\tcb@vig@xA-1mm}{\tcb@vig@yA}}%
        {\pgfpoint{\tcb@vig@xB+1mm}{\tcb@vig@ya}}};
    \end{scope}
  \fi%
  \ifdim\tcb@vig@xA<\tcb@vig@xa\relax%
    \begin{scope}
    \tcb@vig@draw@west{clip}%
    \begingroup\edef\x{\endgroup\noexpand\path[fill,\expandonce\tcb@vig@style@west]}%
    \x\pgfextra{%
      \pgfpathrectanglecorners{\pgfpoint{\tcb@vig@xA}{\tcb@vig@yA-1mm}}%
        {\pgfpoint{\tcb@vig@xa}{\tcb@vig@yB+1mm}}};
    \end{scope}
  \fi%
}

\newcommand{\tcbvignette}[1]{%
  \ifdefined\pgfpictureid%
    \begingroup%
    \tcbset{vig/.cd,#1}%
    \tcbdimto\tcb@vig@xA{\tcb@vig@xmin}%
    \tcbdimto\tcb@vig@xB{\tcb@vig@xmax}%
    \tcbdimto\tcb@vig@yA{\tcb@vig@ymin}%
    \tcbdimto\tcb@vig@yB{\tcb@vig@ymax}%
    \tcbdimto\tcb@vig@xa{\tcb@vig@xA+\tcb@vig@size@west}%
    \tcbdimto\tcb@vig@xb{\tcb@vig@xB-(\tcb@vig@size@east)}%
    \tcbdimto\tcb@vig@ya{\tcb@vig@yA+\tcb@vig@size@south}%
    \tcbdimto\tcb@vig@yb{\tcb@vig@yB-(\tcb@vig@size@north)}%
    \begin{scope}[tcb@vig@scope]%
    \tcb@vig@draw%
    \end{scope}
    \endgroup%
  \else%
    \tcb@warning{'tcbvignette' was found outside a 'tikzpicture' environment and is ignored}%
  \fi%
}

\tcbset{%
  vig/.cd,
  xmin/.store in=\tcb@vig@xmin,
  xmax/.store in=\tcb@vig@xmax,
  ymin/.store in=\tcb@vig@ymin,
  ymax/.store in=\tcb@vig@ymax,
  lower left corner/.code={\tcb@gettikzxy{(#1)}{\tcb@vig@xmin}{\tcb@vig@ymin}},
  upper right corner/.code={\tcb@gettikzxy{(#1)}{\tcb@vig@xmax}{\tcb@vig@ymax}},
  %
  inside node/.style={lower left corner={#1.south west},upper right corner={#1.north east}},
  outside node/.style={lower left corner={[xshift=-\tcb@vig@size@west,yshift=-\tcb@vig@size@south]#1.south west},
    upper right corner={[xshift=\tcb@vig@size@east,yshift=\tcb@vig@size@north]#1.north east}},
  %
  on node/.style={lower left corner={#1.south west},upper right corner={#1.north east}},
  over node offset/.store in=\tcb@vig@onoffset,%
  over node/.style={lower left corner={[xshift=-\tcb@vig@onoffset,yshift=-\tcb@vig@onoffset]#1.south west},
    upper right corner={[xshift=\tcb@vig@onoffset,yshift=\tcb@vig@onoffset]#1.north east}},
  north size/.store in=\tcb@vig@size@north,
  south size/.store in=\tcb@vig@size@south,
  east size/.store in=\tcb@vig@size@east,
  west size/.store in=\tcb@vig@size@west,
  vertical size/.style={north size=#1,south size=#1},
  horizontal size/.style={east size=#1,west size=#1},
  size/.style={north size=#1,south size=#1,east size=#1,west size=#1},
  north style/.store in=\tcb@vig@style@north,
  south style/.store in=\tcb@vig@style@south,
  east style/.store in=\tcb@vig@style@east,
  west style/.store in=\tcb@vig@style@west,
  scope/.code={\tikzset{tcb@vig@scope/.style={#1}}},
  draw method/.is choice,
  draw method/direct/.code={\let\tcb@vig@draw\tcb@vig@draw@direct},%
  draw method/clipped/.code={\let\tcb@vig@draw\tcb@vig@draw@clipped},%
  base color/.colorlet=tcbcol@vig@base,
  raised color/.style={%
    base color=#1,
    north style={tcbcol@vig@base!50!white},
    east style={tcbcol@vig@base!75!black},
    south style={tcbcol@vig@base!50!black},
    west style={tcbcol@vig@base!75!white},
  },
  lowered color/.style={%
    base color=#1,
    north style={tcbcol@vig@base!50!black},
    east style={tcbcol@vig@base!75!white},
    south style={tcbcol@vig@base!50!white},
    west style={tcbcol@vig@base!75!black},
  },
  color from/.style args={#1 to #2}{%
    north style={bottom color=#1,top color=#2},
    east style={left color=#1,right color=#2},
    south style={top color=#1,bottom color=#2},
    west style={right color=#1,left color=#2},
  },
  fade in/.style={%
    north style={#1,path fading=south},
    east style={#1,path fading=west},
    south style={#1,path fading=north},
    west style={#1,path fading=east},
  },
  fade in/.default=white,
  fade out/.style={%
    north style={#1,path fading=north},
    east style={#1,path fading=east},
    south style={#1,path fading=south},
    west style={#1,path fading=west},
  },
  fade out/.default=white,
  semi fade in/.style={%
    north style={#1,path fading=semi south},
    east style={#1,path fading=semi west},
    south style={#1,path fading=semi north},
    west style={#1,path fading=semi east},
  },
  semi fade in/.default=white,
  semi fade out/.style={%
    north style={#1,path fading=semi north},
    east style={#1,path fading=semi east},
    south style={#1,path fading=semi south},
    west style={#1,path fading=semi west},
  },
  semi fade out/.default=white,
  %
  scope=,
  draw method=direct,
  xmin=0pt,
  xmax=1cm,
  ymin=0pt,
  ymax=1cm,
  size=2mm,
  over node offset=0.1mm,
  raised color=red,
}

\tcbset{%
  finish@vignette/.style 2 args={finish #1={%
    \begin{tcbclipframe}\tcbvignette{%
      scope={transparency group,opacity=0.25},
      north style=white,
      east style=black!75,
      south style=black,
      west style=black!25,#2,inside node=frame
      }\end{tcbclipframe}}},
  finish vignette/.style={%
    finish@vignette={unbroken}{#1},%
    finish@vignette={first}{#1,south size=0pt},%
    finish@vignette={middle}{#1,north size=0pt,south size=0pt},%
    finish@vignette={last}{#1,north size=0pt}%
  },
%
  finish@raised@vignette/.style 2 args={finish #1={%
    \begin{tcbclipframe}\tcbvignette{%
      draw method=clipped,
      north style={white,path fading=semi south},
      east style={black!75,path fading=semi west},
      south style={black,path fading=semi north},
      west style={black!25,path fading=semi east},#2,inside node=frame
      }\end{tcbclipframe}}},
  finish raised fading vignette/.style={%
    finish@raised@vignette={unbroken}{#1},%
    finish@raised@vignette={first}{#1,south size=0pt},%
    finish@raised@vignette={middle}{#1,north size=0pt,south size=0pt},%
    finish@raised@vignette={last}{#1,north size=0pt}%
  },
%
  finish@fading@vignette/.style 2 args={finish #1={%
    \tcbvignette{%
      draw method=clipped,fade in=tcbcol@vig@base,#2,over node=frame}}},
  finish fading vignette/.style={%
    finish@fading@vignette={unbroken}{base color=white,#1},%
    finish@fading@vignette={first}{base color=white,#1,south size=0pt},%
    finish@fading@vignette={middle}{base color=white,#1,north size=0pt,south size=0pt},%
    finish@fading@vignette={last}{base color=white,#1,north size=0pt}%
  },
%
  underlay@vignette/.style 2 args={underlay #1={%
    \begin{tcbclipframe}\tcbvignette{%
      raised color=tcbcolframe,
      north size=\kvtcb@top@rule@stand,
      south size=\kvtcb@bottom@rule@stand,
      west size=\kvtcb@left@rule,
      east size=\kvtcb@right@rule,#2,inside node=frame
      }\end{tcbclipframe}}},
  underlay vignette/.style={%
    underlay@vignette={unbroken}{#1},%
    underlay@vignette={first}{#1,south size=0pt},%
    underlay@vignette={middle}{#1,north size=0pt,south size=0pt},%
    underlay@vignette={last}{#1,north size=0pt}%
  },
%
  underlay@fading@vignette/.style 2 args={underlay #1={%
    \begin{tcbclipframe}\tcbvignette{%
      draw method=clipped,
      north style={white,path fading=semi south},
      east style={black!75,path fading=semi west},
      south style={black,path fading=semi north},
      west style={black!25,path fading=semi east},#2,inside node=frame,
      }\end{tcbclipframe}}},
  underlay raised fading vignette/.style={%
    underlay@fading@vignette={unbroken}{#1},%
    underlay@fading@vignette={first}{#1,south size=0pt},%
    underlay@fading@vignette={middle}{#1,north size=0pt,south size=0pt},%
    underlay@fading@vignette={last}{#1,north size=0pt}%
  },
  %
  underlay raised shading vignette/.style={%
    underlay vignette={draw method=clipped,
      north style={bottom color=tcbcolframe,top color=tcbcolframe!33!white},
      east style={left color=tcbcolframe,right color=tcbcolframe!66!black},
      south style={top color=tcbcolframe,bottom color=tcbcolframe!33!black},
      west style={right color=tcbcolframe,left color=tcbcolframe!66!white},#1}},
  %
  underlay shade in vignette/.style={%
    underlay vignette={draw method=clipped,color from=tcbcolback to tcbcolframe,#1}},
}


==> tcbxparse.code.tex <==
%% The LaTeX package tcolorbox - version 4.30 (2020/04/28)
%% tcbxparse.code.tex: Code for xparse features
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2020 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{4.30}

\RequirePackage{xparse}[2013/12/31]

\tcbset{%
  IfNoValueTF/.code n args={3}{\IfNoValueTF{#1}{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}},
  IfValueTF/.code n args={3}{\IfValueTF{#1}{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}},
  IfBooleanTF/.code n args={3}{\IfBooleanTF{#1}{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}},
  verbatim/.style={fontupper=\ttfamily,nobeforeafter,tcbox raise base,top=0pt,bottom=0pt,left=1mm,right=1mm,boxrule=0.3mm}
}

%-- tcolorbox --
\long\def\tcb@New@TColorBox#1#2#3{%
  \tcb@newenvironment{#1}{#2}{\tcolorbox[#3,options@for=#1]}{\endtcolorbox}}

\def\DeclareTColorBox{%
  \let\tcb@newenvironment\DeclareDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TColorBox%
  \tcb@process@newenvironment}

\def\NewTColorBox{%
  \let\tcb@newenvironment\NewDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TColorBox%
  \tcb@process@newenvironment}

\def\RenewTColorBox{%
  \let\tcb@newenvironment\RenewDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TColorBox%
  \tcb@process@newenvironment}

\def\ProvideTColorBox{%
  \let\tcb@newenvironment\ProvideDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TColorBox%
  \tcb@process@newenvironment}

%-- tcolorbox (total) --
\long\def\tcb@New@TotalTColorBox#1#2#3#4{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\begin{tcolorbox}[#3,options@for=#1]#4\end{tcolorbox}}}

\def\DeclareTotalTColorBox{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTColorBox%
  \tcb@process@newcommand}

\def\NewTotalTColorBox{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTColorBox%
  \tcb@process@newcommand}

\def\RenewTotalTColorBox{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTColorBox%
  \tcb@process@newcommand}

\def\ProvideTotalTColorBox{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTColorBox%
  \tcb@process@newcommand}

%-- tcbox --
\long\def\tcb@New@TCBox#1#2#3{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcbox[#3,options@for=#1]}}

\def\DeclareTCBox{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBox%
  \tcb@process@newcommand}

\def\NewTCBox{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBox%
  \tcb@process@newcommand}

\def\RenewTCBox{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBox%
  \tcb@process@newcommand}

\def\ProvideTCBox{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBox%
  \tcb@process@newcommand}

%-- tcbox (total) --
\long\def\tcb@New@TotalTCBox#1#2#3#4{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcbox[#3,options@for=#1]{#4}}}

\def\DeclareTotalTCBox{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBox%
  \tcb@process@newcommand}

\def\NewTotalTCBox{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBox%
  \tcb@process@newcommand}

\def\RenewTotalTCBox{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBox%
  \tcb@process@newcommand}

\def\ProvideTotalTCBox{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBox%
  \tcb@process@newcommand}

\DeclareTotalTCBox{\tcboxverb}{ O{} v }{verbatim,#1}{#2}

%-- tcboxfit --
\long\def\tcb@New@TCBoxFit#1#2#3{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcboxfit[#3,options@for=#1]}}

\def\DeclareTCBoxFit{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBoxFit%
  \tcb@process@newcommand}

\def\NewTCBoxFit{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBoxFit%
  \tcb@process@newcommand}

\def\RenewTCBoxFit{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBoxFit%
  \tcb@process@newcommand}

\def\ProvideTCBoxFit{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBoxFit%
  \tcb@process@newcommand}

\long\def\tcb@New@TotalTCBoxFit#1#2#3#4{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcboxfit[#3,options@for=#1]{#4}}}

\def\DeclareTotalTCBoxFit{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBoxFit%
  \tcb@process@newcommand}

\def\NewTotalTCBoxFit{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBoxFit%
  \tcb@process@newcommand}

\def\RenewTotalTCBoxFit{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBoxFit%
  \tcb@process@newcommand}

\def\ProvideTotalTCBoxFit{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBoxFit%
  \tcb@process@newcommand}


%-- tcblisting --
\long\def\tcb@New@TCBListing#1#2#3{%
  \tcb@newenvironment{#1}{#2}{\tcblisting{#3,options@for=#1}}{\endtcblisting}}

\def\DeclareTCBListing{%
  \let\tcb@newenvironment\DeclareDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBListing%
  \tcb@process@newenvironment}

\def\NewTCBListing{%
  \let\tcb@newenvironment\NewDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBListing%
  \tcb@process@newenvironment}

\def\RenewTCBListing{%
  \let\tcb@newenvironment\RenewDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBListing%
  \tcb@process@newenvironment}

\def\ProvideTCBListing{%
  \let\tcb@newenvironment\ProvideDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBListing%
  \tcb@process@newenvironment}

%-- tcbinputlisting --
\long\def\tcb@New@TCBInputListing#1#2#3{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcbinputlisting{#3,options@for=#1}}%
}

\def\DeclareTCBInputListing{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBInputListing%
  \tcb@process@newcommand}

\def\NewTCBInputListing{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBInputListing%
  \tcb@process@newcommand}

\def\RenewTCBInputListing{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBInputListing%
  \tcb@process@newcommand}

\def\ProvideTCBInputListing{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBInputListing%
  \tcb@process@newcommand}


%-- sidebyside --

\def\tcb@sbs@content@none{\tcb@sbs@text@left\tcblower\tcb@sbs@text@right}
\def\tcb@sbs@content@left{\box\tcb@upperbox\tcblower\tcb@sbs@text@right}
\def\tcb@sbs@content@right{\tcb@sbs@text@left\tcblower\box\tcb@lowerbox}
\def\tcb@sbs@content@both{\box\tcb@upperbox\tcblower\box\tcb@lowerbox}

\def\tcb@sbs@save@upper{%
  \colorlet{tcbcol@origin}{.}%
  \tcb@set@color{tcbcolupper}%
  \sbox{\tcb@upperbox}{\kvtcb@fontupper\kvtcb@halignupper\tcb@insert@before@upper\tcb@sbs@text@left\tcb@insert@after@upper}%
  \tcb@reset@color%
}
\def\tcb@sbs@save@lower{%
  \colorlet{tcbcol@origin}{.}%
  \tcb@set@color{tcbcollower}%
  \sbox{\tcb@lowerbox}{\kvtcb@fontlower\kvtcb@halignlower\tcb@insert@before@lower\tcb@sbs@text@right\tcb@insert@after@lower}%
  \tcb@reset@color%
}

\tcbset{%
  sidebyside adapt/.is choice,
  sidebyside adapt/none/.style={%
    sidebyside@adapt@process/.style={%
      code={\let\tcb@sbs@content\tcb@sbs@content@none},
    }%
  },
  sidebyside adapt/left/.style={%
    sidebyside@adapt@process/.style={%
      code={\tcb@sbs@save@upper\let\tcb@sbs@content\tcb@sbs@content@left},
      lefthand width=\wd\tcb@upperbox,
    }%
  },
  sidebyside adapt/right/.style={%
    sidebyside@adapt@process/.style={%
      code={\tcb@sbs@save@lower\let\tcb@sbs@content\tcb@sbs@content@right},
      righthand width=\wd\tcb@lowerbox,
    }%
  },
  sidebyside adapt/both/.style={%
    sidebyside@adapt@process/.style={%
      code={\tcb@sbs@save@upper\tcb@sbs@save@lower\let\tcb@sbs@content\tcb@sbs@content@both},
      text width=\wd\tcb@upperbox+\kvtcb@sbs@gap+\wd\tcb@lowerbox,
      lefthand width=\wd\tcb@upperbox,
    }%
  },
  %
  sidebyside switch/.is choice,
  sidebyside switch/true/.style={%
    sidebyside@switch/.code={%
      \tcb@swap{\tcb@sbs@text@left}{\tcb@sbs@text@right}
    }%
  },
  sidebyside switch/false/.style={%
    sidebyside@switch/.style=%
  },
  sidebyside switch/.default=true
}


\DeclareTotalTColorBox{\tcbsidebyside}{ +O{} +m +m }{%
  code={\long\def\tcb@sbs@text@left{#2}\long\def\tcb@sbs@text@right{#3}},%
  #1,%
  sidebyside,%
  sidebyside@switch,sidebyside@adapt@process%
}{\tcb@sbs@content}


\tcbset{%
  reset@xparse/.style={%
    sidebyside adapt=none,sidebyside switch=false,%
  },
  initialize@reset=reset@xparse,
}


==> tcolorbox.doc.breakable.tex <==
% !TeX root = tcolorbox.tex
% include file of tcolorbox.tex (manual of the LaTeX package tcolorbox)
\clearpage
\section{Library \mylib{breakable}}\label{sec:breakable}%
\tcbset{external/prefix=external/breakable_}%
The library is loaded by a package option or inside the preamble by:
\begin{dispListing}
\tcbuselibrary{breakable}
\end{dispListing}

\subsection{Technical Overview}
The library \mylib{breakable} supports the automatic breaking of a |tcolorbox|.
This feature is enabled by \refKey{/tcb/breakable}
and disabled by \refKey{/tcb/unbreakable}.

{
\tcbset{colframe=Navy,colback=AliceBlue,fonttitle=\bfseries,
  watermark color=AliceBlue!85!Navy,enhanced}
If a |tcolorbox| is set to be \refKey{/tcb/breakable}, then the following
algorithm is executed:
\begin{enumerate}
\item The box content is read to a box register similar but not identical
  to the unbreakable case.
\item If the total box fits into the current page, it is shipped out visibly
  unbroken and the algorithm stops.
  \begin{tcolorbox}[title=Unbroken Box,watermark text=unbroken]
  The box.
  \end{tcolorbox}
\item Otherwise, it is checked if at least \refKey{/tcb/lines before break}
  of the upper box can be placed on the current page.
  If not, a page break is inserted and the algorithm goes back to Step 2.
\item Now, the \emph{break sequence} starts.
  The upper box part or the lower box part is split such that it fits
  into the current page. The fitting part is named \emph{first part} of
  the \emph{break sequence} and shipped out.
  \begin{tcolorbox}[title=Broken Box,watermark text=first,skin=enhancedfirst]
  The box.
  \end{tcolorbox}
\item
  If the remaining content of the total box
  fits into the current page, the algorithm continues with Step 7, else
  with Step 6.
\item
  The upper box part or the lower box part is split such that it fits
  into the current page. The fitting part is named \emph{middle part} of
  the \emph{break sequence} and shipped out.
  Then, the algorithm goes back to Step 5.
  \begin{tcolorbox}[watermark text=middle,skin=enhancedmiddle]
  The box.
  \end{tcolorbox}
\item
  The remaining part is named \emph{last part} of
  the \emph{break sequence} and shipped out. The algorithm stops.
  \begin{tcolorbox}[watermark text=last,skin=enhancedlast]
  The box.
  \end{tcolorbox}
\end{enumerate}
}

The algorithm takes care that the optional segmentation line never appears at
the end of a box. The optional lower box part is also checked to
have at least \refKey{/tcb/lines before break}.

\clearpage
In principle, all boxes of the \emph{break sequence} share the same geometric
parameters. The differences are:
\begin{itemize}
\item The given \refKey{/tcb/before} and \refKey{/tcb/after} values are
  used only before the \emph{first} and after the \emph{last} part
  of the \emph{break sequence}.
\item A special behavior between the parts of the \emph{break sequence} can
  be given by \refKey{/tcb/toprule at break},
  \refKey{/tcb/bottomrule at break},
  \refKey{/tcb/enlarge top at break by}, and
  \refKey{/tcb/enlarge bottom at break by}.
\item The \refKey{/tcb/skin} decides \emph{how} the \emph{first}, \emph{middle},
  and \emph{last} part look like. Actually, every part type has its own
  skin given by the options  \refKey{/tcb/skin first}, \refKey{/tcb/skin middle}, and
  \refKey{/tcb/skin last}. Typically, these options are set automatically by
  the main skin, see Subsection \ref{subsec:breaksequence} from
  page \pageref{subsec:breaksequence}.
\end{itemize}


\subsection{Limitations and Known Bugs}
\begin{itemize}
\item  The maximal total height of the upper and of the lower part
  of normal breakable |tcolorbox|es is about 65536pt (ca.\,2300cm)
  apiece. If such a part gets longer, the output will get buggy
  without warning.
  For very oversized boxes which are longer than 65536pt, use
  the \docValue{unlimited} value for  \refKey{/tcb/breakable}.
  With the \docValue{unlimited} setting,
  the applied algorithm has (virtually) no height limit for boxes, but
  very likely the compiler memory will have to be increased for boxes longer
  than 300 pages (depending on compiler settings and box content).
  But it is recommended to use \docValue{unlimited} for critical large boxes only.
  %,since there \emph{may} be a single interline space deviation (lost glue) around
  %every 2300cm, e.\,g.\ a \refCom{tcbline*} \emph{may} get lost.
\item You can nest an unbreakable |tcolorbox| inside another |tcolorbox|,
  even inside a breakable one.
  But you cannot not nest a breakable box inside a breakable box.
  The \refKey{/tcb/breakable} key for a nested box is ignored
  automatically\footnote{Until |tcolorbox| 3.04, the \refKey{/tcb/breakable} key
  was not ignored for nested boxes.}, i.\,e.\ inner
  boxes are always unbreakable.\par
  After all, in the unlikely case you really want to have the nested box to be breakable,
  use \refKey{/tcb/enforce breakable} for the nested
  box\footnote{\refKey{/tcb/enforce breakable} acts like \refKey{/tcb/breakable} until |tcolorbox| 3.04.}.
  \textbf{But, a breakable box inside a breakable box will usually give a mess.}
\item If your text content contains some text color changing commands,
  your color will not survive the break to the next box.
  But, with the |fontspec| package and |xelatex| or |lualatex|,
  you can use
  |\addfontfeatures{Color=mycolor}|
  to add a font color which survives the break.
\item\tcbdocmarginnote{\tcbdocnew{2014-10-30}}
  The |perpage| option of the |footmisc| package is deliberately deactivated
  inside a breakable box since all footnotes are placed at the end
  of the box (possibly far away from the reference point).
\item\tcbdocmarginnote{\tcbdocnew{2016-02-15}}
  Making a box \refKey{/tcb/breakable} which actually is not broken creates
  a box which acts \emph{almost} like an unbreakable box. Visual differences
  are kept as indiscernible as possible, but can appear with certain
  \refKey{/tcb/before} and \refKey{/tcb/after} settings, especially, if there
  is an automatic page break before the box.
\item\tcbdocmarginnote{\tcbdocnew{2016-05-25}}
  Lua\TeX\ version 0.95 changes the behaviour of the basic |\vsplit| (a bug?!)
  resulting in badly broken boxes. Thanks to Jeremy Engel,
  the \mylib{breakable} library contains a patch for this which
  also loads the the |ifluatex| package.
\end{itemize}


\clearpage
\subsection{Main Option Keys}
\begin{docTcbKey}[][doc updated=2017-02-01]{breakable}{\colOpt{=true\textbar false\textbar unlimited}}{default |true|, initially |false|}
  Allows the |tcolorbox| to be breakable. If the box is larger than the
  available space at the current page, the box is automatically broken
  and continued to the next page. All sorts of |tcolorbox| can be made
  breakable. It depends on the skin how the breaking looks like.
  If you do not know better, use \refKey{/tcb/enhanced} for breaking a box.
  The parts of the \emph{break sequence} are numbered
  by the counter |tcbbreakpart|.
  \begin{itemize}
  \item\docValue{false}: Sets the |tcolorbox| to be unbreakable.
  \item\docValue{true}: Breaks the |tcolorbox| from one page to another.
    The maximal total height of the upper and of the lower part is
    about 65536pt (ca.\,2300cm or ca.\,90 pages) apiece.
  \item\docValue{unlimited}: Experimental code for unlimited total height of
    breakable boxes.
    %There \emph{may} be a single interline space deviation (lost glue) around every 2300cm.
    For boxes longer than 300 pages (or even shorter ones) the
    compiler memory will have to be increased.
  \end{itemize}

\begin{dispListing}
% \usepackage{lipsum}  % preamble
\tcbset{enhanced jigsaw,colback=red!5!white,colframe=red!75!black,
  watermark color=yellow!25!white,watermark text=\arabic{tcbbreakpart},
  fonttitle=\bfseries}

\begin{tcolorbox}[breakable,title=My breakable box]
\lipsum[1-6]
\end{tcolorbox}
\end{dispListing}
\end{docTcbKey}
{\tcbusetemp}


\begin{docTcbKey}{unbreakable}{}{no value, initially set}
  Sets the |tcolorbox| to be unbreakable.
\end{docTcbKey}


\begin{docTcbKey}{enforce breakable}{}{no value}
  A |tcolorbox| inside a |tcolorbox| is automatically set to be unbreakable.
  Using \refKey{/tcb/breakable} on such an inner box has no effect.
  If one \emph{really} wants the inner box to be breakable, use \refKey{/tcb/enforce breakable}.
  \textbf{This will usually give a mess of shattered boxes. You are advised to not use this option.}\\
  Note that \refKey{/tcb/enforce breakable} has the functionality
  that \refKey{/tcb/breakable} had until package version 3.04
  and exists for backward compatibility.
\end{docTcbKey}


\begin{docTcbKey}[][doc updated=2018-07-26]{title after break}{=\meta{text}}{no default, initially empty}
  The \refKey{/tcb/title} is used only for the \emph{first} part of a
  \emph{break sequence}. Use |title after break| to create a heading line
  with \meta{text} as content for all following parts.
  Also see \refKey{/tcb/extras title after break} for formatting the title text.
\end{docTcbKey}


\begin{docTcbKey}{notitle after break}{}{no value, initially set}
  Removes the title line or following parts in a  \emph{break sequence} if set before.
\end{docTcbKey}


\begin{docTcbKey}{adjusted title after break}{=\meta{text}}{style, no default, initially unset}
  Works like \refKey{/tcb/adjusted title} but applied to \refKey{/tcb/title after break}.
\end{docTcbKey}


\begin{docTcbKey}{lines before break}{=\meta{number}}{no default, initially |2|}
  Assures that the given \meta{number} of lines of the upper box part or
  the lower box part are placed before a break happens.
\end{docTcbKey}

\clearpage
\begin{docTcbKey}[][doc updated=2017-07-05]{break at}{=\meta{length}\colOpt{/\meta{length}/\ldots/\meta{length}}}{no default, initially |0pt|}
  Defines break points at the given \meta{length} values.
  The first \meta{length} defines the (maximal) height of the first partial box,
  the second \meta{length} defines the (maximal) height of the second partial box,
  and so on. The last \meta{length} value is applied to all following partial boxes if any.
  \begin{itemize}
  \item Setting a \meta{length} to |0pt| means that the naturally available
        space is used for breaking.
  \item Setting a \meta{length} to a negative value means that
        the sum of this negative value and the naturally available space is used
        for breaking (boxes will shrink in height).
        That that before version 4.10 negative values were treated like |0pt|.
  \end{itemize}
\begin{dispExample}
% \usepackage{multicol,lipsum}
\begin{multicols}{3}\footnotesize
Breakable boxes inside a |multicols| environment need special attendance.
They are broken by default at |\textheight|.
The |break at| option can be used to insert better break points by hand.
\begin{tcolorbox}[enhanced jigsaw,size=small,vfill before first,
  colframe=red,colback=yellow!10!white,before title=\raggedright,
  title={Broken box inside a |multicols| environment},fonttitle=\bfseries,
  enforce breakable,% use only breakable in the real world!
  pad at break=1mm,break at=3cm/6.3cm ]
\lipsum[1]
\end{tcolorbox}
\refKey{/tcb/height fixed for} may also be considered for |multicols| environments.
\end{multicols}
\end{dispExample}
\end{docTcbKey}

\enlargethispage*{1cm}

\begin{docTcbKey}{enlargepage}{=\meta{length}\colOpt{/\meta{length}/\ldots/\meta{length}}}{no default, initially |0pt|}
  Inserts a |\enlargethispage|\marg{length} to the pages of the break sequence,
  i.\,e.\ allows one to enlarge (or shrink) partial boxes. The first \meta{length} is applied
  to the first partial box, the second \meta{length} is applied
  to the second partial box, and so on. The last \meta{length} value is applied
  to all following partial boxes if any. Note that floating boxes will not be enlarged.
\begin{dispListing}
\begin{tcolorbox}[breakable,enlargepage=0mm/\baselineskip/2\baselineskip/0mm,...
\end{dispListing}
  The example code enlarged the second partial box by one line, the third
  partial box by two lines, and all following parts are not enlarged.
  \begin{marker}
  If an automated page break occures before the first partial box, the
  page enlargement is applied to the page before the first partial box \emph{and}
  again to the page of the first partial box. Insert a manual break to prevent this.\\
  In general, |enlargepage| should be used at the final stage of a document
  for fine-tuning only.
  \end{marker}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{enlargepage flexible}{=\meta{length}}{no default, initially |0pt|}
  This allows an automated page enlargement for up to \meta{length}.
  The algorithm can use this to avoid breaking a box, if there is anough room
  after enlargement. Also, the \emph{last} partial box of a break sequence
  may be enlarged to avoid further breaking.\\
  Note that this potential enlargement is \emph{additive} to settings of
  \refKey{/tcb/enlargepage}.
  But \refKey{/tcb/enlargepage flexible} overwrites settings of
  \refKey{/tcb/pad before break*} or \refKey{/tcb/pad at break*}.
\begin{dispListing}
% The following setting hinders orphan lines for the last partial box
\tcbset{enlargepage flexible=\baselineskip}
\end{dispListing}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2014-12-15]{compress page}{\colOpt{=\meta{option}}}{default |all|, initially |baselineskip|}
  This option controls the space management on the page which contains the
  unbroken box or the first part of a \emph{break sequence}.
  Feasible \meta{option} values are:
  \begin{itemize}
  \item\docValue{all} (default value):
    All shrinkable glue on the page is potentially used for the
    unbroken box or the first part of a \emph{break sequence}. Thus, all
    vertical spaces on the page will potentially be reduced to their
    minimal values.
  \item\docValue{baselineskip} (initial value):
    Shrinkable glue up to one |\baselineskip| on the page is potentially used for the
    unbroken box or the first part of a \emph{break sequence}.
  \item\docValue{none}:
    The break algorithm respects the target size of the given glue values
    on the page. This was the inital value before version |3.34|.
  \end{itemize}
  \begin{marker}
  Note that the box \emph{content} is not influenced by this option.
  \end{marker}
\end{docTcbKey}


\begin{docTcbKey}{shrink break goal}{=\meta{length}}{no default, initially |0pt|}
  This is an emergency parameter if the break algorithm produces unpleasant
  breaks.
  It shrinks the goal height of the current box part by \meta{length}
  which may result in smaller boxes. Never use negative values.
  \emph{Usually, this option will never be needed at all.}
\end{docTcbKey}


\clearpage
\subsection{Option Keys for the Break Appearance}

\begin{docTcbKey}{toprule at break}{=\meta{length}}{no default, initially \texttt{0.5mm}}
  Sets the line width of the top rule to \meta{length} \emph{if} the box is \refKey{/tcb/breakable}.
  In this case, it is applied to \emph{middle} and \emph{last} parts in a
  break sequence. Note that \refKey{/tcb/toprule} overwrites this value
  if used afterwards.
\end{docTcbKey}


\begin{docTcbKey}{bottomrule at break}{=\meta{length}}{no default, initially \texttt{0.5mm}}
  Sets the line width of the bottom rule to \meta{length} \emph{if} the box is \refKey{/tcb/breakable}.
  In this case, it is applied to \emph{first} and \emph{middle} parts in a
  break sequence. Note that \refKey{/tcb/bottomrule} overwrites this value
  if used afterwards.
\end{docTcbKey}


\begin{docTcbKey}{topsep at break}{=\meta{length}}{no default, initially \texttt{0mm}}
  Additional vertical space of \meta{length} which is added at the top of
  \emph{middle} and \emph{last} parts in a break sequence. In general,
  it is not advisable to change this value if these parts start with a rule or a title.
\end{docTcbKey}

\begin{docTcbKey}{bottomsep at break}{=\meta{length}}{no default, initially \texttt{0mm}}
  Additional vertical space of \meta{length} which is added at the bottom of
  \emph{first} and \emph{middle} parts in a break sequence.
  In general, it is not advisable to change this value if these parts end with a rule.
\end{docTcbKey}

\begin{docTcbKey}{pad before break}{=\meta{length}}{style, no default, initially \texttt{3.5mm}}
  Sets the total amount of vertical space after the text content and before the
  break point to \meta{length}. This style sets \refKey{/tcb/toprule at break} to |0pt|
  and changes \refKey{/tcb/topsep at break} as required.
  In general, it is not advisable to change this value if the
  \emph{middle} and \emph{last} parts in a break sequence start with a rule or a title.
\end{docTcbKey}

\begin{docTcbKey}{pad before break*}{=\meta{length}}{style, no default}
  Sets \refKey{/tcb/pad before break} to \meta{length} and
  \refKey{/tcb/enlargepage flexible} to an appropriate value such that
  empty closing frames are avoided.
\end{docTcbKey}

\begin{docTcbKey}{pad after break}{=\meta{length}}{style, no default, initially \texttt{3.5mm}}
  Sets the total amount of vertical space after the break point and before the
  text content to \meta{length}. This style sets \refKey{/tcb/bottomrule at break} to |0pt|
  and changes \refKey{/tcb/bottomsep at break} as required.
  In general, it is not advisable to change this value if the
  \emph{first} and \emph{middle} parts in a break sequence end with a rule.
\end{docTcbKey}

\begin{docTcbKey}{pad at break}{=\meta{length}}{style, no default, initially \texttt{3.5mm}}
  Abbreviation for setting \meta{length} to \refKey{/tcb/pad before break}
  and \refKey{/tcb/pad after break}.
\end{docTcbKey}

\enlargethispage*{5mm}

\begin{docTcbKey}{pad at break*}{=\meta{length}}{style, no default}
  Sets \refKey{/tcb/pad at break} to \meta{length} and
  \refKey{/tcb/enlargepage flexible} to an appropriate value such that
  empty closing frames are avoided.
\end{docTcbKey}

\begin{dispListing}
% \usepackage{lipsum}  % preamble
\tcbset{colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[enhanced jigsaw,breakable,pad at break*=0mm,
  title={For this box, the pad space at the break point is set to 0mm}]
  \lipsum[1-2]
\end{tcolorbox}
\end{dispListing}
{\tcbusetemp}


\begin{marker}
\refKey{/tcb/pad at break} or \refKey{/tcb/pad at break*}
should be used as very last option in an option list, because
they adapt other settings.
\end{marker}


\begin{marker}
Also see \refKey{/tcb/enlarge top at break by}
and \refKey{/tcb/enlarge bottom at break by}.
\end{marker}


\begin{docTcbKey}{height fixed for}{=\meta{part}}{no default, initially |none|}
  When certain amount of space is available for a partial box of a
  break sequence, the partial box typically is smaller than this space
  (depending on the box content). For given \meta{part}(s), the height can be
  set to all available space.
  \begin{itemize}
  \item\docValue{none}: Every partial |tcolorbox| is set with its natural height.
  \item\docValue{first}: The \emph{first} partial box is set to a height which matches the available space.
  \item\docValue{middle}: All \emph{middle} partial boxes are set to a height which matches the available space.
  \item\docValue{last}: The \emph{last} partial box is set to a height which matches
    the available space.
  \item\docValue{first and middle}: The \emph{first} and
    all \emph{middle} partial boxes are set to a height which matches the available space.
  \item\docValue{middle and last}: All \emph{middle} partial boxes and the \emph{last} partial box
    are set to a height which matches the available space.
  \item\docValue{all}: All partial boxes are set to a height which matches the available space.
  \end{itemize}
\begin{marker}
  If the box keeps unbroken, this option is not applied.
  See \refKey{/tcb/height} for setting a fixed height for unbroken boxes.
  See \refKey{/tcb/height fill} for giving unbroken boxes maximum height.
\end{marker}
\end{docTcbKey}


\begin{docTcbKey}{vfill before first}{\colOpt{=true\textbar false}}{default |true|, initially |false|}
  Inserts a |\vfill| at the begin of the \emph{first} partial box to move this
  partial box to the end of the current page. This may be used as an alternative
  to \refKey{/tcb/height fixed for}|=|\docValue{first} to get justified
  columns or pages. The |\vfill| is not inserted, if the box gets not
  actually broken.
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2017-03-20]{segmentation at break}{\colOpt{=true\textbar false}}{default |true|, initially |true|}
  If a breakable box contains an \emph{upper part} and a \emph{lower part} and
  the break happens at the \emph{segmentation} between both parts, then
  \begin{itemize}
  \item the segmenation line (or similar) is drawn as first element of the
    partial box containing the \emph{lower part}, if \refKey{/tcb/segmentation at break}
    is set to be |true|.
  \item the segmenation line (or similar) is not drawn at all, if
    \refKey{/tcb/segmentation at break} is set to be |false|.
    This may be preferable for skins like \refSkin{bicolor}, \refSkin{tile},
    or \refSkin{beamer}.
  \end{itemize}
\end{docTcbKey}


\clearpage
\subsection{Extra Options for Partial Boxes}\label{subsec:extras}


\begin{docTcbKey}[][doc new=2015-07-16]{extras}{=\marg{options}}{no default, initially unset}
  Adds |tcolorbox| \meta{options} to every box of a \emph{break sequence}
  after skin settings are done. This is quite late in box processing.
  Geometry and break settings should \emph{not be used} here, because they
  will either be ignored or have unexpected negative results. But it is possible
  to change most colors, skin effects, shadows, borders, frame code, etc.
  Note that using \refKey{/tcb/extras} for every box is very seldom an
  advantage over setting the options directly. Usually, \refKey{/tcb/extras first},
  \refKey{/tcb/extras middle}, etc.\ are sensible to apply.
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2015-07-16]{no extras}{}{style, no default, initially set}
  Removes all extras if set before.
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2015-07-16]{extras broken}{=\marg{options}}{no default, initially unset}
  If the box is set to be \refKey{/tcb/breakable} and \emph{is} broken actually,
  then the \meta{options} are added to every box of the \emph{break sequence}.
  \refKey{/tcb/extras} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-07-16]{extras unbroken}{=\marg{options}}{no default, initially unset}
  If the box is set to be \refKey{/tcb/breakable} but \emph{is not} broken actually
  or if the box is set to be \refKey{/tcb/unbreakable},
  then the \meta{options} are added to the box.
  \refKey{/tcb/extras} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-07-16]{no extras unbroken}{}{style, no default, initially set}
  Removes the unbroken extras if set before.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-07-16]{extras first}{=\marg{options}}{no default, initially unset}
  If the box is set to be \refKey{/tcb/breakable} and \emph{is} broken actually,
  then the \meta{options} are added to the \emph{first} box of the break sequence.
  \refKey{/tcb/extras} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-07-16]{no extras first}{}{style, no default, initially set}
  Removes the first extras if set before.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-07-16]{extras middle}{=\marg{options}}{no default, initially unset}
  If the box is set to be \refKey{/tcb/breakable} and \emph{is} broken actually,
  then the \meta{options} are added to every \emph{middle} box (if any) of the break sequence.
  \refKey{/tcb/extras} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-07-16]{no extras middle}{}{style, no default, initially set}
  Removes the middle extras if set before.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-07-16]{extras last}{=\marg{options}}{no default, initially unset}
  If the box is set to be \refKey{/tcb/breakable} and \emph{is} broken actually,
  then the \meta{options} are added to the \emph{last} box of the break sequence.
  \refKey{/tcb/extras} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-07-16]{no extras last}{}{style, no default, initially set}
  Removes the last extras if set before.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-07-16]{extras unbroken and first}{=\marg{options}}{no default, initially unset}
  This is an abbreviation for setting
  \refKey{/tcb/extras unbroken} and
  \refKey{/tcb/extras first} together.
  \refKey{/tcb/extras} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-07-16]{extras middle and last}{=\marg{options}}{no default, initially unset}
  This is an abbreviation for setting
  \refKey{/tcb/extras middle} and
  \refKey{/tcb/extras last} together.
  \refKey{/tcb/extras} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-07-16]{extras unbroken and last}{=\marg{options}}{no default, initially unset}
  This is an abbreviation for setting
  \refKey{/tcb/extras unbroken} and
  \refKey{/tcb/extras last} together.
  \refKey{/tcb/extras} overwrites this key.
\end{docTcbKey}

\clearpage

\begin{docTcbKey}[][doc new=2015-07-16]{extras first and middle}{=\marg{options}}{no default, initially unset}
  This is an abbreviation for setting
  \refKey{/tcb/extras first} and
  \refKey{/tcb/extras middle} together.
  \refKey{/tcb/extras} overwrites this key.
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2018-07-26]{extras title after break}{=\marg{options}}{no default, initially unset}
  If the box has a \refKey{/tcb/title after break}, then the \meta{options}
  are added for all titles after the first break, i.e.\ all middle and last.
  The color, font, and alignment of titles after break can be adapted choosing
  \meta{options}, e.g.\ by \refKey{/tcb/coltitle}, \refKey{/tcb/fonttitle},
  \refKey{/tcb/halign title}.
  Note that \refKey{/tcb/colbacktitle} has to be placed into
  \refKey{/tcb/extras middle and last}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2018-07-26]{no extras title after break}{}{style, no default, initially set}
  Removes the title after break extras if set before.
\end{docTcbKey}

\bigskip

\begin{exdispExample}{extras}
% \usepackage{lipsum,multicol}
% \usetikzlibrary{decorations.pathmorphing}
% \tcbuselibrary{skins}
\newtcolorbox{mybox}[1][]{
  tile,
  colback=green!7,coltitle=blue!50!black,colbacktitle=blue!5,
  center title,
  toprule=1.25mm,bottomrule=1.25mm,
  extras unbroken and first={
    borderline north={0.25mm}{0.5mm}{blue,decoration={zigzag,amplitude=0.5mm},decorate}},
  extras unbroken and last={
    borderline south={0.25mm}{0.5mm}{blue,decoration={zigzag,amplitude=0.5mm},decorate}},
  #1
}

\begin{mybox}[title=My unbroken box]
\lipsum[1]
\end{mybox}

\begin{multicols}{3}
  \begin{mybox}[title=My broken box,
    enforce breakable,% use only breakable in the real world!
    break at=4.2cm,pad at break=2mm,
    height fixed for=first and middle,  ]
  \lipsum[2]
  \end{mybox}
\end{multicols}
\end{exdispExample}




\clearpage
\subsection{Breakable boxes and the \texttt{multicol} package}\label{subsec:multicol}
\begin{marker}
With version 4.10, the algorithm for detecting the available height
for a |tcolorbox| inside a |multicol| environment was improved with help
of Frank Mittelbach. This change \emph{may} impact existing user
code which \emph{may} have to be adapted.
\end{marker}

\begin{multicols}{2}
\begin{tcolorbox}[enhanced jigsaw,size=small,breakable,colback=yellow!10!white,
  colframe=red!50!white,break at=3cm,height fixed for=all]
Unbreakable |tcolorbox|es can be used without special care inside a
|multicols| environment from the |multicol| package \cite{mittelbach:multicol}.

Since version 3.10, a breakable |tcolorbox| detects, if it is used inside
a |multicols| environment. But choosing break points for a breakable box
cannot be done by the balancing routine of |multicols|. By default, boxes
will break at maximum column height. To get pleasant results, use the
\refKey{/tcb/break at} and \refKey{/tcb/height fixed for} options.
\end{tcolorbox}
\end{multicols}

\enlargethispage{\baselineskip}
\begin{dispListing}
% \usepackage{lipsum,multicol}  % preamble
\footnotesize
\begin{multicols}{2}
  \lipsum[1]
  \begin{tcolorbox}[enhanced jigsaw,breakable,size=title,
    colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries,
    title=My breakable box,pad at break=1mm, break at=-\baselineskip/0pt ]
  \lipsum[2-4]
  \end{tcolorbox}
  \lipsum[4]
\end{multicols}
\end{dispListing}
{\tcbusetemp}

\clearpage

\begin{multicols}{2}
\small
This example is already set inside a |multicols| environment.
This time, a \emph{middle} part has full column height (here |\textheight|).
\refKey{/tcb/height fixed for} is used to spread this box part over the full
height to align with neighboring columns.
\begin{dispListing}
% \usepackage{lipsum,multicol}
\lipsum[1]
\begin{tcolorbox}[enhanced jigsaw,
  breakable,
  size=title,
  colback=red!5!white,
  colframe=red!75!black,
  fonttitle=\bfseries,
  title=My breakable box,
  pad at break=2mm,
  break at=-\baselineskip/0pt,
  height fixed for=middle ]
\lipsum[2-7]
\end{tcolorbox}
\lipsum[8]
\end{dispListing}
{\tcbusetemp}
\end{multicols}


The following example has a |\tcolorbox| which fills the |\multicols|
environment completely. Here, \refKey{/tcb/height fixed for} is used
to give all three columns the full height.
Note that the appropriate \refKey{/tcb/break at} value is not computed
automatically but set manually.

\begin{dispListing}
% \usepackage{lipsum,multicol}  % preamble
\small
\begin{multicols}{3}
  \begin{tcolorbox}[enhanced jigsaw,breakable,size=small,
    colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries,
    title=My breakable box,pad at break=2mm,drop fuzzy shadow,
    height fixed for=all, break at=11.4cm ]
  \lipsum[1-3]
  \end{tcolorbox}
\end{multicols}
\end{dispListing}
{\tcbusetemp}

\clearpage
\subsection{Break Point Insertion}\label{subsec:breakpoints}

\begin{docCommand}[doc new=2017-07-05]{tcbbreak}{}
  A \emph{breakable} box is not broken, if there is enough
  space on the current page or column.
  Therefore, typical penalty insertion with
  |\break|, |\pagebreak|, |\columnbreak|, \ldots \emph{may} only work as
  expected, if the box is broken at least into two parts
  \emph{without} inserting the penalties.\par\smallskip
  To \emph{force} a page or column break, \refCom{tcbbreak}
  starts a new paragraph and inserts an insane tall rule which causes a
  break and which is immediately discarded. You may ignore this technical
  information and just use it as you would use |\pagebreak|.\par\smallskip
  For an \emph{unbreakable box}, \refCom{tcbbreak} is identical to insert |\par|,
  i.e.\ it just starts a new paragraph.\par\smallskip
  Also see \refKey{/tcb/break at} for defining height dependend breaks.

\begin{dispListing}
% \usepackage{lipsum,multicol}  % preamble
\begin{multicols}{3}
  \begin{tcolorbox}[breakable,enhanced jigsaw,size=small,
    colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries,
    title=Break into parts
  ]
  First part\tcbbreak
  Second part\tcbbreak
  Third part
  \end{tcolorbox}
\end{multicols}

\begin{multicols}{3}
  \begin{tcolorbox}[enhanced jigsaw,size=small,
    colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries,
    title=You shall not break
  ]
  First part\tcbbreak
  Second part\tcbbreak
  Third part
  \end{tcolorbox}
\end{multicols}

\end{dispListing}
{\tcbusetemp}

\end{docCommand}



\clearpage
\subsection{Break Sequence for the Skins}\label{subsec:breaksequence}
The following diagrams document the \emph{break sequence} for different
skins. Depending on the main skin of a |tcolorbox|, the actual skins of
the \emph{break sequence} parts are displayed.

\def\tcbbreakskininto#1#2#3#4#5{%
\begin{center}\begin{tikzpicture}
\tcbset{width=7cm,colframe=Navy,colback=AliceBlue,fonttitle=\bfseries,
  watermark color=AliceBlue!85!Navy,#5
  }
\node[above] (unbroken) at (0,0) {\begin{tcolorbox}[title=Unbroken Box,skin=#1,watermark text=unbroken,height=3.8cm]
\texttt{skin=#1}
\end{tcolorbox}};
\node[above] (first) at (8.7,2.4) {\begin{tcolorbox}[title=Broken Boxes,skin=#2,watermark text=first,height=1.4cm]
\texttt{skin=#2}
\end{tcolorbox}};
\node[above] (middle) at (8.7,1.2) {\begin{tcolorbox}[skin=#3,watermark text=middle,height=1cm]
\texttt{skin=#3}
\end{tcolorbox}};
\node[above] (last) at (8.7,0) {\begin{tcolorbox}[skin=#4,watermark text=last,height=1cm]
\texttt{skin=#4}
\end{tcolorbox}};
\path[draw=FireBrick,line width=2pt,->] (unbroken) edge (first.west) edge (middle.west) edge (last.west);
\end{tikzpicture}\end{center}}

\tcbbreakskininto{standard}{standard}{standard}{standard}{watermark text/.style={}}
\tcbbreakskininto{standard jigsaw}{standard jigsaw}{standard jigsaw}{standard jigsaw}{watermark text/.style={}}
\tcbbreakskininto{spartan}{spartan}{spartan}{spartan}{}
\clearpage
\tcbbreakskininto{enhanced}{enhancedfirst}{enhancedmiddle}{enhancedlast}{}
\tcbbreakskininto{enhancedfirst}{enhancedfirst}{enhancedmiddle}{enhancedmiddle}{}
\tcbbreakskininto{enhancedmiddle}{enhancedmiddle}{enhancedmiddle}{enhancedmiddle}{}
\tcbbreakskininto{enhancedlast}{enhancedmiddle}{enhancedmiddle}{enhancedlast}{}
\clearpage
\tcbbreakskininto{enhanced jigsaw}{enhancedfirst jigsaw}{enhancedmiddle jigsaw}{enhancedlast jigsaw}{}
\tcbbreakskininto{enhancedfirst jigsaw}{enhancedfirst jigsaw}{enhancedmiddle jigsaw}{enhancedmiddle jigsaw}{}
\tcbbreakskininto{enhancedmiddle jigsaw}{enhancedmiddle jigsaw}{enhancedmiddle jigsaw}{enhancedmiddle jigsaw}{}
\tcbbreakskininto{enhancedlast jigsaw}{enhancedmiddle jigsaw}{enhancedmiddle jigsaw}{enhancedlast jigsaw}{}
\clearpage
{\tcbset{borderline={2pt}{0pt}{black!10!white}}%
\tcbbreakskininto{empty}{emptyfirst}{emptymiddle}{emptylast}{}
\tcbbreakskininto{emptyfirst}{emptyfirst}{emptymiddle}{emptymiddle}{}
\tcbbreakskininto{emptymiddle}{emptymiddle}{emptymiddle}{emptymiddle}{}
\tcbbreakskininto{emptylast}{emptymiddle}{emptymiddle}{emptylast}{}
}
\clearpage
\tcbbreakskininto{bicolor}{bicolorfirst}{bicolormiddle}{bicolorlast}{bicolor}
\tcbbreakskininto{bicolorfirst}{bicolorfirst}{bicolormiddle}{bicolormiddle}{bicolor}
\tcbbreakskininto{bicolormiddle}{bicolormiddle}{bicolormiddle}{bicolormiddle}{bicolor}
\tcbbreakskininto{bicolorlast}{bicolormiddle}{bicolormiddle}{bicolorlast}{bicolor}
\clearpage
\tcbbreakskininto{tile}{tilefirst}{tilemiddle}{tilelast}{tile,colbacktitle=Navy}
\tcbbreakskininto{tilefirst}{tilefirst}{tilemiddle}{tilemiddle}{tile,colbacktitle=Navy}
\tcbbreakskininto{tilemiddle}{tilemiddle}{tilemiddle}{tilemiddle}{tile,colbacktitle=Navy}
\tcbbreakskininto{tilelast}{tilemiddle}{tilemiddle}{tilelast}{tile,colbacktitle=Navy}
\clearpage
\tcbbreakskininto{beamer}{beamerfirst}{beamermiddle}{beamerlast}{beamer}
\tcbbreakskininto{beamerfirst}{beamerfirst}{beamermiddle}{beamermiddle}{beamer}
\tcbbreakskininto{beamermiddle}{beamermiddle}{beamermiddle}{beamermiddle}{beamer}
\tcbbreakskininto{beamerlast}{beamermiddle}{beamermiddle}{beamerlast}{beamer}
\clearpage
\tcbbreakskininto{widget}{widgetfirst}{widgetmiddle}{widgetlast}{widget}
\tcbbreakskininto{widgetfirst}{widgetfirst}{widgetmiddle}{widgetmiddle}{widget}
\tcbbreakskininto{widgetmiddle}{widgetmiddle}{widgetmiddle}{widgetmiddle}{widget}
\tcbbreakskininto{widgetlast}{widgetmiddle}{widgetmiddle}{widgetlast}{widget}
\tcbbreakskininto{draft}{draft}{draft}{draft}{draft}
\clearpage
\tcbbreakskininto{freelance}{freelancefirst}{freelancemiddle}{freelancelast}{}
\tcbbreakskininto{freelancefirst}{freelancefirst}{freelancemiddle}{freelancemiddle}{}
\tcbbreakskininto{freelancemiddle}{freelancemiddle}{freelancemiddle}{freelancemiddle}{}
\tcbbreakskininto{freelancelast}{freelancemiddle}{freelancemiddle}{freelancelast}{}




\clearpage
\subsection{Break by Hand (Faked Break)}

\begin{marker}
See \Vref{subsec:multicol} for \emph{real} column breaks.
\end{marker}

Since the appearance of broken boxes is done by skins, it is quite easy
to 'fake a break'. For this, you actually don't need the
\mylib{breakable} library at
all.

\begin{dispExample}
\tcbset{enhanced,equal height group=fakedbreak,
  colback=LightGreen,colframe=DarkGreen,
  width=(\linewidth-6mm)/3,nobeforeafter,
  left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm}
%
\begin{tcolorbox}[title=My broken box,skin=enhancedfirst]
This is a box which breaks from one column to another
\end{tcolorbox}\hfill
\begin{tcolorbox}[skin=enhancedmiddle]
column. I am sorry to say that this is a trick.
Nevertheless, you may use this trick for your
\end{tcolorbox}\hfill
\begin{tcolorbox}[skin=enhancedlast]
own purposes.
\end{tcolorbox}
\end{dispExample}




==> tcolorbox.doc.coremacros.tex <==
% !TeX root = tcolorbox.tex
% include file of tcolorbox.tex (manual of the LaTeX package tcolorbox)
\clearpage
\section{Macros for Box Creation}%
\tcbset{external/prefix=external/coremacros_}%
\begin{docEnvironment}{tcolorbox}{\oarg{options}}
  This is the main environment to create an accentuated colored text box with
  rounded corners and, optionally, two parts. The appearance of this box
  is controlled by numerous options.
  In the most simple case the source code

\begin{dispListing}
\begin{tcolorbox}
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{dispListing}

creates the following compiled text box:
\begin{tcolorbox}
This is a \textbf{tcolorbox}.
\end{tcolorbox}

The text content of the box can be divided
in an upper and a lower part
by the command \refCom{tcblower}. Visually, both parts are separated by a line.
For example:

\begin{dispListing}
\begin{tcolorbox}
This is another \textbf{tcolorbox}.
\tcblower
Here, you see the lower part of the box.
\end{tcolorbox}
\end{dispListing}

This code gives the following box:
\begin{tcolorbox}
This is another \textbf{tcolorbox}.
\tcblower
Here, you see the lower part of the box.
\end{tcolorbox}

The \meta{options} control the appearance and several functions of the boxes,
see \Vref{sec:optkeys} for the complete list.
A quick example is given here:

\begin{dispExample}
\begin{tcolorbox}[colback=red!5!white,colframe=red!75!black,title=My nice heading]
This is another \textbf{tcolorbox}.
\tcblower
Here, you see the lower part of the box.
\end{tcolorbox}
\end{dispExample}
\end{docEnvironment}


\begin{docCommand}{tcblower}{}
  Used inside \refEnv{tcolorbox} to separate the upper box part from
  the optional lower box part. The upper and the lower part are treated
  as separate functional units. If you only want to draw a line, see
  \refCom{tcbline}.
\end{docCommand}


\clearpage
\begin{docCommand}{tcbset}{\marg{options}}
  Sets options for every following \refEnv{tcolorbox} inside the current \TeX\ group.
  By default, this does not apply to nested boxes, see \Vref{subsec:everybox}.\par
  For example, the colors of the boxes may be defined for the whole document by this:
\begin{dispListing}
\tcbset{colback=red!5!white,colframe=red!75!black}
\end{dispListing}
\end{docCommand}


\begin{docCommand}{tcbsetforeverylayer}{\marg{options}}
  Sets options for every following \refEnv{tcolorbox} inside the current \TeX\ group.
  In contrast to \refCom{tcbset}, this does also
  apply to nested boxes, see \Vref{subsec:everybox}.
  Technically, the \meta{options} are appended to the default values for every
  tcolorbox which are applied by \refKey{/tcb/reset}.\par
  You should not use this macro, if you are not completely sure that you
  want to have the \meta{options} also for boxes in boxes (in boxes in boxes \ldots).
\begin{dispExample}
\tcbset{colback=green!10!white}
\tcbsetforeverylayer{colframe=red!75!black}

\begin{tcolorbox}[title=All options for this box]
  This is a tcolorbox.\par\medskip
  \begin{tcolorbox}[title=Nested box]
    Note that this nested box has a red frame but no green background.
  \end{tcolorbox}
\end{tcolorbox}
\bigskip

\begin{tcolorbox}[reset]
  Options given with |\tcbsetforeverylayer| survive a |reset|.
\end{tcolorbox}
\end{dispExample}
\end{docCommand}


\clearpage
\begin{docCommand}{tcbox}{\oarg{options}\marg{box content}}
  Creates a colored box which is fitted to the width of the given
  \meta{box content}. In principle, most \meta{options} for a \refEnv{tcolorbox}
  can be used for |\tcbox| with some restrictions. A |\tcbox| cannot have
  a lower part and cannot be broken.

\begin{dispExample}
\tcbset{colframe=blue!50!black,colback=white,colupper=red!50!black,
        fonttitle=\bfseries,nobeforeafter,center title}

Text \tcbox[tcbox raise base]{Hello World}\hfill
%
\tcbox[left=0mm,right=0mm,top=0mm,bottom=0mm,boxsep=0mm,
  toptitle=0.5mm,bottomtitle=0.5mm,title=My table]{%
  \arrayrulecolor{blue!50!black}\renewcommand{\arraystretch}{1.2}%
  \begin{tabular}{r|c|l}
  One   & Two    & Three \\\hline\hline
  Men   & Mice   & Lions \\\hline
  Upper & Middle & Lower
  \end{tabular}}\hfill
%
\tcbox[colback=blue!85!black,
  left=0mm,right=0mm,top=0mm,bottom=0mm,boxsep=1mm,arc=0mm,boxrule=0.5pt,
  title=My picture]{%
  \includegraphics[width=5cm]{Basilica_5.png}}
\end{dispExample}

\begin{dispExample}
% \usepackage{tikz}
\tcbset{colframe=blue!50!black,colback=white,colupper=red!50!black,
        fonttitle=\bfseries,center title}

% Fixed width box
\begin{tcolorbox}Hello\\World!\end{tcolorbox}

% Fitted width box (like hbox or makebox)
\tcbox{Hello\\World!}

% Fitted width box (using a \tikzname\  node)
\tcbox[tikznode]{Hello\\World!}
\end{dispExample}

\end{docCommand}

\clearpage
\begin{marker}
See \Vref{subsec:xparse_tcolorbox} and \Vref{subsec:xparse_tcbox} for more
elaborate methods to create new environments and commands.
\end{marker}

\begin{docCommand}{newtcolorbox}{\oarg{init options}\marg{name}\oarg{number}\oarg{default}\marg{options}}
  Creates a new environment \meta{name} based on \refEnv{tcolorbox}.
  Basically, |\newtcolorbox| operates like |\newenvironment|. This means,
  the new environment \meta{name} optionally takes \meta{number} arguments, where
  \meta{default} is the default value for the optional first argument.
  The \meta{options} are given to the underlying |tcolorbox|.
  Note that \refKey{/tcb/savedelimiter} is set to the given \meta{name}
  automatically.
  The \meta{init options} allow setting up automatic numbering,
  see Section \ref{sec:initkeys} from page \pageref{sec:initkeys}.
\begin{dispExample*}{sbs,lefthand ratio=0.6}
\newtcolorbox{mybox}{colback=red!5!white,
  colframe=red!75!black}

\begin{mybox}
This is my own box.
\end{mybox}
\end{dispExample*}

\begin{dispExample*}{sbs,lefthand ratio=0.6}
\newtcolorbox{mybox}[1]{colback=red!5!white,
  colframe=red!75!black,fonttitle=\bfseries,
  title=#1}

\begin{mybox}{Hello there}
This is my own box with a mandatory title.
\end{mybox}
\end{dispExample*}

\begin{dispExample*}{sbs,lefthand ratio=0.6}
\newtcolorbox{mybox}[2][]{colback=red!5!white,
  colframe=red!75!black,fonttitle=\bfseries,
  colbacktitle=red!85!black,enhanced,
attach boxed title to top center={yshift=-2mm},
  title=#2,#1}

\begin{mybox}[colback=yellow]{Hello there}
This is my own box with a mandatory title
and options.
\end{mybox}
\end{dispExample*}

\inputpreamblelisting{A}

\begin{dispExample*}{sbs,lefthand ratio=0.6}
\begin{pabox}[colback=yellow]{Hello there}
This is my own box with a mandatory
numbered title and options.
\end{pabox}
\end{dispExample*}
\end{docCommand}


\begin{docCommand}{renewtcolorbox}{\oarg{init options}\marg{name}\oarg{number}\oarg{default}\marg{options}}
  Operates like \refCom{newtcolorbox}, but based on |\renewenvironment| instead of |\newenvironment|.
  An existing environment is redefined.
\end{docCommand}


\clearpage
\begin{docCommand}{newtcbox}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\oarg{number}\oarg{default}\marg{options}}
  Creates a new macro \texttt{\textbackslash}\meta{name} based on \refCom{tcbox}.
  Basically, |\newtcbox| operates like |\newcommand|.
  The new macro \texttt{\textbackslash}\meta{name} optionally takes \meta{number}$+1$ arguments, where
  \meta{default} is the default value for the optional first argument.
  The \meta{options} are given to the underlying |tcbox|.
  The \meta{init options} allow setting up automatic numbering,
  see Section \ref{sec:initkeys} from page \pageref{sec:initkeys}.
\begin{dispExample*}{sbs,lefthand ratio=0.6}
\newtcbox{\mybox}{colback=red!5!white,
  colframe=red!75!black}

\mybox{This is my own box.}
\end{dispExample*}

\begin{dispExample*}{sbs,lefthand ratio=0.6}
\newtcbox{\mybox}[1]{colback=red!5!white,
  colframe=red!75!black,fonttitle=\bfseries,
  title=#1}

\mybox{Hello there}{This is my own box.}
\end{dispExample*}

\begin{dispExample*}{sbs,lefthand ratio=0.6}
\newtcbox{\mybox}[2][]{colback=red!5!white,
  colframe=red!75!black,fonttitle=\bfseries,
  title=#2,#1}

\mybox[colback=yellow]{Hello there}%
  {This is my own box.}
\end{dispExample*}

\inputpreamblelisting{B}

\begin{dispExample*}{sbs,lefthand ratio=0.6}
\pbbox[colback=yellow]{Hello there}%
  {This is my own box.}
\end{dispExample*}

\begin{dispExample}
\newtcbox{\mybox}[1][red]{on line,
  arc=0pt,outer arc=0pt,colback=#1!10!white,colframe=#1!50!black,
  boxsep=0pt,left=1pt,right=1pt,top=2pt,bottom=2pt,
  boxrule=0pt,bottomrule=1pt,toprule=1pt}
\newtcbox{\xmybox}[1][red]{on line,
  arc=7pt,colback=#1!10!white,colframe=#1!50!black,
  before upper={\rule[-3pt]{0pt}{10pt}},boxrule=1pt,
  boxsep=0pt,left=6pt,right=6pt,top=2pt,bottom=2pt}

The \mybox[green]{quick} brown \mybox{fox} \mybox[blue]{jumps} over the
\mybox[green]{lazy} \mybox{dog}.\par
The \xmybox[green]{quick} brown \xmybox{fox} \xmybox[blue]{jumps} over the
\xmybox[green]{lazy} \xmybox{dog}.
\end{dispExample}

\end{docCommand}


\enlargethispage*{1cm}
\begin{docCommand}{renewtcbox}{\oarg{init options}\brackets{\texttt{\textbackslash}\rmfamily\meta{name}}\oarg{number}\oarg{default}\marg{options}}
  Operates like \refCom{newtcbox}, but based on |\renewcommand| instead of |\newcommand|.
  An existing macro is redefined.
\end{docCommand}

\clearpage

\begin{docCommand}[doc new=2014-10-20]{tcolorboxenvironment}{\marg{name}\marg{options}}
  An existing environment \meta{name} is redefined to be boxed inside a
  |tcolorbox| with the given \meta{options}.
\begin{dispExample*}{sbs,lefthand ratio=0.6}
% tcbuselibrary{skins}
\newenvironment{myitemize}{%
  \begin{itemize}}{\end{itemize}}

\tcolorboxenvironment{myitemize}{blanker,
  before skip=6pt,after skip=6pt,
  borderline west={3mm}{0pt}{red}}

Some text.
\begin{myitemize}
\item Alpha
\item Beta
\item Gamma
\end{myitemize}
More text.
\end{dispExample*}

\medskip
See further examples in \Vref{subsec:theorems_other}.
\end{docCommand}



==> tcolorbox.doc.coreoptions.tex <==
% !TeX root = tcolorbox.tex
% include file of tcolorbox.tex (manual of the LaTeX package tcolorbox)
\clearpage
\section{Option Keys}\label{sec:optkeys}%
\tcbset{external/prefix=external/coreoptions_}%
For the \meta{options} in \refEnv{tcolorbox} respectively \refCom{tcbset}
the following |pgf| keys can be applied. The key tree path |/tcb/| is not to
be used inside these macros. It is easy to add your own style keys using
the syntax for |pgf| keys, see \cite{tantau:tikz_and_pgf,sturm:latex} or the examples
starting from page~\pageref{sec:latextutorial}.


\subsection{Title}
\begin{docTcbKey}{title}{=\meta{text}}{no default, initially empty}
  Creates a heading line with \meta{text} as content.
\begin{exdispExample*}{title}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[title=My heading line]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\begin{docTcbKey}{notitle}{}{no value, initially set}
  Removes the title line if set before.
\end{docTcbKey}


\begin{docTcbKey}{adjusted title}{=\meta{text}}{style, no default, initially unset}
  Creates a heading line with \meta{text} as content. The minimal height of
  this line is adjusted to fit the text given by \refKey{/tcb/adjust text}.
  This option makes sense
  for single line headings if boxes are set side by side with equal height.
  Note that it is very easy to trick this adjustment.
\begin{exdispExample}[runs=2]{adjusted_title}
\tcbset{colback=White,arc=0mm,width=(\linewidth-4pt)/4,
equal height group=AT,before=,after=\hfill,fonttitle=\bfseries}

The following titles are not adjusted:\\
\foreach \n in {xxx,ggg,AAA,\"Agypten}
{\begin{tcolorbox}[title=\n,colframe=red!75!black]
  Some content.\end{tcolorbox}}
Now, we try again with adjusted titles:\\
\foreach \n in {xxx,ggg,AAA,\"Agypten}
{\begin{tcolorbox}[adjusted title=\n,colframe=blue!75!black]
  Some content.\end{tcolorbox}}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}{adjust text}{=\meta{text}}{no default, initially \texttt{\"Apgjy}}
  This sets the reference text for \refKey{/tcb/adjusted title}. If your texts
  never exceed '\"Apgjy' in depth and height you don't need to care about this option.
\end{docTcbKey}

\clearpage

\begin{docTcbKey}[][doc new=2014-11-24]{squeezed title}{=\meta{text}}{style, no default, initially unset}
  Creates a single heading line with \meta{text} as content.
  If the \meta{text} is longer than the available space, the text is
  squeezed to fit into the available space.
\begin{exdispExample}{squeezed_title}
% \tcbuselibrary{raster}
\begin{tcbitemize}[raster columns=3,raster equal height,
  colframe=red!75!black,colback=red!5!white,fonttitle=\bfseries]
\tcbitem[squeezed title={Short title}]
  First box
\tcbitem[squeezed title={This is a very very long title}]
  Second box
\tcbitem[squeezed title={This title is clearly to long for this application}]
  Third box
\end{tcbitemize}
\end{exdispExample}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-11-24]{squeezed title*}{=\meta{text}}{style, no default, initially unset}
  This is a combination of \refKey{/tcb/adjusted title} and  \refKey{/tcb/squeezed title}.
\begin{exdispExample}{squeezed_title_2}
% \tcbuselibrary{raster}
\begin{tcbitemize}[raster columns=3,raster equal height,
  colframe=red!75!black,colback=red!5!white,fonttitle=\bfseries]
\tcbitem[squeezed title*={Short title}]
  First box
\tcbitem[squeezed title*={This is a very very long title}]
  Second box
\tcbitem[squeezed title*={This title is clearly to long for this application}]
  Third box
\end{tcbitemize}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2019-03-01]{titlebox}{=\meta{mode}}{no default, initially \texttt{visible}}
  Controls the treatment of the title part of the box.
  Feasible values for \meta{mode} are:
  \begin{itemize}
  \item\docValue{visible}: usual type setting of the title box,
  \item\docValue{invisible}: empty space instead of the title contents.
  \end{itemize}
\begin{exdispExample}{titlebox}
\begin{tcolorbox}[title=My invisible title,
  titlebox=invisible]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}



\clearpage
\begin{docTcbKey}{detach title}{}{no value}
Detaches the title from its normal position. The text of the title is
stored into \docAuxCommand{tcbtitletext} and the formatted title is
available by \docAuxCommand{tcbtitle}.
The main application is to move the title from its usual place to another one.
\begin{exdispExample}{detach_title}
\newtcolorbox{mybox}[2][]{colbacktitle=red!10!white,
  colback=blue!10!white,coltitle=red!70!black,
  title={#2},fonttitle=\bfseries,#1}

\begin{mybox}{My title}
  This is a \textbf{tcolorbox}.
\end{mybox}
\begin{mybox}[detach title,before upper={\tcbtitle\quad}]{My title}
  This is a \textbf{tcolorbox}.
\end{mybox}
\begin{mybox}[detach title,after upper={\par\hfill\tcbtitle}]{My title}
  This is a \textbf{tcolorbox}.
\end{mybox}
\end{exdispExample}
\end{docTcbKey}

\begin{docTcbKey}{attach title}{}{no value}
Attaches the title to its normal position. This option is used to reverse
\refKey{/tcb/detach title}.
\end{docTcbKey}


\begin{docTcbKey}[][doc updated=2015-07-08]{attach title to upper}{\colOpt{=\meta{text}}}{style, default empty, initially unset}
Attaches the title to the begin of the upper part of the box content.
The optional \meta{text} is set between the formatted title and the box content.
\begin{exdispExample}{attach_title_to_upper}
\newtcolorbox{mybox}[2][]{colbacktitle=red!10!white,
  colback=blue!10!white,coltitle=red!70!black,
  title={#2},fonttitle=\bfseries,#1}

\begin{mybox}[attach title to upper={\ ---\ }]{My title}
  This is a \textbf{tcolorbox}.
\end{mybox}
\begin{mybox}[attach title to upper,after title={:\ }]{My title}
  This is a \textbf{tcolorbox}.
\end{mybox}
\end{exdispExample}
\end{docTcbKey}


\bigskip
\begin{marker}
More title options are documented in \Vref{subsec:contentadditions}
and \Vref{subsec:skinboxedtitle}.
\end{marker}



\clearpage
\subsection{Subtitle}

Inside the box content, one or more subtitles can be added.
In general, a subtitle is a further \refEnv{tcolorbox} which inherits some
color and geometry options from the enclosing box. It may be customized
just like any other \refEnv{tcolorbox}.

\begin{docCommand}[doc new=2014-10-10]{tcbsubtitle}{\oarg{options}\marg{text}}
  Used inside a \refEnv{tcolorbox} to add a subtitle box with the given \meta{text}.
  This is an independent \refEnv{tcolorbox} which is formatted by several
  inherited properties of the enclosing box, by further settings from
  \refKey{/tcb/subtitle style}, and by the given \meta{options}.
\begin{exdispExample*}{tcbsubtitle_1}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[title=My title,
    colback=red!5!white,
    colframe=red!75!black,
    fonttitle=\bfseries]
  This is a \textbf{tcolorbox}.
\tcbsubtitle[before skip=\baselineskip]%
  {My subtitle}
  Further text.
\end{tcolorbox}
\end{exdispExample*}
\begin{exdispExample*}{tcbsubtitle_2}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[title=My title,
    colback=red!5!white,
    colframe=red!75!black,
    colbacktitle=yellow!50!red,
    coltitle=red!25!black,
    fonttitle=\bfseries]
  This is a \textbf{tcolorbox}.
\tcbsubtitle[before skip=\baselineskip]%
  {My subtitle}
  Further text.
\end{tcolorbox}
\end{exdispExample*}
\end{docCommand}

\begin{docTcbKey}[][doc new=2014-10-10]{subtitle style}{=\meta{options}}{no default, initially empty}
  Adds |tcolorbox| \meta{options} to the settings for \refCom{tcbsubtitle}.
\begin{exdispExample*}{subtitle_style}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[title=My title,
  colback=red!5!white,
  colframe=red!75!black,
  colbacktitle=yellow!50!red,
  coltitle=red!25!black,
  fonttitle=\bfseries,
  subtitle style={boxrule=0.4pt,
    colback=yellow!50!red!25!white} ]
  This is a \textbf{tcolorbox}.
\tcbsubtitle{My subtitle}
  Further text.
\tcbsubtitle{Second subtitle}
  Further text.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\clearpage
\subsection{Upper Part}
The text content of a \refEnv{tcolorbox} may be parted into a mandatory \emph{upper part}
and an optional \emph{lower part}. These parts are separated by
\refCom{tcblower}. If there is no \refCom{tcblower} present, there is no
\emph{lower part} and the \emph{upper part} forms the complete text content.

\begin{docTcbKey}[][doc new=2015-01-06]{upperbox}{=\meta{mode}}{no default, initially \texttt{visible}}
  Controls the treatment of the upper part of the box. If there is no lower part,
  this is the complete text content.
  Feasible values for \meta{mode} are:
  \begin{itemize}
  \item\docValue{visible}: usual type setting of the upper part,
  \item\docValue{invisible}: empty space instead of the upper part contents.
  \end{itemize}
\begin{exdispExample}{upperbox}
\begin{tcolorbox}[upperbox=invisible,colback=white]
This is a \textbf{tcolorbox} (but invisible).
\end{tcolorbox}

\bigskip

\begin{tcolorbox}[upperbox=invisible,colback=white]
This is a \textbf{tcolorbox} (but invisible).
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new and updated={2015-01-06}{2019-03-01}]{visible}{}{style, no value}
  Shortcut for setting \refKey{/tcb/upperbox}, \refKey{/tcb/lowerbox}, and \refKey{/tcb/titlebox}
  to be \docValue{visible}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new and updated={2015-01-06}{2019-03-01}]{invisible}{}{style, no value}
  Shortcut for setting \refKey{/tcb/upperbox}, \refKey{/tcb/lowerbox}, and \refKey{/tcb/titlebox}
  to be \docValue{invisible}.
\begin{exdispExample}{invisible}
\begin{tcolorbox}[invisible]
This is a \textbf{tcolorbox} (but invisible).
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\clearpage
\begin{docTcbKey}[][doc new=2015-05-04]{saveto}{=\meta{file name}}{no default, initially empty}
  Saves the content of the box into a file for an optional later usage.
  This is the counterpart of \refKey{/tcb/savelowerto}, but is saves not
  only the upper part but the whole content. If a lower part is present,
  it is also saved including \refCom{tcblower}.
  \begin{marker}
  This option cannot be combined with \refKey{/tcb/savelowerto}.
  \end{marker}

\begin{exdispExample}{saveto_1}
\begin{tcolorbox}[invisible,saveto=\jobname_mysave1.tex,colback=white]
This is a \textbf{tcolorbox} which seems to be empty.
The content is saved for later usage.
\end{tcolorbox}

Now, we load the saved text:\\
\input{\jobname_mysave1.tex}
\end{exdispExample}

\begin{exdispExample}{saveto_2}
\begin{tcolorbox}[saveto=\jobname_mysave2.tex]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}

Now, we load the saved text:
\begin{tcolorbox}[colframe=red,colback=red!10,
  coltitle=black,colbacktitle=red!20,sidebyside,
  title=Here we see the saved content including the lower part]
\input{\jobname_mysave2.tex}
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}



\clearpage
\subsection{Lower Part}
\begin{docTcbKey}{lowerbox}{=\meta{mode}}{no default, initially \texttt{visible}}
  Controls the treatment of the lower part of the box.
  Feasible values for \meta{mode} are:
  \begin{itemize}
  \item\docValue{visible}: usual type setting of the lower part,
  \item\docValue{invisible}: empty space instead of the lower part contents,
  \item\docValue{ignored}: the lower part is not used (here).
  \end{itemize}
  The last two values are usually applied in connection with |savelowerto|.
\begin{exdispExample}{lowerbox}
\begin{tcolorbox}[lowerbox=invisible,colback=white]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part (but invisible).
\end{tcolorbox}

\begin{tcolorbox}[lowerbox=ignored,colback=white]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part (but ignored).
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc updated=2014-11-28]{savelowerto}{=\meta{file name}}{no default, initially empty}
  Saves the content of the lower part into a file for an optional later usage.
\begin{exdispExample}{savelowerto}
\begin{tcolorbox}[lowerbox=invisible,savelowerto=\jobname_bspsave.tex,colback=white]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part which may be quite complex:
$\displaystyle f(x)=\frac{1+x^2}{1-x^2}$.
\end{tcolorbox}

Now, we load the saved text:\\
\input{\jobname_bspsave.tex}
\end{exdispExample}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{lower separated}{\colOpt{=true\textbar false}}{default |true|, initially |true|}
If set to |true|, the lower part is visually separated from the upper part.
It depends on the chosen skin how the visualization of the separation is done.
\enlargethispage*{1cm}
\begin{exdispExample}{lower_separated}
% \tcbuselibrary{skins,raster}
\begin{tcbraster}[colback=red!5!white,colframe=red!75!black,
  fonttitle=\bfseries,fontlower=\itshape]
%
\begin{tcolorbox}[title=Lower separated]
This is the upper part.
\tcblower
This is the lower part.
\end{tcolorbox}
%
\begin{tcolorbox}[title=Lower not separated,lower separated=false]
This is the upper part.
\tcblower
This is the lower part.
\end{tcolorbox}
%
\begin{tcolorbox}[sidebyside,title=Lower separated]
This is the upper part.
\tcblower
This is the lower part.
\end{tcolorbox}
%
\begin{tcolorbox}[sidebyside,title=Lower not separated,lower separated=false]
This is the upper part.
\tcblower
This is the lower part.
\end{tcolorbox}
%
\begin{tcolorbox}[beamer,title=Lower separated]
This is the upper part.
\tcblower
This is the lower part.
\end{tcolorbox}
%
\begin{tcolorbox}[beamer,title=Lower not separated,lower separated=false]
This is the upper part.
\tcblower
This is the lower part.
\end{tcolorbox}
%
\end{tcbraster}
\end{exdispExample}
\end{docTcbKey}


\clearpage
\begin{docTcbKey}{savedelimiter}{=\meta{name}}{no default, initially \texttt{tcolorbox}}
  Used in connection with new environment definitions which extend
  |tcolorbox| and use or allow the option |savelowerto|.
  To catch the end of the new box environment \meta{name} has to be the name of
  this environment. Additionally, the environment definition has to use
  |\tcolorbox| instead of
  |\begin{tcolorbox}| and |\endtcolorbox| instead of |\end{tcolorbox}|.
\begin{exdispExample}{savedelimiter1}
\newenvironment{mybox}[1]{%
  \tcolorbox[savedelimiter=mybox,
             savelowerto=\jobname_bspsave2.tex,lowerbox=ignored,
             colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries,
             title=#1]}%
  {\endtcolorbox}

\begin{mybox}{My Example}
Upper part.
\tcblower
Saved lower part!
\end{mybox}

Now, the saved part is used:
\begin{tcolorbox}[colback=green!5]
\input{\jobname_bspsave2.tex}
\end{tcolorbox}
\end{exdispExample}

The |savedelimiter| is used implicitely with \refCom{newtcolorbox} which
allows a more convenient usage:
\begin{exdispExample}{savedelimiter2}
\newtcolorbox{mybox}[1]{%
             savelowerto=\jobname_bspsave2.tex,lowerbox=ignored,
             colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries,
             title=#1}%

\begin{mybox}{My Example}
Upper part.
\tcblower
Saved lower part!
\end{mybox}

Now, the saved part is used:
\begin{tcolorbox}[colback=green!5]
\input{\jobname_bspsave2.tex}
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}



\clearpage
\subsection{Colors and Fonts}
\begin{docTcbKey}{colframe}{=\meta{color}}{no default, initially \texttt{black!75!white}}
  Sets the frame \meta{color} of the box.
\begin{exdispExample*}{colframe}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[colframe=red!50!white]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\begin{docTcbKey}{colback}{=\meta{color}}{no default, initially \texttt{black!5!white}}
  Sets the background \meta{color} of the box.
\begin{exdispExample*}{colback}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[colback=red!50!white]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{title filled}{\colOpt{=true\textbar false}}{default |true|, initially |false|}
  Switches the drawing of the title background according to the given value.
  This option is set to |true| automatically by \refKey{/tcb/colbacktitle},
  \refKey{/tcb/opacitybacktitle}, and \refKey{/tcb/title style},
  and \refKey{/tcb/title code}.

\begin{exdispExample*}{title_filled}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[title=My title,title filled]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\begin{tcolorbox}[title=My title,
  title filled=false]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{colbacktitle}{=\meta{color}}{no default, initially \texttt{black!50!white}}
  Sets the background \meta{color} of the title area of the box.
\begin{exdispExample*}{colbacktitle}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[colbacktitle=red!50!white,
  title=My title,coltitle=black,
  fonttitle=\bfseries]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}



\clearpage

\begin{docTcbKey}{colupper}{=\meta{color}}{no default, initially \texttt{black}}
  Sets the text \meta{color} of the upper part.
\begin{exdispExample*}{colupper}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[colupper=red!75!black]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{collower}{=\meta{color}}{no default, initially \texttt{black}}
  Sets the text \meta{color} of the lower part.
\begin{exdispExample*}{collower}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[collower=red!75!black]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{coltext}{=\meta{color}}{style, no default, initially \texttt{black}}
  Sets the text \meta{color} of the box. This is an abbreviation for setting
  |colupper| and |collower| to the same value.
\begin{exdispExample*}{coltext}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[coltext=red!75!black]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{coltitle}{=\meta{color}}{no default, initially \texttt{white}}
  Sets the title text \meta{color} of the box.
\begin{exdispExample*}{coltitle}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[coltitle=red!75!black,
  colbacktitle=black!10!white,title=Test]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\clearpage

\begin{docTcbKey}{fontupper}{=\meta{text}}{no default, initially empty}
  Sets \meta{text} before the content of the upper part (e.\,g.\ font settings).
\begin{exdispExample}{fontupper}
\begin{tcolorbox}[fontupper=Hello!~\sffamily]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}{fontlower}{=\meta{text}}{no default, initially empty}
  Sets \meta{text} before the content of the lower part (e.\,g.\ font settings).
\begin{exdispExample}{fontlower}
\begin{tcolorbox}[fontlower=\sffamily\bfseries]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}{fonttitle}{=\meta{text}}{no default, initially empty}
  Sets \meta{text} before the content of the title text (e.\,g.\ font settings).
\begin{exdispExample}{fonttitle}
\begin{tcolorbox}[fonttitle=\sffamily\bfseries\large,title=Hello]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\bigskip
\begin{marker}
  More color options are provided by using skins documented in
  Section \ref{sec:skins} from page \pageref{sec:skins}.
\end{marker}


\clearpage
\subsection{Text Alignment}

\begin{docTcbKey}[][doc new=2015-05-07]{halign}{=\meta{alignment}}{no default, initially \texttt{justify}}
  If there is no lower part, |halign| determines the horizontal \meta{alignment}
  of the text content.
  Otherwise, |halign| determines the horizontal \meta{alignment}
  of the upper part of the box only.
  The feasible values for \meta{alignment} are more or less identical to
  the corresponding |/tikz/align| settings, even if the implementation differs.
  \begin{itemize}
  \item\docValue{justify}: usual left and right justified type setting.
  \item\docValue{left}: left border justification in analogy to plain \TeX.
  \item\docValue{flush left}: left border justification with |\raggedright| of \LaTeX.
  \item\docValue{right}: right border justification in analogy to plain \TeX.
  \item\docValue{flush right}: right border justification with |\raggedleft| of \LaTeX.
  \item\docValue{center}: centering in analogy to plain \TeX.
  \item\docValue{flush center}: centering with |\centering| of \LaTeX.
  \end{itemize}
  The differences between the flush and non-flush version are explained in
  detail in the \tikzname\ manual \cite{tantau:tikz_and_pgf}. The short story is that
  the non-flush versions will often look more balanced but with more
  hyphenations.

\begin{exdispExample}{halign}
\tcbset{colback=red!5!white,colframe=red!75!black,size=small,
  fonttitle=\bfseries,width=3.5cm,box align=top,
  nobeforeafter}

\begin{tcolorbox}[adjusted title=flush center,halign=flush center]
This is a demonstration text for showing how line breaking works.
\end{tcolorbox}
\begin{tcolorbox}[adjusted title=flush left,halign=flush left]
This is a demonstration text for showing how line breaking works.
\end{tcolorbox}
\begin{tcolorbox}[adjusted title=flush right,halign=flush right]
This is a demonstration text for showing how line breaking works.
\end{tcolorbox}

\begin{tcolorbox}[adjusted title=center,halign=center]
This is a demonstration text for showing how line breaking works.
\end{tcolorbox}
\begin{tcolorbox}[adjusted title=left,halign=left]
This is a demonstration text for showing how line breaking works.
\end{tcolorbox}
\begin{tcolorbox}[adjusted title=right,halign upper=right]
This is a demonstration text for showing how line breaking works.
\end{tcolorbox}
\end{exdispExample}

\end{docTcbKey}


\begin{docTcbKey}[][doc new=2015-05-07]{halign upper}{=\meta{alignment}}{no default, initially \texttt{justify}}
  Alias for \refKey{/tcb/halign}.
\end{docTcbKey}

\newpage
\begin{docTcbKey}[][doc new=2015-05-07]{halign lower}{=\meta{alignment}}{no default, initially \texttt{justify}}
  |halign lower| determines the horizontal \meta{alignment} of the lower part of the box.
  The feasible values for \meta{alignment} are the same as for \refKey{/tcb/halign}.

\begin{exdispExample}{halign_lower}
\begin{tcbraster}[raster columns=3,fonttitle=\bfseries,
  colback=red!5!white,colframe=red!75!black]

  \begin{tcolorbox}[adjusted title=flush center,halign lower=flush center]
    Upper part. \tcblower Lower part.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=flush left,halign lower=flush left]
    Upper part. \tcblower Lower part.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=flush right,halign lower=flush right]
    Upper part. \tcblower Lower part.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=center,halign lower=center]
    Upper part. \tcblower Lower part.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=left,halign lower=left]
    Upper part. \tcblower Lower part.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=right,halign lower=right]
    Upper part. \tcblower Lower part.
  \end{tcolorbox}

\end{tcbraster}
\end{exdispExample}
\end{docTcbKey}


\clearpage
\begin{docTcbKey}[][doc new=2015-05-07]{halign title}{=\meta{alignment}}{no default, initially \texttt{justify}}
  |halign lower| determines the horizontal \meta{alignment} of the title of the box.
  The feasible values for \meta{alignment} are the same as for \refKey{/tcb/halign}.

\begin{exdispExample}{halign_title}
\begin{tcbraster}[raster columns=3,fonttitle=\bfseries,
  colback=red!5!white,colframe=red!75!black]

  \begin{tcolorbox}[adjusted title=flush center,halign title=flush center]
    This is a \textbf{tcolorbox}.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=flush left,halign title=flush left]
    This is a \textbf{tcolorbox}.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=flush right,halign title=flush right]
    This is a \textbf{tcolorbox}.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=center,halign title=center]
    This is a \textbf{tcolorbox}.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=left,halign title=left]
    This is a \textbf{tcolorbox}.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=right,halign title=right]
    This is a \textbf{tcolorbox}.
  \end{tcolorbox}

\end{tcbraster}
\end{exdispExample}
\end{docTcbKey}

\enlargethispage*{1cm}

\begin{docTcbKey}[][doc updated=2015-05-07]{flushleft upper}{}{style, no value}
  Shortcut for setting \refKey{/tcb/halign} to \docValue{flush left}.
\end{docTcbKey}

\begin{docTcbKey}[][doc updated=2015-05-07]{center upper}{}{style, no value}
  Shortcut for setting \refKey{/tcb/halign} to \docValue{flush center}.
\end{docTcbKey}

\begin{docTcbKey}[][doc updated=2015-05-07]{flushright upper}{}{style, no value}
  Shortcut for setting \refKey{/tcb/halign} to \docValue{flush right}.
\end{docTcbKey}

\begin{docTcbKey}[][doc updated=2015-05-07]{flushleft lower}{}{style, no value}
  Shortcut for setting \refKey{/tcb/halign lower} to \docValue{flush left}.
\end{docTcbKey}

\begin{docTcbKey}[][doc updated=2015-05-07]{center lower}{}{style, no value}
  Shortcut for setting \refKey{/tcb/halign lower} to \docValue{flush center}.
\end{docTcbKey}

\begin{docTcbKey}[][doc updated=2015-05-07]{flushright lower}{}{style, no value}
  Shortcut for setting \refKey{/tcb/halign lower} to \docValue{flush right}.
\end{docTcbKey}

\clearpage

\begin{docTcbKey}[][doc updated=2015-05-07]{flushleft title}{}{style, no value}
  Shortcut for setting \refKey{/tcb/halign title} to \docValue{flush left}.
\end{docTcbKey}

\begin{docTcbKey}[][doc updated=2015-05-07]{center title}{}{style, no value}
  Shortcut for setting \refKey{/tcb/halign title} to \docValue{flush center}.
\end{docTcbKey}

\begin{docTcbKey}[][doc updated=2015-05-07]{flushright title}{}{style, no value}
  Shortcut for setting \refKey{/tcb/halign title} to \docValue{flush right}.
\end{docTcbKey}


\begin{marker}
The vertical alignment settings are only relevant for boxes which are larger
than their natural height, see \Fullref{sec:heightcontrol}.
\end{marker}

\begin{docTcbKey}[][doc updated=2015-07-16]{valign}{=\meta{alignment}}{no default, initially |top|}
  If the height of a |tcolorbox| is not the natural height, |valign|
  determines the vertical \meta{alignment} of the upper part.
  Feasible values are
  \begin{itemize}
  \item\docValue{top}: Anchor text at top.
  \item\docValue{center}: Anchor text at center.
  \item\docValue{bottom}: Anchor text at bottom.
  \item\docValue{scale}: Scale text vertically to fit into the available space.
    This is brutal and may not look very good. Consider \Fullref{sec:fitting}
    alternatively.
  \item\docValue{scale*}: Like \docValue{scale}, but scaling is bounded by
    \refKey{/tcb/valign scale limit}.
  \end{itemize}
  For a box with natural height, these settings are meaningless.
\begin{exdispExample}{valign}
\tcbset{width=(\linewidth-2mm)/4,before=,after=\hfill,
colframe=blue!75!black,colback=white,height=2cm}

\foreach \myalign in {top,center,bottom,scale}
{\begin{tcolorbox}[valign=\myalign]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2015-05-07]{valign upper}{=\meta{alignment}}{no default, initially \texttt{top}}
  Alias for \refKey{/tcb/valign}.
\end{docTcbKey}

\begin{docTcbKey}{valign lower}{=\meta{alignment}}{no default, initially |top|}
  This key has the same meaning for the lower part as |valign|
  for the upper part, i.\,e., it determines
  the vertical \meta{alignment} of the lower part with feasible values
  |top|, |center|, |bottom|, |scale|, and |scale*|.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-07-16]{valign scale limit}{=\meta{real number}}{no default, initially \texttt{1.1}}
  Sets an upper scale limit for the \docValue{scale*} setting in
  \refKey{/tcb/valign} and \refKey{/tcb/valign lower}.
  Note that this value is not reset by \refKey{/tcb/reset}. So, changes
  also apply to embedded boxes.
\end{docTcbKey}


Also see \refKey{/tcb/sidebyside align} for alignment settings when
upper part and lower part are set side-by-side.

\clearpage
\subsection{Geometry}
\subsubsection{Width}

\begin{docTcbKey}{width}{=\meta{length}}{no default, initially \cs{linewidth}}
  Sets the total width of the colored box to \meta{length}.
  See also \refKey{/tcb/height}.
\begin{exdispExample}{width}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[width=\linewidth/2]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2014-10-31]{text width}{=\meta{length}}{style, no default}
  Sets the text width of the upper part to \meta{length}.
  See also \refKey{/tcb/text height}.
\begin{exdispExample}{text_width}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[text width=4cm]
This is a \textbf{tcolorbox} where the text has a width of 4cm.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-11-07]{add to width}{=\meta{length}}{style, no default}
  Adds \meta{length} to the current total width of the colored box.
\begin{exdispExample*}{add_to_width}{sbs,lefthand ratio=0.6}
\tcbset{width=4cm,colback=red!5!white,
  colframe=red!75!black}

\begin{tcolorbox}
This is a \textbf{tcolorbox}.
\end{tcolorbox}

\begin{tcolorbox}[add to width=1cm]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


See \Fullref{sec:heightcontrol} for setting fixed height values.


\clearpage
\subsubsection{Rules}
\begin{docTcbKey}{toprule}{=\meta{length}}{no default, initially \texttt{0.5mm}}
  Sets the line width of the top rule to \meta{length}.
\begin{exdispExample}{toprule}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[toprule=3mm]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}{bottomrule}{=\meta{length}}{no default, initially \texttt{0.5mm}}
  Sets the line width of the bottom rule to \meta{length}.
\begin{exdispExample}{bottomrule}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[bottomrule=3mm]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\begin{docTcbKey}{leftrule}{=\meta{length}}{no default, initially \texttt{0.5mm}}
  Sets the line width of the left rule to \meta{length}.
\begin{exdispExample}{leftrule}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[leftrule=3mm]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}{rightrule}{=\meta{length}}{no default, initially \texttt{0.5mm}}
  Sets the line width of the right rule to \meta{length}.
\begin{exdispExample}{rightrule}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[rightrule=3mm]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{titlerule}{=\meta{length}}{no default, initially \texttt{0.5mm}}
  Sets the line width of the rule below the title to \meta{length}.
\begin{exdispExample}{titlerule}
\tcbset{enhanced,colback=red!5!white,colframe=red!75!black,
  colbacktitle=red!90!black}

\begin{tcolorbox}[titlerule=3mm,title=This is the title]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}{boxrule}{=\meta{length}}{style, no default, initially \texttt{0.5mm}}
  Sets all rules of the frame to \meta{length}, i.\,e.\ 
  \refKey{/tcb/toprule}, \refKey{/tcb/bottomrule}, \refKey{/tcb/leftrule},
  \refKey{/tcb/rightrule}, and \refKey{/tcb/titlerule}.
\begin{exdispExample}{boxrule}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[boxrule=3mm]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\bigskip
\begin{marker}
  More options for drawing a \refKey{/tcb/borderline} are provided by using skins documented in
  Section \ref{sec:skins} from page \pageref{sec:skins}.
\end{marker}


\subsubsection{Arcs}
\begin{docTcbKey}{arc}{=\meta{length}}{no default, initially \texttt{1mm}}
  Sets the inner radius of the four frame arcs to \meta{length}.
\begin{exdispExample}{arc}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[arc=0mm]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\begin{tcolorbox}[arc=3mm]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\clearpage
\begin{docTcbKey}[][doc new=2015-05-05]{circular arc}{}{style, no value}
  Sets \refKey{/tcb/arc} to match the half of the inner width of the colored box.
  If width and height of the box are identical, this gives a circle.
  \begin{marker}
  If the height of the box is smaller than the width, the result will look
  quite ugly.
  \end{marker}
\begin{exdispExample*}{circular_arc}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[width=3cm,
  colback=red!5!white,
  colframe=red!75!black,
  halign=center,valign=center,
  square,circular arc]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2015-05-05]{bean arc}{}{style, no value}
  Sets \refKey{/tcb/arc} to match the smaller value of the
  half of the inner width and of the inner height of the colored box.
  \begin{marker}
  This only works for a fixed \refKey{/tcb/height}. Also, \refKey{/tcb/bean arc}
  must be used \emph{after} width and height are set by option keys.
  \end{marker}
\begin{exdispExample*}{bean_arc}{sbs,lefthand ratio=0.6}
\tcbset{size=fbox,boxrule=0.5mm,
  colback=red!5!white,
  colframe=red!75!black,
  halign=center,valign=center}

\begin{tcolorbox}[width=3cm,height=2cm,
  bean arc]
Box A
\end{tcolorbox}

\begin{tcolorbox}[width=2cm,height=3cm,
  bean arc]
Box B
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-05-05]{octogon arc}{}{style, no value}
  Sets \refKey{/tcb/arc} to match $\frac{1}{2+\sqrt{2}}$ of the inner width
  of the colored box. If width and height of the box are identical,
  the interior is a regular octogon.
\begin{exdispExample*}{octogon_arc}{sbs,lefthand ratio=0.8}
\begin{tcolorbox}[enhanced,
  size=minimal,auto outer arc,
  width=2.1cm,octogon arc,
  colback=red,colframe=white,colupper=white,
  fontupper=\fontsize{7mm}{7mm}\selectfont\bfseries\sffamily,
  halign=center,valign=center,
  square,arc is angular,
  borderline={0.2mm}{-1mm}{red}  ]
STOP
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}[][doc new=2015-05-05]{arc is angular}{}{no value, initially unset}
  Using this options applies a patch which straightens the corners arcs of
  the boxes. The little arcs are replaced by little straight lines.
  \begin{marker}
  This patch is considered as an experimental feature.
  It changes some of the original \tikzname\ code. This change may break
  with future updates of \tikzname.
  \end{marker}

\begin{exdispExample*}{arc_is_angular}{sbs,lefthand ratio=0.6}
\tcbset{colback=red!5!white,colframe=red!75!black,
  arc=3mm}

\begin{tcolorbox}[arc is angular]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\begin{tcolorbox}[arc is curved]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}

\end{docTcbKey}


\begin{docTcbKey}[][doc new=2015-05-05]{arc is curved}{}{no value, initially set}
  This option resets the patch from \refKey{/tcb/arc is angular}. The
  original \tikzname\ code is activated.
\end{docTcbKey}


\begin{docTcbKey}{outer arc}{=\meta{length}}{no default, initially unset}
  Sets the outer radius of the four frame arcs to \meta{length}.
\begin{exdispExample}{outer_arc}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[arc=4mm,outer arc=1mm]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}{auto outer arc}{}{no value, initially set}
  Sets the outer radius of the four frame arcs automatically in
  dependency of the inner radius given by \refKey{/tcb/arc}.
\end{docTcbKey}


\clearpage
\subsubsection{Spacing}
\begin{docTcbKey}{boxsep}{=\meta{length}}{no default, initially \texttt{1mm}}
  Sets a common padding of \meta{length} between the text content and the
  frame of the box. This value is added to the key values of
  |left|, |right|, |top|, |bottom|, and |middle| at the appropriate places.
\begin{exdispExample}{boxsep}
\tcbset{colback=red!5!white,colframe=red!75!black,width=(\linewidth-4mm)/2,
  before=,after=\hfill}

\begin{tcolorbox}[boxsep=5mm]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\begin{tcolorbox}[boxsep=5mm,draft]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}{left}{=\meta{length}}{style, no default, initially \texttt{4mm}}
  Sets the left space between all text parts and frame (additional to |boxsep|).
  This is an abbreviation for setting
  |lefttitle|, |leftupper|, and |leftlower| to the same value.
\begin{exdispExample}{left}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[left=0mm]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2017-02-16]{left*}{=\meta{length}}{style, no default}
  Sets \refKey{/tcb/left} such that \meta{length} is the distance between
  the left bounding box and the text parts.
\begin{exdispExample}{left_star}
\tcbset{colback=red!5!white,colframe=red!75!black}

This is some text.
\begin{tcolorbox}[grow to left by=5mm,left*=0mm,
  enhanced,show bounding box]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{lefttitle}{=\meta{length}}{no default, initially \texttt{4mm}}
  Sets the left space between title text and frame (additional to |boxsep|).
\begin{exdispExample}{lefttitle}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[lefttitle=3cm,title=My Title]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}{leftupper}{=\meta{length}}{no default, initially \texttt{4mm}}
  Sets the left space between upper text and frame (additional to |boxsep|).
\begin{exdispExample}{leftupper}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[leftupper=3cm,title=My Title]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\begin{docTcbKey}{leftlower}{=\meta{length}}{no default, initially \texttt{4mm}}
  Sets the left space between lower text and frame (additional to |boxsep|).
\begin{exdispExample}{leftlower}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[leftlower=3cm]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\enlargethispage*{1cm}

\begin{docTcbKey}{right}{=\meta{length}}{style, no default, initially \texttt{4mm}}
  Sets the right space between all text parts and frame (additional to |boxsep|).
  This is an abbreviation for setting
  |righttitle|, |rightupper|, and |rightlower| to the same value.
\begin{exdispExample}{right}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[width=5cm,right=2cm]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\clearpage

\begin{docTcbKey}[][doc new=2017-02-16]{right*}{=\meta{length}}{style, no default}
  Sets \refKey{/tcb/right} such that \meta{length} is the distance between
  the right bounding box and the text parts.
\begin{exdispExample}{right_star}
\tcbset{colback=red!5!white,colframe=red!75!black}

\flushright This is some text.
\begin{tcolorbox}[grow to right by=5mm,right*=0mm,
  halign=right,enhanced,show bounding box]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}



\begin{docTcbKey}{righttitle}{=\meta{length}}{no default, initially \texttt{4mm}}
  Sets the right space between title text and frame (additional to |boxsep|).
\begin{exdispExample}{righttitle}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[width=5cm,righttitle=2cm,title=My very long title text]
This is a \textbf{tcolorbox} with standard upper box dimensions.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}{rightupper}{=\meta{length}}{no default, initially \texttt{4mm}}
  Sets the right space between upper text and frame (additional to |boxsep|).
\begin{exdispExample}{rightupper}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[width=5cm,rightupper=2cm,title=My very long title text]
This is a \textbf{tcolorbox} with compressed upper box dimensions.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\clearpage
\begin{docTcbKey}{rightlower}{=\meta{length}}{no default, initially \texttt{4mm}}
  Sets the right space between lower text and frame (additional to |boxsep|).
\begin{exdispExample}{rightlower}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[width=5cm,rightlower=2cm]
This is a \textbf{tcolorbox} with standard upper box dimensions.
\tcblower
This is the lower part with large space at right.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}



\begin{docTcbKey}{top}{=\meta{length}}{no default, initially \texttt{2mm}}
  Sets the top space between text and frame (additional to |boxsep|).
\begin{exdispExample}{top}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[top=0mm]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}{toptitle}{=\meta{length}}{no default, initially \texttt{0mm}}
  Sets the top space between title and frame (additional to |boxsep|).
\begin{exdispExample}{toptitle}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[toptitle=3mm,title=My title]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{bottom}{=\meta{length}}{no default, initially \texttt{2mm}}
  Sets the bottom space between text and frame (additional to |boxsep|).
\begin{exdispExample}{bottom}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[bottom=0mm]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\begin{docTcbKey}{bottomtitle}{=\meta{length}}{no default, initially \texttt{0mm}}
  Sets the bottom space between title and frame (additional to |boxsep|).
\begin{exdispExample}{bottomtitle}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[bottomtitle=3mm,title=My title]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}{middle}{=\meta{length}}{no default, initially \texttt{2mm}}
  Sets the space between upper and lower text to the separation line
  (additional to |boxsep|).
\begin{exdispExample}{middle}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[middle=0mm,boxsep=0mm]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\clearpage
\subsubsection{Size Shortcuts}
\begin{docTcbKey}{size}{=\meta{name}}{no default, initially \texttt{normal}}
  Sets all geometry keys with exception of \refKey{/tcb/width} to
  predefined length values.
  For \meta{name}, the following values are feasible:
  \begin{itemize}
  \item\docValue{normal}: normal sized boxes e.g. of width |\linewidth|.
  \item\docValue{title}: title line sized boxes.
  \item\docValue{small}: small boxes e.g. for keyword highlighting.
  \item\docValue{fbox}: identical to the standard |\fbox|.
  \item\docValue{tight}: no padding space at all.
  \item\docValue{minimal}: no padding space, no box rules.
  \end{itemize}

\begin{exdispExample}{size_1}
\tcbset{colback=red!5!white,colframe=red!75!black}

\foreach \s in {normal,title,small,fbox,tight,minimal} {
  \tcbox[size=\s,on line]{\s} }

\foreach \s in {normal,title,small,fbox,tight,minimal} {
  \tcbox[size=\s,on line,title=Test]{\s} }

\foreach \s in {normal,title,small,fbox,tight,minimal} {
  \begin{tcolorbox}[size=\s,on line,title=Test,width=2.2cm]
    \s \tcblower lower\end{tcolorbox} }
\end{exdispExample}

\bigskip

\begin{tcolorbox}[tabularx={l|XXXXXX},title=Predefined values,
enhanced,fonttitle=\small\bfseries,fontupper=\small\ttfamily,
colback=yellow!10!white,colframe=red!50!black,colbacktitle=Salmon!30!white,
coltitle=black,center title
]
            & normal & title  & small & fbox  & tight & minimal\\\hline
boxrule     & 0.5mm  & 0.4mm  & 0.3mm & 0.4pt & 0.4pt & 0.0pt \\
boxsep      & 1.0mm  & 1.0mm  & 1.0mm & 3.0pt & 0.0pt & 0.0pt \\
left        & 4.0mm  & 2.0mm  & 1.0mm & 0.0pt & 0.0pt & 0.0pt \\
right       & 4.0mm  & 2.0mm  & 1.0mm & 0.0pt & 0.0pt & 0.0pt \\
top         & 2.0mm  & 0.25mm & 0.0mm & 0.0pt & 0.0pt & 0.0pt \\
bottom      & 2.0mm  & 0.25mm & 0.0mm & 0.0pt & 0.0pt & 0.0pt \\
toptitle    & 0.0mm  & 0.0mm  & 0.0mm & 0.0pt & 0.0pt & 0.0pt \\
bottomtitle & 0.0mm  & 0.0mm  & 0.0mm & 0.0pt & 0.0pt & 0.0pt \\
middle      & 2.0mm  & 0.75mm & 0.5mm & 1.0pt & 0.2pt & 0.0pt \\
arc         & 1.0mm  & 0.75mm & 0.5mm & 1.0pt & 0.0pt & 0.0pt \\
outer arc   & auto   & auto   & auto  & auto  & 0.0pt & 0.0pt \\
\end{tcolorbox}
\end{docTcbKey}


\clearpage
\begin{docTcbKey}{oversize}{\colOpt{=\meta{length}}}{style, default |0pt|}
  Sets the text width of the upper part to the current line width plus an
  optional \meta{length}.
  This is achieved by changing the keys \refKey{/tcb/width}
  \refKey{/tcb/enlarge left by}, and
  \refKey{/tcb/enlarge right by} appropriately.
  The resulting box is overlapping into the left and right margin of
  the page.
  Note that this style option has to be given \emph{after} all other
  geometry keys!
  Also see \refKey{/tcb/grow sidewards by} and \refKey{/tcb/spread sidewards}.
\begin{dispListing}
\tcbset{colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries}

\textit{Normal text for comparison:}\\
\lipsum[2]

\begin{tcolorbox}[oversize,title=Oversized box]
\lipsum[2]
\end{tcolorbox}

\begin{tcolorbox}[title=Normal box]
\lipsum[2]
\end{tcolorbox}
\end{dispListing}
\end{docTcbKey}

{\tcbusetemp}


\clearpage
\subsubsection{Toggle Left and Right}
\begin{docTcbKey}[][doc updated=2017-02-16]{toggle left and right}{=\meta{toggle preset}}{default |evenpage|, initially |none|}
  According to the \meta{toggle preset}, the left and the right settings
  of the |tcolorbox| are switched or not. Feasible values are:
  \begin{itemize}
  \item\docValue{none}: no switching.
  \item\docValue{forced}: the values of the left and right rules, spaces, and corners are switched.
  \item\docValue{evenpage}: if the page is an even page, the values of the left and
    right rules, spaces, and corners are switched. This value also sets
    \refKey{/tcb/check odd page} to |true|.
  \end{itemize}
\begin{marker}
Horizontal bounding box enlargements are not toggled by this option.
They can be toggled independently by \refKey{/tcb/toggle enlargement}.
For example, \refKey{/tcb/oversize} changes the bounding box.
\end{marker}
\begin{dispListing}
% \usepackage{lipsum}
% \usetikzlibrary{patterns}
% \tcbuselibrary{skins,breakable}
\begin{tcolorbox}[enhanced,breakable,
  toggle left and right,sharp corners,
  boxrule=0mm,top=0mm,bottom=0mm,left=1mm,right=1mm,
  rightrule=1cm,colupper=blue!25!black,
  interior style={fill overzoom image=lichtspiel.jpg,fill image opacity=0.25},
  frame style={pattern=crosshatch dots light steel blue},
  overlay={%
    \begin{tcbclipframe}
    \tcbifoddpage{\coordinate (X) at ([xshift=-5mm]frame.east);}
                 {\coordinate (X) at ([xshift=5mm]frame.west);}
    \fill[shading=ball,ball color=blue!50!white,opacity=0.5] (X) circle (4mm);
    \end{tcbclipframe}}]
\lipsum[1-6]
\end{tcolorbox}
\end{dispListing}
\medskip

This example switches a |1cm| thick rule from the left to the right side
depending on the page number. Thereby, the rule is always on the outer side
of the double-sided paper. Additionally, a ball is drawn on the outer side
with help of an overlay.
\bigskip

\tcbusetemp
\end{docTcbKey}

\clearpage
\subsection{Corners}\label{subsec:corners}

The four corners of any |tcolorbox| can be set individually as
\refKey{/tcb/sharp corners} or as \refKey{/tcb/rounded corners}.
These settings are also reflected in the behavior of \refKey{/tcb/borderline}
and \refKey{/tcb/shadow} as one would expect.

By default, all four corners are \emph{rounded}. So, only the
\refKey{/tcb/sharp corners} option will be necessary for most use cases.
The \refKey{/tcb/rounded corners} option can be used to revert a \refKey{/tcb/sharp corners}
setting.

\begin{docTcbKey}{sharp corners}{=\meta{position}}{default |all|, initially unset}
The \meta{position} denotes one or more of the four box corners to be set as
\emph{sharp} corners. The not assigned corners will retain their mode.
Feasible values for \meta{position} are:
\begin{itemize}
\foreach \p in {northwest,northeast,southwest,southeast,north,south,east,west,downhill,uphill,all}
{
\item\tcbox[on line,size=title,arc=2mm,colframe=red!75!black,colback=red!5!white,
  enlarge top by=0.5mm,enlarge bottom by=0.5mm,sharp corners=\p]{\docValue{\p}}
}
\end{itemize}
\begin{exdispExample*}{sharp_corners_1}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[colback=red!5!white,
  colframe=red!75!black,
  sharp corners=northwest ]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\begin{exdispExample*}{sharp_corners_2}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[colback=red!5!white,
  colframe=red!75!black,
  sharp corners ]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{rounded corners}{=\meta{position}}{default |all|, initially |all|}
The \refKey{/tcb/rounded corners} can be used to revert a \refKey{/tcb/sharp corners}
setting. The \meta{position} denotes one or more of the four box corners to be set as
\emph{rounded} corners. The not assigned corners will retain their mode.
Feasible values for \meta{position} are\footnote{The graphical examples assume
  that the boxes where set to have sharp corners before.}:
\begin{itemize}
\foreach \p in {northwest,northeast,southwest,southeast,north,south,east,west,downhill,uphill,all}
{
\item\tcbox[on line,size=title,arc=2mm,colframe=red!75!black,colback=red!5!white,
  enlarge top by=0.5mm,enlarge bottom by=0.5mm,sharp corners,rounded corners=\p]{\docValue{\p}}
}
\end{itemize}
\begin{exdispExample*}{rounded_corners}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[colback=red!5!white,
  colframe=red!75!black,sharp corners,
  rounded corners=northwest ]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{sharpish corners}{}{style, no value}
  Shortcut for setting \refKey{/tcb/arc} and \refKey{/tcb/outer arc}
  to |0pt|. With this setting, rounded corners will appear as quasi-sharp,
  but e.\,g.\ the shadow will be somewhat rounder than the shadow
  of really sharp corners.
  \begin{marker}
  Corners are still of type \emph{rounded} with this option, but appear
  \emph{sharp}. To switch back to rounded corners, one has to adapt
  \refKey{/tcb/arc} and \refKey{/tcb/outer arc}.
  \end{marker}
\begin{exdispExample*}{sharpish_corners}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[colback=red!5!white,
  colframe=red!75!black,
  sharpish corners ]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\clearpage

The following examples will show the differences between
\refKey{/tcb/rounded corners}, \refKey{/tcb/sharpish corners}, and \refKey{/tcb/sharp corners}.
The later two give the same core box, but \refKey{/tcb/borderline}
and \refKey{/tcb/shadow} settings are slightly different.
The following examples use \refKey{/tcb/drop fuzzy shadow}.

\begin{extcolorbox}[minipage]{corners_comparison}[blankest]
\foreach \n in {rounded corners,sharpish corners,sharp corners}{
\begin{tcolorbox}[enhanced jigsaw,frame empty,interior empty,fuzzy halo,halign=center,beforeafter skip=4mm]
\begin{tcolorbox}[enhanced,drop fuzzy shadow,width=\linewidth-1cm,
  colback=red!5!white, colframe=red!75!black, fonttitle=\bfseries,
  title=My title,\n,
  tikz={spy using outlines={circle, magnification=8, size=2cm, connect spies}},
  overlay={\spy [blue, size=4cm] on (frame.south east)
      in node at ([xshift=-2.5cm,yshift=-2.5cm]frame.south east);
  \node[right] at ([xshift=2cm,yshift=-1cm]frame.south west) {\textbf{\Large\ttfamily\n}};
  }]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{tcolorbox}}
\end{extcolorbox}

\clearpage
\subsection{Transparency}

\begin{marker}
Transparency effects are likely to be used in conjunction with \emph{jigsaw}
skin variants, see \Vref{subsec:skinjigsaw}.
\end{marker}

\begin{docTcbKey}{opacityframe}{=\meta{fraction}}{no default, initially \texttt{1.0}}
  Sets the frame opacity of the box to the given \meta{fraction}.
\begin{exdispExample*}{opacityframe}{sbs,lefthand ratio=0.6,segmentation style={preaction={fill=white},pattern=checkerboard,pattern color=gray!40}}
\begin{tcolorbox}[opacityframe=0.25,
  colframe=red]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\begin{docTcbKey}{opacityback}{=\meta{fraction}}{no default, initially \texttt{1.0}}
  Sets the background opacity of the box to the given \meta{fraction}.
\begin{exdispExample*}{opacityback}{sbs,lefthand ratio=0.6,segmentation style={preaction={fill=white},pattern=checkerboard,pattern color=gray!40}}
\begin{tcolorbox}[standard jigsaw,colframe=red,
  opacityframe=0.5, opacityback=0.5]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{opacitybacktitle}{=\meta{fraction}}{no default, initially \texttt{1.0}}
  Sets the title background opacity of the box to the given \meta{fraction}.
\begin{exdispExample*}{opacitybacktitle}{sbs,lefthand ratio=0.6,segmentation style={preaction={fill=white},pattern=checkerboard,pattern color=gray!40}}
\begin{tcolorbox}[standard jigsaw,colframe=red,
  opacityframe=0.5, opacitybacktitle=0.5,
  title filled, title=This is a title]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{opacityfill}{=\meta{fraction}}{style, no default, initially \texttt{1.0}}
  Sets the fill opacity for frame, interior and optionally the title background
  to the given \meta{fraction}.
\begin{exdispExample*}{opacityfill}{sbs,lefthand ratio=0.6,segmentation style={preaction={fill=white},pattern=checkerboard,pattern color=gray!40}}
\begin{tcolorbox}[standard jigsaw,colframe=red,
  opacityfill=0.7, title=This is a title]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{opacityupper}{=\meta{fraction}}{no default, initially \texttt{1.0}}
  Sets the text opacity of the upper box part to the given \meta{fraction}.
\begin{exdispExample*}{opacityupper}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[enhanced,opacityupper=0.5,
  interior style={preaction={fill=white},pattern=checkerboard,pattern color=gray!40}]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{opacitylower}{=\meta{fraction}}{no default, initially \texttt{1.0}}
  Sets the text opacity of the lower box part to the given \meta{fraction}.
\begin{exdispExample*}{opacitylower}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[enhanced,opacitylower=0.5,
  interior style={preaction={fill=white},pattern=checkerboard,pattern color=gray!40}]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\begin{docTcbKey}{opacitytext}{=\meta{fraction}}{no default, initially \texttt{1.0}}
  Sets the text opacity of the upper and the lower box part to the given \meta{fraction}.
\begin{exdispExample*}{opacitytext}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[enhanced,opacitytext=0.5,
  interior style={preaction={fill=white},pattern=checkerboard,pattern color=gray!40}]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{opacitytitle}{=\meta{fraction}}{no default, initially \texttt{1.0}}
  Sets the text opacity of the box title to the given \meta{fraction}.
\begin{exdispExample*}{opacitytitle}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[enhanced,opacitytitle=0.7,
  coltitle=black,
  fonttitle=\bfseries,title=This is a title,
  title style={preaction={fill=white},pattern=checkerboard,pattern color=gray!40}]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{exdispExample*}{opacity_general}{segmentation style={preaction={fill=white},pattern=checkerboard,pattern color=gray!40}}
\begin{tcolorbox}[enhanced jigsaw,fonttitle=\bfseries,title=This is a title,
  opacityframe=0.5,opacityback=0.25,opacitybacktitle=0.25,opacitytext=0.8,
  colback=red!5!white,colframe=red!75!black,colbacktitle=yellow!20!red]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}



\clearpage
\subsection{Height Control}\label{sec:heightcontrol}
In a typical usage scenario, the height of a |tcolorbox| is computed automatically
to fit the content. Nevertheless, the height can be set to a fixed value
or to fit commonly for several boxes, e.\,g. if boxes are set side by side.

\bigskip
\begin{marker}
  The height control keys are only applicable to unbreakable boxes.
  If a box is set to be \refKey{/tcb/breakable}, the height is always
  computed according to the \emph{natural height}.
\end{marker}
\bigskip


\begin{docTcbKey}{natural height}{}{no value, initially set}
  Sets the total height of the colored box to its natural height depending
  on the box content.
\end{docTcbKey}

\begin{docTcbKey}{height}{=\meta{length}}{no default}
  Sets the total height of the colored box to \meta{length} independent
  of the box content. \meta{length} is the minimum height of the box, if
  \refKey{/tcb/height plus} is larger than zero.
\begin{exdispExample}{height}
\tcbset{width=(\linewidth-2mm)/3,before=,after=\hfill,
colframe=blue!75!black,colback=white}

\begin{tcolorbox}[height=1cm,valign=center]
  This box has a height of 1cm.
\end{tcolorbox}
\begin{tcolorbox}[height=2cm,valign=center]
  This box has a height of 2cm.
\end{tcolorbox}
\begin{tcolorbox}[height=3cm,split=0.5,valign=center,valign lower=center]
  This box has a height of 3cm.
  \tcblower
  Lower part.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\enlargethispage*{10mm}
\begin{docTcbKey}{height plus}{=\meta{length}}{no default, initially |0pt|}
  The box may extend a given fixed \refKey{/tcb/height} up to the given \meta{length}.
\begin{exdispExample}{height_plus}
\tcbset{colback=red!5!white,colframe=red!75!black,left=1mm,top=1mm,bottom=1mm,
  right=1mm,boxsep=0mm,width=3cm,nobeforeafter}

\begin{tcolorbox}[height=1cm]
This is a tcolorbox.
\end{tcolorbox}
\begin{tcolorbox}[height=1cm,height plus=1cm]
This is a tcolorbox.
\end{tcolorbox}
\begin{tcolorbox}[height=1cm,height plus=1cm]
This is a tcolorbox. This is a tcolorbox. This is a tcolorbox.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}{height from}{=\meta{min} \texttt{to} \meta{max}}{style, no default}
  Sets the box height to a dimension between \meta{min} and \meta{max}.
\begin{exdispExample}{height_from}
% \usepackage{lipsum}
\newtcolorbox{mybox}{colback=red!5!white,colframe=red!75!black,left=1mm,top=1mm,
  bottom=1mm,right=1mm,boxsep=0mm,width=4.5cm,nobeforeafter,
  height from=2cm to 8cm}

\begin{mybox}
This is a tcolorbox.
\end{mybox}
\begin{mybox}
This is a tcolorbox. This is a tcolorbox. This is a tcolorbox.
\end{mybox}
\begin{mybox}
\lipsum[2]
\end{mybox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2014-10-31]{text height}{=\meta{length}}{style, no default}
  Sets the text height to \meta{length}. This is the length from the top
  of the upper part to the bottom of the optional lower part.
  See also \refKey{/tcb/text width}.
\begin{exdispExample}{text_height}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[text height=2cm]
This is a \textbf{tcolorbox} where the text area has a height of 2cm.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\clearpage

\begin{docTcbKey}[][doc new=2014-11-07]{add to height}{=\meta{length}}{style, no default}
  Adds \meta{length} to the current height of the colored box.
  \refKey{/tcb/height} has to be set before this key is used!
  If this option is used several times, then the \refKey{/tcb/height} is
  also increased several times.
\begin{exdispExample}{add_to_height}
\tcbset{height=2cm,
  valign=center,width=(\linewidth-2mm)/2,
  before=,after=\hfill,colframe=blue!75!black,colback=white}

\begin{tcolorbox}
  This box has a height of 2cm.
\end{tcolorbox}
\begin{tcolorbox}[add to height=1cm]
  This box has a height of 3cm.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2016-02-16]{add to natural height}{=\meta{length}}{style, no default}
  The application of this option generates a box with natural height plus
  the given \meta{length}. If this option is used several times, then the
  last setting of \meta{length} wins. The resulting box is not considered
  a fixed height box and the implementation is quite different to
  \refKey{/tcb/add to height}.
\begin{exdispExample}{add_to_natural_height}
\tcbset{valign=center,width=(\linewidth-2mm)/2,
  before=,after=\hfill,colframe=blue!75!black,colback=white}

\begin{tcolorbox}
  This box has natural height.
\end{tcolorbox}
\begin{tcolorbox}[add to natural height=1cm]
  This box has natural height plus 1 cm.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\clearpage
\begin{docTcbKey}[][doc new and updated={2014-09-22}{2016-02-17}]{height fill}{\colOpt{=true\textbar false\textbar maximum}}{default |true|, initially |false|}
If set to \docValue*{true}, the height of the |tcolorbox| is set to the rest of the
available vertical space of the current page.
If set to \docValue{maximum}, the page is compressed as much as possible.
Note that the |tcolorbox|
is always set as its own paragraph using this option.
Also see \refKey{/tcb/text fill}.
\begin{marker}
Note that the library \mylib{breakable} has to be loaded to use this key!
\end{marker}
This height control key is only applicable to unbreakable boxes, but it
uses code from the library \mylib{breakable}.
The counterpart for breakable boxes is \refKey{/tcb/height fixed for}.

This option can and should not be used for boxes in boxes, but it can be
used for boxes inside a \refEnv{tcbraster}.

\begin{dispListing}
% \usepackage{lipsum}
% \tcbuselibrary{breakable}
\begin{tcolorbox}[height fill,
  colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries,
  title=Box which fills the rest of the page]
\lipsum[1]
\end{tcolorbox}
\end{dispListing}
\end{docTcbKey}
{\tcbusetemp}


\clearpage
\begin{docTcbKey}[][doc new={2017-06-28}]{inherit height}{\colOpt{=fraction}}{default |1|, initially unset}
  If this option is used for a |tcolorbox| which is embedded inside
  another (outer) |tcolorbox| \emph{and} if this outer |tcolorbox| has
  a fixed height, then the given \meta{fraction} of the available text height
  of the outer |tcolorbox| is used as \refKey{/tcb/height} for the current
  |tcolorbox|.
  Otherwise, \refKey{/tcb/natural height} is applied for the current
  |tcolorbox|.

\begin{exdispExample}{inherit_height}
\tcbset{colframe=blue!75!black,colback=white,fonttitle=\bfseries}

\begin{tcolorbox}[title=Outer box with fixed height 4cm,height=4cm]
  \begin{tcolorbox}[title=Inner box,nobeforeafter,inherit height]
    This inner box matches the available space.
  \end{tcolorbox}
\end{tcolorbox}

\begin{tcolorbox}[title=Outer box with natural height]
  \begin{tcolorbox}[title=Inner box,nobeforeafter,inherit height]
    This inner box has its natural height.
  \end{tcolorbox}
\end{tcolorbox}

\begin{tcolorbox}[title=Outer box with fixed height 5cm,height=5cm]
  \begin{tcolorbox}[title=Inner box,nobeforeafter,inherit height]
    \begin{tcolorbox}[colframe=red,beforeafter skip=0pt,inherit height=0.6]
      Deeply nested box using 60 percent of the available space.
    \end{tcolorbox}
    \begin{tcolorbox}[colframe=red,beforeafter skip=0pt,inherit height=0.4]
      Deeply nested box using 40 percent of the available space.
    \end{tcolorbox}
  \end{tcolorbox}
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\clearpage

\begin{docTcbKey}[][doc new=2015-05-05]{square}{}{style, no value}
  Sets \refKey{/tcb/height} to match the width of the colored box.
\begin{exdispExample*}{square}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[width=3cm,
  colback=red!5!white,
  colframe=red!75!black,
  halign=center,valign=center,
  square]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}



\begin{docTcbKey}{space}{=\meta{fraction}}{no default, initially 0}
  If the height of a |tcolorbox| is not the natural height, the space
  difference between the forced and the natural size is distributed
  between the upper and the lower part of the box. This space could also
  be negative.
  \meta{fraction} with a value between 0 and 1 is the amount of space
  which is added to the upper part, the rest is added to the lower part.
  If there is no lower part, then all of the space is added to
  the upper part always.
\begin{exdispExample}{fraction}
\tcbset{width=(\linewidth-2mm)/3,before=,after=\hfill,
colframe=blue!75!black,colback=white,height=3cm}

\foreach \f in {0.2,0.4,0.7}
{\begin{tcolorbox}[space=\f]
    This is the upper part.
    \tcblower
    This is the lower part.
\end{tcolorbox}}
\end{exdispExample}
\end{docTcbKey}

\begin{docTcbKey}{space to upper}{}{style}
  This is an abbreviation for |space=1|, i.\,e. all extra space is added
  to the upper part.
\end{docTcbKey}

\begin{docTcbKey}{space to lower}{}{style, initially set}
  This is an abbreviation for |space=0|, i.\,e. all extra space is added
  to the lower part (if there is any).
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{space to both}{}{style}
  This is an abbreviation for |space=0.5|, i.\,e. the extra space
  equally distributed between the upper and the lower part.
\begin{exdispExample}{space_to_both}
\tcbset{width=(\linewidth-2mm)/3,before=,after=\hfill,
colframe=blue!75!black,colback=white,height=3cm}

\foreach \myspace in {space to upper,space to both,space to lower}
{\begin{tcolorbox}[\myspace]
    This is the upper part.
    \tcblower
    This is the lower part.
\end{tcolorbox}}
\end{exdispExample}
\end{docTcbKey}



\begin{docTcbKey}[][doc new=2015-02-15]{space to}{=\meta{macro}}{no default, initially unset}
  If the height of a |tcolorbox| is not the natural height, the space
  difference between the forced and the natural size is saved into the
  given local \meta{macro}. This \meta{macro} can and should be used inside
  the box content to add content which is vertically sized to match \meta{macro}.
  \begin{marker}
    \begin{itemize}
    \item The actual length saved into \meta{macro} is adapted dynamically
      during several compilations -- at least two, but maybe more.
    \item Due to the adaption algorithm, objects can be sized with
      \meta{macro} plus any offset length.
    \item Never ever use \meta{macro} multiplied with a factor. The only
      exception to this rule is that the space can be split into parts which
      sum to \meta{macro}.
    \item Never use this in combination with \refKey{/tcb/fit}.
    \end{itemize}
  \end{marker}
\begin{exdispExample}[runs=3]{space_to_1}
\begin{tcolorbox}[colframe=blue!75!black,colback=white,height=3cm,
    space to=\myspace]
  This is my box of height 3cm. The space is filled with a picture:\\[2mm]
  \includegraphics[width=\linewidth,height=\myspace]{goldshade.png}\\[1mm]
  This is some other text.
\end{tcolorbox}
\end{exdispExample}

\begin{exdispExample}[runs=3]{space_to_2}
\begin{tcolorbox}[colframe=blue!75!black,colback=white,height=3cm,
    space to=\myspace]
  \includegraphics[width=\linewidth,
    height=0.33\dimexpr\myspace]{blueshade.png}\\[1mm]
  This is my box of height 3cm.\\[2mm]
  \includegraphics[width=\linewidth,
    height=0.67\dimexpr\myspace]{goldshade.png}
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}




\begin{docTcbKey}{split}{=\meta{fraction}}{no default}
  If the height of a |tcolorbox| is not the natural height, the
  \meta{fraction} with a value between 0 and 1 determines the positioning
  of the segmentation between the upper and the lower part. Here, 0 stands
  for top and 1 for bottom. Note that the box is split regardless of
  the actual dimensions of the text parts!
\begin{exdispExample}{split}
\tcbset{width=(\linewidth-2mm)/3,before=,after=\hfill,height=3cm,
colback=white,colframe=blue!75!black,valign=center,valign lower=center}

\foreach \f in {0.1,0.5,0.8}
{\begin{tcolorbox}[split=\f]
This is the upper part.
\tcblower
This is the lower part with a lot of text in several lines.
\end{tcolorbox}}
\end{exdispExample}
\end{docTcbKey}




\clearpage
\begin{docTcbKey}[][doc updated=2014-11-07]{equal height group}{=\meta{id}}{no default}
  Boxes which are members of an |equal height group| will all get the
  same height, i.\,e. the maximum of all their natural heights. The
  \meta{id} serves to distinguish between different height groups.
  %This \meta{id} should contain only characters which are feasible
  %for \TeX\ macro names, typically alphabetic characters but no numerals
  %and spaces.
  Note that you have to compile twice to see changes and
  that height groups are global definitions.


\begin{exdispExample}[runs=2]{equal_height_group}
\tcbset{width=(\linewidth-2mm)/3,before=,after=\hfill,arc=0mm,
colframe=blue!75!black,colback=white,fonttitle=\bfseries}

\begin{tcolorbox}[equal height group=A,adjusted title={One}]
  My smallest box.
\end{tcolorbox}%
\begin{tcolorbox}[equal height group=A,adjusted title={Two}]
  This box is also small.
  \tcblower
  But with a lower part.
\end{tcolorbox}%
\begin{tcolorbox}[equal height group=A,adjusted title={Three}]
  This box contains a lot of text just to fill the space
  with word flowing and flowing and flowing until the box
  is filled with all of it.
\end{tcolorbox}\linebreak
%
\tcbset{width=(\linewidth-1mm)/2,before=,after=\hfill,arc=0mm,
colframe=red!75!black,colback=white}
%
\begin{tcolorbox}[equal height group=B]
  Now, we use another equal height group.
\end{tcolorbox}%
\begin{tcolorbox}[equal height group=B,after=]
  \begin{equation*}
    \int\limits_{0}^{1} x^2 = \frac13.
  \end{equation*}
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\medskip
\begin{marker}
See \Vref{sec:raster} for more equal height options.
\end{marker}

\clearpage
\begin{docTcbKey}{minimum for equal height group}{=\meta{id}:\meta{length}}{no default, initially unset}
  Plants a \meta{length} into the equal height group with
  the given \meta{id}. This ensures that the height will not drop below
  \meta{length}. Note that you cannot reduce a computed height value
  by using this key with a small value.
  The difference to applying \refKey{/tcb/height} directly is that the boxes
  are never too small for their content.

\begin{dispExample}
\tcbset{colframe=blue!75!black,colback=white,arc=0mm,
  before=,after=\hfill,fonttitle=\bfseries,left=2mm,right=2mm,
  width=3.5cm,
  equal height group=C,
  minimum for equal height group=C:3.5cm}

\begin{tcolorbox}
  My first box. All boxes will get 3.5cm times 3.5cm
  if the content height is not too large.
\end{tcolorbox}%
\begin{tcolorbox}
  My second box.
  \tcblower
  This is the lower part.
\end{tcolorbox}%
\begin{tcblisting}{}
\textbf{Mixed}
with a listing.
\end{tcblisting}
\begin{tcolorbox}[title={Fourth box}]
  My final box.
\end{tcolorbox}%
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2016-03-24]{minimum for current equal height group}{=\meta{length}}{no default, initially unset}
  Sets \refKey{/tcb/minimum for equal height group} for the current equal height
  group. Apparently, this only works for an already known equal height group, i.e.
  \refKey{/tcb/equal height group} has to be set \emph{before} this option is used.
  This option is likely to be used in combination with \refKey{/tcb/raster equal height}

\begin{exdispExample}[runs=2]{minimum_for_current_equal_height_group}
% \tcbuselibrary{raster}
\begin{tcbitemize}[raster equal height,colframe=blue!75!black,colback=white,
  raster every box/.style={minimum for current equal height group=2cm}]
  \tcbitem A
  \tcbitem B
\end{tcbitemize}
\end{exdispExample}

\end{docTcbKey}


\clearpage
\begin{docTcbKey}[][doc new and updated={2015-11-27}{2016-02-22}]{use height from group}{\colOpt{=\meta{id}}}{style, default current group}
  Sets the current box to a fixed \refKey{/tcb/height} which is copied from
  an equal height group with the given \meta{id}. If this height is not
  available during the current compilation, no fixed height setting is used.
  If \meta{id} is omitted, the current equal height group is used which has
  to be set before by \refKey{/tcb/equal height group}.\par
  Note that the natural height of the current box is not considered for
  computation of the group height. The main application for
  \refKey{/tcb/use height from group} is that the height can be adapted
  further by \refKey{/tcb/add to height}.

\begin{dispExample}
\begin{tcolorbox}[use height from group=C,add to height=-2cm,
  colframe=blue!75!black,colback=white]
Height from group 'C' of the previous example, but reduced by 2cm.
\end{tcolorbox}%
\end{dispExample}

\begin{exdispExample}[runs=2]{use_height_from_group}
% \tcbuselibrary{raster}
Every line is inside an equal height group:
\begin{tcbraster}[raster equal height=rows,
    title=Box \thetcbrasternum,
    enhanced,size=small,colframe=red!50!black,colback=red!10!white]
  \begin{tcolorbox}First line\\second line\\
    The height of this box rules.\end{tcolorbox}
  \begin{tcolorbox}[use height from group]Test\end{tcolorbox}
  \begin{tcolorbox}[use height from group]
    First line\\second line\end{tcolorbox}
  \begin{tcolorbox}The height of this box rules.\end{tcolorbox}
\end{tcbraster}
\end{exdispExample}
\end{docTcbKey}



\begin{docCommand}[doc new=2015-11-27]{tcbheightfromgroup}{\marg{macro}\marg{id}}
  Saves the height from an equal height group with the given \meta{id}
  to a \meta{macro}. If this height is not available during the current compilation,
  \meta{macro} is set to |0pt|.
\end{docCommand}


\clearpage
\subsection{Box Content Additions}\label{subsec:contentadditions}
The following options introduce some arbitrary \meta{code} to the content
of a |tcolorbox|. These additions can be given at the beginning or at the ending
of the title, the upper part, or the lower part.

\begin{docTcbKey}{before title}{=\meta{code}}{no default, initially unset}
  The given \meta{code} is placed \emph{after} the color and font settings
  and \emph{before} the content of the title.
\begin{exdispExample}{before_title}
\tcbset{before title={\textcolor{yellow}{\large Important:}~},
  colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[title=My title]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}{after title}{=\meta{code}}{no default, initially unset}
  The given \meta{code} is placed \emph{after} the content of the title.
\begin{exdispExample}{after_title}
\tcbset{after title={\hfill\colorbox{Navy}{approved}},
  colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[title=My title]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\clearpage
\begin{docTcbKey}{before upper}{=\meta{code}}{no default, initially empty}
  The given \meta{code} is placed \emph{after} the color and font settings
  and \emph{before} the content of the upper part.
  The \meta{code} is appended by a final |\ignorespaces|.
\begin{exdispExample}{before_upper}
\tcbset{before upper={\textit{The story:}\par},
  colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[title=My title]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2019-02-26]{before upper*}{=\meta{code}}{no default, initially unset}
  The given \meta{code} is placed \emph{after} the color and font settings
  and \emph{before} the content of the upper part.
  In contrast to \refKey{/tcb/before upper}, no |\ignorespaces| is appended.
  Use this for situations where |\ignorespaces| is not needed or causes harm.
\begin{exdispExample}{before_upper_star}
\begin{tcolorbox}[size=small,tile,
  colback=yellow!20,colbacktitle=yellow!70!black,
  title=My table,hbox,center,center title,
  before upper*=\begin{tabular}{cc},
  after upper*=\end{tabular},
]
  \multicolumn{2}{c}{Title}\\
  one & two \\
  three & four\\
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\clearpage

\begin{docTcbKey}[][doc updated=2016-10-21]{after upper}{=\meta{code}}{no default, initially empty}
  The given \meta{code} is placed \emph{after} the content of the upper part.
  The \meta{code} is prepended by a leading |\unskip|.

\begin{exdispExample}{after_upper_1}
\tcbset{after upper={\par\hfill\textit{Read more next week}},
  colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[title=My title]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}

\begin{exdispExample}{after_upper_2}
\begin{tcolorbox}[before upper=\flqq,after upper=\frqq,
  colback=red!5!white,colframe=red!75!black]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new and updated={2016-10-21}{2019-02-28}]{after upper*}{=\meta{code}}{no default, initially unset}
  The given \meta{code} is placed \emph{after} the content of the upper part.
  In contrast to \refKey{/tcb/after upper}, no |\unskip| is prepended.
  Use this for situations where |\unskip| is not needed or causes harm.
  See \refKey{/tcb/before upper*} for an example.

\begin{marker}
  From version 3.80 to 3.94, this option prepended an |\unskip| to the given \meta{code}.\\
  From version 3.95 to 4.15, this option was deprecated.\\
  From version 4.20, this option is re-established with changed semantic (no |\unskip|!)
\end{marker}
\end{docTcbKey}


\clearpage
\begin{docTcbKey}{before lower}{=\meta{code}}{no default, initially empty}
  The given \meta{code} is placed \emph{after} the color and font settings
  and \emph{before} the content of the lower part.
  The \meta{code} is appended by a final |\ignorespaces|.
\begin{exdispExample}{before_lower}
\tcbset{before lower=\textit{Behold:~},colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2019-02-26]{before lower*}{=\meta{code}}{no default, initially unset}
  The given \meta{code} is placed \emph{after} the color and font settings
  and \emph{before} the content of the lower part.
  In contrast to \refKey{/tcb/before lower}, no |\ignorespaces| is appended.
  Use this for situations where |\ignorespaces| is not needed or causes harm.
\begin{exdispExample}{before_lower_star}
\begin{tcolorbox}[size=small,bicolor,sidebyside,center lower,
  colback=yellow!30,colbacklower=yellow!20,colframe=yellow!80!black,
  before lower*=\begin{tabular}{cc},
  after lower*=\end{tabular},
]
My table
\tcblower
  \multicolumn{2}{c}{Title}\\
  one & two \\
  three & four\\
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\clearpage

\begin{docTcbKey}[][doc updated=2016-10-21]{after lower}{=\meta{code}}{no default, initially empty}
  The given \meta{code} is placed \emph{after} the content of the lower part.
  The \meta{code} is prepended by a leading |\unskip|.


\begin{exdispExample}{after_lower_2}
\begin{tcolorbox}[after lower=\ \textit{This is the end.},
  colback=red!5!white,colframe=red!75!black]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new and updated={2016-10-21}{2019-02-28}]{after lower*}{=\meta{code}}{no default, initially unset}
  The given \meta{code} is placed \emph{after} the content of the lower part.
  In contrast to \refKey{/tcb/after upper}, no |\unskip| is prepended.
  Use this for situations where |\unskip| is not needed or causes harm.

\begin{exdispExample}{after_lower_1}
\begin{tcolorbox}[before lower*=$,after lower*=$,
  colback=red!5!white,colframe=red!75!black]
This is a \textbf{tcolorbox}.
\tcblower
\sin^2(x)+\cos^2(x)=1.
\end{tcolorbox}
\end{exdispExample}

\begin{marker}
  From version 3.80 to 3.94, this option prepended an |\unskip| to the given \meta{code}.\\
  From version 3.95 to 4.15, this option was deprecated.\\
  From version 4.20, this option is re-established with changed semantic (no |\unskip|!)
\end{marker}
\end{docTcbKey}


\clearpage
\begin{marker}
If \refKey{/tcb/text fill} is used, one cannot have a lower part
and the box is unbreakable.
\end{marker}

\begin{docTcbKey}[][doc new=2015-07-15]{text fill}{}{style, no value}
  This style sets \refKey{/tcb/before upper} and \refKey{/tcb/after upper}
  to embed the upper part with a minipage. If a fixed height was applied
  e.g.\ by \refKey{/tcb/height} or \refKey{/tcb/height fill}, this minipage
  gets a matching height. This allows to use vertical glue macros like
  |\vfill| to act like expected. If the box has no fixed height,
  setting \refKey{/tcb/text fill} has no other effect as making the box
  unbreakable.
\begin{exdispExample}{text_fill}
\begin{tcolorbox}[colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries,
  height=8cm,text fill,
  title=My filled box]
This is a \textbf{tcolorbox}.
\par\vfill
\begin{center}
  My middle text.
\end{center}
\par\vfill
This is the end of my box.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\clearpage

\begin{docTcbKey}[][doc new={2019-09-19}]{tabulars}{=\meta{preamble}}{style}
  This style sets \refKey{/tcb/before upper} and \refKey{/tcb/after upper}
  and several geometry keys to support a |tabular*| with the
  given \meta{preamble}.
  The packages |array| and |colortbl| have to be loaded separately.
\begin{exdispExample}{tabulars_1}
% \usepackage{array}
% \usepackage{colortbl} - or - \usepackage[table]{xcolor}
\tcbset{enhanced,fonttitle=\bfseries\large,fontupper=\normalsize\sffamily,
  colback=yellow!10!white,colframe=red!50!black,colbacktitle=Salmon!30!white,
  coltitle=black,center title}

\begin{tcolorbox}[tabulars={@{\extracolsep{\fill}\hspace{5mm}}lrrrrr@{\hspace{5mm}}},
  boxrule=0.5pt,title=My table]
Group & One     & Two     & Three    & Four     & Sum\\\hline\hline
Red   & 1000.00 & 2000.00 &  3000.00 &  4000.00 & 10000.00\\\hline
Green & 2000.00 & 3000.00 &  4000.00 &  5000.00 & 14000.00\\\hline
Blue  & 3000.00 & 4000.00 &  5000.00 &  6000.00 & 18000.00\\\hline\hline
Sum   & 6000.00 & 9000.00 & 12000.00 & 15000.00 & 42000.00
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new={2019-09-19}]{tabulars*}{=\marg{code}\marg{preamble}}{style}
  This is a variant of \refKey{/tcb/tabulars} which adds some \meta{code}
  before the table starts.
\begin{exdispExample}{tabulars_2}
% \usepackage{array}
% \usepackage{colortbl} - or - \usepackage[table]{xcolor}
\tcbset{enhanced,fonttitle=\bfseries\large,fontupper=\normalsize\sffamily,
  colback=yellow!10!white,colframe=red!50!black,colbacktitle=Salmon!30!white,
  coltitle=black,center title}

\begin{tcolorbox}[tabulars*={\arrayrulewidth0.5mm\renewcommand\arraystretch{1.4}}%
    {@{\extracolsep{\fill}\hspace{20mm}}lll@{\hspace{20mm}}},
  title=My table]
One     & Two     & Three \\\hline\hline
1000.00 & 2000.00 &  3000.00\\\hline
2000.00 & 3000.00 &  4000.00
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}



\clearpage
\begin{marker}
If \refKey{/tcb/tabularx} or \refKey{/tcb/tabularx*} are used, one cannot
have a lower part.
\end{marker}

\begin{docTcbKey}{tabularx}{=\meta{preamble}}{style}
  This style sets \refKey{/tcb/before upper} and \refKey{/tcb/after upper}
  and several geometry keys to support a |tabularx| with the
  given \meta{preamble}.
  The packages |tabularx| \cite {carlisle:tabularx}, |array|, and |colortbl|
  have to be loaded separately.
\begin{exdispExample}{tabularx_1}
% \usepackage{array,tabularx}
% \usepackage{colortbl} - or - \usepackage[table]{xcolor}
\newcolumntype{Y}{>{\raggedleft\arraybackslash}X}% see tabularx
\tcbset{enhanced,fonttitle=\bfseries\large,fontupper=\normalsize\sffamily,
  colback=yellow!10!white,colframe=red!50!black,colbacktitle=Salmon!30!white,
  coltitle=black,center title}

\begin{tcolorbox}[tabularx={X||Y|Y|Y|Y||Y},title=My table]
Group & One     & Two     & Three    & Four     & Sum\\\hline\hline
Red   & 1000.00 & 2000.00 &  3000.00 &  4000.00 & 10000.00\\\hline
Green & 2000.00 & 3000.00 &  4000.00 &  5000.00 & 14000.00\\\hline
Blue  & 3000.00 & 4000.00 &  5000.00 &  6000.00 & 18000.00\\\hline\hline
Sum   & 6000.00 & 9000.00 & 12000.00 & 15000.00 & 42000.00
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}{tabularx*}{=\marg{code}\marg{preamble}}{style}
  This is a variant of \refKey{/tcb/tabularx} which adds some \meta{code}
  before the table starts.
\begin{exdispExample}{tabularx_2}
% \usepackage{array,tabularx}
% \usepackage{colortbl} - or - \usepackage[table]{xcolor}
\tcbset{enhanced,fonttitle=\bfseries\large,fontupper=\normalsize\sffamily,
  colback=yellow!10!white,colframe=red!50!black,colbacktitle=Salmon!30!white,
  coltitle=black,center title}

\begin{tcolorbox}[tabularx*={\arrayrulewidth0.5mm}{X|X|X},title=My table]
One     & Two     & Three \\\hline\hline
1000.00 & 2000.00 &  3000.00\\\hline
2000.00 & 3000.00 &  4000.00
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}



\clearpage
\begin{docTcbKey}{tikz upper}{\colOpt{=\meta{options}}}{style}
  This style adds a centered |tikzpicture| environment to the start and end
  of the upper part. The \meta{options} may be given as \tikzname\  picture options.
\begin{exdispExample}{tikz_upper}
% \usepackage{tikz}

\begin{tcolorbox}[tikz upper,fonttitle=\bfseries,colback=white,colframe=black,
                  title=\tikzname\ drawing]
  \path[fill=yellow,draw=yellow!75!red] (0,0) circle (1cm);
  \fill[red] (45:5mm) circle (1mm);
  \fill[red] (135:5mm) circle (1mm);
  \draw[line width=1mm,red] (215:5mm) arc (215:325:5mm);
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}{tikz lower}{\colOpt{=\meta{options}}}{style}
  This style adds a centered |tikzpicture| environment to the start and end
  of the lower part. The \meta{options} may be given as \tikzname\  picture options.
\begin{exdispExample}{tikz_lower}
% \usepackage{tikz}
% \tcbuselibrary{skins,listings}

\begin{tcblisting}{tikz lower,listing side text,fonttitle=\bfseries,
  bicolor,colback=LightBlue!50!white,colbacklower=white,colframe=black,
  righthand width=3cm,title=\tikzname\ drawing}
\path[fill=yellow,draw=yellow!75!red]
    (0,0) circle (1cm);
\fill[red] (45:5mm) circle (1mm);
\fill[red] (135:5mm) circle (1mm);
\draw[line width=1mm,red]
    (215:5mm) arc (215:325:5mm);
\end{tcblisting}
\end{exdispExample}
\end{docTcbKey}


\clearpage
\begin{docTcbKey}{tikznode upper}{\colOpt{=\meta{options}}}{style}
  This style places the upper part content into a centered
  \tikzname\  node. The \meta{options} may be given as \tikzname\  node options.
  This style is especially useful for boxes with multiline texts which are
  fitted to the text width.
\begin{exdispExample}{tikznode_upper}
% \usepackage{tikz}
\newtcbox{\headline}[1][]{enhanced,center,
  ignore nobreak,fontupper=\Large\bfseries,
  colframe=red!50!black,colback=red!10!white,
  drop fuzzy shadow=yellow,tikznode upper,#1}

\headline{Important\\Headline}
\end{exdispExample}
\end{docTcbKey}

\begin{docTcbKey}{tikznode lower}{\colOpt{=\meta{options}}}{style}
  This style places the lower part content into a centered
  \tikzname\ node. The \meta{options} may be given as \tikzname\  node options.
\begin{exdispExample}{tikznode_lower}
% \usepackage{tikz}
\begin{tcolorbox}[bicolor,colback=LightBlue!50!white,colbacklower=white,
  colframe=black,tikznode lower={inner sep=2pt,draw=red,fill=yellow}]
Upper part.
\tcblower
Lower part.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\begin{docTcbKey}{tikznode}{\colOpt{=\meta{options}}}{style}
  Shortcut for setting \refKey{/tcb/tikznode upper} and \refKey{/tcb/tikznode lower}
  the same time.
\end{docTcbKey}


\begin{docTcbKey}{varwidth upper}{\colOpt{=\meta{length}}}{style, default \refKey{/tcb/width}}
  This style places the upper part content into a |varwidth| environment.
  This style needs the |varwidth| package \cite{arseneau:2011a} to be loaded manually.
  The resulting box has a maximal width of \meta{length}.
  This option is only senseful for a \refCom{tcbox}.
\begin{exdispExample*}{varwidth_upper}{sbs,lefthand ratio=0.6}
% \usepackage{varwidth}
\newtcbox{\varbox}{colframe=red!50!black,
  colback=red!10!white,varwidth upper}

\varbox{Short text.}
\varbox{This box contains is a longer text
  which is broken.}
\end{exdispExample*}
\end{docTcbKey}


\clearpage
\subsection{Overlays}\label{subsec:overlays}
With an overlay, arbitrary \meta{graphical code} can be added to a
|tcolorbox|. This code is executed \emph{after} the frame and interior are
drawn and \emph{before} the text content is drawn. Therefore, you can
decorate the |tcolorbox| with your own extensions.
Common special cases are \emph{watermarks} which are implemented using overlays.
See Subsection \ref{subsec:watermarks} from page \pageref{subsec:watermarks} if
you want to add \emph{watermarks}.
\begin{marker}
If you use the core package only, the \meta{graphical code} has to be |pgf| code
and there is not much assistance for positioning.
Therefore, the usage of the \refKey{/tcb/enhanced} mode from the library skins
is recommended which allows |tikz| code and gives access to
\refKey{/tcb/geometry nodes} for positioning.
\end{marker}

\begin{docTcbKey}{overlay}{=\meta{graphical code}}{no default, initially unset}
  Adds \meta{graphical code} to the box drawing process. This \meta{graphical code}
  is drawn \emph{after} the frame and interior and \emph{before} the text content.

\begin{exdispExample}{overlay_1}
% \tcbuselibrary{skins} % preamble
\tcbset{frogbox/.style={enhanced,colback=green!10,colframe=green!65!black,
  enlarge top by=5.5mm,
  overlay={\foreach \x in {2cm,3.5cm} {
    \begin{scope}[shift={([xshift=\x]frame.north west)}]
      \path[draw=green!65!black,fill=green!10,line width=1mm] (0,0) arc (0:180:5mm);
      \path[fill=black] (-0.2,0) arc (0:180:1mm);
    \end{scope}}}}}

\begin{tcolorbox}[frogbox,title=My title]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}

\enlargethispage*{5mm}
\begin{exdispExample}{overlay_2}
% \usetikzlibrary{patterns} % preamble
% \tcbuselibrary{skins}     % preamble
\tcbset{ribbonbox/.style={enhanced,colback=red!5!white,colframe=red!75!black,
  fonttitle=\bfseries,
  overlay={\path[fill=blue!75!white,draw=blue,double=white!85!blue,
    preaction={opacity=0.6,fill=blue!75!white},
    line width=0.1mm,double distance=0.2mm,
    pattern=fivepointed stars,pattern color=white!75!blue]
    ([xshift=-0.2mm,yshift=-1.02cm]frame.north east)
    -- ++(-1,1) -- ++(-0.5,0) -- ++(1.5,-1.5) -- cycle;}}}

\begin{tcolorbox}[ribbonbox,title=My title]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{no overlay}{}{style, no default, initially set}
  Removes the overlay if set before.
\end{docTcbKey}

\begin{docTcbKey}{overlay broken}{=\meta{graphical code}}{no default, initially unset}
  If the box is set to be \refKey{/tcb/breakable} and \emph{is} broken actually,
  then the \meta{graphical code} is added to the box drawing process.
  \refKey{/tcb/overlay} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}{overlay unbroken}{=\meta{graphical code}}{no default, initially unset}
  If the box is set to be \refKey{/tcb/breakable} but \emph{is not} broken actually
  or if the box is set to be \refKey{/tcb/unbreakable},
  then the \meta{graphical code} is added to the box drawing process.
  \refKey{/tcb/overlay} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}{overlay first}{=\meta{graphical code}}{no default, initially unset}
  If the box is set to be \refKey{/tcb/breakable} and \emph{is} broken actually,
  then the \meta{graphical code} is added to the box drawing process for
  the \emph{first} part of the break sequence.
  \refKey{/tcb/overlay} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}{overlay middle}{=\meta{graphical code}}{no default, initially unset}
  If the box is set to be \refKey{/tcb/breakable} and \emph{is} broken actually,
  then the \meta{graphical code} is added to the box drawing process for
  the \emph{middle} parts (if any) of the break sequence.
  \refKey{/tcb/overlay} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}{overlay last}{=\meta{graphical code}}{no default, initially unset}
  If the box is set to be \refKey{/tcb/breakable} and \emph{is} broken actually,
  then the \meta{graphical code} is added to the box drawing process for
  the \emph{last} part of the break sequence.
  \refKey{/tcb/overlay} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}{overlay unbroken and first}{=\meta{graphical code}}{no default, initially unset}
  This is an optimized abbreviation for setting
  \refKey{/tcb/overlay unbroken} and
  \refKey{/tcb/overlay first} together.
  \refKey{/tcb/overlay} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}{overlay middle and last}{=\meta{graphical code}}{no default, initially unset}
  This is an optimized abbreviation for setting
  \refKey{/tcb/overlay middle} and
  \refKey{/tcb/overlay last} together.
  \refKey{/tcb/overlay} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}{overlay unbroken and last}{=\meta{graphical code}}{no default, initially unset}
  This is an optimized abbreviation for setting
  \refKey{/tcb/overlay unbroken} and
  \refKey{/tcb/overlay last} together.
  \refKey{/tcb/overlay} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-09-19]{overlay first and middle}{=\meta{graphical code}}{no default, initially unset}
  This is an optimized abbreviation for setting
  \refKey{/tcb/overlay first} and
  \refKey{/tcb/overlay middle} together.
  \refKey{/tcb/overlay} overwrites this key.
\end{docTcbKey}


\begin{dispListing*}{breakable,vfill before first,before upper={This example demonstrates
the application of break sequence specific overlay options.
Here, we define an environment |myexample| based
on |tcolorbox| where the visible drawing is done totally by overlay keys.\par
Here, the first application of |myexample| produces an unbroken |tcolorbox|.
The frame is drawn by the code given with \refKey{/tcb/overlay unbroken}.\par
The second application of |myexample| is broken into several parts which
are drawn by the codes given with
\refKey{/tcb/overlay first}, \refKey{/tcb/overlay middle}, and
\refKey{/tcb/overlay last}.
\par\bigskip
}}
% Preamble:
%\usepackage{tikz,lipsum}
%\tcbuselibrary{skins,breakable}
%\newcounter{example}
\colorlet{colexam}{red!75!black}
\newtcolorbox[use counter=example]{myexample}{%
  empty,title={Example \thetcbcounter},attach boxed title to top left,
  boxed title style={empty,size=minimal,toprule=2pt,top=4pt,
    overlay={\draw[colexam,line width=2pt]
      ([yshift=-1pt]frame.north west)--([yshift=-1pt]frame.north east);}},
  coltitle=colexam,fonttitle=\Large\bfseries,
  before=\par\medskip\noindent,parbox=false,boxsep=0pt,left=0pt,right=3mm,top=4pt,
  breakable,pad at break*=0mm,vfill before first,
  overlay unbroken={\draw[colexam,line width=1pt]
    ([yshift=-1pt]title.north east)--([xshift=-0.5pt,yshift=-1pt]title.north-|frame.east)
    --([xshift=-0.5pt]frame.south east)--(frame.south west); },
  overlay first={\draw[colexam,line width=1pt]
    ([yshift=-1pt]title.north east)--([xshift=-0.5pt,yshift=-1pt]title.north-|frame.east)
    --([xshift=-0.5pt]frame.south east); },
  overlay middle={\draw[colexam,line width=1pt] ([xshift=-0.5pt]frame.north east)
    --([xshift=-0.5pt]frame.south east); },
  overlay last={\draw[colexam,line width=1pt] ([xshift=-0.5pt]frame.north east)
    --([xshift=-0.5pt]frame.south east)--(frame.south west);},%
}

\begin{myexample}
\lipsum[1]
\end{myexample}

\begin{myexample}
\lipsum[2-11]
\end{myexample}

\lipsum[12]% following text
\end{dispListing*}
{\tcbusetemp}


%\begin{dispExample}
%% \tcbuselibrary{skins}
%% \newcounter{example}
%\newtcolorbox[use counter=example]{FancyTitle}[3][]{%
%  enhanced,colback=blue!10!white,colframe=orange,top=4mm,
%  enlarge top by=\baselineskip/2+1mm,
%  enlarge top at break by=0mm,pad at break=2mm,
%  fontupper=\normalsize,label={#3},
%  overlay unbroken and first={%
%    \node[rectangle,rounded corners,draw=black,fill=blue!20!white,
%      inner sep=1mm,anchor=west,font=\small]
%      at ([xshift=4.5mm]frame.north west)
%         {\strut\textbf{Example \thetcbcounter: #2}};},
%  #1}%

%\begin{FancyTitle}{My fancy title}{fancy:title}
%  \lipsum[1]
%\end{FancyTitle}
%\end{dispExample}

\clearpage
\subsection{Floating Objects}
\begin{docTcbKey}{floatplacement}{=\meta{values}}{no default, initially \texttt{htb}}
  Sets \meta{values} as default values for the usage of \refKey{/tcb/float}
  and \refKey{/tcb/float*}.
  Feasible are the usual parameters for floating objects.
\begin{dispListing}
\tcbset{enhanced,colback=red!5!white,colframe=red!75!black,
   watermark color=red!15!white}

\begin{tcolorbox}[floatplacement=t,float,
                  title=Floating box from |floatplacement|,
                  watermark text={I am floating}]
  This floating box is placed at the top of a page.
\end{tcolorbox}
\end{dispListing}
\end{docTcbKey}
{\tcbusetemp}


\begin{docTcbKey}{float}{\colOpt{=\meta{values}}}{default from \texttt{floatplacement}}
  Turns the box to a floating object where \meta{values} are the
  usual parameters for such floating objects.
  If they are not used, the placement uses the default values given by
 |floatplacement|.
\begin{dispListing}
\begin{tcolorbox}[float, title=Floating box from |float|,
    enhanced,watermark text={I'm also floating}]
  This box floats to a feasible place automatically. You do not have to
  use a numbering for this floating object.
\end{tcolorbox}
\end{dispListing}
\end{docTcbKey}
{\tcbusetemp}


\begin{docTcbKey}{float*}{\colOpt{=\meta{values}}}{default from \texttt{floatplacement}}
  Identical to \refKey{/tcb/float}, but for wide boxes spanning the whole page
  width of two column documents or in conjunction with the packages
  |multicol| or |paracol|. Note that you have to set |width=\textwidth|
  additionally, if the box should span the whole page width in these cases!
\begin{dispListing}
\begin{tcolorbox}[float*=b, title=Floating box from |float*|,width=\textwidth,
    enhanced,watermark text={I'm also floating}]
  In this single column document, you will see no difference to |float|.
\end{tcolorbox}
\end{dispListing}
\end{docTcbKey}
{\tcbusetemp}


\begin{docTcbKey}{nofloat}{}{style, initially set}
  Turns the floating behavior off.
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2014-09-19]{every float}{=\meta{code}}{no default, initially empty}
  For floating objects, the \refKey{/tcb/before} and \refKey{/tcb/after}
  settings are ignored. Instead, the given \meta{code} is inserted before
  a floating box. If the box is \refKey{/tcb/breakable}, the given \meta{code} is
  inserted before every part of the break sequence.
  The most common use case is |every float=\centering|.

\begin{dispListing}
\tcbox[float=htb,title={Floating box},every float=\centering,
  colback=blue!50!black,colframe=blue!50!white,colbacktitle=blue!10!white,
  coltitle=black,center title]
  {\includegraphics[height=6cm]{lichtspiel.jpg}}
\end{dispListing}
{\tcbset{reset}\tcbusetemp}

\end{docTcbKey}



\clearpage
\subsection{Embedding into the Surroundings}\label{subsec:surroundings}
Typically, but not necessarily, a |tcolorbox| is put inside a separate paragraph
and has some vertical space before and after it.
This behavior is controlled by the keys |before| and |after|.

\begin{docTcbKey}{before}{=\meta{code}}{no default, initially see \refKey{/tcb/autoparskip}}
  Sets the \meta{code} which is executed before the colored box.
  It is not used for floating boxes.
  Also, it is not used, if the box follows a heading immediately
  and \refKey{/tcb/ignore nobreak} is set to \docValue{false}.
\end{docTcbKey}

\begin{docTcbKey}{after}{=\meta{code}}{no default, initially see \refKey{/tcb/autoparskip}}
  Sets the \meta{code} which is executed after the colored box.
  It is not used for floating boxes.
\end{docTcbKey}

\begin{docTcbKey}[][doc updated=2017-02-01]{parskip}{}{style, no value}
  Sets the keys |before| and |after| to values which are
  recommended, if the package |parskip| \emph{is} used and there is no better
  idea for |before| and |after|. This is similar to:
\begin{dispListing}
\tcbset{parskip/.style={before={\par\pagebreak[0]\parindent=0pt},
                        after={\par}}}
\end{dispListing}
\end{docTcbKey}

\begin{docTcbKey}[][doc updated=2017-02-01]{noparskip}{}{style, no value}
  Sets the keys |before| and |after| to values which are
  recommended, if the package |parskip| is \emph{not} used and there is no better
  idea for |before| and |after|. This is similar to:
\begin{dispListing}
\tcbset{noparskip/.style={before={\par\pagebreak[0]\smallskip\parindent=0pt},
                          after={\par\smallskip}}}
\end{dispListing}
\end{docTcbKey}

\begin{docTcbKey}{autoparskip}{}{style, no value, initially set}
  Tries to detect the usage of the package |parskip| and sets
  the keys |before| and |after| accordingly. Actually, the following is done:
  \begin{itemize}
  \item If the length of |\parskip| is greater than |0pt| at the beginning of the document,
    \refKey{/tcb/parskip} is executed. Here, the usage of package |parskip| is \emph{assumed}.
  \item Otherwise, if the length of |\parskip| is not greater than |0pt| at the beginning of the document,
    \refKey{/tcb/noparskip} is executed. Here, the absence of package |parskip| is \emph{assumed}.
  \end{itemize}
  |autoparskip| is the default for the package |tcolorbox|, if |before| or |after|
  are not changed otherwise.
\end{docTcbKey}

\begin{docTcbKey}{nobeforeafter}{}{style, no value}
  Abbreviation for clearing the keys |before| and |after|. The colored box
  is not put into a paragraph and there is no space before or after the box.
\begin{exdispExample}{nobeforeafter}
\tcbset{myone/.style={colback=LightGreen,colframe=DarkGreen,
  equal height group=nobefaf,width=\linewidth/4,nobeforeafter}}
\begin{tcolorbox}[myone,title=Box 1]Box 1\end{tcolorbox}%
\begin{tcolorbox}[myone,title=Box 2]Box 2\end{tcolorbox}%
\begin{tcolorbox}[myone,title=Box 3]Box 3\end{tcolorbox}%
\begin{tcolorbox}[myone,title=Box 4]Box 4\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\enlargethispage*{1cm}
\begin{docTcbKey}{forces nobeforeafter}{}{style, no value}
  Forces the setting of \refKey{/tcb/nobeforeafter} even if
  \refKey{/tcb/before} and \refKey{/tcb/after} are set to other values
  later. Do not use this option globally unless you \emph{really} know what you do.
  Note that embedded boxes do not inherit this forced clearance.
\end{docTcbKey}


\clearpage

\begin{docTcbKey}{baseline}{=\meta{length}}{no default, initially |0pt|}
  Used to set the |\pgfsetbaseline| value of the resulting |tcolorbox|.
\begin{exdispExample}{baseline}
\tcbset{colframe=red!50!white,width=4cm,nobeforeafter}
Some text\dotfill
\begin{tcolorbox}[baseline=3mm]
One line.
\end{tcolorbox}
\begin{tcolorbox}[baseline=3mm]
First line.\\Second line.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2014-10-10]{box align}{=\meta{alignment}}{style, no default, initially |bottom|}
  Used to set the \refKey{/tcb/baseline} value of the resulting |tcolorbox|.
  Feasible values for \meta{alignment} are:
  \begin{itemize}
  \item\docValue{bottom}: alignment with the box bottom,
  \item\docValue{top}: alignment with the box top,
  \item\docValue{center}: alignment with the box center,
  \item\docValue{base}: alignment with the box content base. This option
    is not applicable for a \refEnv{tcolorbox} but for a \refCom{tcbox} only.
    It is an alias for \refKey{/tcb/tcbox raise base}.
  \end{itemize}

\begin{exdispExample}{box_align_1}
\tcbset{colframe=red!50!white,width=4cm,nobeforeafter}
Some text\dotfill
\begin{tcolorbox}[box align=bottom]
One line.
\end{tcolorbox}
\begin{tcolorbox}[box align=bottom]
First line.\\Second line.
\end{tcolorbox}
\end{exdispExample}

\begin{exdispExample}{box_align_2}
\tcbset{colframe=red!50!white,width=4cm,nobeforeafter}
Some text\dotfill
\begin{tcolorbox}[box align=top]
One line.
\end{tcolorbox}
\begin{tcolorbox}[box align=top]
First line.\\Second line.
\end{tcolorbox}
\end{exdispExample}

\begin{exdispExample}{box_align_3}
\tcbset{colframe=red!50!white,width=4cm,nobeforeafter}
Some text\dotfill
\begin{tcolorbox}[box align=center]
One line.
\end{tcolorbox}
\begin{tcolorbox}[box align=center]
First line.\\Second line.
\end{tcolorbox}
\end{exdispExample}

\begin{exdispExample}{box_align_4}
\tcbset{colframe=red!50!white,nobeforeafter}
Some text\dotfill
\tcbox[nobeforeafter,box align=base]{One line}
\tcbox[nobeforeafter,box align=base,size=fbox]{Another line}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new and updated={2014-10-10}{2015-03-16}]{before skip}{=\meta{glue}}{style, no default}
  Inserts some vertical space of the given \meta{glue} before the colored box.
  This style sets \refKey{/tcb/before}.
\begin{exdispExample*}{before_skip}{sbs,lefthand ratio=0.6}
Some text.
\begin{tcolorbox}[before skip=1cm,
    colframe=red!50!white]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\begin{docTcbKey}[][doc new and updated={2014-10-10}{2017-02-01}]{after skip}{=\meta{glue}}{style, no default}
  Inserts some vertical space of the given \meta{glue} after the colored box.
  This style sets \refKey{/tcb/after}.
\begin{exdispExample*}{after_skip}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[after skip=1cm,
    colframe=red!50!white]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
Some text.
\end{exdispExample*}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-10-10]{beforeafter skip}{=\meta{glue}}{style, no default}
  Inserts some vertical space of the given \meta{glue} before \emph{and} after the colored box.
  This style sets \refKey{/tcb/before} and \refKey{/tcb/after}.
\begin{exdispExample*}{beforeafter_skip}{sbs,lefthand ratio=0.6}
\tcbset{beforeafter skip=0pt,
  colframe=red!50!white}
\begin{tcolorbox}
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\begin{tcolorbox}
  Second box.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\clearpage

\begin{docTcbKey}[][doc new=2014-11-07]{left skip}{=\meta{length}}{style, no default, initially |0mm|}
  Inserts some horizontal space of the given \meta{length} before the colored box.
  This style sets \refKey{/tcb/grow to left by} with the negated \meta{length},
  i.e. the bounding box and box width are changed.
\begin{exdispExample*}{left_skip}{sbs,lefthand ratio=0.6}
\noindent\rule{\linewidth}{2pt}

\begin{tcolorbox}[left skip=1cm,
    colframe=red!50!white]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-11-07]{right skip}{=\meta{length}}{style, no default, initially |0mm|}
  Inserts some horizontal space of the given \meta{length} after the colored box.
  This style sets \refKey{/tcb/grow to right by} with the negated \meta{length},
  i.e. the bounding box and box width are changed.
\begin{exdispExample*}{right_skip}{sbs,lefthand ratio=0.6}
\noindent\rule{\linewidth}{2pt}

\begin{tcolorbox}[right skip=1cm,
    colframe=red!50!white]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-10-10]{leftright skip}{=\meta{length}}{style, no default}
  Inserts some horizontal space of the given \meta{length} before \emph{and} after the colored box.
  This style changes the bounding box and the box width.
\begin{exdispExample*}{leftright_skip}{sbs,lefthand ratio=0.6}
\noindent\rule{\linewidth}{2pt}

\begin{tcolorbox}[leftright skip=1cm,
    colframe=red!50!white]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2014-12-11]{ignore nobreak}{\colOpt{=true\textbar false}}{default |true|, initially |false|}
After a heading, \LaTeX\ tries to avoid a break by setting a |nobreak| boolean value.
Starting from version |3.33|, the \refKey{/tcb/before} respectively \refKey{/tcb/before skip}
settings are not used after a heading if \refKey{/tcb/ignore nobreak} is
set to \docValue{false}. For an unbreakable box, \refKey{/tcb/before nobreak} is used instead.
Further, a \refKey{/tcb/breakable} box will also try to
avoid a break between a heading and a directly following first part of a
break sequence.

Set \refKey{/tcb/ignore nobreak} to \docValue{true}, if |nobreak| should be
ignored as prior to version |3.33|. Also, such a setting may be used locally to
enforce the \refKey{/tcb/before} setting.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-12-16]{before nobreak}{=\meta{code}}{no default, initially \cs{noindent}}
  Sets the \meta{code} which is executed before the colored box if it
  is unbreakable, if \refKey{/tcb/ignore nobreak} is not set, and if
  the box follows a heading.
\end{docTcbKey}

\enlargethispage*{1cm}

\begin{docTcbKey}[][doc new=2017-02-23]{parfillskip restore}{\colOpt{=true\textbar false}}{default |true|, initially |true|}
  If this option is set to be |true|, the minimum value of |\parfillskip| is
  tested at specific spots, if it is greater than |0pt|.
  If so, |\parfillskip| is restored to |\@flushglue| which happens to be
  the default value.

  These tests are executed for
  \refKey{/tcb/parskip},
  \refKey{/tcb/noparskip},
  \refKey{/tcb/after skip},
  \refKey{/tcb/breakable}, and
  \refEnv{tcbraster}.

  This option was created to automatically
  avoid overfull box warnings with |\parfillskip| changing packages.
\end{docTcbKey}



\clearpage
\subsection{Bounding Box}
Normally, every |tcolorbox| has a bounding box which fits exactly to the
dimensions of the outer frame. Therefore, \LaTeX\ reserves exactly the space
needed for the box.
This behavior can be changed by enlarging (or shrinking) the bounding box.
If the bounding box is enlarged, the |tcolorbox| will get some clearance
around it. If the bounding box is shrunk, i.\,e.\ enlarged with negative
values, the |tcolorbox| will overlap to other parts of the page.
For example, the |tcolorbox| could be stretched into the page margin.

\begin{marker}
The following examples use \refKey{/tcb/show bounding box} to display the
actual bounding box. For this, the library \mylib{skins} has to be included and
\refKey{/tcb/enhanced} has to be set.
\end{marker}

\subsubsection{Shifting Bounding Box Borders}

\begin{docTcbKey}{enlarge top initially by}{=\meta{length}}{no default, initially |0mm|}
  Enlarges the bounding box distance to the top of the box by \meta{length}.
  If the box is \emph{breakable}, only the first box of the break sequence
  gets enlarged. \refKey{/tcb/enlarge top by} overwrites this key.
\begin{exdispExample}{enlarge_top_initially_by}
\tcbset{colframe=blue!75!black,colback=white}

\begin{tcolorbox}[enlarge top initially by=-5mm]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\begin{tcolorbox}[enlarge top initially by=5mm,enhanced,show bounding box]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}



\begin{docTcbKey}{enlarge bottom finally by}{=\meta{length}}{no default, initially |0mm|}
  Enlarges the bounding box distance to the bottom of the box by \meta{length}.
  If the box is \emph{breakable}, only the last box of the break sequence
  gets enlarged. \refKey{/tcb/enlarge bottom by} overwrites this key.
\begin{exdispExample}{enlarge_bottom_finally_by}
\tcbset{colframe=blue!75!black,colback=white}

\begin{tcolorbox}[enlarge bottom finally by=5mm]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\begin{tcolorbox}[enlarge bottom finally by=-5mm,enhanced,show bounding box]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\clearpage


\begin{docTcbKey}{enlarge top at break by}{=\meta{length}}{no default, initially \texttt{0mm}}
  Enlarges the bounding box distance to the top of the box by \meta{length},
  \emph{if} the box is \refKey{/tcb/breakable}.
  In this case, it is applied to \emph{middle} and \emph{last} parts in a
  break sequence.
  \refKey{/tcb/enlarge top by} overwrites this key.
\end{docTcbKey}


\begin{docTcbKey}{enlarge bottom at break by}{=\meta{length}}{no default, initially \texttt{0mm}}
  Enlarges the bounding box distance to the bottom of the box by \meta{length},
  \emph{if} the box is \refKey{/tcb/breakable}.
  In this case, it is applied to \emph{first} and \emph{middle} parts in a
  break sequence. \refKey{/tcb/enlarge bottom by} overwrites this key.
\end{docTcbKey}


\begin{docTcbKey}{enlarge top by}{=\meta{length}}{no default, initially |0mm|}
  Enlarges the bounding box distance to the top of the box by \meta{length}.
  \refKey{/tcb/enlarge top initially by} and
  \refKey{/tcb/enlarge top at break by} are set to \meta{length}.
\end{docTcbKey}


\begin{docTcbKey}{enlarge bottom by}{=\meta{length}}{no default, initially |0mm|}
  Enlarges the bounding box distance to the bottom of the box by \meta{length}.
  \refKey{/tcb/enlarge bottom finally by} and
  \refKey{/tcb/enlarge bottom at break by} are set to \meta{length}.
\end{docTcbKey}


\begin{docTcbKey}{enlarge left by}{=\meta{length}}{no default, initially |0mm|}
  Enlarges the bounding box distance to the left side of the box by \meta{length}.
\begin{exdispExample}[safety=2cm]{enlarge_left_by}
\tcbset{colframe=blue!75!black,colback=white}

\begin{tcolorbox}[enlarge left by=2cm,width=5cm,enhanced,show bounding box]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\begin{tcolorbox}[enlarge left by=-2cm,width=\linewidth+2cm]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\begin{docTcbKey}{enlarge right by}{=\meta{length}}{no default, initially |0mm|}
  Enlarges the bounding box distance to the right side of the box by \meta{length}.
\begin{exdispExample}[safety=2cm]{enlarge_right_by}
\tcbset{colframe=blue!75!black,colback=white}

\begin{tcolorbox}[enlarge right by=-2cm,width=\linewidth+2cm,
  enhanced,show bounding box]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\begin{tcolorbox}[enlarge right by=2cm,width=\linewidth-2cm]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{enlarge by}{=\meta{length}}{no default, initially |0mm|}
  Enlarges the bounding box distance to all sides of the box by \meta{length}.
\begin{exdispExample}{enlarge_by}
\tcbset{colframe=blue!75!black,colback=white,width=5cm,nobeforeafter}

\begin{tcolorbox}
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\begin{tcolorbox}[enlarge by=5mm,enhanced,show bounding box]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}



\begin{docTcbKey}{grow to left by}{=\meta{length}}{no default, initially |0mm|}
  Enlarges the current box width by \meta{length} and
  enlarges (shrinks) the bounding box distance to the left side of the box by
  $-$\meta{length}. Also see \refKey{/tcb/left skip}.
\begin{exdispExample}[safety=2cm]{grow_to_left_by}
\tcbset{colframe=blue!75!black,colback=white}

\begin{tcolorbox}[width=5cm,grow to left by=2cm,enhanced,show bounding box]
This is a \textbf{tcolorbox} with a width of 7cm.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\begin{docTcbKey}{grow to right by}{=\meta{length}}{no default, initially |0mm|}
  Enlarges the current box width by \meta{length} and
  enlarges (shrinks) the bounding box distance to the right side of the box by
  $-$\meta{length}. Also see \refKey{/tcb/right skip}.
\begin{exdispExample}[safety=2cm]{grow_to_right_by}
\tcbset{colframe=blue!75!black,colback=white}

\begin{tcolorbox}[grow to right by=2cm,enhanced,show bounding box]
This is a \textbf{tcolorbox}.
\end{tcolorbox}

\bigskip

\begin{tcolorbox}[grow to right by=2cm,grow to left by=1cm,
  enhanced,show bounding box]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}

\clearpage

\begin{docTcbKey}[][doc new=2018-03-22]{grow sidewards by}{=\meta{length}}{no default, initially |0mm|}
  Shortcut for setting \refKey{/tcb/grow to left by} and \refKey{/tcb/grow to right by}
  to \meta{length}. Also see \refKey{/tcb/oversize} and \refKey{/tcb/spread sidewards}.
\begin{exdispExample}[safety=2cm]{grow_sidewards_by}
\tcbset{colframe=blue!75!black,colback=white}

\begin{tcolorbox}[grow sidewards by=2cm,enhanced,show bounding box]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\subsubsection{Box Alignment}

\begin{docTcbKey}[][doc new=2015-11-20]{flush left}{}{style, no value}
  Enlarges the bounding box to the right side to fill the line completely.
\begin{exdispExample}{flush_left}
\tcbset{colframe=blue!75!black,colback=white}

\begin{tcolorbox}[flush left,width=5cm,enhanced,show bounding box]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2015-11-20]{flush right}{}{style, no value}
  Enlarges the bounding box to the left side to fill the line completely.
\begin{exdispExample}{flush_right}
\tcbset{colframe=blue!75!black,colback=white}

\begin{tcolorbox}[flush right,width=5cm,enhanced,show bounding box]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2015-11-20]{center}{}{style, no value}
  Enlarges the bounding box equally to both sides to fill the line completely.
\begin{exdispExample}{center}
\tcbset{colframe=blue!75!black,colback=white}

\begin{tcolorbox}[center,width=5cm,enhanced,show bounding box]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\clearpage
\subsubsection{Toggle Enlargements}

\begin{docTcbKey}[][doc updated=2015-11-13]{toggle enlargement}{=\meta{toggle preset}}{default |evenpage|, initially |none|}
  According to the \meta{toggle preset}, the left and the right enlargements of
  the bounding box are switched or not. Feasible values are:
  \begin{itemize}
  \item\docValue{none}: no switching.
  \item\docValue{forced}: the values of the left and right enlargement are switched.
  \item\docValue{evenpage}: if the page is an even page, the values of the left and
    right enlargement are switched. This value also sets
    \refKey{/tcb/check odd page} to |true|.
  \end{itemize}
\begin{marker}
See \refKey{/tcb/toggle left and right} to toggle geometry settings.
\end{marker}

\begin{dispExample}
\tcbset{colframe=blue!75!black,colback=white,
  grow to left by=20mm,grow to right by=-5mm}

\begin{tcolorbox}[toggle enlargement=none,enhanced,show bounding box]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\begin{tcolorbox}[toggle enlargement=forced]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\begin{tcolorbox}[toggle enlargement=evenpage]
  This page is an \tcbifoddpage{odd}{even} page.
  Therefore, the left and right enlargements
  \tcbifoddpage{are not}{are} toggled.
\end{tcolorbox}
\end{dispExample}

\begin{dispListing}
\begin{tcolorbox}[colframe=red!60!black,colback=red!15!white,
  fonttitle=\bfseries,title=Floating box from \texttt{toggle enlargement},
  width=\textwidth,grow to right by=2cm,toggle enlargement,float=t]
  This page is an \tcbifoddpage{odd}{even} page.
  Therefore, the left and right enlargements \tcbifoddpage{are not}{are} toggled.
  This box stretches to the right margin on odd pages and to the left
  margin on even pages. The current document is one-sided -- this feature makes
  sense for two-sided documents only.
\end{tcolorbox}
\end{dispListing}
\tcbusetemp
\end{docTcbKey}



\clearpage
\subsubsection{Spread Box to Page Borders}

\begin{marker}
The following border options are \emph{not} applicable to nested boxes, boxes insides
tables, etc.
For boxes inside lists, the options \emph{may} work, but not necessarily.
Also, boxes should be set with |\noindent| and full width.
\end{marker}

\begin{docTcbKey}[][doc new=2017-02-13]{spread inwards}{\colOpt{=\meta{length}}}{default |0pt|, initially unset}
Enlarges the current box width to match the inner page border (left-handed side for one-sided
documents). If the optional \meta{length} is greater than |0pt|, the box
grows over the border, if \meta{length} is lower than |0pt|, there is a
margin between box and page border.
\refKey{/tcb/toggle enlargement} is set automatically.
\begin{dispListing}
\begin{tcolorbox}[enhanced,spread inwards,
  colframe=blue!75!black,colback=white,show bounding box]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{dispListing}
{\tcbusetemp}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2017-02-13]{spread outwards}{\colOpt{=\meta{length}}}{default |0pt|, initially unset}
Enlarges the current box width to match the outer page border (right-handed side for one-sided
documents). If the optional \meta{length} is greater than |0pt|, the box
grows over the border, if \meta{length} is lower than |0pt|, there is a
margin between box and page border.
\refKey{/tcb/toggle enlargement} is set automatically.
\begin{dispListing}
\begin{tcolorbox}[enhanced,spread outwards,
  colframe=blue!75!black,colback=white,show bounding box]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{dispListing}
{\tcbusetemp}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2017-02-13]{move upwards}{\colOpt{=\meta{length}}}{default |0pt|, initially unset}
Starts a new page with the box at the very top page border.
If the optional \meta{length} is greater than |0pt|, the box
moves over the border, if \meta{length} is lower than |0pt|, there is a
margin between box and page border.
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2017-02-13]{move upwards*}{\colOpt{=\meta{length}}}{default |0pt|, initially unset}
Identical to \refKey{/tcb/move upwards}, but without starting a new page.
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2017-02-13]{fill downwards}{\colOpt{=\meta{length}}}{default |0pt|, initially unset}
Enlarges the height of the box until the very bottom page border.
The library \mylib{breakable} has to be loaded, and
\refKey{/tcb/height fill} is set automatically.
If the optional \meta{length} is greater than |0pt|, the box
moves over the border, if \meta{length} is lower than |0pt|, there is a
margin between box and page border.
\begin{dispListing}
\begin{tcolorbox}[enhanced,fill downwards,
  colframe=blue!75!black,colback=white,show bounding box]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{dispListing}
{\tcbusetemp}
\end{docTcbKey}


\begin{tcolorbox}[enhanced,spread upwards,sharp corners=north,height=3cm,
  colframe=blue!75!black,interior style={top color=blue!50,bottom color=white}]
This is an example for 'spread upwards'.
\end{tcolorbox}
\begin{docTcbKey}[][doc new=2017-02-13]{spread upwards}{\colOpt{=\meta{length}}}{default |0pt|, initially unset}
Combination of
\refKey{/tcb/move upwards}, \refKey{/tcb/spread inwards}, and \refKey{/tcb/spread outwards}.
The optional \meta{length} is used for all these keys.
\begin{dispListing}
\begin{tcolorbox}[enhanced,spread upwards,sharp corners=north,height=3cm,
  colframe=blue!75!black,interior style={top color=blue!50,bottom color=white}]
This is an example for 'spread upwards'.
\end{tcolorbox}
\end{dispListing}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2017-02-13]{spread upwards*}{\colOpt{=\meta{length}}}{default |0pt|, initially unset}
Identical to \refKey{/tcb/move upwards}, but without starting a new page.
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2017-02-13]{spread sidewards}{\colOpt{=\meta{length}}}{default |0pt|, initially unset}
Combination of \refKey{/tcb/spread inwards} and \refKey{/tcb/spread outwards}.
The optional \meta{length} is used for all these keys.
Also see \refKey{/tcb/oversize} and \refKey{/tcb/grow sidewards by}.
\begin{dispListing}
\begin{tcolorbox}[enhanced,spread sidewards,
  colframe=blue!75!black,colback=white,show bounding box]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{dispListing}
{\tcbusetemp}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2017-02-13]{spread}{\colOpt{=\meta{length}}}{default |0pt|, initially unset}
Combination of
\refKey{/tcb/move upwards}, \refKey{/tcb/fill downwards}, \refKey{/tcb/spread inwards},
and \refKey{/tcb/spread outwards}.
Such, the box fills the whole page.
The optional \meta{length} is used for all these keys.
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2017-02-13]{spread downwards}{\colOpt{=\meta{length}}}{default |0pt|, initially unset}
Combination of
\refKey{/tcb/fill downwards}, \refKey{/tcb/spread inwards}, and \refKey{/tcb/spread outwards}.
The optional \meta{length} is used for all these keys.
\begin{dispListing}
\begin{tcolorbox}[enhanced,spread downwards,sharp corners=south,
  colframe=red!75!black,interior style={top color=white,bottom color=red!50}]
This is an example for 'spread downwards'.
\end{tcolorbox}
\end{dispListing}
\end{docTcbKey}
\begin{tcolorbox}[enhanced,spread downwards,sharp corners=south,
  colframe=red!75!black,interior style={top color=white,bottom color=red!50}]
This is an example for 'spread downwards'.
\end{tcolorbox}




\clearpage
\subsubsection{Box Extrusion}

\begin{marker}
The following keys should not be used with breakable boxes or boxes with a
lower part.
\end{marker}

\begin{docTcbKey}{shrink tight}{}{style, no value, initially unset}
  The total colored box is shrunk to the dimensions of the upper
  part. There should be no lower part and no title.
  This style sets the \refKey{/tcb/boxsep} to |0pt| and other geometry keys
  to fitting values. This option is likely to be used with the following
  extrusion keys.
\begin{exdispExample}{shrink_tight}
\tcbset{colframe=blue!75!black,colback=white,arc=0mm,boxrule=0.4pt,
        nobeforeafter,tcbox raise base,shrink tight}

\begin{tcolorbox}
This is a \textbf{tcolorbox}.
\end{tcolorbox}

Lorem \tcbox{ipsum} dolor sit amet, consectetuer adipiscing elit.
\end{exdispExample}
\end{docTcbKey}

\begin{docTcbKey}[][doc updated=2014-09-19]{extrude left by}{=\meta{length}}{style, no default, initially unset}
  The (upper part of the) colored box is extruded by the given \meta{length} to the left side.
  The inner width and the bounding box is kept unchanged and the operation
  is additive!
\begin{exdispExample}{extrude_left_by}
\tcbset{enhanced,colframe=red,colback=yellow!25!white,
  frame style={opacity=0.25},interior style={opacity=0.5},
  nobeforeafter,tcbox raise base,shrink tight,extrude by=2mm}

Lorem ipsum dolor sit amet, consectetuer adipiscing elit. Ut purus elit,
vestibulum ut, placerat ac, adipiscing vitae, felis.
\tcbox[extrude left by=1cm]{Curabitur} dictum gravida mauris.
Nam arcu libero, nonummy eget, consectetuer id, vulputate a, magna.
\end{exdispExample}
\end{docTcbKey}

\begin{docTcbKey}[][doc updated=2014-09-19]{extrude right by}{=\meta{length}}{style, no default, initially unset}
  The (upper part of the) colored box is extruded by the given \meta{length} to the right side.
  The inner width and the bounding box is kept unchanged and the operation
  is additive!
\begin{exdispExample}{extrude_right_by}
\tcbset{enhanced,colframe=red,colback=yellow!25!white,
  frame style={opacity=0.25},interior style={opacity=0.5},
  nobeforeafter,tcbox raise base,shrink tight,extrude by=2mm}

Lorem ipsum dolor sit amet, consectetuer adipiscing elit. Ut purus elit,
vestibulum ut, placerat ac, adipiscing vitae, felis.
\tcbox[extrude right by=1cm]{Curabitur} dictum gravida mauris.
Nam arcu libero, nonummy eget, consectetuer id, vulputate a, magna.
\end{exdispExample}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{extrude top by}{=\meta{length}}{style, no default, initially unset}
  The (upper part of the) colored box is extruded by the given \meta{length} to the top side.
  The inner width and the bounding box is kept unchanged and the operation
  is additive!
\begin{exdispExample}{extrude_top_by}
\tcbset{enhanced,colframe=red,colback=yellow!25!white,
  frame style={opacity=0.25},interior style={opacity=0.5},
  nobeforeafter,tcbox raise base,shrink tight,extrude by=2mm}

Lorem ipsum dolor sit amet, consectetuer adipiscing elit. Ut purus elit,
vestibulum ut, placerat ac, adipiscing vitae, felis.
\tcbox[extrude top by=1cm]{Curabitur} dictum gravida mauris.
Nam arcu libero, nonummy eget, consectetuer id, vulputate a, magna.
\end{exdispExample}
\end{docTcbKey}

\begin{docTcbKey}{extrude bottom by}{=\meta{length}}{style, no default, initially unset}
  The (upper part of the) colored box is extruded by the given \meta{length} to the bottom side.
  The inner width and the bounding box is kept unchanged and the operation
  is additive!
\begin{exdispExample}[safety=1cm]{extrude_bottom_by}
\tcbset{enhanced,colframe=red,colback=yellow!25!white,
  frame style={opacity=0.25},interior style={opacity=0.5},
  nobeforeafter,tcbox raise base,shrink tight,extrude by=2mm}

Lorem ipsum dolor sit amet, consectetuer adipiscing elit. Ut purus elit,
vestibulum ut, placerat ac, adipiscing vitae, felis.
\tcbox[extrude bottom by=1cm]{Curabitur} dictum gravida mauris.
Nam arcu libero, nonummy eget, consectetuer id, vulputate a, magna.
\end{exdispExample}
\end{docTcbKey}

\begin{docTcbKey}{extrude by}{=\meta{length}}{style, no default, initially unset}
  The (upper part of the) colored box is extruded by the given \meta{length} to all sides.
  The inner width and the bounding box is kept unchanged and the operation
  is additive!
\begin{exdispExample}{extrude_by}
\tcbset{enhanced,colframe=red,colback=yellow!25!white,
  frame style={opacity=0.25},interior style={opacity=0.5},
  nobeforeafter,tcbox raise base,shrink tight,extrude by=2mm}

Lorem ipsum dolor sit amet, consectetuer adipiscing elit. Ut purus elit,
vestibulum ut, placerat ac, adipiscing vitae, felis. \tcbox{Curabitur} dictum
gravida mauris. \tcbox[colframe=Green,interior style={opacity=0.0}]{Nam}
arcu libero, nonummy eget, consectetuer id, \tcbox{vulputate} a, magna. Donec
vehicula augue eu neque. Pellentesque habitant morbi tristique senectus et netus
et malesuada fames ac turpis egestas. \tcbox{Mauris ut leo.}
\end{exdispExample}
\end{docTcbKey}

\clearpage
\subsection{Layered Boxes and Every Box Settings}\label{subsec:everybox}
A |tcolorbox| may contain another |tcolorbox| and so on. The package
takes track of the nesting level using a counter |tcblayer|. Counter values
may be used for doing some fancy things, but you should never change
the counter value yourself.

The package takes special care for the first four layers or nesting levels,
called managed layers.
Here, footnote texts are administrated to find their intended place
and specific layer dependent options may be set by changing
\refKey{/tcb/every box on layer n}.
If needed, the number of managed layers can be increased by setting
\refCom{tcbsetmanagedlayers} to a higher value than~4.

The following styles have a considerable influence on how layered boxes
are processed. Note especially that nested boxes are getting a
\refKey{/tcb/reset} by default. You can change this, but be prepared for
surprises if you do.

If the defaults are \emph{not changed}, a |tcolorbox| gets its options
in the following order. Following options overwrite preceding options.
\begin{enumerate}
\item On package load, all options are set to default values.
\item Every \refCom{tcbset} command adds or changes options for the following boxes
  inside the current \TeX\ group.
\item While entering a |tcolorbox|, a \refKey{/tcb/every box on layer n} or
  \refKey{/tcb/every box on higher layers} option list is applied.
  With default settings this means:
  \begin{itemize}
  \item For layer 1 (lowest layer), the \refKey{/tcb/every box} option list is applied.
    Not overwritten options given by a preceding \refCom{tcbset} survive.
  \item For layer 2 and above (nested boxes), a \refKey{/tcb/reset} followed by
    \refKey{/tcb/every box} option list is applied.
    Every resettable options given by a preceding \refCom{tcbset}
    and by the sourrounding box(es) are reset.
  \end{itemize}
\item The \meta{options} given to the |tcolorbox| are applied.
  Or, if the box was generated by \refCom{newtcolorbox} or friends,
  the \meta{options} given there are applied.
\item If the box was generated by \refCom{newtcolorbox} or friends,
  some automated options are applied.
\end{enumerate}


\begin{docTcbKey}{every box}{}{style}
By default, this style is empty.
\begin{dispListing}
% default setting:
\tcbset{every box/.style={}}
\end{dispListing}
It may be changed by redefining this style.
\begin{dispListing}
% setting all boxes to be enhanced:
\tcbset{every box/.style={enhanced}}
\end{dispListing}

\medskip
\begin{marker}
The alternative for setting something for every box (on every layer) is\\
\refCom{tcbsetforeverylayer}:
\begin{dispListing}
% setting all boxes to be enhanced:
\tcbsetforeverylayer{enhanced}
\end{dispListing}
\end{marker}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{every box on layer n}{}{style}
Here, |n| has to be replaced by a number ranging from 1 to the highest
managed layer number (4 by default).
\begin{dispListing}
% default settings:
\tcbset{
  every box on layer 1/.style={every box},
  every box on layer 2/.style={reset,every box},
  every box on layer 3/.style={reset,every box},
  every box on layer 4/.style={reset,every box},
  }
\end{dispListing}
\end{docTcbKey}


\begin{docTcbKey}{every box on higher layers}{}{style}
Higher layers are layers above the highest
managed layer number (4 by default).
\begin{dispListing}
\tcbset{every box on higher layers/.style={reset,every box}}
\end{dispListing}
\end{docTcbKey}


\begin{docCommand}{tcbsetmanagedlayers}{\marg{number}}
Replaces the highest managed layer number by \meta{number} where 4 is
the default. This macro can only be used inside the preamble.
Using a \meta{number} lower than 4 typically makes no sense, but is
not forbidden.
\end{docCommand}

\begin{tcboutputlisting}
% \usepackage{lipsum}
% \tcbuselibrary{skins,breakable}
\tcbset{colframe=red!75!black,fonttitle=\bfseries,
  colback=red!5!white,
  every box/.style={enhanced,watermark text=\thetcblayer,
    before=\par\smallskip,after=\par\smallskip},
  every box on layer 2/.style={reset,every box,colback=yellow!10!white,
    drop fuzzy shadow}}
\begin{tcolorbox}[enhanced jigsaw,breakable,title=Layer 1 Box]
Here comes a footnote\footnote{Footnote from layer 1 box}.
\lipsum[2]
  \begin{tcolorbox}[title=Layer 2 Box]
  abc\footnote{The footnote of abc}
  \end{tcolorbox}
  \begin{tcolorbox}[title=Another Box,ams equation]
    \tcbhighmath{\sum\limits_{n=1}^{\infty} \frac{1}{n}} = \infty.
  \end{tcolorbox}
Some text\footnote{Footnote from some text}.
  \begin{tcolorbox}[title=Yet Another Box]
    \tcboxfit[height=2cm]{\lipsum[1]}
    My text.
    \begin{tcolorbox}
      Another lipsum text\footnote{A lipsum text}. \lipsum[3]
      \begin{tcolorbox}[title=Layer 4,colframe=blue,colback=white]
        Layer 4\footnote{Layer 4 footnote}
      \end{tcolorbox}
      The End\footnote{Last footnote}.
    \end{tcolorbox}
  \end{tcolorbox}
\end{tcolorbox}
\end{tcboutputlisting}

\tcbinputlisting{base example,listing only,listing style=mydocumentation}

{\tcbuselistingtext}


\clearpage
\subsection{Capture Mode}\label{subsec:capture}

\begin{docTcbKey}{capture}{=\meta{mode}}{no default, initially |minipage|}
  The capture \meta{mode} defines how the box content is processed.

Feasible values for \meta{mode} are:
\begin{itemize}
\item\docValue{minipage}:\\
  This is the default \meta{mode} for \refEnv{tcolorbox}.
  The content may have an upper and a lower part. Optionally, the box
  can be \refKey{/tcb/breakable}. The box content is put into a
  minipage or into something similar to a minipage.
\item\docValue{hbox}:\\
  This is the default \meta{mode} for \refCom{tcbox}. The content cannot have
  a lower part and cannot be broken. The colored box is sized according
  to the dimensions of the content.
  A shortcut to set this mode is \refKey{/tcb/hbox}.
\item\docValue{fitbox}: (needs the \mylib{fitting} library)\\
  This is the default \meta{mode} for \refCom{tcboxfit}. The content cannot have
  a lower part and cannot be broken.
  The content is sized according to the dimensions of the colored box.
  A shortcut to set this mode is \refKey{/tcb/fit}.
\end{itemize}

\begin{exdispExample}{capture}
\tcbset{colframe=blue!75!black,colback=white}

\begin{tcolorbox}[capture=minipage]
This is a tcolorbox.
\end{tcolorbox}

\begin{tcolorbox}[capture=hbox]
This is a tcolorbox.
\end{tcolorbox}

\begin{tcolorbox}[capture=fitbox,height=9mm]% needs the 'fitting' library
This is a tcolorbox.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}



\begin{docTcbKey}{hbox}{}{style, no default}
  Shortcut for |capture=hbox|.
\begin{exdispExample}{hbox}
\tcbset{colframe=blue!75!black,colback=white}

\begin{tcolorbox}[hbox]
This is a tcolorbox.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}{minipage}{}{style, no default}
  Shortcut for |capture=minipage|.
\end{docTcbKey}


\clearpage
\subsection{Text Characteristics}
\begin{docTcbKey}[][doc updated=2015-10-14]{parbox}{\colOpt{=true\textbar false}}{default |true|, initially |true|}
  The text inside a |tcolorbox| is formatted using a \LaTeX\ |minipage|
  if the box is unbreakable. If breakable, the box tries a mimicry of
  a |minipage|. In a |minipage| or |parbox|, paragraphs are formatted slightly different
  as the main text. If the key value is set to |false|, the normal main text
  behavior is restored. In some situations, this has some unwanted side
  effects. It is recommended that you use this experimental setting only
  where you really want to have this feature.
\end{docTcbKey}

\begin{dispListing}
% \usepackage{lipsum}  % preamble
\tcbset{width=(\linewidth-2mm)/2,nobeforeafter,arc=1mm,
  colframe=blue!75!black,colback=white,fonttitle=\bfseries,fontupper=\small,
  left=2mm,right=2mm,top=1mm,bottom=1mm,equal height group=parbox}

\begin{tcolorbox}[parbox,adjusted title={parbox=true (normal)}]
  \lipsum[1-2]
\end{tcolorbox}\hfill%
\begin{tcolorbox}[parbox=false,adjusted title={parbox=false}]
  \lipsum[1-2]
\end{tcolorbox}%
\end{dispListing}
{\tcbusetemp}


\clearpage
\begin{docTcbKey}{hyphenationfix}{\colOpt{=true\textbar false}}{default |true|, initially |false|}
  Long words at the beginning of paragraphs in very narrow boxes
  will not be hyphenated using |pdflatex|. This problem is circumvented by
  applying the |hyphenationfix| option.

\begin{exdispExample*}{hyphenationfix}{sbs,lefthand ratio=0.6}
\tcbset{colframe=blue!75!black,
  fontupper=\normalsize,
  colback=blue!5!white,width=4cm}

\begin{tcolorbox}
Rechnungsadjunktentochter.\par
Statthaltereikonzipist.
\end{tcolorbox}

\begin{tcolorbox}[hyphenationfix]
Rechnungsadjunktentochter.\par
Statthaltereikonzipist.
\end{tcolorbox}
\end{exdispExample*}

\smallskip
\begin{marker}
|parbox=false| and |hyphenationfix| should not be used together. They are
targeting different box types and they do not blend very well.
\end{marker}
\end{docTcbKey}


\subsection{Files}
\begin{docTcbKey}{tempfile}{=\meta{file name}}{no default, initially \cs{jobname.tcbtemp}}
  Sets \meta{file name} as name for the temporary file which is used inside
  \refEnv{tcbwritetemp} and \refCom{tcbusetemp} implicitely.
\end{docTcbKey}

\subsection{\texttt{\textbackslash tcbox} Specials}
The following options are applicable for \refCom{tcbox} and \refCom{tcboxmath}
only.

\begin{docTcbKey}{tcbox raise}{=\meta{length}}{no default, initially \texttt{0pt}}
  Raises the \refCom{tcbox} by the given \meta{length}.
 % Sets the line width of the right rule to \meta{length}.
\begin{exdispExample}{tcbox_raise}
\tcbset{colframe=blue!50!black,colback=white,colupper=red!50!black,
        fonttitle=\bfseries,nobeforeafter,center title}

Test\dotfill
\tcbox[tcbox raise base]{Hello World 1}\dotfill
\tcbox{Hello World 2}\dotfill
\tcbox[tcbox raise=5mm]{Hello World 3}
\end{exdispExample}
\end{docTcbKey}

\begin{docTcbKey}{tcbox raise base}{}{style, no value, initially unset}
  Raises the \refCom{tcbox} such that the base of its content matches
  the base of the environmental line; see example above.
\end{docTcbKey}

\begin{docTcbKey}{on line}{}{style, no value, initially unset}
  Combines \refKey{/tcb/tcbox raise base} with \refKey{/tcb/nobeforeafter}.
  The resulting box behaves analogue to |\fbox|.
\end{docTcbKey}

\clearpage
\begin{docTcbKey}[][doc new=2015-03-23]{tcbox width}{=\meta{mode}}{no default, initially \texttt{auto}}
Controls how \refCom{tcbox} respects a \refKey{/tcb/width} setting.
Feasible values for \meta{mode} are:
\begin{itemize}
\item\docValue{auto} (initial setting):
  ignore \refKey{/tcb/width} and set box width according to its content.
\item\docValue{auto limited}:
  Set box width according to its content, if it is smaller than \refKey{/tcb/width}.
  Otherwise, the content is set like in a \refEnv{tcolorbox} with line breaks.
\item\docValue{forced center}:
  Set box width according to \refKey{/tcb/width}.
  The content is centered and may overlap the box borders.
\item\docValue{forced left}:
  Set box width according to \refKey{/tcb/width}.
  The content is left aligned and may overlap the box borders.
\item\docValue{forced right}:
  Set box width according to \refKey{/tcb/width}.
  The content is right aligned and may overlap the box borders.
\item\docValue{minimum center}:
  Set box width according to \refKey{/tcb/width}, if the content fits into.
  The content is centered and the box width may grow beyond \refKey{/tcb/width}.
\item\docValue{minimum left}:
  Set box width according to \refKey{/tcb/width}, if the content fits into.
  The content is left aligned and the box width may grow beyond \refKey{/tcb/width}.
\item\docValue{minimum right}:
  Set box width according to \refKey{/tcb/width}, if the content fits into.
  The content is right aligned and the box width may grow beyond \refKey{/tcb/width}.
\end{itemize}

\enlargethispage*{1cm}

\begin{exdispExample}{tcbox_width}
\tcbset{size=small,on line,before upper=\strut,
  colframe=blue!75!black,colback=blue!5!white,
  fontupper=\normalsize,width=4cm}

\tcbox[tcbox width=auto]{auto}\qquad
\tcbox[tcbox width=auto limited]{auto limited}\qquad
\tcbox[tcbox width=auto limited]{auto limited with long text}\\
\tcbox[tcbox width=forced center]{forced center}\qquad
\tcbox[tcbox width=forced center]{forced center with long text}\\
\tcbox[tcbox width=forced left]{forced left}\qquad
\tcbox[tcbox width=forced left]{forced left with long text}\\
\tcbox[tcbox width=forced right]{forced right}\qquad
\tcbox[tcbox width=forced right]{forced right with long text}\\
\tcbox[tcbox width=minimum center]{minimum center}\qquad
\tcbox[tcbox width=minimum center]{minimum center with long text}\\
\tcbox[tcbox width=minimum left]{minimum left}\qquad
\tcbox[tcbox width=minimum left]{minimum left with long text}\\
\tcbox[tcbox width=minimum right]{minimum right}\qquad
\tcbox[tcbox width=minimum right]{minimum right with long text}
\end{exdispExample}
\end{docTcbKey}


%\subsection{Skins}
%There are additional option keys which change the appearance of a |tcolorbox|.
%If only the core package is used, there is only one \emph{skin} and these
%keys are meaningless.
%The library \mylib{skins} adds more skins. The appropriate option keys for skins of
%the core package are therefore described in \Vref{sec:skincorekeys} from
%page \pageref{sec:skincorekeys}.

\clearpage
\subsection{Counters, Labels, and References}

\begin{docTcbKey}{phantom}{=\meta{code}}{no default, initially unset}
The \meta{code} is put in a box at the upper left corner of the |tcolorbox|.
If the |tcolorbox| is breakable, the \meta{code} is executed for the first box of
the break sequence only. If there already was some phantom code given, the
new \meta{code} is appended.\par
The \meta{code} is intended to be used for counter stepping, labelling, and
related operations which do not produce visible text.
\begin{itemize}
\item The \meta{code} is executed before the title and box content, i.\,e.\ counter
  values are ensured to be increased before usage.
\item Labels are ensured to reference the correct page number.
\item The \meta{code} is executed only once even during fitting operations for
  title and box content.
\item In combination with the |hyperref| package, the hyper anchor is set
  to the upper left corner of the |tcolorbox|, i.\,e.\ links inside the pdf document
  will jump to the box pleasantly.
\item Since the \meta{code} is executed inside a \TeX\ group, only global
  operations can survive this group.
\end{itemize}
Examples for the |phantom| usage are given in Section \ref{listing:exercises}
from page \pageref{listing:exercises}, e.\,g.\
Example \ref{exe:tabular_example} on page \pageref{exe:tabular_example}.
\end{docTcbKey}

\begin{docTcbKey}{nophantom}{}{no value, initially set}
Removes the phantom code if set before.
\end{docTcbKey}

\begin{docTcbKey}{label}{=\meta{marker}}{no default, initially unset}
The \meta{marker} is set as label text for a reference with the |\ref| macro.
Typically, this option is used for numbered boxes, see Subsection \ref{sec:numberedboxes}
from page \pageref{sec:numberedboxes}, e.\,g.\ \refKey{/tcb/new/auto counter}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-11-28]{phantomlabel}{=\meta{marker}}{no default, initially unset}
Equivalent to \refKey{/tcb/label} for an \emph{unnumbered} box.
A |\phantomsection| from the package |hyperref| \cite{rahtz:hyperref} is used to set a correct
hyperlink target. This is not needed for a numbered box.
\end{docTcbKey}


\begin{docTcbKey}{label type}{=\meta{type}}{no default, initially unset}
This option key can be used only in conjunction with the |cleveref| package
\cite{cubitt:2018a} which has to be loaded separately.
\meta{type} has to be a cross-reference type \emph{known} to |cleveref|
like |theorem|, |algorithm|, |result|, etc. References made with |cleveref|
will use this type. Note that using |label type| will result in compilation
errors, if |cleveref| is not loaded.
For an example, see \Vref{theo:meanvaluetheorem}.
\end{docTcbKey}

\begin{docTcbKey}{no label type}{}{no value, initially set}
Removes a \refKey{/tcb/label type}, if set before.
\end{docTcbKey}

\begin{docTcbKey}{step}{=\meta{counter}}{no default, initially unset}
Shortcut for |phantom={\refstepcounter{#1}}|. The given \meta{counter} is
increased and ready for labelling. This option is not needed when
using the convenient automated numbering introduced with version 2.40,
see Subsection \ref{sec:numberedboxes}
from page \pageref{sec:numberedboxes}.
\end{docTcbKey}

\begin{docTcbKey}{step and label}{=\marg{counter}\marg{marker}}{no default, initially unset}
Shortcut for using \refKey{/tcb/step} and \refKey{/tcb/label}. This option is not needed when
using the convenient automated numbering introduced with version 2.40,
see Subsection \ref{sec:numberedboxes}
from page \pageref{sec:numberedboxes}.
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{list entry}{=\meta{text}}{no default, initially unset}
If the \flqq list of tcolorbox(es)\frqq\ feature described in Subsection
\ref{sec:listsof} from page \pageref{sec:listsof} is used, this key
describes the \meta{text} for an entry into the generated list, e.\,g.
\begin{dispListing}
list entry={\protect\numberline{\thetcbcounter}My beautiful Example}
\end{dispListing}
See Section \ref{listing:exercises} from page \pageref{listing:exercises}
for a complete example.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-09-19]{list text}{=\meta{text}}{style, no default}
This is a shortcut for setting \refKey{/tcb/list entry} to\\
|\protect\numberline{\thetcbcounter}|\meta{text}.
So, the following settings are identical:
\begin{dispListing}
list text={My beautiful Example},
list entry={\protect\numberline{\thetcbcounter}My beautiful Example}
\end{dispListing}
See Section \ref{listing:exercises} from page \pageref{listing:exercises}
for a complete example.
\end{docTcbKey}

\begin{docTcbKey}{add to list}{=\marg{list}\marg{type}}{no default, initially unset}
If the \flqq list of tcolorbox(es)\frqq\ feature described in Subsection
\ref{sec:listsof} from page \pageref{sec:listsof} is used, list entries are
generated automatically. With this key, you can enforce an entry to the
given \meta{list} with the given \meta{type}.
This issues:\\
|\addcontentsline|\marg{list}\marg{type}\marg{entry text}
\end{docTcbKey}


\begin{docTcbKey}[][doc new and updated={2016-06-22}{2016-11-18}]{nameref}{=\meta{text}}{no default, initially unset}
If the |nameref| package is loaded, the given \meta{text} is used for
corresponding |\nameref| macros. Typically, the \meta{text} will be chosen
to be identical or nearly identical to the one for \refKey{/tcb/title}.

\inputpreamblelisting{A}

\begin{dispExample}
\begin{pabox}[label={mynamelabel},nameref={Title or anything else}]{Title text}
This is a tcolorbox.
\end{pabox}
This box is automatically numbered with \ref{mynamelabel} on page
\pageref{mynamelabel}.

The box is titled '\nameref{mynamelabel}'.
\end{dispExample}

\begin{marker}
\refKey{/tcb/nameref} is used automatically inside \refCom{newtcbtheorem}.
\end{marker}

\end{docTcbKey}

\clearpage
\begin{docTcbKey}[][doc new=2017-02-03]{hypertarget}{=\meta{marker}}{no default, initially unset}
A |\hypertarget| from the package |hyperref| \cite{rahtz:hyperref} is used to
create an internal link of an anchor \meta{marker}.
This \meta{marker} can be referenced by |\hyperlink| or
\refKey{/tcb/hyperlink}.
  \begin{dispExample*}{sbs,lefthand ratio=0.7}
% \usepackage{hyperref}%
\begin{tcolorbox}[enhanced,
  colback=red!10,colframe=red!50!black,
  hypertarget=hypertwinA,
  hyperlink=hypertwinB,
  title=Box A]
Click me to jump to Box B.
\end{tcolorbox}
  \end{dispExample*}
\end{docTcbKey}



\begin{docTcbKey}[][doc new=2017-02-10]{bookmark}{=\meta{text}}{no default, initially unset}
  Sets a PDF bookmark with the given \meta{text}, if the package |bookmark| \cite{oberdiek:bookmark}
  is loaded. This bookmark is set with an automated destination (the current box)
  and is set one level below the current bookmark level.
  \begin{dispExample*}{sbs,lefthand ratio=0.7}
% \usepackage{bookmark}%
\begin{tcolorbox}[colback=blue!10,colframe=blue!50!black,
  bookmark=Example for using a bookmark,
  title=Example for using a bookmark]
Open the bookmark view of the previewer
to see the bookmark.
\end{tcolorbox}
  \end{dispExample*}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2017-02-10]{bookmark*}{=\marg{options}\marg{text}}{no default, initially unset}
  Identical to \refKey{/tcb/bookmark}, but additional \meta{options}
  from the package |bookmark| \cite{oberdiek:bookmark} can be given.
  \begin{dispExample*}{sbs,lefthand ratio=0.7}
% \usepackage{bookmark}%
\begin{tcolorbox}[colback=red!10,colframe=red!50!black,
  bookmark*={color=red,italic,bold}%
            {Another bookmark example},
  title=Red and bold bookmark]
Open the bookmark view of the previewer
to see the bookmark.
\end{tcolorbox}
  \end{dispExample*}
\end{docTcbKey}



\begin{docTcbKey}[][doc new=2018-07-26]{index}{=\meta{entry}}{no default, initially unset}
  Adds an index \meta{entry} for the box. This is a shortcut for
  setting |\index|\marg{entry} to \refKey{/tcb/phantom}.
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2018-07-26]{index*}{=\marg{name}\marg{entry}}{no default, initially unset}
  Adds an \meta{entry} to an index with a specific \meta{name}.
  This is a shortcut for
  setting |\index|\oarg{name}\marg{entry} to \refKey{/tcb/phantom}.
  An index extension package like |imakeidx| has to be loaded to use
  this option key.
\end{docTcbKey}








\clearpage
\subsection{Even and Odd Pages}

\begin{marker}
Also see
\refKey{/tcb/toggle left and right} and
\refKey{/tcb/toggle enlargement}
for further even/odd options.
\end{marker}

\begin{docTcbKey}[][doc updated=2015-11-13]{check odd page}{\colOpt{=true\textbar false}}{default |true|, initially |false|}
If set to |true|, a precise even/odd page testing for the current box
is applied. This is done by using labels. If a box moves to another page,
the document has to be compiled twice for the correct settings.
If set to |false|, even/odd page tests may give wrong results for the first box
of a page.

\refKey{/tcb/toggle left and right},
\refKey{/tcb/toggle enlargement}, and
\refKey{/tcb/if odd page}
automatically set |check odd page|, but for
\refCom{tcbifoddpage} this option has to be set explicitely.
\end{docTcbKey}

\enlargethispage*{1cm}
\begin{docTcbKey}[][doc new=2015-11-13]{if odd page}{=\marg{odd options}\marg{even options}}{style, no default}
If the current box is on an odd page, the \meta{odd options} are applied.
On an even page, the \meta{even options} are applied.
\refKey{/tcb/check odd page} is automatically set for precise even/odd page testing.

\begin{dispExample}
\begin{tcolorbox}[if odd page={colback=yellow!50}{colback=red!50}]
  This box is colored in yellow on an odd page
  and is colored in red on an even page.
\end{tcolorbox}
\end{dispExample}

\begin{marker}
If a box is \refKey{/tcb/breakable}, using \refKey{/tcb/if odd page}
only acts upon the \emph{first} box. If the setting should be
repeated for every partial box of the break sequence, the option should be
packed into \refKey{/tcb/extras}. In this case, \refKey{/tcb/check odd page}
has to be set explicitely! Also see \refKey{/tcb/if odd page*}.
\end{marker}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2016-11-18]{if odd page or oneside}{=\marg{odd options}\marg{even options}}{style, no default}
  For onesided documents, the \meta{odd options} are applied always.
  For twosided documents, this style is identical to \refKey{/tcb/if odd page}.
\end{docTcbKey}


\clearpage
\begin{docTcbKey}[][doc new=2015-11-13]{if odd page*}{=\marg{odd options}\marg{even options}}{style, no default}
\begin{marker}
This option needs the \mylib{breakable} library, see \Fullref{sec:breakable}.
\end{marker}
For breakable boxes, if the current partial box is on an odd page, the \meta{odd options} are applied.
On an even page, the \meta{even options} are applied.
\refKey{/tcb/check odd page} is automatically set for precise even/odd page testing.

In contrast to \refKey{/tcb/if odd page}, \refKey{/tcb/if odd page*} is used
on \emph{every} partial box of a break sequences and not only on the
\emph{first} box. Another difference is that \refKey{/tcb/if odd page*}
is applied quite \emph{late} during option processing, while
\refKey{/tcb/if odd page} is applied immediately.

\refKey{/tcb/if odd page*} is implemented as \refKey{/tcb/if odd page}
packed into \refKey{/tcb/extras}.

\begin{dispExample}
% \tcbuselibrary{breakable}
\begin{tcolorbox}[breakable,if odd page*={colback=yellow!50}{colback=red!50}]
  This breakable box is colored in yellow on an odd page
  and is colored in red on an even page. For every partial box, the
  test is repeated, i.e. this would give a yellow, red, yellow, red, \ldots\
  sequence for a long content.
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2016-11-18]{if odd page or oneside*}{=\marg{odd options}\marg{even options}}{style, no default}
  For onesided documents, the \meta{odd options} are applied always.
  For twosided documents, this style is identical to \refKey{/tcb/if odd page*}.
\end{docTcbKey}


\clearpage
\begin{docCommand}[doc new=2015-11-13]{tcbifoddpage}{\marg{odd code}\marg{even code}}
If the current box is on an odd page, the \meta{odd code} is executed.
On an even page, the \meta{even code} is executed.
For precise even/odd page testing, the \refKey{/tcb/check odd page} has to be
set manually inside the box options.

The macro \refCom{tcbifoddpage} can be used inside underlay, overlay, or watermark code to
test if the box is on an odd page. This will work also for boxes in a break sequence.

The macro can also be used inside the box \textbf{content text}. For unbreakable boxes,
the correct page test is applied.
But for \refKey{/tcb/breakable} boxes, \refCom{tcbifoddpage}
will always give the result for the page of the \emph{first} box inside
the box \textbf{content text}. If needed, the methods from the packages
|changepage| or |ifoddpage| could be used here.
%To mention it again, for overlays, watermarks, etc, \refCom{tcbifoddpage} gives
%the correct page test.

\begin{dispExample}
\tcbset{colframe=blue!75!black,colback=white,fonttitle=\bfseries}

\begin{tcolorbox}[enhanced,check odd page,
  title={Example for a box on an \tcbifoddpage{odd}{even} page},
  watermark text={\tcbifoddpage{Odd}{Even} page!}]
\lipsum[1]
\end{tcolorbox}
\end{dispExample}
\end{docCommand}


\begin{docCommand}[doc new=2016-11-18]{tcbifoddpageoroneside}{\marg{odd code}\marg{even code}}
  For onesided documents, the \meta{odd code} is executed always.
  For twosided documents, this macro is identical to \refCom{tcbifoddpage}.
\end{docCommand}

\clearpage
\begin{docCommand}[doc new=2015-11-13]{thetcolorboxnumber}{}
This is a unique identifier (arabic number) for a tcolorbox. It is locally
defined inside boxes and has no meaning outside. It is used for
precise even/odd page testing, but may also be valuable for elaborate user
code.

\begin{dispExample}
\begin{tcolorbox}[colback=yellow!5,title=Box \thetcolorboxnumber]
  This box is \thetcolorboxnumber.
  \tcbox[on line,size=fbox]{This box is \thetcolorboxnumber} and
  \tcbox[on line,size=fbox]{this box is \thetcolorboxnumber}.
  This box is \thetcolorboxnumber.
\end{tcolorbox}
\end{dispExample}
\end{docCommand}


\begin{docCommand}[doc new=2015-11-13]{thetcolorboxpage}{}
This macro contains the expanded arabic page number of the current tcolorbox.
It is locally defined inside boxes and has no meaning outside.
It is precise only, if \refKey{/tcb/check odd page} was set.

\begin{dispExample}
\begin{tcolorbox}[colback=yellow!5,check odd page,
    title=Box on page~\thetcolorboxpage]
  This box is located on page~\thetcolorboxpage.
\end{tcolorbox}
\end{dispExample}
\end{docCommand}





\clearpage
\subsection{Externalization}
\begin{marker}
See \Fullref{sec:external} for the \mylib{external} library of |tcolorbox|.
\end{marker}

If the \emph{externalization} library of the \texttt{tikz} package is used
and \refKey{/tcb/graphical environment} is set to |tikzpicture|,
a |tcolorbox| could trigger the externalization process which will arise
a compilation error.

To avoid this, there are two possible strategies:
\begin{itemize}
\item Ensure, that |\tikzexternaldisable| is set before a |tcolorbox| is used.
  If you typically use the pattern |\tikzexternalenable| \textit{some picture} |\tikzexternaldisable|,
  there is nothing to care about.
\item If \emph{externalization} is enabled globally, use \refKey{/tcb/shield externalize} to
  shield any |tcolorbox|. The preamble code could look like this:
\begin{dispListing}
\usetikzlibrary{external}
\tikzexternalize
\tcbset{shield externalize}
\end{dispListing}
\end{itemize}

\begin{docTcbKey}{shield externalize}{\colOpt{=true\textbar false}}{default |true|, initially |false|}
If set to |true|, the drawing part of the |tcolorbox| is not being externalized
which is a good thing at the current state of art. Nevertheless, if the
|tcolorbox| contains a |tikzpicture|, this picture is still externalized.
Pictures drawn with help of \refKey{/tcb/tikz upper} or alike are \emph{not}
externalized.
\end{docTcbKey}

\begin{marker}
If a |tcolorbox| is used inside a node of an encircling |tikzpicture| which is externalized,
do \emph{not} use |\tikzexternaldisable| in front of the |tcolorbox|.
\refKey{/tcb/shield externalize} is deactivated automatically inside a |tikzpicture|.
\end{marker}

\begin{marker}
\refKey{/tcb/shield externalize} is applied for every following |tcolorbox|
inside the current \TeX\ group and is not affected by \refKey{/tcb/reset}.
\end{marker}

\begin{docTcbKey}{external}{=\meta{file name}}{no default, initially unset}
  Convenience option which calls |\tikzsetnextfilename|\marg{file name}. Typically,
  it may be used inside the option list of a |tcolorbox| to set the
  externalization \meta{file name} for the first |tikzpicture| which is discovered
  \emph{inside} the box content.
  The package |tikz| \cite{tantau:tikz_and_pgf} or the library \mylib{skins} has to be loaded to use this option.
  Additionally, |\usetikzlibrary{external}| has to be used.
\end{docTcbKey}

\begin{docTcbKey}{remake}{\colOpt{=true\textbar false}}{default |true|, initially |false|}
  Convenience option which calls |/tikz/external/remake next|. Typically,
  it may be used inside the option list of a |tcolorbox| to force the remake
  of the first |tikzpicture| which is discovered \emph{inside} the box content.
  The package |tikz| \cite{tantau:tikz_and_pgf} or the library \mylib{skins} has to be loaded to use this option.
  Additionally, |\usetikzlibrary{external}| has to be used.
\end{docTcbKey}


\clearpage
\subsection{Miscellaneous}
\begin{docTcbKey}{reset}{}{no value, initially set}
Sets (nearly) all |tcolorbox| settings (including loaded libraries) back to their default values
\emph{plus} any settings given by \refCom{tcbsetforeverylayer}.
\refKey{/tcb/savedelimiter}, \refKey{/tcb/capture}, and
\refKey{/tcb/shield externalize} keep their values.
Also, all raster values (see \Vref{sec:raster}) are not resetted.

This option is useful for boxes in boxes where the inner box should not inherit
the settings of the outer box.
Note that for boxes inside boxes the |reset| is done automatically, if the
standard settings of the package are used (v2.40 and above), see
Section \ref{subsec:everybox} from page \pageref{subsec:everybox}.
%See \refCom{tcbhighmath} for an example.
\end{docTcbKey}




\begin{docTcbKey}{code}{=\meta{code}}{no default, initially unset}
  The given \meta{code} is executed immediately. This option is useful
  to place some arbitrary code into an option list.
\begin{exdispExample}{code}
\tcbset{colback=red!5!white,colframe=red!75!black,
  code={Useless at this spot but functional.},
  fonttitle=\bfseries}

\begin{tcolorbox}[code={\newcommand{\mycommand}{\textit{working}}},
  title=My \mycommand\ title]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample}
\end{docTcbKey}


\clearpage
\begin{docTcbKey}[][doc new=2016-10-21]{void}{}{no value, initially unset}
  Annihilates the current |tcolorbox| as far as possible.
  Basically, this comments out the whole |tcolorbox| by using a key.
  If the option list of the current |tcolorbox| contains arbitrary code with global
  impact (like counter settings), these actions are not undone automatically.
  Nevertheless, the effects of \refKey{/tcb/phantom}, \refKey{/tcb/step},
  \refKey{/tcb/new/auto counter}, etc., are removed by \refKey{/tcb/void}.

\begin{exdispExample}{void}
A%
  \begin{tcolorbox}[
      title=This box is completely removed by the following key,
      void
    ]
  This is a \textbf{tcolorbox}.
  \end{tcolorbox}
B
\end{exdispExample}

\begin{marker}
  This option key cannot be applied for every situation.
  For example, if several box environments with the same environment name
  are nested, for the outer environment \refKey{/tcb/void} cannot be used,
  since the end of the inner environment will be misinterpreted as
  end of the outer environment.
\end{marker}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2019-03-01]{nirvana}{}{no value, initially unset}
  The contents of the current |tcolorbox| are processed including counter
  settings, but the box is just not drawn.
  Therefore, \refKey{/tcb/nirvana} is less radical than \refKey{/tcb/void}
  and several box environments can be nested without problems.

\begin{exdispExample}{nirvana}
A%
  \begin{tcolorbox}[
      title=This box is completely removed by the following key,
      nirvana
    ]
  This is a \textbf{tcolorbox}.
    \begin{tcolorbox}
    Nested Box
    \end{tcolorbox}
  \end{tcolorbox}%
B
\end{exdispExample}
\end{docTcbKey}


==> tcolorbox.doc.documentation.tex <==
% !TeX root = tcolorbox.tex
% include file of tcolorbox.tex (manual of the LaTeX package tcolorbox)
\clearpage
\section{Library \mylib{documentation}}\label{sec:documentation}%
\tcbset{external/prefix=external/documentation_}%
This library has the single purpose to support \LaTeX\ package documentations
like this one. Actually, the visual nature follows the approach from
Till Tantau's |pgf| \cite{tantau:tikz_and_pgf} documentation.
Typically, this library is assumed to be used in conjunction with the
class |ltxdoc| or alike.
Denis Bitouz\'e, Muzimuzhi, and many others provided very valuable input for this library.

The library is loaded by a package option or inside the preamble by:
\begin{dispListing}
  \tcbuselibrary{documentation}
\end{dispListing}
This also loads
the library \mylib{skins}, see \Vref{sec:skins},
the library \mylib{raster}, see \Vref{sec:raster},
the library \mylib{listings}, see \Vref{sec:listings},
the library \mylib{xparse}, see \Vref{sec:xparse},
and a bunch of packages, namely
|pifont|, |marvosym|, |makeidx|, |marginnote|, |refcount|, and |hyperref|.

\begin{marker}
The package |makeidx| is loaded only, if \docAuxCommand*{printindex} is
\emph{not} already defined. Therefore, one can include an alternative to |makeidx| like
|imakeidx| \emph{before} the library |documentation| is used.
\end{marker}
\begin{marker}
The package |marginnote| is loaded only, if \docAuxCommand*{marginnote} is
\emph{not} already defined.
\end{marker}
\begin{marker}
In contrast to other |tcolorbox| options, the option
settings for \mylib{documentation} are typically not
getting reset by \refKey{/tcb/reset}, i.e. they keep their
values for embedded boxes.
\end{marker}
\begin{marker}
In combination with DocStrip, \refKey{/tcb/verbatim ignore percent} may be helpful.
\end{marker}

For UTF-8 support load (ignore this when using Xe\LaTeX):
\begin{dispListing}
  \tcbuselibrary{listingsutf8,documentation}
\end{dispListing}

For |minted| \cite{poore:minted} support, load:
\begin{dispListing}
  \tcbuselibrary{documentation,minted}
  \tcbset{listing engine=minted}
\end{dispListing}


%\clearpage
%-------------------------------------------------------------------------------
\subsection{Macros of the Library}

\begin{docEnvironment}[doclang/environment content=command description,doc updated=2020-04-22]
    {docCommand}{\oarg{options}\marg{name}\marg{parameters}}
  Documents a \LaTeX\ macro with given \meta{name} where \meta{name} is
  written without backslash. The given \meta{options} are set with \refCom{tcbset}.
  This macro takes mandatory or optional \meta{parameters}.
  It is automatically indexed and can be referenced with
  \refCom{refCom}\marg{name}.
\begin{dispExample}
\begin{docCommand}{foomakedocSubKey}{\marg{name}\marg{key path}}
  Creates a new environment \meta{name} based on \refEnv{docKey} for the
  documentation of keys with the given \meta{key path}.
\end{docCommand}
\end{dispExample}
\begin{dispExample}
\begin{docCommand}[color definition=blue]{foomakedocSubKey*}%
    {\marg{name}\marg{key path}}
  Creates a new environment \meta{name} based on \refEnv{docKey} for the
  documentation of keys with the given \meta{key path}.
\end{docCommand}
\end{dispExample}
\end{docEnvironment}


\begin{docEnvironment}[doclang/environment content=command description,doc updated=2020-04-22]
    {docCommand*}{\oarg{options}\marg{name}\marg{parameters}}
  Identical to \refEnv{docCommand}, but without index entry.
\end{docEnvironment}


\begin{docEnvironment}[doclang/environment content=command description,doc new=2020-04-22]
    {docCommands}{\oarg{options}\brackets{\marg{variant1},\marg{variant2},...}}
  Documents several (similar) \LaTeX\ macro variants simultaneously.
  The given \meta{options} are set with \refCom{tcbset} and are valid for
  all variants and the documentation text.
  Every variant is described by an option set \meta{variant1}, \meta{variant2}, and so on.
  The most crucial options are \refKey{/tcb/doc name} and \refKey{/tcb/doc parameter}.
\begin{dispExample}
\begin{docCommands}[
    doc no index,  %  no index entries for this example
    doc name      = newtheorem,
    doc parameter = \marg{envname},
  ]
  {
    {  },
    { doc parameter = \marg{envname}\oarg{numbered within} },
    { doc parameter = \oarg{numbered like}\marg{envname} },
    { doc name      = newtheorem* },
  }
  example
\end{docCommands}
\end{dispExample}
\end{docEnvironment}



\clearpage
{\let\xdocEnvironment\docEnvironment
\let\endxdocEnvironment\enddocEnvironment
\begin{xdocEnvironment}[doclang/environment content=environment description,doc updated=2020-04-22]
    {docEnvironment}{\oarg{options}\marg{name}\marg{parameters}}
  Documents a \LaTeX\ environment with given \meta{name}.
  The given \meta{options} are set with \refCom{tcbset}.
  This environment takes mandatory or optional \meta{parameters}.
  It is automatically indexed and can be referenced with
  \refCom{refEnv}\marg{name}.
\begin{dispExample}
\begin{docEnvironment}{foocolorbox}{\oarg{options}}
  This is the main environment to create an accentuated colored text box with
  rounded corners and, optionally, two parts.
\end{docEnvironment}
\end{dispExample}
\begin{dispExample}
\begin{docEnvironment}%
    [doclang/environment content=My content text]%
    {foocolorbox*}{\oarg{options}}
  This is the main environment to create an accentuated colored text box with
  rounded corners and, optionally, two parts.
\end{docEnvironment}
\end{dispExample}
\end{xdocEnvironment}}

{\let\xdocEnvironment\docEnvironment
\let\endxdocEnvironment\enddocEnvironment
\begin{xdocEnvironment}[doclang/environment content=environment description,doc updated=2020-04-22]
    {docEnvironment*}{\oarg{options}\marg{name}\marg{parameters}}
  Identical to \refEnv{docEnvironment}, but without index entry.
\end{xdocEnvironment}}


\clearpage
{\let\xdocEnvironment\docEnvironment
\let\endxdocEnvironment\enddocEnvironment
\begin{xdocEnvironment}[doclang/environment content=environment description,doc new=2020-04-22]
    {docEnvironments}{\oarg{options}\brackets{\marg{variant1},\marg{variant2},...}}
  Documents several (similar) \LaTeX\ environment variants simultaneously.
  The given \meta{options} are set with \refCom{tcbset} and are valid for
  all variants and the documentation text.
  Every variant is described by an option set \meta{variant1}, \meta{variant2}, and so on.
  The most crucial options are \refKey{/tcb/doc name} and \refKey{/tcb/doc parameter}.
\begin{dispExample}
\begin{docEnvironments}[
    doc no index,   %  no index entries for this example
    doc parameter = \oarg{options}\marg{title},
    doclang/environment content = box content,
  ]
  {
    {
      doc name        = redbox,
      doc description = a red colored box,
    },
    {
      doc name        = greenbox,
      doc description = a green colored box,
    },
    {
      doc name        = bluebox,
      doc description = a blue colored box,
    },
    {
      doc name        = custombox,
      doc parameter   = \oarg{options}\marg{color}\marg{title},
      doc description = a colored box,
    },
  }
  example
\end{docEnvironments}
\end{dispExample}
\end{xdocEnvironment}}


\clearpage
\begin{docEnvironment}[doclang/environment content=key description,doc updated=2020-04-22]
    {docKey}{\oarg{key path}\oarg{options}\marg{name}\marg{parameters}\marg{description}}
  Documents a key with given \meta{name} and an optional \meta{key path}.
  The given \meta{options} are set with \refCom{tcbset}.
  This key takes mandatory or optional \meta{parameters} as value
  with a short \meta{description}.
  It is automatically indexed and can be referenced with
  \refCom{refKey}\marg{name}.
\begin{dispExample}
\begin{docKey}[foo]{footitle}{=\meta{text}}{no default, initially empty}
  Creates a heading line with \meta{text} as content.
\end{docKey}
\end{dispExample}
\end{docEnvironment}


\begin{docEnvironment}[doclang/environment content=key description,doc updated=2020-04-22]
    {docKey*}{\oarg{key path}\oarg{options}\marg{name}\marg{parameters}\marg{description}}
  Identical to \refEnv{docKey}, but without index entry.
\end{docEnvironment}


\begin{docEnvironment}[doclang/environment content=key description,doc new=2020-04-22]
    {docKeys}{\oarg{options}\brackets{\marg{variant1},\marg{variant2},...}}
  Documents several (similar) key variants simultaneously.
  The given \meta{options} are set with \refCom{tcbset} and are valid for
  all variants and the documentation text.
  Every variant is described by an option set \meta{variant1}, \meta{variant2}, and so on.
  The most crucial options are
  \refKey{/tcb/doc keypath}, \refKey{/tcb/doc name}, \refKey{/tcb/doc parameter},
  and \refKey{/tcb/doc description}.
\begin{dispExample}
\begin{docKeys}[
    doc no index,   %  no index entries for this example
    doc keypath   = mykeyroot,
    doc parameter = {=\meta{length}},
  ]
  {
    {
      doc name        = width,
      doc description = initially \texttt{10cm},
    },
    {
      doc name        = height,
      doc description = initially \texttt{7cm},
    },
  }
  example
\end{docKeys}
\end{dispExample}
\end{docEnvironment}


\clearpage
\begin{docEnvironment}[doclang/environment content=operation description,
    doc new and updated={2019-09-18}{2020-04-22}]{docPathOperation}{\oarg{options}\marg{name}\marg{parameters}}
  Documents a \tikzname\ path operation with given \meta{name}.
  The given \meta{options} are set with \refCom{tcbset}.
  This \tikzname\ path operation takes mandatory or optional \meta{parameters}.
  It is automatically indexed and can be referenced with
  \refCom{refPathOperation}\marg{name}.
\begin{dispExample}
\begin{docPathOperation}{fooop}{\oarg{opt}(\meta{name})\colOpt{at(\meta{coord})}}
  Imaginary path operation for illustration.
\end{docPathOperation}
\end{dispExample}
\end{docEnvironment}


\begin{docEnvironment}[doclang/environment content=command description,
    doc new and updated={2019-09-18}{2020-04-22}]{docPathOperation*}{\oarg{options}\marg{name}\marg{parameters}}
  Identical to \refEnv{docPathOperation}, but without index entry.
\end{docEnvironment}


\begin{docEnvironment}[doclang/environment content=command description,
    doc new={2020-04-22}]{docPathOperations}{\oarg{options}\brackets{\marg{variant1},\marg{variant2},...}}
  Documents several (similar) \tikzname\ path operation variants simultaneously.
  The given \meta{options} are set with \refCom{tcbset} and are valid for
  all variants and the documentation text.
  Every variant is described by an option set \meta{variant1}, \meta{variant2}, and so on.
  The most crucial options are \refKey{/tcb/doc name} and \refKey{/tcb/doc parameter}.
\begin{dispExample}
\begin{docPathOperations}[
    doc no index,   %  no index entries for this example
  ]
  {
    {
      doc name      = rectangle,
      doc parameter = \meta{corner or cycle},
    },
    {
      doc name      = circle,
      doc parameter = \oarg{options},
    },
    {
      doc name      = ellipse,
      doc parameter = \oarg{options},
    },
  }
  example
\end{docPathOperations}
\end{dispExample}
\end{docEnvironment}


\clearpage
\begin{docCommands}[doc parameter=\oarg{options}\marg{name}]
  {
    {
      doc name = docValue,
      doc updated=2020-04-23,
    },
    {
      doc name = docValue*,
    },
  }
  Documents a value with given \meta{name}. Typically, this is a value for a key.
  The given \meta{options} are set with \refCom{tcbset}.
  This value is automatically indexed for \refCom{docValue}
  and has no index entry for \refCom{docValue*}.
\begin{dispExample}
A feasible value for \refKey{/foo/footitle} is \docValue*{foovalue}.
\end{dispExample}
\end{docCommands}



\begin{docCommands}[doc parameter=\oarg{options}\marg{name}]
  {
    {
      doc name    = docAuxCommand,
      doc updated = 2020-04-23,
    },
    {
      doc name = docAuxCommand*,
    },
  }
  Documents an auxiliary or minor \LaTeX\ macro with given \meta{name}
  where \meta{name} is written without backslash.
  The given \meta{options} are set with \refCom{tcbset}.
  This macro is automatically indexed for \refCom{docAuxCommand}
  and has no index entry for \refCom{docAuxCommand*}.
\begin{dispExample}
The macro \docAuxCommand{fooaux} holds some interesting data.
\end{dispExample}
\end{docCommands}



\begin{docCommands}[doc parameter=\oarg{options}\marg{name}]
  {
    {
      doc name    = docAuxEnvironment,
      doc updated = 2020-04-23,
    },
    {
      doc name = docAuxEnvironment*,
    },
  }
  Documents an auxiliary or minor \LaTeX\ environment with given \meta{name}.
  The given \meta{options} are set with \refCom{tcbset}.
  This macro is automatically indexed indexed for \refCom{docAuxEnvironment}
  and has no index entry for \refCom{docAuxEnvironment*}.
\begin{dispExample}
The environment \docAuxEnvironment{fooauxenv} holds some interesting data.
\end{dispExample}
\end{docCommands}


\begin{docCommands}[doc parameter=\oarg{key path}\oarg{options}\marg{name}]
  {
    {
      doc name    = docAuxKey,
      doc updated = 2020-04-23,
    },
    {
      doc name = docAuxKey*,
    },
  }
  Documents an auxiliary key with given \meta{name} and an optional \meta{key path}.
  The given \meta{options} are set with \refCom{tcbset}.
  It is automatically indexed for \refCom{docAuxKey}
  and has no index entry for \refCom{docAuxKey*}.
\begin{dispExample}
The key \docAuxKey[foo]{fooaux} holds some interesting data.
\end{dispExample}
\end{docCommands}



\begin{docCommands}[doc parameter=\oarg{options}\marg{name}]
  {
    {
      doc name    = docCounter,
      doc updated = 2020-04-23,
    },
    {
      doc name = docCounter*,
    },
  }
  Documents a counter with given \meta{name}.
  The given \meta{options} are set with \refCom{tcbset}.
  The counter is automatically indexed for \refCom{docCounter}
  and has no index entry for \refCom{docCounter*}.
\begin{dispExample}
The counter \docCounter{foocounter} can be used for computation.
\end{dispExample}
\end{docCommands}


\clearpage
\begin{docCommands}[doc parameter=\oarg{options}\marg{name}]
  {
    {
      doc name    = docLength,
      doc updated = 2020-04-23,
    },
    {
      doc name = docLength*,
    },
  }
  Documents a length with given \meta{name}.
  The given \meta{options} are set with \refCom{tcbset}.
  The length is automatically indexed for \refCom{docLength}
  and has no index entry for \refCom{docLength*}.
\begin{dispExample}
The length \docLength{foolength} can be used for computation.
\end{dispExample}
\end{docCommands}


\begin{docCommands}[doc parameter=\oarg{options}\marg{name}]
  {
    {
      doc name    = docColor,
      doc updated = 2020-04-23,
    },
    {
      doc name = docColor*,
    },
  }
  Documents a color with given \meta{name}.
  The given \meta{options} are set with \refCom{tcbset}.
  The color is automatically indexed for \refCom{docColor}
  and has no index entry for \refCom{docColor*}.
\begin{dispExample}
The color \docColor{foocolor} is available.
\end{dispExample}
\end{docCommands}



\begin{docCommand}{cs}{\marg{name}}
  Macro from |ltxdoc| \cite{carlisle:ltxdoc} to typeset a command word \meta{name}
  where the backslash is prefixed. The library overwrites the original macro.
\begin{dispExample}
This is a \cs{foocommand}.
\end{dispExample}
\end{docCommand}

\begin{docCommand}{meta}{\marg{text}}
  Macro from |doc| \cite{mittelbach:2011a} to typeset a meta \meta{text}.
  The library overwrites the original macro.
\begin{dispExample}
This is a \meta{text}.
\end{dispExample}
\end{docCommand}


\begin{docCommand}{marg}{\marg{text}}
  Macro from |ltxdoc| \cite{carlisle:ltxdoc} to typeset a \meta{text} with
  curly brackets as a mandatory argument. The library overwrites the original macro.
\begin{dispExample}
This is a mandatory \marg{argument}.
\end{dispExample}
\end{docCommand}

\begin{docCommand}{oarg}{\marg{text}}
  Macro from |ltxdoc| \cite{carlisle:ltxdoc} to typeset a \meta{text} with
  square brackets as an optional argument. The library overwrites the original macro.
\begin{dispExample}
This is an optional \oarg{argument}.
\end{dispExample}
\end{docCommand}

\clearpage

\begin{docCommand}{brackets}{\marg{text}}
  Sets the given \meta{text} with curly brackets.
\begin{dispExample}
  Here we use \brackets{some text}.
\end{dispExample}
\end{docCommand}


{\let\xdispExample\dispExample
  \let\endxdispExample\enddispExample
\begin{docEnvironment}[doc updated=2014-10-10]{dispExample}{}
  Creates a colored box based on a \refEnv{tcolorbox}.
  It displays the environment content as source code in the upper part
  and as compiled text in the lower part of the box.
  The appearance is controlled by \refKey{/tcb/documentation listing style}
  and the style \refKey{/tcb/docexample}. It may be
  changed by redefining this style.
{
%\tcbset{before lower app={\tcbset{docexample/.style={docexample original}}}}
%\tcbset{docexample/.style={docexample original}}%
\begin{xdispExample}
\begin{dispExample}
This is a \LaTeX\ example.
\end{dispExample}
\end{xdispExample}
}
\end{docEnvironment}}


{\let\xdispExample\dispExample
  \let\endxdispExample\enddispExample
\begin{docEnvironment}[doc updated=2014-10-10]{dispExample*}{\marg{options}}
  The starred version of \refEnv{dispExample} takes \refEnv{tcolorbox} \meta{options}
  as parameter. These \meta{options} are executed after \refKey{/tcb/docexample}.
\begin{xdispExample}
\begin{dispExample*}{sidebyside}
This is a \LaTeX\ example.
\end{dispExample*}
\end{xdispExample}
\end{docEnvironment}}


\clearpage
\begin{docEnvironment}{dispListing}{}
  Creates a colored box based on a \refEnv{tcolorbox}.
  It displays the environment content as source code.
  The appearance is controlled by \refKey{/tcb/documentation listing style}
  and the style \refKey{/tcb/docexample}. It may be
  changed by redefining this style.
\begin{dispExample}
\begin{dispListing}
This is a \LaTeX\ example.
\end{dispListing}
\end{dispExample}
\end{docEnvironment}

\begin{docEnvironment}{dispListing*}{\marg{options}}
  The starred version of \refEnv{dispListing} takes \refEnv{tcolorbox} \meta{options}
  as parameter. These \meta{options} are executed after \refKey{/tcb/docexample}.
\begin{dispExample}
\begin{dispListing*}{title=My listing}
This is a \LaTeX\ example.
\end{dispListing*}
\end{dispExample}
\end{docEnvironment}


\begin{docEnvironment}{absquote}{}
  Used to typeset an abstract as quoted and small text.
\begin{dispExample}
\begin{absquote}
|tcolorbox| provides an environment for colored and framed text boxes with a
heading line. Optionally, such a box can be split in an upper and a lower part.
\end{absquote}
\end{dispExample}
\end{docEnvironment}

\clearpage
\begin{docCommand}[doc updated=2020-04-22]{tcbmakedocSubKey}{\marg{name}\marg{key path}}
  Creates a new environment \meta{name} based on \refEnv{docKey} for the
  documentation of keys with the given \meta{key path} as root.
  The new environment \meta{name} takes the same para\-meters as \refEnv{docKey} itself.
  A second starred environment \meta{name} is also created, which is identical
  to \meta{name} but without index entry.
\begin{dispExample}
\tcbmakedocSubKey{docFooKey}{foo}

\begin{docFooKey}{foodummy}{=\meta{nothing}}{no default, initially empty}
Some key.
\end{docFooKey}

\begin{docFooKey*}{foo another dummy}{=\meta{nothing}}{no default, initially empty}
Some key (not indexed).
\end{docFooKey*}
\end{dispExample}
\end{docCommand}


\begin{docCommand}[doc new=2020-04-22]{tcbmakedocSubKeys}{\marg{name}\marg{key path}}
  Creates a new environment \meta{name} based on \refEnv{docKeys} for the
  documentation of keys with the given \meta{key path} as root.
  The new environment \meta{name} takes the same para\-meters as \refEnv{docKeys} itself.
\begin{dispExample}
\tcbmakedocSubKeys{docFooKeys}{foo}

\begin{docFooKeys}[
    doc parameter   = {=\meta{nothing}},
    doc description = {no default, initially empty},
  ]
  {
    {
      doc name = foodummy 2,
    },
    {
      doc name = foo another dummy 2,
      doc no index,
    }
  }
Some description.
\end{docFooKeys}
\end{dispExample}
\end{docCommand}


\clearpage

\begin{docCommand}{refCom}{\marg{name}}
  References a documented \LaTeX\ macro with given \meta{name} where \meta{name} is
  written without backslash. The page reference is suppressed if it links
  to the same page.
\begin{dispExample}
We have created \refCom{foomakedocSubKey} as an example.
\end{dispExample}
\end{docCommand}

\begin{docCommand}{refCom*}{\marg{name}}
  References a documented \LaTeX\ macro with given \meta{name} where \meta{name} is
  written without backslash. There is no page reference.
\begin{dispExample}
We have created \refCom*{foomakedocSubKey} as an example.
\end{dispExample}
\end{docCommand}


\begin{docCommand}{refEnv}{\marg{name}}
  References a documented \LaTeX\ environment with given \meta{name}.
  The page reference is suppressed if it links to the same page.
\begin{dispExample}
We have created \refEnv{foocolorbox} as an example.
\end{dispExample}
\end{docCommand}

\begin{docCommand}{refEnv*}{\marg{name}}
  References a documented \LaTeX\ environment with given \meta{name}.
  There is no page reference.
\begin{dispExample}
We have created \refEnv*{foocolorbox} as an example.
\end{dispExample}
\end{docCommand}


\begin{docCommand}{refKey}{\marg{name}}
  References a documented key with given \meta{name} where \meta{name}
  is the full path name of the key.
  The page reference is suppressed if it links to the same page.
\begin{dispExample}
We have created \refKey{/foo/footitle} as an example.
\end{dispExample}
\end{docCommand}

\begin{docCommand}{refKey*}{\marg{name}}
  References a documented key with given \meta{name} where \meta{name}
  is the full path name of the key.
  There is no page reference.
\begin{dispExample}
We have created \refKey*{/foo/footitle} as an example.
\end{dispExample}
\end{docCommand}

\clearpage

\begin{docCommand}[doc new=2019-09-17]{refPathOperation}{\marg{name}}
  References a documented \tikzname\ path operation with given \meta{name}.
  The page reference is suppressed if it links to the same page.
\begin{dispExample}
We have created \refPathOperation{fooop} as an example.
\end{dispExample}
\end{docCommand}

\begin{docCommand}[doc new=2019-09-17]{refPathOperation*}{\marg{name}}
  References a documented \tikzname\ path operation with given \meta{name}.
  There is no page reference.
\begin{dispExample}
We have created \refPathOperation*{fooop} as an example.
\end{dispExample}
\end{docCommand}



\begin{docCommand}[doc updated=2020-02-11]{refAux}{\marg{name}}
  References some auxiliary environment, key, value, or color.
  The \meta{name} is colored according to \refKey{/tcb/color hyperlink},
  if |hyperref| colorlinks are set, but there is no real link.
\begin{dispExample}
Some pages back, one can see \refAux{/foo/footitle} as an example.
\end{dispExample}
\end{docCommand}

\begin{docCommand}[doc updated=2020-02-11]{refAuxcs}{\marg{name}}
  References some auxiliary macro \meta{name} where \meta{name} is
  written without backslash.
  The \meta{name} is colored according to \refKey{/tcb/color hyperlink},
  if |hyperref| colorlinks are set, but there is no real link.
\begin{dispExample}
Some pages back, one can see \refAuxcs{fooaux} as an example.
\end{dispExample}
\end{docCommand}


\begin{docCommand}{colDef}{\marg{text}}
Sets \meta{text} with the command color, see \refKey{/tcb/color command}.
\begin{dispExample}
This is my \colDef{text}.
\end{dispExample}
\end{docCommand}

\begin{docCommand}{colOpt}{\marg{text}}
  Sets \meta{text} with the option color, see \refKey{/tcb/color option}.
\begin{dispExample}
This is my \colOpt{text}.
\end{dispExample}
\end{docCommand}

\clearpage

\begin{docCommand}[doc new=2019-09-18]{colFade}{\marg{text}}
  Sets \meta{text} with the fade color, see \refKey{/tcb/color fade}.
\begin{dispExample}
This is my \colFade{text}.
\end{dispExample}
\end{docCommand}


\begin{docCommand}[doc new=2014-09-19]{tcbdocmarginnote}{\oarg{options}\marg{text}}
  Creates a |tcolorbox| note with the given \meta{text} inside the margin using
  the |marginnote| package. The style of the |tcolorbox| is predefined and can be
  altered by \refKey{/tcb/doc marginnote} and the given \meta{options}.
\begin{dispExample}
Some text\tcbdocmarginnote{Note A}
which is commented by a note inside the margin.
Alternatively to |\tcbdocmarginnote|, you can always use
|\marginnote| with a |tcolorbox| directly.\par
This is further text%
\tcbdocmarginnote[colframe=blue!50!white,colback=blue!5!white]{Note B}
with another note.
\end{dispExample}
\end{docCommand}

\begin{docCommand}[doc new=2014-09-19]{tcbdocnew}{\marg{date}}
  Auxiliary macro which typesets the \refKey{/tcb/doclang/new} text with
  the given \meta{date}. It may be redefined for customization.
  \makeatletter\renewcommand*{\tcbdocnew}[1]{\kvtcb@text@new: #1}\makeatother%
\begin{dispExample*}{sidebyside}
\tcbdocnew{1981-10-29}.
% Next one is displayed in the margin:
\tcbdocmarginnote{\tcbdocnew{1978-02-09}}
\end{dispExample*}
\end{docCommand}

\begin{docCommand}[doc new=2014-09-19]{tcbdocupdated}{\marg{date}}
  Auxiliary macro which typesets the \refKey{/tcb/doclang/updated} text with
  the given \meta{date}. It may be redefined for customization.
  \makeatletter\renewcommand*{\tcbdocupdated}[1]{\kvtcb@text@updated: #1}\makeatother%
\begin{dispExample*}{sidebyside}
\tcbdocupdated{2014-09-19}.
\end{dispExample*}
\end{docCommand}


\clearpage
%-------------------------------------------------------------------------------
\subsection{Entry Content Option Keys}


\begin{docTcbKey}[][doc new={2020-04-22}]{doc name}{=\meta{name}}{no default, initially empty}
  Sets the \meta{name} of the entry to document, i.e. the \meta{name} of the
  command, environment, key, etc. For \refEnv{docCommand}, \refEnv{docEnvironment}, etc.
  the \meta{name} is set by a mandatory parameter, but can also be set
  by \refKey{/tcb/doc name}.
  \refKey{/tcb/doc name} also sets \meta{name} to
  \refKey{/tcb/doc label}, \refKey{/tcb/doc index},
  and \refKey{/tcb/doc sort index}.
\begin{dispExample}
\begin{docCommands}[
    doc no index,  %  no index entries for this example
    doc name      = bfseries,
  ] {}
  Font setting to bold face.
\end{docCommands}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new={2020-04-22}]{doc parameter}{=\meta{parameters}}{no default, initially empty}
  Sets the \meta{parameters} of the entry to document, i.e. the \meta{parameters} of the
  command, environment, key, etc. For \refEnv{docCommand}, \refEnv{docEnvironment}, etc.
  the \meta{parameters} is set by a mandatory option, but can also be set
  by \refKey{/tcb/doc parameter}.
\begin{dispExample}
\begin{docCommands}[
    doc no index,  %  no index entries for this example
    doc name      = textbf,
    doc parameter = \marg{text},
  ] {}
  Sets \meta{text} in bold face.
\end{docCommands}
\end{dispExample}
\end{docTcbKey}



\begin{docTcbKey}[][doc new={2020-04-22}]{doc keypath}{=\meta{key path}}{no default, initially empty}
  Sets the \meta{key path} of the key to document. For \refEnv{docKey}
  and \refEnv{docKey*} the \meta{key path}  is set by a specialized option,
  but can also be set by \refKey{/tcb/doc keypath}.
\begin{dispExample}
\begin{docKeys}[
    doc no index,  %  no index entries for this example
    doc keypath     = tikz,
    doc name        = fill,
    doc parameter   = \colOpt{=\meta{color}},
    doc description = default is scope's color setting,
  ] {}
  This option causes the path to be filled.
\end{docKeys}
\end{dispExample}
\end{docTcbKey}

\clearpage

\begin{docTcbKey}{doc description}{=\meta{description}}{no default, initially empty}
  Sets a (short!) additional \meta{description} for
  \refEnv{docCommand}, \refEnv{docEnvironment}, or \refEnv{docPathOperation}.
  Such a description is
  mandatory for \refEnv{docKey}.
\begin{dispExample}
\begin{docCommand*}[doc description=my description]{myCommandF}{\marg{argument}}
  This is the documentation of \refCom{myCommandF} which takes one \meta{argument}.
  \refCom{myCommandF} does some funny things with its \meta{argument}.
\end{docCommand*}
\end{dispExample}
\begin{marker}
Note that the description \meta{text} may overlap with the text on the left
hand side if too long. Linebreaks can be used inside the \meta{text}.
\end{marker}
\end{docTcbKey}


\begin{docTcbKey}[][doc new={2019-09-18}]{doc label}{=\meta{text}}{no default, initially unset}
  If used inside the option list of \refEnv{docCommand}, \refEnv{docEnvironment},
  \refEnv{docKey}, etc, then \meta{text} is used
  for labeling instead of the name of the definition.
\begin{dispExample}
\begin{docPathOperation*}[doc label=pathline]{-{}-}{\meta{coordinate or cycle}}
  This is the documentation of \refPathOperation{pathline}.
\end{docPathOperation*}
\end{dispExample}
\end{docTcbKey}

\begin{docTcbKey}[][doc new={2020-01-07}]{doc index}{=\meta{text}}{no default, initially unset}
  If used inside the option list of \refEnv{docCommand}, \refEnv{docEnvironment},
  \refEnv{docKey}, etc, then \meta{text} is used
  for the index instead of the name of the definition.
\begin{dispExample}
\begin{docPathOperation}[doc index=foo path (horizontal then vertical),
    doc label=pathline2]{-\textbar}{\meta{coordinate or cycle}}
  This is the documentation of \refPathOperation{pathline2}.
\end{docPathOperation}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new={2020-04-23}]{doc sort index}{=\meta{text}}{no default, initially unset}
  If used inside the option list of \refEnv{docCommand}, \refEnv{docEnvironment},
  \refEnv{docKey}, etc, then \meta{text} is used
  for as sort key for the index instead of the name of the definition.
\begin{dispListing}
\begin{docCommands}[
    doc name        = l_tcobox_example_tl,
    doc sort index  = example_tl,  % sorted unter e like example
  ]{}
\end{docCommands}
\end{dispListing}
\end{docTcbKey}

\clearpage

\begin{docTcbKey}{doc into index}{\colOpt{=true\textbar false}}{default |true|, initially |true|}
  If set to |false|, no index entries are written for the main documentation
  environments. The same effect is achieved by using e.\,g.\ \refEnv{docCommand*}
  instead of \refEnv{docCommand}.
\end{docTcbKey}


\begin{docTcbKey}[][doc new={2020-04-22}]{doc no index}{}{style, initially unset}
  If set, no index entries are written for the main documentation
  environments. This is a shortcut for using \refKey{/tcb/doc into index}|=false|.
\end{docTcbKey}



\begin{docTcbKey}[][doc new=2014-09-19]{doc marginnote}{=\meta{options}}{no default, initially empty}
  Sets style \meta{options} for the displayed box of the \refCom{tcbdocmarginnote} command.
\begin{dispExample}
\tcbset{doc marginnote={colframe=blue!50!white,colback=blue!5!white}}%
This is some text\tcbdocmarginnote{Note A}
which is commented by a note inside the margin.
\end{dispExample}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-09-19]{doc new}{=\meta{date}}{style, no default}
  Adds a a marginnote with a 'New: \meta{data}' message at the beginning of
  the upper box part. The intended use is inside the option list of
  \refEnv{docCommand}, \refEnv{docEnvironment}, etc.
  \makeatletter\renewcommand*{\tcbdocnew}[1]{\kvtcb@text@new: #1}\makeatother%
\begin{dispExample}
\begin{docCommand}[doc new=2000-01-01]{foosomething}{\marg{text}}
Some command for something.
\end{docCommand}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2014-09-19]{doc updated}{=\meta{date}}{style, no default}
  Adds a marginnote with a 'Updated: \meta{data}' message at the beginning of
  the upper box part. See \refKey{/tcb/doc new}.
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2014-09-19]{doc new and updated}{=\marg{new date}\marg{update date}}{style, no default}
  Adds a marginnote with 'New: \meta{new date}' and 'Updated: \meta{update data}' messages at the beginning of
  the upper box part. See \refKey{/tcb/doc new}.
\end{docTcbKey}



\clearpage
%-------------------------------------------------------------------------------
\subsection{Entry Customization Option Keys}


\begin{docTcbKey}{doc left}{=\meta{length}}{no default, initially |2em|}
  Sets the left hand offset of the documentation texts from
  \refEnv{docCommand}, \refEnv{docEnvironment}, \refEnv{docKey}, etc, to \meta{length}.
\begin{dispExample}
\begin{docCommand*}[doc left=2cm,doc left indent=-2cm]{myCommandA}{\marg{argument}}
  This is the documentation of \refCom{myCommandA} which takes one \meta{argument}.
  \refCom{myCommandA} does some funny things with its \meta{argument}.
\end{docCommand*}
\end{dispExample}
\end{docTcbKey}

\begin{docTcbKey}{doc right}{=\meta{length}}{no default, initially |0em|}
  Sets the right hand offset of the documentation texts from
  \refEnv{docCommand}, \refEnv{docEnvironment}, \refEnv{docKey}, etc, to \meta{length}.
\begin{dispExample}
\begin{docCommand*}[doc right=2cm]{myCommandB}{\marg{argument}}
  This is the documentation of \refCom{myCommandB} which takes one \meta{argument}.
  \refCom{myCommandB} does some funny things with its \meta{argument}.
\end{docCommand*}
\end{dispExample}
\end{docTcbKey}

\begin{docTcbKey}{doc left indent}{=\meta{length}}{no default, initially |-2em|}
  Sets the left hand indent of documentation heads from
  \refEnv{docCommand}, \refEnv{docEnvironment}, \refEnv{docKey}, etc, to \meta{length}.
\begin{dispExample}
\begin{docCommand*}[doc left indent=2cm]{myCommandC}{\marg{argument}}
  This is the documentation of \refCom{myCommandC} which takes one \meta{argument}.
  \refCom{myCommandC} does some funny things with its \meta{argument}.
\end{docCommand*}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{doc right indent}{=\meta{length}}{no default, initially |0pt|}
  Sets the right hand indent of documentation heads from
  \refEnv{docCommand}, \refEnv{docEnvironment}, \refEnv{docKey}, etc, to \meta{length}.
\begin{dispExample}
\begin{docCommand*}[doc right indent=-10mm,doc right=10mm,
    doc description=test value]{myCommandD}{\marg{argument}}
  This is the documentation of \refCom{myCommandD} which takes one \meta{argument}.
  \refCom{myCommandD} does some funny things with its \meta{argument}.
\end{docCommand*}
\end{dispExample}
\end{docTcbKey}

\clearpage
The head lines of the main documentation environments \refEnv{docCommand},
\refEnv{docEnvironment}, \refEnv{docKey}, etc, are |tcolorbox|es inside a
\refEnv{tcbraster}.
Options to the surrounding |tcbraster|s and the embedded
|tcolorbox|es can be given using the following keys.


\begin{docTcbKeys}[
  doc name        = doc raster command,
  doc parameter   = {=\meta{options}},
  doc description = {no default, initially empty},
  doc new         = 2020-04-24,
]{}
  Sets \meta{options} for the surrounding \refEnv{tcbraster} of\\
  \refEnv{docCommand}, \refEnv{docCommand*}, and \refEnv{docCommands}.

\begin{dispExample}
\tcbset{doc raster command={raster before skip=7mm,raster after skip=0mm}}

The is an example text.

\begin{docCommand*}{myCommandI}{\marg{argument}}
  This is the documentation of \refCom{myCommandI} which takes one \meta{argument}.
  \refCom{myCommandI} does some funny things with its \meta{argument}.
\end{docCommand*}
\end{dispExample}

\end{docTcbKeys}


\begin{docTcbKeys}[
  doc name        = doc raster environment,
  doc parameter   = {=\meta{options}},
  doc description = {no default, initially empty},
  doc new         = 2020-04-24,
]{}
  Sets \meta{options} for the surrounding \refEnv{tcbraster} of\\
  \refEnv{docEnvironment}, \refEnv{docEnvironment*}, and \refEnv{docEnvironments}.
\end{docTcbKeys}


\begin{docTcbKeys}[
  doc name        = doc raster key,
  doc parameter   = {=\meta{options}},
  doc description = {no default, initially empty},
  doc new         = 2020-04-24,
]{}
  Sets \meta{options} for the surrounding \refEnv{tcbraster} of\\
  \refEnv{docKey}, \refEnv{docKey*}, and \refEnv{docKeys}.
\end{docTcbKeys}


\begin{docTcbKeys}[
  doc name        = doc raster path,
  doc parameter   = {=\meta{options}},
  doc description = {no default, initially empty},
  doc new         = 2020-04-24,
]{}
  Sets \meta{options} for the surrounding \refEnv{tcbraster} of\\
  \refEnv{docPathOperation}, \refEnv{docPathOperation*}, and \refEnv{docPathOperations}.
\end{docTcbKeys}


\begin{docTcbKeys}[
  doc name        = doc raster,
  doc parameter   = {=\meta{options}},
  doc description = {no default, initially empty},
  doc new         = 2020-04-24,
]{}
  Shortcut for setting the same \meta{options} for
  \refKey{/tcb/doc raster command}, \refKey{/tcb/doc raster environment},
  \refKey{/tcb/doc raster key}, and \refKey{/tcb/doc raster path}.
\end{docTcbKeys}


\begin{docTcbKey}{doc head command}{=\meta{options}}{no default, initially empty}
  Sets \meta{options} for the head line of
  \refEnv{docCommand}, \refEnv{docCommand*}, and \refEnv{docCommands}.
\begin{dispExample}
\tcbset{doc head command={interior style={fill,left color=red!20!white,
  right color=blue!20!white}}}

\begin{docCommand*}{myCommandE}{\marg{argument}}
  This is the documentation of \refCom{myCommandE} which takes one \meta{argument}.
  \refCom{myCommandE} does some funny things with its \meta{argument}.
\end{docCommand*}
\end{dispExample}
\end{docTcbKey}


\clearpage

\begin{docTcbKey}{doc head environment}{=\meta{options}}{no default, initially empty}
  Sets \meta{options} for the head line of
  \refEnv{docEnvironment}, \refEnv{docEnvironment*}, and \refEnv{docEnvironments}.
\begin{dispExample}
\tcbset{doc head environment={beamer,boxsep=2pt,arc=2pt,colback=green!20!white}}

\begin{docEnvironment*}{myEnvironment}{\marg{argument}}
  This is the documentation of \refEnv{myEnvironment} which
  takes one \meta{argument}.
\end{docEnvironment*}
\end{dispExample}
\end{docTcbKey}

\begin{docTcbKey}{doc head key}{=\meta{options}}{no default, initially empty}
  Sets \meta{options} for the head line of
  \refEnv{docKey}, \refEnv{docKey*}, and \refEnv{docKeys}.
\begin{dispExample}
\tcbset{doc head key={boxsep=4pt,arc=4pt,boxrule=0.6pt,
  frame style=fill,interior style=fill,colframe=green!50!black}}

\begin{docKey}{/foo/myKey}{}{no value}
  This is the documentation of \refKey{/foo/myKey}.
\end{docKey}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2019-09-18]{doc head path}{=\meta{options}}{no default, initially empty}
  Sets \meta{options} for the head line of
  \refEnv{docPathOperation}, \refEnv{docPathOperation*}, and \refEnv{docPathOperations}.
\begin{dispExample}
\tcbset{doc head command={interior style={fill,left color=red!7!white,
  right color=blue!7!white}}}

\begin{docPathOperation*}{-{}-}{\meta{coordinate or cycle}}
  This is the documentation of \refPathOperation{-{}-}.
\end{docPathOperation*}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc updated=2019-09-18]{doc head}{=\meta{options}}{no default, initially empty}
  Shortcut for setting the same \meta{options} for
  \refKey{/tcb/doc head command}, \refKey{/tcb/doc head environment},
  \refKey{/tcb/doc head key}, and \refKey{/tcb/doc head path}.
\end{docTcbKey}


\clearpage

The description texts of the main documentation environments \refEnv{docCommand},
\refEnv{docEnvironment}, \refEnv{docKey}, etc, are set in a compact form without
indention and |parskip=0pt|. This settings can overruled by using the following
keys to insert code before (or after) the description texts.

\begin{docTcbKey}[][doc new=2015-10-09]{before doc body command}{=\meta{code}}{no default, initially empty}
  Executes \meta{code} before the description texts
  of \refEnv{docCommand} and \refEnv{docCommand*}.
\begin{dispExample}
\tcbset{before doc body command={%
    \setlength{\parindent}{2.5em}%
    \setlength{\parskip}{1ex plus 0.75ex minus 0.25ex}%
}}

\begin{docCommand*}{myCommandG}{\marg{argument}}
  This is the documentation of \refCom{myCommandG} which takes one \meta{argument}.
  \refCom{myCommandG} does some funny things with its \meta{argument}.
\end{docCommand*}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2015-10-09]{after doc body command}{=\meta{code}}{no default, initially empty}
  Executes \meta{code} after the description texts
  of \refEnv{docCommand} and \refEnv{docCommand*}.
\begin{dispExample}
\tcbset{after doc body command={%
    \hfill\nolinebreak[1]\hspace*{\fill}\textcolor{red}{$\diamondsuit$}%
}}

\begin{docCommand*}{myCommandH}{\marg{argument}}
  This is the documentation of \refCom{myCommandH} which takes one \meta{argument}.
  \refCom{myCommandH} does some funny things with its \meta{argument}.
\end{docCommand*}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2015-10-09]{before doc body environment}{=\meta{code}}{no default, initially empty}
  Executes \meta{code} before the description texts
  of \refEnv{docEnvironment} and \refEnv{docEnvironment*}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-10-09]{after doc body environment}{=\meta{code}}{no default, initially empty}
  Executes \meta{code} after the description texts
  of \refEnv{docEnvironment} and \refEnv{docEnvironment*}.
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2015-10-09]{before doc body key}{=\meta{code}}{no default, initially empty}
  Executes \meta{code} before the description texts
  of \refEnv{docKey} and \refEnv{docKey*}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-10-09]{after doc body key}{=\meta{code}}{no default, initially empty}
  Executes \meta{code} after the description texts
  of \refEnv{docKey} and \refEnv{docKey*}.
\end{docTcbKey}

\clearpage

\begin{docTcbKey}[][doc new=2019-09-18]{before doc body path}{=\meta{code}}{no default, initially empty}
  Executes \meta{code} before the description texts
  of \refEnv{docPathOperation} and \refEnv{docPathOperation*}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2019-09-18]{after doc body path}{=\meta{code}}{no default, initially empty}
  Executes \meta{code} after the description texts
  of \refEnv{docPathOperation} and \refEnv{docPathOperation*}.
\end{docTcbKey}


\begin{docTcbKey}[][doc new and updated={2015-10-09}{2019-09-18}]{before doc body}{=\meta{options}}{no default, initially empty}
  Shortcut for setting the same \meta{options} for
  \refKey{/tcb/before doc body command}, \refKey{/tcb/before doc body environment},
  \refKey{/tcb/before doc body key}, and \refKey{/tcb/before doc body path}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new and updated={2015-10-09}{2019-09-18}]{after doc body}{=\meta{options}}{no default, initially empty}
  Shortcut for setting the same \meta{options} for
  \refKey{/tcb/after doc body command}, \refKey{/tcb/after doc body environment},
  \refKey{/tcb/after doc body key}, and \refKey{/tcb/after doc body path}.
\end{docTcbKey}







\clearpage
\subsection{General Customization Option Keys}

\begin{docTcbKey}[][doc updated=2015-03-16]{docexample}{}{style, no value}
  Sets the style for \refEnv{dispExample} and \refEnv{dispListing}
  with the colors |ExampleBack| and |ExampleFrame|.
  To change the appearance of the examples, this style can be
  redefined.
\begin{dispListing}
% Predefined style:
\tcbset{
  docexample/.style={colframe=ExampleFrame,colback=ExampleBack,
    before skip=\medskipamount,after skip=\medskipamount,
    fontlower=\footnotesize}
}
\end{dispListing}
\end{docTcbKey}

\begin{docTcbKey}{documentation listing options}{=\meta{key list}}{no default,\\\hspace*{\fill} initially |style=tcbdocumentation|}
  Sets the options from the package |listings| \cite{hoffmann:listings}.
  They are used inside \refEnv{dispExample} and \refEnv{dispListing} to typeset
  the listings. Note that this is not identical to the key
  \refKey{/tcb/listing options} which is used for 'normal' listings.\\
  Used for \refKey{/tcb/listing engine}|=listings| only.
\end{docTcbKey}

\begin{docTcbKey}{documentation listing style}{=\meta{listing style}}{no default, initially |tcbdocumentation|}
  Abbreviation for |documentation listing options={style=...}|.
  This key sets a \meta{style}
  for the |listings| package, see \cite{hoffmann:listings}.
  Note that this is not identical to the key
  \refKey{/tcb/listing style} which is used for 'normal' listings.\\
  Used for \refKey{/tcb/listing engine}|=listings| only.
\end{docTcbKey}

\begin{docTcbKey}{documentation minted options}{=\meta{minted style}}{no default,\\\hspace*{\fill} initially |tabsize=2,fontsize=\textbackslash small|}
  Sets the options from the package |minted| \cite{poore:minted}
  which are used during typesetting of the listing, if used.
  Note that this is not identical to the key
  \refKey{/tcb/minted options} which is used for 'normal' listings.\\
  Used for \refKey{/tcb/listing engine}|=minted| only.
\end{docTcbKey}

\begin{docTcbKey}{documentation minted style}{=\meta{key list}}{no default, initially unset}
  Sets a \meta{style} known to |Pygments| \cite{pygments:web} for
  the package |minted| \cite{poore:minted}, if used.
  Note that this is not identical to the key
  \refKey{/tcb/minted style} which is used for 'normal' listings.\\
  Used for \refKey{/tcb/listing engine}|=minted| only.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2017-04-24]{documentation minted language}{=\meta{programming language}}{no default, initially |latex|}
  Sets a \meta{programming language} known to |Pygments| \cite{pygments:web}
  for the package |minted| \cite{poore:minted}, if used.
  Note that this is not identical to the key
  \refKey{/tcb/minted language} which is used for 'normal' listings.\\
  Used for \refKey{/tcb/listing engine}|=minted| only.
\end{docTcbKey}


\begin{marker}
The following two keys are deprecated and without function (v3.50 and above).
Use \refKey{/tcb/before} and \refKey{/tcb/after} with appropriate values
instead. Also see \refKey{/tcb/docexample}.
\end{marker}

\begin{docTcbKey}[][doc updated=2015-03-16]{before example}{=\meta{macros}}{no default, initially empty}
\smallskip\begin{deprecated}
  Sets the \meta{macros} which are executed before \refEnv{dispExample} and \refEnv{dispListing}
  additional to \refKey{/tcb/before}.
\end{deprecated}
\end{docTcbKey}

\begin{docTcbKey}{after example}{=\meta{macros}}{no default, initially empty}
\smallskip\begin{deprecated}
  Sets the \meta{macros} which are executed after \refEnv{dispExample} and \refEnv{dispListing}
  additional to \refKey{/tcb/after}.
\end{deprecated}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}[][doc new=2017-04-25]{keywords bold}{\colOpt{=true\textbar false}}{default |true|, initially |true|}
  Keyword used in \refEnv{docEnvironment}, \refEnv{docCommand}, etc. are printed
  boldface (or not). Since the typewriter font is used, the effect may be
  invisible with Computer Modern fonts or similar which do not
  have a bold variant. Note that references to keywords are not printed boldface at all.
\begin{dispExample*}{sidebyside}
\LARGE
\docAuxCommand{fooaux}, \refCom{tcbset}

\tcbset{keywords bold=false}
\docAuxCommand{fooaux}, \refCom{tcbset}
\end{dispExample*}
\end{docTcbKey}



\begin{docTcbKey}[][doc new=2015-01-09]{index command}{=\meta{macro}}{no default, initially \cs{index}}
  Replaces the internally used \cs{index} macro by the given \meta{macro}.
  The \meta{macro} has to take one mandatory argument like \cs{index}.
  This option is mutually exclusive with \refKey{/tcb/index command name}.
\begin{dispListing}
\tcbset{index command=\myindexcommand}
\end{dispListing}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2015-01-09]{index command name}{=\meta{name}}{no default, initially unset}
  Replaces the internally used \cs{index} macro by
  \mbox{\cs{index}\texttt{[\meta{name}]}}, i.e.\ 
  \mbox{\cs{index}\texttt{\textbraceleft\ldots\textbraceright}} is replaced by
  \mbox{\cs{index}\texttt{[\meta{name}]\textbraceleft\ldots\textbraceright}}.
  This option is intended to be used with |imakeidx| and is
  mutually exclusive with \refKey{/tcb/index command}.
\begin{dispListing}
\tcbset{index command name=mydoc}
\end{dispListing}
\end{docTcbKey}



\begin{docTcbKey}{index format}{=\meta{format}}{no default, initially |pgf|}
  Determines the basic \meta{format} of the generated index.
  Feasible values are:
  \begin{itemize}
  \item\docValue{pgfsection}: The index is formatted like in the |pgf| documentation (as a section).
  \item\docValue{pgfchapter}: The index is formatted like in the |pgf| documentation (as a chapter).
  \item\docValue{pgf}: Alias for |pgfsection|.
  \item\docValue{doc}: The index is assumed to be formatted by |doc| or |ltxdoc|. The usage of |makeindex|
    with |-s gind.ist| is assumed. The package |hypdoc| has to be loaded
    \emph{before} |tcolorbox|. Only a limited set of customizations will
    work! This option cannot be unset when used!
  \item\docValue{off}: The index is not formatted by |tcolorbox|. Use this, if
    the index is formatted by other package like |imakeidx|.
  \end{itemize}
\end{docTcbKey}


\begin{docTcbKey}{index actual}{=\meta{character}}{no default, initially |@|}
  Sets the character for 'actual' in automatic indexing.
\end{docTcbKey}

\begin{docTcbKey}{index quote}{=\meta{character}}{no default, initially |"|}
  Sets the character for 'quote' in automatic indexing.
\end{docTcbKey}

\begin{docTcbKey}{index level}{=\meta{character}}{no default, initially |!|}
  Sets the character for 'level' in automatic indexing.
\end{docTcbKey}

\begin{docTcbKey}{index default settings}{}{style, no value}
  Sets the |makeindex| default values for
  \refKey{/tcb/index actual},
  \refKey{/tcb/index quote}, and
  \refKey{/tcb/index level}.
\end{docTcbKey}


\begin{docTcbKey}{index german settings}{}{style, no value}
  Sets the |makeindex| values recommended for German language texts.
  This is identical to setting the following:
\begin{dispListing}
\tcbset{index actual={=},index quote={!},index level={>}}
\end{dispListing}
\end{docTcbKey}

\clearpage

\begin{docTcbKey}{index annotate}{\colOpt{=true\textbar false}}{default |true|, initially |true|}
  If set to |true|, the index entries are annotated with short descriptions
  given by \refKey{/tcb/doclang/environment}, \refKey{/tcb/doclang/key},
  and others.
\end{docTcbKey}

\begin{docTcbKey}{index colorize}{\colOpt{=true\textbar false}}{default |true|, initially |false|}
  If set to |true|, the index entries colorized according to the color
  settings given by \refKey{/tcb/color environment}, \refKey{/tcb/color key},
  and others.
\end{docTcbKey}


\begin{docTcbKey}{color command}{=\meta{color}}{no default, initially |Definition|}
  Sets the highlight color used by macro definitions.
\end{docTcbKey}

\begin{docTcbKey}{color environment}{=\meta{color}}{no default, initially |Definition|}
  Sets the highlight color used by environment definitions.
\end{docTcbKey}

\begin{docTcbKey}{color key}{=\meta{color}}{no default, initially |Definition|}
  Sets the highlight color used by key definitions.
\end{docTcbKey}

\begin{docTcbKey}[][doc new={2019-09-18}]{color path}{=\meta{color}}{no default, initially |Definition|}
  Sets the highlight color used by \tikzname\ path operation definitions.
\end{docTcbKey}

\begin{docTcbKey}{color value}{=\meta{color}}{no default, initially |Definition|}
  Sets the highlight color used by value definitions.
\end{docTcbKey}

\begin{docTcbKey}[][doc new={2015-01-08}]{color counter}{=\meta{color}}{no default, initially |Definition|}
  Sets the highlight color used by counter definitions.
\end{docTcbKey}

\begin{docTcbKey}[][doc new={2015-01-08}]{color length}{=\meta{color}}{no default, initially |Definition|}
  Sets the highlight color used by length definitions.
\end{docTcbKey}

\begin{docTcbKey}{color color}{=\meta{color}}{no default, initially |Definition|}
  Sets the highlight color used by color definitions.
\end{docTcbKey}

\begin{docTcbKey}[][doc updated={2019-09-18}]{color definition}{=\meta{color}}{no default, initially |Definition|}
  Sets the highlight color for \refKey{/tcb/color command}, \refKey{/tcb/color environment},
  \refKey{/tcb/color key}, \refKey{/tcb/color path}, \refKey{/tcb/color value}, \refKey{/tcb/color counter},
  \refKey{/tcb/color length}, and \refKey{/tcb/color color}.
\end{docTcbKey}

\begin{docTcbKey}{color option}{=\meta{color}}{no default, initially |Option|}
  Sets the color used for optional arguments.
\end{docTcbKey}

\begin{docTcbKey}{color fade}{=\meta{color}}{no default, initially |Fade|}
  Sets the color used for faded text like \colFade{\textbackslash path}
  in \refEnv{docPathOperation}.
\end{docTcbKey}


\begin{docTcbKey}{color hyperlink}{=\meta{color}}{no default, initially |Hyperlink|}
  Sets the color for all hyper-links, i.\,e. all internal and external links.
\end{docTcbKey}


\clearpage
%-------------------------------------------------------------------------------
\subsection{Language Option Keys}

The following keys are provided for language specific settings.
The English language is predefined.

\begin{docTcbKey}{english language}{}{style, no value}
  Sets all language specific settings to English.
\end{docTcbKey}

\begin{langTcbKey}{color}{=\meta{text}}{no default, initially |color|}
  Text used in the index for colors.
\end{langTcbKey}

\begin{langTcbKey}{colors}{=\meta{text}}{no default, initially |Colors|}
  Heading text in the index for colors.
\end{langTcbKey}

\begin{langTcbKey}[][doc new={2015-01-08}]{counter}{=\meta{text}}{no default, initially |counter|}
  Text used in the index for counters.
\end{langTcbKey}

\begin{langTcbKey}[][doc new={2015-01-08}]{counters}{=\meta{text}}{no default, initially |Counters|}
  Heading text in the index for counters.
\end{langTcbKey}

\begin{langTcbKey}{environment}{=\meta{text}}{no default, initially |environment|}
  Text used in the index for environments.
\end{langTcbKey}

\begin{langTcbKey}{environments}{=\meta{text}}{no default, initially |Environments|}
  Heading text in the index for environments.
\end{langTcbKey}

\begin{langTcbKey}{environment content}{=\meta{text}}{no default, initially |environment content|}
  Text used in \refEnv{docEnvironment}.
\end{langTcbKey}

\begin{langTcbKey}{index}{=\meta{text}}{no default, initially |Index|}
  Heading text for the index.
\end{langTcbKey}

\begin{langTcbKey}{key}{=\meta{text}}{no default, initially |key|}
  Text used in the index for keys.
\end{langTcbKey}

\begin{langTcbKey}{keys}{=\meta{text}}{no default, initially |Keys|}
  Heading text used in the index for keys.
\end{langTcbKey}

\begin{langTcbKey}[][doc new={2015-01-08}]{length}{=\meta{text}}{no default, initially |length|}
  Text used in the index for lengths.
\end{langTcbKey}

\begin{langTcbKey}[][doc new={2015-01-08}]{lengths}{=\meta{text}}{no default, initially |Lengths|}
  Heading text in the index for lengths.
\end{langTcbKey}

\begin{langTcbKey}[][doc new={2014-09-19}]{new}{=\meta{text}}{no default, initially |New|}
  Announcement text for new content.
\end{langTcbKey}

\begin{langTcbKey}[][doc new={2019-09-18}]{path}{=\meta{text}}{no default, initially |path operation|}
  Text used in the index for path operations.
\end{langTcbKey}

\begin{langTcbKey}[][doc new={2019-09-18}]{paths}{=\meta{text}}{no default, initially |Path operations|}
  Heading text in the index for path operations.
\end{langTcbKey}

\begin{langTcbKey}{pageshort}{=\meta{text}}{no default, initially |P.|}
  Short text for page references.
\end{langTcbKey}

\begin{langTcbKey}[][doc new={2014-09-19}]{updated}{=\meta{text}}{no default, initially |Updated|}
  Announcement text for updated content.
\end{langTcbKey}

\begin{langTcbKey}{value}{=\meta{text}}{no default, initially |value|}
  Text used in the index for values.
\end{langTcbKey}

\begin{langTcbKey}{values}{=\meta{text}}{no default, initially |Values|}
  Heading text in the index for values.
\end{langTcbKey}






\clearpage



\subsection{Predefined Colors of the Library}\tcbdocmarginnote{\tcbdocupdated{2019-09-18}}
The following colors are predefined. They are used as default colors
in some library commands.

\def\dispColor#1{\docColor{#1}~\tikz[baseline=1mm]\path[fill=#1,draw] (0,0) rectangle (0.4,0.4);~}

\dispColor{Option},
\dispColor{Definition},
\dispColor{ExampleFrame},
\dispColor{ExampleBack},
\dispColor{Hyperlink},
\dispColor{Fade}.




==> tcolorbox.doc.filling.tex <==
% !TeX root = tcolorbox.tex
% include file of tcolorbox.tex (manual of the LaTeX package tcolorbox)
\clearpage
\section{\tikzname\ Image and Picture Fill Extensions; Auxiliary Macros}\label{sec:tikzimagefilling}%
\tcbset{external/prefix=external/filling_}%
The \mylib{skins} library adds some image and picture fill options to the vast option set of
\tikzname\ \cite{tantau:tikz_and_pgf}. These options can be used in any |tikzpicture|.
For the following options, the \mylib{skins} library has to be loaded
by a package option or inside the preamble by:
\begin{dispListing}
\tcbuselibrary{skins}
\end{dispListing}

See \Vref{sec:skins} for the documentation of all other options of the \mylib{skins} library.

\subsection{Fill Plain}
\begin{docTikzKey}{fill plain image}{=\meta{file name}}{no default, initially unset}
  Fills the current path with an external image referenced by \meta{file name}.
  The image is put in the center of the path, but it is not resized to fit into
  the path area.
\begin{dispExample*}{sbs,lefthand ratio=0.66,right=2mm,sidebyside gap=5mm,center lower}
\begin{tikzpicture}
\path[draw,fill plain image=goldshade.png]
  (2.75,-0.75) -- (3,0) -- (2.75,0.75)
  \foreach \w in {45,90,...,315}
    { -- (\w:1.5cm) } -- cycle;
\end{tikzpicture}
\end{dispExample*}
\end{docTikzKey}


\begin{docTikzKey}{fill plain image*}{=\meta{file name}}{no default, initially unset}
  Fills the current path with an external image referenced by \meta{file name}.
  The image is put in the center of the path, but it is not resized to fit into
  the path area.
  The \meta{graphics options} are given to the underlying \docAuxCommand*{includegraphics} command.
\begin{dispExample*}{sbs,lefthand ratio=0.66,right=2mm,sidebyside gap=5mm,center lower}
\begin{tikzpicture}
\path[draw,
    fill plain image*={width=2.5cm}{goldshade.png}]
  (2.75,-0.75) -- (3,0) -- (2.75,0.75)
  \foreach \w in {45,90,...,315}
    { -- (\w:1.5cm) } -- cycle;
\end{tikzpicture}
\end{dispExample*}
\end{docTikzKey}


\begin{docTikzKey}{fill plain picture}{=\meta{graphical code}}{no default, initially unset}
  Fills the current path with the given \meta{graphical code}.
  The result is put in the center of the path, but it is not resized to fit into
  the path area. Note that this is almost identical to the standard |path picture| option.
\begin{dispExample*}{sbs,lefthand ratio=0.66,right=2mm,sidebyside gap=5mm,center lower}
\begin{tikzpicture}
\path[draw,fill plain picture={%
  \draw[red!50!yellow,line width=2mm]
    (0,0) circle (1cm);
  \draw[red,line width=5mm] (-1,-1) -- (1,1);
  \draw[red,line width=5mm] (-1,1) -- (1,-1);
  }]
  (2.75,-0.75) -- (3,0) -- (2.75,0.75)
  \foreach \w in {45,90,...,315}
    { -- (\w:1.5cm) } -- cycle;
\end{tikzpicture}
\end{dispExample*}
\end{docTikzKey}


\clearpage
\subsection{Fill Stretch}
\begin{docTikzKey}{fill stretch image}{=\meta{file name}}{no default, initially unset}
  Fills the current path with an external image referenced by \meta{file name}.
  The image is stretched to fill the path area.
\begin{dispExample*}{sbs,lefthand ratio=0.66,right=2mm,sidebyside gap=5mm,center lower}
\begin{tikzpicture}
\path[fill stretch image=goldshade.png]
  (2.75,-0.75) -- (3,0) -- (2.75,0.75)
  \foreach \w in {45,90,...,315}
    { -- (\w:1.5cm) } -- cycle;
\end{tikzpicture}
\end{dispExample*}
\end{docTikzKey}


\begin{docTikzKey}{fill stretch image*}{=\marg{graphics options}\marg{file name}}{no default, initially unset}
  Fills the current path with an external image referenced by \meta{file name}.
  The \meta{graphics options} are given to the underlying \docAuxCommand*{includegraphics} command.
  The image is stretched to fill the path area.
\begin{dispExample*}{sbs,lefthand ratio=0.66,right=2mm,sidebyside gap=5mm,center lower}
\begin{tikzpicture}
\path[fill stretch image*=
  {angle=90,origin=c}{goldshade.png}]
  (2.75,-0.75) -- (3,0) -- (2.75,0.75)
  \foreach \w in {45,90,...,315}
    { -- (\w:1.5cm) } -- cycle;
\end{tikzpicture}
\end{dispExample*}
\end{docTikzKey}


\begin{docTikzKey}{fill stretch picture}{=\meta{graphical code}}{no default, initially unset}
  Fills the current path with the given \meta{graphical code}.
  The result is stretched to fill the path area.
\begin{dispExample*}{sbs,lefthand ratio=0.66,right=2mm,sidebyside gap=5mm,center lower}
\begin{tikzpicture}
\path[draw,fill stretch picture={%
  \draw[red!50!yellow,line width=2mm]
    (0,0) circle (1cm);
  \draw[red,line width=5mm] (-1,-1) -- (1,1);
  \draw[red,line width=5mm] (-1,1) -- (1,-1);
  }]
  (2.75,-0.75) -- (3,0) -- (2.75,0.75)
  \foreach \w in {45,90,...,315}
    { -- (\w:1.5cm) } -- cycle;
\end{tikzpicture}
\end{dispExample*}
\end{docTikzKey}


\clearpage
\subsection{Fill Overzoom}
\begin{docTikzKey}{fill overzoom image}{=\meta{file name}}{no default, initially unset}
  Fills the current path with an external image referenced by \meta{file name}.
  The image is zoomed such that the path area fills the image.
\begin{dispExample*}{sbs,lefthand ratio=0.66,right=2mm,sidebyside gap=5mm,center lower}
\begin{tikzpicture}
\path[fill overzoom image=goldshade.png]
  (2.75,-0.75) -- (3,0) -- (2.75,0.75)
  \foreach \w in {45,90,...,315}
    { -- (\w:1.5cm) } -- cycle;
\end{tikzpicture}
\end{dispExample*}
\end{docTikzKey}


\begin{docTikzKey}{fill overzoom image*}{=\marg{graphics options}\marg{file name}}{no default, initially unset}
  Fills the current path with an external image referenced by \meta{file name}.
  The \meta{graphics options} are given to the underlying \docAuxCommand*{includegraphics} command.
  The image is zoomed such that the path area fills the image.
\begin{dispExample*}{sbs,lefthand ratio=0.66,right=2mm,sidebyside gap=5mm,center lower}
\begin{tikzpicture}
\path[fill overzoom image*=
  {angle=90,origin=c}{goldshade.png}]
  (2.75,-0.75) -- (3,0) -- (2.75,0.75)
  \foreach \w in {45,90,...,315}
    { -- (\w:1.5cm) } -- cycle;
\end{tikzpicture}
\end{dispExample*}
\end{docTikzKey}


\begin{docTikzKey}{fill overzoom picture}{=\meta{graphical code}}{no default, initially unset}
  Fills the current path with the given \meta{graphical code}.
  The result is zoomed such that the path area fills the image.
\begin{dispExample*}{sbs,lefthand ratio=0.66,right=2mm,sidebyside gap=5mm,center lower}
\begin{tikzpicture}
\path[draw,fill overzoom picture={%
  \draw[red!50!yellow,line width=2mm]
    (0,0) circle (1cm);
  \draw[red,line width=5mm] (-1,-1) -- (1,1);
  \draw[red,line width=5mm] (-1,1) -- (1,-1);
  }]
  (2.75,-0.75) -- (3,0) -- (2.75,0.75)
  \foreach \w in {45,90,...,315}
    { -- (\w:1.5cm) } -- cycle;
\end{tikzpicture}
\end{dispExample*}
\end{docTikzKey}


\clearpage
\subsection{Fill Zoom}
\begin{docTikzKey}{fill zoom image}{=\meta{file name}}{no default, initially unset}
  Fills the current path with an external image referenced by \meta{file name}.
  The image is zoomed such that it fits inside the path area.
  Typically, some parts of the path area will stay unfilled.
\begin{dispExample*}{sbs,lefthand ratio=0.66,right=2mm,sidebyside gap=5mm,center lower}
\begin{tikzpicture}
\path[draw,fill zoom image=goldshade.png]
  (2.75,-0.75) -- (3,0) -- (2.75,0.75)
  \foreach \w in {45,90,...,315}
    { -- (\w:1.5cm) } -- cycle;
\end{tikzpicture}
\end{dispExample*}
\end{docTikzKey}


\begin{docTikzKey}{fill zoom image*}{=\marg{graphics options}\marg{file name}}{no default, initially unset}
  Fills the current path with an external image referenced by \meta{file name}.
  The \meta{graphics options} are given to the underlying \docAuxCommand*{includegraphics} command.
  The image is zoomed such that it fits inside the path area.
  Typically, some parts of the path area will stay unfilled.
\begin{dispExample*}{sbs,lefthand ratio=0.66,right=2mm,sidebyside gap=5mm,center lower}
\begin{tikzpicture}
\path[draw,fill zoom image*=
  {angle=90,origin=c}{goldshade.png}]
  (2.75,-0.75) -- (3,0) -- (2.75,0.75)
  \foreach \w in {45,90,...,315}
    { -- (\w:1.5cm) } -- cycle;
\end{tikzpicture}
\end{dispExample*}
\end{docTikzKey}


\begin{docTikzKey}{fill zoom picture}{=\meta{graphical code}}{no default, initially unset}
  Fills the current path with the given \meta{graphical code}.
  The result is zoomed such that it fits inside the path area.
  Typically, some parts of the path area will stay unfilled.
\begin{dispExample*}{sbs,lefthand ratio=0.66,right=2mm,sidebyside gap=5mm,center lower}
\begin{tikzpicture}
\path[draw,fill zoom picture={%
  \draw[red!50!yellow,line width=2mm]
    (0,0) circle (1cm);
  \draw[red,line width=5mm] (-1,-1) -- (1,1);
  \draw[red,line width=5mm] (-1,1) -- (1,-1);
  }]
  (2.75,-0.75) -- (3,0) -- (2.75,0.75)
  \foreach \w in {45,90,...,315}
    { -- (\w:1.5cm) } -- cycle;
\end{tikzpicture}
\end{dispExample*}
\end{docTikzKey}


\clearpage
\subsection{Fill Shrink}
\begin{docTikzKey}{fill shrink image}{=\meta{file name}}{no default, initially unset}
  Fills the current path with an external image referenced by \meta{file name}.
  The image is zoomed such that it fits inside the path area, but it never
  gets enlarged.
  Typically, some parts of the path area will stay unfilled.
\begin{dispExample*}{sbs,lefthand ratio=0.66,right=2mm,sidebyside gap=5mm,center lower}
\begin{tikzpicture}
\path[draw,fill shrink image=goldshade.png]
  (2.75,-0.75) -- (3,0) -- (2.75,0.75)
  \foreach \w in {45,90,...,315}
    { -- (\w:1.5cm) } -- cycle;
\end{tikzpicture}
\end{dispExample*}
\end{docTikzKey}


\begin{docTikzKey}{fill shrink image*}{=\meta{file name}}{no default, initially unset}
  Fills the current path with an external image referenced by \meta{file name}.
  The \meta{graphics options} are given to the underlying \docAuxCommand*{includegraphics} command.
  The image is zoomed such that it fits inside the path area, but it never
  gets enlarged.
  Typically, some parts of the path area will stay unfilled.
\begin{dispExample*}{sbs,lefthand ratio=0.66,right=2mm,sidebyside gap=5mm,center lower}
\begin{tikzpicture}
\path[draw,
    fill shrink image*={width=1.5cm}{goldshade.png}]
  (2.75,-0.75) -- (3,0) -- (2.75,0.75)
  \foreach \w in {45,90,...,315}
    { -- (\w:1.5cm) } -- cycle;
\end{tikzpicture}
\end{dispExample*}
\end{docTikzKey}


\begin{docTikzKey}{fill shrink picture}{=\meta{graphical code}}{no default, initially unset}
  Fills the current path with the given \meta{graphical code}.
  The result is zoomed such that it fits inside the path area, but it never
  gets enlarged.
  Typically, some parts of the path area will stay unfilled.
\begin{dispExample*}{sbs,lefthand ratio=0.66,right=2mm,sidebyside gap=5mm,center lower}
\begin{tikzpicture}
\path[draw,fill shrink picture={%
  \draw[red!50!yellow,line width=2mm]
    (0,0) circle (1cm);
  \draw[red,line width=5mm] (-1,-1) -- (1,1);
  \draw[red,line width=5mm] (-1,1) -- (1,-1);
  }]
  (2.75,-0.75) -- (3,0) -- (2.75,0.75)
  \foreach \w in {45,90,...,315}
    { -- (\w:1.5cm) } -- cycle;
\end{tikzpicture}
\end{dispExample*}
\end{docTikzKey}


\clearpage
\subsection{Fill Tile}
\begin{docTikzKey}{fill tile image}{=\meta{file name}}{no default, initially unset}
  Fills the current path with a tile pattern using an external image referenced by \meta{file name}.
\begin{dispExample*}{sbs,lefthand ratio=0.66,right=2mm,sidebyside gap=5mm,center lower}
\begin{tikzpicture}
\path[fill tile image=pink_marble.png]
  (2.75,-0.75) -- (3,0) -- (2.75,0.75)
  \foreach \w in {45,90,...,315}
    { -- (\w:1.5cm) } -- cycle;
\end{tikzpicture}
\end{dispExample*}
\end{docTikzKey}


\begin{docTikzKey}{fill tile image*}{=\marg{graphics options}\marg{file name}}{no default, initially unset}
  Fills the current path with a tile pattern using an external image referenced by \meta{file name}.
  The \meta{graphics options} are given to the underlying \docAuxCommand*{includegraphics} command.
\begin{dispExample*}{sbs,lefthand ratio=0.66,right=2mm,sidebyside gap=5mm,center lower}
\begin{tikzpicture}
\path[fill tile image*={width=1cm}{pink_marble.png}]
  (2.75,-0.75) -- (3,0) -- (2.75,0.75)
  \foreach \w in {45,90,...,315}
    { -- (\w:1.5cm) } -- cycle;
\end{tikzpicture}
\end{dispExample*}
\end{docTikzKey}

\begin{docTikzKey}{fill tile picture}{=\meta{graphical code}}{no default, initially unset}
  Fills the current path with a tile pattern using the given \meta{graphical code}.
\begin{dispExample*}{sbs,lefthand ratio=0.66,right=2mm,sidebyside gap=5mm,center lower}
\begin{tikzpicture}
\path[draw,fill tile picture={%
  \draw[red!50!yellow,line width=2mm]
    (0,0) circle (1cm);
  \draw[red,line width=5mm] (-1,-1) -- (1,1);
  \draw[red,line width=5mm] (-1,1) -- (1,-1);
  }]
  (2.75,-0.75) -- (3,0) -- (2.75,0.75)
  \foreach \w in {45,90,...,315}
    { -- (\w:1.5cm) } -- cycle;
\end{tikzpicture}
\end{dispExample*}
\end{docTikzKey}


\begin{docTikzKey}{fill tile picture*}{=\marg{fraction}\marg{graphical code}}{no default, initially unset}
  Fills the current path with a tile pattern using the given \meta{graphical code}.
  The graphic is resized by \meta{fraction}.
\begin{dispExample*}{sbs,lefthand ratio=0.66,right=2mm,sidebyside gap=5mm,center lower}
\begin{tikzpicture}
\path[draw,fill tile picture*={0.25}{%
  \draw[red!50!yellow,line width=2mm]
    (0,0) circle (1cm);
  \draw[red,line width=5mm] (-1,-1) -- (1,1);
  \draw[red,line width=5mm] (-1,1) -- (1,-1);
  }]
  (2.75,-0.75) -- (3,0) -- (2.75,0.75)
  \foreach \w in {45,90,...,315}
    { -- (\w:1.5cm) } -- cycle;
\end{tikzpicture}
\end{dispExample*}
\end{docTikzKey}


\clearpage
\subsection{Filling Options}
\begin{docTikzKey}{fill image opacity}{=\meta{fraction}}{no default, initially |1.0|}
  Sets the fill opacity for the image or picture fill options to the given \meta{fraction}.
\begin{dispExample}
\begin{tikzpicture}
\path[fill stretch image=goldshade.png] (0,0) circle (1cm);
\path[fill=red,fill stretch image=goldshade.png,fill image opacity=0.75]
  (2,0) circle (1cm);
\path[fill=red,fill stretch image=goldshade.png,fill image opacity=0.5]
  (4,0) circle (1cm);
\path[fill=red,fill stretch image=goldshade.png,fill image opacity=0.25]
  (6,0) circle (1cm);
\path[fill=red] (8,0) circle (1cm);
\end{tikzpicture}
\end{dispExample}
\end{docTikzKey}


\begin{docTikzKey}{fill image scale}{=\meta{fraction}}{no default, initially |1.0|}
  Stretches, zooms, overzooms or shrinks the image or picture to the given \meta{fraction} of the
  width and height of the current path.
\begin{dispExample}
\begin{tikzpicture}
\path[draw,fill zoom image=goldshade.png]
  (0,0) rectangle +(2,2);

\path[draw,fill zoom image=goldshade.png,fill image scale=0.75]
  (3,0) rectangle +(2,2);

\path[draw,fill zoom image=goldshade.png,fill image scale=1.5]
  (6,0) rectangle +(2,2);
\end{tikzpicture}
\end{dispExample}
\end{docTikzKey}


\begin{docTikzKey}[][doc updated=2018-03-18]{fill image options}{=\meta{graphics options}}{no default, initially empty}
  The \meta{graphics options} are given to the underlying \docAuxCommand*{includegraphics} command
  for the image fill options. This can be just together with
  \refKey{/tikz/fill stretch image}, \refKey{/tikz/fill overzoom image}, \refKey{/tikz/fill zoom image},
  and \refKey{/tikz/fill tile image}.
\begin{dispExample*}{sbs,lefthand ratio=0.66,right=2mm,sidebyside gap=5mm,center lower}
\begin{tikzpicture}
\path[fill image options={width=1cm},
  fill tile image=pink_marble.png]
  (2.75,-0.75) -- (3,0) -- (2.75,0.75)
  \foreach \w in {45,90,...,315}
    { -- (\w:1.5cm) } -- cycle;
\end{tikzpicture}
\end{dispExample*}
\end{docTikzKey}


\begin{dispExample*}{sbs,lefthand ratio=0.6,center lower,fonttitle=\bfseries,
  title=Image blending example}
\begin{tikzpicture}[every node/.style=
  {circle,minimum width=2cm}]
\node[fill stretch image=blueshade.png]
  (A) at (120:3cm) {A};
\node[fill stretch image=goldshade.png]
  (B) at (60:3cm) {B};
\node[
  preaction={fill stretch image=blueshade.png},
  fill stretch image=goldshade.png,
  fill image opacity=0.5] (C) {C};
\path (A) -- node{$+$} (B);
\draw[->,very thick] (A)--(C);
\draw[->,very thick] (B)--(C);
\end{tikzpicture}
\end{dispExample*}


\subsection{Straightening of the Arcs}

\begin{marker}
This patch is considered as an experimental feature.
It changes some of the original \tikzname\ code. This change may break
with future updates of \tikzname.
\end{marker}

\begin{docCommand}[doc new=2014-05-05]{tcbpatcharcangular}{}
The \tikzname\ package provides a nice |rounded corners| option to replace
all corners by little arcs. |\tcbpatcharcangular| is a patch which
straightens the arcs. To say it more prosaic, the little arcs are replaced
by little straight lines.

\begin{dispExample*}{sbs,lefthand ratio=0.66,right=2mm,sidebyside gap=5mm,center lower}
\begin{tikzpicture}
  \draw[thick,rounded corners=8pt]
    (0,0) -- (0,2) -- (1,3.25) -- (2,2) -- (2,0)
     -- (0,2) -- (2,2) -- (0,0) -- (2,0);
  \tcbpatcharcangular
  \draw[thick,rounded corners=8pt,xshift=2.5cm]
    (0,0) -- (0,2) -- (1,3.25) -- (2,2) -- (2,0)
     -- (0,2) -- (2,2) -- (0,0) -- (2,0);
\end{tikzpicture}
\end{dispExample*}

\end{docCommand}


\begin{docCommand}[doc new=2014-05-05]{tcbpatcharcround}{}
This macro reverts \refCom{tcbpatcharcangular}, i.e., the patch from
\refCom{tcbpatcharcangular} is replaced by the original code.
\end{docCommand}


\clearpage
\subsection{Extracting Node Dimensions}
The following auxiliary macros are defined by the \mylib{skins} library.
They allow to determine the width and height of an arbitrary \tikzname\ node.
To be more specific, they determine the east-to-west and the north-to-south dimensions
which may be not the maximal dimensions for a non-rectangular node.
Note that the following dimensions are measured exactly including the line width
of the border line. If a new rectangle or node with the same dimensions
and a border is to be drawn, this border width has to be substracted.

\begin{docCommand}[doc new=2014-09-19]{tcbsettowidthofnode}{\marg{register}\marg{node}}
  Sets the east-to-west dimension of the given \meta{node}
  to the \TeX\ \meta{register}.
\end{docCommand}

\begin{docCommand}[doc new=2014-09-19]{tcbsetmacrotowidthofnode}{\marg{macro}\marg{node}}
  Defines \meta{macro} as the east-to-west dimension of the given \meta{node}.
\end{docCommand}

\begin{docCommand}[doc new=2014-09-19]{tcbsettoheightofnode}{\marg{register}\marg{node}}
  Sets the north-to-south dimension of the given \meta{node}
  to the \TeX\ \meta{register}.
\end{docCommand}

\begin{docCommand}[doc new=2014-09-19]{tcbsetmacrotoheightofnode}{\marg{macro}\marg{node}}
  Defines \meta{macro} as the north-to-south dimension of the given \meta{node}.
\end{docCommand}

\begin{dispExample}
\begin{tikzpicture}
  \node[align=center,draw=red,fill=yellow] (A) {This is my\\example node};
  \tcbsetmacrotowidthofnode\mywidth{A}
  \tcbsetmacrotoheightofnode\myheight{A}
  \path[fill=blue!25!white]           %  rectangle widthout border
    ([xshift=2mm]A.south east)
    rectangle node{Copy} +(\mywidth,\myheight);
  \node[draw=blue,fill=blue!25!white, % standard border width 0.4pt
    minimum width=\mywidth-0.4pt,     % minus width of border
    minimum height=\myheight-0.4pt    % minus height of border
    ]
    at ([xshift=5cm]A) {Copy 2};
\end{tikzpicture}
\end{dispExample}


\subsection{Hyper Nodes}
The following auxiliary macro is defined by the \mylib{skins} library.
\enlargethispage*{1cm}

\begin{docCommand}[doc new=2016-02-03]{tcbhypernode}{\marg{macro}\marg{node}}
%  Sets the east-to-west dimension of the given \meta{node}
%  to the \TeX\ \meta{register}.
  Applies a hyperlink creating \meta{macro} from the package |hyperref| \cite{rahtz:hyperref}
  to an existing |tikz| \meta{node}. \refCom{tcbhypernode} can only
  be used inside a |tikzpicture| environment.
  The last argument of the \meta{macro} is to be omitted and should stand
  for an object (text) which is to be made a hyperlink.
  For example, use  |\hyperref[name]| instead of |\hyperref[name]{text}|.

\begin{dispExample}
% \usepackage{hyperref}
\begin{tikzpicture}
  \node[align=center,draw=red,fill=red!5] (mybutton)
    {Click me to jump to Section~\ref*{sec:tikzimagefilling}};
  \tcbhypernode{\hyperref[sec:tikzimagefilling]}{mybutton}
\end{tikzpicture}
\end{dispExample}

\end{docCommand}



==> tcolorbox.doc.graphics.tex <==
% !TeX root = tcolorbox.tex
% include file of tcolorbox.tex (manual of the LaTeX package tcolorbox)
\clearpage
\section{Inclusion of Boxed Image Files}\label{sec:includegraphics}%
\tcbset{external/prefix=external/graphics_}%
The \mylib{skins} library adds some commands to conveniently include
boxed image files.
For the following macros and options, the \mylib{skins} library has to be loaded
by a package option or inside the preamble by:
\begin{dispListing}
\tcbuselibrary{skins}
\end{dispListing}

See \Vref{sec:skins} for the documentation of all other options of the \mylib{skins} library.

\subsection{Macros}

\begin{docCommand}[doc new and updated={2014-11-14}{2016-07-13}]{tcbincludegraphics}{\oarg{options}\marg{file name}}
  In principle, this macro includes an image file denoted by \meta{file name}
  using the standard |\includegraphics| and puts it into a \refEnv{tcolorbox}.
  The \meta{options} are |tcolorbox| keys to set up the colored box.
  Use \refKey{/tcb/graphics options} to specify options for the underlying
  |\includegraphics|.
  Some |tcolorbox| option keys are automatically set, namely \refKey{/tcb/enhanced} and
  options to center the image inside the box.

  The sizing of the included image is done depending on the following:
  \begin{itemize}
  \item If a \refKey{/tcb/width} is specified, but no fixed \refKey{/tcb/height},
    the image is sized to fill the inner width of the box. The height of the
    box adapts to the image.
  \item If a fixed \refKey{/tcb/height} is specified, the image is sized to fill
    the fixed inner area of the box.
  \item If the \refKey{/tcb/capture} mode \refKey{/tcb/hbox} is specified,
    the image is sized according to given |\includegraphics| options only.
    The box adapts to the image.
  \end{itemize}

\begin{dispExample}
% \tcbuselibrary{raster}
\begin{tcbraster}[raster columns=3,raster force size=false,size=fbox,
    colframe=red!50!black,colback=red!20!black,
    fonttitle=\bfseries,center title,drop fuzzy shadow]
  \tcbincludegraphics[title=Normal]{goldshade.png}
  \tcbincludegraphics[title=Fixed height,height=3cm]{goldshade.png}
  \tcbincludegraphics[title=hbox mode,hbox,graphics options={width=3cm}]
    {goldshade.png}
\end{tcbraster}
\end{dispExample}

\clearpage
The auxiliary macro \docAuxCommand{imagename} may be used inside
\refCom{tcbincludegraphics} to display the name of the file.
\docAuxCommand{imagename} is already partially detokenized and is allowed to
contain special characters like the underscore. Note that an appropriate
font is required to display such characters.
%\docAuxCommand{imagepath}%

\begin{dispExample}
% \tcbuselibrary{raster}
\begin{tcbraster}[size=fbox,
    colframe=red!50!black,colback=red!20!black,
    fonttitle=\bfseries\ttfamily,center title,drop fuzzy shadow]
  \tcbincludegraphics[title=\imagename]{goldshade.png}
  \tcbincludegraphics[finish={
    \node[fill=white,fill opacity=0.5,text opacity=1]
    at (frame.center) {\bfseries\ttfamily\imagename};}]{blueshade.png}
\end{tcbraster}
\end{dispExample}
\end{docCommand}

\clearpage
\begin{docCommand}[doc new=2014-11-14]{tcbincludepdf}{\oarg{options}\marg{file name}}
This is a generalized version of \refCom{tcbincludegraphics} which allows
to include a complete PDF file denoted by \meta{file name}.
Every page is boxed into an own \refEnv{tcolorbox} customized by the
given \meta{options}. It is reasonable to put such a series of boxes
inside a \refEnv{tcbraster} for alignment.

Use \refKey{/tcb/graphics pages} to use a selection of pages instead of
using the whole file.

The auxiliary macro \docAuxCommand{imagepage} may be used inside
\refCom{tcbincludepdf} to display the current page number.
\end{docCommand}


\begin{dispListing}
% \tcbuselibrary{raster}
\begin{tcbraster}[raster columns=3,colframe=blue,colback=white,
  colbacktitle=blue!50!white,fonttitle=\small\bfseries\ttfamily,
  left=0pt,right=0pt,top=0pt,bottom=0pt,boxsep=0pt,boxrule=0.6pt,
  toptitle=1mm,bottomtitle=1mm,drop lifted shadow,center title,
  graphics pages={1,...,6},title={\imagename\ [\imagepage]}]
\tcbincludepdf{tcolorbox-example.pdf}
\end{tcbraster}
\end{dispListing}
{\tcbusetemp}


\clearpage
\subsection{Option Keys}

\begin{docTcbKey}[][doc new and updated={2014-11-14}{2018-03-18}]{graphics options}{=\meta{options}}{no default, initially empty}
Used for \refCom{tcbincludegraphics} and \refCom{tcbincludepdf} to
specify |\includegraphics| \meta{options}.

\begin{dispExample}
% \tcbuselibrary{raster}
\begin{tcbraster}[raster columns=3,size=fbox,raster equal height,
    colframe=red!50!black,colback=red!20!black,drop fuzzy shadow]
  \tcbincludegraphics{goldshade.png}
  \newcommand{\myangle}{angle=20}%
  \tcbincludegraphics[graphics options=\myangle]{goldshade.png}
  \tcbincludegraphics[graphics options={viewport=0cm 0cm 8cm 4cm,clip}]
    {goldshade.png}
\end{tcbraster}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2014-11-14]{graphics directory}{=\meta{directory}}{no default, initially empty}
Used for \refCom{tcbincludegraphics} and \refCom{tcbincludepdf} to
specify a file system \meta{directory} where the image files are located.
\begin{dispListing}
\tcbset{
  graphics directory={.},
  graphics directory={examples},
  graphics directory={../../pictures},
}
\end{dispListing}
\smallskip
\begin{marker}
The |\graphicspath| macro from the |graphics| package is superior to this option.
\refKey{/tcb/graphics directory} may be used especially for
\refCom{tcbincludepdf}.
\end{marker}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-11-14]{graphics pages}{=\meta{selection}}{no default, initially |1,...,|\cs{pdfpages}}
Used for \refCom{tcbincludepdf} to specify a \meta{selection} of pages to be included.
The largest page number is accessible by \docAuxCommand{pdfpages}.
The \meta{selection} has to be given using the |\foreach| syntax of \tikzname.
\begin{dispListing}
\tcbset{
  graphics pages={1,3,7},
  graphics pages={1,...,10},
  graphics pages={1,3,...,18},
  graphics pages={100,...,\pdfpages},
}
\end{dispListing}
\end{docTcbKey}

\clearpage


\begin{docTcbKey}[][doc new=2018-03-21]{graphics orientation}{=\meta{orientation}}{no default, initially |as-is|}
  Used for \refCom{tcbincludegraphics} and \refCom{tcbincludepdf} to
  guarantee a certain \meta{orientation} of the included image.
  After all other options for the image are processed, the result is possibly
  rotated to be in landscape or portrait mode.

  Feasible values for \meta{orientation} are:
  \begin{itemize}
  \item\docValue{as-is}: no rotation of the processed image.
  \item\docValue{landscape}:
    the processed image is possibly rotated by 90 degrees
    to ensure that the final width is not smaller than the final height.
  \item\docValue{landscape*}:
    the processed image is possibly rotated by -90 degrees
    to ensure that the final width is not smaller than the final height.
  \item\docValue{portrait}:
    the processed image is possibly rotated by 90 degrees
    to ensure that the final height is not smaller than the final width.
  \item\docValue{portrait*}:
    the processed image is possibly rotated by -90 degrees
    to ensure that the final height is not smaller than the final width.
  \end{itemize}

\begin{dispExample}
% \tcbuselibrary{raster}
\begin{tcbraster}[raster columns=6,size=fbox,raster equal height,
    colframe=red!50!black,colback=red!20!black,drop fuzzy shadow]
  \tcbincludegraphics{Basilica_5.png}
  \tcbincludegraphics[graphics orientation=landscape]{Basilica_5.png}
  \tcbincludegraphics[graphics orientation=portrait]{Basilica_5.png}
  \tcbincludegraphics[graphics orientation=portrait*]{Basilica_5.png}
  \tcbincludegraphics[graphics options={viewport=0cm 0cm 2cm 3cm,clip}]
    {goldshade.png}
  \tcbincludegraphics[graphics options={viewport=0cm 0cm 2cm 3cm,clip},
    graphics orientation=landscape]{goldshade.png}
\end{tcbraster}
\end{dispExample}


\end{docTcbKey}




==> tcolorbox.doc.hooks.tex <==
% !TeX root = tcolorbox.tex
% include file of tcolorbox.tex (manual of the LaTeX package tcolorbox)
\clearpage
\section{Library \mylib{hooks}}\label{sec:hooks}%
\tcbset{external/prefix=external/hooks_}%
The library is loaded by a package option or inside the preamble by:
\begin{dispListing}
\tcbuselibrary{hooks}
\end{dispListing}

For the skin related options, the library \mylib{skins} has to be loaded
separately.


\subsection{Concept of Hooks}
A hook is a placeholder in some \LaTeX\ code where additional code
can be added. For example, the \LaTeX\ macro |\AtBeginDocument| adds code to a
hook which is placed at the beginning of every document.

Several option keys of |tcolorbox| allow providing some code which is
added to specific places of a colored box. For example, \refKey{/tcb/before upper}
places code before the content of the upper part. A following usage of this
key overwrites any prior settings.

The library \mylib{hooks} extends \refKey{/tcb/before upper} and several more
existing keys to 'hookable' versions, e.\,g.\ 
\refKey{/tcb/before upper app} and \refKey{/tcb/before upper pre}.
The 'hookable' keys don't overwrite prior settings but either \emph{app}end
or \emph{pre}pend the newly given code to the existing code.

The general naming convention (with some small exceptions) is:
\begin{itemize}
\item \meta{option key} |app|: works like \meta{option key} but
  \emph{app}ends its code to the existing code.
\item \meta{option key} |pre|: works like \meta{option key} but
  \emph{pre}pends its code to the existing code.
\end{itemize}
If the original \meta{option key} is used (again), all code will be overwritten.
Therefore, the order of the option key usage is crucial.



\begin{dispExample}
% \usepackage{array,tabularx}
\newcolumntype{Y}{>{\raggedleft\arraybackslash}X}% see tabularx
\tcbset{enhanced,fonttitle=\bfseries\large,fontupper=\normalsize\sffamily,
  colback=yellow!10!white,colframe=red!50!black,colbacktitle=Salmon!30!white,
  coltitle=black,center title,
  tabularx={X||Y|Y|Y|Y||Y},% this sets 'before upper' and 'after upper'
  before upper app={Group & One & Two & Three & Four & Sum\\\hline\hline}  }

\begin{tcolorbox}[title=My table]
Red   & 1000.00 & 2000.00 &  3000.00 &  4000.00 & 10000.00\\\hline
Green & 2000.00 & 3000.00 &  4000.00 &  5000.00 & 14000.00\\\hline
Blue  & 3000.00 & 4000.00 &  5000.00 &  6000.00 & 18000.00\\\hline\hline
Sum   & 6000.00 & 9000.00 & 12000.00 & 15000.00 & 42000.00
\end{tcolorbox}
\end{dispExample}



\clearpage
\subsection{Box Content Additions}\label{subsec:hookscontentadditions}
The following option keys extend the options given in Subsection \ref{subsec:contentadditions}
from page \pageref{subsec:contentadditions}.

\begin{docTcbKey}{before title app}{=\meta{code}}{no default}
  Appends the given \meta{code} to \refKey{/tcb/before title} \emph{after} the color and font settings
  and \emph{before} the content of the title.
\end{docTcbKey}

\begin{docTcbKey}{before title pre}{=\meta{code}}{no default}
  Prepends the given \meta{code} to \refKey{/tcb/before title} \emph{after} the color and font settings
  and \emph{before} the content of the title.
\end{docTcbKey}

\begin{docTcbKey}{after title app}{=\meta{code}}{no default}
  Appends the given \meta{code} to \refKey{/tcb/after title} \emph{after} the content of the title.
\end{docTcbKey}

\begin{docTcbKey}{after title pre}{=\meta{code}}{no default}
  Prepends the given \meta{code} to \refKey{/tcb/after title} \emph{after} the content of the title.
\end{docTcbKey}

\begin{docTcbKey}{before upper app}{=\meta{code}}{no default}
  Appends the given \meta{code} to \refKey{/tcb/before upper} or \refKey{/tcb/before upper*} \emph{after} the color and font settings
  and \emph{before} the content of the upper part.
\end{docTcbKey}

\begin{docTcbKey}{before upper pre}{=\meta{code}}{no default}
  Prepends the given \meta{code} to \refKey{/tcb/before upper} or \refKey{/tcb/before upper*} \emph{after} the color and font settings
  and \emph{before} the content of the upper part.
\end{docTcbKey}

\begin{docTcbKey}{after upper app}{=\meta{code}}{no default}
  Appends the given \meta{code} to \refKey{/tcb/after upper} or \refKey{/tcb/after upper*} \emph{after} the content of the upper part.
\end{docTcbKey}

\begin{docTcbKey}{after upper pre}{=\meta{code}}{no default}
  Prepends the given \meta{code} to \refKey{/tcb/after upper} or \refKey{/tcb/after upper*} \emph{after} the content of the upper part.
\begin{dispExample}
% \tcbuselibrary{theorems}

\begin{tcolorbox}[
  ams align,%  this sets 'before upper*' and 'after upper*'
  colback=yellow!10!white,colframe=red!50!black,
  before upper app={\frac{2}{\sqrt{2}}&=\sqrt{2}.\\},
  after upper pre={\\\sin\left(\frac{\pi}{2}\right)&=1.},
]
  \sum\limits_{n=1}^{\infty} \frac{1}{n} &= \infty.\\
  \int x^2 ~\text{d}x &= \frac13 x^3 + c.
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{before lower app}{=\meta{code}}{no default}
  Appends the given \meta{code} to \refKey{/tcb/before lower} or \refKey{/tcb/before lower*} \emph{after} the color and font settings
  and \emph{before} the content of the lower part.
\end{docTcbKey}

\begin{docTcbKey}{before lower pre}{=\meta{code}}{no default}
  Prepends the given \meta{code} to \refKey{/tcb/before lower} or \refKey{/tcb/before lower*} \emph{after} the color and font settings
  and \emph{before} the content of the lower part.
\end{docTcbKey}

\begin{docTcbKey}{after lower app}{=\meta{code}}{no default}
  Appends the given \meta{code} to \refKey{/tcb/after lower} or \refKey{/tcb/after lower*} \emph{after} the content of the lower part.
\end{docTcbKey}

\begin{docTcbKey}{after lower pre}{=\meta{code}}{no default}
  Prepends the given \meta{code} to \refKey{/tcb/after lower} or \refKey{/tcb/after lower*} \emph{after} the content of the lower part.
\end{docTcbKey}


\subsection{Embedding into the Surroundings}
The following option keys extend the options given in Subsection \ref{subsec:surroundings}
from page \pageref{subsec:surroundings}.

\begin{marker}
The 'hookable' versions are usable inside the document.
In the preamble, they can only be used after explicit setting of
\refKey{/tcb/before} and \refKey{/tcb/after} or by e.\,g.\ \refKey{/tcb/parskip}.
\end{marker}

\begin{docTcbKey}{before app}{=\meta{code}}{no default}
  Appends the given \meta{code} to \refKey{/tcb/before} before the colored box.
\end{docTcbKey}

\begin{docTcbKey}{before pre}{=\meta{code}}{no default}
  Prepends the given \meta{code} to \refKey{/tcb/before} before the colored box.
\end{docTcbKey}

\begin{docTcbKey}{after app}{=\meta{code}}{no default}
  Appends the given \meta{code} to \refKey{/tcb/after} after the colored box.
\end{docTcbKey}

\begin{docTcbKey}{after pre}{=\meta{code}}{no default}
  Prepends the given \meta{code} to \refKey{/tcb/after} after the colored box.
\end{docTcbKey}

\begin{dispExample}
\tcbset{colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[title=My title,before app={The box follows:\\[4pt]},
  after app={This is the end.}]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{dispExample}


\clearpage
\subsection{Overlays}
The following option keys extend the options given in Subsection \ref{subsec:overlays}
from page \pageref{subsec:overlays}.

\begin{docTcbKey}{overlay app}{=\meta{graphical code}}{no default}
  Appends the given \meta{graphical code} to \refKey{/tcb/overlay}.


\begin{dispExample}
% \usetikzlibrary{patterns} % preamble
% \tcbuselibrary{skins} % preamble
\tcbset{frogbox/.style={enhanced,colback=green!10,colframe=green!65!black,
  enlarge top by=5.5mm,
  overlay={\foreach \x in {2cm,3.5cm} {
    \begin{scope}[shift={([xshift=\x]frame.north west)}]
      \path[draw=green!65!black,fill=green!10,line width=1mm] (0,0) arc (0:180:5mm);
      \path[fill=black] (-0.2,0) arc (0:180:1mm);
    \end{scope}}}]}}
\tcbset{ribbon/.style={overlay app={%
  \path[fill=blue!75!white,draw=blue,double=white!85!blue,
    preaction={opacity=0.6,fill=blue!75!white},
    line width=0.1mm,double distance=0.2mm,
    pattern=fivepointed stars,pattern color=white!75!blue]
    ([xshift=-0.2mm,yshift=-1.02cm]frame.north east)
    -- ++(-1,1) -- ++(-0.5,0) -- ++(1.5,-1.5) -- cycle;}}}

\begin{tcolorbox}[frogbox,title=My title]
This is a \textbf{tcolorbox}.
\end{tcolorbox}

\begin{tcolorbox}[frogbox,ribbon,title=My title]
This is a \textbf{tcolorbox}.\par
Here, we apply a second overlay.
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}

\begin{docTcbKey}{overlay pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/overlay}.
\end{docTcbKey}

\begin{docTcbKey}{overlay unbroken app}{=\meta{graphical code}}{no default}
  Appends the given \meta{graphical code} to \refKey{/tcb/overlay unbroken}.
\end{docTcbKey}

\begin{docTcbKey}{overlay unbroken pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/overlay unbroken}.
\end{docTcbKey}

\begin{docTcbKey}{overlay first app}{=\meta{graphical code}}{no default}
  Appends the given \meta{graphical code} to \refKey{/tcb/overlay first}.
\end{docTcbKey}

\begin{docTcbKey}{overlay first pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/overlay first}.
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{overlay middle app}{=\meta{graphical code}}{no default}
  Appends the given \meta{graphical code} to \refKey{/tcb/overlay middle}.
\end{docTcbKey}

\begin{docTcbKey}{overlay middle pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/overlay middle}.
\end{docTcbKey}

\begin{docTcbKey}{overlay last app}{=\meta{graphical code}}{no default}
  Appends the given \meta{graphical code} to \refKey{/tcb/overlay last}.
\end{docTcbKey}

\begin{docTcbKey}{overlay last pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/overlay last}.
\end{docTcbKey}

\begin{docTcbKey}{overlay broken app}{=\meta{graphical code}}{no default}
  Appends the given \meta{graphical code} to \refKey{/tcb/overlay broken}.
\end{docTcbKey}

\begin{docTcbKey}{overlay broken pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/overlay broken}.
\end{docTcbKey}

\begin{docTcbKey}{overlay unbroken and first app}{=\meta{graphical code}}{no default}
  Appends the given \meta{graphical code} to \refKey{/tcb/overlay unbroken and first}.
\end{docTcbKey}

\begin{docTcbKey}{overlay unbroken and first pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/overlay unbroken and first}.
\end{docTcbKey}

\begin{docTcbKey}{overlay middle and last app}{=\meta{graphical code}}{no default}
  Appends the given \meta{graphical code} to \refKey{/tcb/overlay middle and last}.
\end{docTcbKey}

\begin{docTcbKey}{overlay middle and last pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/overlay middle and last}.
\end{docTcbKey}

\begin{docTcbKey}{overlay unbroken and last app}{=\meta{graphical code}}{no default}
  Appends the given \meta{graphical code} to \refKey{/tcb/overlay unbroken and last}.
\end{docTcbKey}

\begin{docTcbKey}{overlay unbroken and last pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/overlay unbroken and last}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-09-19]{overlay first and middle app}{=\meta{graphical code}}{no default}
  Appends the given \meta{graphical code} to \refKey{/tcb/overlay first and middle}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-09-19]{overlay first and middle pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/overlay first and middle}.
\end{docTcbKey}


\clearpage
\subsection{Watermarks}
The following option keys extend the options given in Subsection \ref{subsec:watermarks}
from page \pageref{subsec:watermarks}.

\begin{marker}
Watermarks are special overlays. The \mylib{hooks} library allows the combination
of several watermarks and overlays.
\end{marker}

\begin{docTcbKey}{watermark text app}{=\meta{text}}{no default}
  Appends a \refKey{/tcb/watermark text} to the colored box.
\begin{dispExample}
\tcbset{colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[enhanced,title=My title,watermark graphics=Basilica_5.png,
  watermark opacity=0.25,
  watermark text app=Basilica,watermark color=Navy
  ]
\lipsum[1-2]
\tcblower
This example uses a public domain picture from\\
\url{http://commons.wikimedia.org/wiki/File:Basilica_5.png}
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}

\begin{docTcbKey}{watermark text pre}{=\meta{text}}{no default}
  Prepends a \refKey{/tcb/watermark text} to the colored box.
\end{docTcbKey}

\begin{docTcbKey}{watermark text app on}{=\meta{part} is \meta{text}}{no default}
  Appends a \refKey{/tcb/watermark text on} the named \meta{part} of a break sequence.
\end{docTcbKey}

\begin{docTcbKey}{watermark text pre on}{=\meta{part} is \meta{text}}{no default}
  Prepends a \refKey{/tcb/watermark text on} the named \meta{part} of a break sequence.
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{watermark graphics app}{=\meta{file name}}{no default}
  Appends a \refKey{/tcb/watermark graphics} referenced by \meta{file name} to the colored box.
\end{docTcbKey}

\begin{docTcbKey}{watermark graphics pre}{=\meta{file name}}{no default}
  Prepends a \refKey{/tcb/watermark graphics} referenced by \meta{file name} to the colored box.
\end{docTcbKey}

\begin{docTcbKey}{watermark graphics app on}{=\meta{part} is \meta{file name}}{no default}
  Appends a \refKey{/tcb/watermark graphics on} the named \meta{part} of a break sequence.
  The picture is referenced by \meta{file name}.
\end{docTcbKey}


\begin{docTcbKey}{watermark graphics pre on}{=\meta{part} is \meta{file name}}{no default}
  Prepends a \refKey{/tcb/watermark graphics on} the named \meta{part} of a break sequence.
  The picture is referenced by \meta{file name}.
\end{docTcbKey}


\begin{docTcbKey}{watermark tikz app}{=\meta{graphical code}}{no default}
  Appends a \refKey{/tcb/watermark tikz} with the  given |tikz| \meta{graphical code} to the colored box.
\end{docTcbKey}

\begin{docTcbKey}{watermark tikz pre}{=\meta{graphical code}}{no default}
  Prepends a \refKey{/tcb/watermark tikz} with the  given |tikz| \meta{graphical code} to the colored box.

\begin{dispExample}
% \usepackage{tikz}
\tcbset{colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries,
  watermark color=Navy,watermark opacity=0.25,
  smiley/.style={watermark tikz pre={%
    \path[fill=yellow,draw=yellow!75!red] (0,0) circle (1cm);
    \fill[red] (45:5mm) circle (1mm);
    \fill[red] (135:5mm) circle (1mm);
    \draw[line width=1mm,red] (215:5mm) arc (215:325:5mm);}}}

\begin{tcolorbox}[enhanced,title=My title, watermark text=Watermark,
  smiley]
\lipsum[1-2]
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}

\enlargethispage*{1cm}

\begin{docTcbKey}{watermark tikz app on}{=\meta{part} is \meta{graphical code}}{no default}
  Appends a \refKey{/tcb/watermark tikz on} the named \meta{part} of a break sequence.
\end{docTcbKey}

\begin{docTcbKey}{watermark tikz pre on}{=\meta{part} is \meta{graphical code}}{no default}
  Prepends a \refKey{/tcb/watermark tikz on} the named \meta{part} of a break sequence.
\end{docTcbKey}


\clearpage
\subsection{Underlays}
The following option keys extend the options given in \Vref{subsec:skinunderlay}.
There are no |app| type keys since underlays are stackable by default.

\begin{docTcbKey}{underlay pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/underlay}.
\end{docTcbKey}

\begin{docTcbKey}{underlay unbroken pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/underlay unbroken}.
\end{docTcbKey}

\begin{docTcbKey}{underlay first pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/underlay first}.
\end{docTcbKey}

\begin{docTcbKey}{underlay middle pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/underlay middle}.
\end{docTcbKey}

\begin{docTcbKey}{underlay last pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/underlay last}.
\end{docTcbKey}

\begin{docTcbKey}{underlay boxed title pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/underlay boxed title}.
\end{docTcbKey}

\begin{docTcbKey}{underlay broken pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/underlay broken}.
\end{docTcbKey}

\begin{docTcbKey}{underlay unbroken and first pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/underlay unbroken and first}.
\end{docTcbKey}

\begin{docTcbKey}{underlay middle and last pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/underlay middle and last}.
\end{docTcbKey}

\begin{docTcbKey}{underlay unbroken and last pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/underlay unbroken and last}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-09-19]{underlay first and middle pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/underlay first and middle}.
\end{docTcbKey}


\clearpage
\subsection{Finishes}
The following option keys extend the options given in \Vref{subsec:skinfinish}.
There are no |app| type keys since finishes are stackable by default.

\begin{docTcbKey}{finish pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/finish}.
\end{docTcbKey}

\begin{docTcbKey}{finish unbroken pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/finish unbroken}.
\end{docTcbKey}

\begin{docTcbKey}{finish first pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/finish first}.
\end{docTcbKey}

\begin{docTcbKey}{finish middle pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/finish middle}.
\end{docTcbKey}

\begin{docTcbKey}{finish last pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/finish last}.
\end{docTcbKey}

\begin{docTcbKey}{finish broken pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/finish broken}.
\end{docTcbKey}

\begin{docTcbKey}{finish unbroken and first pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/finish unbroken and first}.
\end{docTcbKey}

\begin{docTcbKey}{finish middle and last pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/finish middle and last}.
\end{docTcbKey}

\begin{docTcbKey}{finish unbroken and last pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/finish unbroken and last}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-09-19]{finish first and middle pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/finish first and middle}.
\end{docTcbKey}


\subsection{Skin Code}
The following option keys extend the options given in Subsection~\ref{subsec:addcodeoptions}
from page~\pageref{subsec:addcodeoptions}.

\begin{docTcbKey}{frame code app}{=\meta{graphical code}}{no default}
  Appends the given \meta{graphical code} to \refKey{/tcb/frame code}.
\end{docTcbKey}

\begin{docTcbKey}{frame code pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/frame code}.
\end{docTcbKey}

\begin{docTcbKey}{interior titled code app}{=\meta{graphical code}}{no default}
  Appends the given \meta{graphical code} to \refKey{/tcb/interior titled code}.
\begin{dispExample}
\begin{tcolorbox}[title=My title,enhanced,colframe=Navy,
  frame code app={\draw[yellow,line width=1cm] (
    frame.south west)--(frame.north east);},
  interior titled code app={\draw[red,line width=1cm]
    (frame.north west)--(frame.south east);},
  ]
\lipsum[1]
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}

\begin{docTcbKey}{interior titled code pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/interior titled code}.
\end{docTcbKey}

\begin{docTcbKey}{interior code app}{=\meta{graphical code}}{no default}
  Appends the given \meta{graphical code} to \refKey{/tcb/interior code}.
\end{docTcbKey}

\begin{docTcbKey}{interior code pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/interior code}.
\end{docTcbKey}

\begin{docTcbKey}{segmentation code app}{=\meta{graphical code}}{no default}
  Appends the given \meta{graphical code} to \refKey{/tcb/segmentation code}.
\end{docTcbKey}

\begin{docTcbKey}{segmentation code pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/segmentation code}.
\end{docTcbKey}


\begin{docTcbKey}{title code app}{=\meta{graphical code}}{no default}
  Appends the given \meta{graphical code} to \refKey{/tcb/title code}.
\end{docTcbKey}

\begin{docTcbKey}{title code pre}{=\meta{graphical code}}{no default}
  Prepends the given \meta{graphical code} to \refKey{/tcb/title code}.
\end{docTcbKey}


\clearpage
\subsection{Extras}
The following option keys extend the options given in \Vref{subsec:extras}.
There are no |app| type keys since extras are stackable by default.

\begin{docTcbKey}[][doc new=2015-07-16]{extras pre}{=\marg{options}}{no default}
  Prepends the given \meta{options} to \refKey{/tcb/extras}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-07-16]{extras unbroken pre}{=\marg{options}}{no default}
  Prepends the given \meta{options} to \refKey{/tcb/extras unbroken}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-07-16]{extras first pre}{=\marg{options}}{no default}
  Prepends the given \meta{options} to \refKey{/tcb/extras first}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-07-16]{extras middle pre}{=\marg{options}}{no default}
  Prepends the given \meta{options} to \refKey{/tcb/extras middle}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-07-16]{extras last pre}{=\marg{options}}{no default}
  Prepends the given \meta{options} to \refKey{/tcb/extras last}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-07-16]{extras broken pre}{=\marg{options}}{no default}
  Prepends the given \meta{options} to \refKey{/tcb/extras broken}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-07-16]{extras unbroken and first pre}{=\marg{options}}{no default}
  Prepends the given \meta{options} to \refKey{/tcb/extras unbroken and first}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-07-16]{extras middle and last pre}{=\marg{options}}{no default}
  Prepends the given \meta{options} to \refKey{/tcb/extras middle and last}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-07-16]{extras unbroken and last pre}{=\marg{options}}{no default}
  Prepends the given \meta{options} to \refKey{/tcb/extras unbroken and last}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2015-07-16]{extras first and middle pre}{=\marg{options}}{no default}
  Prepends the given \meta{options} to \refKey{/tcb/extras first and middle}.
\end{docTcbKey}


\subsection{Listings}
The following option keys extend the options given in
Section~\ref{sec:listings}
from page~\pageref{sec:listings}.


\begin{docTcbKey}[][doc new=2019-07-11]{listing options app}{=\marg{options}}{no default}
  Appends the given \meta{options} to \refKey{/tcb/listing options}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2019-07-11]{listing options pre}{=\marg{options}}{no default}
  Prepends the given \meta{options} to \refKey{/tcb/listing options}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2019-07-11]{minted options app}{=\marg{options}}{no default}
  Appends the given \meta{options} to \refKey{/tcb/minted options}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2019-07-11]{minted options pre}{=\marg{options}}{no default}
  Prepends the given \meta{options} to \refKey{/tcb/minted options}.
\end{docTcbKey}




==> tcolorbox.doc.initoptions.tex <==
% !TeX root = tcolorbox.tex
% include file of tcolorbox.tex (manual of the LaTeX package tcolorbox)
\clearpage
\section{Initialization Option Keys}\label{sec:initkeys}%
\tcbset{external/prefix=external/initoptions_}%
The \emph{initialization} options are only applicable for the generation
of new environments and commands based on |tcolorbox| and friends.
Particularly, they can be used for
\begin{itemize}
\item\refCom{newtcolorbox},
\item\refCom{newtcbox},
\item\refCom{newtcblisting},
\item\refCom{newtcbinputlisting},
\item\refCom{newtcbtheorem}, and
\item\refCom{newtcboxfit}.
\end{itemize}

\bigskip
\begin{marker}
Typically, these options may generate counters and alike.
It is \textbf{strongly} recommended that you use initialization options inside
the preamble only. Otherwise, you may get trouble when using \LaTeX's |\include| features.
\end{marker}


\subsection{Numbered Boxes}\label{sec:numberedboxes}
Counters assigned using the initialization options are administrated
automatically. Especially, they are increased for each new box.
Independent from the real counter name, the counter value can be
referenced by \docAuxCommand{thetcbcounter}, e.\,g.\ inside the title of
the box. The real counter name is stored inside \docAuxCommand{tcbcounter}.

\begin{newTcbKey}{auto counter}{}{no value, initially unset}
Creates a new counter automatically.
With \refKey{/tcb/new/number format} and
\refKey{/tcb/new/number within}, the appearance and behavior of the counter
can be changed. The counter value is referenced by \docAuxCommand{thetcbcounter}.

\inputpreamblelisting{A}

\begin{dispExample}
\begin{pabox}[label={myautocounter}]{Title with number}
This box is automatically numbered with \ref{myautocounter} on page
\pageref{myautocounter}. Inside the box, the \thetcbcounter\ can
also be referenced by |\thetcbcounter|.
The real counter name is \texttt{\tcbcounter}.
\end{pabox}
\end{dispExample}
\end{newTcbKey}

\clearpage
\begin{newTcbKey}{use counter from}{=\meta{tcolorbox}}{no default, initially unset}
Here, a counter from another \meta{tcolorbox} is reused.
Note that the settings for \refKey{/tcb/new/number format} and
\refKey{/tcb/new/number within} are inherited and cannot be changed.
The counter value is referenced by \docAuxCommand{thetcbcounter}.

\begin{dispExample}
\newtcolorbox[use counter from=pabox]{mybox}[2][]{%
colback=blue!5!white,colframe=blue!75!black,fonttitle=\bfseries,
title=Some Box \thetcbcounter: #2,#1}

\begin{mybox}[label={myusecounterfrom}]{Title with continued number}
This box is automatically numbered with \ref{myusecounterfrom} on page
\pageref{myusecounterfrom}. Inside the box, the \thetcbcounter\ can
also be referenced by |\thetcbcounter|.
The real counter name is \texttt{\tcbcounter}.
\end{mybox}
\end{dispExample}
\end{newTcbKey}


\begin{newTcbKey}{use counter}{=\meta{counter}}{no default, initially unset}
Here, an ordinary existing \LaTeX\ \meta{counter} is used for numbering.
With \refKey{/tcb/new/number format} and
\refKey{/tcb/new/number within}, the appearance and behavior of the counter
can be changed. The counter value is referenced by \docAuxCommand{thetcbcounter}.

\begin{dispExample}
% \newcounter{myexample}%  preamble
\newtcolorbox[use counter=myexample,number format=\Alph]{mybox}[2][]{%
colback=green!5!white,colframe=green!55!black,fonttitle=\bfseries,
title=Some Box \thetcbcounter: #2,#1}

\begin{mybox}[label={myusecounter}]{Title with \LaTeX\ number}
This box is automatically numbered with \ref{myusecounter} on page
\pageref{myusecounter}. Inside the box, the \thetcbcounter\ can
also be referenced by |\thetcbcounter|.
The real counter name is \texttt{\tcbcounter}.
\end{mybox}
\end{dispExample}
\end{newTcbKey}


\begin{newTcbKey}[][doc new=2014-09-19]{use counter*}{=\meta{counter}}{no default, initially unset}
An existing \LaTeX\ \meta{counter} is used for numbering. In contrast to
\refKey{/tcb/new/use counter}, the options \refKey{/tcb/new/number format} and
\refKey{/tcb/new/number within} are ignored. Use this for counters which
are already configured outside the |tcolorbox| package, e.\,g.\ the standard
|figure| counter.
\end{newTcbKey}


\begin{newTcbKey}{no counter}{}{no value, initially set}
The created boxes are not numbered. This is the default. The option may
be used to overrule a previous option.
\end{newTcbKey}

\enlargethispage*{1cm}

\begin{newTcbKey}[][doc new=2019-10-18]{reset counter on overlays}{\colOpt{=true\textbar false}}{default |true|, initially |false|}
For |beamer| slides, this invokes the |\resetcounteronoverlays| command
for the box counter. The counter is automatically reset on subsequent
overlay slides of a frame.
Thereby, the counter will be the same on all slides of every frame.
\end{newTcbKey}


\clearpage
\begin{newTcbKey}{number within}{=\meta{counter}}{no default, initially unset}
The automatic counter is set to zero, if \meta{counter} is increased.
Additionally, during output, the value of \meta{counter} is prepended to the value of
the automatic counter.\par
To prepend the automatic counter with the chapter number and to reset it
with every new chapter, use:
\begin{dispListing}
number within=chapter
\end{dispListing}
See \refKey{/tcb/new/use counter} for a complete example.
\end{newTcbKey}


\begin{newTcbKey}{number format}{=\meta{format macro}}{no default, initially \texttt{\textbackslash arabic}}
Declares the format of the automatic counter. The \meta{format macro} can be
any valid \LaTeX\ number formatting macro like |\arabic|, |\roman|, etc.\par
To display the counter value in large roman numbers, use:
\begin{dispListing}
number format=\Roman
\end{dispListing}
See \refKey{/tcb/new/auto counter} for a complete example.
\end{newTcbKey}


\begin{newTcbKey}{number freestyle}{=\meta{code}}{no default, initially unset}
Allows advanced control over the complete number format. This option overrules
the format given by \refKey{/tcb/new/number within} and \refKey{/tcb/new/number format}.
Nevertheless, you can combine it with \refKey{/tcb/new/number within} to
get the desired reset property.\par
The \meta{code} is some formatting code which should contain |\tcbcounter| to
reference the automated counter. Since this \meta{code} is expanded, you have
to secure each macro with |\noexpand| with \emph{exception} of |\tcbcounter|.

\inputpreamblelisting{H}

\begin{dispExample}
\begin{phbox}[label={myfreestyle}]{Title with freestyle number}
This box is automatically numbered with \ref{myfreestyle} on page
\pageref{myfreestyle}. Inside the box, the \thetcbcounter\ can
also be referenced by |\thetcbcounter|.
The real counter name is \texttt{\tcbcounter}.
\end{phbox}
\end{dispExample}
\end{newTcbKey}

\clearpage
\begin{marker}
The following options \refKey{/tcb/new/crefname} and \refKey{/tcb/new/Crefname}
need to be set inside the preamble.
\end{marker}

\begin{newTcbKey}[][doc updated=2014-12-01]{crefname}{=\marg{singular}\marg{plural}}{no default, initially unset}
  This option key can be used only in conjunction with the |cleveref| package
  \cite{cubitt:2018a} which has to be loaded separately.
  It creates a cross-reference type for the new |tcolorbox|'es, where the
  lowercase \meta{singular} and \meta{plural} forms of the cross-reference are given.
  This type is the environment or macro name and \refKey{/tcb/label type} is set automatically.
  See \refKey{/tcb/label type} and \cite{cubitt:2018a} for more information.
\end{newTcbKey}


\begin{newTcbKey}[][doc updated=2014-12-01]{Crefname}{=\marg{singular}\marg{plural}}{no default, initially unset}
  This option key can be used only in conjunction with the |cleveref| package
  \cite{cubitt:2018a} which has to be loaded separately.
  It creates a cross-reference type for the new |tcolorbox|'es, where the
  uppercase \meta{singular} and \meta{plural} forms of the cross-reference are given.
  This type is the environment or macro name and \refKey{/tcb/label type} is set automatically.
  See \refKey{/tcb/label type} and \cite{cubitt:2018a} for more information.
\end{newTcbKey}

\inputpreamblelisting{I}
\begin{dispExample}
% \usepackage{varioref}
% \usepackage{cleveref}
\begin{mybluebox}[label={myreference}]{My title}
This is an example.
\end{mybluebox}

\Cref{myreference}, \cref{myreference}.\\
\Cpageref{myreference}, \cpageref{myreference}.\\
\nameCref{myreference}, \namecref{myreference}.\\
\labelcref{myreference}, \labelcpageref{myreference}.\\
With \texttt{varioref}:\\
\Vref{myreference}, \vref{myreference}.\\
\Vref*{myreference}, \vref*{myreference}.
\end{dispExample}

\clearpage

\begin{newTcbKey}[][doc new=2014-09-19]{blend into}{=\meta{name}}{style, no default, initially unset}
Used to comfortably blend into an existing schema of naming and numbering for
some selected cases. For example, a |tcolorbox| can be used to display
and entitle an image pretending to be a standard |figure| environment.
Here, \refKey{/tcb/title} is used instead of the standard |\caption|
and \refKey{/tcb/list text} can be used instead of the optional parameter
of the standard |\caption|.

Feasible values for \meta{name} are:
\begin{itemize}
\item\docValue{figures}: blend into the standard |figure| environment.
\item\docValue{tables}: blend into the standard |table| environment.
\item\docValue{listings}: blend into the standard |lstlisting| environment
  of the package |listings| \cite{hoffmann:listings}.
  \begin{marker}
  Note that |blend into=listings| can only be used in the document content
  or, preferably, inside a |\AtBeginDocument| clause! Using it without
  |\AtBeginDocument| inside the preamble does not work since the |listings|
  packages initializes its counter also inside |\AtBeginDocument|.
  \end{marker}
\end{itemize}
\end{newTcbKey}

\enlargethispage*{5cm}
\begin{dispListing}
\begin{figure}[htb]
  \centering\includegraphics[height=4cm]{lichtspiel.jpg}
  \caption{A standard figure}
\end{figure}

\newtcolorbox[blend into=figures]{myfigure}[2][]{float=htb,capture=hbox,
  title={#2},every float=\centering,#1}

\begin{myfigure}{A tcolorbox figure}
  \includegraphics[height=4cm]{lichtspiel.jpg}
\end{myfigure}
\end{dispListing}
{\tcbusetemp}



\clearpage
\begin{docTcbKey}[][doc new=2015-03-13]{blend before title}{=\meta{value}}{no default, initially \docValue{colon}}
  This option formats the title output of \refKey{/tcb/new/blend into}.
  Note that this is a common |tcolorbox| option which should be set
  globally or in the normal option part of \refCom{newtcolorbox}.

Feasible values for \meta{value} are:
\begin{itemize}
\item\docValue{colon}: use name/number plus colon.
\item\docValue{dash}: use name/number plus dash.
\item\docValue{colon hang}: use name/number plus colon with hanging indent.
\item\docValue{dash hang}: use name/number plus dash with hanging indent.
\end{itemize}

\begin{dispListing}
\newtcolorbox[blend into=figures]{myfigure}[2][]{float=htb,capture=hbox,
  blend before title=dash hang,title={#2},every float=\centering,#1}

\begin{myfigure}{A tcolorbox figure with quite a long title}
  \includegraphics[height=5cm]{lichtspiel.jpg}
\end{myfigure}
\end{dispListing}
{\tcbusetemp}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}[][doc new=2015-03-13]{blend before title code}{=\meta{code}}{no default}
  This option formats the title output of \refKey{/tcb/new/blend into}.
  The \meta{code} takes one parameter, the name/number.
  Use this, if \refKey{/tcb/blend before title} is not flexible enough.

\begin{dispListing}
\newtcolorbox[blend into=figures]{myfigure}[2][]{float=htb,capture=hbox,
  blend before title code={\fbox{##1}\ },title={#2},every float=\centering,#1}

\begin{myfigure}{A tcolorbox figure}
  \includegraphics[height=6cm]{lichtspiel.jpg}
\end{myfigure}
\end{dispListing}
{\tcbusetemp}
\end{docTcbKey}



\clearpage
\subsection{Lists of \texttt{tcolorbox}es}\label{sec:listsof}
For figures and tables, \LaTeX\ provides the |\listoffigures| and
|\listoftables| commands to create lists of these numbered entities.
Also, a |tcolorbox| can be part of such a kind of list.
\begin{enumerate}
\item Assign a list \meta{name} by the \emph{initialization} option
  \refKey{/tcb/new/list inside}.
\item Optionally, a new \meta{type} for list entries may be assigned
  by the \emph{initialization} option \refKey{/tcb/new/list type}.
\item List entries a generated automatically within each new |tcolorbox|
  using the above initialization.
  \begin{itemize}
  \item If \refKey{/tcb/list entry} is set, the entry is generated with it.
  \item Otherwise, if \refKey{/tcb/title} is set, the entry is generated with it.
  \item Otherwise, the entry is generated with the current number and the environment name.
  \end{itemize}
\item The generated list is displayed by \refCom{tcblistof}.
\end{enumerate}

\begin{newTcbKey}{list inside}{=\meta{name}}{no default, initially unset}
Assigns a list or contents file to the generated |tcolorbox|es.
Entries to this list are saved to a file which gets the \meta{name} as
file name extension. The list is referenced by this name in
\refCom{tcblistof}.
For example:
\begin{dispListing}
list inside=exam
\end{dispListing}
See Section \ref{listing:exercises} from page \pageref{listing:exercises}
for a complete example.
\end{newTcbKey}


\begin{newTcbKey}{list type}{=\meta{type}}{no default, initially |tcolorbox|}
Optionally, some \meta{type} can be assigned to the list entries.
For a new \meta{type}, a macro |\l@|\meta{type} has to exist which controls
the format of the list entry. The default type is defined by
\begin{dispListing}
\newcommand*\l@tcolorbox{\@dottedtocline{1}{1.5em}{2.3em}}
\end{dispListing}
This is identical to the |\l@section| setting of \LaTeX. |\l@tcolorbox| can
be redefined or a new \meta{type} can be assigned.
\end{newTcbKey}


\begin{docCommand}{tcblistof}{\oarg{macro}\marg{name}\marg{title text}}
Displays the generated list of |tcolorbox|es with the given \meta{name}.
The heading is generated by \meta{macro}\marg{title text} where \texttt{\textbackslash section}
is the default setting for \meta{macro}.\par
To display the list inside a subsection, use for example:
\begin{dispListing}
\tcblistof[\subsection]{exam}{List of Exercises}
\end{dispListing}
The result of the example is found as Subsection \ref{listofexercises} on
page \pageref{listofexercises}.
\begin{marker}
The core of the list is generated by |\@starttoc|\marg{name} which
can be wrapped into an own macro.
\end{marker}
\end{docCommand}



==> tcolorbox.doc.intro.tex <==
% !TeX root = tcolorbox.tex
% include file of tcolorbox.tex (manual of the LaTeX package tcolorbox)
\clearpage
\section{Introduction}%
\tcbset{external/prefix=external/intro_}%
The package originates from the first edition of my book
\flqq{\citetitle{sturm:latex}\frqq~\cite{sturm:latex}
in about 2006.
For the \LaTeX\ examples and tutorials given there, I wanted to have
accentuated and colored boxes to display source code and
compiled text in combination.
Since, in my opinion, this type of boxes is also quite useful to highlight definitions
and theorems, I applied them for my lecture notes in
mathematics \cite{sturm:mathe1,sturm:mathe2,sturm:mathe3}
as well.
With this package, you are invited to apply these boxes for similar projects.

The breaking news for version 2.00 was the support for breakable boxes.
This feature allows new applications of the package without
affecting the core package too much if you do not need boxes to break automatically.
With version 2.20, the often requested 'side by side' mode for listings has been added.
With version 3.00, boxed titles are introduced together with improved
customization options for overlays, underlays, finishes, and own code extensions.

\begin{tcolorbox}[enhanced,boxrule=0mm,boxsep=0mm,frame hidden,interior hidden,
  left=0mm,right=0mm,top=0mm,bottom=0mm,watermark opacity=0.25,watermark zoom=1.2,before=\par\smallskip,
  clip watermark=false,
  watermark tikz={%
    \path[fill=yellow,draw=yellow!75!red] (0,0) circle (1cm);
    \fill[red] (45:5mm) circle (1mm);
    \fill[red] (135:5mm) circle (1mm);
    \draw[line width=1mm,red] (215:5mm) arc (215:325:5mm);}]
Since the first public release in 2011, I received a lot of feedback from all over the world.
I want to thank all who wrote me for supporting this package by sending bug reports
and ideas for new or better features.
\end{tcolorbox}


\subsection{Installation}
Typically, |tcolorbox| will be installed as part of a major \LaTeX\ distribution
and there is nothing special to do for a user.

If you intend to make a local
installation \emph{by hand}, see the |README| file of the |tcolorbox| package
for some hints. The short story is: you have to install not only
|tcolorbox.sty|, but also all |*.code.tex| files in the local |texmf| tree.


\subsection{Loading the Package}
The base package |tcolorbox| loads the packages
|pgf| \cite{tantau:tikz_and_pgf}, |verbatim| \cite{schoepf:2001a},
|etoolbox| \cite{lehmann:etoolbox},
and |environ| \cite{robertson:2014a}.
|tcolorbox| itself is loaded in the usual manner in the preamble:
\begin{dispListing}
\usepackage{tcolorbox}
\end{dispListing}
The package takes option keys in the key-value syntax.
Alternatively, you may use these keys later in the preamble with
\refCom{tcbuselibrary} (see there).
For example, the key to typeset listings is:
\begin{dispListing}
\usepackage[listings]{tcolorbox}
\end{dispListing}


\clearpage
\subsection{Libraries}\label{sec:bibliothek}
The base package |tcolorbox| is extendable by program libraries.
This is done by using option keys while loading the package or inside
the preamble by applying the following macro with the same set of keys.

\begin{docCommand}{tcbuselibrary}{\marg{key list}}
  Loads the libraries given by the \meta{key list}.
\begin{dispListing}
\tcbuselibrary{listings,theorems}
\end{dispListing}
\end{docCommand}

The following keys are used inside |\tcbuselibrary| respectively
|\usepackage| without the key tree path |/tcb/library/|.

\begin{docTcbKey}[library]{skins}{}{\mylib{skins}}
  Loads the package |tikz| \cite{tantau:tikz_and_pgf} and provides additional
  styles (skins) for the appearance of the colored boxes; see
  Section~\ref{sec:skins} from page~\pageref{sec:skins}.
\end{docTcbKey}

\begin{docTcbKey}[library]{vignette}{}{\mylib{vignette}}
  Provides code for more ornamental; see
  Section~\ref{sec:vignette} from page~\pageref{sec:vignette}.
\end{docTcbKey}

\begin{docTcbKey}[library]{raster}{}{\mylib{raster}}
  Provides additional macros and options for typesetting multiple
  boxes arranged in a kind of raster;
  see Section~\ref{sec:raster} from page~\pageref{sec:raster}.
\end{docTcbKey}

\begin{docTcbKey}[library]{listings}{}{\mylib{listings}}
  Loads the package |listings| \cite{hoffmann:listings} and provides additional
  macros for typesetting listings which are described in Section~\ref{sec:listings}
  from page~\pageref{sec:listings}.
\end{docTcbKey}

\begin{docTcbKey}[library]{listingsutf8}{}{\mylib{listingsutf8}}
  Loads the packages |listings| \cite{hoffmann:listings} and
  |listingsutf8| \cite{oberdiek:listingsutf8} for UTF-8 support.
  This is a variant of the library \mylib{listings}
  and is described in Section \ref{sec:listings}
  from page~\pageref{sec:listings}.
\end{docTcbKey}

\begin{docTcbKey}[library]{minted}{}{\mylib{minted}}
  Loads the package |minted| \cite{poore:minted} to
  typeset listings with the |Pygments| \cite{pygments:web} tool,
  also see \Vref{sec:listings}.
\end{docTcbKey}

\begin{docTcbKey}[library]{theorems}{}{\mylib{theorems}}
  Provides additional
  macros for typesetting theorems which are described in Section~\ref{sec:theorems}
  from page~\pageref{sec:theorems}.
\end{docTcbKey}


\begin{docTcbKey}[library]{breakable}{}{\mylib{breakable}}
  Provides support for automatic box breaking from one page to another;
  see \Fullref{sec:breakable}.
\end{docTcbKey}

\begin{docTcbKey}[library]{magazine}{}{\mylib{magazine}}
  Provides support for storing broken box parts to be used later or
  in interchanged order, \Fullref{sec:magazine}.
\end{docTcbKey}

\begin{docTcbKey}[library]{poster}{}{\mylib{poster}}
  Provides support for creating posters, \Fullref{sec:poster}.
\end{docTcbKey}

\begin{docTcbKey}[library]{fitting}{}{\mylib{fitting}}
  Provides support for font size adaption of the box content to
  the box dimensions;
  see Section~\ref{sec:fitting} from page~\pageref{sec:fitting}.
\end{docTcbKey}

\begin{docTcbKey}[library]{hooks}{}{\mylib{hooks}}
  Extends several option keys to 'hookable' keys;
  see Section~\ref{sec:hooks} from page~\pageref{sec:hooks}.
\end{docTcbKey}

\clearpage
\begin{docTcbKey}[library]{xparse}{}{\mylib{xparse}}
  Provides document command production with |xparse| for |tcolorbox|;
  see Section~\ref{sec:xparse} from page~\pageref{sec:xparse}.
\end{docTcbKey}

\begin{docTcbKey}[library]{external}{}{\mylib{external}}
  Provides externalization support for stand-alone document snippets,
  see \Fullref{sec:external}.
\end{docTcbKey}

\begin{docTcbKey}[library]{documentation}{}{\mylib{documentation}}
  Provides additional
  macros for typesetting \LaTeX\ documentations
  which are described in Section~\ref{sec:documentation}
  from page~\pageref{sec:documentation}.
\end{docTcbKey}

\begin{docTcbKey}[library]{many}{}{style, no value}
  Loads the libraries \mylib{skins}, \mylib{breakable}, \mylib{raster}, \mylib{hooks},
  \mylib{theorems}, \mylib{fitting}, and \mylib{xparse}.
  Use this shortcut, if you want to use all features of |tcolorbox|
  with exception of typesetting listings and using
  the specialized \mylib{documentation} library.
\end{docTcbKey}

\begin{docTcbKey}[library]{most}{}{style, no value}
  Loads all libraries except \mylib{minted} and \mylib{documentation}.
  Use this shortcut, if you want to use all features of |tcolorbox|
  with exception of using the |minted| package and using
  the specialized \mylib{documentation} library.
\end{docTcbKey}

\begin{docTcbKey}[library]{all}{}{style, no value}
  Loads all libraries. Use this shortcut only, if you intend to use the
  \mylib{documentation} library.
\end{docTcbKey}


\begin{extcolorbox}[runs=2]{intro_packageoverview}
  [title={Package \texttt{tcolorbox}},center title,fonttitle=\bfseries,arc=0pt,
  colback=red!10!white,
  interior style={fill tile image*={width=2cm}{pink_marble.png},fill image opacity=0.5},
  colframe=red!50!black]
  \begin{tcolorbox}[beamer,adjusted title=Basic Features,colframe=blue!50!black,colback=blue!10!white]
  Base package
  \end{tcolorbox}
  \begin{tcbitemize}[raster columns=3,raster before skip=2mm,raster after skip=0pt,
    raster equal height,beamer,colframe=blue!50!black,colback=blue!10!white]
  \tcbitem[adjusted title=Advanced Features]
    \mylib{breakable}\\
    \mylib{external}\\
    \mylib{fitting}\\
    \mylib{hooks}\\
    \mylib{magazine}\\
    \mylib{poster}\\
    \mylib{raster}\\ 
    \mylib{skins}\\
    \mylib{theorems}\\
    \mylib{vignette}\\
    \mylib{xparse}
  \tcbitem[adjusted title=Advanced Listings]
    \mylib{listings}\\
    \mylib{listingsutf8}
    \tcblower
    \mylib{minted}
  \tcbitem[adjusted title=Documentation]
    \mylib{documentation}
  \end{tcbitemize}
\end{extcolorbox}



==> tcolorbox.doc.listings.tex <==
% !TeX root = tcolorbox.tex
% include file of tcolorbox.tex (manual of the LaTeX package tcolorbox)
\clearpage
\section{Libraries
  \mylib{listings},
  \mylib{listingsutf8}, and
  \mylib{minted}}\label{sec:listings}%
\tcbset{external/prefix=external/listings_}%

\subsection{Loading the Libraries}
In contrast to other |tcolorbox| libraries, the libraries
\mylib{listings}, \mylib{listingsutf8}, and \mylib{minted} are concurrent in the sense that
they all do the same thing, i.\,e.\ displaying listings with or without typesetting
the listing in \LaTeX\ parallel.
The difference is the underlying \LaTeX\ package which does the core job for
displaying a listing. So, typically, you need just \emph{one} of these
libraries. If you do not have a clue which one of them you should use
and you are using |pdflatex|, you should take \mylib{listingsutf8}.
If you are using |xelatex| or |lualatex|, you should take \mylib{listings}
as |xelatex| and |lualatex| are not compatible with \mylib{listingsutf8}.

\begin{marker}
The order in which the libraries are included influences the default settings and
the \refKey{/tcb/reset} behavior. The settings of a later loaded library overwrite
the settings of a previous loaded library. A library is never loaded twice.
\end{marker}


\subsubsection{Loading \mylib{listings}}
This library uses the package |listings| \cite{hoffmann:listings} to typeset
listings. It is loaded by a package option or inside the preamble by:
\begin{dispListing}
\tcbuselibrary{listings}
\end{dispListing}
This also loads the package |listings| \cite{hoffmann:listings}.

The \refKey{/tcb/listing engine} is set to |listings| by the library.
To reactivate this setting, if overwritten by other libraries, use
\begin{dispListing}
\tcbset{listing engine=listings}
\end{dispListing}

\subsubsection{Loading \mylib{listingsutf8}}
\begin{marker}
This library is not needed (and troublesome) when using Xe\LaTeX\ or Lua\LaTeX.
Therefore, loading this library is automatically replaced by loading
\mylib{listings} only, if pdf\LaTeX\ is \emph{not} used.
\end{marker}
To extend |listings| for UTF-8 encoded sources, you can use the support from
the package |listingsutf8| \cite{oberdiek:listingsutf8} by loading the library
variant \mylib{listingsutf8}.
\begin{dispListing}
\tcbuselibrary{listingsutf8}
\tcbset{listing utf8=latin1}% optional; 'latin1' is the default.
\end{dispListing}
This also loads the library \mylib{listings}
and the packages |listings| \cite{hoffmann:listings}
and |listingsutf8| \cite{oberdiek:listingsutf8}.

The \refKey{/tcb/listing engine} is set to |listings| by the library.
To reactivate this setting, if overwritten by other libraries, use
\begin{dispListing}
\tcbset{listing engine=listings}
\end{dispListing}


\clearpage
\subsubsection{Loading \mylib{minted}}
This library uses the package |minted| \cite{poore:minted} to typeset
listings. It is loaded by a package option or inside the preamble by:
\begin{dispListing}
\tcbuselibrary{minted}
\end{dispListing}
This also loads the package |minted| \cite{poore:minted}.

\begin{marker}
The |minted| package uses the external tool |Pygments| \cite{pygments:web}
to apply syntax highlighting. It has to be installed and set up, before the
library can be used, see \cite{poore:minted} and \cite{pygments:web}.
The |tcolorbox| library \mylib{minted} does not work, if the package
|minted| \cite{poore:minted} does not work.
\end{marker}

The \refKey{/tcb/listing engine} is set to |minted| by the library.
To reactivate this setting, if overwritten by other libraries, use
\begin{dispListing}
\tcbset{listing engine=minted}
\end{dispListing}


\subsection{Common Macros of the Libraries}

\begin{docEnvironment}{tcblisting}{\marg{options}}
  Creates a colored box based on a \refEnv{tcolorbox}.
  Controlled by the given \meta{options}, the
  environment content is typeset normally and/or as a listing.
  Furthermore, the \meta{options} control appearance and functions of
  the |tcolorbox|.
  By default, the listing is interpreted as a \LaTeX\ listing.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black}
This is a \LaTeX\ example which displays the text as source code
and in compiled form.
\end{tcblisting}
\end{dispExample}

\clearpage

\begin{dispExample}
% \tcbuselibrary{listings} /or/ \tcbuselibrary{listingsutf8}
\begin{tcblisting}{colback=yellow!5,colframe=yellow!50!black,listing only,
    title=This is source code in another language (XML), fonttitle=\bfseries,
  listing options={language=XML,columns=fullflexible,keywordstyle=\color{red}}}
<?xml version="1.0"?>
<project name="Package tcolorbox" default="documentation" basedir=".">
  <description>
    Apache Ant build file (http://ant.apache.org/)
  </description>
</project>
\end{tcblisting}
\end{dispExample}

\enlargethispage*{10mm}

\begin{dispExample}
% \tcbuselibrary{minted}
\begin{tcblisting}{colback=yellow!5,colframe=yellow!50!black,listing only,
    title=This is source code in another language (XML), fonttitle=\bfseries,
  listing engine=minted,minted language=xml}
<?xml version="1.0"?>
<project name="Package tcolorbox" default="documentation" basedir=".">
  <description>
    Apache Ant build file (http://ant.apache.org/)
  </description>
</project>
\end{tcblisting}
\end{dispExample}



\begin{dispExample}
% This box is as wide as needed (listing only !!)
% \tcbuselibrary{skins}
\begin{tcblisting}{colback=green!5!white,colframe=green!50!black,listing only,
  hbox,enhanced,drop fuzzy shadow,before=\begin{center},after=\end{center}}
\begin{tikzpicture}
\fill[red] (0,0) rectangle (1,1);
\end{tikzpicture}
\end{tcblisting}
\end{dispExample}
\end{docEnvironment}


\clearpage
\begin{docEnvironment}{tcboutputlisting}{}
  Saves the environment content to a file which is named by the key value of
  |listing file|. Later, this file can be loaded by
  |\tcbinputlisting| or |\tcbuselistingtext| or |\tcbuselistinglisting|.
\begin{dispListing}
\begin{tcboutputlisting}
This \textbf{text} is written to a standardized file for later usage.
\end{tcboutputlisting}
\end{dispListing}
\end{docEnvironment}


\begin{docCommand}{tcbinputlisting}{\marg{options}}
  Creates a colored boxed based on a |tcolorbox|. The text content is read
  from a file named by the key value of |listing file|. Apart from that,
  the function is equal to that of \refEnv{tcblisting}.
\begin{dispExample}
\tcbinputlisting{colback=red!5!white,colframe=red!75!black,text only}
\tcbinputlisting{colback=green!5,colframe=green!75!black,listing only}
\end{dispExample}
\end{docCommand}

\begin{docCommand}{tcbuselistingtext}{}
  Loads text from a file named by the key value of |listing file|.
\begin{dispExample}
\tcbuselistingtext
\end{dispExample}
\end{docCommand}


\begin{docCommand}{tcbuselistinglisting}{}
  Typesets text as listing from a file named by the key value of |listing file|.
\begin{dispExample}
\tcbuselistinglisting
\end{dispExample}
\end{docCommand}

%\enlargethispage*{5mm}
\begin{docCommand}{tcbusetemplisting}{}
  Typesets text as listing from a temporary file which was written by
  \refEnv{tcbwritetemp}.
\end{docCommand}


\clearpage
\begin{marker}
See \Vref{subsec:xparse_listing} and \Vref{subsec:xparse_inputlisting} for more
elaborate methods to create new environments and commands.
\end{marker}
\begin{marker}
If a new sort of |tcblisting| environments should be created with
one optional argument only, one is highly recommended to use
\refCom{DeclareTCBListing} or \refCom{NewTCBListing}
instead of \refCom{newtcblisting} to
avoid content scanning problems.
\end{marker}

\begin{docCommand}{newtcblisting}{\oarg{init options}\marg{name}\oarg{number}\oarg{default}\marg{options}}
  Creates a new environment \meta{name} based on \refEnv{tcblisting}.
  Basically, |\newtcblisting| operates like |\newenvironment|. This means,
  the new environment \meta{name} optionally takes \meta{number} arguments, where
  \meta{default} is the default value for the optional first argument.
  The \meta{options} are given to the underlying |tcblisting|.
  Note that \refKey{/tcb/savedelimiter} is set to the given \meta{name}
  automatically.
  The \meta{init options} allow setting up automatic numbering,
  see Section \ref{sec:initkeys} from page \pageref{sec:initkeys}.
\begin{dispExample*}{sbs,lefthand ratio=0.5}
\newtcblisting{mybox}{%
  colback=red!5!white,
  colframe=red!75!black}

\begin{mybox}
This is my \LaTeX\ box.
\end{mybox}
\end{dispExample*}

\begin{dispExample*}{sbs,lefthand ratio=0.5}
\newtcblisting{mybox}[1]{%
  colback=red!5!white,
  colframe=red!75!black,
  fonttitle=\bfseries,
  title=#1}

\begin{mybox}{Listing Box}
This is my \LaTeX\ box.
\end{mybox}
\end{dispExample*}

\begin{dispExample*}{sbs,lefthand ratio=0.5}
\newtcblisting{mybox}[2][]{%
  colback=red!5!white,
  colframe=red!75!black,
  fonttitle=\bfseries,
  title=#2,#1}

\begin{mybox}[listing only]
  {Listing Box}
This is my \LaTeX\ box.
\end{mybox}
\bigskip

\begin{mybox}[listing side text]
  {Listing Box}
This is my
\LaTeX\ box.
\end{mybox}
\end{dispExample*}

\clearpage
\inputpreamblelisting{C}

\begin{dispExample*}{sbs,lefthand ratio=0.5}
\begin{mycbox}{Listing Box}
This is my \LaTeX\ box.
\end{mycbox}
\end{dispExample*}
\end{docCommand}


%\enlargethispage*{1cm}
\begin{docCommand}{renewtcblisting}{\oarg{init options}\marg{name}\oarg{number}\oarg{default}\marg{options}}
  Operates like \refCom{newtcblisting}, but based on |\renewenvironment| instead of |\newenvironment|.
  An existing environment is redefined.
\end{docCommand}


\clearpage
\begin{docCommand}{newtcbinputlisting}{\oarg{init options}\brackets{\texttt{\textbackslash}\rmfamily\meta{name}}\oarg{number}\oarg{default}\marg{options}}
  Creates a new macro \texttt{\textbackslash}\meta{name} based on \refCom{tcbinputlisting}.
  Basically, |\newtcbinputlisting| operates like |\newcommand|.
  The new macro \texttt{\textbackslash}\meta{name} optionally takes \meta{number} arguments, where
  \meta{default} is the default value for the optional first argument.
  The \meta{options} are given to the underlying |tcbinputlisting|.
  The \meta{init options} allow setting up automatic numbering,
  see Section \ref{sec:initkeys} from page \pageref{sec:initkeys}.

\begin{dispExample}
\newtcbinputlisting[use counter from=mycbox]{\mylisting}[2][]{%
  listing file={#2},
  title=Listing (\thetcbcounter) of \texttt{#2},
  colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries,
  listing only,breakable,#1}

\mylisting[before upper=\textit{This is the included file content:}]
          {\jobname.tcbtemp}
\end{dispExample}

\begin{dispExample}
\newtcbinputlisting[use counter from=mycbox]{\mylisting}[2][]{%
  listing engine=minted,minted language=latex,minted style=colorful,
  listing file={#2},
  title=Listing (\thetcbcounter) of \texttt{#2},
  colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries,
  listing only,breakable,#1}

\mylisting[before upper=\textit{This is the included file content:}]
          {\jobname.tcbtemp}
\end{dispExample}
\end{docCommand}


\begin{docCommand}{renewtcbinputlisting}{\oarg{init options}\brackets{\texttt{\textbackslash}\rmfamily\meta{name}}\oarg{number}\oarg{default}\marg{options}}
  Operates like \refCom{newtcbinputlisting}, but based on |\renewcommand| instead of |\newcommand|.
  An existing macro is redefined.
\end{docCommand}


\clearpage
\subsection{Option Keys of the \mylib{listings} Library}\label{sec:speclistingkeys}

\begin{docTcbKey}{listing options}{=\meta{key list}}{no default, initially |style=tcblatex|}
  Sets the options from the package |listings| \cite{hoffmann:listings}
  which are used during typesetting of the listing.
  For \LaTeX\ listings, there is a predefined |listings| style named |tcblatex|
  which can be used.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!25,left=6mm,
listing options={style=tcblatex,numbers=left,numberstyle=\tiny\color{red!75!black}}}
This is a \LaTeX\ example which displays the text as source code
and in compiled form. Additionally, we use line numbers here.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{no listing options}{}{no value, initially unset}
  Abbreviation for |listing options={}|.
  This removes all options for the |listings| package.
  This includes the |tcblisting| standard style |tcblatex| and the encoding presets.
  Use this option, if you want to set the |listings| options outside of |tcblisting|, e.\,g.\ globally in
  the preamble.
\begin{dispExample}
\begin{tcblisting}{no listing options}
All \textit{listings} options removed.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{listing style}{=\meta{style}}{no default, initially |tcblatex|}
  Abbreviation for |listing options={style=...}|. This key sets a \meta{style}
  for the |listings| package, see \cite{hoffmann:listings}.
  For \LaTeX, there is a predefined style named |tcblatex|.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,
listing style=tcblatex}
Here, we use the predefined style.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{listing inputencoding}{=\meta{encoding}}{no default, initially \texttt{\cs inputencodingname}}
  Sets the input encoding value for the predefined listing style |tcblatex|
  and |tcbdocumentation| from the library \mylib{documentation}.
  The initial value is derived from the package |inputenc| if used.
\end{docTcbKey}

\begin{docTcbKey}{listing remove caption}{\colOpt{=true\textbar false}}{default |true|, initially |true|}
If set to |true|, some part of the caption building code of the |listings| package
is silenced to prevent some unwanted interaction with the |hyperref| package resulting
in additional vertical space.
If set to |false|, the |listings| package code is kept unchanged.
Note that listings outside \refEnv{tcblisting} and
\refCom{tcbinputlisting} are always processed normally.
Typically, a user is not expected to use this key at all.
\end{docTcbKey}

\begin{docTcbKey}{every listing line}{=\meta{text}}{no default, initially unset/empty}
Inserts some \meta{text} to the begin of every line of a listing.
Note that this a hack of the |listings| package code. This may become unusable
or superfluous in the future.
\begin{dispExample}
\newtcblisting{commandshell}{colback=black,colupper=white,colframe=yellow!75!black,
  listing only,listing options={style=tcblatex,language=sh},
  every listing line={\textcolor{red}{\small\ttfamily\bfseries root \$> }}}

\begin{commandshell}
ls -al
cd /usr/lib
\end{commandshell}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{every listing line*}{=\meta{text}}{no default, initially unset/empty}
Identical to \refKey{/tcb/every listing line} plus additional enlargement
of \refKey{/tcb/rightupper} by the width of \meta{text}. Therefore, this
option has to be used after the geometry settings are done.
This option is intended to be used in conjunction with \refKey{/tcb/hbox}.

\begin{dispExample}
\newtcblisting{commandshell}{colback=black,colupper=white,colframe=yellow!75!black,
  listing only,listing options={style=tcblatex,language=sh},hbox,
  every listing line*={\textcolor{red}{\small\ttfamily\bfseries root \$> }}}

\begin{commandshell}
ls -al
cd /usr/lib
\end{commandshell}
\end{dispExample}
\end{docTcbKey}

See further options in \Vref{sec:commonlistingkeys}.

\begin{marker}
For an combined example of using |\lstinline| inside a |tcolorbox|, see
\refCom{DeclareTotalTCBox}.
\end{marker}

\clearpage
\subsection{Option Keys of the \mylib{listingsutf8} Library}
\begin{marker}
The \mylib{listingsutf8} library is not needed (and troublesome) when using Xe\LaTeX\ or Lua\LaTeX.
Therefore, loading this library is automatically replaced by loading
\mylib{listings} only, if pdf\LaTeX\ is \emph{not} used.
\end{marker}

The \mylib{listingsutf8} library is an extension of the
\mylib{listings} library, so
all options from \Vref{sec:speclistingkeys} are applicable.

\begin{docTcbKey}{listing utf8}{=\meta{one-byte-encoding}}{style, no default, initially |latin1|}
  Abbreviation for using \refKey{/tcb/listing inputencoding}
  together with UTF-8 support from the package |listingsutf8| \cite{oberdiek:listingsutf8}.
  This option is available only for the library variant \mylib{listingsutf8}.
  The \meta{one-byte-encoding} is one of
  the applicable encodings from \cite{oberdiek:listingsutf8}, e.\,g.\ |latin1|
  which is the default.\par
  Be aware that this means restriction to this specific \meta{one-byte-encoding}:
  e.\,g.\ |latin1| comprises umlauts and other accented characters, but not
  the Euro sign. If you want to use the |listings| package \emph{and} \flqq real\frqq\
  UTF-8 source code, then do \emph{not} use \mylib{listingsutf8} but \mylib{listings}
  with
  \refKey{/tcb/listing inputencoding}|=utf8|
  \emph{and} with specific manual hacks for specific UTF-8-encoded characters.

\end{docTcbKey}

See further options in \Vref{sec:commonlistingkeys}.

\clearpage
\subsection{Option Keys of the \mylib{minted} Library}

\begin{docTcbKey}{minted language}{=\meta{programming language}}{no default, initially |latex|}
Sets a \meta{programming language} known to |Pygments| \cite{pygments:web}.
\begin{dispExample}
\begin{tcblisting}{listing engine=minted,minted style=trac,
  minted language=java,
  colback=red!5!white,colframe=red!75!black,listing only}
    public class HelloWorld {
      // A 'Hello World' in Java
      public static void main(String[] args) {
        System.out.println("Hello World!");
      }
    }
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc updated={2017-07-05}]{minted options}{=\meta{key list}}{no default, initially
    |tabsize=2,fontsize=\textbackslash small,|\linebreak|breaklines,autogobble|}
  Sets the options from the package |minted| \cite{poore:minted}
  which are used during typesetting of the listing.
\begin{dispExample}
% \tcbuselibrary{skins}
\newtcblisting{myjava}{listing engine=minted,
  minted style=colorful,
  minted language=java,
  minted options={fontsize=\small,breaklines,autogobble,linenos,numbersep=3mm},
  colback=blue!5!white,colframe=blue!75!black,listing only,
  left=5mm,enhanced,
  overlay={\begin{tcbclipinterior}\fill[red!20!blue!20!white] (frame.south west)
    rectangle ([xshift=5mm]frame.north west);\end{tcbclipinterior}}}

\begin{myjava}
  public class HelloWorld {
    // A 'Hello World' in Java
    public static void main(String[] args) {
      System.out.println("Hello World!");
    }
  }
\end{myjava}
\end{dispExample}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{minted style}{=\meta{style}}{no default, initially unset}
Sets a \meta{style} known to |Pygments| \cite{pygments:web}. This is
independent from \refKey{/tcb/minted options}. Note that styles are always
applied globally; all following examples will be set in the given \meta{style}
until a new style is set. Also note that
setting |\usemintedstyle|\marg{style} only once per document is more economic, if
all styles in a document are the same.
For examples of different styles, see
\refKey{/tcb/minted language} and \refKey{/tcb/minted options}.
\end{docTcbKey}

See further options in \Vref{sec:commonlistingkeys}.


\clearpage
\subsection{Common Option Keys of all Libraries}\label{sec:commonlistingkeys}
For the \meta{options} in \refEnv{tcblisting} respectively \refCom{tcbinputlisting}
the following |pgf| keys can be applied. The key tree path |/tcb/| is not to
be used inside these macros.

\begin{docTcbKey}{listing engine}{=\meta{engine}}{no default}
  Sets the \meta{engine} which typesets the listings. Feasible values are
  \begin{itemize}
  \item\docValue{listings}, if library \mylib{listings} or
  \mylib{listingsutf8} is loaded.
  \item\docValue{minted}, if library \mylib{minted} is loaded.
  \end{itemize}
\end{docTcbKey}

\begin{docTcbKey}{listing file}{=\meta{file name}}{no default, initially \cs{jobname.listing}}
  Sets the \meta{file name} of the file which is used to save listings.
\end{docTcbKey}


\begin{docTcbKey}{listing and text}{}{no value, initially set}
  Typesets the environment content as listing in the upper part and
  as compiled text in the lower part.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,listing and text}
This is a \LaTeX\ example.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{text and listing}{}{no value}
  Typesets the environment content as compiled text in the upper part and
  as listing in the lower part.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,text and listing}
This is a \LaTeX\ example.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{listing only}{}{no value}
  Typesets the environment content as listing.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,listing only}
This is a \LaTeX\ example.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}


\clearpage
\begin{docTcbKey}{text only}{}{no value}
  Typesets the environment content as compiled text.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,text only}
This is a \LaTeX\ example.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}



\begin{docTcbKey}{comment}{=\meta{text}}{no default, initially empty}
  Records a comment with \meta{text} as content. The comment is displayed
   e.\,g.\ in conjunction with \refKey{/tcb/listing and comment}
  and \refKey{/tcb/comment and listing}.
\begin{dispExample}
\begin{tcblisting}{comment={This comment is really only a comment},
  colback=red!5!white,colframe=red!75!black}
This is a \textbf{tcolorbox}.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2014-11-17]{comment only}{}{no value}
  Typesets the environment content with the comment text.
\begin{dispExample}
\begin{tcblisting}{comment only,
  comment={This is a comment.},
  colback=red!5!white,colframe=red!75!black}
This is a \textbf{tcolorbox}.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}



\begin{docTcbKey}{image comment}{=\marg{options}\marg{filename}}{style, no default, initially unset}
  Uses an image denoted by \meta{filename} as \textit{comment} for the listing.
  The image is included by the standard |\includegraphics| macro with
  given \meta{options}.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,listing side comment,
  image comment={width=2.5cm}{example-image-a.pdf},center lower}
This is a \LaTeX\ example.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}


\clearpage
\begin{docTcbKey}[][doc new=2014-11-14]{tcbimage comment}{=\meta{filename}}{style, no default, initially unset}
  Uses an image denoted by \meta{filename} as \textit{comment} for the listing.
  The image is included by the \refCom{tcbincludegraphics} macro.
  The inclusion can be customized by \refKey{/tcb/comment style}.
  \begin{marker}
  The library \mylib{skins} is needed to apply this option.
  \end{marker}
  \medskip
\begin{dispExample}
% \tcbuselibrary{skins}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,listing side comment,
  righthand width=3cm,lower separated=false,
  tcbimage comment={example-image-a.pdf},
  comment style={size=fbox,colframe=blue,colback=blue!50,sharp corners,
    drop fuzzy shadow}}
This is a \LaTeX\ example.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}

\clearpage

\begin{docTcbKey}[][doc new=2014-11-14]{pdf comment}{\colOpt{=\meta{filename}}}{style, default listing file, initially unset}
  Uses a PDF file denoted by \meta{filename} as \textit{comment} for the listing.
  The image is included by \refCom{tcbincludepdf} inside a \refEnv{tcbraster}.
  The inclusion can be customized by \refKey{/tcb/comment style}.
  \begin{marker}
  The libraries \mylib{skins} and \mylib{raster} are needed to apply this option.
  \end{marker}
  \medskip
\begin{dispExample}
% \tcbuselibrary{skins,raster}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,listing and comment,
  righthand width=3cm,lower separated=false,middle=1mm,
  pdf comment={tcolorbox-example.pdf},
  comment style={raster columns=3,graphics pages={1,2,3},
    colframe=blue,drop fuzzy shadow}}
This is a \LaTeX\ example.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}

\clearpage


\begin{docTcbKey}[][doc new=2014-11-14]{pdf extension}{=\meta{extension}}{no default, initially |pdf|}
  Sets the PDF file name extension for \refKey{/tcb/pdf comment} to \meta{extension}.
  Note that \meta{extension} always overwrites any actual extension given
  inside \refKey{/tcb/pdf comment}.
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2014-11-14]{comment style}{=\meta{options}}{no default, initially empty}
  Sets the \meta{options} for \refKey{/tcb/tcbimage comment} and \refKey{/tcb/pdf comment}.
  These are |tcolorbox| options to customize the colored box drawn around the
  image(s), also image options encapsulated by \refKey{/tcb/graphics options},
  and \refEnv{tcbraster} options for \refKey{/tcb/pdf comment}.
\end{docTcbKey}


\begin{docTcbKey}{listing and comment}{}{no value}
  Typesets the environment content as listing in the upper part and
  a given comment in the lower part.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,listing and comment,
  comment={This is my comment. It may contain line breaks.\par
    It can even use the environment content
    \flqq\ignorespaces\tcbuselistingtext\unskip\frqq}}
This is a \LaTeX\ example.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}

\enlargethispage*{10mm}
\begin{docTcbKey}{comment and listing}{}{no value}
  Typesets a given comment in the upper part and
  the environment content as listing in the lower part.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,comment and listing,
comment={This is my comment.}}
This is a \LaTeX\ example.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}


\clearpage
\begin{docTcbKey}{listing side text}{}{style, no value}
Typesets the environment content side by side as listing in the left (upper)
part and as compiled text in the right (lower) part.
This is a shortcut for setting \refKey{/tcb/listing and text} and \refKey{/tcb/sidebyside}.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,listing side text}
This is a \LaTeX\ example.
\end{tcblisting}
\end{dispExample}
\begin{marker}
Note that |sidebyside=false| has to be added, if the setting of
\refKey{/tcb/listing side text} is to be annihilated.
\end{marker}
\end{docTcbKey}


\begin{docTcbKey}{text side listing}{}{style, no value}
Typesets the environment content side by side as compiled text in the left (upper)
part and as listing in the right (lower) part.
This is a shortcut for setting \refKey{/tcb/text and listing} and \refKey{/tcb/sidebyside}.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,text side listing}
This is a \LaTeX\ example.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{listing outside text}{}{no value}
Typesets the environment content side by side as listing in a |tcolorbox|
and as compiled text outside the box in the right part of the page.
Nevertheless, the outside text is treated as \emph{lower} part of the
|tcolorbox| and can be formatted with all lower part options.
The space partitioning is done with the side by side options from
\Fullref{sec:sidebyside}.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,listing outside text}
This is a \LaTeX\ example.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}

\clearpage

\begin{docTcbKey}{text outside listing}{}{no value}
Typesets the environment content side by side as listing in a |tcolorbox|
and as compiled text outside the box in the left part of the page.
Nevertheless, the outside text is treated as \emph{lower} part of the
|tcolorbox| and can be formatted with all lower part options.
The space partitioning is done with the side by side options from
\Fullref{sec:sidebyside}.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,text outside listing}
This is a \LaTeX\ example.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}



\begin{docTcbKey}{listing side comment}{}{style, no value}
Typesets the environment content side by side as listing in the left (upper)
part and a given comment in the right (lower) part.
This is a shortcut for setting \refKey{/tcb/listing and comment} and \refKey{/tcb/sidebyside}.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,listing side comment,
  righthand width=1.5cm,image comment={width=1.5cm}{example-image-a.pdf}}
This is a \LaTeX\ example.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{comment side listing}{}{style, no value}
Typesets the environment content side by side with a given comment in the left (upper)
part and as listing in the right (lower) part.
This is a shortcut for setting \refKey{/tcb/comment and listing} and \refKey{/tcb/sidebyside}.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,comment side listing,
  lefthand width=1.5cm,image comment={width=1.5cm}{example-image-a.pdf}}
This is a \LaTeX\ example.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}

\clearpage

\begin{docTcbKey}{listing outside comment}{}{no value}
Typesets the environment content side by side as listing in a |tcolorbox|
and a given comment outside the box in the right part of the page.
Nevertheless, the outside text is treated as \emph{lower} part of the
|tcolorbox| and can be formatted with all lower part options.
The space partitioning is done with the side by side options from
\Fullref{sec:sidebyside}.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,listing outside comment,
  righthand width=1.5cm,image comment={width=1.5cm}{example-image-a.pdf}}
This is a \LaTeX\ example.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{comment outside listing}{}{no value}
Typesets the environment content side by side as listing in a |tcolorbox|
and a given comment outside the box in the left part of the page.
Nevertheless, the outside text is treated as \emph{lower} part of the
|tcolorbox| and can be formatted with all lower part options.
The space partitioning is done with the side by side options from
\Fullref{sec:sidebyside}.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,comment outside listing,
  lefthand width=1.5cm,image comment={width=1.5cm}{example-image-a.pdf}}
This is a \LaTeX\ example.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}



\begin{docTcbKey}{listing above text}{}{no value}
  Typesets the environment content as listing in a |tcolorbox|
  and as compiled text outside and below the box.
  The outside text is treated as \emph{lower} part of the
  |tcolorbox| and can be formatted with all lower part options.
  The distance between box and text is controlled by \refKey{/tcb/middle}.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,listing above text}
This is a \LaTeX\ example.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2014-11-07]{listing above* text}{}{no value}
  Widely equal to \refKey{/tcb/listing above text}, but the outside text is
  not formatted with the lower part options.
  Also, it is not put into a minipage and it may span several pages.
  The distance between box and text is controlled by \refKey{/tcb/after}.
\end{docTcbKey}

\clearpage

\begin{docTcbKey}{text above listing}{}{no value}
  Typesets the environment content as listing in a |tcolorbox|
  and as compiled text outside and above the box.
  The outside text is treated as \emph{lower} part of the
  |tcolorbox| and can be formatted with all lower part options.
  The distance between box and text is controlled by \refKey{/tcb/middle}.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,text above listing}
This is a \LaTeX\ example.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2014-11-07]{text above* listing}{}{no value}
  Widely equal to \refKey{/tcb/text above listing}, but the outside text is
  not formatted with the lower part options.
  Also, it is not put into a minipage and it may span several pages.
  The distance between box and text is controlled by \refKey{/tcb/before}.
\end{docTcbKey}



\begin{docTcbKey}{listing above comment}{}{no value}
  Typesets the environment content as listing in a |tcolorbox|
  and a given comment outside and below the box.
  The outside text is treated as \emph{lower} part of the
  |tcolorbox| and can be formatted with all lower part options.
  The distance between box and comment is controlled by \refKey{/tcb/middle}.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,listing above comment,
  center lower,image comment={width=3cm}{example-image-a.pdf}}
This is a \LaTeX\ example.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2014-11-07]{listing above* comment}{}{no value}
  Widely equal to \refKey{/tcb/listing above comment}, but the outside comment is
  not formatted with the lower part options.
  Also, it is not put into a minipage and it may span several pages.
  The distance between box and comment is controlled by \refKey{/tcb/after}.
\end{docTcbKey}

\clearpage

\begin{docTcbKey}{comment above listing}{}{no value}
  Typesets the environment content as listing in a |tcolorbox|
  and a given comment outside and above the box.
  The outside text is treated as \emph{lower} part of the
  |tcolorbox| and can be formatted with all lower part options.
  The distance between box and comment is controlled by \refKey{/tcb/middle}.
\begin{dispExample}
\begin{tcblisting}{colback=red!5!white,colframe=red!75!black,comment above listing,
  center lower,image comment={width=3cm}{example-image-a.pdf}}
This is a \LaTeX\ example.
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2014-11-07]{comment above* listing}{}{no value}
  Widely equal to \refKey{/tcb/comment above listing}, but the outside comment is
  not formatted with the lower part options.
  Also, it is not put into a minipage and it may span several pages.
  The distance between box and comment is controlled by \refKey{/tcb/before}.
\end{docTcbKey}


\clearpage
\subsection{Option Keys for Processing and Full Document Examples}\label{sec:proclistingkeys}
A complete \LaTeX\ document including |\documentclass|, |\begin{document}|
and |\end{document}| cannot be processed directly by |tcolorbox|.
It always has to be compiled separately. There are two methods supported
by the package to process and display such a full document example:
\begin{itemize}
\item Prepare and compile the example document independent from your main
  document. The source file and the resulting PDF file can be included
  into the main document afterwards. This is the most economic way since
  the example document can be left untouched after the example is complete.
\item The other possibility is to compile the example on the fly while
  the main document is compiled. This way has some charm, because the
  example can be edited inside the main document. But be aware that the
  compilation of the example is issued on every run of the main document.
  Also, there are fewer degrees of freedom how the example is compiled.
\end{itemize}

For both methods, the resulting example PDF file can be included
as a \refKey{/tcb/pdf comment}.

The following example shows how to apply the first method.
There already is a file |tcolorbox-example.tex| and a PDF file
|tcolorbox-example.pdf|. Both of them are input partly by the following:

\begin{dispListing}
% \tcbuselibrary{breakable,skins,raster}
\tcbinputlisting{
  enhanced jigsaw,breakable,pad at break*=2mm,height fixed for=first and middle,
  lower separated=false,
  leftlower=0pt,rightlower=0pt,middle=0pt,
  colframe=red!50!black,colback=yellow!10!white,
  listing and comment,
  listing file={tcolorbox-example},
  listing options=
    {style=tcblatex,texcsstyle=*\color{red!70!black},firstline=20,lastline=85},
  after upper={\par\bigskip\texttt{\ldots}\par},
  pdf comment,
  comment style={drop lifted shadow,graphics pages={1,...,4}},
}
\end{dispListing}
{\tcbusetemp}


\clearpage


\begin{docTcbKey}[][doc new=2014-11-14]{no process}{}{no default}
  Removes all processing commands if set before.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-11-14]{process code}{=\meta{code}}{no default, initially empty}
  Adds \meta{code} which is executed during \refCom{tcbinputlisting}
  and \refEnv{tcblisting}. At the time of executing the given \meta{code},
  the listing is already written to \refKey{/tcb/listing file}, but
  the colored box is not constructed yet.
  Its intended use is to process the listing somehow before displaying.
  The processing result can be used inside a \refKey{/tcb/comment}.
  Several \refKey{/tcb/process code} options can be given which are
  processed in the given order.
  Typically, \meta{code} is added by using the following styles
  \refKey{/tcb/run system command}, \refKey{/tcb/run pdflatex}, etc.
\end{docTcbKey}

\begin{marker}
To use the further options, the compiler has to be called with the
|-shell-escape| permission to authorize potentially dangerous system calls.
Be warned that this is a security risk. Anyway, it's more economic to
compile examples independent from the main document and to include them as
shown in the previous pages.
\end{marker}

\begin{docTcbKey}[][doc new=2014-11-14]{run system command}{=\meta{system command}}{style, no default, initially unset}
Runs a \meta{system command}, if the document is compiled with the
|-shell-escape| permission.
The current listing file can be accessed as |\filename@area\filename@base\filename@ext|.
This \meta{system command} is added to \refKey{/tcb/process code}.
\end{docTcbKey}


\begin{docTcbKey}[][doc new and updated={2014-11-14}{2016-05-27}]{compilable listing}{}{style, no default}
  Sets \refKey{/tcb/listing file} to |\jobname|\texttt{-listing-}\meta{counter}.
  \begin{marker}
  The default \refKey{/tcb/listing file} setting cannot be used to compile
  a listing, since the base name equals the |\jobname| and the included PDF
  files should be unique.
  Therefore, to use \refKey{/tcb/run pdflatex} etc., the \refKey{/tcb/listing file}
  has to be set to a unique value.
  One may use \refKey{/tcb/compilable listing} for this purpose.
  \end{marker}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2014-11-14]{run pdflatex}{\colOpt{=\meta{arguments}}}{style, no default, initially unset}
Issues a |pdflatex| compilation of the listing with the given \meta{arguments}.
\begin{itemize}
\item The main document has to be compiled with the |-shell-escape| permission.
\item The \refKey{/tcb/listing file} has to be unique for the listing.
\item If the listing has to be compiled twice, add |run pdflatex| two times to
  the option list.
\end{itemize}

\begin{dispListing*}{breakable,enhanced,pad at break*=2mm,before upper=,after skip=3mm}
\begin{tcblisting}{enhanced jigsaw,lower separated=false,
  leftlower=0pt,rightlower=0pt,
  colframe=red!50!black,colback=yellow!10!white,
  listing options={style=tcblatex,texcsstyle=*\color{red!70!black}},
  listing and comment,
  pdf comment,freeze pdf,
  compilable listing,
  run pdflatex
}
\documentclass{beamer}
\usetheme{Warsaw}
\begin{document}
\begin{frame}{Beamer example}
  \begin{block}{Hello World}
    \begin{itemize}[<+->]
      \item One
      \item Two
    \end{itemize}
  \end{block}

  \begin{alertblock}{Integral}
    \begin{equation}
      \visible<3->{\int\limits_1^x \frac{1}{t}~dt}
      \visible<4->{ = \ln(x).}
    \end{equation}
  \end{alertblock}
\end{frame}
\end{document}
\end{tcblisting}
\end{dispListing*}
{\tcbusetemp}
\end{docTcbKey}


\clearpage
\begin{docTcbKey}[][doc new=2014-11-14]{run xelatex}{\colOpt{=\meta{arguments}}}{style, no default, initially unset}
Issues a |xelatex| compilation of the listing with the given \meta{arguments}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-11-14]{run lualatex}{\colOpt{=\meta{arguments}}}{style, no default, initially unset}
Issues a |lualatex| compilation of the listing with the given \meta{arguments}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-11-14]{run makeindex}{\colOpt{=\meta{arguments}}}{style, no default, initially unset}
Issues a |makeindex| compilation of the listing with the given \meta{arguments}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-11-14]{run bibtex}{\colOpt{=\meta{arguments}}}{style, no default, initially unset}
Issues a |bibtex| compilation of the listing with the given \meta{arguments}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-11-14]{run biber}{\colOpt{=\meta{arguments}}}{style, no default, initially unset}
Issues a |biber| compilation of the listing with the given \meta{arguments}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-11-14]{run arara}{\colOpt{=\meta{arguments}}}{style, no default, initially unset}
Issues an |arara| compilation of the listing with the given \meta{arguments}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-11-14]{run latex}{\colOpt{=\meta{arguments}}}{style, no default, initially unset}
Issues a |latex| compilation of the listing with the given \meta{arguments}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-11-14]{run dvips}{\colOpt{=\meta{arguments}}}{style, no default, initially unset}
Issues a |dvips| compilation of the listing with the given \meta{arguments}.
\end{docTcbKey}

\enlargethispage*{1cm}
\begin{docTcbKey}[][doc new=2014-11-14]{run ps2pdf}{\colOpt{=\meta{arguments}}}{style, no default, initially unset}
Issues a |ps2pdf| compilation of the listing with the given \meta{arguments}.
\end{docTcbKey}

\begin{dispListing*}{breakable,enhanced,pad at break*=2mm,before upper=,after skip=3mm}
\begin{tcblisting}{enhanced jigsaw,
  title={PSTricks with pdflatex},fonttitle=\bfseries,
  colframe=red!50!black,colback=yellow!10!white,
  listing options={style=tcblatex,texcsstyle=*\color{red!70!black}},
  lower separated=false,middle=0pt,
  listing side comment,righthand width=4cm,
  compilable listing,
  run latex,run dvips,run ps2pdf,
  pdf comment,freeze pdf,
  comment style={raster columns=1,
    graphics options={viewport=0.5in 7.7in 3.5in 10.5in,clip}},
}
\documentclass{article}
\usepackage{pstricks,multido}
\begin{document}
\psset{unit=3}%
\multido{\nHue=0.01+0.01}{100}{%
\definecolor{MyColor}{hsb}{\nHue,1,1}%
\pscircle[linewidth=0.01,linecolor=MyColor]{\nHue}}
\end{document}
\end{tcblisting}
\end{dispListing*}
{\tcbusetemp}

\clearpage

\begin{marker}
  For most applications, you will like to add \refKey{/tcb/freeze pdf} as option,
  since the included |pdf| file is only refreshed, if the source for this file
  has changed.
\end{marker}

\begin{docTcbKey}[][doc new=2016-07-14]{freeze file}{=\meta{file}}{no default, initially unset}
  Observes some \meta{file}, usually the final file produced by \refKey{/tcb/process code},
  \refKey{/tcb/run system command}, \refKey{/tcb/run pdflatex}, etc.
  If the MD5 checksum of the current \refKey{/tcb/listing file} is unchanged
  and \meta{file} exists, the processing is skipped and
  the \meta{file} is kept (frozen).
  Typically, the style \refKey{/tcb/freeze pdf} can be used for
  convenience.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2016-07-14]{freeze none}{}{no default, initially set}
  Freeze no file and always execute the given process commands.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2016-07-14]{freeze extension}{=\meta{text}}{style, no default}
  Calls \refKey{/tcb/freeze file} with the current \refKey{/tcb/listing file}
  stripped with its extension plus \meta{text} as new extension.
\begin{dispListing}
  ...
  listing file=myfile.tex,
  freeze extension=-modified.pdf,    % ->   myfile-modified.pdf   is observed
  ...
\end{dispListing}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2016-07-14]{freeze pdf}{}{no value}
  Calls \refKey{/tcb/freeze file} with the current \refKey{/tcb/listing file}
  stripped with its extension plus |.pdf| as new extension.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2016-07-14]{freeze png}{}{no value}
  Calls \refKey{/tcb/freeze file} with the current \refKey{/tcb/listing file}
  stripped with its extension plus |.png| as new extension.
  See the examples for \refKey{/tcb/run pdflatex} and \refKey{/tcb/run ps2pdf}.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2016-07-14]{freeze jpg}{}{no value}
  Calls \refKey{/tcb/freeze file} with the current \refKey{/tcb/listing file}
  stripped with its extension plus |.jpg| as new extension.
\end{docTcbKey}




\clearpage
\subsection{Creation of \LaTeX\ Tutorials}\label{sec:latextutorial}
The following source code gives a guideline for the creation of \LaTeX\ tutorials.
In the next section, a framework for \LaTeX\ exercises is described.
All examples shall be numbered optionally.

Firstly, some additional |tcb| keys are defined for the appearance.
For the examples, three environments |texexp|, |texexptitled|,
and |texexptitledspec| are defined with automatic numbering.

\begin{itemize}
\item |texexp| is used for untitled examles,
\item |texexptitled| is used for titled examles,
\item |texexptitledspec| is used for titled examles with special treatment.
\end{itemize}

\inputpreamblelisting{D}

\begin{dispExample}
\begin{tcblisting}{texexp}
This is a \LaTeX\ example which displays the text as source code
and in compiled form.
\end{tcblisting}
\end{dispExample}


\begin{dispExample}
\begin{texexptitled}{First example with a title line}{firstExample}
Here, we use Example \ref{firstExample} with a title line.
\end{texexptitled}
\end{dispExample}


\begin{dispExample}
\begin{texexp}{}
This is a \LaTeX\ example which displays the text as source code
and in compiled form.
\end{texexp}
\end{dispExample}


\begin{dispExample}
\begin{texexp}{text and listing}
This is a \LaTeX\ example which displays the text as source code
and in compiled form.
\end{texexp}
\end{dispExample}


\begin{dispExample}
\begin{texexp}{listing only}
This is a \LaTeX\ example which displays the text as source code only.
\end{texexp}
\end{dispExample}


\begin{dispExample}
\begin{texexp}{text only}
This is a \LaTeX\ example which displays the text in compiled form only.
\end{texexp}
\end{dispExample}


\begin{dispExample}
\begin{texexptitled}{An Example with a Heading}{heading1}
This is a \LaTeX\ example with a numbered heading line
which can be referred to.
\end{texexptitled}
Here, we see Example \ref{heading1}.
\end{dispExample}


\begin{dispExample}
\begin{texexptitled}[listing only]{Another Example with a Heading}{heading2}
The keys can be used in combination. Here, an example with a heading line
and source code only is given.
\end{texexptitled}
Here, we see Example \ref{heading2}.
\end{dispExample}


\begin{dispListing}
\begin{texexptitled}[float]{A floating Example with a Heading}{heading3}
This is another \LaTeX\ example with numbered heading line.
But now, the box is a floating object.
\end{texexptitled}
\end{dispListing}
\tcbusetemp

\begin{dispExample}
The floating box of the last example is seen as Example \ref{heading3}
on page \pageref{heading3}.
\end{dispExample}


\begin{dispExample}
\begin{texexptitledspec}{Special application}{texexpbox1}
\begin{lstlisting}[style=tcblatex]
Some \LaTeX\ source code.
\end{lstlisting}
\tcblower
For special cases, the environment |texexptitledspec| with style
|example| can be used directly. As one can see, the upper and the lower
part of the box can be used uncoupled also.
\end{texexptitledspec}
\end{dispExample}


The following series of examples demonstrate the application of
\refEnv{tcolorbox} options for diversification.

\begin{dispExample}
\begin{texexptitled}{How to use options (1):\par The basic example}{options1}
\begin{tikzpicture}
\path[fill=yellow!50!white] (0,0) circle (11mm);
\path[fill=white] (0,0) circle (9mm);
\foreach \w/\c in {90/red,210/green,330/blue}
{\path[shading=ball,ball color=\c] (\w:1cm) circle (7mm);}
\end{tikzpicture}
\end{texexptitled}
\end{dispExample}


\begin{dispExample}
\begin{texexptitled}[center lower,enhanced,segmentation hidden,middle=0mm]
  {How to use options (2):\par The text output is centered and the
    segmentation line has vanished.}{options2}
\begin{tikzpicture}
\path[fill=yellow!50!white] (0,0) circle (11mm);
\path[fill=white] (0,0) circle (9mm);
\foreach \w/\c in {90/red,210/green,330/blue}
{\path[shading=ball,ball color=\c] (\w:1cm) circle (7mm);}
\end{tikzpicture}
\end{texexptitled}
\end{dispExample}

\begin{dispExample}
\begin{texexptitled}[tikz lower,bicolor,colbacklower=white]
  {How to use options (3):\par Here, the |tikzpicture| is totally hidden.
    The |bicolor| skin highlights the output.}{options3}
\path[fill=yellow!50!white] (0,0) circle (11mm);
\path[fill=white] (0,0) circle (9mm);
\foreach \w/\c in {90/red,210/green,330/blue}
{\path[shading=ball,ball color=\c] (\w:1cm) circle (7mm);}
\end{texexptitled}
\end{dispExample}

\begin{dispExample}
\begin{texexptitled}[center lower,listing side text,righthand width=3.5cm,
  bicolor,colbacklower=white]
  {How to use options (4):\par The |bicolor| skin also works with side
   by side mode}{options4}
\begin{tikzpicture}
\path[fill=yellow!50!white] (0,0) circle (11mm);
\path[fill=white] (0,0) circle (9mm);
\foreach \w/\c in {90/red,210/green,330/blue}
{\path[shading=ball,ball color=\c]
    (\w:1cm) circle (7mm);}
\end{tikzpicture}
\end{texexptitled}
\end{dispExample}


\begin{dispExample}
\begin{texexptitled}[center lower,listing outside text,righthand width=3.5cm]
  {How to use options (5):\par Putting our picture outside is just
    a matter of one word.}{options5}
\begin{tikzpicture}
\path[fill=yellow!50!white] (0,0) circle (11mm);
\path[fill=white] (0,0) circle (9mm);
\foreach \w/\c in {90/red,210/green,330/blue}
{\path[shading=ball,ball color=\c]
    (\w:1cm) circle (7mm);}
\end{tikzpicture}
\end{texexptitled}
\end{dispExample}


\begin{dispExample}
\begin{texexptitled}[center lower,text above listing]
  {How to use options (6):\par The picture may also be put above
    the listing box.}{options6}
\begin{tikzpicture}
\path[fill=yellow!50!white] (0,0) circle (11mm);
\path[fill=white] (0,0) circle (9mm);
\foreach \w/\c in {90/red,210/green,330/blue}
{\path[shading=ball,ball color=\c]
    (\w:1cm) circle (7mm);}
\end{tikzpicture}
\end{texexptitled}
\end{dispExample}


\begin{dispExample}
\begin{texexptitled}[beamer,center lower,text outside listing,lefthand width=3.5cm]
  {How to use options (7):\par Our style is easily transformed into
    a beamerish one.}{options7}
\begin{tikzpicture}
\path[fill=yellow!50!white] (0,0) circle (11mm);
\path[fill=white] (0,0) circle (9mm);
\foreach \w/\c in {90/red,210/green,330/blue}
{\path[shading=ball,ball color=\c]
    (\w:1cm) circle (7mm);}
\end{tikzpicture}
\end{texexptitled}
\end{dispExample}


\clearpage
\subsection{Creation of \LaTeX\ Exercises}\label{listing:exercises}
In the following, a guideline is given for the creation of \LaTeX\ exercises
with solutions. These solutions are saved to disk for application at a place of
choice.
Therefore, all used exercises are logged to a file |\jobname.records| for automatic
processing. The solution contents themselves are saved to a subdirectory named
|solutions|. Also see \Vref{sec:recording}.

\begin{itemize}
\item Before the first exercise is given,
  \refCom{tcbstartrecording} has to be called to start recording.
\item The solution is given as content of a \refEnv{tcboutputlisting}
  environment. Note, that you can use this content also inside the
  exercise with \refCom{tcbuselistingtext} in compiled form.
\item After the last exercise is given (and before using the solutions),
  \refCom{tcbstoprecording} has to be called to stop recording.
\item The solutions are loaded by \refCom{tcbinputrecords}.
\end{itemize}

Inside the exercise text, there may be text parts which are needed as
\LaTeX\ source code and as compiled text as well. These parts can be
saved by \refEnv{tcbwritetemp} and used in compiled form by \refCom{tcbusetemp}
or as source code by \refCom{tcbusetemplisting}.

At first, we generate some a common style for the exercises and the
solutions. Further, since exercises and solutions should
be numbered, we force to use a label \meta{marker}.
Automatically, the label |exe:|\meta{marker} is used to mark the exercise
and the label |sol:|\meta{marker} is used to mark the solution.

\begin{dispListing}
\tcbset{texercisestyle/.style={arc=0.5mm, colframe=blue!25!yellow!90!white,
  colback=blue!25!yellow!5!white, coltitle=blue!25!yellow!40!black,
  fonttitle=\small\sffamily\bfseries, fontupper=\small, fontlower=\small,
  listing options={style=tcblatex,texcsstyle=*\color{red!40!black}},
}}
\end{dispListing}
\tcbusetemp

With these preparations, the kernel environment |texercise| for our
exercises is created quickly:

\inputpreamblelisting{E}

\clearpage
The following examples demonstrate the application.

\begin{dispListing}
\tcbstartrecording
\end{dispListing}
\tcbusetemp


\begin{dispExample}
\begin{texercise}{tabular_example}
\textit{Create the following table:}\par\smallskip%
\begin{tcboutputlisting}
\begin{tabular}{|p{3cm}|p{3cm}|p{3cm}|p{3cm}|}\hline
\multicolumn{4}{|c|}{\bfseries\itshape Das alte Italien}\\\hline
\multicolumn{2}{|c|}{\bfseries Antike} &
\multicolumn{2}{c|}{\bfseries Mittelalter}\\\hline
\multicolumn{1}{|c|}{\itshape Republik}&
\multicolumn{1}{c|}{\itshape Kaiserreich}&
\multicolumn{1}{c|}{\itshape Franken}&
\multicolumn{1}{c|}{\itshape Teilstaaten}\\\hline
In den Zeiten der r\"{o}mischen Republik standen dem Staat jeweils zwei
Konsuln vor, deren Machtbefugnisse identisch waren. &
Das r\"{o}mische Kaiserreich wurde von einem Alleinherrscher, dem Kaiser,
regiert.
& In der V\"{o}lkerwanderungszeit \"{u}bernahmen die Goten und sp\"{a}ter die
Franken die Vorherrschaft.
& Im sp\"{a}teren Mittelalter regierten F\"{u}rsten einen Fleckenteppich
von Einzelstaaten.\\\hline
\end{tabular}
\end{tcboutputlisting}
\tcbuselistingtext%
\end{texercise}
\end{dispExample}


\begin{dispExample}
\begin{texercise}{macro_oneparam}
\begin{tcboutputlisting}
\newcommand{\headingline}[1]{%
  \begin{center}\Large\bfseries #1\end{center}}
\end{tcboutputlisting}
\tcbuselistingtext%

Create a new macro \verb+\headingline+ which produces the
following output:\par\smallskip
\begin{tcbwritetemp}
\headingline{Very important heading}
\end{tcbwritetemp}
\tcbusetemplisting\tcbusetemp%
\end{texercise}
\end{dispExample}



\begin{dispExample}
\begin{texercise}{macro_twoparam}
\begin{tcboutputlisting}
\newcommand{\minitable}[2]{%
  \begin{center}\begin{tabular}{p{10cm}}\hline%
  \multicolumn{1}{c}{\bfseries#1}\\\hline%
  #2\\\hline%
  \end{tabular}\end{center}}
\end{tcboutputlisting}
\tcbuselistingtext%
Create a new macro \verb+\minitable+ which produces the
following output:\par\smallskip
\begin{tcbwritetemp}
\minitable{My heading}{In this tiny tabular, there is only a heading
  and some text below which has a width of ten centimeters.}
\end{tcbwritetemp}
\tcbusetemplisting\par\smallskip\tcbusetemp%
\end{texercise}
\end{dispExample}


\begin{dispExample}
\begin{texercise}{macro_threeparam}
\begin{tcboutputlisting}
\newcommand{\synop}[3]{%
  \begin{tabular}{@{}p{(\linewidth-\tabcolsep*2-\arrayrulewidth)/2}|%
    p{(\linewidth-\tabcolsep*2-\arrayrulewidth)/2}@{}}\hline
  \multicolumn{2}{c}{\bfseries #1}\\\hline
  \multicolumn{1}{c|}{\itshape English}&
  \multicolumn{1}{c}{\itshape German}\\\hline
  #2 & #3
  \end{tabular}}
\end{tcboutputlisting}
\tcbuselistingtext%
Create a new macro \verb+\synop+ which typesets a synoptic text according
to the following example. Base your macro on a tabular which takes the
total line width.\par\smallskip
\begin{tcbwritetemp}
\synop{Neil Armstrong}%
{That's one small step for a man, one giant leap for mankind.}%
{Das ist ein kleiner Schritt f\"{u}r einen Mann,
   ein riesiger Sprung f\"{u}r die Menschheit.}
\end{tcbwritetemp}
\tcbusetemplisting\par\smallskip\tcbusetemp%
\end{texercise}
\end{dispExample}
%\closeoutsol

\begin{dispListing}
\tcbstoprecording
\end{dispListing}
\tcbusetemp

\bigskip

Now, we give a list of all exercises with:

\begin{dispListing}
\tcblistof[\subsection]{exam}{List of Exercises%
  \label{listofexercises}}
\end{dispListing}
\tcbusetemp

\clearpage
\subsection{Solutions for the given \LaTeX\ Exercises}

For all solutions, a macro |\processsol| was written to the file |\jobname.records|.
Now, we need a definition for this macro to use the solutions.

\begin{dispListing}
% \usepackage{hyperref} % for phantomlabel
\newtcbinputlisting{\processsol}[2]{%
  texercisestyle,
  listing only,
  listing file={#1},
  phantomlabel={sol:#2},%
  title={Solution for Exercise \ref{exe:#2} on page \pageref{exe:#2}},
}
\end{dispListing}
\tcbusetemp

The loading of all solutions is done by:

\begin{dispListing}
\tcbinputrecords
\end{dispListing}

With this, we get:

\tcbusetemp





==> tcolorbox.doc.magazine.tex <==
% !TeX root = tcolorbox.tex
% include file of tcolorbox.tex (manual of the LaTeX package tcolorbox)
\clearpage
\section{Library \mylib{magazine}}\label{sec:magazine}%
\tcbset{external/prefix=external/magazine_}%
\newboxarray{myarticle}

\begin{tcolorbox}[
  enhanced jigsaw,
  size=small,width=6cm,
  title=Example Article,
  fonttitle=\bfseries,center title,
  fontupper=\small,
  %height fixed for=first and middle,
  watermark text=\arabic{tcbbreakpart},
  breakable,
  break at=8.5\baselineskip/9\baselineskip,
  reset and store to box array=myarticle,
  colframe=green!50!black,
  colback=green!10,
  pad at break=5mm,
  ]
This is an example for an article which starts right here and
is continued to the following pages.
The body text for the article is written inside a single
|tcolorbox|. This box is split into parts using the tools from
this section, namely \refKey{/tcb/reset and store to box array}
with a new box array |myarticle| which was created by
|\newboxarray{myarticle}|.

The resulting parts are distributed throughout this
\Fullref{sec:magazine} using \refCom{consumetcboxarray}
at the appropriate places you see.
The linking texts like \emph{continued on page x} are created
by \refKey{/tcb/finish} commands for the embedding \refCom{tcbox}.
To label the box parts, \refKey{/tcb/phantomlabel} is used.

These quite small partial boxes are for demonstration purposes.
With the tools of this section, a magazine type document could be
created, but this still needs a lot of manual control.
\end{tcolorbox}

\newtcolorbox{articleside}[1][]{blanker,sidebyside,sidebyside gap=5mm,sidebyside align=top seam,
  parbox=false,righthand width=6cm,
  goto/.style={finish={\node[above=-2pt,color=green!50!black] at (frame.south)
    {\slshape\scriptsize --- continued on page~\hypersetup{linkcolor=green!50!black}\pageref{myarticle-##1}\ \textcolor{green!50!black}{---}};}},
  from/.style={finish={\node[below=-1pt,color=green!50!black] at (frame.north)
    {\slshape\scriptsize --- continued from page~\hypersetup{linkcolor=green!50!black}\pageref{myarticle-##1}\ \textcolor{green!50!black}{---}};}},
  #1}

\begin{articleside}[after skip=6pt]
The main purpose of this library is to store a |tcolorbox| into an array
of box registers for later usage.

If the |tcolorbox| is not breakable, there is not much add-on
compared to usual \TeX/\LaTeX\ box storage and usage (and you do not really need this
library for that use case).
For a breakable |tcolorbox|, this library allows to capture all partial boxes
into a sequence of registers. The partial boxes can be used anywhere in
arbitrary order.
\tcblower\consumetcboxarray[myarticle]{1}{blanker,nobeforeafter,phantomlabel=myarticle-one,goto=two}
\end{articleside}

The name of this library indicates \emph{magazine} in the sense of storage,
but also in the sense of a journal where an article often is \emph{continued on page x}.
An example for this kind of application is given throughout this section starting
on the right hand side. The creation of this library was motivated by
Ulrike Fischer and Steven B.~Segletes.

The library is loaded by a package option or inside the preamble by:
\begin{dispListing}
  \tcbuselibrary{magazine}
\end{dispListing}
This also loads the library \mylib{breakable}, see \Fullref{sec:breakable}.

\begin{marker}
The box register operations of this library are global. \TeX\ grouping will
not clear the registers when leaving the current group. Also be aware that
extensive use of large box arrays may eat up \TeX's available memory and
registers.
\end{marker}

\subsection{Creation and Resetting of Box Arrays}\label{subsec:magazine_creation}

\begin{docCommand}[doc new=2015-07-13]{newboxarray}{\marg{name}}
  This creates a new box array called \meta{name}. There already is a
  box array available with name |default| which can be used directly.
  Note that the creation is a global operation.
\begin{dispListing}
\newboxarray{myarray}
\end{dispListing}
\end{docCommand}


\begin{docCommand}[doc new=2015-07-13]{boxarrayreset}{\oarg{name}}
  Resets the size counter of a box array \meta{name} to zero.
  If \meta{name} is not provided, |default| is used as name.
  Use this or \refKey{/tcb/reset box array} before
  you apply \refKey{/tcb/store to box array}. Otherwise, all boxes would
  be appended to the already existing boxes.
  This command does not clear box registers.
\begin{dispListing}
\boxarrayreset            % resets 'default'
\boxarrayreset{myarray}   % resets 'myarray'
\end{dispListing}
\end{docCommand}

\enlargethispage*{20mm}

\begin{docTcbKey}[][doc new=2015-07-13]{reset box array}{\colOpt{=\meta{name}}}{default |default|, initially unset}
  Resets the size counter of a box array \meta{name} to zero.
  Use this or \refCom{boxarrayreset} (which does the same) before
  you apply \refKey{/tcb/store to box array}.
\begin{dispListing}
\tcbset{
  reset box array,         % resets 'default'
  reset box array=myarray, % resets 'myarray'
}
\end{dispListing}
\end{docTcbKey}

\clearpage
\begin{docCommand}[doc new=2015-07-13]{boxarrayclear}{\oarg{name}}
  Works like \refCom{boxarrayreset} to reset the size counter of a
  box array \meta{name} to zero. Additionally, all allocated box registers
  of the box array are cleared of their content.
  Note that the allocated box registers stay allocated. So, this may be
  useful to clear memory, but not to free registers for other applications.
  If \refCom{consumeboxarray} or \refCom{consumetcboxarray} was used to
  apply the stored boxes, there is no advantage in using \refCom{boxarrayclear}.
\begin{dispListing}
\boxarrayclear            % clears 'default'
\boxarrayclear{myarray}   % clears 'myarray'
\end{dispListing}
\end{docCommand}



\subsection{Storing Content}\label{subsec:magazine_storing}

\begin{docTcbKey}[][doc new=2015-07-13]{store to box array}{\colOpt{=\meta{name}}}{default |default|, initially unset}
Stores a |tcolorbox| or all parts of a break sequence of a |tcolorbox| into
a box array \meta{name}. If no \meta{name} is given, the already existing |default|
box array is used. Otherwise, the box array has to be created beforehand
with \refCom{newboxarray}. Note that the box has to be \refKey{/tcb/breakable},
if the box shall break into several parts.
Typically, manual break points are additionally defined by \refKey{/tcb/break at}.
Otherwise, the box parts will have a length of about |\textheight|.
For most use cases, a \refKey{/tcb/reset box array} should be applied
to reset the box array counter.\enlargethispage*{2cm}

\begin{exdispExample}{storetoboxarray_1}
% \usepackage{lipsum}
\begin{tcolorbox}[enhanced jigsaw,size=fbox,width=4cm,
  colback=yellow!10,colframe=yellow!10!black,
  enforce breakable,% use only breakable in the real world!
  break at=7cm/4cm,
  height fixed for=all,
  watermark text=\arabic{tcbbreakpart},
  reset box array,
  store to box array
  ]
\lipsum[1]
\end{tcolorbox}

\useboxarray{1}\hfill
\begin{tabular}[b]{cc}
\multicolumn{2}{c}{\includegraphics[width=7cm]{Basilica_5.png}}\\
\useboxarray{2} & \useboxarray{3}
\end{tabular}
\end{exdispExample}

\clearpage
If the first box part should fill the rest of the available space of
the current page, you can use |\pagegoal-\pagetotal| minus some distance for
the first element of \refKey{/tcb/break at}. You may want to have some
additional distance to the preceeding text.

\begin{dispListing}
% \usepackage{lipsum}
\begin{tcolorbox}[enhanced,breakable,
  reset box array,
  store to box array,
  break at=\pagegoal-\pagetotal-5mm/0pt,
  height fixed for=first and middle]
\lipsum[1-15]
\end{tcolorbox}%
%
\consumetcboxarray{1}{blanker,before=\par\vfill\noindent}
\end{dispListing}


\begin{exdispExample}{storetoboxarray_2}
\begin{tcolorbox}[blanker,width=4cm,
  fontupper=\footnotesize,
  enforce breakable,% use only breakable in the real world!
  break at=4cm,
  height fixed for=all,
  watermark text=\arabic{tcbbreakpart},
  reset box array,
  store to box array
  ]
\includegraphics[width=\linewidth]{Basilica_5.png}\par
\lipsum[1-2]
\end{tcolorbox}

\begin{tcbitemize}[raster columns=3,raster equal height,
  size=small,halign=center,sharp corners,colback=blue!5]
\tcbitem\consumeboxarray{5}
\tcbitem\consumeboxarray{6}
\tcbitem\consumeboxarray{1}
\tcbitem\consumeboxarray{2}
\tcbitem\consumeboxarray{3}
\tcbitem\consumeboxarray{4}
\end{tcbitemize}
\end{exdispExample}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2015-07-13]{reset and store to box array}{\colOpt{=\meta{name}}}{style, default |default|, initially unset}
  Combination of \refKey{/tcb/reset box array} and \refKey{/tcb/store to box array}.
\end{docTcbKey}



\begin{docTcbKey}[][doc new=2015-07-13]{do not store to box array}{}{style, no default, initially set}
Disables the \refKey{/tcb/store to box array} option, if set before.
\end{docTcbKey}


\begin{docEnvironment}[doc new=2015-07-13]{boxarraystore}{\marg{name}}
  Stores the environment content into a box array \meta{name}.
  This corresponds to the standard \LaTeX\ environment |lrbox|, but
  the storage operation is global. As long as \refCom{boxarrayreset} is
  not used, every new \refEnv{boxarraystore} adds a further box to
  the array.

\begin{dispExample}
\boxarrayreset
\begin{boxarraystore}{default}\fbox{Mary}\end{boxarraystore}
\begin{boxarraystore}{default}\fbox{Had}\end{boxarraystore}
\begin{boxarraystore}{default}\fbox{a}\end{boxarraystore}
\begin{boxarraystore}{default}\fbox{Little}\end{boxarraystore}
\begin{boxarraystore}{default}\fbox{Lamb}\end{boxarraystore}
\useboxarray{5}\useboxarray{4}\useboxarray{3}\useboxarray{2}\useboxarray{1}\hfill
\useboxarray{1}\useboxarray{5}
\end{dispExample}
\end{docEnvironment}

\subsection{Retrieving Content}\label{subsec:magazine_retrieve}

\begin{docCommand}[doc new=2015-07-13]{boxarraygetsize}{\oarg{name}\marg{macro}}
\begin{articleside}[before skip=5pt]
  Stores the current size of a box array \meta{name} into a given \meta{macro}.
  If no \meta{name} is given, the already existing |default| box array is used.
\begin{dispExample}
\boxarraygetsize{\mysize}
Current size of the default box array:
\mysize.
\end{dispExample}
\tcblower\consumetcboxarray[myarticle]{2}{blanker,nobeforeafter,phantomlabel=myarticle-two,from=one,goto=three}
\end{articleside}
\end{docCommand}

\begin{docCommand}[doc new=2015-07-13]{useboxarray}{\oarg{name}\marg{index}}
  Typesets the box with the given \meta{index} number from the box array \meta{name}.
  If no \meta{name} is given, the already existing |default| box array is used.
  It is considered an error, if a not existing box array \meta{name} is used.
  It is silently ignored, if the \meta{index} is out of range.
  Note that \refCom{useboxarray} corresponds to the standard |\usebox| macro,
  respectively, |\copy|.
\begin{dispExample}
\boxarraygetsize{\mysize}
\foreach \n in  {1,...,\mysize} { \useboxarray{\n} }
\end{dispExample}
\end{docCommand}

\clearpage
\begin{docCommand}[doc new=2015-07-13]{usetcboxarray}{\oarg{name}\marg{index}\marg{options}}
  Typesets the box with the given \meta{index} number from the box array \meta{name}
  using \refCom{useboxarray} as content of a \refCom{tcbox}.
  If no \meta{name} is given, the already existing |default| box array is used.
  It is considered an error, if a not existing box array \meta{name} is used.
  It is silently ignored, if the \meta{index} is out of range.
  The \refCom{tcbox} can be customized by |tcolorbox| \meta{options}.
\begin{dispExample}
\boxarraygetsize{\mysize}
\foreach \n in  {1,...,\mysize} { \usetcboxarray{\n}{on line,colframe=yellow,
  colback=yellow!10} }
\end{dispExample}
\end{docCommand}


\begin{docCommand}[doc new=2015-07-13]{consumeboxarray}{\oarg{name}\marg{index}}
  Typesets the box with the given \meta{index} number from the box array \meta{name}.
  If no \meta{name} is given, the already existing |default| box array is used.
  It is considered an error, if a not existing box array \meta{name} is used.
  It is silently ignored, if the \meta{index} is out of range.
  In contrast to \refCom{useboxarray},
  \refCom{consumeboxarray} corresponds to the standard |\box| macro, i.e.
  after typesetting the box register is cleared and cannot be used again.
\begin{dispExample}
\boxarraygetsize{\mysize}
First run: \foreach \n in  {1,...,\mysize} { \consumeboxarray{\n} }
\par
Second run: \foreach \n in  {1,...,\mysize} { \consumeboxarray{\n} }
\end{dispExample}
\end{docCommand}


\begin{docCommand}[doc new=2015-07-13]{consumetcboxarray}{\oarg{name}\marg{index}\marg{options}}
\begin{articleside}[before skip=5pt]
  Typesets the box with the given \meta{index} number from the box array \meta{name}
  using \refCom{consumeboxarray} as content of a \refCom{tcbox}.
  If no \meta{name} is given, the already existing |default| box array is used.
  It is considered an error, if a not existing box array \meta{name} is used.
  It is silently ignored, if the \meta{index} is out of range.
  The \refCom{tcbox} can be customized by |tcolorbox| \meta{options}.
  After typesetting the box register is cleared and cannot be used again.
\tcblower\consumetcboxarray[myarticle]{3}{blanker,nobeforeafter,phantomlabel=myarticle-three,,from=two,goto=four}
\end{articleside}
\begin{exdispExample}{consumetcboxarray}
% \usepackage{lipsum}
\begin{tcolorbox}[enhanced jigsaw,size=fbox,width=6cm,
  colback=yellow!10,colframe=yellow!10!black,
  enforce breakable,% use only breakable in the real world!
  break at=5cm,
  watermark text=\arabic{tcbbreakpart},
  reset and store to box array
  ]
\lipsum[1]
\end{tcolorbox}

\consumeboxarray{2} \hfill \consumeboxarray{1} \hfill \consumeboxarray{1}
\end{exdispExample}
\end{docCommand}


\begin{docCommand}[doc new=2015-07-13]{boxarraygetbox}{\oarg{name}\marg{macro}\marg{index}}
  Assigns the box with the given \meta{index} number from the box array \meta{name}
  to a \meta{macro}.
  If no \meta{name} is given, the already existing |default| box array is used.
  It is considered an error, if a not existing box array \meta{name} is used.
  If the \meta{index} is out of range, the \meta{macro} will be undefined.
\begin{exdispExample}{boxarraygetbox}
\tcbox[size=small,colframe=blue!20,colback=yellow!5,on line,
  reset and store to box array]{Test}

\boxarraygetsize{\mysize} Array size: \mysize

\boxarraygetbox{\mybox}{1}
Box width: \the\wd\mybox
\quad\usebox{\mybox}
\end{exdispExample}
\end{docCommand}


\begin{docCommand}[doc new=2017-06-27]{ifboxarrayempty}{\oarg{name}\marg{index}\marg{true}\marg{false}}
  Tests the box with the given \meta{index} number from the box array \meta{name}
  for emptiness be empty and executes \meta{true} if it is empty, and \meta{false} otherwise.
  If no \meta{name} is given, the already existing |default| box array is used.
  It is considered an error, if a not existing box array \meta{name} is used.
\begin{exdispExample}{ifboxarrayempty}
\tcbox[size=small,colframe=blue!20,colback=yellow!5,on line,
  reset and store to box array]{Test}

\ifboxarrayempty{1}{no Box~1}{Box~1: \useboxarray{1}},
\ifboxarrayempty{2}{no Box~2}{Box~2: \useboxarray{2}}
\end{exdispExample}
\end{docCommand}


\clearpage
\subsection{Box Dimensions}\label{subsec:magazine_dimensions}

\begin{docCommand}[doc new=2015-07-13]{boxarraygetwidth}{\oarg{name}\marg{macro}\marg{index}}
  Assigns the width of the box with the given \meta{index} number from the box array \meta{name}
  to a \meta{macro}.
  If no \meta{name} is given, the already existing |default| box array is used.
  It is considered an error, if a not existing box array \meta{name} is used.
  If the \meta{index} is out of range, the \meta{macro} will be set to |0pt|.
\begin{exdispExample}{boxarraygetwidth}
\tcbox[size=small,colframe=blue!20,colback=yellow!5,on line,
  reset and store to box array]{Test}

\begin{tabular}{ll}
\useboxarray{1} & width of box 1: \boxarraygetwidth{\mylen}{1} \mylen\\
\useboxarray{2} & width of box 2: \boxarraygetwidth{\mylen}{2} \mylen
\end{tabular}
\end{exdispExample}
\end{docCommand}


\begin{docCommand}[doc new=2015-07-13]{boxarraygetheight}{\oarg{name}\marg{macro}\marg{index}}
  Assigns the height of the box with the given \meta{index} number from the box array \meta{name}
  to a \meta{macro}.
  If no \meta{name} is given, the already existing |default| box array is used.
  It is considered an error, if a not existing box array \meta{name} is used.
  If the \meta{index} is out of range, the \meta{macro} will be set to |0pt|.
\begin{exdispExample}{boxarraygetheight}
\tcbox[size=small,colframe=blue!20,colback=yellow!5,on line,
  reset and store to box array]{Test}

\begin{tabular}{ll}
\useboxarray{1} & height of box 1: \boxarraygetheight{\mylen}{1} \mylen\\
\useboxarray{2} & height of box 2: \boxarraygetheight{\mylen}{2} \mylen
\end{tabular}
\end{exdispExample}
\end{docCommand}


\begin{docCommand}[doc new=2015-07-13]{boxarraygetdepth}{\oarg{name}\marg{macro}\marg{index}}
  Assigns the depth of the box with the given \meta{index} number from the box array \meta{name}
  to a \meta{macro}.
  If no \meta{name} is given, the already existing |default| box array is used.
  It is considered an error, if a not existing box array \meta{name} is used.
  If the \meta{index} is out of range, the \meta{macro} will be set to |0pt|.
\begin{exdispExample}{boxarraygetdepth}
\tcbox[size=small,colframe=blue!20,colback=yellow!5,on line,
  reset and store to box array]{Test}

\begin{tabular}{ll}
\useboxarray{1} & depth of box 1: \boxarraygetdepth{\mylen}{1} \mylen\\
\useboxarray{2} & depth of box 2: \boxarraygetdepth{\mylen}{2} \mylen
\end{tabular}
\end{exdispExample}
\end{docCommand}


\clearpage
\begin{docCommand}[doc new=2015-07-13]{boxarraygettotalheight}{\oarg{name}\marg{macro}\marg{index}}
\begin{articleside}[before skip=5pt]
  Assigns the total height of the box with the given \meta{index} number from the box array \meta{name}
  to a \meta{macro}.
  If no \meta{name} is given, the already existing |default| box array is used.
  It is considered an error, if a not existing box array \meta{name} is used.
  If the \meta{index} is out of range, the \meta{macro} will be set to |0pt|.
\tcblower\consumetcboxarray[myarticle]{4}{blanker,nobeforeafter,phantomlabel=myarticle-four,from=three}
\end{articleside}
\begin{exdispExample}{boxarraygettotalheight}
\boxarrayreset
\tcbox[size=small,colframe=blue!20,colback=yellow!5,on line,
  store to box array]{Test}

\begin{tabular}{ll}
\useboxarray{1} & total height of box 1: \boxarraygettotalheight{\mylen}{1} \mylen\\
\useboxarray{2} & total height of box 2: \boxarraygettotalheight{\mylen}{2} \mylen
\end{tabular}
\end{exdispExample}
\end{docCommand}

\clearpage
\subsection{Leaflet Example}
The following full application example can be used to create leaflets.
Obviously, the code can be adapted and customized in many ways.

\begin{tcblisting}{
  enhanced jigsaw,lower separated=false,breakable,
  listing style=mydocumentation,base example,
  listing and comment,
  pdf comment,freeze pdf,
  comment style={raster columns=1},
  compilable listing,
  run pdflatex}
\documentclass[a4paper,landscape]{article}
\usepackage[noheadfoot,margin=0pt]{geometry}
\usepackage[skins,raster,magazine]{tcolorbox}
\usepackage{lipsum}

\newenvironment{leaflet}[1][]{%
  \begin{tcolorbox}[nobeforeafter,empty,colback=white,
    sharp corners,size=minimal,left=10mm,right=10mm,top=10mm,bottom=10mm,
    width=\textwidth/3,
    breakable,
    break at=\textheight,
    height fixed for=all,
    reset box array,
    store to box array,#1]}
  {\end{tcolorbox}%
    \begin{tcbitemize}[raster columns=3,raster equal skip=0pt,blankest]
      \tcbitem\consumeboxarray{5}
      \tcbitem\consumeboxarray{6}
      \tcbitem\consumeboxarray{1}
      \tcbitem\consumeboxarray{2}
      \tcbitem\consumeboxarray{3}
      \tcbitem\consumeboxarray{4}
    \end{tcbitemize}%
  }

\pagestyle{empty}
\begin{document}

\begin{leaflet}[underlay={\node[above=5mm,font=\footnotesize]
    at (frame.south) {- \arabic{tcbbreakpart} -};}]
  \includegraphics[width=\linewidth]{Basilica_5.png}
  \begin{center}
  \bfseries\LARGE Example
  \end{center}

  \section{Introduction}
  \lipsum[1]

  \section{Main Part A}
  \lipsum[2-8]

  \section{Main Part B}
  \lipsum[9-15]

  \section{Conclusion}
  \lipsum[16-18]
\end{leaflet}

\end{document}
\end{tcblisting}




==> tcolorbox.doc.picturecredits.tex <==
% !TeX root = tcolorbox.tex
% include file of tcolorbox.tex (manual of the LaTeX package tcolorbox)
\clearpage
\section{Picture Credits}%
\tcbset{external/prefix=external/picturecredits_}%
The following pictures were used inside this documentation.

\DeclareTotalTColorBox{\diabox}{ O{} v  m }
  { bicolor,fonttitle=\bfseries\ttfamily,adjusted title={#2},center title,
    colframe=blue!20!black,leftupper=0mm,rightupper=0mm,colback=black!75!white,
    finish vignette={size=1.5mm},#1}
  { \tikz\path[fill zoom image={#2}] (0,0) rectangle (\linewidth,4cm);%
    \tcblower#3}

\begin{tcbraster}[raster equal height]
\diabox{Basilica_5.png}{
  \url{http://commons.wikimedia.org/wiki/File:Basilica_5.png}}
\diabox{lichtspiel.jpg}{
  Photograph taken by Thomas F.~Sturm.}
\diabox{crinklepaper.png}{%
  Created with |GIMP|.\\
  \url{http://www.gimp.org}}
\diabox{pink_marble.png}{%
  Created with |GIMP|.\\
  \url{http://www.gimp.org}}
\diabox{blueshade.png}{%
  Created with |GIMP|.\\
  \url{http://www.gimp.org}}
\diabox{goldshade.png}{%
  Created with |GIMP|.\\
  \url{http://www.gimp.org}}
\end{tcbraster}



==> tcolorbox.doc.poster.tex <==
% !TeX root = tcolorbox.tex
% include file of tcolorbox.tex (manual of the LaTeX package tcolorbox)
\clearpage
\section{Library \mylib{poster}}\label{sec:poster}%
\tcbset{external/prefix=external/poster_}%

The main purpose of this library is to support creation of single page posters
with |tcolorbox|es.

A \refEnv{tcbposter} is a |tikzpicture| where |tcolorbox|es can be
placed in a column oriented manner using \refCom{posterbox} commands.
This base concept is more or less copied from the great |baposter| package.

The \mylib{raster} library, see \Fullref{sec:raster}, can produce
similar looking results and may be more appropriate
depending on the actual project.
\begin{itemize}
\item The \mylib{raster} library has a flow oriented concept, just like a
  convential text flow. The text flow (box flow) is a merely endless ribbon
  which gets broken into lines (and paragraphs) and the lines are broken
  into pages. \mylib{raster} shapes the boxes to convenient sizes to fill
  lines and pages in a pleasant way.
\item The \mylib{tcbposter} library supports a quite free placement of
  boxes inside a page.
  Basically, boxes are placed like |node|s are placed inside a |tikzpicture|.
  In contrast to \mylib{raster}, this is a \emph{single} page
  and not a flow of pages.
  The poster is divided into columns and rows.
  There is a more or less gentle force to use the columns (or spans of columns)
  for positioning and sizing while the row placement is completely optional.
\end{itemize}
The creation of this library was motivated by Ignasi.

\begin{marker}
Inside a |tikzpicture| there should be no embedded |tikzpicture|s.
This rule is violated by the \mylib{poster} library. Be aware that there
may be some unwanted interactions between the main |tikzpicture| and
the embedded ones inside the |tcolorbox|es.
\end{marker}

The library is loaded by a package option or inside the preamble by:
\begin{dispListing}
\tcbuselibrary{poster}
\end{dispListing}
This also loads the libraries
\mylib{skins}, see \Fullref{sec:skins},
\mylib{breakable}, see \Fullref{sec:breakable},
\mylib{magazine}, see \Fullref{sec:magazine}, and
\mylib{fitting}, see \Fullref{sec:fitting}.


%--------------------------
\subsection{Overview}\label{subsec:poster_overview}


\begin{tcolorbox}[base example,hyperurl={tcolorbox-tutorial-poster.pdf},title=Click me to see the tutorial]
You get the best overview of the \mylib{poster} library and its facilities,
if you look at the \textbf{Poster Tutorial} which is part of the |tcolorbox|
documentation:\par
\texttt{tcolorbox-tutorial-poster.pdf}
\end{tcolorbox}



\clearpage
%--------------------------
\subsection{Main Poster Environment}\label{subsec:poster_environment}

\begin{docEnvironment}[doc new=2017-07-03]{tcbposter}{\oarg{options}}
  This creates a |tikzpicture| environment with suitable additional
  settings defined by the given \meta{options}.
  Basically, \refCom{posterbox} and \refEnv{posterboxenv} are
  used to place |tcolorboxes| as nodes into the environment,
  but additional \tikzname\ code can also be used.
  As \meta{options} all |/tcb/posterset/| keys may be applied, namely:
\begin{itemize}
\item\refKey{/tcb/posterset/poster}: poster settings like columns, rows, sizes\ldots
\item\refKey{/tcb/posterset/coverage} and \refKey{/tcb/posterset/no coverage}:
  settings for a surrounding |tcolorbox| for background and margins.
\item\refKey{/tcb/posterset/boxes}: style of the |tcolorbox|es used for the poster.
\item\refKey{/tcb/posterset/fontsize}: scaling of used fonts.
\end{itemize}

\begin{exdispExample}{tcbposter}
  \begin{tcbposter}[
    poster = {showframe,height=10cm,spacing=2mm},
    boxes  = {beamer,colframe=blue!50!black,colback=blue!50,colupper=yellow!50},
  ]
  \posterbox{name=A,column=3,row=2}{My first box}
  \posterbox[adjusted title=Second box]
            {name=B,column=2,span=2,below=A}{My second box}
  \posterbox[adjusted title=Third box]
            {name=C,column=2,between=B and bottom}{My third box}
  \end{tcbposter}
\end{exdispExample}
\end{docEnvironment}

\clearpage
  Inside \refEnv{tcbposter}, there are several predefined \tikzname\ nodes.
  These nodes share a common \refKey{/tcb/poster/prefix} which is
  |TCBPOSTER@| by default. This prefix is used to discriminate the
  poster nodes from local nodes of any embedded |tikzpicture| environment.
  You will never need this prefix using \refCom{posterbox} and its
  placement options, but if you want to refer to a predefined node using
  pure \tikzname\ code.
  The predefined nodes (shown without prefix) are:
  \begin{itemize}
  \item|poster|: defines the bounding box of the poster (without the coverage).
  \item|top|: top position plus row spacing
  \item|bottom|: bottom position minus row spacing
  \item|middle|: vertical middle position
  \item|col1|, |col2|, \ldots: bounding box of column~1, column~2, \ldots
  \item|row1|, |row2|, \ldots: bounding box of row~1, row~2, \ldots
  \end{itemize}
  Further nodes are defined using the \refKey{/tcb/posterloc/name} option.

  \begin{marker}
  Never use a \refEnv{tcbposter} inside a \refEnv{tcbposter}.
  But, if you do anyway, use a different \refKey{/tcb/poster/prefix} for
  the embedded poster or you surely get a total mess.
  \end{marker}

  There are several properties inside a \refEnv{tcbposter} which may be useful
  for advanced code (skip the following on first reading):
  \begin{itemize}
  \item\docAuxCommand{tcbposterwidth}: Width of the poster (without margins).
  \item\docAuxCommand{tcbposterheight}: Height of the poster (without margins).
  \item\docAuxCommand{tcbpostercolspacing}: Column distance.
  \item\docAuxCommand{tcbposterrowspacing}: Row distance.
  \item\docAuxCommand{tcbpostercolumns}: Column quantity.
  \item\docAuxCommand{tcbposterrows}: Row quantity.
  \item\docAuxCommand{tcbpostercolwidth}: Width of a column.
  \item\docAuxCommand{tcbposterrowheight}: Height of a row.
  \end{itemize}

\medskip
\begin{docCommand}[doc new=2017-07-03]{tcbposterset}{\marg{options}}
  Sets options for every following \refEnv{tcbposter} inside the current \TeX\ group.
  For example, the numbers for rows and columns may be defined for the whole document by this:
\begin{dispListing}
\tcbposterset{poster={columns=2,rows=3}}
\end{dispListing}
  See \refEnv{tcbposter} for all feasible options.
\end{docCommand}


\clearpage
%--------------------------
\subsection{Poster Settings}\label{subsec:poster_settings}

\begin{postersetTcbKey}[][doc new=2017-07-03]{poster}{=\marg{option list}}{style, no default}
  This option can be applied inside \refEnv{tcbposter} and \refCom{tcbposterset}
  to set the given poster \meta{option list}, e.g.
\begin{dispListing}
\tcbposterset{poster={width=20cm,height=15cm}}
\end{dispListing}
  For the \meta{option list}, see the following keys.
\end{postersetTcbKey}


\begin{posterTcbKey}[][doc new=2017-07-03]{columns}{=\meta{number}}{no default, initially |3|}
  Sets the \meta{number} of columns for a |tcbposter|.
\begin{exdispExample}{columns}
  \begin{tcbposter}[
    poster = {showframe,columns=5,rows=2,spacing=1mm,height=4cm},
  ]
  \end{tcbposter}
\end{exdispExample}
\end{posterTcbKey}

\begin{posterTcbKey}[][doc new=2017-07-03]{rows}{=\meta{number}}{no default, initially |4|}
  Sets the \meta{number} of rows for a |tcbposter|.
\end{posterTcbKey}


\begin{posterTcbKey}[][doc new=2017-07-03]{colspacing}{=\meta{length}}{no default, initially |4mm|}
  Sets \meta{length} as distance between columns.
\end{posterTcbKey}

\begin{posterTcbKey}[][doc new=2017-07-03]{rowspacing}{=\meta{length}}{no default, initially |4mm|}
  Sets \meta{length} as distance between rows.
\end{posterTcbKey}

\begin{posterTcbKey}[][doc new=2017-07-03]{spacing}{=\meta{length}}{style, no default, initially |4mm|}
  Sets \meta{length} as distance between columns and rows.
\end{posterTcbKey}


\begin{posterTcbKey}[][doc new=2017-07-03]{showframe}{\colOpt{=true\textbar false}}{default |true|, initially |false|}
  Displays a red auxiliary mesh as optical support during poster creation.
  Also, every \refKey{/tcb/posterloc/name} is displayed.
\end{posterTcbKey}


\begin{posterTcbKey}[][doc new=2017-07-03]{width}{=\meta{length}}{no default, initially \cs{linewidth}}
  Sets \meta{length} as width of the poster. For a typical poster, this has not
  to be set manually. Especially, if \refKey{/tcb/posterset/coverage} is present,
  use |coverage={width=|\meta{length}|}| instead to change the overall width.
\end{posterTcbKey}

\enlargethispage*{1cm}

\begin{posterTcbKey}[][doc new=2017-07-03]{height}{=\meta{length}}{no default, initially unset}
  Sets \meta{length} as height of the poster. For a typical poster, this has not
  to be set manually, but is set automatically to an appropriate value.
  If \refKey{/tcb/posterset/coverage} is present, use only one if any option
  |coverage={height=|\meta{length}|}| or |poster={height=|\meta{length}|}|.
\end{posterTcbKey}


\begin{posterTcbKey}[][doc new=2017-07-03]{prefix}{=\meta{name}}{no default, initially |TCBPOSTER@|}
  \meta{name} is set as prefix for any \tikzname\ node which is generated
  automatically by the \mylib{poster} library. This encompasses predefined
  nodes like |top|, |bottom|, \ldots, and nodes defined by using
  \refKey{/tcb/posterloc/name}. Also, see~\Fullref{subsec:poster_environment}.
  For a typical poster, this value can stay as it is.
\end{posterTcbKey}


%--------------------------
\subsection{Coverage}\label{subsec:poster_coverage}

\begin{postersetTcbKey}[][doc new=2017-07-03]{coverage}{=\marg{option list}}{style, no default}
  This option can be applied inside \refEnv{tcbposter} and \refCom{tcbposterset}
  and it adds an optional coverage for the poster which is a surrounding |tcolorbox|
  with the given \meta{option list}. Here, margins and background settings
  for the poster can be given.
  The \emph{coverage} has several default |tcolorbox| settings
  suitable for the purpose:
\begin{dispListing}
enhanced, frame hidden, sharp corners, boxsep=0pt, boxrule=0pt,
top=4mm, bottom=4mm, left=4mm, right=4mm,
toptitle=2mm, bottomtitle=2mm, colback=white
\end{dispListing}

The \meta{option list} can contain any |tcolorbox| option.

\begin{exdispExample}{coverage}
\begin{tcbposter}[
  poster   = {showframe,spacing=1mm},
  coverage = {height=5cm,
              interior style={top color=yellow,bottom color=yellow!50!red},
              watermark text={My Poster},watermark color=white,
             },
]
\end{tcbposter}
\end{exdispExample}

\begin{itemize}
\item For a typical poster, the option \refKey{/tcb/spread} will use the
  whole page for the poster coverage.
\item Poster margins can be adapted by \refKey{/tcb/left}, \refKey{/tcb/right},
  \refKey{/tcb/top}, \refKey{/tcb/bottom}.
\item Poster background can be changed by \refKey{/tcb/colback},
  \refKey{/tcb/interior style}, \refKey{/tcb/interior style image}, etc.
\item Do not use \refKey{/tcb/poster/width} and \refKey{/tcb/poster/height}
  in combination with a \emph{coverage}. Note that you may use
  \refKey{/tcb/width} and \refKey{/tcb/height} inside
  the \emph{coverage} \meta{option list}. Note that this also is not
  necessary when \refKey{/tcb/spread} is applied.
\end{itemize}
\end{postersetTcbKey}


\begin{postersetTcbKey}[][doc new=2017-07-03]{no coverage}{}{style, no value, initially set}
  Removes the surrounding |tcolorbox| completely.
\end{postersetTcbKey}

\clearpage
%--------------------------
\subsection{Common Box Settings}\label{subsec:poster_boxsettings}


\begin{postersetTcbKey}[][doc new=2017-07-03]{boxes}{=\marg{option list}}{style, no default}
  This option can be applied inside \refEnv{tcbposter} and \refCom{tcbposterset}
  and it is used to set up the style of the |tcolorbox|es inside the poster.
  The \meta{option list} can contain any |tcolorbox| option, but box size
  options are not assumed to be useful here, because the size will be
  determined by the placement options.

\begin{exdispExample}{boxes}
\begin{tcbposter}[
  poster   = {spacing=2mm,columns=3,rows=2},
  coverage = {height=5cm,
              interior style={top color=yellow,bottom color=yellow!50!red},
             },
  boxes    = {sharp corners=downhill,arc=3mm,boxrule=1mm,
              colback=white,colframe=cyan,
              title style={left color=black,right color=cyan},
              fonttitle=\bfseries\scshape}
]
  \posterbox[adjusted title=First]{column=1,row=1,span=2}{First box}
  \posterbox[adjusted title=Second]{column=1,row=2,span=2}{Second box}
  \posterbox[adjusted title=Third]{column=3,row=1,rowspan=2}{Third box}
\end{tcbposter}
\end{exdispExample}

\end{postersetTcbKey}


%--------------------------
\subsection{Font Scaling}\label{subsec:poster_fontsize}

\begin{postersetTcbKey}[][doc new=2017-07-03]{fontsize}{=\meta{length}}{style, no default, initially unset}
  This option can be applied inside \refEnv{tcbposter} and \refCom{tcbposterset}.
  It uses \refKey{/tcb/fit basedim} and \refKey{/tcb/fit fontsize macros}
  to redefine |\normalsize| to \meta{length} and all other standard
  font size macros like |\small| and |\large| accordingly.\par
  This needs a freely scalable font family like |lmodern| to work.
  If \refKey{/tcb/posterset/fontsize} is not applied, there standard
  font size macros are not changed in any way.

\begin{dispListing}
\begin{tcbposter}[
  poster   = {spacing=2mm,columns=3,rows=2},
  coverage = {height=5cm,
              interior style={top color=yellow,bottom color=yellow!50!red},
             },
  fontsize = 15pt,   % <--- \normalsize is now 15pt
]
...
\end{dispListing}
\end{postersetTcbKey}


\clearpage
%--------------------------
\subsection{Box Placement}\label{subsec:poster_boxplacement}

\begin{docCommand}[doc new=2017-07-03]{posterbox}{\oarg{options}\marg{placement}\marg{box content}}
  Inside a \refEnv{tcbposter} environment, this places a |tcolorbox| with
  additional |tcolorbox| \meta{options} and the given \meta{box content}
  at a place determined by \meta{placement}.
  All \meta{placement} options are described in the following.
  Note that \meta{box content} cannot contain \emph{verbatim} material,
  see \refEnv{posterboxenv}.
\begin{exdispExample}{posterbox}
\begin{tcbposter}[
  poster = {showframe,height=4cm,spacing=2mm,rows=2},
  boxes  = {beamer,colframe=blue!50!black,colback=blue!50,colupper=yellow!50},
]
\posterbox[title=My title]{name=A,column=2,row=2}{My first box}
\end{tcbposter}
\end{exdispExample}
\end{docCommand}

\begin{docEnvironment}[doc new=2017-07-03]{posterboxenv}{\oarg{options}\marg{placement}}
  This is the environment version of \refCom{posterbox}, i.e.\ inside a
  \refEnv{tcbposter} environment, this places a |tcolorbox| with
  additional |tcolorbox| \meta{options} and the given \meta{environment content}
  at a place determined by \meta{placement}.
  In contrast to \refCom{posterbox}, the \meta{environment content} is
  allowed to contain \emph{verbatim} material. Note that the implementation
  of \refCom{posterbox} is more efficient than the implementation of \refEnv{posterboxenv}.

\enlargethispage*{1cm}
\begin{exdispExample}{posterboxenv}
\begin{tcbposter}[
  poster = {showframe,height=4cm,spacing=2mm,rows=2},
  boxes  = {size=small,beamer,
            colframe=blue!50!black,colback=blue!50,colupper=yellow!50},
]
\begin{posterboxenv}[title=My title]{name=A,column=2,between=top and bottom}
  My first box.
  \begin{tcblisting}{size=small,colback=yellow!10}
My \textbf{first}
poster listing.
  \end{tcblisting}
\end{posterboxenv}
\end{tcbposter}
\end{exdispExample}

\end{docEnvironment}


\clearpage
\begin{posterlocTcbKey}[][doc new=2017-07-03]{name}{=\meta{name}}{no default, initially |@|}
  Sets \meta{name} as reference for the current \refCom{posterbox} or
  \refEnv{posterboxenv}.
  A \tikzname\ shape name is constructed automatically as combination
  of \refKey{/tcb/poster/prefix} and \meta{name}.
\begin{exdispExample}{name}
\begin{tcbposter}[
  poster = {showframe,height=2.5cm,spacing=2mm,rows=2},
  boxes  = {beamer,colframe=blue!50!black,colback=blue!50,colupper=yellow!50},
]
\posterbox{name=A,column=2,row=2}{My first box}
\node[below right=4mm,fill=yellow] (X) at (TCBPOSTER@poster.north west) {Example A};
\draw[blue,very thick,->] (X) |- (TCBPOSTER@A);
\end{tcbposter}
\end{exdispExample}
\end{posterlocTcbKey}


\begin{posterlocTcbKey}[][doc new=2017-07-03]{column}{=\meta{number}}{no default, initially |1|}
  Places the box at the column denoted by \meta{number}. If \refKey{/tcb/posterloc/span}
  is not |1|, the box is aligned to the left side of column \meta{number}.
\begin{exdispExample}{column}
\begin{tcbposter}[
  poster = {showframe,height=2.5cm,spacing=2mm,rows=2},
  boxes  = {beamer,colframe=blue!50!black,colback=blue!50,colupper=yellow!50},
]
\posterbox{row=1,column=2,span=2}{First box}
\posterbox{row=2,column=2,span=0.8}{Second box}
\end{tcbposter}
\end{exdispExample}
\end{posterlocTcbKey}

\enlargethispage*{1cm}
\begin{posterlocTcbKey}[][doc new=2017-07-03]{column*}{=\meta{number}}{no default, initially unset}
  Places the box at the column denoted by \meta{number}. If \refKey{/tcb/posterloc/span}
  is not |1|, the box is aligned to the right side of column \meta{number}.
\begin{exdispExample}{columnstar}
\begin{tcbposter}[
  poster = {showframe,height=2.5cm,spacing=2mm,rows=2},
  boxes  = {beamer,colframe=blue!50!black,colback=blue!50,colupper=yellow!50},
]
\posterbox{row=1,column*=2,span=2}{First box}
\posterbox{row=2,column*=2,span=0.8}{Second box}
\end{tcbposter}
\end{exdispExample}
\end{posterlocTcbKey}


\clearpage
\begin{posterlocTcbKey}[][doc new=2017-07-03]{span}{=\meta{number}}{no default, initially |1|}
  Sets the width of the current box to span \meta{number} columns.
  \meta{number} is also allowed to be a real number like |0.5| or |1.7|.
  See \refKey{/tcb/posterloc/column} and \refKey{/tcb/posterloc/column*}
  for examples.
\end{posterlocTcbKey}

\begin{posterlocTcbKey}[][doc new=2017-07-03]{row}{=\meta{number}}{no default, initially unset}
  If this option is applied, the box is placed at the row denoted by \meta{number}.
  Also, the height is set as fixed according to \refKey{/tcb/posterloc/rowspan}.
\begin{exdispExample}{row}
\begin{tcbposter}[
  poster = {showframe,height=2.5cm,spacing=2mm,rows=2},
  boxes  = {beamer,colframe=blue!50!black,colback=blue!50,colupper=yellow!50},
]
\posterbox{row=1,column=1}{First box}
\posterbox{row=1,column=2,rowspan=2}{Second box}
\posterbox[natural height]{row=1,column=3}{Third box}
\end{tcbposter}
\end{exdispExample}
\end{posterlocTcbKey}

\begin{posterlocTcbKey}[][doc new=2017-07-03]{rowspan}{=\meta{number}}{no default, initially |1|}
  Sets the height of the current box to span \meta{number} rows.
  \meta{number} is also allowed to be a real number like |0.5| or |1.7|.
\begin{exdispExample}{rowspan}
\begin{tcbposter}[
  poster = {showframe,height=2.5cm,spacing=2mm,rows=2},
  boxes  = {beamer,colframe=blue!50!black,colback=blue!50,colupper=yellow!50},
]
\posterbox{row=1,column=1,rowspan=0.9}{First box}
\posterbox{row=1,column=2,rowspan=1.5}{Second box}
\posterbox{row=1,column=3,rowspan=2}{Third box}
\end{tcbposter}
\end{exdispExample}
\end{posterlocTcbKey}

\begin{posterlocTcbKey}[][doc new=2017-07-03]{fixed height}{}{no value, initially |0pt|}
  Sets the height of the current box span rows as denoted by
  \refKey{/tcb/posterloc/rowspan}.
  This can be used, if not \refKey{/tcb/posterloc/row}, but another
  height placement option is applied.
\end{posterlocTcbKey}


\clearpage
\begin{posterlocTcbKey}[][doc new=2017-07-03]{below}{=\meta{name}}{no default, initially |top|}
  The box is placed below another box with the given \meta{name}. Also,
  \meta{name} can be a predefined node, see \Fullref{subsec:poster_environment}.
\begin{exdispExample}{below}
\begin{tcbposter}[
  poster = {showframe,height=3cm,spacing=2mm,rows=2},
  boxes  = {beamer,colframe=blue!50!black,colback=blue!50,colupper=yellow!50},
]
\posterbox{name=A,column=1,below=top}{First box}
\posterbox{name=B,column=1,below=A}{Second box}
\posterbox{name=C,column=2,below=B}{Third box}
\posterbox{name=D,column=3,below=row1}{Fourth box}
\end{tcbposter}
\end{exdispExample}
\end{posterlocTcbKey}


\begin{posterlocTcbKey}[][doc new=2017-07-03]{above}{=\meta{name}}{no default, initially unset}
  The box is placed above another box with the given \meta{name}. Also,
  \meta{name} can be a predefined node, see \Fullref{subsec:poster_environment}.
\begin{exdispExample}{above}
\begin{tcbposter}[
  poster = {showframe,height=3cm,spacing=2mm,rows=2},
  boxes  = {beamer,colframe=blue!50!black,colback=blue!50,colupper=yellow!50},
]
\posterbox{name=A,column=1,above=bottom}{First box}
\posterbox{name=B,column=1,above=A}{Second box}
\posterbox{name=C,column=2,above=B}{Third box}
\posterbox{name=D,column=3,above=row2}{Fourth box}
\end{tcbposter}
\end{exdispExample}
\end{posterlocTcbKey}


\clearpage
\begin{posterlocTcbKey}[][doc new=2017-07-03]{at}{=\meta{name}}{no default, initially unset}
  The box is placed at the position with the given \meta{name}. This is
  quite likely a predefined node, see \Fullref{subsec:poster_environment}.
\begin{exdispExample}{at}
\begin{tcbposter}[
  poster = {showframe,height=3cm,spacing=2mm,rows=2},
  boxes  = {beamer,colframe=blue!50!black,colback=blue!50,colupper=yellow!50},
]
\posterbox{name=A,column=1,at=middle}{First box}
\posterbox{name=B,column=2,at=row1}{Second box}
\end{tcbposter}
\end{exdispExample}
\end{posterlocTcbKey}


\begin{posterlocTcbKey}[][doc new=2017-07-03]{between}{=\meta{name1} and \meta{name2}}{no default, initially unset}
  The box is placed below a box \meta{name1} and above another box \meta{name2}. Also,
  \meta{name1} and \meta{name2} can be predefined nodes, see \Fullref{subsec:poster_environment}.
\begin{exdispExample}{between}
\begin{tcbposter}[
  poster = {showframe,height=3cm,spacing=2mm,rows=2},
  boxes  = {beamer,colframe=blue!50!black,colback=blue!50,colupper=yellow!50},
]
\posterbox{name=A,column=1,below=top}{First box}
\posterbox{name=B,column=1,between=A and bottom}{Second box}
\posterbox{name=C,column=2,above=bottom}{Third box}
\posterbox{name=D,column=2,between=top and C,span=2}{Fourth box}
\posterbox{name=E,column=3,between=D and bottom}{Fifth box}
\end{tcbposter}
\end{exdispExample}
\end{posterlocTcbKey}


\clearpage
\begin{posterlocTcbKey}[][doc new=2017-07-03]{sequence}{=\meta{sequence}}{no default, initially unset}
  The box is broken into partial boxes. These partial boxes are placed
  following the given \meta{sequence} of placements.
  The feasible syntax for the \meta{sequence} is:\par\medskip
  \meta{column a} |between| \meta{name a1} |and| \meta{name a2} |then|\\
  \meta{column b} |between| \meta{name b1} |and| \meta{name b2} |then|\\
  \meta{column c} |between| \meta{name c1} |and| \meta{name c2} |then|\ldots\par\medskip
  Obviously, this places the first part box at \meta{column a} between
  \meta{name a2} and \meta{name a2}. The second box part is placed
  at \meta{column b} between
  \meta{name b2} and \meta{name b2}, and so on.

\begin{exdispExample}{sequence}
\begin{tcbposter}[
  poster = {showframe,height=6cm,spacing=2mm,rows=2},
  boxes  = {beamer,colframe=blue!50!black,colback=blue!50,colupper=yellow!50},
]
\posterbox[adjusted title=A]{name=A,column=1,below=top,span=2}{First box}
\posterbox{name=B,column=2,above=bottom,span=2}{Second box}
\posterbox[adjusted title=C,colframe=red!50!black,colback=red!50]{
  name=C, sequence=1 between A and bottom then
                   2 between A and B then
                   3 between top and B
  }{\lipsum[2]}
\end{tcbposter}
\end{exdispExample}
\end{posterlocTcbKey}

\clearpage

\begin{docTcbKey}[][doc new=2017-07-03]{placeholder}{}{style, no value}
  If the box content of a \refKey{/tcb/posterloc/sequence} is too short
  to fill all reserved box parts, the empty boxes are drawn with
  the \refKey{/tcb/placeholder} style. This style can be redefined, e.g.
  to \refKey{/tcb/blankest}, if nothing should be drawn for empty boxes.
\begin{exdispExample}{placeholder}
\begin{tcbposter}[
  poster = {showframe,height=2.5cm,spacing=2mm,rows=2},
  boxes  = {beamer,colframe=blue!50!black,colback=blue!50,colupper=yellow!50},
]
\posterbox{name=A,column=1,below=top,span=2}{First box}
\posterbox[colframe=red!50!black,colback=red!50]{
  name=B, sequence=1 between A and bottom then
                   2 between A and bottom then
                   3 between top and bottom
  }{Second box followed by placeholder boxes}
\end{tcbposter}
\end{exdispExample}
\end{docTcbKey}



\begin{posterlocTcbKey}[][doc new=2017-07-03]{xshift}{=\meta{length}}{no default, initially |0pt|}
  Horizontal shift of a box by \meta{length}.
\begin{exdispExample}{xshift}
\begin{tcbposter}[
  poster = {showframe,height=3cm,spacing=2mm,rows=2},
  boxes  = {beamer,colframe=blue!50!black,colback=blue!50,colupper=yellow!50},
]
\posterbox{name=A,column=1,row=1,xshift=6mm}{First box}
\posterbox{name=B,column=2,row=2,xshift=-6mm}{Second box}
\end{tcbposter}
\end{exdispExample}
\end{posterlocTcbKey}

\clearpage

\begin{posterlocTcbKey}[][doc new=2017-07-03]{yshift}{=\meta{length}}{no default, initially |0pt|}
  Vertical shift of a box by \meta{length}.
\begin{exdispExample}{yshift}
\begin{tcbposter}[
  poster = {showframe,height=3cm,spacing=2mm,rows=2},
  boxes  = {beamer,colframe=blue!50!black,colback=blue!50,colupper=yellow!50},
]
\posterbox{name=A,column=1,row=1,yshift=-4mm}{First box}
\posterbox{name=B,column=2,row=2,yshift=4mm}{Second box}
\end{tcbposter}
\end{exdispExample}
\end{posterlocTcbKey}



==> tcolorbox.doc.recording.tex <==
% !TeX root = tcolorbox.tex
% include file of tcolorbox.tex (manual of the LaTeX package tcolorbox)
\clearpage
\section{Recording}\label{sec:recording}%
\tcbset{external/prefix=external/recording_}%
The package provides some macros and options to take \emph{records} during
compilation. This is done by \LaTeX\ file operations to save some data
to a file for later usage. The main application scenario is depicted in
\Vref{sec:recording-exercises} where
information about example solutions is recorded and read again
in \Vref{sec:recording-solutions}.

\subsection{Macros}\label{sec:recording-makros}
\begin{docCommand}[doc new=2014-11-28]{tcbstartrecording}{\oarg{file name}}
  Opens a file denoted by \meta{file name} for writing the records.
  The default file name is |\jobname.records|.
  See \Vref{sec:recording-exercises} for an example application.
  \begin{marker}
  In some situations, a not existing optional parameter may cause parsing
  problems. If this happens (or just for precaution), use
\begin{dispListing}
\tcbstartrecording\relax
\end{dispListing}
  or
\begin{dispListing}
\tcbstartrecording[\jobname.records]
\end{dispListing}
  \end{marker}
\end{docCommand}

\begin{docCommand}[doc new=2014-11-28]{tcbrecord}{\marg{content}}
  Records any \meta{content} to the record file.
  \refCom{tcbrecord} is implemented as |\immediate\write|.
  \refCom{tcbstartrecording} has to be called before; otherwise, \refCom{tcbrecord}
  is silently ignored.
\begin{dispListing}
\tcbrecord{\string\solution{\thetcbcounter}{solutions/exercise-\thetcbcounter.tex}}
\end{dispListing}
\end{docCommand}

\begin{docCommand}[doc new=2014-11-28]{tcbstoprecording}{}
  Closes the current record file which was opened by \refCom{tcbstartrecording}
  before.
\end{docCommand}

\begin{docCommand}[doc new=2014-11-28]{tcbinputrecords}{\oarg{file name}}
  Opens a file denoted by \meta{file name} for reading the records via |\input|.
  The default file name is the name of the last used record file for saving.
  \refCom{tcbstoprecording} has to be called before.
\end{docCommand}


\subsection{Options}\label{sec:recording-options}
\begin{docTcbKey}[][doc new=2014-11-28]{record}{=\meta{content}}{style, no default}
  Records any \meta{content} to the record file, see \refCom{tcbrecord}.
  This key can be used several times to write several lines.
  \begin{dispListing}
  record={\string\solution{\thetcbcounter}{solutions/exercise-\thetcbcounter.tex}}
  \end{dispListing}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-11-28]{no recording}{}{}
  Disables \refCom{tcbrecord} and \refKey{/tcb/record} inside the current
  group.
\end{docTcbKey}


\clearpage
\subsection{Example: Exercises}\label{sec:recording-exercises}
The following application example creates exercises and their corresponding
solutions. Each pair is generated inside a single |tcolorbox| where the
solution is given below \refCom{tcblower}. For every example, the solution part
is saved by \refKey{/tcb/savelowerto} to a file. The saving is recorded using
\refKey{/tcb/record}. To enlighten the possibilities, the second exercise
has no solution. Finally, the solutions are input in \Vref{sec:recording-solutions}.

\inputpreamblelisting{L}

\begin{dispListing*}{breakable,before upper=}
\tcbstartrecording\relax

\begin{exercise}
  Compute the derivative of the following function:
  \begin{equation*}
    f(x)=\sin((\sin x)^2)
  \end{equation*}
\tcblower
  The derivative is:
  \begin{align*}
    f'(x) &= \left( \sin((\sin x)^2) \right)'
    =\cos((\sin x)^2) 2\sin x \cos x.
  \end{align*}
\end{exercise}

\begin{exercise}[no solution]
  It holds:
  \begin{equation*}
    \frac{d}{dx}\left(\ln|x|\right) = \frac{1}{x}.
  \end{equation*}
\end{exercise}

\begin{exercise}
  Compute the derivative of the following function:
  \begin{equation*}
    f(x)=(\sin(\sin x))^2
  \end{equation*}
\tcblower
  The derivative is:
  \begin{align*}
    f'(x) &= \left( (\sin(\sin x))^2 \right)'
    =2\sin(\sin x)\cos(\sin x)\cos x.
  \end{align*}
\end{exercise}

\begin{exercise}
  Compute the derivative of the following function:
  \begin{equation*}
    f(x)=\sqrt{x^3-6x^2+2x}
  \end{equation*}
\tcblower
  The derivative is:
  \begin{align*}
    f'(x) &= \left( \sqrt{x^3-6x^2+2x} \right)'
    = \frac{3x^2-12x+2}{2\sqrt{x^3-6x^2+2x}}.
  \end{align*}
\end{exercise}

\begin{exercise}
  Compute the derivative of the following function:
  \begin{equation*}
    f(x)=\left(\frac{2+3x}{1-2x}\right)^3
  \end{equation*}
\tcblower
  The derivative is:
  \begin{align*}
    f'(x) &= \left( \left(\frac{2+3x}{1-2x}\right)^3 \right)'
    = 3 \left(\frac{2+3x}{1-2x}\right)^2 \frac{(1-2x)3-(2+3x)(-2)}{(1-2x)^2}
    = \frac{21(2+3x)^2}{(1-2x)^4}.
  \end{align*}
\end{exercise}

\begin{exercise}
  Compute the derivative of the following function:
  \begin{equation*}
    f(x)=\frac{\cos x}{(\tan 2x)^2}
  \end{equation*}
\tcblower
  The derivative is:
  \begin{align*}
    f'(x) &= \left( \frac{\cos x}{(\tan 2x)^2} \right)'
    = \left( \frac{\cos x (\cos 2x)^2}{(\sin 2x)^2} \right)'\\
    &= \frac{(\sin 2x)^2 [(-\sin x)(\cos 2x)^2+(\cos x)4\cos 2x (-\sin 2x)]
       - \cos x (\cos 2x)^2 4\sin 2x \cos 2x}{(\sin 2x)^4}\\
    &= -\frac{\cos(2x) [\sin x \sin 2x \cos 2x+ 4\cos x(\sin 2x)^2
       + 4 \cos x (\cos 2x)^2]}{(\sin 2x)^3}\\
    &= -\frac{\cos(2x) [\sin x \sin 2x \cos 2x+ 4\cos x]}{(\sin 2x)^3}.
  \end{align*}
\end{exercise}

\begin{exercise}
  Compute the derivative of the following function:
  \begin{equation*}
    f(x)=\cos((2x^2+3)^3)
  \end{equation*}
\tcblower
  The derivative is:
  \begin{align*}
    f'(x) &= \left( \cos((2x^2+3)^3) \right)'
    =-\sin((2x^2+3)^3) 3(2x^2+3)^2 2\cdot 2x\\
    &=-12x(2x^2+3)^2\sin((2x^2+3)^3).
  \end{align*}
\end{exercise}

\begin{exercise}
  Compute the derivative of the following function:
  \begin{equation*}
    f(x)=(x^2+1)\sqrt{x^4+1}
  \end{equation*}
\tcblower
  The derivative is:
  \begin{align*}
    f'(x) &= \left( (x^2+1)\sqrt{x^4+1} \right)'
    = 2x\sqrt{x^4+1} + \frac{2x^3(x^2+1)}{\sqrt{x^4+1}}.
  \end{align*}
\end{exercise}

\tcbstoprecording
\end{dispListing*}
\tcbusetemp

\subsection{Example: Solutions}\label{sec:recording-solutions}
This concludes the example given in \Vref{sec:recording-exercises}.
Now, the saved and recorded solutions are included.

\begin{dispListing*}{breakable,before upper=}
\tcbinputrecords
\end{dispListing*}
\tcbusetemp


==> tcolorbox.doc.skins.tex <==
% !TeX root = tcolorbox.tex
% include file of tcolorbox.tex (manual of the LaTeX package tcolorbox)
\clearpage
\section{Library \mylib{skins}}\label{sec:skins}%
\tcbset{external/prefix=external/skins_}%
The library is loaded by a package option or inside the preamble by:
\begin{dispListing}
\tcbuselibrary{skins}
\end{dispListing}
This also loads the package |tikz| \cite{tantau:tikz_and_pgf}. Typically but not necessarily,
the following skins use |tikz| instead of |pgf|.

\subsection{Style Option Keys}\label{subsec:addstyleoptions}
The following style options are applicable for all skins which
use engines of type |path|, |pathfirst|, |pathmiddle|, or |pathlast|.
Especially, the skin \refSkin{enhanced} supports \emph{all} of them
and \refSkin{standard} \emph{none}.

\begin{docTcbKey}{frame style}{=\meta{\texttt{\upshape tikz} keys}}{style, no default}
  The \meta{\texttt{\upshape tikz} keys} are used inside the |tikz| path command
  for drawing the \emph{frame} of the box.\\
  This option is available if the \refKey{/tcb/frame engine} is set to
  |path|, |pathfirst|, |pathmiddle|, or |pathlast|.
  It is \emph{not} available for |standard|.
\begin{exdispExample*}{frame_style}{sbs,lefthand ratio=0.66}
\tcbset{colback=red!5!white,fonttitle=\bfseries}

\begin{tcolorbox}[enhanced,title=My title,
  frame style={left color=red!75!black,
               right color=blue!75!black}]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{frame style image}{=\meta{file name}}{no default, initially unset}
  Fills the frame with an external image referenced by \meta{file name}.
  For advanced features like blending of a picture with the background,
  use \refKey{/tcb/frame style} together with \refKey{/tikz/fill stretch image}.
\begin{exdispExample*}{frame_style_image}{sbs,lefthand ratio=0.66}
\tcbset{colback=red!5!white,fonttitle=\bfseries}

\begin{tcolorbox}[enhanced,title=My title,
  frame style image=blueshade.png]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{frame style tile}{=\marg{graphics options}\marg{file name}}{no default, initially unset}
  Fills the frame with a tile pattern based on an external image referenced by \meta{file name}.
  The \meta{graphics options} are given to the underlying \docAuxCommand*{includegraphics} command.
  For advanced features like blending of a picture with the background,
  use \refKey{/tcb/frame style} together with \refKey{/tikz/fill tile image}.
\begin{exdispExample*}{frame_style_tile}{sbs,lefthand ratio=0.66}
\tcbset{colback=red!5!white,coltitle=red!30!black,
  opacityback=0.75,fonttitle=\bfseries}

\begin{tcolorbox}[enhanced,title=My title,
  frame style tile={width=1cm}{pink_marble.png}]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{frame hidden}{}{style, no value}
  This is a shortcut for |frame style={draw=none,fill=none}|.
  Depending on the skin, this option switches off the drawing of the
  frame.
  Alternatively, use \refKey{/tcb/frame empty}.
\begin{exdispExample*}{frame_hidden}{sbs,lefthand ratio=0.66}
\tcbset{colback=red!5!white,colframe=red!75!black,
  fonttitle=\bfseries,coltitle=black}

\begin{tcolorbox}[enhanced,title=My title,
  frame hidden]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{interior style}{=\meta{\texttt{\upshape tikz} keys}}{style, no default}
  The \meta{\texttt{\upshape tikz} keys} are used inside the |tikz| path command
  for drawing the \emph{interior} of the box. They are used for the titled
  and for the untitled version as well.\\
  This option is available if the \refKey{/tcb/interior titled engine}
  or \refKey{/tcb/interior engine} is set to
  |path|, |pathfirst|, |pathmiddle|, or |pathlast|.
  It is \emph{not} available for |standard|.
\begin{exdispExample*}{interior_style}{sbs,lefthand ratio=0.66}
\tcbset{colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[enhanced,title=My title,
  interior style={left color=red!20!white,
                  right color=yellow!50!white}]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{interior style image}{=\meta{file name}}{no default, initially unset}
  Fills the interior with an external image referenced by \meta{file name}.
  For advanced features like blending of a picture with the background,
  use \refKey{/tcb/interior style} together with \refKey{/tikz/fill stretch image}.
\begin{exdispExample*}{interior_style_image}{sbs,lefthand ratio=0.66}
\tcbset{colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[enhanced,title=My title,
  interior style image=goldshade.png]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{interior style tile}{=\marg{graphics options}\marg{file name}}{no default, initially unset}
  Fills the interior with a tile pattern based on an external image referenced by \meta{file name}.
  The \meta{graphics options} are given to the underlying \docAuxCommand*{includegraphics} command.
  For advanced features like blending of a picture with the background,
  use \refKey{/tcb/interior style} together with \refKey{/tikz/fill tile image}.

\begin{exdispExample*}{interior_style_tile}{sbs,lefthand ratio=0.66}
\tcbset{colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[enhanced,title=My title,
  interior style tile={width=2cm}{crinklepaper.png}]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{interior hidden}{}{style, no value}
  This is a shortcut for |interior style={draw=none,fill=none}|.
  Depending on the skin, this option switches off the drawing of the
  interior.
  Alternatively, use \refKey{/tcb/interior empty} and/or \refKey{/tcb/interior titled empty}.
\begin{exdispExample*}{interior_hidden}{sbs,lefthand ratio=0.66}
\tcbset{frame style={top color=red!20!white,
  bottom color=red!20!white!75!black},
  fonttitle=\bfseries,coltitle=black}

\begin{tcolorbox}[enhanced,title=My title,
  interior hidden]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{segmentation style}{=\meta{\texttt{\upshape tikz} keys}}{style, no default}
  The \meta{\texttt{\upshape tikz} keys} are used inside the |tikz| path command
  for drawing the \emph{segmentation} line of the box.\\
  This option is available if the \refKey{/tcb/segmentation engine}
  is set to |path|.
  It is \emph{not} available for |standard|.
\begin{exdispExample*}{segmentation_style}{sbs,lefthand ratio=0.66}
\tcbset{colback=red!5!white,colframe=red!75!black,
  fonttitle=\bfseries}

\begin{tcolorbox}[enhanced,title=My title,
  segmentation style={double=white,draw=blue,
                  double distance=1pt,solid}]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{segmentation hidden}{}{style, no value}
  This is a shortcut for |segmentation style={draw=none,fill=none}|.
  Depending on the skin, this option switches off the drawing of the
  segmentation line. See also \refKey{/tcb/lower separated} which
  has the same effect for most skins.
  Alternatively, use \refKey{/tcb/segmentation empty}.
\begin{exdispExample*}{segmentation_hidden}{sbs,lefthand ratio=0.66}
\tcbset{colback=red!5!white,colframe=red!75!black,
  fonttitle=\bfseries}

\begin{tcolorbox}[title=My title,
  enhanced,segmentation hidden]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{title style}{=\meta{\texttt{\upshape tikz} keys}}{style, no default}
  The \meta{\texttt{\upshape tikz} keys} are used inside the |tikz| path command
  for drawing the \emph{title area} of the box.\\
  This option is available if the \refKey{/tcb/title engine} is set to
  |path|, |pathfirst|, |pathmiddle|, or |pathlast|.
  It is \emph{not} available for |standard|.
\begin{exdispExample*}{title_style}{sbs,lefthand ratio=0.66}
\tcbset{colback=red!5!white,colframe=red!75!black,
  coltitle=blue!50!black,fonttitle=\bfseries}

\begin{tcolorbox}[enhanced,title=My title,
  title style={left color=blue!15!yellow,
               right color=red!85!black}]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{title style image}{=\meta{file name}}{no default, initially unset}
  Fills the title area with an external image referenced by \meta{file name}.
  For advanced features like blending of a picture with the background,
  use \refKey{/tcb/title style} together with \refKey{/tikz/fill stretch image}.

\begin{exdispExample*}{title_style_image}{sbs,lefthand ratio=0.66}
\tcbset{colback=blue!5!white,colframe=blue!75!black,
  fonttitle=\bfseries}

\begin{tcolorbox}[enhanced,title=My title,
  title style image=blueshade.png]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{title style tile}{=\marg{graphics options}\marg{file name}}{no default, initially unset}
  Fills the title area with a tile pattern based on an external image referenced by \meta{file name}.
  The \meta{graphics options} are given to the underlying \docAuxCommand*{includegraphics} command.
  For advanced features like blending of a picture with the background,
  use \refKey{/tcb/title style} together with \refKey{/tikz/fill tile image}.

\begin{exdispExample*}{title_style_tile}{sbs,lefthand ratio=0.66}
\tcbset{colback=red!5!white,colframe=red!75!black,
  coltitle=blue!50!black,fonttitle=\bfseries}

\begin{tcolorbox}[enhanced,title=My title,
  title style tile={width=1cm}{pink_marble.png}]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{title hidden}{}{style, no value}
  This is a shortcut for |title style={draw=none,fill=none}|.
  Depending on the skin, this option switches off the drawing of the
  title background. See also \refKey{/tcb/title filled} for a similar effect.
  Alternatively, use \refKey{/tcb/title empty}.
\begin{exdispExample*}{title_hidden}{sbs,lefthand ratio=0.66}
\tcbset{colback=red!5!white,colframe=red!75!black,
  fonttitle=\bfseries}

\begin{tcolorbox}[title=My title,
  enhanced,title hidden]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\clearpage


\begin{docTcbKey}[][doc new=2015-01-14]{titlerule style}{=\meta{\texttt{\upshape tikz} keys}}{style, no default}
  The \meta{\texttt{\upshape tikz} keys} are used to draw a title rule,
  i.e.\ a rule below the optional title. The width of the rule is controlled
  by \refKey{/tcb/titlerule}. It may be set directly to a smaller width
  to create mixed effects with the standard rule.
  This option is implemented as an \refKey{/tcb/underlay}. Thus, it is not
  available for \refSkin{standard} and \refSkin{standard jigsaw}, but for
  all other skins, e.g.\ \refSkin{enhanced}.
  As an underlay, this option can be used multiple times and is removed
  by \refKey{/tcb/no underlay}.
\begin{exdispExample*}{titlerule_style_1}{sbs,lefthand ratio=0.66}
\begin{tcolorbox}[enhanced,
  colback=red!5!white,colframe=red!75!black,
  colbacktitle=red!50!yellow,fonttitle=\bfseries,
  title=My title,
  titlerule=1mm,
  titlerule style=yellow  ]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}

\begin{exdispExample*}{titlerule_style_2}{sbs,lefthand ratio=0.66}
\begin{tcolorbox}[enhanced,
  colback=red!5!white,colframe=red!75!black,
  colbacktitle=red!50!yellow,fonttitle=\bfseries,
  title=My title,
  titlerule=1mm,
  titlerule style={yellow,line width=0.5mm}  ]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}

\begin{exdispExample*}{titlerule_style_3}{sbs,lefthand ratio=0.66}
\begin{tcolorbox}[enhanced,
  colback=red!10!white,colframe=red!75!black,
  colbacktitle=red!50!yellow,fonttitle=\bfseries,
  frame hidden,
  title=My title,
  boxrule=0pt,titlerule=1mm,
  titlerule style=red!50!black  ]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}

\begin{exdispExample*}{titlerule_style_4}{sbs,lefthand ratio=0.66}
%\usetikzlibrary{arrows.meta}
\begin{tcolorbox}[empty,
  coltitle=red!75!black,fonttitle=\bfseries,
  borderline horizontal={0.5mm}{0pt}{red!50!white},
  title=My title,
  titlerule style={red,
    arrows = {Hooks[arc=270]-Hooks[arc=270]}} ]
This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\clearpage

The combined \tikzname\ style applied to frame, interior, and title
background can used by authors in customizing code.

\begin{docTikzKey}{tcb fill frame}{}{style, no value}
This is a \tikzname\ style which is finally applied to the \emph{frame}
of the box.

\begin{exdispExample*}{tcb_fill_frame}{sbs,lefthand ratio=0.66}
% \tcbuselibrary{hooks}
\tcbset{enhanced,colback=red!5!white,
  colframe=red!75!black,fonttitle=\bfseries,
  frame code app={\path[tcb fill frame]
    ([yshift=-2mm]frame.north)
        circle (8mm); }  }

\begin{tcolorbox}[title=My title]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTikzKey}


\begin{docTikzKey}{tcb fill interior}{}{style, no value}
This is a \tikzname\ style which is finally applied to the \emph{interior}
of the box.

\begin{exdispExample*}{tcb_fill_interior}{sbs,lefthand ratio=0.66}
% \tcbuselibrary{hooks}
\tcbset{enhanced,colback=red!5!white,
  colframe=red!75!black,fonttitle=\bfseries,
  interior titled code app={\path[tcb fill interior]
      ([yshift=-0.1pt]interior.north east)
    --([yshift=3pt]interior.north)
    --([yshift=-0.1pt]interior.north west)
    --cycle;}  }

\begin{tcolorbox}[title=My title]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTikzKey}


\begin{docTikzKey}{tcb fill title}{}{style, no value}
This is a \tikzname\ style which is finally applied to the \emph{title area}
of the box.

\begin{exdispExample*}{tcb_fill_title}{sbs,lefthand ratio=0.66}
% \tcbuselibrary{hooks}
\tcbset{enhanced,colback=red!5!white,
  colframe=red!75!black,fonttitle=\bfseries,
  colbacktitle=blue!75!black,
  title code app={\path[tcb fill title]
    (title) circle (5mm); }  }

\begin{tcolorbox}[title=My title]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{exdispExample*}
\end{docTikzKey}


\clearpage
\subsection{Boxed Title Option Keys}\label{subsec:skinboxedtitle}

\subsubsection{Boxed Title Placement}
The following options place the title text into an own \refCom{tcbox}.
This boxed title can be customized independently from the main box using
\refKey{/tcb/boxed title style}.
The placement can be influenced by \meta{boxtitle options}.

\begin{docTcbKey}{attach boxed title to top left}{\colOpt{=\marg{boxtitle options}}}{style, default empty}
The title is boxed with a \refCom{tcbox} and attached to
the top left corner of the main box.
\begin{exdispExample*}{attach_boxed_title_to_top_left}{sbs,lefthand ratio=0.66}
\begin{tcolorbox}[enhanced,title=My title,
  attach boxed title to top left]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\begin{docTcbKey}{attach boxed title to top center}{\colOpt{=\marg{boxtitle options}}}{style, default empty}
The title is boxed with a \refCom{tcbox} and attached to
the top of the main box.
\begin{exdispExample*}{attach_boxed_title_to_top_center}{sbs,lefthand ratio=0.66}
\begin{tcolorbox}[enhanced,title=My title,
  attach boxed title to top center]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\begin{docTcbKey}{attach boxed title to top right}{\colOpt{=\marg{boxtitle options}}}{style, default empty}
The title is boxed with a \refCom{tcbox} and attached to
the top right corner of the main box.
\begin{exdispExample*}{attach_boxed_title_to_top_right}{sbs,lefthand ratio=0.66}
\begin{tcolorbox}[enhanced,title=My title,
  attach boxed title to top right]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\begin{docTcbKey}{attach boxed title to bottom left}{\colOpt{=\marg{boxtitle options}}}{style, default empty}
The title is boxed with a \refCom{tcbox} and attached to
the bottom left corner of the main box.
\begin{exdispExample*}{attach_boxed_title_to_bottom_left}{sbs,lefthand ratio=0.66}
\begin{tcolorbox}[enhanced,title=My title,
  attach boxed title to bottom left]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\begin{docTcbKey}{attach boxed title to bottom center}{\colOpt{=\marg{boxtitle options}}}{style, default empty}
The title is boxed with a \refCom{tcbox} and attached to
the bottom of the main box.
\begin{exdispExample*}{attach_boxed_title_to_bottom_center}{sbs,lefthand ratio=0.66}
\begin{tcolorbox}[enhanced,title=My title,
  attach boxed title to bottom center]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}

\begin{docTcbKey}{attach boxed title to bottom right}{\colOpt{=\marg{boxtitle options}}}{style, default empty}
The title is boxed with a \refCom{tcbox} and attached to
the bottom right corner of the main box.
\begin{exdispExample*}{attach_boxed_title_to_bottom_right}{sbs,lefthand ratio=0.66}
\begin{tcolorbox}[enhanced,title=My title,
  attach boxed title to bottom right]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{docTcbKey}


\clearpage
\begin{docTcbKey}[][doc new=2016-02-26]{attach boxed title to top}{\colOpt{=\marg{boxtitle options}}}{style, default empty}
  This is a convenient style to mimic a standard title.
  It uses \refKey{/tcb/attach boxed title to top center},
  \refKey{/tcb/minipage boxed title}, and sizes the boxed title to match
  the base box.
\begin{dispExample*}{sbs,lefthand ratio=0.66}
\begin{tcolorbox}[enhanced,title=My title,
  attach boxed title to top,
  boxed title style={colframe=red}]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2016-02-26]{attach boxed title to top*}{\colOpt{=\marg{boxtitle options}}}{style, default empty}
  In contrast to \refKey{/tcb/attach boxed title to top}, this style
  uses smaller left and right rules to avoid previewer glitches.
  Typically, one would not use different colors for the frame as in the
  example below.
\begin{dispExample*}{sbs,lefthand ratio=0.66}
\begin{tcolorbox}[enhanced,title=My title,
  attach boxed title to top*,
  boxed title style={colframe=red}]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2016-02-26]{attach boxed title to bottom}{\colOpt{=\marg{boxtitle options}}}{style, default empty}
  This is a convenient style to produce a standard-like title at the bottom
  of the box.
  It uses \refKey{/tcb/attach boxed title to bottom center},
  \refKey{/tcb/minipage boxed title}, and sizes the boxed title to match
  the base box.
\begin{dispExample*}{sbs,lefthand ratio=0.66}
\begin{tcolorbox}[enhanced,title=My title,
  attach boxed title to bottom,
  boxed title style={colframe=red}]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2016-02-26]{attach boxed title to bottom*}{\colOpt{=\marg{boxtitle options}}}{style, default empty}
  In contrast to \refKey{/tcb/attach boxed title to top}, this style
  uses smaller left and right rules to avoid previewer glitches.
\begin{dispExample*}{sbs,lefthand ratio=0.66}
\begin{tcolorbox}[enhanced,title=My title,
  attach boxed title to bottom*]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2016-02-26]{flip title}{\colOpt{=\marg{options}}}{style, default empty}
  This style combines \refKey{/tcb/attach boxed title to bottom*}
  with \refKey{/tcb/boxed title style}. The \meta{options} are given to
  \refKey{/tcb/boxed title style}.
\begin{dispExample*}{sbs,lefthand ratio=0.66}
\begin{tcolorbox}[tile,flip title={sharp corners},
  title=My title,colback=red!10,
  colbacktitle=red!75!black]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}

\clearpage

\subsubsection{Options for the Boxed Title Placement}
The \meta{boxtitle options} of the keys described above are shift values.
The dimensions of the boxed title are stored into two macros
\docAuxCommand{tcboxedtitleheight} and
\docAuxCommand{tcboxedtitlewidth}. These macros can be used inside the
following \meta{boxtitle options}:

\begin{boxTcbKey}{xshift}{=\meta{length}}{no default, initially |0pt|}
The boxed title is shifted by \meta{length} in the horizontal direction.
\begin{exdispExample*}{xshift}{sbs,lefthand ratio=0.66}
\begin{tcolorbox}[enhanced,title=My title,
  attach boxed title to top left={xshift=-2mm},
  boxed title style={size=small,colback=blue}]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{boxTcbKey}

\begin{boxTcbKey}{yshift}{=\meta{length}}{no default, initially |0pt|}
The boxed title is shifted by \meta{length} in the vertical direction.
\begin{exdispExample*}{yshift}{sbs,lefthand ratio=0.66}
\begin{tcolorbox}[enhanced,title=My title,
  attach boxed title to top center=
    {yshift=-\tcboxedtitleheight/2},
  boxed title style={size=small,colback=blue}]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{boxTcbKey}

\begin{boxTcbKey}{yshifttext}{=\meta{length}}{no default, initially |0pt|}
The text inside the main box is shifted by \meta{length} to give room for e.\,g.\ a sunken title.
\begin{exdispExample*}{yshifttext}{sbs,lefthand ratio=0.66}
\begin{tcolorbox}[enhanced,title=My title,
  attach boxed title to top center=
    {yshift=-3mm,yshifttext=-1mm},
  boxed title style={size=small,colback=blue}]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{boxTcbKey}

\begin{boxTcbKey}{yshift*}{=\meta{length}}{no default, initially |0pt|}
Sets \refKey{/tcb/boxtitle/yshift} and \refKey{/tcb/boxtitle/yshifttext}
the same time.\\
\refKey{/tcb/boxtitle/yshifttext} is only set if necessary.
\begin{exdispExample*}{yshiftstar}{sbs,lefthand ratio=0.66}
\begin{tcolorbox}[enhanced,title=My title,
  attach boxed title to top center={yshift*=-3mm},
  boxed title style={size=small,colback=blue}]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}
\end{boxTcbKey}

\begin{marker}
The bounding box of the resulting total |tcolorbox| is adapted automatically to the
\emph{vertical} dimensions of the boxed title. Possible horizontal enlargements
are \emph{not} automatically computed.
\end{marker}


\begin{exdispExample*}{boxed_title_example_1}{sbs,lefthand ratio=0.66}
\begin{tcolorbox}[enhanced,title=My title,
  attach boxed title to top left=
    {xshift=-2mm,yshift=-2mm},
  boxed title style={size=small,colback=blue},
  show bounding box]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}


\clearpage
\subsubsection{Options for the Boxed Title Box}
\begin{marker}
  The boxed title options are implemented as an underlay, see \Vref{subsec:skinunderlay}.
  Therefore, a boxed title is not drawn, if a skin does not support underlays
  like \refSkin{standard}. Still, the room for the boxed
  titles gets reserved in these cases.
\end{marker}

\begin{marker}
  A \tikzname\ node |title| is produced by a boxed title which can be used
  inside \refKey{/tcb/frame code}, \refKey{/tcb/interior code},
  underlays, overlays, and finishes.
\end{marker}

\begin{marker}
  A boxed title is almost always the first underlay. The only exceptions are
  underlays defined by \refKey{/tcb/underlay boxed title} which are drawn
  before. Additionally, underlays defined by \refKey{/tcb/underlay boxed title}
  are only drawn, if a boxed title is actually set. They are ignored, if
  there is no boxed title.
\end{marker}



\begin{docTcbKey}[][doc new=2016-02-26]{boxed title size}{=\meta{size}}{no default, initially |title|}
  This setting defines the basic size for the title box. Further settings
  can be applied using \refKey{/tcb/boxed title style}.
  Feasible values for \meta{size} are:
  \begin{itemize}
  \item\docValue{title}: Sets the size according to \refKey{/tcb/size}|=|\docValue{title}.
  \item\docValue{standard}: No size setting. Typically, this is identical to
    \refKey{/tcb/size}|=|\docValue{normal}.
  \item\docValue{copy}: The size values for a title of the base box are copied
    for the title box.
  \end{itemize}

\begin{dispExample}
% \tcbuselibrary{raster}
\begin{tcbraster}[raster columns=3,enhanced,boxrule=0.4pt,
    title=My title,attach boxed title to top center]
  \begin{tcolorbox}[boxed title size=title]
    This is a \textbf{tcolorbox}.
  \end{tcolorbox}
  \begin{tcolorbox}[boxed title size=standard]
    This is a \textbf{tcolorbox}.
  \end{tcolorbox}
  \begin{tcolorbox}[boxed title size=copy]
    This is a \textbf{tcolorbox}.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}

\end{docTcbKey}


\clearpage
\begin{docTcbKey}[][doc updated=2016-02-26]{boxed title style}{=\meta{options}}{style, initially empty}
By default, a boxed title is dimensioned with \refKey{/tcb/size}|=|\docValue*{title}
and inherits the \refKey{/tcb/skin} and \refKey{/tcb/colframe} of the main box.
Also, the \refKey{/tcb/colback} is inherited from the main \refKey{/tcb/colbacktitle}.
Font and color of the title text are set as usual.
All other \meta{options} are set by the \refKey{/tcb/boxed title style} key.
Since a boxed title is set by \refCom{tcbox}, all |tcolorbox| options are
applicable here. If \refKey{/tcb/boxed title style} is used several times,
the \meta{options} are is appended.

\begin{exdispExample*}{boxed_title_style_1}{sbs,lefthand ratio=0.66}
\begin{tcolorbox}[enhanced,title=My title,
  fonttitle=\bfseries,coltitle=green!25!black,
  attach boxed title to top center=
    {yshift=-2mm,yshifttext=-1mm},
  boxed title style={colframe=green!75!black,
    colback=yellow!50!green}]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}


\begin{exdispExample*}{boxed_title_style_2}{sbs,lefthand ratio=0.66}
\begin{tcolorbox}[enhanced,title=My title,
  colframe=red!50!black,colback=red!10!white,
  arc=1mm,colbacktitle=red!10!white,
  fonttitle=\bfseries,coltitle=red!50!black,
  attach boxed title to top left=
    {xshift=3.2mm,yshift=-0.50mm},
  boxed title style={skin=enhancedfirst jigsaw,
    size=small,arc=1mm,bottom=-1mm,
    interior style={fill=none,
      top color=red!30!white,
      bottom color=red!20!white}}]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{exdispExample*}

\begin{exdispExample}{boxed_title_style_3}
\begin{tcolorbox}[enhanced,title=My title,
  colframe=blue!50!black,colback=blue!10!white,colbacktitle=blue!5!yellow!10!white,
  fonttitle=\bfseries,coltitle=black,attach boxed title to top center=
    {yshift=-0.25mm-\tcboxedtitleheight/2,yshifttext=2mm-\tcboxedtitleheight/2},
  boxed title style={boxrule=0.5mm,
    frame code={ \path[tcb fill frame] ([xshift=-4mm]frame.west)
    -- (frame.north west) -- (frame.north east) -- ([xshift=4mm]frame.east)
    -- (frame.south east) -- (frame.south west) -- cycle; },
    interior code={ \path[tcb fill interior] ([xshift=-2mm]interior.west)
    -- (interior.north west) -- (interior.north east)
    -- ([xshift=2mm]interior.east) -- (interior.south east) -- (interior.south west)
    -- cycle;}  }]
  \lipsum[2]
\end{tcolorbox}
\end{exdispExample}


\begin{exdispExample}{boxed_title_style_4}
% \usepackage{varwidth}
\newtcolorbox{mybox}[2][]{enhanced,skin=enhancedlast jigsaw,
  attach boxed title to top left={xshift=-4mm,yshift=-0.5mm},
  fonttitle=\bfseries\sffamily,varwidth boxed title=0.7\linewidth,
  colbacktitle=blue!45!white,colframe=red!50!black,
  interior style={top color=blue!10!white,bottom color=red!10!white},
  boxed title style={empty,arc=0pt,outer arc=0pt,boxrule=0pt},
  underlay boxed title={
    \fill[blue!45!white] (title.north west) -- (title.north east)
      -- +(\tcboxedtitleheight-1mm,-\tcboxedtitleheight+1mm)
      -- ([xshift=4mm,yshift=0.5mm]frame.north east) -- +(0mm,-1mm)
      -- (title.south west) -- cycle;
    \fill[blue!45!white!50!black] ([yshift=-0.5mm]frame.north west)
      -- +(-0.4,0) -- +(0,-0.3) -- cycle;
    \fill[blue!45!white!50!black] ([yshift=-0.5mm]frame.north east)
      -- +(0,-0.3) -- +(0.4,0) -- cycle;  },
  title={#2},#1}

\begin{mybox}{My title}
  \lipsum[2]
\end{mybox}
\end{exdispExample}


\begin{exdispExample}{boxed_title_style_5}
% \usepackage{varwidth}
\newtcolorbox{mybox}[2][]{enhanced,
  attach boxed title to top left={xshift=1cm,yshift=-2mm},
  fonttitle=\bfseries,varwidth boxed title=0.7\linewidth,
  colbacktitle=green!45!white,coltitle=green!10!black,colframe=green!50!black,
  interior style={top color=yellow!10!white,bottom color=green!10!white},
  boxed title style={boxrule=0.75mm,colframe=white,
    borderline={0.1mm}{0mm}{green!50!black},
    borderline={0.1mm}{0.75mm}{green!50!black},
    interior style={top color=green!10!white,bottom color=green!10!white,
      middle color=green!50!white},
    drop fuzzy shadow},
  title={#2},#1}

\begin{mybox}{My title}
  \lipsum[2]
\end{mybox}
\end{exdispExample}


\begin{exdispExample}{boxed_title_style_6}
\newtcolorbox{flipbox}[2][]{
  enhanced,colframe=blue!50!black,colback=yellow!5,fonttitle=\bfseries,
  flip title={interior hidden},title={#2},#1}

\begin{flipbox}{My title}
\lipsum[2]
\end{flipbox}
\end{exdispExample}


\begin{exdispExample}{boxed_title_style_7}
% \usepackage{varwidth}
\newtcolorbox{mybox}[2][]{skin=enhancedlast jigsaw,interior hidden,
  boxsep=0pt,top=0pt,colframe=red,coltitle=red!50!black,
  fonttitle=\bfseries\sffamily,
  attach boxed title to bottom center,
  boxed title style={empty,boxrule=0.5mm},
  varwidth boxed title=0.5\linewidth,
  underlay boxed title={
    \draw[white,line width=0.5mm]
      ([xshift=0.3mm-\tcboxedtitleheight*2,yshift=0.3mm]title.north west)
      --([xshift=-0.3mm+\tcboxedtitleheight*2,yshift=0.3mm]title.north east);
    \path[draw=red,top color=white,bottom color=red!50!white,line width=0.5mm]
    ([xshift=0.25mm-\tcboxedtitleheight*2,yshift=0.25mm]title.north west)
    cos +(\tcboxedtitleheight,-\tcboxedtitleheight/2)
    sin +(\tcboxedtitleheight,-\tcboxedtitleheight/2)
    -- ([xshift=0.25mm,yshift=0.25mm]title.south west)
    -- ([yshift=0.25mm]title.south east)
    cos +(\tcboxedtitleheight,\tcboxedtitleheight/2)
    sin +(\tcboxedtitleheight,\tcboxedtitleheight/2); },
  title={#2},#1}

\begin{mybox}{My title}
  \lipsum[2]
\end{mybox}
\end{exdispExample}


\begin{exdispExample}{boxed_title_style_8}
% \usepackage{varwidth}
\newtcolorbox{mybox}[2][]{enhanced,
  before skip=2mm,after skip=2mm,
  colback=black!5,colframe=black!50,boxrule=0.2mm,
  attach boxed title to top left={xshift=1cm,yshift*=1mm-\tcboxedtitleheight},
  varwidth boxed title*=-3cm,
  boxed title style={frame code={
    \path[fill=tcbcolback!30!black]
      ([yshift=-1mm,xshift=-1mm]frame.north west)
        arc[start angle=0,end angle=180,radius=1mm]
      ([yshift=-1mm,xshift=1mm]frame.north east)
        arc[start angle=180,end angle=0,radius=1mm];
    \path[left color=tcbcolback!60!black,right color=tcbcolback!60!black,
      middle color=tcbcolback!80!black]
      ([xshift=-2mm]frame.north west) -- ([xshift=2mm]frame.north east)
      [rounded corners=1mm]-- ([xshift=1mm,yshift=-1mm]frame.north east)
      -- (frame.south east) -- (frame.south west)
      -- ([xshift=-1mm,yshift=-1mm]frame.north west)
      [sharp corners]-- cycle;
    },interior engine=empty,
  },
  fonttitle=\bfseries,
  title={#2},#1}

\begin{mybox}[colbacktitle=green]{My title}
\lipsum[2]
\end{mybox}
\begin{mybox}[colbacktitle=red]{My title}
\lipsum[3]
\end{mybox}
\end{exdispExample}
\end{docTcbKey}



\begin{docTcbKey}[][doc new=2016-02-26]{no boxed title style}{}{style, initially set}
  Removes all options which were set by \refKey{/tcb/boxed title style}.
\end{docTcbKey}


\clearpage
\begin{docTcbKey}{hbox boxed title}{}{no value, initially set}
The title text content is captured with a horizontal box.
Especially, there are no linebreak possible.
\begin{exdispExample*}{hbox_boxed_title}{sbs,lefthand ratio=0.66}
\newtcolorbox{mybox}[1]{hbox boxed title,
  enhanced,attach boxed title to top center=
    {yshift=-3mm,yshifttext=-1mm},
  boxed title style={size=small,colback=red},
  title={#1}}

\begin{mybox}{Short title}
  This is a \textbf{tcolorbox}.
\end{mybox}\bigskip

\begin{mybox}{This title is not really very short}
  This is a \textbf{tcolorbox}.
\end{mybox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{minipage boxed title}{\colOpt{=\meta{length}}}{initially unset}
The title text content is captured with a minipage with a width of \meta{length}.
By default, the resulting boxed title is somewhat smaller than the main box.
\begin{exdispExample*}{minipage_boxed_title}{sbs,lefthand ratio=0.66}
\newtcolorbox{mybox}[1]{minipage boxed title,
  enhanced,attach boxed title to top center=
    {yshift=-3mm,yshifttext=-1mm},
  boxed title style={size=small,colback=red},
  center title,title={#1}}

\begin{mybox}{Short title}
  This is a \textbf{tcolorbox}.
\end{mybox}\bigskip

\begin{mybox}{This title is not really very short}
  This is a \textbf{tcolorbox}.
\end{mybox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{minipage boxed title*}{\colOpt{=\meta{length}}}{initially unset}
The title text content is captured with a minipage with a width of main box width plus \meta{length}.
By default, the resulting boxed title is somewhat smaller than the main box.
\begin{exdispExample*}{minipage_boxed_title_star}{sbs,lefthand ratio=0.66}
\newtcolorbox{mybox}[1]{minipage boxed title*=-2cm,
  enhanced,attach boxed title to top center=
    {yshift=-3mm,yshifttext=-1mm},
  boxed title style={size=small,colback=red},
  center title,title={#1}}

\begin{mybox}{Short title}
  This is a \textbf{tcolorbox}.
\end{mybox}\bigskip

\begin{mybox}{This title is not really very short}
  This is a \textbf{tcolorbox}.
\end{mybox}
\end{exdispExample*}
\end{docTcbKey}


\clearpage
\begin{docTcbKey}{tikznode boxed title}{=\meta{options}}{initially unset}
The title text content is captured with a \tikzname\ node with given \tikzname\ \meta{options}.
The text is centered by default
\begin{exdispExample*}{tikznode_boxed_title}{sbs,lefthand ratio=0.66}
\newtcolorbox{mybox}[1]{tikznode boxed title,
  enhanced,attach boxed title to top center=
    {yshift=-3mm,yshifttext=-1mm},
  boxed title style={size=small,colback=red},
  title={#1}}

\begin{mybox}{Short title}
  This is a \textbf{tcolorbox}.
\end{mybox}\bigskip

\begin{mybox}{This title\\is not really\\very short}
  This is a \textbf{tcolorbox}.
\end{mybox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{varwidth boxed title}{\colOpt{=\meta{length}}}{initially unset}
The title text content is captured with a |varwidth| environment with a width of \meta{length}.
This style needs the |varwidth| package \cite{arseneau:2011a} to be loaded manually.
By default, the resulting boxed title is somewhat smaller than the main box.
\begin{exdispExample*}{varwidth_boxed_title}{sbs,lefthand ratio=0.66}
% \usepackage{varwidth}
\newtcolorbox{mybox}[1]{varwidth boxed title,
  enhanced,attach boxed title to top center=
    {yshift=-3mm,yshifttext=-1mm},
  boxed title style={size=small,colback=red},
  center title,title={#1}}

\begin{mybox}{Short title}
  This is a \textbf{tcolorbox}.
\end{mybox}\bigskip

\begin{mybox}{This title is not really very short}
  This is a \textbf{tcolorbox}.
\end{mybox}
\end{exdispExample*}
\end{docTcbKey}


\begin{docTcbKey}{varwidth boxed title*}{\colOpt{=\meta{length}}}{initially unset}
The title text content is captured with a |varwidth| environment with a width of main box width plus \meta{length}.
This style needs the |varwidth| package \cite{arseneau:2011a} to be loaded manually.
By default, the resulting boxed title is somewhat smaller than the main box.
\begin{exdispExample*}{varwidth_boxed_title_star}{sbs,lefthand ratio=0.66}
% \usepackage{varwidth}
\newtcolorbox{mybox}[1]{varwidth boxed title*=-2cm,
  enhanced,attach boxed title to top center=
    {yshift=-3mm,yshifttext=-1mm},
  boxed title style={size=small,colback=red},
  center title,title={#1}}

\begin{mybox}{Short title}
  This is a \textbf{tcolorbox}.
\end{mybox}\bigskip

\begin{mybox}{This title is not really very short}
  This is a \textbf{tcolorbox}.
\end{mybox}
\end{exdispExample*}
\end{docTcbKey}


\clearpage
\subsection{Watermark Option Keys}\label{subsec:watermarks}
The following watermark options are applicable for all skins which
use |tikzpicture| as \refKey{/tcb/graphical environment}.
Therefore, the skin \refSkin{standard} does not support these watermarks,
but all other skins, e.\,g.\ \refSkin{enhanced}.

\begin{marker}
The watermark options rely on the more general overlay options described in
Section \ref{subsec:overlays} from page \pageref{subsec:overlays}.
Therefore, \emph{watermarks} and \emph{overlays} cannot be used mixed.
But a mixture is possible with the \mylib{hooks} library, see Section \ref{sec:hooks}.
\end{marker}


\begin{docTcbKey}{watermark text}{=\meta{text}}{no default, initially unset}
  Writes some \meta{text} in the center of the interior region of a |tcolorbox|.
  This \meta{text} is written \emph{after} the
  frame and interior are drawn and \emph{before} the text content is drawn.
  It is zoomed or stretched according the values of
  \refKey{/tcb/watermark zoom} or \refKey{/tcb/watermark stretch}.
\begin{dispExample}
\tcbset{colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[enhanced,title=My title,watermark text=My Watermark]
\lipsum[1]
\tcblower
\lipsum[2]
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}

\enlargethispage*{1cm}

\begin{docTcbKey}{watermark text on}{=\meta{part} is \meta{text}}{no default, initially unset}
  This option writes some \meta{text} in the center of the interior region of a |tcolorbox|
  as described for \refKey{/tcb/watermark text}.
  But this is done only for boxes named \meta{part} of a break sequence, see
  \refKey{/tcb/breakable}.\\ 
  Feasible values for \meta{part} are:
  \begin{itemize}
  \item\docValue{broken}: all broken box parts,
  \item\docValue{unbroken}: unbroken boxes only,
  \item\docValue{first}: first parts of a break sequence,
  \item\docValue{middle}: middle parts of a break sequence,
  \item\docValue{last}: last parts of a break sequence,
  \item\docValue{unbroken and first}: unbroken boxes and first parts of a break sequence,
  \item\docValue{middle and last}: middle and last parts of a break sequence.
  \item\docValue{first and middle}: first and middle parts of a break sequence.
  \end{itemize}
\end{docTcbKey}


\clearpage


\begin{docTcbKey}{watermark graphics}{=\meta{file name}}{no default, initially unset}
  Draws an external picture referenced by \meta{file name}
  in the center of the interior region of a |tcolorbox|.
  The picture is drawn \emph{after} the
  frame and interior are drawn and \emph{before} the text content is drawn.
  It is zoomed or stretched according the values of
  \refKey{/tcb/watermark zoom} or \refKey{/tcb/watermark stretch}.
\begin{dispExample}
\tcbset{colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[enhanced,title=My title,watermark graphics=Basilica_5.png,
  watermark opacity=0.15]
\lipsum[1-2]
\tcblower
This example uses a public domain picture from\\
\url{http://commons.wikimedia.org/wiki/File:Basilica_5.png}
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{watermark graphics on}{=\meta{part} is \meta{file name}}{no default, initially unset}
  This option draws a picture referenced by \meta{file name} in the center of the interior region of a |tcolorbox|
  as described for \refKey{/tcb/watermark graphics}.
  But this is done only for boxes named \meta{part} of a break sequence, see
  \refKey{/tcb/breakable}.\\ 
  Feasible values for \meta{part} are:
  \begin{itemize}
  \item\docValue{broken}: all broken box parts,
  \item\docValue{unbroken}: unbroken boxes only,
  \item\docValue{first}: first parts of a break sequence,
  \item\docValue{middle}: middle parts of a break sequence,
  \item\docValue{last}: last parts of a break sequence,
  \item\docValue{unbroken and first}: unbroken boxes and first parts of a break sequence,
  \item\docValue{middle and last}: middle and last parts of a break sequence.
  \end{itemize}
\end{docTcbKey}



\clearpage
\begin{docTcbKey}{watermark tikz}{=\meta{graphical code}}{no default, initially unset}
  Draws the given |tikz| \meta{graphical code}
  in the center of the interior region of a |tcolorbox|.
  The code is executed \emph{after} the
  frame and interior are drawn and \emph{before} the text content is drawn.
  The result is zoomed or stretched according the values of
  \refKey{/tcb/watermark zoom} or \refKey{/tcb/watermark stretch}.
\begin{dispExample}
\tcbset{colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[enhanced,title=My title,
  watermark tikz={\draw[line width=2mm] circle (1cm)
    node{\fontfamily{ptm}\fontseries{b}\fontsize{20mm}{20mm}\selectfont ?};}]
\lipsum[1]
\tcblower
\lipsum[2]
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}



\begin{docTcbKey}{watermark tikz on}{=\meta{part} is \meta{graphical code}}{no default, initially unset}
  This option draws the given |tikz| \meta{graphical code} in the center of the interior region of a |tcolorbox|
  as described for \refKey{/tcb/watermark tikz}.
  But this is done only for boxes named \meta{part} of a break sequence, see
  \refKey{/tcb/breakable}.\\ 
  Feasible values for \meta{part} are:
  \begin{itemize}
  \item\docValue{broken}: all broken box parts,
  \item\docValue{unbroken}: unbroken boxes only,
  \item\docValue{first}: first parts of a break sequence,
  \item\docValue{middle}: middle parts of a break sequence,
  \item\docValue{last}: last parts of a break sequence,
  \item\docValue{unbroken and first}: unbroken boxes and first parts of a break sequence,
  \item\docValue{middle and last}: middle and last parts of a break sequence.
  \end{itemize}
\end{docTcbKey}


\begin{docTcbKey}{no watermark}{}{style, no default, initially set}
  Removes the watermark if set before. This is an alias for
  \refKey{/tcb/no overlay}.
\end{docTcbKey}


\clearpage
\begin{docTcbKey}{watermark opacity}{=\meta{fraction}}{no default, initially |1.00|}
  Sets the opacity value $\in[0,1]$ for a watermark.
\begin{dispExample}
\tcbset{enhanced,colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries,
  watermark text=Watermark,nobeforeafter,width=(\linewidth-2mm)/2}

\begin{tcolorbox}[title=Opacity 1.00,watermark opacity=1.00]
\lipsum[2]
\end{tcolorbox}\hfill%
\begin{tcolorbox}[title=Opacity 0.50,watermark opacity=0.50]
\lipsum[2]
\end{tcolorbox}%
\end{dispExample}
\end{docTcbKey}

\enlargethispage{5mm}
\begin{docTcbKey}{watermark zoom}{=\meta{fraction}}{no default, initially |0.75|}
  Sets the zoom value for a watermark. The zoom respects the aspect ratio.
  The value $1.0$ means to fill the whole box until the watermark touches the frame.
\begin{dispExample}
\tcbset{enhanced,colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries,
  watermark text=Watermark,nobeforeafter,width=(\linewidth-2mm)/2}

\begin{tcolorbox}[title=Zoom 1.0,watermark zoom=1.0]
\lipsum[2]
\end{tcolorbox}\hfill%
\begin{tcolorbox}[title=Zoom 0.5,watermark zoom=0.5]
\lipsum[2]
\end{tcolorbox}%
\end{dispExample}
\end{docTcbKey}

\clearpage

\begin{docTcbKey}{watermark shrink}{=\meta{fraction}}{no default, initially unset}
  Identically to \refKey{/tcb/watermark zoom}, but the watermark
  never gets enlarged. Thus, the watermark keeps its original size or is shrunk.
\end{docTcbKey}


\begin{docTcbKey}{watermark overzoom}{=\meta{fraction}}{no default, initially unset}
  Sets the overzoom value for a watermark. The overzoom respects the aspect ratio.
  The value $1.0$ means to fill the whole box until the watermark touches
  all four sides of the frame.
\begin{dispExample}
\tcbset{enhanced,colback=white,colframe=blue!50!black,fonttitle=\bfseries,
  watermark opacity=0.5,
  watermark graphics=lichtspiel.jpg,nobeforeafter,width=(\linewidth-2mm)/2}

\begin{tcolorbox}[title=Zoom 1.0,watermark zoom=1.0]
\lipsum[1]
\end{tcolorbox}\hfill%
\begin{tcolorbox}[title=Overzoom 1.0,watermark overzoom=1.0]
\lipsum[1]
\end{tcolorbox}%
\end{dispExample}
\end{docTcbKey}

\begin{marker}
If a \refKey{/tcb/watermark overzoom} value of |1.0| is used in connection
with invisible top and bottom rules which still have a thickness greater than |0pt|,
the space of these invisible rules may not be covered by the watermark.
For example, this situation may occur during the breaking of \refKey{/tcb/enhanced} boxes.
To avoid this optical glitch, just set \refKey{/tcb/pad at break} to any desired value.
\end{marker}

\clearpage
\begin{docTcbKey}{watermark stretch}{=\meta{fraction}}{no default, initially unset}
  Sets the stretch value for a watermark. The stretch value is applied to width
  and height in relation to the box dimensions. It does not respect the aspect ratio.
  The value $1.0$ means to fill the whole box.
\begin{dispExample}
\tcbset{enhanced,colback=white,colframe=blue!50!black,fonttitle=\bfseries,
  watermark graphics=lichtspiel.jpg,watermark opacity=0.5,
  nobeforeafter,width=(\linewidth-2mm)/2}

\begin{tcolorbox}[title=Stretch 1.00,watermark stretch=1.00]
\lipsum[2]
\end{tcolorbox}\hfill%
\begin{tcolorbox}[title=Stretch 0.50,watermark stretch=0.50]
\lipsum[2]
\end{tcolorbox}%
\end{dispExample}
\end{docTcbKey}

\begin{docTcbKey}{watermark color}{=\meta{color}}{no default, initially mixed background and frame color}
  Sets the color for the watermark.
\begin{dispExample}
\tcbset{colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[enhanced,title=My title,watermark text=My Watermark,
  watermark color=yellow!50!red]
\lipsum[1]
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}

\clearpage

\begin{docTcbKey}{clip watermark}{\colOpt{=true\textbar false}}{default |true|, initially |true|}
  Sets the watermark to be clipped to the interior area.
\begin{dispExample}
\tcbset{enhanced,colback=white,colframe=blue!50!white,fonttitle=\bfseries,
  watermark opacity=0.5,watermark stretch=1.00,arc=3mm,
  watermark graphics=lichtspiel.jpg}

\begin{tcolorbox}[title=Clip (default),clip watermark]
\lipsum[1]
\end{tcolorbox}

\begin{tcolorbox}[title=No clip,clip watermark=false]
\lipsum[1]
\end{tcolorbox}%
\end{dispExample}
\end{docTcbKey}



\clearpage
\subsection{Clip Environments}\label{subsec:clipping}
The following clip environments are applicable for all skins which
use engines of type |path|, |pathfirst|, |pathmiddle|, or |pathlast|.
Especially, the skin \refSkin{enhanced} supports \emph{all} of them
and \refSkin{standard} \emph{none}. The typical area of application
is inside overlay code, see Section \ref{subsec:overlays} from
page \pageref{subsec:overlays}.


\begin{docEnvironment}{tcbclipframe}{}
Defines a |Tikz| scope which clips to the frame area path.
\begin{dispExample}
\makeatletter
\newtcolorbox{picturebox}[2][]{%
  enhanced,frame hidden,interior hidden,fonttitle=\bfseries,
  overlay={\begin{tcbclipframe}\node at (frame)
    {\includegraphics[width=\tcb@width,height=\tcb@height]{#2}};\end{tcbclipframe}%
    \begin{tcbclipinterior}\fill[white,opacity=0.75]
    (frame.south west) rectangle (frame.north east);\end{tcbclipinterior}},#1}
\makeatother

\begin{picturebox}[title=My Picture Box]{lichtspiel.jpg}
\lipsum[1]
\end{picturebox}
\end{dispExample}
\end{docEnvironment}

\clearpage
\begin{docEnvironment}{tcbinvclipframe}{}
Defines a |Tikz| scope which clips to the \emph{outside} of the frame area path.

\begin{dispExample*}{segmentation style={preaction={fill=white},pattern=checkerboard,pattern color=gray!40}}
\tcbset{enhanced jigsaw,fonttitle=\bfseries,opacityback=0.35,colback=blue!5!white,
  frame style={left color=red!75!black,right color=red!10!yellow}}

\begin{tikzpicture}% draw two balls
  \path[use as bounding box] (0,0.8) rectangle +(0.1,0.1);
  \shadedraw [shading=ball] (0,0) circle (1cm);
  \shadedraw [ball color=red] (3,-2.2) circle (1cm);
\end{tikzpicture}

\begin{tcolorbox}[title=A translucent box,
  overlay={\begin{tcbinvclipframe}
    \draw[red,line width=1cm] ([xshift=-2mm,yshift=2mm]frame.north west)
      --([xshift=2mm,yshift=-2mm]frame.south east);
    \draw[red,line width=1cm] ([xshift=-2mm,yshift=-2mm]frame.south west)
      --([xshift=2mm,yshift=2mm]frame.north east);
  \end{tcbinvclipframe}}]
  \lipsum[2]
\end{tcolorbox}
\end{dispExample*}
\end{docEnvironment}

\clearpage
\begin{docEnvironment}{tcbclipinterior}{}
Defines a |Tikz| scope which clips to the interior area path.
\begin{dispExample}
\begin{tcolorbox}[enhanced,title=My Title,
  overlay={\begin{tcbclipinterior}
    \draw[red,line width=1cm] (interior.north west)--(interior.south east);
    \draw[red,line width=1cm] (interior.south west)--(interior.north east);
  \end{tcbclipinterior}}]
\lipsum[1]
\end{tcolorbox}
\end{dispExample}
\end{docEnvironment}

\begin{docEnvironment}{tcbcliptitle}{}
Defines a |Tikz| scope which clips to the title area path.
\begin{dispExample}
\begin{tcolorbox}[enhanced,title=My Title,colframe=blue,colback=yellow!10!white,
  overlay={\begin{tcbcliptitle}\node at (title)
  {\includegraphics[width=\linewidth]{lichtspiel.jpg}};\end{tcbcliptitle}}]
\lipsum[1]
\end{tcolorbox}
\end{dispExample}
\end{docEnvironment}

\clearpage
\begin{docTcbKey}{clip title}{\colOpt{=true\textbar false}}{default |true|, initially |false|}
  Sets the title to be clipped to the title area.
\begin{dispExample}
\tcbset{enhanced,width=5cm,colframe=red!50!white,coltitle=black,
  colbacktitle=yellow!50!white}

\begin{tcolorbox}[title=\mbox{This is a title which is unbreakable and far too long}]
This is a tcolorbox.
\end{tcolorbox}

\begin{tcolorbox}[title=\mbox{This is a title which is unbreakable and far too long},
  clip title]
This is a tcolorbox.
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{clip upper}{\colOpt{=true\textbar false}}{default |true|, initially |false|}
  Sets the upper part to be clipped to the interior area.
\begin{dispExample}
\newcommand{\mygraphics}[2][]{%
  \tcbox[enhanced,boxsep=0pt,top=0pt,bottom=0pt,left=0pt,
    right=0pt,boxrule=0.4pt,drop fuzzy shadow,clip upper,
    colback=black!75!white,toptitle=2pt,bottomtitle=2pt,nobeforeafter,
    center title,fonttitle=\small\sffamily,title=\detokenize{#2}]
  {\includegraphics[width=\the\dimexpr(\linewidth-4mm)/2\relax]{#2}}}

\mygraphics{lichtspiel.jpg}\hfill
\mygraphics{Basilica_5.png}
\end{dispExample}
\end{docTcbKey}

\clearpage
The example for \refKey{/tcb/clip upper} sizes the box according to
the dimensions of the picture. To do it the other way around, the watermark
options provide an easy solution.
\begin{dispExample}
\newcommand{\mygraphics}[2][]{%
  \tcbox[enhanced,capture=minipage,boxsep=0pt,top=0pt,bottom=0pt,left=0pt,
    right=0pt,boxrule=0.4pt,drop fuzzy shadow,nobeforeafter,
    colback=black!75!white,toptitle=2pt,bottomtitle=2pt,
    center title,fonttitle=\small\sffamily,title=\detokenize{#2},
    width=(\linewidth-4mm)/2,height=6cm,colbacktitle={black},
    watermark zoom=1.0,watermark graphics={#2}]{}}

\mygraphics{lichtspiel.jpg}\hfill
\mygraphics{Basilica_5.png}
\end{dispExample}


\begin{docTcbKey}{clip lower}{\colOpt{=true\textbar false}}{default |true|, initially |false|}
  Sets the lower part to be clipped to the interior area.
\begin{dispExample}
\tcbset{enhanced,width=5cm,colframe=red!50!black,text and listing}

\begin{tcblisting}{}
Donau\-dampf\-schiff\-fahrts\-ka\-pi\-t\"ans\-m\"ut\-zen\-fran\-sen
\end{tcblisting}

\begin{tcblisting}{clip lower}
Donau\-dampf\-schiff\-fahrts\-ka\-pi\-t\"ans\-m\"ut\-zen\-fran\-sen
\end{tcblisting}
\end{dispExample}
\end{docTcbKey}


\clearpage
\subsection{Border Line Option Keys}\label{subsec:borderline}
The following borderline options are applicable for most skins which
use |tikzpicture| as \refKey{/tcb/graphical environment}.
Therefore, the skin \refSkin{standard} does not support these border lines,
but most other skins, e.\,g.\ \refSkin{enhanced}.

The borderlines are independent from the normal |tcolorbox| rules.
They may be used with or without the \refKey{/tcb/segmentation engine}.

The borderlines are stackable, i.\,e.\ several different border lines can be
used on the same |tcolorbox|. They are drawn \emph{after} the box frame and box
interior and \emph{before} overlays or watermarks.

\begin{marker}
Technically, the normal |tcolorbox| rules result from a \tikzname\  \emph{filling}
process. The border lines are created by a \tikzname\  \emph{drawing} process.
This can be used to apply different effects.
\end{marker}


\begin{docTcbKey}{borderline}{=\marg{width}\marg{offset}\marg{options}}{no default, initially unset}
  Adds a new borderline to the stack of border lines.
  This border line is drawn with the given \meta{width} and gets an
  \meta{offset} computed from the frame outline. A positive \meta{offset} value
  moves the borderline inside the |tcolorbox| and a negative \meta{offset} value
  moves it outside without changing the bounding box.\\
  The border line is drawn along a \tikzname\  path with the given \tikzname\  \meta{options}.
  Note that the \tikzname\  |line width| option should not be used here.\\
  The border lines adapt to the rounded corners of the |tcolorbox|. An inside
  borderline will switch to sharp corners if necessary, an outside borderline will
  always be rounded except for \refKey{/tcb/sharp corners}.
\begin{dispExample}
\begin{tcolorbox}[enhanced,title=Rounded corners,fonttitle=\bfseries,boxsep=5pt,
  arc=8pt,
  borderline={0.5pt}{0pt}{red},
  borderline={0.5pt}{5pt}{blue,dotted},
  borderline={0.5pt}{-5pt}{green} ]
This is a tcolorbox.
\end{tcolorbox}
\bigskip
\begin{tcolorbox}[enhanced,title=Sharp corners,fonttitle=\bfseries,boxsep=5pt,
  arc=8pt,sharp corners=downhill,
  borderline={0.5pt}{0pt}{red},
  borderline={0.5pt}{5pt}{blue,dotted},
  borderline={0.5pt}{-5pt}{green} ]
This is a tcolorbox.
\end{tcolorbox}
\end{dispExample}

\begin{dispExample}
% \usepackage{lipsum}
\begin{tcolorbox}[enhanced,arc=3mm,boxrule=1.5mm,boxsep=1.5mm,
  colback=yellow!20!white,
  colframe=blue,
  borderline={1mm}{1mm}{white},
  borderline={1mm}{2mm}{red} ]
  \lipsum[1]
\end{tcolorbox}
\end{dispExample}


\begin{dispExample}
% \usepackage{lipsum}
\begin{tcolorbox}[enhanced,arc=3mm,boxrule=1.5mm,
  frame hidden,colback=blue!10!white,
  borderline={1mm}{0mm}{blue,dotted} ]
  \lipsum[2]
\end{tcolorbox}
\end{dispExample}


\begin{dispExample}
% \usepackage{lipsum}
\begin{tcolorbox}[enhanced,skin=enhancedmiddle,
  frame hidden,interior hidden,top=0mm,bottom=0mm,boxsep=0mm,
  borderline={0.75mm}{0mm}{red},
  borderline={0.75mm}{0.75mm}{red!50!yellow},
  borderline={0.75mm}{1.5mm}{yellow}, ]
  \lipsum[3]
\end{tcolorbox}
\end{dispExample}

\begin{dispExample}
% \usepackage{lipsum}
\newtcolorbox{mygreenbox}[2][]{%
  enhanced,width=\linewidth-6pt,
  enlarge top by=3pt,enlarge bottom by=3pt,
  enlarge left by=3pt,enlarge right by=3pt,
  title={#2},frame hidden,boxrule=0pt,top=1mm,bottom=1mm,
  colframe=green!30!black, colbacktitle=green!50!yellow,
  coltitle=black, colback=green!25!white,
  borderline={0.5pt}{-0.5pt}{green!75!blue},
  borderline={1pt}{-3pt}{green!50!blue},#1}

\begin{mygreenbox}{My title}
  \lipsum[4]
\end{mygreenbox}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{no borderline}{}{no default, initially set}
  Removes all borderlines if set before.
\end{docTcbKey}


\begin{docTcbKey}{show bounding box}{\colOpt{=\meta{color}}}{default |red|, initially unset}
  Displays the bounding box borderline of a |tcolorbox|.
  Its intended use is debugging and fine tuning.
  It should not be part of a final document.
  The optional \meta{color} is the base color for the bounding box
  borderline.
\begin{dispExample}
\tcbset{enhanced,nobeforeafter,width=4cm,fonttitle=\bfseries}

\begin{tcolorbox}[show bounding box,title=Normal]
This is a tcolorbox.
\end{tcolorbox}%
\begin{tcolorbox}[show bounding box=blue,title=Shadow,drop fuzzy shadow]
This is a tcolorbox.
\end{tcolorbox}%
\begin{tcolorbox}[show bounding box=green,title=Enlarged,drop fuzzy shadow,
  enlarge by=2mm]
This is a tcolorbox.
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}

\clearpage

\begin{marker}
The following \emph{partial} borderlines act slightly different from the
complete borderlines described before. They ignore rounded corner settings,
their length is not modified by their \meta{offset}, they ignore skin settings
but adapt to breakable boxes.
\end{marker}

\begin{docTcbKey}[][doc new=2014-10-20]{borderline north}{=\marg{width}\marg{offset}\marg{options}}{no default, initially unset}
  Adds a new borderline with the given \meta{width} to the
  north of the |tcolorbox|.
  A positive \meta{offset} value
  moves the borderline inside the |tcolorbox| and a negative \meta{offset} value
  moves it outside without changing the bounding box.
\begin{dispExample*}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[enhanced,
  borderline north={2pt}{-2pt}{red}]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-10-20]{borderline south}{=\marg{width}\marg{offset}\marg{options}}{no default, initially unset}
  Adds a new borderline with the given \meta{width} to the
  south of the |tcolorbox|.
  A positive \meta{offset} value
  moves the borderline inside the |tcolorbox| and a negative \meta{offset} value
  moves it outside without changing the bounding box.
\begin{dispExample*}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[enhanced,
  borderline south={2pt}{-2pt}{red}]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-10-20]{borderline east}{=\marg{width}\marg{offset}\marg{options}}{no default, initially unset}
  Adds a new borderline with the given \meta{width} to the
  east of the |tcolorbox|.
  A positive \meta{offset} value
  moves the borderline inside the |tcolorbox| and a negative \meta{offset} value
  moves it outside without changing the bounding box.
\begin{dispExample*}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[enhanced,
  borderline east={2pt}{-2pt}{red}]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-10-20]{borderline west}{=\marg{width}\marg{offset}\marg{options}}{no default, initially unset}
  Adds a new borderline with the given \meta{width} to the
  west of the |tcolorbox|.
  A positive \meta{offset} value
  moves the borderline inside the |tcolorbox| and a negative \meta{offset} value
  moves it outside without changing the bounding box.
\begin{dispExample*}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[enhanced,
  borderline west={2pt}{-2pt}{red}]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}[][doc new=2014-10-20]{borderline horizontal}{=\marg{width}\marg{offset}\marg{options}}{no default, initially unset}
  Adds a new borderline with the given \meta{width} to the
  north and south of the |tcolorbox|.
  A positive \meta{offset} value
  moves the borderlines inside the |tcolorbox| and a negative \meta{offset} value
  moves them outside without changing the bounding box.
\begin{dispExample*}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[blanker,top=3mm,bottom=3mm,
   borderline horizontal={2pt}{0pt}{red}]
  This is a \textbf{tcolorbox}.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2014-10-20]{borderline vertical}{=\marg{width}\marg{offset}\marg{options}}{no default, initially unset}
  Adds a new borderline with the given \meta{width} to the
  east and west of the |tcolorbox|.
  A positive \meta{offset} value
  moves the borderlines inside the |tcolorbox| and a negative \meta{offset} value
  moves them outside without changing the bounding box.
\begin{dispExample*}{sbs,lefthand ratio=0.6}
\begin{tcolorbox}[blanker,left=3mm,right=3mm,
   borderline vertical={2pt}{0pt}{red}]
  This is a \textbf{tcolorbox}.\\
  My second line.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}

\begin{dispExample}
\begin{tcolorbox}[enhanced,colback=yellow!10!white,boxrule=0pt,frame hidden,
  borderline north={1mm}{-2mm}{red},
  borderline south={1mm}{-2mm}{blue},
  borderline west={1mm}{-2mm}{green},
  borderline east={1mm}{-2mm}{yellow}]
\lipsum[1]
\end{tcolorbox}
\end{dispExample}

\clearpage
\subsection{Shadow Option Keys}\label{subsec:shadows}
The following shadow options are applicable for most skins which
use |tikzpicture| as \refKey{/tcb/graphical environment}.
Therefore, the skin \refSkin{standard} does not support these shadows,
but most other skins, e.\,g.\ \refSkin{enhanced}.

The shadows are stackable, i.\,e.\ several different shadows can be
used on the same |tcolorbox|. They are drawn \emph{before} the box frame is drawn.

\begin{docTcbKey}{no shadow}{}{no default}
  Removes all shadows if set before.
\end{docTcbKey}

\subsubsection{Common Shadows and Halos}

\begin{docTcbKey}{drop shadow}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new shadow with standard dimensions to the stack of shadows.
  Optionally, the \meta{color} for the shadow can be changed.
\begin{dispExample*}{sbs,lefthand ratio=0.6}
\tcbset{enhanced,colback=red!5!white,
  colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[drop shadow]
This is a tcolorbox.
\end{tcolorbox}\par\bigskip
\begin{tcolorbox}[title=Another shadow,
  drop shadow=blue]
This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}


\begin{docTcbKey}{drop fuzzy shadow}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new fuzzy shadow with standard dimensions to the stack of shadows.
  Optionally, the \meta{color} for the shadow can be changed.
\begin{dispExample*}{sbs,lefthand ratio=0.6}
\tcbset{enhanced,colback=red!5!white,
  colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[drop fuzzy shadow]
This is a tcolorbox.
\end{tcolorbox}\par\bigskip
\begin{tcolorbox}[title=Another shadow,
  drop fuzzy shadow=blue]
This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}


\begin{docTcbKey}{drop midday shadow}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new shadow with standard dimensions to the stack of shadows.
  Optionally, the \meta{color} for the shadow can be changed.
\begin{dispExample*}{sbs,lefthand ratio=0.6}
\tcbset{enhanced,colback=red!5!white,
  colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[drop midday shadow]
This is a tcolorbox.
\end{tcolorbox}\par\bigskip
\begin{tcolorbox}[title=Another shadow,
  drop midday shadow=blue]
This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}

%\enlargethispage*{2cm}
\begin{docTcbKey}{drop fuzzy midday shadow}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new fuzzy shadow with standard dimensions to the stack of shadows.
  Optionally, the \meta{color} for the shadow can be changed.
\begin{dispExample*}{sbs,lefthand ratio=0.6}
\tcbset{enhanced,colback=red!5!white,
  colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[drop fuzzy midday shadow]
This is a tcolorbox.
\end{tcolorbox}\par\bigskip
\begin{tcolorbox}[title=Another shadow,
  drop fuzzy midday shadow=blue]
This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}


\begin{docTcbKey}{halo}{\colOpt{=\meta{size} \texttt{with} \meta{color}}}{style, default |0.9mm with yellow|}
  Adds a new halo shadow with the given \meta{color}
  which overlaps the colorbox an all sides by \meta{size}.
\begin{dispExample*}{sbs,lefthand ratio=0.6}
\tcbset{enhanced,colback=red!5!white,
  colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[title=My own halo,halo]
This is a tcolorbox.
\end{tcolorbox}
\par\bigskip\bigskip
\begin{tcolorbox}[title=Another halo,
  halo=2mm with green]
This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}

\enlargethispage*{2cm}
\begin{docTcbKey}{fuzzy halo}{\colOpt{=\meta{size} \texttt{with} \meta{color}}}{style, default |0.9mm with yellow|}
  Adds a new fuzzy halo shadow with the given \meta{color}
  which overlaps the colorbox an all sides by \meta{size} plus |0.48mm|.
\begin{dispExample*}{sbs,lefthand ratio=0.6}
\tcbset{enhanced,colback=red!5!white,
  colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[title=My own halo,fuzzy halo]
This is a tcolorbox.
\end{tcolorbox}
\par\bigskip\bigskip
\begin{tcolorbox}[title=Another halo,
  fuzzy halo=2mm with green]
This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}

\begin{dispExample}
\begin{tcolorbox}[blank,enhanced jigsaw,boxsep=2pt,arc=2pt,
  fuzzy halo=2mm with red!50!white,
  fuzzy halo=1mm with white]
\lipsum[1]
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}


\clearpage
For all following shadows, the optionally given \meta{color} for the shadow can be changed
equivalent to the preceding examples.

\begin{docTcbKey}{drop shadow southeast}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new shadow with standard dimensions to the stack of shadows.
  This shadow is identical to \refKey{/tcb/drop shadow}.
\begin{dispExample*}{sbs,lefthand ratio=0.7}
\begin{tcolorbox}[drop shadow southeast,
  enhanced,colback=red!5!white,colframe=red!75!black]
  This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}%

\begin{docTcbKey}{drop shadow south}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new shadow with standard dimensions to the stack of shadows.
  This shadow is identical to \refKey{/tcb/drop midday shadow}.
\begin{dispExample*}{sbs,lefthand ratio=0.7}
\begin{tcolorbox}[drop shadow south,
  enhanced,colback=red!5!white,colframe=red!75!black]
  This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}%

\begin{docTcbKey}{drop shadow southwest}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new shadow with standard dimensions to the stack of shadows.
\begin{dispExample*}{sbs,lefthand ratio=0.7}
\begin{tcolorbox}[drop shadow southwest,
  enhanced,colback=red!5!white,colframe=red!75!black]
  This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}%

\begin{docTcbKey}{drop shadow west}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new shadow with standard dimensions to the stack of shadows.
\begin{dispExample*}{sbs,lefthand ratio=0.7}
\begin{tcolorbox}[drop shadow west,
  enhanced,colback=red!5!white,colframe=red!75!black]
  This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}%

\begin{docTcbKey}{drop shadow northwest}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new shadow with standard dimensions to the stack of shadows.
\begin{dispExample*}{sbs,lefthand ratio=0.7}
\begin{tcolorbox}[drop shadow northwest,
  enhanced,colback=red!5!white,colframe=red!75!black]
  This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}%

\begin{docTcbKey}{drop shadow north}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new shadow with standard dimensions to the stack of shadows.
\begin{dispExample*}{sbs,lefthand ratio=0.7}
\begin{tcolorbox}[drop shadow north,
  enhanced,colback=red!5!white,colframe=red!75!black]
  This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}%

\clearpage
\begin{docTcbKey}{drop shadow northeast}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new shadow with standard dimensions to the stack of shadows.
\begin{dispExample*}{sbs,lefthand ratio=0.7}
\begin{tcolorbox}[drop shadow northeast,
  enhanced,colback=red!5!white,colframe=red!75!black]
  This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}%

\begin{docTcbKey}{drop shadow east}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new shadow with standard dimensions to the stack of shadows.
\begin{dispExample*}{sbs,lefthand ratio=0.7}
\begin{tcolorbox}[drop shadow east,
  enhanced,colback=red!5!white,colframe=red!75!black]
  This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}%


\begin{docTcbKey}{drop fuzzy shadow southeast}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new fuzzy shadow with standard dimensions to the stack of shadows.
  This shadow is identical to \refKey{/tcb/drop fuzzy shadow}.
\begin{dispExample*}{sbs,lefthand ratio=0.7}
\begin{tcolorbox}[drop fuzzy shadow southeast,
  enhanced,colback=red!5!white,colframe=red!75!black]
  This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}%

\begin{docTcbKey}{drop fuzzy shadow south}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new fuzzy shadow with standard dimensions to the stack of shadows.
  This shadow is identical to \refKey{/tcb/drop fuzzy midday shadow}.
\begin{dispExample*}{sbs,lefthand ratio=0.7}
\begin{tcolorbox}[drop fuzzy shadow south,
  enhanced,colback=red!5!white,colframe=red!75!black]
  This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}%

\begin{docTcbKey}{drop fuzzy shadow southwest}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new fuzzy shadow with standard dimensions to the stack of shadows.
\begin{dispExample*}{sbs,lefthand ratio=0.7}
\begin{tcolorbox}[drop fuzzy shadow southwest,
  enhanced,colback=red!5!white,colframe=red!75!black]
  This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}%

\begin{docTcbKey}{drop fuzzy shadow west}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new fuzzy shadow with standard dimensions to the stack of shadows.
\begin{dispExample*}{sbs,lefthand ratio=0.7}
\begin{tcolorbox}[drop fuzzy shadow west,
  enhanced,colback=red!5!white,colframe=red!75!black]
  This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}%

\clearpage
\begin{docTcbKey}{drop fuzzy shadow northwest}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new fuzzy shadow with standard dimensions to the stack of shadows.
\begin{dispExample*}{sbs,lefthand ratio=0.7}
\begin{tcolorbox}[drop fuzzy shadow northwest,
  enhanced,colback=red!5!white,colframe=red!75!black]
  This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}%

\begin{docTcbKey}{drop fuzzy shadow north}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new fuzzy shadow with standard dimensions to the stack of shadows.
\begin{dispExample*}{sbs,lefthand ratio=0.7}
\begin{tcolorbox}[drop fuzzy shadow north,
  enhanced,colback=red!5!white,colframe=red!75!black]
  This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}%

\begin{docTcbKey}{drop fuzzy shadow northeast}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new fuzzy shadow with standard dimensions to the stack of shadows.
\begin{dispExample*}{sbs,lefthand ratio=0.7}
\begin{tcolorbox}[drop fuzzy shadow northeast,
  enhanced,colback=red!5!white,colframe=red!75!black]
  This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}%

\begin{docTcbKey}{drop fuzzy shadow east}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new fuzzy shadow with standard dimensions to the stack of shadows.
\begin{dispExample*}{sbs,lefthand ratio=0.7}
\begin{tcolorbox}[drop fuzzy shadow east,
  enhanced,colback=red!5!white,colframe=red!75!black]
  This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}%


\clearpage
\subsubsection{Lifted Shadows}

\begin{docTcbKey}{drop lifted shadow}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new lifted shadow with standard dimensions to the stack of shadows.
  Optionally, the \meta{color} for the shadow can be changed.
\begin{dispExample*}{sbs,lefthand ratio=0.6}
\tcbset{enhanced,colback=red!5!white,
  boxrule=0.4pt,sharp corners,
  colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[drop lifted shadow]
This is a tcolorbox.
\end{tcolorbox}\par\bigskip
\begin{tcolorbox}[title=Another shadow,
  drop lifted shadow=blue]
This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}


\begin{docTcbKey}{drop small lifted shadow}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new small lifted shadow with standard dimensions to the stack of shadows.
  Optionally, the \meta{color} for the shadow can be changed.
\begin{dispExample*}{sbs,lefthand ratio=0.6}
\tcbset{enhanced,colback=red!5!white,
  boxrule=0.4pt,sharp corners,
  colframe=red!75!black,fonttitle=\bfseries}

\tcbox[drop small lifted shadow,size=fbox]
  {This is a tcolorbox.}
\par\bigskip
\begin{tcolorbox}[title=Another shadow,
  drop small lifted shadow=black]
This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}


\begin{docTcbKey}{drop large lifted shadow}{\colOpt{=\meta{color}}}{style, default |black!50!white|}
  Adds a new large lifted shadow with standard dimensions to the stack of shadows.
  Optionally, the \meta{color} for the shadow can be changed.
\begin{dispExample*}{sbs,lefthand ratio=0.6}
\tcbset{enhanced,colback=red!5!white,
  colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[drop large lifted shadow]
This is a tcolorbox.
\end{tcolorbox}\par\bigskip
\begin{tcolorbox}[title=Another shadow,
  drop large lifted shadow=blue]
This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}


\clearpage

\subsubsection{Generic Shadows}
\begin{docTcbKey}{shadow}{=\marg{xshift}\marg{yshift}\marg{offset}\marg{options}}{no default}
  Adds a new shadow to the stack of shadows.
  This shadow follows the outline of the |tcolorbox| but is shifted by
  \meta{xshift} and \meta{yshift}. The \meta{offset} value is a distance value
  from the frame outline.  A positive \meta{offset} value shrinks the shadow
  and a negative \meta{offset} value enlarges the shadow.
  The shadow is filled along a \tikzname\  path with the given \tikzname\  \meta{options}.\\
  The shadows adapt to the rounded corners of the |tcolorbox|. An shrinked shadow
  will switch to sharp corners if necessary, an enlarged shadow may become
  more rounded depending on several factors. But \refKey{/tcb/sharp corners}
  have sharp shadows.
  \begin{marker}
  Shadows are not considered for the bounding box computation by default.
  Large shadows may be overlaped by the following content. But, the
  bounding box can be adapted if necessary.
  \end{marker}

\begin{dispExample*}{sbs,lefthand ratio=0.6}
\tcbset{enhanced,colback=red!5!white,
  colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[title=My own shadow,
  shadow={2mm}{-1mm}{0mm}{black!50!white}]
This is a tcolorbox.
\end{tcolorbox}
\par\bigskip
\begin{tcolorbox}[title=Another shadow,
  shadow={-1mm}{-2mm}{0mm}{fill=blue,
    opacity=0.5}]
This is a tcolorbox.
\end{tcolorbox}
\par\bigskip
\begin{tcolorbox}[title=Double shadow,
  shadow={-1.5mm}{-1.5mm}{0mm}{fill=blue,
    opacity=0.25},
  shadow={1.5mm}{-1.5mm}{0mm}{fill=red,
    opacity=0.25}]
This is a tcolorbox.
\end{tcolorbox}
\par\bigskip
\begin{tcolorbox}[title=Far shadow,
  shadow={5.5mm}{-3.5mm}{2mm}{fill=black,
    opacity=0.25}]
This is a tcolorbox.
\end{tcolorbox}
\par\bigskip\bigskip
\begin{tcolorbox}[title=Halo shadow,
  shadow={0mm}{0mm}{-1.5mm}%
     {fill=yellow!75!red,opacity=0.5}]
This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{fuzzy shadow}{=\marg{xshift}\marg{yshift}\marg{offset}\marg{step}\marg{options}}{no default}
  Adds a new fuzzy shadow to the stack of shadows. Actually, this option
  adds several shadows which appear like a shadow with a fuzzy border.
  This fuzzy shadow follows the outline of the |tcolorbox| but is shifted by
  \meta{xshift} and \meta{yshift}. The \meta{offset} value is a distance value
  from the frame outline.  A positive \meta{offset} value shrinks the shadow
  and a negative \meta{offset} value enlarges the shadow.
  The \marg{step} value describes a shrink
  offset used for the combination of the partial shadows.
  The shadow is filled along a \tikzname\  path with the given \tikzname\  \meta{options} but
  any |opacity| value will be ignored.
\begin{dispExample*}{sbs,lefthand ratio=0.6}
\tcbset{enhanced,colback=red!5!white,
  colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[title=My own shadow,
  fuzzy shadow={2mm}{-1mm}{0mm}{0.1mm}%
               {black!50!white}]
This is a tcolorbox.
\end{tcolorbox}
\par\bigskip
\begin{tcolorbox}[title=Another shadow,
  fuzzy shadow={-1mm}{-2mm}{0mm}{0.2mm}%
               {fill=blue}]
This is a tcolorbox.
\end{tcolorbox}
\par\bigskip
\begin{tcolorbox}[title=Double shadow,
  fuzzy shadow={-1.5mm}{-1.5mm}{0mm}{0.1mm}%
               {blue},
  fuzzy shadow={1.5mm}{-1.5mm}{0mm}{0.1mm}%
               {red}]
This is a tcolorbox.
\end{tcolorbox}
\par\bigskip
\begin{tcolorbox}[title=Far shadow,
  fuzzy shadow={5.5mm}{-3.5mm}{0mm}{0.3mm}%
               {black}]
This is a tcolorbox.
\end{tcolorbox}
\par\bigskip\bigskip
\begin{tcolorbox}[title=Glow shadow,
  fuzzy shadow={0mm}{0mm}{-1.5mm}{0.15mm}%
               {yellow!75!red}]
This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}

\begin{dispExample}
\newtcolorbox{mybox}[1][]{enhanced,
  fuzzy shadow={1.0mm}{-1.0mm}{0.12mm}{0mm}{blue!50!white},
  fuzzy shadow={-1.0mm}{-1.0mm}{0.12mm}{0mm}{red!50!white},
  fuzzy shadow={-1.0mm}{1.0mm}{0.12mm}{0mm}{green!50!white},
  fuzzy shadow={1.0mm}{1.0mm}{0.12mm}{0mm}{yellow!50!white},#1
}

\begin{mybox}[title=A multi shadow box]
This is a tcolorbox.
\end{mybox}
\end{dispExample}
\end{docTcbKey}


\clearpage
\begin{docTcbKey}[][doc new=2015-05-05]{smart shadow arc}{\colOpt{=true\textbar false}}{default |true|,
  initially |true|}
If set to |true|, the shadow drawing algorithm tries to do a somewhat
smart calculation of the arc for the shadow. The result is pleasing for typical boxes
with rounded corners, but gives strange results for circular boxes.

\begin{dispExample}
\tcbset{enhanced,nobeforeafter,colback=red!5!white,
  colframe=red!75!black,width=3cm,square,halign=center,valign=center
  }

\begin{tcolorbox}[drop shadow]
Smart shadow arc (arguably better than normal)
\end{tcolorbox}
\hfill
\begin{tcolorbox}[smart shadow arc=false, drop shadow]
Normal shadow arc
\end{tcolorbox}
\hfill
\begin{tcolorbox}[circular arc, drop shadow]
Smart shadow arc (worse than normal)
\end{tcolorbox}
\hfill
\begin{tcolorbox}[circular arc, smart shadow arc=false, drop shadow]
Normal shadow arc
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{lifted shadow}{=\marg{xshift}\marg{yshift}\marg{bend}\marg{step}\marg{options}}{no default}
  Adds a new lifted shadow to the stack of shadows. Actually, this option
  adds several shadows which appear like a shadow with a fuzzy border.
  This lifted shadow follows the outline of the |tcolorbox| but is shifted by
  \meta{xshift} and \meta{yshift} on the lower left corner and by
  $-$\meta{xshift} and \meta{yshift} on the lower right corner.
  Additionally, there is a \meta{bend} in the middle.
  The \marg{step} value describes a shrink
  offset used for the combination of the partial shadows.
  The shadow is filled along a \tikzname\  path with the given \tikzname\  \meta{options} but
  any |opacity| value will be ignored.
\begin{dispExample*}{sbs,lefthand ratio=0.6}
\tcbset{enhanced,colback=red!5!white,
  boxrule=0.1pt,
  colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[title=My own shadow,
  lifted shadow={1mm}{-2mm}{3mm}{0.1mm}%
               {black!50!white}]
This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}

\clearpage
\subsubsection{\tikzname\ Shadows}
Alternativ to the package shadow options described before, shadows from
the \flqq Shadows Library\frqq\ of \tikzname\ can be used.
Such shadows can be added directly to the frame path using \refKey{/tcb/frame style}.

\begin{exdispExample*}{tikz_shadow_1}{sbs,lefthand ratio=0.7}
% \usetikzlibrary{shadows}
\begin{tcolorbox}[enhanced,
  colback=red!5!white,colframe=red!75!black,
  frame style={drop shadow} ]
  This is a tcolorbox.
\end{tcolorbox}
\end{exdispExample*}

\begin{exdispExample*}{tikz_shadow_2}{sbs,lefthand ratio=0.7}
% \usetikzlibrary{shadows}
\begin{tcolorbox}[enhanced,height=3cm,
  colback=red!5!white,colframe=red!75!black,
  halign=center,valign=center,
  frame style={circular drop shadow} ]
  This is a tcolorbox.
\end{tcolorbox}
\end{exdispExample*}

\begin{exdispExample*}{tikz_shadow_3}{sbs,lefthand ratio=0.7}
% \usetikzlibrary{shadows}
\begin{tcolorbox}[enhanced,width=2.5cm,
  square,circular arc,
  halign=center,valign=center,
  colback=red!5!white,colframe=red!75!black,
  frame style={circular glow={fill=red}} ]
  tcolorbox
\end{tcolorbox}
\end{exdispExample*}


\clearpage
\subsection{\tikzname\  Picture Option Keys}\label{subsec:tikzpicture}
The following general options are applicable for skins which
use |tikzpicture| as \refKey{/tcb/graphical environment}.
Therefore, the skin \refSkin{standard} does not support these options,
but most other skins, e.\,g.\ \refSkin{enhanced}.


\begin{docTcbKey}{tikz}{=\meta{tikz option list}}{no default, initially empty}
  Adds the given \meta{tikz option list} to the main |tikzpicture| environment
  used to draw the color box, see \cite{tantau:tikz_and_pgf}. If this option is
  applied a second time, the new \meta{tikz option list} is appended to the
  current option list.
\begin{dispExample*}{sbs,lefthand ratio=0.66,
  segmentation style={preaction={fill=white},pattern=checkerboard,pattern color=gray!40}}
\tcbset{enhanced,colback=red!5!white,
  colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[title=Transparent box,
  tikz={opacity=0.5,transparency group}]
This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}

\begin{dispExample*}{sbs,lefthand ratio=0.66}
\tcbset{enhanced,colback=red!5!white,
  colframe=red!75!black,fonttitle=\bfseries,
  fontupper=\bfseries\Huge,
  halign title=center,halign=center}

\begin{tcolorbox}[title=Rotated box,
  tikz={rotate=30}]
Sold!
\end{tcolorbox}
\end{dispExample*}

\end{docTcbKey}


\begin{docTcbKey}{tikz reset}{}{initially set}
  Removes all options given by \refKey{/tcb/tikz}.
\end{docTcbKey}


\begin{docTcbKey}{at begin tikz}{=\meta{tikz code}}{no default, initially empty}
  The given \meta{tikz code} is executed at the beginning of the |tikzpicture| environment
  after the \tikzname\  option |execute at begin picture| was applied.
  If this option is applied a second time, the new \meta{tikz code} is appended to the current code.
\end{docTcbKey}


\begin{docTcbKey}{at begin tikz reset}{}{initially set}
  Removes all code given by \refKey{/tcb/at begin tikz}.
\end{docTcbKey}


\begin{docTcbKey}{at end tikz}{=\meta{tikz code}}{no default, initially empty}
  The given \meta{tikz code} is executed at the ending of the |tikzpicture| environment
  before the \tikzname\  option |execute at end picture| was applied.
  If this option is applied a second time, the new \meta{tikz code} is appended to the current code.
\end{docTcbKey}


\begin{docTcbKey}{at end tikz reset}{}{initially set}
  Removes all code given by \refKey{/tcb/at end tikz}.
\end{docTcbKey}


\clearpage
\begin{docTcbKey}{rotate}{=\meta{angle}}{no default, initially unset}
  Rotates the |tcolorbox| by the given \meta{angle}. Note that this is
  a \tikzname\  coordinate transformation i.e. not all graphical elements like shadings
  will really be rotated.
\begin{dispExample*}{sbs,lefthand ratio=0.66}
\tcbset{enhanced,colback=red!5!white,
  colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[title=Rotated box,rotate=30]
This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}

\begin{docTcbKey}{scale}{=\meta{fraction}}{no default, initially unset}
  Scales the |tcolorbox| by the given \meta{fraction}. Note that this is
  a \tikzname\  coordinate transformation i.e. not all graphical elements like line widths
  will really be scaled.
\begin{dispExample*}{sbs,lefthand ratio=0.66}
\tcbset{enhanced,colback=red!5!white,
  colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[title=Scaled box,scale=0.5]
This is a tcolorbox.
\end{tcolorbox}
\begin{tcolorbox}[title=Scaled box,scale=1.25]
This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}


\begin{docTcbKey}{remember}{}{style, initially unset}
  Shortcut for |tikz={remember picture}|. This allows one to reference nodes
  in other \tikzname\  pictures.
\begin{dispExample}
\begin{tcolorbox}[enhanced,remember,colback=red!5!white,colframe=red!75!black,
  fonttitle=\bfseries,title=The four corners of a paper,
  overlay={\draw[red!50!white,line width=1mm,opacity=0.5,shorten >=3mm]
    (frame.north west) edge[->] (current page.north west)
    (frame.north east) edge[->] (current page.north east)
    (frame.south west) edge[->] (current page.south west)
    (frame.south east) edge[->] (current page.south east);}]
This is a tcolorbox.
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}

\clearpage
\tcbinterruptdraftmode%
\begin{docTcbKey}{remember as}{=\meta{name}}{style, no default, initially unset}
  The |frame| node will be remembered by the given \meta{name} to be referenced
  in other \tikzname\  pictures.
\begin{dispExample}
% \usepackage{lipsum}
\newtcolorbox{mybox}[1][]{enhanced,colframe=blue!75!black,colback=blue!10!white,
  fonttitle=\bfseries,#1}

\begin{mybox}[title=First Box,nobeforeafter,width=\linewidth/4,remember as=one]
This is a test.
\end{mybox}
\hfill
\begin{mybox}[title=Second Box,nobeforeafter,width=\linewidth/4,remember as=two]
This is a test.
\end{mybox}
\hfill
\begin{mybox}[title=Third Box,nobeforeafter,width=\linewidth/4,remember as=three]
This is a test.
\end{mybox}

\lipsum[2]

\begin{mybox}[title=Fourth Box,remember as=four]
This is a test.
\end{mybox}

\begin{tikzpicture}[overlay,remember picture,line width=1mm,draw=red!75!black]
  \draw[->] (one.east) to[bend right] node[above] {A} (two.west);
  \draw[->] (two.east) to[bend left] node[above] {B} (three.west);
  \draw[->] (three.east) to[bend left=90] node[right] {C} (four.east);
  \draw[->] (four.west) to[bend left=90] node[left] {D} (one.west);
\end{tikzpicture}
\end{dispExample}
\end{docTcbKey}
\tcbcontinuedraftmode%


\clearpage
\subsection{Underlay Option Keys}\label{subsec:skinunderlay}

Underlays are quite similar to overlays described in \Vref{subsec:overlays}.
Underlays are drawn \emph{after} the frame and interior are
drawn and \emph{before} overlays and the text content is drawn; see
\Vref{subsec:tcolorboxdrawing} for the general drawing scheme.

The differences between underlays and overlays are:
\begin{itemize}
\item Underlays are not applicable for the skins
  \refSkin{standard} and
  \refSkin{standard jigsaw},
  whereas overlays are applicable also for these skins.
  The skin \refSkin{spartan} supports underlays but no overlays.
  \begin{marker}
  If an underlay is used with the \refSkin{standard} skin, it is silently ignored.
  \end{marker}
\item Underlays are stackable, i.\,e.\ several different underlays can be
  used on the same |tcolorbox|. Overlays are not stackable by default (but with
  some help of the library \mylib{hooks}).
\item Boxed titles are implemented with underlays (\Vref{subsec:skinboxedtitle}),
  watermarks are implemented with overlays (\Vref{subsec:watermarks}).
\end{itemize}


\begin{docTcbKey}{underlay}{=\meta{graphical code}}{no default, initially unset}
  Adds \meta{graphical code} to the box drawing process. This \meta{graphical code}
  is drawn \emph{after} the frame and interior and \emph{before} the text content.
\begin{dispExample}
\newtcolorbox{mybox}[1][]{enhanced,colback=red!5!white,
  colbacktitle=red!85!black!50!white,
  colframe=red!75!black,fonttitle=\bfseries,watermark color=yellow!50!white,
  underlay={\begin{tcbclipinterior}
    \draw[red!40!white,line width=1cm] (interior.south west)--(interior.north east);
    \end{tcbclipinterior}},
  attach boxed title to top center={yshift=-2mm},#1}

\begin{mybox}[title=My box,watermark text=My Watermark]
\lipsum[2]
\end{mybox}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{no underlay}{}{style, no default, initially set}
  Removes the underlay if set before.
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{underlay broken}{=\meta{graphical code}}{no default, initially unset}
  If the box is set to be \refKey{/tcb/breakable} and \emph{is} broken actually,
  then the \meta{graphical code} is added to the box drawing process.
  \refKey{/tcb/underlay} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}{underlay unbroken}{=\meta{graphical code}}{no default, initially unset}
  If the box is set to be \refKey{/tcb/breakable} but \emph{is not} broken actually
  or if the box is set to be \refKey{/tcb/unbreakable},
  then the \meta{graphical code} is added to the box drawing process.
  \refKey{/tcb/underlay} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}{no underlay unbroken}{}{style, no default, initially set}
  Removes the unbroken underlay if set before.
\end{docTcbKey}

\begin{docTcbKey}{underlay first}{=\meta{graphical code}}{no default, initially unset}
  If the box is set to be \refKey{/tcb/breakable} and \emph{is} broken actually,
  then the \meta{graphical code} is added to the box drawing process for
  the \emph{first} part of the break sequence.
  \refKey{/tcb/underlay} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}{no underlay first}{}{style, no default, initially set}
  Removes the first underlay if set before.
\end{docTcbKey}

\begin{docTcbKey}{underlay middle}{=\meta{graphical code}}{no default, initially unset}
  If the box is set to be \refKey{/tcb/breakable} and \emph{is} broken actually,
  then the \meta{graphical code} is added to the box drawing process for
  the \emph{middle} parts (if any) of the break sequence.
  \refKey{/tcb/underlay} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}{no underlay middle}{}{style, no default, initially set}
  Removes the middle underlay if set before.
\end{docTcbKey}

\begin{docTcbKey}{underlay last}{=\meta{graphical code}}{no default, initially unset}
  If the box is set to be \refKey{/tcb/breakable} and \emph{is} broken actually,
  then the \meta{graphical code} is added to the box drawing process for
  the \emph{last} part of the break sequence.
  \refKey{/tcb/underlay} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}{no underlay last}{}{style, no default, initially set}
  Removes the last underlay if set before.
\end{docTcbKey}

\begin{docTcbKey}{underlay boxed title}{=\meta{graphical code}}{no default, initially unset}
  If the box has a \emph{boxed title}, see \Vref{subsec:skinboxedtitle},
  then the \meta{graphical code} is added to the box drawing process
  \emph{before} the boxed title is drawn.
\end{docTcbKey}

\begin{docTcbKey}{no underlay boxed title}{}{style, no default, initially set}
  Removes the boxed title underlay if set before.
\end{docTcbKey}

\begin{docTcbKey}{underlay unbroken and first}{=\meta{graphical code}}{no default, initially unset}
  This is an abbreviation for setting
  \refKey{/tcb/underlay unbroken} and
  \refKey{/tcb/underlay first} together.
  \refKey{/tcb/underlay} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}{underlay middle and last}{=\meta{graphical code}}{no default, initially unset}
  This is an abbreviation for setting
  \refKey{/tcb/underlay middle} and
  \refKey{/tcb/underlay last} together.
  \refKey{/tcb/underlay} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}{underlay unbroken and last}{=\meta{graphical code}}{no default, initially unset}
  This is an abbreviation for setting
  \refKey{/tcb/underlay unbroken} and
  \refKey{/tcb/underlay last} together.
  \refKey{/tcb/underlay} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-09-19]{underlay first and middle}{=\meta{graphical code}}{no default, initially unset}
  This is an abbreviation for setting
  \refKey{/tcb/underlay first} and
  \refKey{/tcb/underlay middle} together.
  \refKey{/tcb/underlay} overwrites this key.
\end{docTcbKey}


\clearpage
\subsection{Finish Option Keys}\label{subsec:skinfinish}

Finishes are quite similar to underlays described in \Vref{subsec:skinunderlay}
and overlays described in \Vref{subsec:overlays}.
Finishes are drawn \emph{after} the text content is drawn; see
\Vref{subsec:tcolorboxdrawing} for the general drawing scheme.
Therefore, a finish will reduce the readability of the text content.

Finishes are intended for special effects like highlights or glosses or text over text.

\begin{itemize}
\item Finishes are only applicable for the skins
  \refSkin{enhanced},
  \refSkin{empty},
  \refSkin{freelance},
  \refSkin{bicolor},
  \refSkin{beamer}, and
  \refSkin{widget}.
  \begin{marker}
  If a finish is used with the \refSkin{standard} skin, it is silently ignored.
  \end{marker}
\item Finishes are stackable, i.\,e.\ several different finishes can be
  used on the same |tcolorbox|.
\end{itemize}

\enlargethispage*{2cm}
\begin{docTcbKey}{finish}{=\meta{graphical code}}{no default, initially unset}
  Adds \meta{graphical code} to the box drawing process. This \meta{graphical code}
  is drawn \emph{after} the text content.
\begin{dispExample}
\newtcolorbox{mybox}[1][]{enhanced,colback=red!5!white,
  colbacktitle=red!85!black!50!white,colframe=red!75!black,fonttitle=\bfseries,
  finish={\begin{tcbclipframe}
    \path[bottom color=black,top color=black!50!white,opacity=0.1]
      (frame.south west) -- (frame.south east) -- (frame.north east) -- cycle;
    \path[top color=white,bottom color=black!50!white,opacity=0.1]
      (frame.south west) -- (frame.north east) -- (frame.north west) -- cycle;
    \end{tcbclipframe}},#1}

\begin{mybox}[title=My box]
\lipsum[2]
\end{mybox}
\end{dispExample}
\begin{dispExample}
\newtcolorbox{mybox}[1][]{enhanced,colback=red!5!white,
  colbacktitle=red!85!black!50!white,colframe=red!75!black,fonttitle=\bfseries,
  finish={\node[draw,fill=white,fill opacity=0.85,inner sep=5mm,
    rounded corners] at (frame.center) {\Huge\bfseries Finish!};},#1}

\begin{mybox}[title=My box]
\lipsum[2]
\end{mybox}
\end{dispExample}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{no finish}{}{style, no default, initially set}
  Removes the finish if set before.
\end{docTcbKey}


\begin{docTcbKey}{finish broken}{=\meta{graphical code}}{no default, initially unset}
  If the box is set to be \refKey{/tcb/breakable} and \emph{is} broken actually,
  then the \meta{graphical code} is added to the box drawing process.
  \refKey{/tcb/finish} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}{finish unbroken}{=\meta{graphical code}}{no default, initially unset}
  If the box is set to be \refKey{/tcb/breakable} but \emph{is not} broken actually
  or if the box is set to be \refKey{/tcb/unbreakable},
  then the \meta{graphical code} is added to the box drawing process.
  \refKey{/tcb/finish} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}{no finish unbroken}{}{style, no default, initially set}
  Removes the unbroken finish if set before.
\end{docTcbKey}

\begin{docTcbKey}{finish first}{=\meta{graphical code}}{no default, initially unset}
  If the box is set to be \refKey{/tcb/breakable} and \emph{is} broken actually,
  then the \meta{graphical code} is added to the box drawing process for
  the \emph{first} part of the break sequence.
  \refKey{/tcb/finish} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}{no finish first}{}{style, no default, initially set}
  Removes the first finish if set before.
\end{docTcbKey}

\begin{docTcbKey}{finish middle}{=\meta{graphical code}}{no default, initially unset}
  If the box is set to be \refKey{/tcb/breakable} and \emph{is} broken actually,
  then the \meta{graphical code} is added to the box drawing process for
  the \emph{middle} parts (if any) of the break sequence.
  \refKey{/tcb/finish} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}{no finish middle}{}{style, no default, initially set}
  Removes the middle finish if set before.
\end{docTcbKey}

\begin{docTcbKey}{finish last}{=\meta{graphical code}}{no default, initially unset}
  If the box is set to be \refKey{/tcb/breakable} and \emph{is} broken actually,
  then the \meta{graphical code} is added to the box drawing process for
  the \emph{last} part of the break sequence.
  \refKey{/tcb/finish} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}{no finish last}{}{style, no default, initially set}
  Removes the last finish if set before.
\end{docTcbKey}

\begin{docTcbKey}{finish unbroken and first}{=\meta{graphical code}}{no default, initially unset}
  This is an abbreviation for setting
  \refKey{/tcb/finish unbroken} and
  \refKey{/tcb/finish first} together.
  \refKey{/tcb/finish} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}{finish middle and last}{=\meta{graphical code}}{no default, initially unset}
  This is an abbreviation for setting
  \refKey{/tcb/finish middle} and
  \refKey{/tcb/finish last} together.
  \refKey{/tcb/finish} overwrites this key.
\end{docTcbKey}

\begin{docTcbKey}{finish unbroken and last}{=\meta{graphical code}}{no default, initially unset}
  This is an abbreviation for setting
  \refKey{/tcb/finish unbroken} and
  \refKey{/tcb/finish last} together.
  \refKey{/tcb/finish} overwrites this key.
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2014-09-19]{finish first and middle}{=\meta{graphical code}}{no default, initially unset}
  This is an abbreviation for setting
  \refKey{/tcb/finish first} and
  \refKey{/tcb/finish middle} together.
  \refKey{/tcb/finish} overwrites this key.
\end{docTcbKey}

\clearpage
\subsection{Hyper Option Keys}\label{subsec:hyper}
All options of this section need the package |hyperref| \cite{rahtz:hyperref}
to be loaded separately. All these options are implemented as
\refKey{/tcb/finish} and can be disabled by \refKey{/tcb/no finish}.

\begin{marker}
If the package |hyperref| \cite{rahtz:hyperref} is not loaded or if
the \refSkin{standard} skin is used, all hyper option are silently ignored.
\end{marker}

\begin{docTcbKey}[][doc new=2017-02-03]{hyperref}{=\meta{marker}}{no default, initially unset}
  The whole \textit{frame} of a |tcolorbox| is make an active hyperlink for a
  \meta{marker} which was given by |\label| or \refKey{/tcb/label} or \refKey{/tcb/phantomlabel}.
  Such, the |tcolorbox| is made a clickable button (depending on the previewer).
  \begin{dispExample*}{sbs,lefthand ratio=0.7}
% \section{Library skins}\label{sec:skins}%
\begin{tcolorbox}[beamer,colback=red!50,
  hyperref=sec:skins]
Jump to the heading of Section~\ref*{sec:skins}.
\end{tcolorbox}
  \end{dispExample*}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2017-02-03]{hyperref interior}{=\meta{marker}}{no default, initially unset}
  Identical to \refKey{/tcb/hyperref}, but only the \textit{interior} of a
  |tcolorbox| is made a hyperlink (without frame and title).
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2017-02-03]{hyperref title}{=\meta{marker}}{no default, initially unset}
  Identical to \refKey{/tcb/hyperref}, but only the \textit{title} of a
  |tcolorbox| is made a hyperlink.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2017-02-03]{hyperref node}{=\marg{marker}\marg{node}}{no default, initially unset}
  Identical to \refKey{/tcb/hyperref}, but only the given \tikzname\ \meta{node}
  is made a hyperlink. This \meta{node} may be |frame|, |interior|, |title|, or
  any other named node used for drawing the |tcolorbox|.
  The \meta{node} may be defined inside
  \refKey{/tcb/underlay}, \refKey{/tcb/overlay} or \refKey{/tcb/finish}.
  If the later is used, define the node \emph{before} \refKey{/tcb/hyperref node}
  is applied.
  \begin{dispExample*}{sbs,lefthand ratio=0.7}
% \section{Library skins}\label{sec:skins}%
\begin{tcolorbox}[enhanced,colback=yellow!10,
  underlay={\node[red,fill=red!30,inner sep=3mm]
   (click) at (frame.center) {X};},
  hyperref node={sec:skins}{click}]
Jump to the heading of Section~\ref*{sec:skins}
(X marks the click point).
\end{tcolorbox}
  \end{dispExample*}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2017-02-03]{hyperlink}{=\meta{marker}}{no default, initially unset}
  The whole \textit{frame} of a |tcolorbox| is make an active hyperlink for a
  \meta{marker} which was given by |\hypertarget| or \refKey{/tcb/hypertarget}.
  Such, the |tcolorbox| is made a clickable button (depending on the previewer).
  \begin{dispExample*}{sbs,lefthand ratio=0.7}
% \usepackage{hyperref}%
\begin{tcolorbox}[enhanced,
  colback=blue!10,colframe=blue!50!black,
  hypertarget=hypertwinB,
  hyperlink=hypertwinA,
  title=Box B]
Click me to jump to Box A.
\end{tcolorbox}
  \end{dispExample*}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}[][doc new=2017-02-03]{hyperlink interior}{=\meta{marker}}{no default, initially unset}
  Identical to \refKey{/tcb/hyperlink}, but only the \textit{interior} of a
  |tcolorbox| is made a hyperlink (without frame and title).
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2017-02-03]{hyperlink title}{=\meta{marker}}{no default, initially unset}
  Identical to \refKey{/tcb/hyperlink}, but only the \textit{title} of a
  |tcolorbox| is made a hyperlink.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2017-02-03]{hyperlink node}{=\marg{marker}\marg{node}}{no default, initially unset}
  Identical to \refKey{/tcb/hyperlink}, but only the given \tikzname\ \meta{node}
  is made a hyperlink. This \meta{node} may be |frame|, |interior|, |title|, or
  any other named node used for drawing the |tcolorbox|.
  The \meta{node} may be defined inside
  \refKey{/tcb/underlay}, \refKey{/tcb/overlay} or \refKey{/tcb/finish}.
  If the later is used, define the node \emph{before} \refKey{/tcb/hyperlink node}
  is applied.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2017-02-03]{hyperurl}{=\meta{url}}{no default, initially unset}
  The whole \textit{frame} of a |tcolorbox| is make an active hyperlink for an
  \meta{url} in the same manner as using |\href| or |\url|.
  Such, the |tcolorbox| is made a clickable button (depending on the previewer).
  \begin{dispExample*}{sbs,lefthand ratio=0.7}
\begin{tcolorbox}[enhanced,colback=red!50,
  hyperurl=https://www.ctan.org/pkg/tcolorbox]
View CTAN with a browser.
\end{tcolorbox}
  \end{dispExample*}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2017-02-03]{hyperurl interior}{=\meta{url}}{no default, initially unset}
  Identical to \refKey{/tcb/hyperurl}, but only the \textit{interior} of a
  |tcolorbox| is made a hyperlink (without frame and title).
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2017-02-03]{hyperurl title}{=\meta{url}}{no default, initially unset}
  Identical to \refKey{/tcb/hyperurl}, but only the \textit{title} of a
  |tcolorbox| is made a hyperlink.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2017-02-03]{hyperurl node}{=\marg{url}\marg{node}}{no default, initially unset}
  Identical to \refKey{/tcb/hyperurl}, but only the given \tikzname\ \meta{node}
  is made a hyperlink. This \meta{node} may be |frame|, |interior|, |title|, or
  any other named node used for drawing the |tcolorbox|.
  The \meta{node} may be defined inside
  \refKey{/tcb/underlay}, \refKey{/tcb/overlay} or \refKey{/tcb/finish}.
  If the later is used, define the node \emph{before} \refKey{/tcb/hyperurl node}
  is applied.
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2017-02-03]{hyperurl*}{=\marg{options}\marg{url}}{no default, initially unset}
  Identical to \refKey{/tcb/hyperurl}, but additional |hyperref| \cite{rahtz:hyperref}
  \meta{options} are applied.
  \begin{dispExample*}{sbs,lefthand ratio=0.7}
\begin{tcolorbox}[enhanced,colback=green!50,
  hyperurl*={page=3,pdfnewwindow=true}%
            {tcolorbox-example.pdf}]
Open example file on Page~3.
\end{tcolorbox}
  \end{dispExample*}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2017-02-03]{hyperurl* interior}{=\marg{options}\marg{url}}{no default, initially unset}
  Identical to \refKey{/tcb/hyperurl interior}, but additional |hyperref| \cite{rahtz:hyperref}
  \meta{options} are applied.
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2017-02-03]{hyperurl* title}{=\marg{options}\marg{url}}{no default, initially unset}
  Identical to \refKey{/tcb/hyperurl title}, but additional |hyperref| \cite{rahtz:hyperref}
  \meta{options} are applied.
\end{docTcbKey}

\enlargethispage*{1cm}

\begin{docTcbKey}[][doc new=2017-02-03]{hyperurl* node}{=\marg{options}\marg{url}\marg{node}}{no default, initially unset}
  Identical to \refKey{/tcb/hyperurl node}, but additional |hyperref| \cite{rahtz:hyperref}
  \meta{options} are applied.
\end{docTcbKey}



\clearpage
\subsection{Jigsaw Skin Variants}\label{subsec:skinjigsaw}
As described in \Vref{sec:skincorekeys}, a |tcolorbox| is drawn by up to
four \emph{engines}. Typically, the \emph{frame} engine fills the complete box area
with color and the other engines fill certain areas with other colors.
Finally, only the area which you see as \emph{frame} of the box will display
the frame color. For most applications, this is a good approach.

For certain boxes, a more delicate procedure is needed. E.g., if the box should
be translucent, an already painted area cannot be made unpainted. Therefore,
more elaborate frame engines saw holes into the frame where the interior area and
optionally the title area will be painted.
The resulting skins are called \emph{jigsaw} skins. For \refSkin{standard}
and \refSkin{enhanced}, there are variants called \refSkin{standard jigsaw}
and \refSkin{enhanced jigsaw}.


\begin{dispExample*}{segmentation style={preaction={fill=white},pattern=checkerboard,pattern color=gray!40}}
\newcommand{\ballexample}{\begin{tikzpicture}
  \path[use as bounding box] (0,0.8) rectangle +(0.1,0.1);
  \shadedraw [shading=ball] (0,0) circle (1cm);
  \shadedraw [ball color=red] (3,-2.2) circle (1cm);
\end{tikzpicture}}

\tcbset{enhanced,colback=blue!5!white,
  frame style={left color=red!75!black,right color=red!10!yellow},
  fonttitle=\bfseries }

\ballexample

\begin{tcolorbox}[title=A normal box]
  \lipsum[2]
\end{tcolorbox}

\ballexample

\begin{tcolorbox}[title=A translucent jigsaw box,
  enhanced jigsaw,opacityback=0.35]
  \lipsum[2]
\end{tcolorbox}
\end{dispExample*}


\begin{dispExample*}{segmentation style={preaction={fill=white},pattern=checkerboard,pattern color=gray!40}}
\tcbset{enhanced,colback=red!10!white,coltitle=black,
  frame style={left color=red!75!black,right color=red!10!yellow},
  fonttitle=\bfseries,interior hidden,title hidden}

\begin{tcolorbox}[title=A normal box with hidden interior and title]
  This is a tcolorbox.
\end{tcolorbox}

\begin{tcolorbox}[enhanced jigsaw,
  title=A jigsaw box with hidden interior and title]
  This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}


\begin{dispExample*}{segmentation style={preaction={fill=white},pattern=checkerboard,pattern color=gray!40}}
\newtcolorbox{mybox}{skin=enhancedmiddle jigsaw,leftrule=5mm,rightrule=5mm,
  boxsep=0mm,top=0mm,bottom=0mm,
  frame style={top color=blue,bottom color=red},interior hidden}

\begin{mybox}
  \lipsum[2]
\end{mybox}
\end{dispExample*}


\clearpage
\subsection{Draft Mode}\label{subsec:draftmode}
To reduce the compiliation time while drafting a document, the \emph{draft mode}
can be applied. Basically, it changes all skins to \refSkin{spartan} and
sets the \refKey{/tcb/fit algorithm} to |squeeze|. Especially,
when fuzzy shadows are used, the speedup will be considerable high.

\begin{marker}
It is strongly recommended that the draft mode is \emph{not} used for the final document.
Use \refSkin{spartan} directly, if you want to stay with it. The draft mode
implementation may change in future.
\end{marker}

\begin{marker}
Normally, switching to the draft mode should not alter the geometry of
your document. Since overlays are deactivated, any code placed there
(e.g. counter changes) is not executed anymore! Also, \refKey{/tcb/remember as}
will not have any effect. You may exclude critical code with
\refCom{tcbinterruptdraftmode} / \refCom{tcbcontinuedraftmode}
from converting to draft mode.
\end{marker}


\begin{docCommand}{tcbstartdraftmode}{}
  Any following |tcolorbox| code is put into \emph{draft mode}. All skin
  settings are overruled with \refSkin{spartan}. Overlays, watermarks,
  shadows, borderlines, and rounded corners are deactivated for all |tcolorbox|
  layers.
\end{docCommand}

\begin{docCommand}{tcbstopdraftmode}{}
  The \emph{draft mode} is deactivated for the following code.
\end{docCommand}

\begin{docCommand}{tcbinterruptdraftmode}{}
  If the compilation is in \emph{draft mode}, the \emph{draft mode} is deactivated
  until a following \refCom{tcbcontinuedraftmode} is detected.\par
  If the compilation is not in \emph{draft mode}, nothing happens and a following
  \refCom{tcbcontinuedraftmode} will not start the \emph{draft mode}.
  \begin{marker}
  The pair |\tcbinterruptdraftmode| and |\tcbcontinuedraftmode| cannot
  be used nested.
  \end{marker}
\end{docCommand}

\begin{docCommand}{tcbcontinuedraftmode}{}
  Continues the \emph{draft mode} which was suspended by a preceding
  \refCom{tcbinterruptdraftmode}. Nothing happens, if there was no draft
  mode before \refCom{tcbinterruptdraftmode}.
  \begin{marker}
  Code, which is place between \refCom{tcbinterruptdraftmode} and
  \refCom{tcbcontinuedraftmode} is shielded from \emph{draft mode}.
  \end{marker}
\end{docCommand}


\clearpage

\begin{docTcbKey}{draftmode}{\colOpt{=true\textbar false}}{default |true|, initially |false|}
  If set to |true|, the \emph{draft mode} is started.
  If set to |false|, the \emph{draft mode} is stopped.

\begin{dispExample*}{}
\newtcolorbox{mybeamer}[2][]{beamer,colback=Salmon!50!white,
  colframe=FireBrick!75!black,adjusted title={#2},#1}

\begin{mybeamer}{Beamer box}
This box looks like a box provided by the \texttt{beamer} class.
\end{mybeamer}\par\medskip
\begin{mybeamer}[draftmode]{Beamer box}
This box looks like a box provided by the \texttt{beamer} class.
\end{mybeamer}
\end{dispExample*}
\end{docTcbKey}



\clearpage
\tcbset{skintable/.style={colframe=red!50!yellow!50!black,
  colback=red!50!yellow!5!white,coltitle=red!50!yellow!3!white,
  fonttitle=\bfseries,before=\par\smallskip,
  title=Environment and engines for the skin '\texttt{#1}'}}

\subsection{Skin Family 'standard'}\label{subsec:skinstandard}
\begin{marker}Note that the option keys \refKey{/tcb/frame style},
  \refKey{/tcb/interior style},
  \refKey{/tcb/segmentation style}, and
  \refKey{/tcb/title style} are not be applicable to the standard skin.
  Also, watermarks (see Subsection \ref{subsec:watermarks})
  are not usable with the standard skin.
\end{marker}

\begin{docSkin}{standard}
  This is the standard skin from the core package. All drawing engines
  are set to type |standard|. The drawing is based on |pgf| commands and
  does not need the |tikz| package.
\begin{tcolorbox}[skintable=standard]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |pgfpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |standard|\\
    \refKey{/tcb/interior titled engine}: \> |standard|\\ 
    \refKey{/tcb/interior engine}:        \> |standard|\\
    \refKey{/tcb/segmentation engine}:    \> |standard|\\
    \refKey{/tcb/title engine}:           \> |standard|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}

\begin{docTcbKey}{standard}{}{style, no value}
  This is an abbreviation for setting |skin=standard|.
\end{docTcbKey}

\begin{dispExample}
\begin{tcbraster}[standard,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,colbacktitle=LimeGreen!75!DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}


\clearpage

\begin{docSkin}{standard jigsaw}
  This is the standard jigsaw skin from the core package. It differs from
  the skin \refSkin{standard} by its frame engine, see \Vref{subsec:skinjigsaw}.
\begin{tcolorbox}[skintable=standard jigsaw]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |pgfpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |standardjigsaw|\\
    \refKey{/tcb/interior titled engine}: \> |standard|\\ 
    \refKey{/tcb/interior engine}:        \> |standard|\\
    \refKey{/tcb/segmentation engine}:    \> |standard|\\
    \refKey{/tcb/title engine}:           \> |standard|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}

\begin{docTcbKey}{standard jigsaw}{}{style, no value}
  This is an abbreviation for setting |skin=standard jigsaw|.
\end{docTcbKey}

\begin{dispExample*}{segmentation style={preaction={fill=white},pattern=checkerboard,pattern color=gray!40}}
\begin{tcbraster}[standard jigsaw,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,colbacktitle=LimeGreen!75!DarkGreen,
    opacityframe=0.5,opacityback=0.5,opacitybacktitle=0.5,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample*}


\clearpage
\subsection{Skin Family 'enhanced'}
\begin{marker}
If you like the standard appearance of a |tcolorbox| but you want to
have some 'enhanced' features, the |enhanced| skin is what you are looking for.
\end{marker}

\begin{docSkin}{enhanced}
  This skin translates the drawing commands of the core package into |tikz|
  path commands. Therefore, it allows all |tikz| high level options for
  these paths and has more flexibility compared to the \refSkin{standard} skin.
  You pay for this with some prolonged compilation time.
  The |tikz| path options can
  be given with the option keys
  \refKey{/tcb/frame style},
  \refKey{/tcb/interior style},
  \refKey{/tcb/segmentation style}, and
  \refKey{/tcb/title style}.
\begin{tcolorbox}[skintable=enhanced]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |path|\\
    \refKey{/tcb/interior titled engine}: \> |path|\\ 
    \refKey{/tcb/interior engine}:        \> |path|\\
    \refKey{/tcb/segmentation engine}:    \> |path|\\
    \refKey{/tcb/title engine}:           \> |path|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}


\begin{docTcbKey}{enhanced}{}{style, no value}
  This is an abbreviation for setting |skin=enhanced|.
\end{docTcbKey}

\begin{dispExample}
\begin{tcbraster}[enhanced,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,colbacktitle=LimeGreen!75!DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}

\begin{dispExample}
% \usetikzlibrary{shadings}         % preamble
\tcbset{skin=enhanced,fonttitle=\bfseries,
  frame style={upper left=blue,upper right=red,lower left=yellow,lower right=green},
  interior style={white,opacity=0.5},
  segmentation style={black,solid,opacity=0.2,line width=1pt}}

\begin{tcolorbox}[title=Nice box in rainbow colors]
  With the 'enhanced' skin, it is quite easy to produce fancy looking effects.
  \tcblower
  Note that this is still a \texttt{tcolorbox}.
\end{tcolorbox}
\end{dispExample}


\begin{dispExample}
% \usetikzlibrary{decorations.pathmorphing} % preamble
\tcbset{skin=enhanced,fonttitle=\bfseries,boxrule=1mm,
  frame style={draw=FireBrick,fill=Salmon},drop fuzzy shadow,
  interior style={draw=FireBrick,top color=Salmon!10,bottom color=Salmon!20},
  segmentation style={draw=FireBrick,solid,decorate,
        decoration={coil,aspect=0,segment length=10.1mm}}}

\begin{tcblisting}{title=A listing box with shadow and some specials}
Of course, skins can be used for listings also.
\begin{equation}
  \int\limits_1^2 \frac{1}{x}~dx = \ln(2).
\end{equation}
\end{tcblisting}
\end{dispExample}


\clearpage


\begin{docTcbKey}{enhanced standard}{}{style, no value}
  For unbreakable boxes, this is identical to using \refKey{/tcb/enhanced}.
  But, for breakable boxes, the \emph{break sequence} is identical to the \refSkin{standard} skin,
  see Section \ref{subsec:breaksequence} from page \pageref{subsec:breaksequence}.
\end{docTcbKey}


\begin{docTcbKey}{blank}{}{style, initially unset}
  This style relies on the skin \refSkin{enhanced}. All drawing operations
  are hidden and all margins are set to |0pt|. See \refKey{/tcb/blanker}
  for switching off the drawing engines.
\begin{dispExample}
\begin{tcolorbox}[blank,watermark text=A blank box]
\lipsum[1]
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}

\clearpage
\begin{docCommand}{tcbline}{}
  Sometimes, a line is only a line. With \refCom{tcblower} you separate
  the box content into two functional units. |\tcbline| draws only a line
  which looks like the segmentation line between upper and lower part.
  Furthermore, you can use |\tcbline| more than just once.
  |\tcbline| always uses the |path| drawing engine. Therefore,
  the \refKey{/tcb/segmentation style} can be applied.

\begin{dispExample}
\tcbset{enhanced,colframe=blue!50!black,colback=white}

\begin{tcolorbox}[colupper=red!50!black,collower=green!50!black]
\lipsum[1]
\tcbline
\lipsum[2]
\tcblower
\lipsum[3]
\tcbline
\lipsum[4]
\end{tcolorbox}
\end{dispExample}
\end{docCommand}

\begin{docCommand}{tcbline*}{}
  Equivalent to \refCom{tcbline}, but in a breakable box, \refCom{tcbline*}
  is removed if at a page/box break. Also, it is removed at the end
  of a box.
\end{docCommand}

\clearpage
\begin{docSkin}{enhancedfirst}
This is a flavor of \refSkin{enhanced} which is used as a \emph{first} part
in a break sequence for \refSkin{enhanced}.
Nevertheless, this skin can be applied independently.
\begin{tcolorbox}[skintable=enhancedfirst]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |pathfirst|\\
    \refKey{/tcb/interior titled engine}: \> |pathfirst|\\ 
    \refKey{/tcb/interior engine}:        \> |pathfirst|\\
    \refKey{/tcb/segmentation engine}:    \> |path|\\
    \refKey{/tcb/title engine}:           \> |pathfirst|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}


\begin{dispExample}
\begin{tcbraster}[skin=enhancedfirst,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,colbacktitle=LimeGreen!75!DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}



\clearpage
\begin{docSkin}{enhancedmiddle}
This is a flavor of \refSkin{enhanced} which is used as a \emph{middle} part
in a break sequence for \refSkin{enhanced}.
Nevertheless, this skin can be applied independently.
\begin{tcolorbox}[skintable=enhancedmiddle]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |pathmiddle|\\
    \refKey{/tcb/interior titled engine}: \> |pathmiddle|\\ 
    \refKey{/tcb/interior engine}:        \> |pathmiddle|\\
    \refKey{/tcb/segmentation engine}:    \> |path|\\
    \refKey{/tcb/title engine}:           \> |pathmiddle|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}


\begin{dispExample}
\begin{tcbraster}[skin=enhancedmiddle,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,colbacktitle=LimeGreen!75!DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}




\clearpage
\begin{docSkin}{enhancedlast}
This is a flavor of \refSkin{enhanced} which is used as a \emph{last} part
in a break sequence for \refSkin{enhanced}.
Nevertheless, this skin can be applied independently.
\begin{tcolorbox}[skintable=enhancedlast]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |pathlast|\\
    \refKey{/tcb/interior titled engine}: \> |pathlast|\\ 
    \refKey{/tcb/interior engine}:        \> |pathlast|\\
    \refKey{/tcb/segmentation engine}:    \> |path|\\
    \refKey{/tcb/title engine}:           \> |pathlast|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}

\begin{dispExample}
\begin{tcbraster}[skin=enhancedlast,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,colbacktitle=LimeGreen!75!DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}


\clearpage
\begin{docSkin}{enhanced jigsaw}
  This is the jigsaw variant of skin \refSkin{enhanced}.
  It differs by its frame engine, see \Vref{subsec:skinjigsaw}.
\begin{tcolorbox}[skintable=enhanced jigsaw]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |pathjigsaw|\\
    \refKey{/tcb/interior titled engine}: \> |path|\\ 
    \refKey{/tcb/interior engine}:        \> |path|\\
    \refKey{/tcb/segmentation engine}:    \> |path|\\
    \refKey{/tcb/title engine}:           \> |path|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}

\begin{docTcbKey}{enhanced jigsaw}{}{style, no value}
  This is an abbreviation for setting |skin=enhanced jigsaw|.
\end{docTcbKey}

\begin{dispExample*}{segmentation style={preaction={fill=white},pattern=checkerboard,pattern color=gray!40}}
\begin{tcbraster}[enhanced jigsaw,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,colbacktitle=LimeGreen!75!DarkGreen,
    opacityframe=0.5,opacityback=0.5,opacitybacktitle=0.5,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample*}


\begin{docTcbKey}[][doc new=2017-07-01]{enhanced standard jigsaw}{}{style, no value}
  For unbreakable boxes, this is identical to using \refKey{/tcb/enhanced jigsaw}.
  But, for breakable boxes, the \emph{break sequence} is identical to the \refSkin{standard jigsaw} skin,
  see Section \ref{subsec:breaksequence} from page \pageref{subsec:breaksequence}.
\end{docTcbKey}


\clearpage
\begin{docSkin}{enhancedfirst jigsaw}
  This is the jigsaw variant of skin \refSkin{enhancedfirst}.
  It differs by its frame engine, see \Vref{subsec:skinjigsaw}.
\begin{tcolorbox}[skintable=enhancedfirst jigsaw]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |pathfirstjigsaw|\\
    \refKey{/tcb/interior titled engine}: \> |pathfirst|\\ 
    \refKey{/tcb/interior engine}:        \> |pathfirst|\\
    \refKey{/tcb/segmentation engine}:    \> |path|\\
    \refKey{/tcb/title engine}:           \> |pathfirst|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}


\begin{dispExample*}{segmentation style={preaction={fill=white},pattern=checkerboard,pattern color=gray!40}}
\begin{tcbraster}[skin=enhancedfirst jigsaw,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,colbacktitle=LimeGreen!75!DarkGreen,
    opacityframe=0.5,opacityback=0.5,opacitybacktitle=0.5,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample*}


\clearpage
\begin{docSkin}{enhancedmiddle jigsaw}
  This is the jigsaw variant of skin \refSkin{enhancedmiddle}.
  It differs by its frame engine, see \Vref{subsec:skinjigsaw}.
\begin{tcolorbox}[skintable=enhancedmiddle jigsaw]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |pathmiddlejigsaw|\\
    \refKey{/tcb/interior titled engine}: \> |pathmiddle|\\ 
    \refKey{/tcb/interior engine}:        \> |pathmiddle|\\
    \refKey{/tcb/segmentation engine}:    \> |path|\\
    \refKey{/tcb/title engine}:           \> |pathmiddle|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}


\begin{dispExample*}{segmentation style={preaction={fill=white},pattern=checkerboard,pattern color=gray!40}}
\begin{tcbraster}[skin=enhancedmiddle jigsaw,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,colbacktitle=LimeGreen!75!DarkGreen,
    opacityframe=0.5,opacityback=0.5,opacitybacktitle=0.5,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample*}


\begin{docTcbKey}{marker}{}{style, no value}
  This styles relies on the skin \refSkin{enhancedmiddle jigsaw}. It is
  intended to be used as an optical marker like a highlighter pen.
\begin{dispExample}
\begin{tcolorbox}[marker]
\lipsum[2]
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}

\clearpage

\begin{dispListing*}{before upper={This examples demonstrates the creation of several
  \emph{text marker} environments based on \refSkin{enhancedmiddle}.\par\medskip}}
\tcbset{textmarker/.style={%
    skin=enhancedmiddle jigsaw,breakable,parbox=false,
    boxrule=0mm,leftrule=5mm,rightrule=5mm,boxsep=0mm,arc=0mm,outer arc=0mm,
    left=3mm,right=3mm,top=1mm,bottom=1mm,toptitle=1mm,bottomtitle=1mm,oversize}}

\newtcolorbox{yellow}{textmarker,colback=yellow!5!white,colframe=yellow}
\newtcolorbox{orange}{textmarker,colback=DarkOrange!5!white,
                        colframe=DarkOrange!75!yellow}
\newtcolorbox{red}{textmarker,colback=red!5!white,colframe=red}
\newtcolorbox{blue}{textmarker,colback=DeepSkyBlue!5!white,colframe=DeepSkyBlue}
\newtcolorbox{green}{textmarker,colback=Chartreuse!5!white,colframe=Chartreuse}
\newtcolorbox{rainbow}{textmarker,interior hidden,
  frame style={top color=blue,bottom color=red,middle color=green}}

\begin{yellow}
  \lipsum[1-3]
\end{yellow}

\begin{orange}
  \lipsum[4]
\end{orange}

\begin{red}
  \lipsum[5]
\end{red}

\begin{green}
  \lipsum[6]
\end{green}

\begin{blue}
  \lipsum[7]
\end{blue}

\begin{rainbow}
  \lipsum[8]
\end{rainbow}
\end{dispListing*}
{\tcbusetemp}


\clearpage
\begin{docSkin}{enhancedlast jigsaw}
  This is the jigsaw variant of skin \refSkin{enhancedlast}.
  It differs by its frame engine, see \Vref{subsec:skinjigsaw}.
\begin{tcolorbox}[skintable=enhancedlast]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |pathlastjigsaw|\\
    \refKey{/tcb/interior titled engine}: \> |pathlast|\\ 
    \refKey{/tcb/interior engine}:        \> |pathlast|\\
    \refKey{/tcb/segmentation engine}:    \> |path|\\
    \refKey{/tcb/title engine}:           \> |pathlast|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}


\begin{dispExample*}{segmentation style={preaction={fill=white},pattern=checkerboard,pattern color=gray!40}}
\begin{tcbraster}[skin=enhancedlast jigsaw,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,colbacktitle=LimeGreen!75!DarkGreen,
    opacityframe=0.5,opacityback=0.5,opacitybacktitle=0.5,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample*}



\clearpage
\subsection{Skin Family 'bicolor'}
\begin{docSkin}{bicolor}
  This skin is quite similar to the \refSkin{standard} and \refSkin{enhanced} skin.
  But instead of a segmentation line, the optional lower part of the box is filled with a
  different color or drawn with a different style.
\begin{tcolorbox}[skintable=bicolor]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |path|\\
    \refKey{/tcb/interior titled engine}: \> \emph{special}\\ 
    \refKey{/tcb/interior engine}:        \> \emph{special}\\
    \refKey{/tcb/segmentation engine}:    \> \emph{special}\\
    \refKey{/tcb/title engine}:           \> |path|
  \end{tabbing}
\end{tcolorbox}
  \begin{itemize}
  \item The most basic usage of this skin is to set the background color of
    the lower part by \refKey{/tcb/colbacklower} and all other options like for
    the \refSkin{standard} skin.
\begin{dispExample}
\begin{tcolorbox}[skin=bicolor,title=The title,
    colframe=FireBrick!75!black,colback=Salmon!50!white,colbacklower=Salmon]
  The upper part.
  \tcblower
  The lower part.
\end{tcolorbox}
\end{dispExample}
  \item The more advanced usage of this skin is to apply the \refKey{/tcb/frame style}
    and the \refKey{/tcb/interior style} like for
    the \refSkin{enhanced} skin. Also, the \refKey{/tcb/segmentation style} can be
    used, but it is applied to the whole lower part.
\begin{dispExample}
\begin{tcolorbox}[skin=bicolor,title=The title,
    frame style={top color=FireBrick,
                 bottom color=FireBrick!15!white,draw=black},
    interior style={left color=Salmon,right color=Salmon!50!white},
    segmentation style={right color=Salmon,left color=Salmon!50!white}]
  The upper part.
  \tcblower
  The lower part.
\end{tcolorbox}
\end{dispExample}
  \end{itemize}
\end{docSkin}

\clearpage

\begin{docTcbKey}{bicolor}{}{style, no value}
  This is an abbreviation for setting |skin=bicolor|.
\end{docTcbKey}


\begin{dispExample}
\begin{tcbraster}[bicolor,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,colbacklower=LimeGreen!75!LightGreen,
    colbacktitle=LimeGreen!75!DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}

\enlargethispage*{1cm}

\begin{docTcbKey}{colbacklower}{=\meta{color}}{no default, initially \texttt{black!15!white}}
  Sets the background \meta{color} of the lower part. It depends on the skin,
  if this value is used.
\end{docTcbKey}

\begin{dispExample}
\tcbset{gitexample/.style={listing and comment,comment={#1},
  skin=bicolor,boxrule=1mm,fonttitle=\bfseries,coltitle=black,
  frame style={draw=black,left color=Gold,right color=Goldenrod!50!Gold},
  colback=black,colbacklower=Goldenrod!75!Gold,
  colupper=white,collower=black,
  listing options={language={bash},aboveskip=0pt,belowskip=0pt,nolol,
  basicstyle=\ttfamily\bfseries,extendedchars=true}}}

\begin{tcblisting}{title={Snapshot of the staging area},
  gitexample={The option '-a' automatically stages all tracked and modified
              files before the commit.\par
              This can be combined with the message option '-m'
              as seen in the third line.}}
git commit
git commit -a
git commit -am 'changes to my example'
\end{tcblisting}
\end{dispExample}


\clearpage


\begin{docSkin}{bicolorfirst}
This is a flavor of \refSkin{bicolor} which is used as a \emph{first} part
in a break sequence for \refSkin{bicolor}.
Nevertheless, this skin can be applied independently.
\begin{tcolorbox}[skintable=bicolorfirst]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |pathfirst|\\
    \refKey{/tcb/interior titled engine}: \> \emph{special}\\ 
    \refKey{/tcb/interior engine}:        \> \emph{special}\\
    \refKey{/tcb/segmentation engine}:    \> \emph{special}\\
    \refKey{/tcb/title engine}:           \> |pathfirst|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}

\begin{dispExample}
\begin{tcbraster}[skin=bicolorfirst,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,colbacklower=LimeGreen!75!LightGreen,
    colbacktitle=LimeGreen!75!DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}


\clearpage
\begin{docSkin}{bicolormiddle}
This is a flavor of \refSkin{bicolor} which is used as a \emph{middle} part
in a break sequence for \refSkin{bicolor}.
Nevertheless, this skin can be applied independently.
\begin{tcolorbox}[skintable=bicolormiddle]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |pathmiddle|\\
    \refKey{/tcb/interior titled engine}: \> \emph{special}\\ 
    \refKey{/tcb/interior engine}:        \> \emph{special}\\
    \refKey{/tcb/segmentation engine}:    \> \emph{special}\\
    \refKey{/tcb/title engine}:           \> |pathmiddle|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}


\begin{dispExample}
\begin{tcbraster}[skin=bicolormiddle,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,colbacklower=LimeGreen!75!LightGreen,
    colbacktitle=LimeGreen!75!DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}


\clearpage
\begin{docSkin}{bicolorlast}
This is a flavor of \refSkin{bicolor} which is used as a \emph{last} part
in a break sequence for \refSkin{bicolor}.
Nevertheless, this skin can be applied independently.
\begin{tcolorbox}[skintable=bicolorlast]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |pathlast|\\
    \refKey{/tcb/interior titled engine}: \> \emph{special}\\ 
    \refKey{/tcb/interior engine}:        \> \emph{special}\\
    \refKey{/tcb/segmentation engine}:    \> \emph{special}\\
    \refKey{/tcb/title engine}:           \> |pathlast|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}


\begin{dispExample}
\begin{tcbraster}[skin=bicolorlast,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,colbacklower=LimeGreen!75!LightGreen,
    colbacktitle=LimeGreen!75!DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}



\clearpage
\subsection{Skin Family 'tile'}
\begin{docSkin}[doc new=2016-02-25]{tile}
  This skin is a variant of skin \refSkin{bicolor}. Especially, the
  optional lower part of the box is colored by \refKey{/tcb/colbacklower}.
  The main difference to \refSkin{bicolor} is that \refSkin{tile} has no
  frame.
\begin{tcolorbox}[skintable=tile]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |empty|\\
    \refKey{/tcb/interior titled engine}: \> \emph{special}\\ 
    \refKey{/tcb/interior engine}:        \> \emph{special}\\
    \refKey{/tcb/segmentation engine}:    \> \emph{special}\\
    \refKey{/tcb/title engine}:           \> |path|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}

\begin{docTcbKey}[][doc new=2016-02-25]{tile}{}{style, no value}
  This is an abbreviation for setting |skin=tile|.
  \begin{marker}It also changes the geometry and some style options.\end{marker}
\end{docTcbKey}


\begin{dispExample}
\begin{tcbraster}[tile,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,colbacklower=LimeGreen!75!LightGreen,
    colbacktitle=LimeGreen!75!DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}


\clearpage
\begin{docSkin}[doc new=2016-02-25]{tilefirst}
This is a flavor of \refSkin{tile} which is used as a \emph{first} part
in a break sequence for \refSkin{tile}.
Nevertheless, this skin can be applied independently.
\begin{tcolorbox}[skintable=tilefirst]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |empty|\\
    \refKey{/tcb/interior titled engine}: \> \emph{special}\\ 
    \refKey{/tcb/interior engine}:        \> \emph{special}\\
    \refKey{/tcb/segmentation engine}:    \> \emph{special}\\
    \refKey{/tcb/title engine}:           \> |pathfirst|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}

\begin{dispExample}
\begin{tcbraster}[skin=tilefirst,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,colbacklower=LimeGreen!75!LightGreen,
    colbacktitle=LimeGreen!75!DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm,boxrule=0pt]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}


\clearpage
\begin{docSkin}[doc new=2016-02-25]{tilemiddle}
This is a flavor of \refSkin{tile} which is used as a \emph{middle} part
in a break sequence for \refSkin{tile}.
Nevertheless, this skin can be applied independently.
\begin{tcolorbox}[skintable=tilemiddle]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |empty|\\
    \refKey{/tcb/interior titled engine}: \> \emph{special}\\ 
    \refKey{/tcb/interior engine}:        \> \emph{special}\\
    \refKey{/tcb/segmentation engine}:    \> \emph{special}\\
    \refKey{/tcb/title engine}:           \> |pathmiddle|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}


\begin{dispExample}
\begin{tcbraster}[skin=tilemiddle,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,colbacklower=LimeGreen!75!LightGreen,
    colbacktitle=LimeGreen!75!DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm,boxrule=0pt]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}


\clearpage
\begin{docSkin}[doc new=2016-02-25]{tilelast}
This is a flavor of \refSkin{tile} which is used as a \emph{last} part
in a break sequence for \refSkin{tile}.
Nevertheless, this skin can be applied independently.
\begin{tcolorbox}[skintable=tilelast]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |empty|\\
    \refKey{/tcb/interior titled engine}: \> \emph{special}\\ 
    \refKey{/tcb/interior engine}:        \> \emph{special}\\
    \refKey{/tcb/segmentation engine}:    \> \emph{special}\\
    \refKey{/tcb/title engine}:           \> |pathlast|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}


\begin{dispExample}
\begin{tcbraster}[skin=tilelast,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,colbacklower=LimeGreen!75!LightGreen,
    colbacktitle=LimeGreen!75!DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm,boxrule=0pt]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}



\clearpage
\subsection{Skin Family 'beamer'}

\begin{docSkin}{beamer}
  This skin resembles boxes known from the |beamer| class and therefore is
  called 'beamer'. It uses the normal colors from the core package but shades
  them a little bit. To use this skin, the |tikz| library |shadings|
  has to be included in the preamble by:
\begin{dispListing}
\usetikzlibrary{shadings}
\end{dispListing}
\begin{tcolorbox}[skintable=beamer]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |path|\\
    \refKey{/tcb/interior titled engine}: \> \emph{special}\\ 
    \refKey{/tcb/interior engine}:        \> \emph{special}\\
    \refKey{/tcb/segmentation engine}:    \> \emph{special}\\
    \refKey{/tcb/title engine}:           \> |path|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}



\begin{docTcbKey}{beamer}{}{style, no value}
  This is an abbreviation for setting |skin=beamer|.
  \begin{marker}It also changes the geometry and some style options.\end{marker}
\end{docTcbKey}



\begin{dispExample}
\begin{tcbraster}[beamer,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}



\begin{dispExample}
\begin{tcolorbox}[beamer,colback=Salmon!50!white,colframe=FireBrick!75!black,
  adjusted title=A colored box with the 'beamer' skin]
This box looks like a box provided by the \texttt{beamer} class.
\end{tcolorbox}
\end{dispExample}


\begin{dispExample}
\begin{tcolorbox}[beamer,colframe=blue,colback=black,
  watermark graphics=lichtspiel.jpg,
  coltext=white,watermark opacity=0.75,watermark stretch=1.0,
  title=Beamer Box with background picture]
\lipsum[1]
\end{tcolorbox}
\end{dispExample}


\begin{dispExample}
\newtcolorbox{myblock}[2][]{%
  beamer,breakable,colback=LightBlue,colframe=DarkBlue,#1,title=#2}%

\begin{myblock}{Beamerish \texttt{block}: \texttt{myblock}}
\lipsum[1]
\end{myblock}
\end{dispExample}


\clearpage
\begin{docSkin}{beamerfirst}
This is a flavor of \refSkin{beamer} which is used as a \emph{first} part
in a break sequence for \refSkin{beamer}.
Nevertheless, this skin can be applied independently.
\begin{tcolorbox}[skintable=beamerfirst]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |pathfirst|\\
    \refKey{/tcb/interior titled engine}: \> \emph{special}\\ 
    \refKey{/tcb/interior engine}:        \> \emph{special}\\
    \refKey{/tcb/segmentation engine}:    \> \emph{special}\\
    \refKey{/tcb/title engine}:           \> |pathfirst|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}


\begin{dispExample}
\begin{tcbraster}[beamer,skin=beamerfirst,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}


\clearpage

\begin{docSkin}{beamermiddle}
This is a flavor of \refSkin{beamer} which is used as a \emph{middle} part
in a break sequence for \refSkin{beamer}.
Nevertheless, this skin can be applied independently.
\begin{tcolorbox}[skintable=beamermiddle]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |pathmiddle|\\
    \refKey{/tcb/interior titled engine}: \> \emph{special}\\ 
    \refKey{/tcb/interior engine}:        \> \emph{special}\\
    \refKey{/tcb/segmentation engine}:    \> \emph{special}\\
    \refKey{/tcb/title engine}:           \> |pathmiddle|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}


\begin{dispExample}
\begin{tcbraster}[beamer,skin=beamermiddle,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}


\clearpage
\begin{docSkin}{beamerlast}
This is a flavor of \refSkin{beamer} which is used as a \emph{last} part
in a break sequence for \refSkin{beamer}.
Nevertheless, this skin can be applied independently.
\begin{tcolorbox}[skintable=beamerlast]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |pathlast|\\
    \refKey{/tcb/interior titled engine}: \> \emph{special}\\ 
    \refKey{/tcb/interior engine}:        \> \emph{special}\\
    \refKey{/tcb/segmentation engine}:    \> \emph{special}\\
    \refKey{/tcb/title engine}:           \> |pathlast|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}

\begin{dispExample}
\begin{tcbraster}[beamer,skin=beamerlast,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}



\clearpage
\subsection{Skin Family 'widget'}
\begin{docSkin}{widget}
  This skin uses the normal colors from the core package but shades
  them a little bit. To use this skin, the |tikz| library |shadings|
  has to be included in the preamble by:
\begin{dispListing}
\usetikzlibrary{shadings}
\end{dispListing}
The appearance of the skin can be controlled by \refKey{/tcb/frame style},
\refKey{/tcb/interior style}, and \refKey{/tcb/segmentation style},
if needed.
\begin{tcolorbox}[skintable=widget]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |path|\\
    \refKey{/tcb/interior titled engine}: \> |path|\\ 
    \refKey{/tcb/interior engine}:        \> |path|\\
    \refKey{/tcb/segmentation engine}:    \> \emph{special}\\
    \refKey{/tcb/title engine}:           \> \emph{special}
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}


\begin{docTcbKey}{widget}{}{style, no value}
  This is an abbreviation for setting |skin=widget|.
  \begin{marker}It also changes the geometry and some style options.\end{marker}
\end{docTcbKey}


\begin{dispExample}
\begin{tcbraster}[widget,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}


\begin{dispExample}
\begin{tcolorbox}[widget,colback=Salmon!50!white,colframe=FireBrick!75!black,
  adjusted title=A colored box with the 'widget' skin]
This is my content.
\end{tcolorbox}
\end{dispExample}



\begin{docSkin}{widgetfirst}
This is a flavor of \refSkin{widget} which is used as a \emph{first} part
in a break sequence for \refSkin{widget}.
Nevertheless, this skin can be applied independently.
\begin{tcolorbox}[skintable=widgetfirst]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |pathfirst|\\
    \refKey{/tcb/interior titled engine}: \> |pathfirst|\\ 
    \refKey{/tcb/interior engine}:        \> |pathfirst|\\
    \refKey{/tcb/segmentation engine}:    \> \emph{special}\\
    \refKey{/tcb/title engine}:           \> \emph{special}
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}


\begin{dispExample}
\begin{tcbraster}[widget,skin=widgetfirst,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}

\clearpage

\begin{docSkin}{widgetmiddle}
This is a flavor of \refSkin{widget} which is used as a \emph{middle} part
in a break sequence for \refSkin{widget}.
Nevertheless, this skin can be applied independently.
\begin{tcolorbox}[skintable=widgetmiddle]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |pathmiddle|\\
    \refKey{/tcb/interior titled engine}: \> |pathmiddle|\\ 
    \refKey{/tcb/interior engine}:        \> |pathmiddle|\\
    \refKey{/tcb/segmentation engine}:    \> \emph{special}\\
    \refKey{/tcb/title engine}:           \> \emph{special}
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}

\begin{dispExample}
\begin{tcbraster}[widget,skin=widgetmiddle,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}


\clearpage
\begin{docSkin}{widgetlast}
This is a flavor of \refSkin{widget} which is used as a \emph{last} part
in a break sequence for \refSkin{widget}.
Nevertheless, this skin can be applied independently.
\begin{tcolorbox}[skintable=widgetlast]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |pathlast|\\
    \refKey{/tcb/interior titled engine}: \> |pathlast|\\ 
    \refKey{/tcb/interior engine}:        \> |pathlast|\\
    \refKey{/tcb/segmentation engine}:    \> \emph{special}\\
    \refKey{/tcb/title engine}:           \> \emph{special}
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}


\begin{dispExample}
\begin{tcbraster}[widget,skin=widgetlast,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}




\clearpage
\subsection{Skin Family 'empty'}

\begin{docSkin}{empty}
  This skin sets all engines to |empty|, i.\,e.\ nothing is drawn at all.
  Therefore, this skin is a good starting point to create a complete
  new style by yourself.
\begin{tcolorbox}[skintable=empty]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |empty|\\
    \refKey{/tcb/interior titled engine}: \> |empty|\\ 
    \refKey{/tcb/interior engine}:        \> |empty|\\
    \refKey{/tcb/segmentation engine}:    \> |empty|\\
    \refKey{/tcb/title engine}:           \> |empty|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}


\begin{docTcbKey}{empty}{}{style, no value}
  This is an abbreviation for setting |skin=empty|.
\end{docTcbKey}

\begin{dispExample}
\begin{tcbraster}[empty,raster equal height,raster columns=4,
    coltitle=Navy,borderline={2pt}{0pt}{black!10!white},
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}


\clearpage
\begin{docTcbKey}{blanker}{}{style, initially unset}
  This style relies on the skin \refSkin{empty}. All engines
  are set to empty and all margins are set to |0pt|.
  In contrast to \refKey{/tcb/blank}, the graphical paths are
  not constructed with exception of the geometry nodes.
\begin{dispExample}
\begin{tcolorbox}[blanker,watermark text=A blank box]
\lipsum[1]
\end{tcolorbox}
\end{dispExample}

\begin{dispExample}
% \tcbuselibrary{fitting}
\newtcboxfit{\mybox}[1]{blanker,width=4cm,height=7cm,top=4pt,
  watermark text=#1}

\begin{tabular}{|c|c|c|}\hline
A & B & C\\\hline
\mybox{A}{\lipsum[1]} & \mybox{B}{\lipsum[2]} & \mybox{C}{\lipsum[3]}\\\hline
\end{tabular}
\end{dispExample}
\end{docTcbKey}



\clearpage
\begin{docTcbKey}{blankest}{}{style, initially unset}
  This style extends \refKey{/tcb/blanker}.
  All engines are set to empty and all margins are set to |0pt|.
  In contrast to \refKey{/tcb/blanker}, also title, shadow, underlay,
  overlay, finish and borderline are removed.

\begin{dispExample}
% \tcbuselibrary{raster}
\begin{tcbraster}[raster columns=3,raster equal height,
    title=Box \thetcbrasternum,
    enhanced,size=small,colframe=red!50!black,colback=red!10!white,
    coltitle=yellow!85!black,
    drop fuzzy shadow,watermark text={Box \thetcbrasternum},
    borderline={.25mm}{-0.5mm}{green!40!black},
    finish={\begin{tcbclipframe}\draw[blue,opacity=0.1,line width=1cm]
      (frame.south west) -- (frame.north east);\end{tcbclipframe}},
    ]
  \begin{tcolorbox}\lipsum[4]\end{tcolorbox}
  \begin{tcolorbox}[blanker]\lipsum[4]\end{tcolorbox}
  \begin{tcolorbox}[blankest]\lipsum[4]\end{tcolorbox}
\end{tcbraster}
\end{dispExample}
\end{docTcbKey}


\clearpage
\begin{docSkin}{emptyfirst}
This is a flavor of \refSkin{empty} which is used as a \emph{first} part
in a break sequence for \refSkin{empty}.
Nevertheless, this skin can be applied independently.
\begin{tcolorbox}[skintable=emptyfirst]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |empty|\\
    \refKey{/tcb/interior titled engine}: \> |empty|\\ 
    \refKey{/tcb/interior engine}:        \> |empty|\\
    \refKey{/tcb/segmentation engine}:    \> |empty|\\
    \refKey{/tcb/title engine}:           \> |empty|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}


\begin{dispExample}
\begin{tcbraster}[empty,skin=emptyfirst,raster equal height,raster columns=4,
    coltitle=Navy,borderline={2pt}{0pt}{black!10!white},
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}


\clearpage

\begin{docSkin}{emptymiddle}
This is a flavor of \refSkin{empty} which is used as a \emph{middle} part
in a break sequence for \refSkin{empty}.
Nevertheless, this skin can be applied independently.
\begin{tcolorbox}[skintable=emptymiddle]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |empty|\\
    \refKey{/tcb/interior titled engine}: \> |empty|\\ 
    \refKey{/tcb/interior engine}:        \> |empty|\\
    \refKey{/tcb/segmentation engine}:    \> |empty|\\
    \refKey{/tcb/title engine}:           \> |empty|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}


\begin{dispExample}
\begin{tcbraster}[empty,skin=emptymiddle,raster equal height,raster columns=4,
    coltitle=Navy,borderline={2pt}{0pt}{black!10!white},
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}


\clearpage
\begin{docSkin}{emptylast}
This is a flavor of \refSkin{empty} which is used as a \emph{last} part
in a break sequence for \refSkin{empty}.
Nevertheless, this skin can be applied independently.
\begin{tcolorbox}[skintable=emptylast]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |empty|\\
    \refKey{/tcb/interior titled engine}: \> |empty|\\ 
    \refKey{/tcb/interior engine}:        \> |empty|\\
    \refKey{/tcb/segmentation engine}:    \> |empty|\\
    \refKey{/tcb/title engine}:           \> |empty|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}

\begin{dispExample}
\begin{tcbraster}[empty,skin=emptylast,raster equal height,raster columns=4,
    coltitle=Navy,borderline={2pt}{0pt}{black!10!white},
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}

\clearpage
\begin{dispListing*}{breakable,phantomlabel=freeboxexample,before upper={This example demonstrates
a breakable customized box. Here, we define an environment |freebox|.
The first application of |freebox| produces an unbroken |tcolorbox|.
The box is drawn by the code given by \refKey{/tcb/frame code}
and \refKey{/tcb/interior code}.\par
The second application of |freebox| is broken into several parts which
are drawn by the codes given by
\refKey{/tcb/skin first is subskin of},
\refKey{/tcb/skin middle is subskin of}, and
\refKey{/tcb/skin last is subskin of}.
\par\bigskip
}}
% Preamble:
%\usepackage{tikz,lipsum}
%\tcbuselibrary{skins,breakable}
\tikzset{coltria/.style={fill=red!15!white}}

\newtcolorbox{freebox}[1][]{empty,
  breakable,height fixed for=first and middle,
  leftrule=5mm,left=2mm,
  frame style={fill,top color=red!75!black,bottom color=red!75!black,middle color=red},
  colback=yellow!50!white,
  watermark color=red!50!yellow!75!white,
  watermark text on=unbroken is unbroken box,
  watermark text on=first is first part,
  watermark text on=middle is middle part,
  watermark text on=last is last part,
  % code for unbroken boxes:
  frame code={\path[tcb fill frame] (frame.south west)--(frame.north west)
    --([xshift=-5mm]frame.north east)--([yshift=-5mm]frame.north east)
    --([yshift=5mm]frame.south east)--([xshift=-5mm]frame.south east)--cycle; },
  interior code={\path[tcb fill interior] (interior.south west)--(interior.north west)
    --([xshift=-4.8mm]interior.north east)--([yshift=-4.8mm]interior.north east)
    --([yshift=4.8mm]interior.south east)--([xshift=-4.8mm]interior.south east)
    --cycle; },
  % code for the first part of a break sequence:
  skin first is subskin of={emptyfirst}{%
    frame code={\path[tcb fill frame] (frame.south west)--(frame.north west)
      --([xshift=-5mm]frame.north east)--([yshift=-5mm]frame.north east)
      --(frame.south east)--cycle;
      \path[coltria] ([xshift=2.5mm,yshift=1mm]frame.south west) -- +(120:2mm)
      -- +(60:2mm)-- cycle; },
    interior code={\path[tcb fill interior] (interior.south west|-frame.south)
      --(interior.north west)--([xshift=-4.8mm]interior.north east)
      --([yshift=-4.8mm]interior.north east)--(interior.south east|-frame.south)
      --cycle; },
  },%
  % code for the middle part of a break sequence:
  skin middle is subskin of={emptymiddle}{%
    frame code={\path[tcb fill frame] (frame.south west)--(frame.north west)
      --(frame.north east)--(frame.south east)--cycle;
      \path[coltria] ([xshift=2.5mm,yshift=-1mm]frame.north west) -- +(240:2mm)
        -- +(300:2mm) -- cycle;
      \path[coltria] ([xshift=2.5mm,yshift=1mm]frame.south west) -- +(120:2mm)
        -- +(60:2mm) -- cycle;
      },
    interior code={\path[tcb fill interior] (interior.south west|-frame.south)
      --(interior.north west|-frame.north)--(interior.north east|-frame.north)
      --(interior.south east|-frame.south)--cycle; },
    },
  % code for the last part of a break sequence:
  skin last is subskin of={emptylast}{%
    frame code={\path[tcb fill frame] (frame.south west)--(frame.north west)
      --(frame.north east)--([yshift=5mm]frame.south east)
      --([xshift=-5mm]frame.south east)--cycle;
      \path[coltria] ([xshift=2.5mm,yshift=-1mm]frame.north west) -- +(240:2mm)
      -- +(300:2mm) -- cycle;
      },
    interior code={\path[tcb fill interior] (interior.south west)
      --(interior.north west|-frame.north)--(interior.north east|-frame.north)
      --([yshift=4.8mm]interior.south east)--([xshift=-4.8mm]interior.south east)
      --cycle; },
    },
  #1}

\begin{freebox}
\lipsum[1]
\end{freebox}

\begin{freebox}
\lipsum[1-12]
\end{freebox}
\end{dispListing*}
{\tcbusetemp}


\clearpage

\subsection{Skin 'spartan'}\label{subsec:spartan}

\begin{docSkin}{spartan}
  This skin is quite \ldots\ spartan.
  It supports no rounded corners, no overlays, no shadows, no borderlines,
  and no finishes. The only exception are underlays.
  One cannot do very fancy things with this skin, but it compiles very fast.
  Therefore, the |spartan| skin is
  used for the draft mode, see \Vref{subsec:draftmode}.
  Nevertheless, it can be used as a normal skin.

\begin{tcolorbox}[skintable=spartan]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |spartan|\\
    \refKey{/tcb/interior titled engine}: \> |spartan|\\ 
    \refKey{/tcb/interior engine}:        \> |spartan|\\
    \refKey{/tcb/segmentation engine}:    \> |spartan|\\
    \refKey{/tcb/title engine}:           \> |spartan|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}


\begin{docTcbKey}{spartan}{}{style, no value}
  This is an abbreviation for setting |skin=spartan|.
\end{docTcbKey}


\begin{dispExample}
\begin{tcbraster}[spartan,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,colbacktitle=LimeGreen!75!DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}


\clearpage

\subsection{Skin 'draft'}\label{subsec:draft}

\begin{docSkin}{draft}
  This skin is intended to be used while drafting new geometric settings
  for a |tcolorbox|.
\begin{tcolorbox}[skintable=draft]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> \emph{special}\\
    \refKey{/tcb/interior titled engine}: \> \emph{special}\\ 
    \refKey{/tcb/interior engine}:        \> \emph{special}\\
    \refKey{/tcb/segmentation engine}:    \> |path|\\
    \refKey{/tcb/title engine}:           \> |path|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}

\begin{docTcbKey}{draft}{}{style, no value}
  This is an abbreviation for setting |skin=draft|.
\end{docTcbKey}


\begin{dispExample}
\begin{tcbraster}[draft,raster equal height,raster columns=4,
    colback=LightGreen,colframe=DarkGreen,colbacktitle=LimeGreen!75!DarkGreen,
    left=1mm,right=1mm,top=1mm,bottom=1mm,middle=1mm]
  \begin{tcolorbox}
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
  \end{tcolorbox}
  \begin{tcolorbox}[adjusted title=My title]
    This is my content.
    \tcblower
    More content.
  \end{tcolorbox}
\end{tcbraster}
\end{dispExample}


\begin{dispExample}
\vspace*{3mm}
\begin{tcolorbox}[draft,title=A colored box with the 'draft' skin]
\lipsum[1-3]
\tcblower
\lipsum[4-6]
\end{tcolorbox}
\end{dispExample}



\clearpage
\subsection{Skin Family 'freelance'}
\begin{marker}
This skin family 'freelance' is deprecated with |tcolorbox| 3.00.
It is not longer needed, because
\refKey{/tcb/frame code},
\refKey{/tcb/interior code},
\refKey{/tcb/interior titled code}, and
\refKey{/tcb/title code}
can be applied to every skin now. In this sense, everything has become
\emph{freelance} now.\par
For users of \refKey{/tcb/freelance}: Old code should continue to work. There may be
exceptions for breakable freelance boxes under certain circumstances.
For new code, use \refKey{/tcb/empty} or \refKey{/tcb/enhanced} where
you would have used \refKey{/tcb/freelance} before.
\end{marker}

\begin{docSkin}{freelance}
  This skin gives full freedom for the appearance of the |tcolorbox|.
  All drawing engines are set to type |freelance|; they use the |tikz| package
  and compute the \refKey{/tcb/geometry nodes}.
  %This skin is useful for boxes which should differ much from the normal
  %appearance. Note that this difference has to be programmed by the user.
  %The drawing code can be given
  %with the following option keys. As default value, the code from the |standard|
  %skin is set.
\begin{tcolorbox}[skintable=freelance]
  \begin{tabbing}
    \refKey{/tcb/interior titled engine}: \=\kill
    \refKey{/tcb/graphical environment}:  \> |tikzpicture|\\ 
    \refKey{/tcb/frame engine}:           \> |freelance|\\
    \refKey{/tcb/interior titled engine}: \> |freelance|\\ 
    \refKey{/tcb/interior engine}:        \> |freelance|\\
    \refKey{/tcb/segmentation engine}:    \> |freelance|\\
    \refKey{/tcb/title engine}:           \> |freelance|
  \end{tabbing}
\end{tcolorbox}
\end{docSkin}

\begin{docTcbKey}{freelance}{}{style, no value}
  This is an abbreviation for setting |skin=freelance|.
\end{docTcbKey}

\begin{docSkin}{freelancefirst}
  This skin equals \refSkin{freelance} with exception of the break sequence,
  see \Vref{subsec:breaksequence}.
  %It is used as first part of the
  %break sequence of \refSkin{freelance}. \refKey{/tcb/extend freelancefirst}
  %can be used to customize this part.
\end{docSkin}

\begin{docSkin}{freelancemiddle}
  This skin equals \refSkin{freelance} with exception of the break sequence,
  see \Vref{subsec:breaksequence}.
  %It is used as middle part of the
  %break sequence of \refSkin{freelance}. \refKey{/tcb/extend freelancemiddle}
  %can be used to customize this part.
\end{docSkin}

\begin{docSkin}{freelancelast}
  This skin equals \refSkin{freelance} with exception of the break sequence,
  see \Vref{subsec:breaksequence}.
  %It is used as last part of the
  %break sequence of \refSkin{freelance}. \refKey{/tcb/extend freelancelast}
  %can be used to customize this part.
\end{docSkin}


\begin{docTcbKey}{extend freelance}{=\meta{options}}{no default, initially empty}
The \meta{options} are added to the skin definition of \refSkin{freelance}.
\end{docTcbKey}

\begin{docTcbKey}{extend freelancefirst}{=\meta{options}}{no default, initially empty}
The \meta{options} are added to the skin definition of \refSkin{freelancefirst} which
is used as first part of the break sequence of \refSkin{freelance}.
See \refKey{/tcb/skin first is subskin of} for a substitute of this key.
\end{docTcbKey}

\begin{docTcbKey}{extend freelancemiddle}{=\meta{options}}{no default, initially empty}
The \meta{options} are added to the skin definition of \refSkin{freelancemiddle} which
is used as middle part of the break sequence of \refSkin{freelance}.
See \refKey{/tcb/skin middle is subskin of} for a substitute of this key.
\end{docTcbKey}

\enlargethispage*{1cm}

\begin{docTcbKey}{extend freelancelast}{=\meta{options}}{no default, initially empty}
The \meta{options} are added to the skin definition of \refSkin{freelancelast} which
is used as last part of the break sequence of \refSkin{freelance}.
See \refKey{/tcb/skin last is subskin of} for a substitute of this key.
\end{docTcbKey}





==> tcolorbox.doc.technical.tex <==
% !TeX root = tcolorbox.tex
% include file of tcolorbox.tex (manual of the LaTeX package tcolorbox)
\clearpage
\section{Technical Overview and Customization}\label{sec:technical}%
\tcbset{external/prefix=external/technical_}%
This section provides a technical overview of the skin concept of |tcolorbox|.
For most applications of |tcolorbox|, one will not need to know the bells and
whistles described herein.
You may proceed to \Vref{sec:skins} where the customization options
for most users are documented.

The following explanations also cover options and settings from the \mylib{skins} library,
see  \Vref{sec:skins}.

\subsection{Skins and Drawing Engines}\label{sec:skincorekeys}
From a technical point of view, a \emph{skin} is a style definition for the
appearance of a |tcolorbox|. The core package provides some additional
option keys for skins but only two skins called \refSkin{standard}
and \refSkin{standard jigsaw}.
The \mylib{skins} library adds several more skins. To change to a skin, only one
option from the core package has to be set.

\begin{docTcbKey}{skin}{=\meta{name}}{style, no default, initially \texttt{standard}}
  Sets the current skin to \meta{name}. This is a style definition which sets all the following
  keys, i.\,e.\ for many use cases there is nothing more to do.
\begin{dispExample}
\tcbset{colback=Salmon!50!white,colframe=FireBrick!75!black,
  width=(\linewidth-8mm)/2,before=,after=\hfill,equal height group=ske}

\begin{tcolorbox}[adjusted title=My title]
  This is my content.
\end{tcolorbox}
\begin{tcolorbox}[skin=beamer,beamer,adjusted title=My title]
  This is my content.
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}

\begin{docTcbKey}{skin first}{=\meta{name}}{style, no default, initially \texttt{standard}}
  If the box is set to be \refKey{/tcb/breakable} and \emph{is} broken actually,
  then the skin for the \emph{first} part of the break sequence
  is set to \meta{name}, see Subsection \ref{subsec:breaksequence} on page \pageref{subsec:breaksequence}.
  Typically, this key is set by a \refKey{/tcb/skin}.
\end{docTcbKey}


\begin{docTcbKey}{skin middle}{=\meta{name}}{style, no default, initially \texttt{standard}}
  If the box is set to be \refKey{/tcb/breakable} and \emph{is} broken actually,
  then the skin for the \emph{middle} parts (if any) of the break sequence
  is set to \meta{name}, see Subsection \ref{subsec:breaksequence} on page \pageref{subsec:breaksequence}.
  Typically, this key is set by a \refKey{/tcb/skin}.
\end{docTcbKey}


\begin{docTcbKey}{skin last}{=\meta{name}}{style, no default, initially \texttt{standard}}
  If the box is set to be \refKey{/tcb/breakable} and \emph{is} broken actually,
  then the skin for the \emph{last} part of the break sequence
  is set to \meta{name}, see Subsection \ref{subsec:breaksequence} on page \pageref{subsec:breaksequence}.
  Typically, this key is set by a \refKey{/tcb/skin}.
\end{docTcbKey}


\clearpage

\begin{docTcbKey}{graphical environment}{=\meta{name}}{no default, initially \texttt{pgfpicture}}
  Sets the graphical environment for the |tcolorbox| to \meta{name}.
  Feasible values are |pgfpicture| and |tikzpicture| or environments which
  inherit from one of these two. This key is set by a \refKey{/tcb/skin} and
  may seldom be used directly.
\end{docTcbKey}

The skin of a |tcolorbox| is drawn by up to four \emph{engines}.
Afterwards, the text content is drawn which is not part of a skin.
The four steps are:
\begin{enumerate}
\item The \emph{frame} of the box, drawn by \refKey{/tcb/frame engine}.
\item The \emph{interior} of the box. The interior of a box with title is
  drawn differently from a box without title.
  \refKey{/tcb/interior titled engine} or \refKey{/tcb/interior engine}
  is used to draw the interior.
\item The \emph{segmentation} (line) of the box, if there is a lower part;
  drawn by \refKey{/tcb/segmentation engine}.
\item The \emph{title area} of the box, if there is a title and
  \refKey{/tcb/title filled} is set to |true|; drawn
  by \refKey{/tcb/title engine}.
\end{enumerate}

%Every engine for the up to four steps can be set to one of the following types:
%\begin{enumerate}
%\item\docValue{standard}: the original code from the core package.
%\item\docValue{path}: a |tikz| path which can be controlled by options.
%\item\docValue{pathfirst}: a |tikz| path which can be controlled by options.
%\item\docValue{pathmiddle}: a |tikz| path which can be controlled by options.
%\item\docValue{pathlast}: a |tikz| path which can be controlled by options.
%\item\docValue{freelance}: arbitrary user code.
%\item\docValue{spartan}: a quite spartan code.
%\end{enumerate}
%\clearpage

\begin{docTcbKey}{frame engine}{=\meta{name}}{no default, initially \texttt{standard}}
  Sets the \emph{frame} drawing engine for a box to \meta{name}.
  Typically, this key is set by a \refKey{/tcb/skin}.
  Feasible values for \meta{name} are:
  \begin{itemize}
  \item\docValue{standard}: the original code from the core package,
  \item\docValue{path}: a |tikz| path which is controlled by \refKey{/tcb/frame style},
  \item\docValue{pathjigsaw}: a |tikz| path which is controlled by \refKey{/tcb/frame style},
  \item\docValue{pathfirst}: a |tikz| path which is controlled by \refKey{/tcb/frame style},
  \item\docValue{pathfirstjigsaw}: a |tikz| path which is controlled by \refKey{/tcb/frame style},
  \item\docValue{pathmiddle}: a |tikz| path which is controlled by \refKey{/tcb/frame style},
  \item\docValue{pathmiddlejigsaw}: a |tikz| path which is controlled by \refKey{/tcb/frame style},
  \item\docValue{pathlast}: a |tikz| path which is controlled by \refKey{/tcb/frame style},
  \item\docValue{pathlastjigsaw}: a |tikz| path which is controlled by \refKey{/tcb/frame style},
  \item\docValue{freelance}: deprecated.
  \item\docValue{spartan}: a quite spartan code.
  \item\docValue{empty}: draw nothing.
\end{itemize}
\end{docTcbKey}

\begin{docTcbKey}{interior titled engine}{=\meta{name}}{no default, initially \texttt{standard}}
  Sets the \emph{interior} drawing engine for a titled box to \meta{name}.
  Typically, this key is set by a \refKey{/tcb/skin}.
  Feasible values for \meta{name} are:
  \begin{itemize}
  \item\docValue{standard}: the original code from the core package,
  \item\docValue{path}: a |tikz| path which is controlled by \refKey{/tcb/interior style},
  \item\docValue{pathfirst}: a |tikz| path which is controlled by \refKey{/tcb/interior style},
  \item\docValue{pathmiddle}: a |tikz| path which is controlled by \refKey{/tcb/interior style},
  \item\docValue{pathlast}: a |tikz| path which is controlled by \refKey{/tcb/interior style},
  \item\docValue{freelance}: deprecated.
  \item\docValue{spartan}: a quite spartan code.
  \item\docValue{empty}: draw nothing.
  \end{itemize}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{interior engine}{=\meta{name}}{no default, initially \texttt{standard}}
  Sets the \emph{interior} drawing engine for an untitled box to \meta{name}.
  Typically, this key is set by a \refKey{/tcb/skin}.
  Feasible values for \meta{name} are:
  \begin{itemize}
  \item\docValue{standard}: the original code from the core package,
  \item\docValue{path}: a |tikz| path which is controlled by \refKey{/tcb/interior style},
  \item\docValue{pathfirst}: a |tikz| path which is controlled by \refKey{/tcb/interior style},
  \item\docValue{pathmiddle}: a |tikz| path which is controlled by \refKey{/tcb/interior style},
  \item\docValue{pathlast}: a |tikz| path which is controlled by \refKey{/tcb/interior style},
  \item\docValue{freelance}: deprecated.
  \item\docValue{spartan}: a quite spartan code.
  \item\docValue{empty}: draw nothing.
  \end{itemize}
\end{docTcbKey}

\begin{docTcbKey}{segmentation engine}{=\meta{name}}{no default, initially \texttt{standard}}
  Sets the \emph{segmentation} (line) drawing engine for a box to \meta{name}.
  Typically, this key is set by a \refKey{/tcb/skin}.
  Feasible values for \meta{name} are:
  \begin{itemize}
  \item\docValue{standard}: the original code from the core package,
  \item\docValue{path}: a |tikz| path which is controlled by \refKey{/tcb/segmentation style},
  \item\docValue{freelance}: deprecated.
  \item\docValue{spartan}: a quite spartan code.
  \item\docValue{empty}: draw nothing.
  \end{itemize}
\end{docTcbKey}

\begin{docTcbKey}{title engine}{=\meta{name}}{no default, initially \texttt{standard}}
  Sets the \emph{title area} drawing engine for a titled box to \meta{name}.
  Typically, this key is set by a \refKey{/tcb/skin}.
  Feasible values for \meta{name} are:
  \begin{itemize}
  \item\docValue{standard}: the original code from the core package,
  \item\docValue{path}: a |tikz| path which is controlled by \refKey{/tcb/title style},
  \item\docValue{pathfirst}: a |tikz| path which is controlled by \refKey{/tcb/title style},
  \item\docValue{pathmiddle}: a |tikz| path which is controlled by \refKey{/tcb/title style},
  \item\docValue{pathlast}: a |tikz| path which is controlled by \refKey{/tcb/title style},
  \item\docValue{freelance}: deprecated.
  \item\docValue{spartan}: a quite spartan code.
  \item\docValue{empty}: draw nothing.
  \end{itemize}
\end{docTcbKey}

\begin{marker}
After an engine is set to an initializing value, the resulting graphical
code can be changed using code option keys, see \Vref{subsec:addcodeoptions}.
\end{marker}

\clearpage
\begin{docTcbKey}{geometry nodes}{\colOpt{=true\textbar false}}{default |true|, initially |false|}
  If set to |true|, up to four |tikz| nodes are defined for a |tcolorbox|
  which are named |frame|, |interior|, |segmentation|, and |title|. These nodes
  describe the boundaries of the equally named parts of a |tcolorbox|.
  They are used by most engines based on \tikzname.
  Typically, this key is set automatically by a \refKey{/tcb/skin}.
\begin{dispExample}
\tcbset{colback=Salmon!50!white,colframe=FireBrick!75!black,
  width=(\linewidth-8mm)/2,before=,after=\hfill,equal height group=geon}

\begin{tcolorbox}[adjusted title=The title]
  The upper part.\tcblower The lower part.
\end{tcolorbox}
\begin{tcolorbox}[enhanced,adjusted title=The title,
  frame code={\path[draw=red,fill=red!25]
      (frame.south west) rectangle (frame.north east);},
  interior titled code={\path[draw=blue,fill=blue!25]
      (interior.south west) rectangle (interior.north east);},
  segmentation code={\path[draw=green,fill=green!25]
      (segmentation.south west) rectangle (segmentation.north east);},
  title code={\path[draw=black,fill=brown!75!black]
      (title.south west) rectangle (title.north east);}]
  The upper part.\tcblower The lower part.
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}






\clearpage
\subsection{Code Option Keys}\label{subsec:addcodeoptions}
The following code options are applicable for all skins.
%which
%use engines of type |freelance|.
%Especially, the skin \refSkin{freelance} supports \emph{all} of them,
%\refSkin{standard} and \refSkin{enhanced} \emph{none} of them.
The used \meta{graphical code} can be any |pgf| code. For all skins
with exception of \refSkin{standard}
and \refSkin{standard jigsaw}, the \meta{graphical code} can also
be any \tikzname\ code.


\begin{docTcbKey}{frame code}{\colOpt{=\meta{graphical code}}}{code, default from |standard|}
  The given \meta{graphical code} is used for drawing the \emph{frame} of the box.
  %This option is available only if the \refKey{/tcb/frame engine} is set to |freelance|.
\begin{dispExample}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[enhanced,frame code={
  \foreach \n in {north east,north west,south east,south west}
  {\path [fill=red!75!black] (interior.\n) circle (3mm); }; }]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{frame empty}{}{style, no value}
  This is a shortcut for setting  \refKey{/tcb/frame code} to empty.
  This option removes the drawing of the frame.
  Alternatively, use \refKey{/tcb/frame hidden}.
\end{docTcbKey}


\begin{docTcbKey}{interior titled code}{\colOpt{=\meta{graphical code}}}{code, default from |standard|}
  The given \meta{graphical code} is used
  for drawing the \emph{interior} of the box, if the box comes with a title.
  %This option is available only if the \refKey{/tcb/interior titled engine} is set to |freelance|.
\begin{dispExample}
\tcbset{colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[enhanced,title=My title,interior titled code={
  \path[draw=red!5!white,line width=5mm,line cap=round]
    ([xshift=3mm,yshift=-3mm]interior.north west)
    --([xshift=-3mm,yshift=3mm]interior.south east)
    ([xshift=3mm,yshift=3mm]interior.south west)
    --([xshift=-3mm,yshift=-3mm]interior.north east);}]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{interior titled empty}{}{style, no value}
  This is a shortcut for setting  \refKey{/tcb/interior titled code} to empty.
  This option removes the drawing of the untitled interior.
  Alternatively, use \refKey{/tcb/interior hidden}.
\end{docTcbKey}



\clearpage
\begin{docTcbKey}{interior code}{\colOpt{=\meta{graphical code}}}{code, default from |standard|}
  The given \meta{graphical code} is used
  for drawing the \emph{interior} of the box, if the box is without a title.%\\
  %This option is available only if the \refKey{/tcb/interior engine} is set to |freelance|.
\begin{dispExample}
\tcbset{colback=red!5!white,colframe=red!75!black}

\begin{tcolorbox}[enhanced,interior code={
  \path[draw=red!5!white,line width=5mm,line cap=round]
    ([xshift=3mm,yshift=-3mm]interior.north west)
    --([xshift=-3mm,yshift=3mm]interior.south east)
    ([xshift=3mm,yshift=3mm]interior.south west)
    --([xshift=-3mm,yshift=-3mm]interior.north east);}]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}

\begin{docTcbKey}{interior empty}{}{style, no value}
  This is a shortcut for setting  \refKey{/tcb/interior code} to empty.
  This option removes the drawing of the interior.
  Alternatively, use \refKey{/tcb/interior hidden}.
\end{docTcbKey}


\begin{docTcbKey}{segmentation code}{\colOpt{=\meta{graphical code}}}{code, default from |standard|}
  The given \meta{graphical code} is used for drawing the
  \emph{segmentation} area of the box.%\\
  %This option is available only if the \refKey{/tcb/segmentation engine} is set to |freelance|.
\begin{dispExample}
\tcbset{colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries}

\begin{tcolorbox}[enhanced,title=My title,segmentation code={
  \path[top color=red!5!white,bottom color=red!5!white,middle color=blue]
  (segmentation.south west) rectangle (segmentation.north east);}]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{segmentation empty}{}{style, no value}
  This is a shortcut for setting  \refKey{/tcb/segmentation code} to empty.
  This option removes the drawing of the segmentation line.
  Alternatively, use \refKey{/tcb/segmentation hidden}.
\end{docTcbKey}



\clearpage
\begin{docTcbKey}{title code}{\colOpt{=\meta{graphical code}}}{code, default from |standard|}
  The given \meta{graphical code} is used for drawing the
  \emph{title} area of the box.
  %\\
  %This option is available only if the \refKey{/tcb/title engine} is set to |freelance|.
\begin{dispExample}
\tcbset{colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries,
  coltitle=black}

\begin{tcolorbox}[enhanced,title=My title,title code={
  \path[draw=yellow,solid,decorate,line width=2mm,
    decoration={coil,aspect=0,segment length=10.1mm}]
    ([xshift=1mm]title.west) -- ([xshift=-1mm]title.east);}]
This is a \textbf{tcolorbox}.
\tcblower
This is the lower part.
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{title empty}{}{style, no value}
  This is a shortcut for setting  \refKey{/tcb/title code} to empty.
  This option removes the drawing of the title area.
  Alternatively, use \refKey{/tcb/title hidden}.
\end{docTcbKey}

\clearpage
\subsection{Subskins}\label{subsec:subskins}
A subskin is a new \refKey{/tcb/skin} based on an existing skin which
is extended or changed.

\begin{marker}
Never use geometry settings or bounding box options inside a subskin definition!
If one skin is replaced by another skin, the overall bounding box should stay
constant. Especially, if a skin is used for a breakable box, unpredictable
and unpleasant results could arise otherwise. If you want to change the
geometry also, use an additional style. See the skin \refSkin{beamer} and
the style \refKey{/tcb/beamer} as pattern.
\end{marker}

\begin{docCommand}{tcbsubskin}{\marg{name}\marg{base skin}\marg{options}}
  Creates a new skin \meta{name} which inherits all properties of an
  existing \meta{base skin} plus the given \meta{options}.
  The new skin \meta{name} can be used as value for the keys
  \refKey{/tcb/skin},
  \refKey{/tcb/skin first},
  \refKey{/tcb/skin middle}, and
  \refKey{/tcb/skin last}.
  As \meta{base skin}, one can take \refSkin{standard}, \refSkin{empty},
  \refSkin{enhanced}, or any skin from the \mylib{skins} library,
  see \Vref{sec:skins}.

\begin{dispExample}
% \tcbuselibrary{skins}
\tcbsubskin{mycross}{empty}{frame code={%
  \draw[red,line width=5pt] (frame.south west)--(frame.north east);
  \draw[red,line width=5pt] (frame.north west)--(frame.south east);},
  skin first=mycross,skin middle=mycross,skin last=mycross }

\begin{tcolorbox}[skin=mycross]
  This is my content.
\end{tcolorbox}
\end{dispExample}

\end{docCommand}


\begin{docTcbKey}{skin first is subskin of}{=\marg{base skin}\marg{options}}{no default, initially unset}
  Creates a new unnamed skin which inherits all properties of an
  existing \meta{base skin} plus the given \meta{options}.
  This skin is set as \refKey{/tcb/skin first}.\\
  See a detailed example on page~\pageref{freeboxexample}.
\end{docTcbKey}


\begin{docTcbKey}{skin middle is subskin of}{=\marg{base skin}\marg{options}}{no default, initially unset}
  Creates a new unnamed skin which inherits all properties of an
  existing \meta{base skin} plus the given \meta{options}.
  This skin is set as \refKey{/tcb/skin middle}.\\
  See a detailed example on page~\pageref{freeboxexample}.
\end{docTcbKey}


\begin{docTcbKey}{skin last is subskin of}{=\marg{base skin}\marg{options}}{no default, initially unset}
  Creates a new unnamed skin which inherits all properties of an
  existing \meta{base skin} plus the given \meta{options}.
  This skin is set as \refKey{/tcb/skin last}.\\
  See a detailed example on page~\pageref{freeboxexample}.
\end{docTcbKey}


\clearpage
\subsection{Drawing Scheme}\label{subsec:tcolorboxdrawing}

\bgroup

Depending on the complexity of a |tcolorbox| definition, the resulting box
is drawn in a more or less complex series of steps.

To document and demonstrate these drawing steps, we consider the
following box definition:

\begin{dispListing}
\newtcolorbox{testbox}[1][]{enhanced,title=Test Box,
  boxrule=1mm,titlerule=0.5mm,colframe=blue!50!black,
  interior style={top color=blue!20!green!50!white,bottom color=blue!20!yellow!50!white},
  colbacktitle=blue!50!green!90!white,segmentation style={solid},
  fonttitle=\bfseries,drop fuzzy shadow,borderline={0.3mm}{0.35mm}{yellow!50!white},
  underlay={\path[fill image opacity=0.15,fill image scale=0.9,
    fill stretch picture={\draw[blue,line width=2mm] circle (1);}]
    (interior.south west) rectangle (interior.north east);},
  watermark text={Watermark},watermark color={green!20!white},
  finish={\begin{tcbclipframe}
    \path[bottom color=black,top color=black!50!white,opacity=0.1]
      (frame.south west) -- (frame.south east) -- (frame.north east) -- cycle;
    \path[top color=white,bottom color=black!50!white,opacity=0.1]
      (frame.south west) -- (frame.north east) -- (frame.north west) -- cycle;
    \end{tcbclipframe}},#1}
\end{dispListing}
\tcbusetemp

For this definition, we get the maximal number of drawing steps:

\newtcolorbox{itembox}{oversize,enhanced,frame empty,segmentation empty,colback=white,middle=2mm,boxsep=0pt,
  fuzzy halo=0.5mm with blue!15!white,
  before lower=\raggedright\begin{itemize},after lower=\end{itemize}}

\tcbset{finishcomment/.style={
  finish={\node[fill=white,draw=black!50!white,rounded corners] at (frame.center) {#1};}
}}


\begin{itembox}
\begin{testbox}[frame empty,interior titled empty,title empty,segmentation empty,
  no shadow,no borderline,no underlay,no overlay,no finish,opacityupper=0,opacitylower=0,opacitytitle=0,
  drop fuzzy shadow=red!75!white,
  finishcomment={1.~shadow}]
\lipsum[2]
\tcblower
Lower part
\end{testbox}
\tcblower
\item Section~\ref{subsec:shadows} on page \pageref{subsec:shadows}.
\end{itembox}

\begin{itembox}
\begin{testbox}[interior titled empty,title empty,segmentation empty,
  no borderline,no underlay,no overlay,no finish,opacityupper=0,opacitylower=0,opacitytitle=0,
  colframe=red!75!white,
  finishcomment={2.~frame}]
\lipsum[2]
\tcblower
Lower part
\end{testbox}
\tcblower
\item\refKey{/tcb/colframe}, \refKey{/tcb/opacityframe}
\item\refKey{/tcb/frame code}
\item\refKey{/tcb/frame style}
\end{itembox}


\begin{itembox}
\begin{testbox}[title empty,segmentation empty,
  no borderline,no underlay,no overlay,no finish,opacityupper=0,opacitylower=0,opacitytitle=0,
  colback=red!75!white,
  finishcomment={3.~interior}]
\lipsum[2]
\tcblower
Lower part
\end{testbox}
\tcblower
\item\refKey{/tcb/colback}, \refKey{/tcb/opacityback}
\item\refKey{/tcb/interior code}, \refKey{/tcb/interior titled code}
\item\refKey{/tcb/interior style}
\end{itembox}


\begin{itembox}
\begin{testbox}[segmentation empty,
  no borderline,no underlay,no overlay,no finish,opacityupper=0,opacitylower=0,opacitytitle=0,
  colbacktitle=red!75!white,
  finishcomment={4.~title area}]
\lipsum[2]
\tcblower
Lower part
\end{testbox}
\tcblower
\item\refKey{/tcb/colbacktitle}, \refKey{/tcb/opacitybacktitle}
\item\refKey{/tcb/title code}
\item\refKey{/tcb/title style}
\end{itembox}


\begin{itembox}
\begin{testbox}[
  no borderline,no underlay,no overlay,no finish,opacityupper=0,opacitylower=0,opacitytitle=0,
  segmentation style={solid,red!75!white},
  finishcomment={5.~segmentation}]
\lipsum[2]
\tcblower
Lower part
\end{testbox}
\tcblower
\item\refKey{/tcb/lower separated}
\item\refKey{/tcb/segmentation code}
\item\refKey{/tcb/segmentation style}
\end{itembox}


\begin{itembox}
\begin{testbox}[
  no borderline,no underlay,no overlay,no finish,opacityupper=0,opacitylower=0,opacitytitle=0,
  borderline={0.3mm}{0.35mm}{red!75!white},
  finishcomment={6.~border line}]
\lipsum[2]
\tcblower
Lower part
\end{testbox}
\tcblower
\item\Vref{subsec:borderline}
\end{itembox}


\begin{itembox}
\begin{testbox}[
  no underlay,no overlay,no finish,opacityupper=0,opacitylower=0,opacitytitle=0,
  underlay={\path[opacity=0.15,fill image scale=0.9,
    fill stretch picture={\draw[red,line width=2mm] circle (1);}]
    (interior.south west) rectangle (interior.north east);},
  finishcomment={7.~underlay}]
\lipsum[2]
\tcblower
Lower part
\end{testbox}
\tcblower
\item\Vref{subsec:skinboxedtitle}
\item\Vref{subsec:skinunderlay}
\end{itembox}


\begin{itembox}
\begin{testbox}[
  no finish,opacityupper=0,opacitylower=0,opacitytitle=0,
  watermark color={red!75!white},
  finishcomment={8.~overlay}]
\lipsum[2]
\tcblower
Lower part
\end{testbox}
\tcblower
\item\Vref{subsec:overlays}
\item\Vref{subsec:watermarks}
\end{itembox}


\begin{itembox}
\begin{testbox}[
  no finish,
  colupper=red!75!white,coltitle=red!75!white,collower=red!75!white,
  finishcomment={9.~text content}]
\lipsum[2]
\tcblower
Lower part
\end{testbox}
\tcblower
\item\refKey{/tcb/colupper}, \refKey{/tcb/collower}, \refKey{/tcb/coltitle}
\item\refKey{/tcb/fontupper}, \refKey{/tcb/fontlower}, \refKey{/tcb/fonttitle}
\item\refKey{/tcb/opacityupper}, \refKey{/tcb/opacitylower}, \refKey{/tcb/opacitytitle}
\end{itembox}


\begin{itembox}
\begin{testbox}[
  finishcomment={10.~finish}]
\lipsum[2]
\tcblower
Lower part
\end{testbox}
\tcblower
\item\Vref{subsec:skinfinish}
\end{itembox}

All together, the box is drawn:
\begin{dispExample}
% \usepackage{lipsum}
\begin{testbox}
\lipsum[2]
\tcblower
Lower part
\end{testbox}
\end{dispExample}

\egroup


\clearpage
\subsection{Color Names}\label{subsec:tech_colornames}
Color settings for a |tcolorbox| are saved into named colors which may be
used inside a box, e.g. for an overlay.
\tcbdocmarginnote{\tcbdocnew{2019-01-18}}
These color names are
\begin{itemize}
\item\docColor{tcbcolframe} set by \refKey{/tcb/colframe} (frame color)
\item\docColor{tcbcolback} set by \refKey{/tcb/colback} (background color)
\item\docColor{tcbcolbacktitle} set by \refKey{/tcb/colbacktitle} (background color of the title)
\item\docColor{tcbcolbacklower} set by \refKey{/tcb/colbacklower} (skin dependend background color
  of the lower part; needs \mylib{skins} to be loaded)
\item\docColor{tcbcolupper} set by \refKey{/tcb/colupper} (text color upper part)
\item\docColor{tcbcollower} set by \refKey{/tcb/collower} (text color lower part)
\item\docColor{tcbcoltitle} set by \refKey{/tcb/coltitle} (text color title)
\end{itemize}

\medskip

\begin{dispExample}
% \tcbuselibrary{skins}
\begin{tcolorbox}[title=Color names,
    colframe=blue!50!black,colback=blue!5,
    colbacktitle=blue!50,colupper=red!35!black]
  \foreach \name in {tcbcolframe,tcbcolback,tcbcolbacktitle,tcbcolbacklower,
    tcbcolupper,tcbcollower,tcbcoltitle}
  {\tikz\path[draw,fill=\name]
    (0,0) rectangle node[right=4mm,font=\ttfamily]{\name} (0.8,0.8);\par}
\end{tcolorbox}
\end{dispExample}



\clearpage
\subsection{Useful Properties}\label{subsec:tech_properties}

The following macros describe certain \textit{properties} which may be
used for the drawing scheme, see \Fullref{subsec:tcolorboxdrawing}.
Sometimes, they are even available inside the box content. All of them are
considered to be \textit{read-only} and should never be redefined by the user.

\begin{docCommand}[doc new=2016-02-16]{tcbheightspace}{}
  If the height of a |tcolorbox| is not the natural height, the space
  difference between the forced and the natural size is hold by
  \refCom{tcbheightspace}.
  This macro is not usable inside the box content, but for skins or
  inside \refKey{/tcb/underlay}, \refKey{/tcb/overlay}, etc.

  If such a space information is needed inside the box content, see
  \refKey{/tcb/space to} instead.
\begin{dispExample}
% \tcbuselibrary{skins}
\newtcolorbox{testbox}[2][]{enhanced,size=fbox,
  colframe=blue!75!black,colback=white,height=#2,
  underlay={\node[above,inner sep=3pt] at (interior.south){%
    \includegraphics[width=\tcbtextwidth,height=\tcbheightspace-3pt]{goldshade.png}};
    },
  #1}
\begin{testbox}{3cm}
  This is my box. The space is filled with a picture.
\end{testbox}
\begin{testbox}{2cm}
  This is my box. The space is filled with a picture.
\end{testbox}
\end{dispExample}
\end{docCommand}


\begin{docCommand}[doc new=2016-02-16]{tcbtextwidth}{}
  This property describes the box content width.
  \begin{itemize}
  \item  If there also is a lower part, it describes the width of the upper part.
  \item For \refKey{/tcb/sidebyside} boxes, it describes the combined text
    width plus segmentation.
  \item This property can be used inside the box content text with exception
    of \refKey{/tcb/fit} boxes.
  \item \refCom{tcbtextwidth} can be used for all box types for skins or
    inside \refKey{/tcb/underlay}, \refKey{/tcb/overlay}, etc.
  \end{itemize}
\begin{dispExample}
\begin{tcolorbox}[colframe=blue!75!black]
  Inside a box: \tcbtextwidth\ (=\the\linewidth).
\end{tcolorbox}
\end{dispExample}
\end{docCommand}

\pagebreak
\begin{docCommand}[doc new=2016-02-16]{tcbtextheight}{}
  This property describes the designated box content height. If the
  box is larger than the natural height, the actual content will be smaller
  than \refCom{tcbtextheight}.
  \begin{itemize}
  \item For boxes with a fixed \refKey{/tcb/height}, this property can
    be used inside the box content text. For other boxes, it denotes |0pt|
    inside the box content.
  \item \refCom{tcbtextheight} can be used for all box types for skins or
    inside \refKey{/tcb/underlay}, \refKey{/tcb/overlay}, etc.
  \end{itemize}

\begin{dispExample}
% \tcbuselibrary{skins}
\begin{tcolorbox}[enhanced,colframe=blue!75!black,
    underlay={\node[left,red] at (frame.east) {Here: \tcbtextheight};}]
  Inside a box with natural height: \tcbtextheight.
\end{tcolorbox}
\begin{tcolorbox}[enhanced,colframe=blue!75!black,height=1cm,
    underlay={\node[left,red] at (frame.east) {Here: \tcbtextheight};}]
  Inside a box with fixed height: \tcbtextheight.
\end{tcolorbox}
\end{dispExample}
\end{docCommand}


\begin{docCommand}[doc new=2017-04-25]{tcbsegmentstate}{}
  This macro contains |0|, |1|, or |2|. Itis set for every unbroken box and every broken partial box
  with the following meaning:
  \begin{itemize}
    \item\docValue{0}: The current (partial) box contains only an upper part.
    \item\docValue{1}: The current (partial) box contains an upper and a lower part.
      The segmentation node can be used for positioning.
    \item\docValue{2}: The current (partial) box contains only a lower part.
      This can only be true for parts of breakable boxes.
  \end{itemize}
  Skins like \refSkin{bicolor} use this property to paint the (partial) boxes.
\begin{dispExample}
% \tcbuselibrary{skins,raster}
\begin{tcbraster}[raster equal height,enhanced,
    watermark text=\tcbsegmentstate]
  \begin{tcolorbox}Upper part\end{tcolorbox}
  \begin{tcolorbox}Upper part\tcblower Lower part\end{tcolorbox}
\end{tcbraster}
\end{dispExample}
\end{docCommand}


==> tcolorbox.doc.theorems.tex <==
% !TeX root = tcolorbox.tex
% include file of tcolorbox.tex (manual of the LaTeX package tcolorbox)
\clearpage
\section{Library \mylib{theorems}}\label{sec:theorems}%
\tcbset{external/prefix=external/theorems_}%
The library is loaded by a package option or inside the preamble by:
\begin{dispListing}
\tcbuselibrary{theorems}
\end{dispListing}
This also loads the package |amsmath|.

\subsection{Macros of the Library}

\begin{docCommand}[doc updated=2016-06-22]{newtcbtheorem}{\oarg{init options}\marg{name}\marg{display name}\marg{options}\marg{prefix}}
  Creates new environments \meta{name} and \meta{name}|*| based on |tcolorbox| to frame a
  (mathematical) theorem. The \meta{display name} is used in the title line
  with a number, e.\,g. \mbox{\flqq Theorem 5.1\frqq}.
  The \meta{options} are given to the underlying |tcolorbox| to control
  the appearance.
  %The \meta{counter} is used for automatic numbering.
  The \meta{init options} allow setting up automatic numbering,
  see \Vref{sec:initkeys}.\par
  The new environment \meta{name} takes one optional and two mandatory
  parameters. The optional parameter supplements the options and should be
  used only in rare cases.
  The first mandatory parameter is the title text for the theorem and
  is also set as \refKey{/tcb/nameref} identifier.
  The second mandatory parameter is a \meta{marker}. The theorem is
  automatically labeled with \meta{prefix}\meta{separator}\meta{marker}
  where \meta{separator} is predefined as '|:|', see \refKey{/tcb/label separator}.\par
  The new environment \meta{name}|*| takes one optional and one mandatory
  parameter and represents an unnumbered variant of the environment \meta{name}.
  This variant is not labeled and not listed in lists of theorems.
\enlargethispage*{20mm}
\inputpreamblelisting{F}
\begin{dispExample}
% usage of '\nameref' needs 'nameref' or 'hyperref' to be loaded
\begin{mytheo}{This is my title}{theoexample}
  This is the text of the theorem. The counter is automatically assigned and,
  in this example, prefixed with the section number. This theorem is numbered with
  \ref{th:theoexample}, it is given on page~\pageref{th:theoexample},
  and it is titled \flqq\nameref{th:theoexample}\frqq.
\end{mytheo}
\end{dispExample}

\begin{dispExample}
\begin{mytheo}[label=myownlabel]{This is my title}{}
  The label parameter can be left empty without \LaTeX\ error.
  Or you may use an own label to reference Theorem \ref{myownlabel}.
\end{mytheo}
\end{dispExample}

\begin{dispExample}
\begin{mytheo}{}{}
  The title can also be left empty without problem. Note that the ':'
  vanished magically.
\end{mytheo}
\end{dispExample}

\begin{dispExample}
\begin{mytheo*}{Unnumbered Theorem}
  This theorem is not numbered.
\end{mytheo*}
\end{dispExample}

\begin{dispExample}
\begin{mytheo*}{}
  This theorem has no number and no title.
\end{mytheo*}
\end{dispExample}

\begin{marker}
To switch off the \texttt{nameref} feature permanently, add
\mbox{\texttt{nameref/.style=\{\}}} inside the \meta{options} list.
\end{marker}

\end{docCommand}


\begin{docCommand}{renewtcbtheorem}{\oarg{init options}\marg{name}\marg{display name}\marg{options}\marg{prefix}}
  Operates like \refCom{newtcbtheorem}, but based on |\renewenvironment| instead of |\newenvironment|.
  An existing environment is redefined.
\end{docCommand}


\begin{docCommand}{tcbmaketheorem}{\marg{name}\marg{display name}\marg{options}\marg{counter}\marg{prefix}}
\smallskip\begin{marker}
\refCom{newtcbtheorem} supersedes this macro.
\end{marker}
\begin{deprecated}
  Creates a new environment \meta{name} based on |tcolorbox| to frame a
  (mathematical) theorem. The \meta{display name} is used in the title line
  with a number, e.\,g. \mbox{\flqq Theorem 5.1\frqq}.
  The \meta{options} are given to the underlying |tcolorbox| to control
  the appearance.
  The \meta{counter} is used for automatic numbering.
  The new environment \meta{name} takes one optional and two mandatory
  parameters. The optional parameter supplements the options and should be
  used only in rare cases.
  The first mandatory parameter is the title text for the theorem and
  the second mandatory parameter is a \meta{marker}. The theorem is
  automatically labeled with \meta{prefix}\meta{separator}\meta{marker}
  where \meta{separator} is predefined as '|:|', see \refKey{/tcb/label separator}.
\end{deprecated}
\end{docCommand}

\clearpage
\begin{docCommand}{tcboxmath}{\oarg{options}\marg{mathematical box content}}
  Creates a \refEnv{tcolorbox} which is fitted to the width of the given
  \meta{mathematical box content}. This box is intended to be applied as
  part of a larger formula and may be used as replacement for the |\boxed|
  macro of |amsmath|.

\begin{dispExample}
\begin{equation}
\tcbset{fonttitle=\scriptsize}
\tcboxmath[colback=LightBlue!25!white,colframe=blue]{ a^2 = 16 }
\quad \Rightarrow \quad
\tcboxmath[colback=Salmon!25!white,colframe=red,title=Implication]%
  { a = 4 ~\vee~ a=-4. }
\end{equation}
\end{dispExample}
\end{docCommand}

\begin{docCommand}{tcbhighmath}{\oarg{options}\marg{mathematical box content}}
  This is a special case of the \refCom{tcboxmath} macro which uses
  the style \refKey{/tcb/highlight math}.
  It is intended to provide context sensitive highlighting of formula parts.
  The color settings via \refKey{/tcb/highlight math style} may be different
  inside theorems or other colored areas and outside.

\begin{dispExample}
\tcbset{myformula/.style={colback=yellow!10!white,colframe=red!50!black,
  every box/.style={highlight math style={colback=LightBlue!50!white,colframe=Navy}}
  }}

\begin{align}
  \tcbhighmath{\sum\limits_{n=1}^{\infty} \frac{1}{n}} &= \infty.\\
  \int x^2 ~\text{d}x                     &= \frac13 x^3 + c.
\end{align}

\begin{tcolorbox}[ams align,myformula]
  \tcbhighmath{\sum\limits_{n=1}^{\infty} \frac{1}{n}} &= \infty.\\
  \int x^2 ~\text{d}x                     &= \frac13 x^3 + c.
\end{tcolorbox}
\end{dispExample}

\clearpage
\refCom{tcbhighmath} can be used in symbiosis with the |empheq| package
which allows to specify own boxing commands to mark multiline formulas.

\begin{dispExample}
% \usepackage{empheq}
\begin{empheq}[box=\tcbhighmath]{align}
a&=\sin(z)\\
E&=mc^2 + \int_a^b x\, dx
\end{empheq}

\tcbset{highlight math style={enhanced,
  colframe=red!60!black,colback=yellow!50!white,arc=4pt,boxrule=1pt,
  drop fuzzy shadow}}

\begin{empheq}[box=\tcbhighmath]{align}
a&=\sin(z)\\
E&=mc^2 + \int_a^b x\, dx
\end{empheq}
\end{dispExample}

Besides \refCom{tcbhighmath}, one can easily define an independent new box
based on \refCom{tcbox} which acts like \refCom{tcbhighmath}:

\begin{dispExample}
% \usepackage{empheq}
\newtcbox{\otherbox}[1][]{nobeforeafter,math upper,tcbox raise base,
  enhanced,frame hidden,boxrule=0pt,interior style={top color=green!10!white,
  bottom color=green!10!white,middle color=green!50!yellow},
  fuzzy halo=1pt with green,#1}

\begin{empheq}[box=\otherbox]{align}
a&=\sin(z)\\
E&=mc^2 + \int_a^b x\, dx
\end{empheq}

\begin{equation}
\tcbhighmath{E} = \otherbox{mc^2}
\end{equation}
\end{dispExample}
\end{docCommand}


\clearpage
\subsection{Option Keys of the Library}


\begin{docTcbKey}{separator sign}{=\meta{sign}}{no default, initially |:|}
  The given \meta{sign} is used inside the title text of a theorem
  as separater between display name combined with number and
  the specific title text. It is omitted, if there is no specific title text.

\begin{dispExample}
% \usepackage{amssymb}
\newtcbtheorem[use counter from=mytheo]{sometheorem}{Theorem}%
  {colback=white,colframe=red!50!black,fonttitle=\bfseries,
   separator sign={\ $\blacktriangleright$}}{theo}
\begin{sometheorem}{My example}{}
My theorem text.
\end{sometheorem}
\end{dispExample}
\end{docTcbKey}

\begin{docTcbKey}{separator sign colon}{}{style, no value, initially set}
Sets \refKey{/tcb/separator sign} to the default colon |:| sign.
\end{docTcbKey}

\begin{docTcbKey}{separator sign dash}{}{style, no value}
Sets \refKey{/tcb/separator sign} to an en-dash sign.
\begin{dispExample}
\newtcbtheorem[use counter from=mytheo]{sometheorem}{Theorem}%
  {colback=white,colframe=red!50!black,fonttitle=\bfseries,
   separator sign dash}{theo}
\begin{sometheorem}{My example}{}
My theorem text.
\end{sometheorem}
\end{dispExample}
\end{docTcbKey}

\begin{docTcbKey}{separator sign none}{}{style, no value}
Sets \refKey{/tcb/separator sign} to empty.
\begin{dispExample}
\newtcbtheorem[use counter from=mytheo]{sometheorem}{Theorem}%
  {colback=white,colframe=red!50!black,fonttitle=\bfseries,
   separator sign none}{theo}
\begin{sometheorem}{My example}{}
My theorem text.
\end{sometheorem}
\end{dispExample}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{description delimiters}{=\marg{left}\marg{right}}{no default, initially empty}
  The given \meta{left} and \meta{right} delimiter signs are used to frame
  the descriptive title text of a theorem.

\begin{dispExample}
\newtcbtheorem[use counter from=mytheo]{sometheorem}{Theorem}%
  {colback=white,colframe=red!50!black,fonttitle=\bfseries,
   description delimiters={\flqq}{\frqq}}{theo}
\begin{sometheorem}{My example}{}
My theorem text.
\end{sometheorem}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{description delimiters parenthesis}{}{style, no value}
Sets \refKey{/tcb/description delimiters} to |(| and |)|.
\begin{dispExample}
\newtcbtheorem[use counter from=mytheo]{sometheorem}{Theorem}%
  {colback=white,colframe=red!50!black,fonttitle=\bfseries,
   description delimiters parenthesis}{theo}
\begin{sometheorem}{My example}{}
My theorem text.
\end{sometheorem}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{description delimiters none}{}{style, no value, initially set}
Sets \refKey{/tcb/description delimiters} to the default empty texts.
\end{docTcbKey}


\begin{docTcbKey}{description color}{\colOpt{=\meta{color}}}{default empty, initially empty}
  Sets the \meta{color} of the descriptive title text deviating from \refKey{/tcb/coltitle}.
  The color is reset to \refKey{/tcb/coltitle}, if |description color| is used without value.

\begin{dispExample}
\newtcbtheorem[use counter from=mytheo]{sometheorem}{Theorem}%
  {colback=white,colframe=red!50!black,fonttitle=\bfseries,
   description color=red!25!yellow}{theo}
\begin{sometheorem}{My example}{}
My theorem text.
\end{sometheorem}
\end{dispExample}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{description font}{\colOpt{=\meta{text}}}{default empty, initially empty}
  Sets \meta{text} (e.\,g.\ font settings) before the descriptive title text deviating from \refKey{/tcb/fonttitle}.
  The \meta{text} is removed, if |description font| is used without value.

\begin{dispExample}
\newtcbtheorem[use counter from=mytheo]{sometheorem}{Theorem}%
  {colback=white,colframe=red!50!black,fonttitle=\bfseries,
   description delimiters={\glqq}{\grqq},
   description font=\mdseries\itshape}{theo}
\begin{sometheorem}{My example}{}
My theorem text.
\end{sometheorem}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{description formatter}{\colOpt{=\meta{macro}}}{default empty, initially empty}
  Sets \meta{macro} as formatter for the descriptive title text. The \meta{macro}
  has to take one mandatory argument (the description text).\\ 
  Note that \refKey{/tcb/description delimiters}, \refKey{/tcb/description color},
  and \refKey{/tcb/description font} are ignored, if this option is used.\\
  If |description formatter| is used without value, the formatter is reset
  to its standard behavior.

\begin{dispExample}
\newtcbox{\formbox}{enhanced,frame empty,size=minimal,boxsep=2pt,arc=1pt,
  on line,interior style image=goldshade.png}

\newtcbtheorem[use counter from=mytheo]{sometheorem}{Theorem}%
  {colback=white,colframe=red!50!black,fonttitle=\bfseries,
   description formatter=\formbox}{theo}
\begin{sometheorem}{My example}{}
My theorem text.
\end{sometheorem}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{terminator sign}{=\meta{sign}}{no default, initially empty}
  The given \meta{sign} is used as terminator at the end of the title text of a theorem.

\begin{dispExample}
\newtcbtheorem[use counter from=mytheo]{sometheorem}{Theorem}%
  {colback=white,colframe=red!50!black,fonttitle=\bfseries,
   terminator sign={.}}{theo}
\begin{sometheorem}{My example}{}
My theorem text.
\end{sometheorem}
\end{dispExample}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{terminator sign colon}{}{style, no value, initially set}
Sets \refKey{/tcb/terminator sign} to the colon |:| sign.
\begin{dispExample}
\newtcbtheorem[use counter from=mytheo]{sometheorem}{Theorem}%
  {colback=white,colframe=red!50!black,fonttitle=\bfseries,
   separator sign dash,terminator sign colon}{theo}
\begin{sometheorem}{My example}{}
My theorem text.
\end{sometheorem}
\end{dispExample}
\end{docTcbKey}

\begin{docTcbKey}{terminator sign dash}{}{style, no value}
Sets \refKey{/tcb/terminator sign} to an en-dash sign.
\begin{dispExample}
\newtcbtheorem[use counter from=mytheo]{sometheorem}{Theorem}%
  {colback=white,colframe=red!50!black,fonttitle=\bfseries,
   terminator sign dash}{theo}
\begin{sometheorem}{My example}{}
My theorem text.
\end{sometheorem}
\end{dispExample}
\end{docTcbKey}

\begin{docTcbKey}{terminator sign none}{}{style, no value}
Sets \refKey{/tcb/terminator sign} to the default empty text.
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2016-04-19]{label separator}{=\meta{separator}}{no default, initially |:|}
  The given \meta{separator} is used for labels created with environments which
  are defined themselves by \refCom{newtcbtheorem}. This \meta{separator} is
  put between \meta{prefix} (defined by \refCom{newtcbtheorem})
  and \meta{marker} (defined by an actual theorem environment).
\begin{dispExample}
\newtcbtheorem[use counter from=mytheo]{sometheorem}{Theorem}%
  {colback=white,colframe=red!50!black,fonttitle=\bfseries,
   label separator=*}{theo}
\begin{sometheorem}{My example}{myex}
My theorem text.
\end{sometheorem}
See Example~\ref{theo*myex}.
\end{dispExample}
\end{docTcbKey}


\clearpage

\begin{docTcbKey}[][doc new=2018-01-12]{theorem full label supplement}{=\marg{style}}{no default, initially empty}
  The given \meta{style} is used in connection with labels created with environments which
  are defined themselves by \refCom{newtcbtheorem}.
  This \meta{style} uses one argument which is automatically set to the
  full label marker of the environment, i.e. a text consisting of
  \meta{prefix} (defined by \refCom{newtcbtheorem}),
  \refKey{/tcb/label separator},
  and \meta{marker} (defined by an actual theorem environment).

\begin{dispExample}
% The following adds a hyper target to all environments
% created with \newtcbtheorem
\tcbset{theorem full label supplement={hypertarget={#1}}}

\newtcbtheorem[use counter from=mytheo]{sometheorem}{Theorem}%
   {colback=white,colframe=red!50!black,fonttitle=\bfseries}{theo}
\begin{sometheorem}{My example}{myex2}
My theorem text.
\end{sometheorem}
This automated \hyperlink{theo:myex2}{hyper target can be linked to with a
 hyper link}.
\end{dispExample}

A second usage of \refKey{/tcb/theorem full label supplement} overwrites
the first setting.
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2018-01-12]{theorem label supplement}{=\marg{style}}{no default, initially empty}
  The given \meta{style} is used in connection with labels created with environments which
  are defined themselves by \refCom{newtcbtheorem}.
  This \meta{style} uses one argument which is automatically set to the
  label \meta{marker} defined by an actual theorem environment.\par
  A second usage of \refKey{/tcb/theorem label supplement} overwrites
  the first setting, but
  \refKey{/tcb/theorem full label supplement}
  and \refKey{/tcb/theorem label supplement} can be used independently.

\begin{dispExample}
% 'marginnote' has to be loaded
\newtcbtheorem[use counter from=mytheo]{sometheorem}{Theorem}%
   {colback=white,colframe=red!50!black,fonttitle=\bfseries,
    theorem label supplement={hypertarget={XYZ-##1}},
    theorem full label supplement={code={\marginnote{##1}}}
   }{theo}
\begin{sometheorem}{My example}{myex3}
My theorem text.
\end{sometheorem}
This automated \hyperlink{XYZ-myex3}{hyper target can be linked to with a
 hyper link}.
\end{dispExample}
\end{docTcbKey}



\clearpage
\begin{docTcbKey}{theorem name and number}{}{style, no value, initially set}
Prints theorem name followed by theorem number inside the title.
\begin{dispExample}
\newtcbtheorem[use counter from=mytheo]{sometheorem}{Theorem}%
  {colback=white,colframe=red!50!black,fonttitle=\bfseries,
   theorem name and number}{theo}
\begin{sometheorem}{My example}{}
My theorem text.
\end{sometheorem}
\end{dispExample}
\end{docTcbKey}


\begin{docTcbKey}{theorem number and name}{}{style, no value}
Prints theorem number followed by theorem name inside the title.
\begin{dispExample}
\newtcbtheorem[use counter from=mytheo]{sometheorem}{Theorem}%
  {colback=white,colframe=red!50!black,fonttitle=\bfseries,
   theorem number and name}{theo}
\begin{sometheorem}{My example}{}
My theorem text.
\end{sometheorem}
\end{dispExample}
\end{docTcbKey}

\begin{docTcbKey}{theorem name}{}{style, no value}
Prints theorem name without number inside the title.
\begin{dispExample}
\newtcbtheorem[use counter from=mytheo]{sometheorem}{Theorem}%
  {colback=white,colframe=red!50!black,fonttitle=\bfseries,
   theorem name,enhanced,watermark text={\thetcbcounter}}{theo}
\begin{sometheorem}{My example}{}
My theorem text.
\end{sometheorem}
\end{dispExample}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{theorem}{=\marg{display name}\marg{counter}\marg{title}\marg{marker}}{no default}
  This key is internally used by \refCom{tcbmaketheorem}, but can be used
  directly in a |tcolorbox| for a more flexible approach.
  The \meta{display name} is used together with the increased \meta{counter} value
  and the \meta{title} for the title line of the box. Additionally, a
  |\label| with the given \meta{marker} is created.
\begin{dispExample}
% \newcounter{texercise}%  preamble
\begin{tcolorbox}[colback=green!10,colframe=green!50!black,arc=4mm,
                  theorem={Test}{texercise}{Direct usage}{myMarker}]
Here, we see the test \ref{myMarker}.
\end{tcolorbox}
\end{dispExample}
For a common appearance inside the document, the key |theorem| should not be
used directly as in the example above, but as part of a new environment
created by hand or using \refCom{tcbmaketheorem} or using its successor
\refCom{newtcbtheorem}.
\end{docTcbKey}


\begin{docTcbKey}{highlight math}{}{style, no value}
  Predefined style which is used for \refCom{tcbhighmath}.
  It can be changed comfortable with \refKey{/tcb/highlight math style}.
\end{docTcbKey}


\begin{docTcbKey}{highlight math style}{=\meta{style definition}}{style, no default}
  Changes the definition for \refKey{/tcb/highlight math} to the given
  \meta{style definition}. See \refCom{tcbhighmath} for another example.
\begin{dispExample}
% \tcbuselibrary{skins}
\tcbset{highlight math style={enhanced,%<-- needed for the 'remember' options
  colframe=red,colback=red!10!white,boxsep=0pt}}
\begin{align*}
\tcbhighmath[remember as=fx]{f(x)}
     &= \int\limits_{1}^{x} \frac{1}{t^2}~dt
      = \left[ -\frac{1}{t} \right]_{1}^{x}\\
     &= -\frac{1}{x} + \frac{1}{1}\\
     &=
\tcbhighmath[remember,overlay={%
    \draw[blue,very thick,->] (fx.south) to[bend right] ([yshift=2mm]frame.west);}]
  {1-\frac{1}{x}.}
\end{align*}
\end{dispExample}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{math upper}{}{style, no value}
  Sets the upper part to mathematical mode with font |\displaystyle|.
\end{docTcbKey}

\begin{docTcbKey}{math lower}{}{style, no value}
  Sets the lower part to mathematical mode with font |\displaystyle|.
\end{docTcbKey}

\begin{docTcbKey}{math}{}{style, no value}
  Sets the upper part \emph{and} lower part to mathematical mode with font |\displaystyle|.
\begin{dispExample}
\begin{tcolorbox}[math,colback=yellow!10!white,colframe=red!50!black]
  \sum\limits_{n=1}^{\infty} \frac{1}{n} = \infty.
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}


\begin{marker}
  The following styles are only tested to work with the original |amsmath| environments.
  If e.g. the |equation| environment is redefined as |gather|, then
  \refKey{/tcb/ams equation} should / could not be used. Obviously, you are encouraged
  to use \refKey{/tcb/ams gather} in this case.
\end{marker}

\begin{docTcbKey}[][doc updated=2014-10-30]{ams equation upper}{}{style, no value}
  Adds an |amsmath| |equation| environment to the start and end
  of the upper part.
\end{docTcbKey}

\begin{docTcbKey}[][doc updated=2014-10-30]{ams equation lower}{}{style, no value}
  Adds an |amsmath| |equation| environment to the start and end
  of the lower part.
\end{docTcbKey}

\begin{docTcbKey}[][doc updated=2014-10-30]{ams equation}{}{style, no value}
  Adds an |amsmath| |equation| environment to the start and end
  of the upper \emph{and} lower part.
\begin{dispExample}
\begin{tcolorbox}[ams equation,colback=yellow!10!white,colframe=red!50!black]
  \sum\limits_{n=1}^{\infty} \frac{1}{n} = \infty.
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}

\begin{docTcbKey}[][doc updated=2014-10-30]{ams equation* upper}{}{style, no value}
  Adds an |amsmath| |equation*| environment to the start and end
  of the upper part.
\end{docTcbKey}

\begin{docTcbKey}[][doc updated=2014-10-30]{ams equation* lower}{}{style, no value}
  Adds an |amsmath| |equation*| environment to the start and end
  of the lower part.
\end{docTcbKey}

\enlargethispage*{1cm}
\begin{docTcbKey}[][doc updated=2014-10-30]{ams equation*}{}{style, no value}
  Adds an |amsmath| |equation*| environment to the start and end
  of the upper \emph{and} lower part.
\begin{dispExample}
\begin{tcolorbox}[ams equation*,colback=yellow!10!white,colframe=red!50!black]
  \sum\limits_{n=1}^{\infty} \frac{1}{n} = \infty.
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{ams align upper}{}{style, no value}
  Adds an |amsmath| |align| environment to the start and end
  of the upper part.
\end{docTcbKey}

\begin{docTcbKey}{ams align lower}{}{style, no value}
  Adds an |amsmath| |align| environment to the start and end
  of the lower part.
\end{docTcbKey}

\begin{docTcbKey}{ams align}{}{style, no value}
  Adds an |amsmath| |align| environment to the start and end
  of the upper \emph{and} lower part.
\begin{dispExample}
\begin{tcolorbox}[ams align,colback=yellow!10!white,colframe=red!50!black]
  \sum\limits_{n=1}^{\infty} \frac{1}{n} &= \infty.\\
  \int x^2 ~\text{d}x                     &= \frac13 x^3 + c.
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}

\begin{docTcbKey}{ams align* upper}{}{style, no value}
  Adds an |amsmath| |align*| environment to the start and end
  of the upper part.
\end{docTcbKey}

\begin{docTcbKey}{ams align* lower}{}{style, no value}
  Adds an |amsmath| |align*| environment to the start and end
  of the lower part.
\end{docTcbKey}

\begin{docTcbKey}{ams align*}{}{style, no value}
  Adds an |amsmath| |align*| environment to the start and end
  of the upper \emph{and} lower part.
\begin{dispExample}
\begin{tcolorbox}[ams align*,colback=yellow!10!white,colframe=red!50!black]
  \sum\limits_{n=1}^{\infty} \frac{1}{n} &= \infty.\\
  \int x^2 ~\text{d}x                     &= \frac13 x^3 + c.
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{ams gather upper}{}{style, no value}
  Adds an |amsmath| |gather| environment to the start and end
  of the upper part.
\end{docTcbKey}

\begin{docTcbKey}{ams gather lower}{}{style, no value}
  Adds an |amsmath| |gather| environment to the start and end
  of the lower part.
\end{docTcbKey}

\begin{docTcbKey}{ams gather}{}{style, no value}
  Adds an |amsmath| |gather| environment to the start and end
  of the upper \emph{and} lower part.
\begin{dispExample}
\begin{tcolorbox}[ams gather,colback=yellow!10!white,colframe=red!50!black]
  \sum\limits_{n=1}^{\infty} \frac{1}{n} = \infty.\\
  \int x^2 ~\text{d}x = \frac13 x^3 + c.
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}

\begin{docTcbKey}{ams gather* upper}{}{style, no value}
  Adds an |amsmath| |gather*| environment to the start and end
  of the upper part.
\end{docTcbKey}

\begin{docTcbKey}{ams gather* lower}{}{style, no value}
  Adds an |amsmath| |gather*| environment to the start and end
  of the lower part.
\end{docTcbKey}

\begin{docTcbKey}{ams gather*}{}{style, no value}
  Adds an |amsmath| |gather*| environment to the start and end
  of the upper \emph{and} lower part.
\begin{dispExample}
\begin{tcolorbox}[ams gather*,colback=yellow!10!white,colframe=red!50!black]
  \sum\limits_{n=1}^{\infty} \frac{1}{n} = \infty.\\
  \int x^2 ~\text{d}x = \frac13 x^3 + c.
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}


\clearpage
\begin{docTcbKey}{ams nodisplayskip upper}{}{style, no value}
  Neutralizes the |\abovedisplayskip| of a following |align| or |gather|
  environment for the upper part. Note that the text content has to
  start with such a formula.
\end{docTcbKey}


\begin{docTcbKey}{ams nodisplayskip lower}{}{style, no value}
  Neutralizes the |\abovedisplayskip| of a following |align| or |gather|
  environment for the lower part. Note that the text content has to
  start with such a formula.
\end{docTcbKey}


\begin{docTcbKey}{ams nodisplayskip}{}{style, no value}
  Neutralizes the |\abovedisplayskip| of a following |align| or |gather|
  environment for the upper part \emph{and} lower part.
  Note that the text content has to start with such a formula.
\begin{dispExample}
\begin{tcolorbox}[ams nodisplayskip,colback=yellow!10!white,colframe=red!50!black]
  \begin{gather}
  \sum\limits_{n=1}^{\infty} \frac{1}{n} = \infty.\\
  \int x^2 ~\text{d}x = \frac13 x^3 + c.
  \end{gather}
  And now for something completely different.
\end{tcolorbox}
\end{dispExample}
\end{docTcbKey}

\bigskip
New colored mathematical environments are easily created using
\refCom{newtcolorbox}:

\begin{dispExample}
\newtcolorbox{mymath}{ams gather*,colback=yellow!10!white,colframe=red!50!black}

\begin{mymath}
  \sum\limits_{n=1}^{\infty} \frac{1}{n} = \infty.\\
  \int x^2 ~\text{d}x = \frac13 x^3 + c.
\end{mymath}
\end{dispExample}

\bigskip
\begin{marker}
  All described options like \refKey{/tcb/ams gather upper}, \refKey{/tcb/ams gather lower},
  \refKey{/tcb/ams gather} are (partially) setting (overwritting) the
  keys \refKey{/tcb/before upper}, \refKey{/tcb/after upper},
  \refKey{/tcb/before lower}, \refKey{/tcb/after lower}.\par
  Therefore, e.\,g.\ |\tcbset{ams gather,before upper={\text{Pythagoras:}}}|
  produces an invalid result. For this case, you are invited to use\\
  |\tcbset{ams gather,before upper app={\text{Pythagoras:}}}|,\\
  see \refKey{/tcb/before upper app}.
\end{marker}


\clearpage
\begin{docTcbKey}{theorem style}{=\meta{name}}{no default, initially |standard|}
Applies a predefined style \meta{name} to the theorem environment. Some of
the feasible \meta{name} values resemble style names from the packages |theorem|
and |ntheorem| to give convenient access to known patterns.
\begin{marker}
The styles alter \refKey{/tcb/separator sign}, \refKey{/tcb/description delimiters},
\refKey{/tcb/terminator sign}, and more. Therefore, one should apply such
keys \emph{after} a theorem style.
\end{marker}

For the following examples, we use:
\inputpreamblelisting{J}

The predefined styles are:
\begin{itemize}
%
\item\docValue{standard}: This is the initial value.
\begin{dispExample}
\begin{theorem}[theorem style=standard]{standard}{}
This is my theorem. \begin{equation*} a^2 + b^2 = c^2. \end{equation*}
\end{theorem}
\end{dispExample}
%
\item\docValue{change standard}
\begin{dispExample}
\begin{theorem}[theorem style=change standard]{change standard}{}
This is my theorem. \begin{equation*} a^2 + b^2 = c^2. \end{equation*}
\end{theorem}
\end{dispExample}
%
\item\docValue{plain}
\begin{dispExample}
\begin{theorem}[theorem style=plain]{plain}{}
This is my theorem. \begin{equation*} a^2 + b^2 = c^2. \end{equation*}
\end{theorem}
\end{dispExample}
%
\clearpage
\item\docValue{break}
\begin{dispExample}
\begin{theorem}[theorem style=break]{break}{}
This is my theorem. \begin{equation*} a^2 + b^2 = c^2. \end{equation*}
\end{theorem}
\end{dispExample}
%
\item\docValue{plain apart}
\begin{dispExample}
\begin{theorem}[theorem style=plain apart]{plain apart}{}
This is my theorem. \begin{equation*} a^2 + b^2 = c^2. \end{equation*}
\end{theorem}
\end{dispExample}
%
\item\docValue{change}
\begin{dispExample}
\begin{theorem}[theorem style=change]{change}{}
This is my theorem. \begin{equation*} a^2 + b^2 = c^2. \end{equation*}
\end{theorem}
\end{dispExample}
%
\item\docValue{change break}
\begin{dispExample}
\begin{theorem}[theorem style=change break]{change break}{}
This is my theorem. \begin{equation*} a^2 + b^2 = c^2. \end{equation*}
\end{theorem}
\end{dispExample}
%
\item\docValue{change apart}
\begin{dispExample}
\begin{theorem}[theorem style=change apart]{change apart}{}
This is my theorem. \begin{equation*} a^2 + b^2 = c^2. \end{equation*}
\end{theorem}
\end{dispExample}
%
\clearpage
\item\docValue{margin}
\begin{dispExample}
\begin{theorem}[theorem style=margin,left=10mm]{margin}{}
This is my theorem. \begin{equation*} a^2 + b^2 = c^2. \end{equation*}
\end{theorem}
\begin{theorem}[theorem style=margin,left=10mm,oversize]{margin}{}
This is my theorem. \begin{equation*} a^2 + b^2 = c^2. \end{equation*}
\end{theorem}
\end{dispExample}
%
\item\docValue{margin break}
\begin{dispExample}
\begin{theorem}[theorem style=margin break,left=10mm]{margin break}{}
This is my theorem. \begin{equation*} a^2 + b^2 = c^2. \end{equation*}
\end{theorem}
\begin{theorem}[theorem style=margin break,left=10mm,oversize]{margin break}{}
This is my theorem. \begin{equation*} a^2 + b^2 = c^2. \end{equation*}
\end{theorem}
\end{dispExample}
%
\item\docValue{margin apart}
\begin{dispExample}
\begin{theorem}[theorem style=margin apart,left=10mm]{margin apart}{}
This is my theorem. \begin{equation*} a^2 + b^2 = c^2. \end{equation*}
\end{theorem}
\begin{theorem}[theorem style=margin apart,left=10mm,oversize]{margin apart}{}
This is my theorem. \begin{equation*} a^2 + b^2 = c^2. \end{equation*}
\end{theorem}
\end{dispExample}
%
\end{itemize}
\end{docTcbKey}


%
\clearpage
\subsection{Examples for Definitions and Theorems}
In the following, the application of \refCom{tcbmaketheorem}
to highlight mathematical definitions, theorems, or the like is demonstrated.

At first, additional |tcb| keys are created for the appearance of
the colored boxes. It is assumed that theorems and corollaries should be
identically colored.
All following environments are numbered with a common counter, but this
can be changed easily. Here, the counter output is supplemented by
the subsection number.
Further, the |cleveref| package \cite{cubitt:2018a} is used for clever
references.

\inputpreamblelisting{G}

By \refCom{newtcbtheorem}, commonly numbered theorem environments are
created now. |defstyle| and |theostyle| are used for the appearance.

Now, everything is prepared for the following examples.

\begin{dispExample}
The following theorem is numbered as \Cref{theo:diffbarstetig} and
referenced with the marker \texttt{theo:diffbarstetig}.\bigskip

\begin{Theorem}{Differenzierbarkeit bedingt Stetigkeit, wobei diese Benennung
  zu Testzwecken ungew\"{o}hnlich lang ist}{diffbarstetig}%
  Eine Funktion $f:I\to\mathbb{R}$ ist in $x_0\in I$ stetig, wenn $f$ in
  $x_0$ differenzierbar ist.
\end{Theorem}
\end{dispExample}


\begin{dispExample}
The following definition is numbered as \Cref{def:diffbarkeit} and
referenced with the marker \texttt{def:diffbarkeit}.\bigskip

\begin{Definition}{Differenzierbarkeit}{diffbarkeit}
  Eine Funktion $f:~I\to\mathbb{R}$ auf einem Intervall $I$ hei\ss{}t in
  $x_0\in I$ differenzierbar oder linear approximierbar,
  wenn der Grenzwert
  \begin{equation*}
  \lim\limits_{x\to x_0}\frac{f(x)-f(x_0)}{x-x_0}=
  \lim\limits_{h\to 0}\frac{f(x_0+h)-f(x_0)}{h}
  \end{equation*}
  existiert. Bei Existenz hei\ss{}t dieser Grenzwert Ableitung
  oder Differentialquotient von $f$ in $x_0$ und man
  schreibt f\"{u}r ihn
  \begin{equation*}
  f'(x_0)\quad\text{oder}\quad\frac{df}{dx}(x_0).
  \end{equation*}
\end{Definition}
\end{dispExample}


\begin{dispExample}
The following corollary is numbered as \Cref{cor:nullstellen} and
referenced with the marker \texttt{cor:nullstellen}.\bigskip

\begin{Corollary}{Nullstellenexistenz}{nullstellen}
  Ist $f:[a,b]\to\mathbb{R}$ stetig und haben $f(a)$ und $f(b)$ entgegengesetzte
  Vorzeichen, also $f(a)f(b)<0$, so besitzt $f$ eine Nullstelle $x_0\in]a,b[$,
  also $f(x_0)=0$.
\end{Corollary}
\end{dispExample}


\begin{dispExample}
\begin{Theorem}[boxrule=2mm,toptitle=-1.5mm,bottomtitle=-1.5mm]{%
    Hinreichende Bedingung f\"{u}r Wendepunkte}{wendehinreichend}%
  $f$ sei eine auf einem Intervall $]a,b[$ dreimal stetig differenzierbare Funktion.
  Ist $f''(x_0)=0$ in $x_0\in]a,b[$ und $f'''(x_0)\ne 0$, so ist
  $(x_0,f(x_0))$ ein Wendepunkt von $f$.
\end{Theorem}
\end{dispExample}

\begin{dispExample}
% \usepackage{varioref}
% \usepackage{cleveref}
% \tcbuselibrary{skins}
\newtcbtheorem[use counter from=Definition]{YetAnotherTheorem}{Theorem}%
  {theorem style=plain apart,label type=theorem,enhanced,frame hidden,
  boxrule=2mm,titlerule=0mm,toptitle=1mm,bottomtitle=1mm,
  fonttitle=\bfseries\large,fontupper=\normalsize,
  coltitle=green!35!black,colbacktitle=green!15!white,
  colback=green!50!yellow!15!white,borderline={1pt}{0pt}{green!25!blue},
  }{theo}

\begin{YetAnotherTheorem}{Mittelwertsatz f\"{u}r $n$ Variable}{meanvaluetheorem}%
  Es sei $n\in\mathbb{N}$, $D\subseteq\mathbb{R}^n$ eine offene Menge und
  $f\in C^{1}(D,\mathbb{R})$. Dann gibt es auf jeder Strecke
  $[x_0,x]\subset D$ einen Punkt $\xi\in[x_0,x]$, so dass gilt
  \begin{equation*}
  f(x)-f(x_0) = \operatorname{grad} f(\xi)^{\top}(x-x_0)
  \end{equation*}
\end{YetAnotherTheorem}

\medskip
Here, |cleveref| support is used to reference \Cref{theo:meanvaluetheorem}
on \Cpageref{theo:meanvaluetheorem}. This \namecref{theo:meanvaluetheorem}
can also be referenced by |\Vref| resulting in \Vref{theo:meanvaluetheorem}.
\end{dispExample}

\begin{marker}
Note that \refKey{/tcb/label type} was used in the example above to feed
|cleveref| \cite{cubitt:2018a} with the needed name information.
\end{marker}

\clearpage

\begin{dispExample}
Here, using |\Vref| resulting in \Vref{theo:meanvaluetheorem} is more interesting\ldots
\end{dispExample}


\begin{dispExample}
% \tcbuselibrary{skins}
\newtcbtheorem[use counter from=Definition]{YetAnotherTheorem}{Theorem}%
  {theorem style=change apart,enhanced,arc=0mm,outer arc=0mm,
  boxrule=0mm,toprule=1mm,bottomrule=1mm,left=1mm,right=1mm,
  titlerule=0mm,toptitle=0mm,bottomtitle=1mm,top=0mm,
  colframe=red!50!black,colback=red!5!white,coltitle=red!50!black,
  title style={top color=yellow!50!white,bottom color=red!5!white,
    middle color=yellow!50!white},
  fonttitle=\bfseries\sffamily\normalsize,fontupper=\normalsize\itshape,
  }{theo}

\begin{YetAnotherTheorem}{Mittelwertsatz f\"{u}r $n$ Variable}{mittelwertsatz_n2}%
  Es sei $n\in\mathbb{N}$, $D\subseteq\mathbb{R}^n$ eine offene Menge und
  $f\in C^{1}(D,\mathbb{R})$. Dann gibt es auf jeder Strecke
  $[x_0,x]\subset D$ einen Punkt $\xi\in[x_0,x]$, so dass gilt
  \begin{equation*}
  f(x)-f(x_0) = \operatorname{grad} f(\xi)^{\top}(x-x_0)
  \end{equation*}
\end{YetAnotherTheorem}
\end{dispExample}


\begin{dispExample}
% \usepackage{varwidth}   \tcbuselibrary{skins}
\newtcbtheorem[use counter from=Definition]{YetAnotherTheorem}{Theorem}%
{enhanced,frame empty,interior empty,colframe=ForestGreen!50!white,
  coltitle=ForestGreen!50!black,fonttitle=\bfseries,colbacktitle=ForestGreen!15!white,
  borderline={0.5mm}{0mm}{ForestGreen!15!white},
  borderline={0.5mm}{0mm}{ForestGreen!50!white,dashed},
  attach boxed title to top center={yshift=-2mm},
  boxed title style={boxrule=0.4pt},varwidth boxed title}{theo}

\begin{YetAnotherTheorem}{Mittelwertsatz f\"{u}r $n$ Variable}{mittelwertsatz_n3}%
  Es sei $n\in\mathbb{N}$, $D\subseteq\mathbb{R}^n$ eine offene Menge und
  $f\in C^{1}(D,\mathbb{R})$. Dann gibt es auf jeder Strecke
  $[x_0,x]\subset D$ einen Punkt $\xi\in[x_0,x]$, so dass gilt
  \begin{equation*}
  f(x)-f(x_0) = \operatorname{grad} f(\xi)^{\top}(x-x_0)
  \end{equation*}
\end{YetAnotherTheorem}
\end{dispExample}


\clearpage
You need more attention for your theorems? Here, you are \ldots

\begin{dispExample}
% tcbuselibrary{skins}  % preamble
\begin{Theorem}[enhanced,
    fuzzy halo=3mm with yellow,
    fuzzy halo=2mm with red,
    fuzzy halo=1mm with yellow,
    watermark color=red!35!white,
    watermark text={Overacting\\Fundamental Theorem}]%
  {Fundamental Theorem of Theorems}{fundamental}%
  \lipsum[1-2]
\end{Theorem}
\end{dispExample}

Let's try a more conservative approach:

\begin{dispExample}
% \tcbuselibrary{skins}
\newtcbtheorem[use counter from=Definition]{YetAnotherTheorem}{Theorem}%
  {theorem style=plain,enhanced,colframe=blue!50!black,colback=yellow!20!white,
   coltitle=red!50!black,fonttitle=\upshape\bfseries,fontupper=\itshape,
   drop fuzzy shadow=blue!50!black!50!white,boxrule=0.4pt}{theo}

\begin{YetAnotherTheorem}{Mittelwertsatz f\"{u}r $n$ Variable}{mittelwertsatz_n4}%
  Es sei $n\in\mathbb{N}$, $D\subseteq\mathbb{R}^n$ eine offene Menge und
  $f\in C^{1}(D,\mathbb{R})$. Dann gibt es auf jeder Strecke
  $[x_0,x]\subset D$ einen Punkt $\xi\in[x_0,x]$, so dass gilt
  \begin{equation*}
  f(x)-f(x_0) = \operatorname{grad} f(\xi)^{\top}(x-x_0)
  \end{equation*}
\end{YetAnotherTheorem}
\end{dispExample}


\clearpage
\subsection{Using other theorem environments with \texttt{tcolorbox}}\label{subsec:theorems_other}

Instead of creating theorem environments with the methods described before,
environments from other packages can be boxed with a |tcolorbox|.

Environments may be created e.g. by methods from the |theorem| package or
the |amsthm| package. \refCom{tcolorboxenvironment} can be used to put a box
around these environments.

\inputpreamblelisting{K}

\begin{dispExample}
\begin{lem}
  \lipsum[2]
\end{lem}

\lipsum[3]

\begin{proof}
  \lipsum*[4]
\end{proof}
\end{dispExample}


==> tcolorbox.doc.verbatim.tex <==
% !TeX root = tcolorbox.tex
% include file of tcolorbox.tex (manual of the LaTeX package tcolorbox)
\clearpage
\section{Saving and Loading of Verbatim Texts}%
\tcbset{external/prefix=external/verbatim_}%
The following macros are slightly modified versions of the original macros
from the known packages |moreverb| and |verbatim|.
They are used implicitly inside of a |tcolorbox| environment,
but they can be used outside also.
\enlargethispage*{1.5cm}

\begin{docEnvironment}{tcbverbatimwrite}{\marg{file name}}
  Saves the \meta{environment content} to a file named by \meta{file name}.
  \TeX\ macros inside the environment are not expanded.
\begin{dispExample}
\begin{tcbverbatimwrite}{\jobname_verbexp.tex}
  This text is saved \textit{as is}.
\end{tcbverbatimwrite}

Now, we are using the file:\par
\input{\jobname_verbexp.tex}
\end{dispExample}

This environment may be used inside an own environment. Note, that inside
the environment definition |\tcbverbatimwrite| has to be used instead of
|\begin{tcbverbatimwrite}| and |\endtcbverbatimwrite| instead of |\end{tcbverbatimwrite}|.
\begin{dispExample}
\newenvironment{myverbatim}{%
  \begingroup\tcbverbatimwrite{\jobname_myverb.tex}}%
  {\endtcbverbatimwrite\endgroup}

\begin{myverbatim}
  This is the text which is saved by my own environment.
\end{myverbatim}

Now, we are using the file:\par
\input{\jobname_myverb.tex}
\end{dispExample}
\end{docEnvironment}

\begin{docEnvironment}{tcbwritetemp}{}
  Has the same function as \refEnv{tcbverbatimwrite}, but uses the key value
  of |tempfile| for the file name.
\begin{dispExample}
\begin{tcbwritetemp}
  This text is saved \textit{as is}.
\end{tcbwritetemp}

Now, we are using the file:\par
\tcbusetemp
\end{dispExample}
\end{docEnvironment}


\begin{docCommand}{tcbusetemp}{}
  Loads the current temporary file which was saved by \refEnv{tcbwritetemp}.
\end{docCommand}

\clearpage

\begin{docTcbKey}[][doc new=2017-07-05]{verbatim ignore percent}{\colOpt{=true\textbar false}}{default |true|, initially |false|}
  If this option is set to be |true|, the percent sign \% is silently
  ignored for \refEnv{tcbverbatimwrite} and all macros and environments
  which are built using \refEnv{tcbverbatimwrite}, e.g.\ 
  \refEnv{tcbwritetemp}, \refEnv{tcblisting}, or \refEnv{dispExample}.\par
  This option may be useful for creating some special effects, but mainly
  it is intended to be applied for documentation with DocStrip.
  The creation of this option was motivated by Yudai Nakata.
  Note that this option is not getting reset by \refKey{/tcb/reset}.
\begin{dispExample*}{sidebyside}
Normal usage:
\begin{tcbwritetemp}
%\begin{center}\bfseries
This is my text.
%\end{center}
\end{tcbwritetemp}

\tcbusetemp

\tcbset{verbatim ignore percent}
\bigskip Option applied:
\begin{tcbwritetemp}
%\begin{center}\bfseries
This is my text.
%\end{center}
\end{tcbwritetemp}

\tcbusetemp
\end{dispExample*}

\begin{marker}
Note that \emph{every} percent sign is removed, also escaped ones.
\end{marker}

\begin{dispExample*}{sidebyside}
% \tcbuselibrary{listings}
\def\percent{\%}

\begin{tcblisting}{title=Normal}
%\begin{center}\bfseries
This is my 5\percent\ text
and this is my 10\% text.
%\end{center}
\end{tcblisting}

\begin{tcblisting}{
  title=Option applied,
  verbatim ignore percent}
%\begin{center}\bfseries
This is my 5\percent\ text
and this is my 10\% text.
%\end{center}
\end{tcblisting}
\end{dispExample*}

\end{docTcbKey}



==> tcolorbox.doc.vignette.tex <==
% !TeX root = tcolorbox.tex
% include file of tcolorbox.tex (manual of the LaTeX package tcolorbox)
\clearpage
\section{Library \mylib{vignette}}\label{sec:vignette}%
\tcbset{external/prefix=external/vignette_}%
The library is loaded by a package option or inside the preamble by:
\begin{dispListing}
\tcbuselibrary{vignette}
\end{dispListing}
This also loads the \mylib{skins} library, see \Fullref{sec:skins},
and the |fadings| library of |tikz| \cite{tantau:tikz_and_pgf}.


\subsection{Vignette Drawing}\label{subsec:vignettedrawing}

\begin{docCommand}[doc new=2016-04-22]{tcbvignette}{\marg{options}}
  In this context, a \emph{vignette} is a four part rectangular frame.
  It is constructed as several \tikzname\ paths and, therefore, can only be
  used inside a |tikzpicture| environment or inside \refEnv{tcolorbox} options.

  The \meta{options} control position, size and style settings of the vignette.
  Theses options have the common key path |/tcb/vig/| and are described in
  the following.

  The next examples show direct \refCom{tcbvignette} usage without
  a \refEnv{tcolorbox}.

\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \tcbvignette{}
\end{tikzpicture}
\end{dispExample*}

\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \node[draw,fill=blue!15!white] (A) {Test};
  \tcbvignette{outside node=A,raised color=blue}
\end{tikzpicture}
\end{dispExample*}

\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \node[draw,fill=blue!15!white] (A) {Another Test};
  \tcbvignette{size=3mm,outside node=A,
    north style=red,east style=yellow,
    south style=blue,west style=green}
\end{tikzpicture}
\end{dispExample*}

\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \node[inner sep=3mm,fill=red!75] (A) {Test};
  \tcbvignette{over node=A,fade in}
\end{tikzpicture}
\end{dispExample*}

\refCom{tcbvignette} can be used directly inside appropriate options keys
for \refEnv{tcolorbox}. Note that options like \refKey{/tcb/underlay} need
\refKey{/tcb/enhanced} or similar settings.

\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tcolorbox}[enhanced,size=small,sharp corners,
  colback=green!10,colframe=green!50!black,
  boxrule=1mm,titlerule=0mm,
  title=My title,center title,fonttitle=\bfseries,
  underlay={\tcbvignette{size=1mm,inside node=frame,
      raised color=green!50!black}}]
    This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}

Mostly, convenient short cuts like \refKey{/tcb/underlay vignette} can
be used to add a \emph{vignette} to a \refEnv{tcolorbox}. Here, \refCom{tcbvignette}
is used internally.

\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tcolorbox}[enhanced,size=small,sharp corners,
  colback=green!10,colframe=green!50!black,
  boxrule=1mm,titlerule=0mm,
  title=My title,center title,fonttitle=\bfseries,
  underlay vignette]
    This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}

\end{docCommand}



\subsection{Generic Geometry Settings}\label{subsec:vignettegeometry}


\begin{vigTcbKey}[][doc new=2016-04-22]{xmin}{=\meta{length}}{no default, initially |0pt|}
  Sets the lower horizontal limit of a \refCom{tcbvignette}.
\end{vigTcbKey}

\begin{vigTcbKey}[][doc new=2016-04-22]{xmax}{=\meta{length}}{no default, initially |1cm|}
  Sets the upper horizontal limit of a \refCom{tcbvignette}.
\end{vigTcbKey}

\begin{vigTcbKey}[][doc new=2016-04-22]{ymin}{=\meta{length}}{no default, initially |0pt|}
  Sets the lower vertical limit of a \refCom{tcbvignette}.
\end{vigTcbKey}

\begin{vigTcbKey}[][doc new=2016-04-22]{ymax}{=\meta{length}}{no default, initially |1cm|}
  Sets the upper vertical limit of a \refCom{tcbvignette}.
\end{vigTcbKey}


\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \fill [black!20] (0,0) rectangle (3,2);
  \path [pattern=checkerboard,pattern color=black!30]
    (0,0) rectangle (3,2);
  \tcbvignette{xmin=1cm,xmax=2.5cm,ymin=0.5cm,ymax=1.75cm}
\end{tikzpicture}
\end{dispExample*}


\begin{vigTcbKey}[][doc new=2016-04-22]{lower left corner}{=\meta{coordinates}}{style, initially |0,0|}
  Sets the lower left corner of a \refCom{tcbvignette}.
  This style sets \refKey{/tcb/vig/xmin} and \refKey{/tcb/vig/ymin}.
\end{vigTcbKey}

\begin{vigTcbKey}[][doc new=2016-04-22]{upper right corner}{=\meta{coordinates}}{style, initially |1,1|}
  Sets the upper right corner of a \refCom{tcbvignette}.
  This style sets \refKey{/tcb/vig/xmax} and \refKey{/tcb/vig/ymax}.
\end{vigTcbKey}


\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \fill [black!20] (0,0) rectangle (3,2);
  \path [pattern=checkerboard,pattern color=black!30]
    (0,0) rectangle (3,2);
  \tcbvignette{lower left corner={1,0.5},
               upper right corner={2.5,1.75}}
\end{tikzpicture}
\end{dispExample*}

\enlargethispage*{1cm}

\begin{vigTcbKey}[][doc new=2016-04-22]{inside node}{=\meta{name}}{style, initally unset}
  Places the \refCom{tcbvignette} inside the node with the given \meta{name}.
  The outer limits of the \emph{vignette} are adapted to the node geometry.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \node[minimum width=2cm,minimum height=1cm] (A) {Node A};
  \tcbvignette{inside node=A}
  \draw[very thick] (A.south west) rectangle (A.north east);
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}

\clearpage

\begin{vigTcbKey}[][doc new=2016-04-22]{outside node}{=\meta{name}}{style, initally unset}
  Places the \refCom{tcbvignette} outside the node with the given \meta{name}.
  The inner limits of the \emph{vignette} are adapted to the node geometry.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \node[minimum width=2cm,minimum height=1cm] (A) {Node A};
  \tcbvignette{outside node=A}
  \draw[very thick] (A.south west) rectangle (A.north east);
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}


\begin{vigTcbKey}[][doc new=2016-04-22]{over node}{=\meta{name}}{style, initally unset}
  Places the \refCom{tcbvignette} over the node with the given \meta{name}.
  The outer limits of the \emph{vignette} are adapted to the node geometry, but
  are shifted to the outside by \refKey{/tcb/vig/over node offset}.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \node[minimum width=2cm,minimum height=1cm] (A) {Node A};
  \tcbvignette{over node offset=1mm,over node=A}
  \draw[very thick] (A.south west) rectangle (A.north east);
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}

\begin{vigTcbKey}[][doc new=2016-04-22]{over node offset}{=\meta{length}}{no default, initially |0.1mm|}
  Determines the shift value for \refKey{/tcb/vig/over node}.
  Note that \refKey{/tcb/vig/over node offset} has to be set \emph{before}
  \refKey{/tcb/vig/over node} is used.
\end{vigTcbKey}


\begin{vigTcbKey}[][doc new=2016-04-22]{north size}{=\meta{length}}{no default, initially |2mm|}
  Sets the thickness of the north \emph{vignette} part.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \tcbvignette{north size=4mm}
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}

\begin{vigTcbKey}[][doc new=2016-04-22]{south size}{=\meta{length}}{no default, initially |2mm|}
  Sets the thickness of the south \emph{vignette} part.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \tcbvignette{south size=4mm}
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}

\begin{vigTcbKey}[][doc new=2016-04-22]{east size}{=\meta{length}}{no default, initially |2mm|}
  Sets the thickness of the east \emph{vignette} part.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \tcbvignette{east size=4mm}
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}

\begin{vigTcbKey}[][doc new=2016-04-22]{west size}{=\meta{length}}{no default, initially |2mm|}
  Sets the thickness of the west \emph{vignette} part.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \tcbvignette{west size=4mm}
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}

\clearpage

\begin{vigTcbKey}[][doc new=2016-04-22]{vertical size}{=\meta{length}}{style, initially |2mm|}
  Sets \refKey{/tcb/vig/north size} and \refKey{/tcb/vig/south size},
  to the given \meta{length}.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \tcbvignette{vertical size=4mm}
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}

\begin{vigTcbKey}[][doc new=2016-04-22]{horizontal size}{=\meta{length}}{style, initially |2mm|}
  Sets \refKey{/tcb/vig/east size} and \refKey{/tcb/vig/west size},
  to the given \meta{length}.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \tcbvignette{horizontal size=4mm}
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}


\begin{vigTcbKey}[][doc new=2016-04-22]{size}{=\meta{length}}{style, initially |2mm|}
  Sets \refKey{/tcb/vig/north size}, \refKey{/tcb/vig/south size},
  \refKey{/tcb/vig/east size}, and \refKey{/tcb/vig/west size} to the given \meta{length}.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \tcbvignette{size=4mm}
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}


\begin{marker}
\refKey{/tcb/vig/north size}, \refKey{/tcb/vig/south size}, etc. have to
be set \emph{before} \refKey{/tcb/vig/outside node} is used.
\end{marker}



\subsection{Generic Color and Style Settings}\label{subsec:vignettestyle}

\begin{vigTcbKey}[][doc new=2016-04-22]{north style}{=\marg{style}}{no default, initially |red!50!white|}
  Sets \tikzname\ \meta{style} options for the north \emph{vignette} part.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \tcbvignette{north style=blue}
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}

\begin{vigTcbKey}[][doc new=2016-04-22]{south style}{=\marg{style}}{no default, initially |red!50!black|}
  Sets \tikzname\ \meta{style} options for the south \emph{vignette} part.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \tcbvignette{south style={draw=blue,fill=yellow}}
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}


\begin{vigTcbKey}[][doc new=2016-04-22]{east style}{=\marg{style}}{no default, initially |red!75!black|}
  Sets \tikzname\ \meta{style} options for the east \emph{vignette} part.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \tcbvignette{east style={left color=yellow!75!black,
    right color=blue!75!black}}
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}

\clearpage

\begin{vigTcbKey}[][doc new=2016-04-22]{west style}{=\marg{style}}{no default, initially |red!75!white|}
  Sets \tikzname\ \meta{style} options for the west \emph{vignette} part.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \tcbvignette{west style={preaction={fill=black!20},
    pattern=checkerboard,
    pattern color=black!30}}
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}


\begin{vigTcbKey}[][doc new=2016-05-24]{scope}{=\marg{style}}{no default, initially empty}
  The four \emph{vignette} parts are drawn inside a \tikzname\ |scope|
  environment which takes the given \meta{style} as option.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \tcbvignette{scope={transparency group,opacity=0.25}}
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}



\begin{vigTcbKey}[][doc new=2016-04-22]{raised color}{=\meta{color}}{no default}
  Creates a raised frame impression by setting the four style options
  \refKey{/tcb/vig/north style},
  \refKey{/tcb/vig/south style},
  \refKey{/tcb/vig/east style}, and
  \refKey{/tcb/vig/west style}
  to darkened and lightened variations of the given \meta{color}.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \tcbvignette{raised color=blue}
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}


\begin{vigTcbKey}[][doc new=2016-04-22]{lowered color}{=\meta{color}}{no default}
  Creates a lowered frame impression by setting the four style options
  \refKey{/tcb/vig/north style},
  \refKey{/tcb/vig/south style},
  \refKey{/tcb/vig/east style}, and
  \refKey{/tcb/vig/west style}
  to darkened and lightened variations of the given \meta{color}.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \tcbvignette{lowered color=green!75!black}
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}


\begin{vigTcbKey}[][doc new=2016-04-22]{color from}{=\meta{inner} |to| \meta{outer}}{no default}
  Sets the four style options
  \refKey{/tcb/vig/north style},
  \refKey{/tcb/vig/south style},
  \refKey{/tcb/vig/east style}, and
  \refKey{/tcb/vig/west style}
  such that the color shades from the
  \meta{inner} color to the \meta{outer} color.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \tcbvignette{color from=red to blue!50}
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}



\begin{vigTcbKey}[][doc new=2016-04-22]{base color}{=\meta{color}}{no default}
  Sets the base color for \refKey{/tcb/vig/raised color},
  \refKey{/tcb/vig/lowered color}, \refKey{/tcb/finish fading vignette}.
  Typically, this value has not to be set directly.
\end{vigTcbKey}


\clearpage
\begin{vigTcbKey}[][doc new=2016-04-22]{draw method}{=\docValue{direct}\textbar\docValue{clipped}}{no default, initially |direct|}
  Especially, if shadings or fadings are used, the drawn \emph{vignette}
  graphs are displayed sometimes not as perfect as expected. Glitches and
  imperfections are very dependent on the previewer software.
  The \refKey{/tcb/vig/draw method} intends to give a choice of alternative
  drawing methods.
  \begin{itemize}
  \item\docValue{direct}: The \emph{vignette} parts are drawn/filled
    by using a single \tikzname\ graph. This is the preferred (and default)
    method for solid color graphs.
  \item\docValue{clipped}: The \emph{vignette} parts are drawn somewhat
    oversized and are clipped to the intended region.
    In combination with shadings and fadings this seems to give a
    better/different optical result (depends on the previewer).
  \end{itemize}
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \tcbvignette{color from=red to yellow}
\end{tikzpicture}
\end{dispExample*}
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \tcbvignette{color from=red to yellow,draw method=clipped}
\end{tikzpicture}
\end{dispExample*}

\begin{marker}
This option is a stopgap and may be changed or preferably removed in
future.
\end{marker}
\end{vigTcbKey}



\subsection{Generic Fading Settings}\label{subsec:vignettefading}

The |fadings| library of |tikz| \cite{tantau:tikz_and_pgf} is loaded
automatically by the \mylib{vignette} library.
Amongst others, the fadings
\docFading{west},
\docFading{east},
\docFading{north}, and
\docFading{south} are defined inside the |fadings| library.

The \mylib{vignette} library adds some more fadings called
\docFading{semi west},
\docFading{semi east},
\docFading{semi north}, and
\docFading{semi south}.
These fadings are much \emph{weaker} than the normal fadings.

\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \fill [black!20] (0,0) rectangle (1,1);
  \path [pattern=checkerboard,pattern color=black!30]
    (0,0) rectangle (1,1);
  \fill [path fading=semi west,blue] (0,0) rectangle (1,1);
\end{tikzpicture}
\end{dispExample*}



\begin{tcboxedraster}{base example,title=Comparison of the Fadings}
  \def\doShadingExample#1{%
    \begin{tcolorbox}[sbs,size=fbox,colback=white,lower separated=false,
      righthand width=2cm,left=5mm]
    \docFading{#1}\tcblower
    \begin{tikzpicture}
        \fill [black!20] (0,0) rectangle (1,1);
        \path [pattern=checkerboard,pattern color=black!30] (0,0) rectangle (1,1);
        \fill [path fading=#1,blue] (0,0) rectangle (1,1);
    \end{tikzpicture}
    \end{tcolorbox}}%
  \doShadingExample{west}
  \doShadingExample{east}
  \doShadingExample{north}
  \doShadingExample{south}
  \doShadingExample{semi west}
  \doShadingExample{semi east}
  \doShadingExample{semi north}
  \doShadingExample{semi south}
\end{tcboxedraster}


\clearpage

\begin{vigTcbKey}[][doc new=2016-04-22]{fade in}{\colOpt{=\marg{style}}}{style, default |white|}
  Sets the four style options
  \refKey{/tcb/vig/north style},
  \refKey{/tcb/vig/south style},
  \refKey{/tcb/vig/east style}, and
  \refKey{/tcb/vig/west style}
  such that the paths fade from outside to inside.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \fill [black!20] (-0.5,-0.5) rectangle (1.5,1.5);
  \path [pattern=checkerboard,pattern color=black!30]
    (-0.5,-0.5) rectangle (1.5,1.5);
  \tcbvignette{fade in=blue}
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}


\begin{vigTcbKey}[][doc new=2016-04-22]{fade out}{\colOpt{=\marg{style}}}{style, default |white|}
  Sets the four style options
  \refKey{/tcb/vig/north style},
  \refKey{/tcb/vig/south style},
  \refKey{/tcb/vig/east style}, and
  \refKey{/tcb/vig/west style}
  such that the paths fade from inside to outside.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \fill [black!20] (-0.5,-0.5) rectangle (1.5,1.5);
  \path [pattern=checkerboard,pattern color=black!30]
    (-0.5,-0.5) rectangle (1.5,1.5);
  \tcbvignette{fade out=blue}
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}


\begin{vigTcbKey}[][doc new=2016-04-22]{semi fade in}{\colOpt{=\marg{style}}}{style, default |white|}
  Sets the four style options
  \refKey{/tcb/vig/north style},
  \refKey{/tcb/vig/south style},
  \refKey{/tcb/vig/east style}, and
  \refKey{/tcb/vig/west style}
  such that the paths fade weak from outside to inside.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \fill [black!20] (-0.5,-0.5) rectangle (1.5,1.5);
  \path [pattern=checkerboard,pattern color=black!30]
    (-0.5,-0.5) rectangle (1.5,1.5);
  \tcbvignette{semi fade in=blue}
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}


\begin{vigTcbKey}[][doc new=2016-04-22]{semi fade out}{\colOpt{=\marg{style}}}{style, default |white|}
  Sets the four style options
  \refKey{/tcb/vig/north style},
  \refKey{/tcb/vig/south style},
  \refKey{/tcb/vig/east style}, and
  \refKey{/tcb/vig/west style}
  such that the paths fade weak from inside to outside.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tikzpicture}
  \fill [black!20] (-0.5,-0.5) rectangle (1.5,1.5);
  \path [pattern=checkerboard,pattern color=black!30]
    (-0.5,-0.5) rectangle (1.5,1.5);
  \tcbvignette{semi fade out=blue}
\end{tikzpicture}
\end{dispExample*}
\end{vigTcbKey}




\clearpage
\subsection{Vignette as Underlay}\label{subsec:vignetteunderlay}

\begin{docTcbKey}[][doc new=2016-04-22]{underlay vignette}{\colOpt{=\marg{options}}}{style, no default}
  This puts a \refCom{tcbvignette} with the given \meta{options}
  as \refKey{/tcb/underlay} to a \refEnv{tcolorbox}.
  The dimensions of the \emph{vignette} are matched to the dimensions of
  the \refEnv{tcolorbox}. For example, \refKey{/tcb/leftrule} is used as
  \refKey{/tcb/vig/west size}. Also, \refKey{/tcb/colframe} is used as
  \refKey{/tcb/vig/raised color}.

  For a \refKey{/tcb/breakable} tcolorbox, the \emph{vignette} is also
  been broken.
  Alternatively, \refCom{tcbvignette} could be used directly inside
  an \refKey{/tcb/underlay} with appropriate settings.

\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tcolorbox}[enhanced,size=small,sharp corners,
  colback=green!10,colframe=green!50!black,
  boxrule=2mm,titlerule=0mm,
  title=My title,center title,fonttitle=\bfseries,
  underlay vignette]
    This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}

\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tcolorbox}[enhanced,size=small,arc=0pt,
  colback=blue!10,colframe=blue,boxrule=2mm,
  underlay vignette={size=1.5mm}]
    This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}

\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tcolorbox}[enhanced,size=small,sharp corners,
  colframe=red,interior hidden,boxrule=2mm,
  colupper=white,center upper,fontupper=\bfseries,
  underlay vignette]
    This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}

\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tcolorbox}[enhanced,size=small,sharp corners,
  colback=red!50!yellow,frame hidden,boxrule=2mm,
  underlay vignette={color from=red!50!yellow to white,
     draw method=clipped,size=2.1mm}]
    This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}

\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\tcbox[enhanced,sharp corners,colback=red!10,colframe=red]
  {Test}

\tcbox[enhanced,sharp corners,colback=red!10,colframe=red,
  underlay vignette]{Test}
\end{dispExample*}

\end{docTcbKey}


\clearpage
\begin{docTcbKey}[][doc new=2016-04-22]{underlay raised shading vignette}{\colOpt{=\marg{options}}}{style, no default}
  This is a special style derived from \refKey{/tcb/underlay vignette},
  where the frame color is shaded to create a soft raised frame impression.

\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tcolorbox}[enhanced,sharp corners,
  colback=green!10,
  colframe=green!50!black,
  size=small,boxrule=2mm,titlerule=0mm,
  title=My title,center title,fonttitle=\bfseries,
  underlay raised shading vignette]
    This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}



\begin{docTcbKey}[][doc new=2016-04-22]{underlay raised fading vignette}{\colOpt{=\marg{options}}}{style, no default}
  This style gives a similar effect as \refKey{/tcb/underlay raised shading vignette},
  but a path fading is used here. Different optical impression are very
  previewer-dependent.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tcolorbox}[enhanced,sharp corners,
  colback=green!10,
  colframe=green!50!black,
  size=small,boxrule=2mm,titlerule=0mm,
  title=My title,center title,fonttitle=\bfseries,
  underlay raised fading vignette]
    This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2016-04-22]{underlay shade in vignette}{\colOpt{=\marg{options}}}{style, no default}
  This is a special style derived from \refKey{/tcb/underlay vignette},
  where the frame color is shaded into the interior color.
\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tcolorbox}[enhanced,sharp corners,frame hidden,
  colback=green!10,
  colframe=green!50!black,
  size=small,boxrule=2mm,titlerule=0mm,
  underlay shade in vignette]
    This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}
\end{docTcbKey}


\clearpage
\subsection{Vignette as Finish}\label{subsec:vignettefinish}


\begin{docTcbKey}[][doc new=2016-04-22]{finish vignette}{\colOpt{=\marg{options}}}{style, no default}
  This puts a \refCom{tcbvignette} with the given \meta{options}
  as \refKey{/tcb/finish} to a \refEnv{tcolorbox}.
  The default style settings create a raised frame impression by
  drawing black and white color parts with reduced opacity.

\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tcolorbox}[enhanced,size=small,
  colback=green!10,colframe=green!50!black,
  boxrule=0.5mm,titlerule=0mm,
  title=My title,center title,fonttitle=\bfseries,
  finish vignette={size=1mm}]
    This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}

\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\tcbincludegraphics[blankest,width=3cm,
  finish vignette={size=3mm}]{pink_marble.png}
\end{dispExample*}
\end{docTcbKey}


\begin{docTcbKey}[][doc new=2016-04-22]{finish raised fading vignette}{\colOpt{=\marg{options}}}{style, no default}
  This puts a \refCom{tcbvignette} with the given \meta{options}
  as \refKey{/tcb/finish} to a \refEnv{tcolorbox}.
  The default style settings create a soft raised frame impression by
  drawing fading black and white color parts.

\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tcolorbox}[enhanced,size=small,
  colback=green!10,colframe=green!50!black,
  boxrule=0.5mm,titlerule=0mm,
  title=My title,center title,fonttitle=\bfseries,
  finish raised fading vignette={size=1mm}]
    This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}

\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\tcbincludegraphics[blankest,width=3cm,
  finish raised fading vignette={size=3mm}]{pink_marble.png}
\end{dispExample*}

\end{docTcbKey}


\clearpage
\begin{docTcbKey}[][doc new=2016-04-22]{finish fading vignette}{\colOpt{=\marg{options}}}{style, no default}
  This puts a \refCom{tcbvignette} with the given \meta{options}
  as \refKey{/tcb/finish} to a \refEnv{tcolorbox}.
  The default style settings fade the box into white from inside to outside.
  Note that \refKey{/tcb/vig/over node} is used here.
  \refKey{/tcb/vig/over node offset} can be adapted to overlap the box
  more or less. The fade color can be set using
  \refKey{/tcb/vig/base color}.

\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tcolorbox}[enhanced,size=small,
  colback=green!10,colframe=green!50!black,
  boxrule=0.5mm,titlerule=0mm,
  title=My title,center title,fonttitle=\bfseries,
  finish fading vignette={size=2mm}]
    This is a tcolorbox.
\end{tcolorbox}
\end{dispExample*}

\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\tcbincludegraphics[blankest,width=3cm,
  finish fading vignette={size=3mm}]{pink_marble.png}
\end{dispExample*}

\begin{dispExample*}{sbs,righthand width=3cm,center lower}
\begin{tcolorbox}[colback=blue!50!black,size=small,
  title=Example]
\tcbincludegraphics[blankest,
  finish fading vignette={base color=blue!50!black,size=3mm,
    over node offset=0.2mm}]{pink_marble.png}
\end{tcolorbox}
\end{dispExample*}

\end{docTcbKey}


\begin{dispExample*}{}
\begin{tcbitemize}[raster columns=3,bicolor,
  raster equal height,sharp corners,boxrule=2mm,
  colframe=red,colback=yellow!5,colbacklower=yellow!25!red!20]
\tcbitem A
\tcbitem[underlay vignette] B
\tcbitem[underlay={\tcbvignette{inside node=interior,
  lowered color=red,size=1mm}}] C
\tcbitem[underlay vignette,
  underlay={\tcbvignette{inside node=interior,
  lowered color=red,size=1mm}}] D
\tcbitem[boxrule=3mm,underlay vignette={size=2mm},
  underlay={\tcbvignette{inside node=interior,
  lowered color=red,size=1mm}}] E
\tcbitem[underlay raised shading vignette] F
\tcbitem[underlay raised shading vignette,
  underlay={\tcbvignette{inside node=interior,
  lowered color=red,size=1mm}}] G
\tcbitem[title=H1,underlay={\tcbvignette{inside node=interior,
  lowered color=red,size=1mm}},finish vignette] H2
\tcbitem[boxrule=0.25mm,colback=red!30,finish vignette] I1 \tcblower I2
\tcbitem[tile,colback=red!30,finish raised fading vignette] J1 \tcblower J2
\tcbitem[boxrule=1mm,underlay={\tcbvignette{inside node=interior,
  raised color=red,size=1mm}}] K
\tcbitem[boxrule=1mm,title=L1,underlay={\tcbvignette{inside node=title,
  lowered color=red,size=0.5mm}}] L2
\end{tcbitemize}
\end{dispExample*}


==> tcolorbox.doc.xparse.tex <==
% !TeX root = tcolorbox.tex
% include file of tcolorbox.tex (manual of the LaTeX package tcolorbox)
\clearpage
\section{Library \mylib{xparse}}\label{sec:xparse}%
\tcbset{external/prefix=external/xparse_}%
The library is loaded by a package option or inside the preamble by:
\begin{dispListing}
\tcbuselibrary{xparse}
\end{dispListing}
This also loads the package |xparse| \cite{latexproject:xparse}.

The purpose of this library is to give comfortable access to the
powerful document command production with |xparse| for |tcolorbox|.
See the |xparse| package documentation \cite{latexproject:xparse}
for details about the argument \meta{specification} used in this section.

%\subsection{Producing Document Commands With \texttt{xparse}}


\subsection{Option Keys}\label{subsec:xparse_options}

\begin{docTcbKey}{verbatim}{}{style, no value}
  Sets options for a \textit{verbatim} style \refCom{tcbox}.
  Since the indented boxes may contain only very few words, the
  dimensions are made smaller and \refKey{/tcb/nobeforeafter}
  and \refKey{/tcb/tcbox raise base} are set.
\begin{dispExample*}{sbs,lefthand ratio=0.6}
\DeclareTotalTCBox{\myverb}{ v }{verbatim,
  colframe=red!75!black,colupper=blue}{#1}

\myverb{\textbf} is a \myverb{\LaTeX} command.
\end{dispExample*}
\end{docTcbKey}


\begin{docTcbKey}{IfNoValueTF}{=\marg{argument}\marg{true options}\marg{false options}}{no default}
  Wraps the |\IfNoValueTF| command of |xparse| for option setting.
  If the \meta{argument} has no value, the \meta{true options} are set.
  Otherwise, the \meta{false options} are set.
\begin{dispExample}
\DeclareTColorBox{mybox}{ o }{colframe=red!75!black,
  IfNoValueTF={#1}{colback=red!5!white}{enhanced,interior style image=#1}}

\begin{mybox}
This is a tcolorbox.
\end{mybox}

\begin{mybox}[goldshade.png]
This is a tcolorbox.
\end{mybox}
\end{dispExample}
\end{docTcbKey}

\clearpage
\begin{docTcbKey}{IfValueTF}{=\marg{argument}\marg{true options}\marg{false options}}{no default}
  Wraps the |\IfValueTF| command of |xparse| for option setting.
  If the \meta{argument} has a value, the \meta{true options} are set.
  Otherwise, the \meta{false options} are set.
\begin{dispExample}
\DeclareTColorBox{mybox}{ o }{colframe=red!75!black,colback=red!5!white,
  IfValueTF={#1}{title={\flqq #1\frqq},fonttitle=\bfseries}{}}

\begin{mybox}
This is a tcolorbox.
\end{mybox}

\begin{mybox}[My title]
This is a tcolorbox.
\end{mybox}
\end{dispExample}
\end{docTcbKey}

\begin{docTcbKey}{IfBooleanTF}{=\marg{argument}\marg{true options}\marg{false options}}{no default}
  Wraps the |\IfBooleanTF| command of |xparse| for option setting.
  If the \meta{argument} is |\BooleanTue|, the \meta{true options} are set.
  If the \meta{argument} is |\BooleanFalse|, the \meta{false options} are set.

\begin{dispExample}
\DeclareTColorBox{mybox}{ s }{colframe=red!75!black,
  IfBooleanTF={#1}{colback=yellow!50!red}{colback=red!5!white}}

\begin{mybox}
This is a tcolorbox.
\end{mybox}

\begin{mybox}*
This is a tcolorbox.
\end{mybox}
\end{dispExample}
\end{docTcbKey}



\clearpage
\subsection{Producing \texttt{tcolorbox} Environments and Commands}\label{subsec:xparse_tcolorbox}

\begin{docCommand}{DeclareTColorBox}{\oarg{init options}\marg{name}\marg{specification}\marg{options}}
  Creates a new environment \meta{name} based on \refEnv{tcolorbox}.\\
  Basically, |\DeclareTColorBox| operates like |\DeclareDocumentEnvironment|. This means,
  the new environment \meta{name} is constructed with the given argument \meta{specification}.
  The \meta{options} are given to the underlying \refEnv{tcolorbox}.\\
  Note that \refKey{/tcb/savedelimiter} is set to the given \meta{name}
  automatically.\\
  The \meta{init options} allow setting up automatic numbering,
  see Section \ref{sec:initkeys} from page \pageref{sec:initkeys}.\\
  The new environment is always created, irrespective of an already existing
  environment with the same name.

\begin{dispExample}
% counter from previous example
\DeclareTColorBox[use counter from=pabox]{mybox}{ O{red} m d"" !O{} }
  {enhanced,colframe=#1!75!black,colback=#1!5!white,
   fonttitle=\bfseries,title={\thetcbcounter~#2},
   IfValueTF={#3}{watermark text={#3}}{},#4}

\begin{mybox}{My title}
This is a tcolorbox.
\end{mybox}

\begin{mybox}[blue]{My title}
This is a tcolorbox.
\end{mybox}

\begin{mybox}[green]{My title}"My Watermark"
This is a tcolorbox.
\end{mybox}

\begin{mybox}[yellow]{My title}[colbacktitle=yellow!50!white,coltitle=black]
This is a tcolorbox.
\end{mybox}

\begin{mybox}[purple]{My title}"All together"[coltitle=yellow]
This is a tcolorbox.
\end{mybox}
\end{dispExample}
\end{docCommand}

\clearpage
\begin{docCommand}{NewTColorBox}{\oarg{init options}\marg{name}\marg{specification}\marg{options}}
  Operates like \refCom{DeclareTColorBox}, but based on |\NewDocumentEnvironment| instead of |\DeclareDocumentEnvironment|.
  An error is issued if \meta{name} has already been defined.
\end{docCommand}

\begin{docCommand}{RenewTColorBox}{\oarg{init options}\marg{name}\marg{specification}\marg{options}}
  Operates like \refCom{DeclareTColorBox}, but based on |\RenewDocumentEnvironment| instead of |\DeclareDocumentEnvironment|.
  An existing environment is redefined.
\end{docCommand}

\begin{docCommand}{ProvideTColorBox}{\oarg{init options}\marg{name}\marg{specification}\marg{options}}
  Operates like \refCom{DeclareTColorBox}, but based on |\ProvideDocumentEnvironment| instead of |\DeclareDocumentEnvironment|.
  The environment \meta{name} is only created if it is not already defined.
\end{docCommand}


\clearpage

\begin{docCommand}{DeclareTotalTColorBox}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}\marg{content}}
  Creates a new command \texttt{\textbackslash}\meta{name} based on \refEnv{tcolorbox}.
  In contrast to \refCom{DeclareTColorBox}, also the \meta{content} of the |tcolorbox| is specified.\\
  Basically, |\DeclareTotalTColorBox| operates like |\DeclareDocumentCommand|. This means,
  the new command \texttt{\textbackslash}\meta{name} is constructed with the given argument \meta{specification}.
  The \meta{options} are given to the underlying \refEnv{tcolorbox} which is filled with
  the specified \meta{content}.\\
  Note that \refKey{/tcb/savedelimiter} is set to the given \meta{name}
  automatically.\\
  The \meta{init options} allow setting up automatic numbering,
  see Section \ref{sec:initkeys} from page \pageref{sec:initkeys}.\\
  The new command is always created, irrespective of an already existing
  command with the same name.

\begin{dispExample}
\DeclareTotalTColorBox{\diabox}{ O{} v  m }
  { bicolor,nobeforeafter,equal height group=diabox,width=5.7cm,
    fonttitle=\bfseries\ttfamily,adjusted title={#2},center title,
    colframe=blue!20!black,leftupper=0mm,rightupper=0mm,colback=black!75!white,#1}
  { \tikz\path[fill zoom image={#2}] (0,0) rectangle (\linewidth,4cm);%
    \tcblower#3}

\diabox{blueshade.png}{Created with |GIMP|.\\\url{http://www.gimp.org}}
\diabox{goldshade.png}{Created with |GIMP|.\\\url{http://www.gimp.org}}

\end{dispExample}
\end{docCommand}

\begin{docCommand}{NewTotalTColorBox}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}\marg{content}}
  Operates like \refCom{DeclareTotalTColorBox}, but based on |\NewDocumentCommand| instead of |\DeclareDocumentCommand|.
  An error is issued if \texttt{\textbackslash}\meta{name} has already been defined.
\end{docCommand}

\begin{docCommand}{RenewTotalTColorBox}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}\marg{content}}
  Operates like \refCom{DeclareTotalTColorBox}, but based on |\RenewDocumentCommand| instead of |\DeclareDocumentCommand|.
  An existing command is redefined.
\end{docCommand}

\begin{docCommand}{ProvideTotalTColorBox}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}\marg{content}}
  Operates like \refCom{DeclareTotalTColorBox}, but based on |\ProvideDocumentCommand| instead of |\DeclareDocumentCommand|.
  The command \texttt{\textbackslash}\meta{name} is only created if it is not already defined.
\end{docCommand}


\clearpage
\subsection{Producing \texttt{tcbox} Commands}\label{subsec:xparse_tcbox}


\begin{docCommand}{DeclareTCBox}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}}
  Creates a new command \texttt{\textbackslash}\meta{name} based on \refCom{tcbox}.
  Basically, |\DeclareTCBox| operates like |\DeclareDocumentCommand|. This means,
  the new command \texttt{\textbackslash}\meta{name} is constructed with the given argument \meta{specification}.
  The \meta{options} are given to the underlying \refCom{tcbox}.\\
  Note that \refKey{/tcb/savedelimiter} is set to the given \meta{name}
  automatically.\\
  The \meta{init options} allow setting up automatic numbering,
  see Section \ref{sec:initkeys} from page \pageref{sec:initkeys}.\\
  The new command is always created, irrespective of an already existing
  command with the same name.

\begin{dispExample}
% counter from previous example
\DeclareTCBox[use counter from=pabox]{\mybox}{ s m s }
{ nobeforeafter,colback=red!5!white,colframe=red!75!black,
  title={#2 (Box \thetcbcounter)},fonttitle=\bfseries,
  IfBooleanTF={#1}{enhanced,drop shadow}{},
  IfBooleanTF={#3}{colbacktitle=red!50!white}{}  }

\mybox{Bird}{This is my first box.}
  \hfill
\mybox*{Tree}{This is my second box.}
  \par\bigskip
\mybox{Bike}*{This is my third box.}
  \hfill
\mybox*{City}*{This is my fourth box.}
\end{dispExample}
\end{docCommand}

\begin{docCommand}{NewTCBox}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}}
  Operates like \refCom{DeclareTCBox}, but based on |\NewDocumentCommand| instead of |\DeclareDocumentCommand|.
  An error is issued if \texttt{\textbackslash}\meta{name} has already been defined.
\end{docCommand}

\begin{docCommand}{RenewTCBox}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}}
  Operates like \refCom{DeclareTCBox}, but based on |\RenewDocumentCommand| instead of |\DeclareDocumentCommand|.
  An existing command is redefined.
\end{docCommand}

\begin{docCommand}{ProvideTCBox}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}}
  Operates like \refCom{DeclareTCBox}, but based on |\ProvideDocumentCommand| instead of |\DeclareDocumentCommand|.
  The command \texttt{\textbackslash}\meta{name} is only created if it is not already defined.
\end{docCommand}



\clearpage

\begin{docCommand}{DeclareTotalTCBox}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}\marg{content}}
  Creates a new command \texttt{\textbackslash}\meta{name} based on \refCom{tcbox}.
  In contrast to \refCom{DeclareTCBox}, also the \meta{content} of the |tcbox| is specified.\\
  Basically, |\DeclareTotalTCBox| operates like |\DeclareDocumentCommand|. This means,
  the new command \texttt{\textbackslash}\meta{name} is constructed with the given argument \meta{specification}.
  The \meta{options} are given to the underlying \refCom{tcbox} which is filled with
  the specified \meta{content}.\\
  Note that \refKey{/tcb/savedelimiter} is set to the given \meta{name}
  automatically.\\
  The \meta{init options} allow setting up automatic numbering,
  see Section \ref{sec:initkeys} from page \pageref{sec:initkeys}.\\
  The new command is always created, irrespective of an already existing
  command with the same name.

\begin{dispExample}
\DeclareTotalTCBox{\myverb}{ O{red} v !O{} }
{ fontupper=\ttfamily,nobeforeafter,tcbox raise base,arc=0pt,outer arc=0pt,
  top=0pt,bottom=0pt,left=0mm,right=0mm,
  leftrule=0pt,rightrule=0pt,toprule=0.3mm,bottomrule=0.3mm,boxsep=0.5mm,
  colback=#1!10!white,colframe=#1!50!black,#3}{#2}

To set a word \textbf{bold} in \myverb{\LaTeX}, use
\myverb[green]{\textbf{bold}}. Alternatively, write
\myverb[yellow]{{\bfseries bold}}.
In \myverb[blue]{\LaTeX}[enhanced,fuzzy halo], other font settings are
done in the same way, e.\,g. \myverb{\textit}, \myverb{\itshape}\\
or \myverb[brown]{\texttt}, \myverb[brown]{\ttfamily}.
\end{dispExample}

The next example uses |\lstinline| from the |listings| package to
typeset the verbatim content.

\begin{dispExample}
% \usepackage{listings} or \tcbuselibrary{listings}
\DeclareTotalTCBox{\commandbox}{ s v }
{verbatim,colupper=white,colback=black!75!white,colframe=black}
{\IfBooleanTF{#1}{\textcolor{red}{\ttfamily\bfseries > }}{}%
  \lstinline[language=command.com,keywordstyle=\color{blue!35!white}\bfseries]^#2^}

\commandbox*{cd "My Documents"} changes to directory \commandbox{My Documents}.

\commandbox*{dir /A} lists the directory content.

\commandbox*{copy example.txt d:\target} copies \commandbox{example.txt} to
  \commandbox{d:\target}.
\end{dispExample}
\end{docCommand}

\clearpage
\begin{docCommand}{NewTotalTCBox}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}\marg{content}}
  Operates like \refCom{DeclareTotalTCBox}, but based on |\NewDocumentCommand| instead of |\DeclareDocumentCommand|.
  An error is issued if \texttt{\textbackslash}\meta{name} has already been defined.
\end{docCommand}

\begin{docCommand}{RenewTotalTCBox}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}\marg{content}}
  Operates like \refCom{DeclareTotalTCBox}, but based on |\RenewDocumentCommand| instead of |\DeclareDocumentCommand|.
  An existing command is redefined.
\end{docCommand}

\begin{docCommand}{ProvideTotalTCBox}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}\marg{content}}
  Operates like \refCom{DeclareTotalTCBox}, but based on |\ProvideDocumentCommand| instead of |\DeclareDocumentCommand|.
  The command \texttt{\textbackslash}\meta{name} is only created if it is not already defined.
\end{docCommand}


\begin{docCommand}{tcboxverb}{\oarg{options}\marg{verbatim box content}}
  Creates a colored box based on \refCom{tcbox} which is fitted to the width of the given
  \meta{verbatim box content}.
  The underlying \refCom{tcbox} is styled with
  \refKey{/tcb/verbatim} plus the given \meta{options}.
  The difference to \refCom{tcbox} is that the \meta{verbatim box content} is
  interpreted \textit{verbatim}. Therefore, |\tcboxverb| acts similar to |\verb|.

\begin{dispExample}
\tcboxverb{\LaTeX}, \tcboxverb[colback=blue!10!white,colupper=blue]{\LaTeX},
\tcboxverb[blank,fuzzy halo]{\LaTeX}, \tcboxverb[beamer]{\LaTeX},
\tcboxverb[enhanced,skin=enhancedmiddle jigsaw,colframe=red]{\LaTeX}.
\end{dispExample}
\end{docCommand}




\clearpage
\subsection{Producing \texttt{tcblisting} Environments}\label{subsec:xparse_listing}
\begin{marker}
Besides \mylib{xparse}, the following commands also need the \mylib{listings} library to be included.
\end{marker}

\begin{docCommand}{DeclareTCBListing}{\oarg{init options}\marg{name}\marg{specification}\marg{options}}
  Creates a new environment \meta{name} based on \refEnv{tcblisting}.\\
  Basically, |\DeclareTCBListing| operates like |\DeclareDocumentEnvironment|. This means,
  the new environment \meta{name} is constructed with the given argument \meta{specification}.
  The \meta{options} are given to the underlying \refEnv{tcblisting}.\\
  Note that \refKey{/tcb/savedelimiter} is set to the given \meta{name}
  automatically.\\
  The \meta{init options} allow setting up automatic numbering,
  see Section \ref{sec:initkeys} from page \pageref{sec:initkeys}.\\
  The new environment is always created, irrespective of an already existing
  environment with the same name.

\begin{dispExample*}{sbs,lefthand ratio=0.5}
\DeclareTCBListing{mybox}{ s O{} m }{%
  colback=red!5!white,
  colframe=red!75!black,
  fonttitle=\bfseries,
  IfBooleanTF={#1}
    {listing side text}
    {text side listing},
  title=#3,#2}

\begin{mybox}{Listing Box}
This is my
\LaTeX\ box.
\end{mybox}
\bigskip

\begin{mybox}*{Listing Box}
This is my
\LaTeX\ box.
\end{mybox}
\bigskip

\begin{mybox}[colback=yellow]
  {Listing Box}
This is my
\LaTeX\ box.
\end{mybox}
\end{dispExample*}
\end{docCommand}



\begin{docCommand}{NewTCBListing}{\oarg{init options}\marg{name}\marg{specification}\marg{options}}
  Operates like \refCom{DeclareTCBListing}, but based on |\NewDocumentEnvironment| instead of |\DeclareDocumentEnvironment|.
  An error is issued if \meta{name} has already been defined.
\end{docCommand}

\begin{docCommand}{RenewTCBListing}{\oarg{init options}\marg{name}\marg{specification}\marg{options}}
  Operates like \refCom{DeclareTCBListing}, but based on |\RenewDocumentEnvironment| instead of |\DeclareDocumentEnvironment|.
  An existing environment is redefined.
\end{docCommand}

\begin{docCommand}{ProvideTCBListing}{\oarg{init options}\marg{name}\marg{specification}\marg{options}}
  Operates like \refCom{DeclareTCBListing}, but based on |\ProvideDocumentEnvironment| instead of |\DeclareDocumentEnvironment|.
  The environment \meta{name} is only created if it is not already defined.
\end{docCommand}

\clearpage


\begin{marker}
With date of 2018-05-12, the |xparse| \cite{latexproject:xparse} package
changed the argument collection process.
Now, spaces are ignored which leads to a serious change for listing environments
ending with an optional argument like \verb+O{}+.
The former behaviour of respecting spaces can be preserved by adding a \flqq\verb+!+\frqq.
Note that the following code uses \verb+!O{}+ now.
\begin{itemize}
\item For older |xparse| versions, the following code is correct when using \verb+O{}+.
\item For |xparse| of 2018-05-12, only the first two examples of
  the following code using \verb+O{}+ are really \flqq good\frqq\ -- all others do not work.
\item For |xparse| of 2018-05-12 and later, the following code is correct when using \verb+!O{}+.
\end{itemize}
\end{marker}





\begin{dispListing*}{title={Caveats of using an environment ending with an
  optional argument},fonttitle=\bfseries}
\DeclareTCBListing{mybox}{ !O{} }{listing only,#1}

\begin{mybox}[colframe=red]
\good
\end{mybox}

\begin{mybox}[colframe=red]\good\end{mybox}

\begin{mybox}
\good
\end{mybox}

\begin{mybox} \good\end{mybox}

\begin{mybox}\bad!\end{mybox}

\begin{mybox}
[\good]
\end{mybox}

\begin{mybox} [\good]\end{mybox}

\begin{mybox}[\bad!]\end{mybox}
\end{dispListing*}

\clearpage
\subsection{Producing \texttt{tcbinputlisting} Commands}\label{subsec:xparse_inputlisting}
\begin{marker}
The following commands need the \mylib{listings} library to be included.
\end{marker}


\begin{docCommand}{DeclareTCBInputListing}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}}
  Creates a new command \texttt{\textbackslash}\meta{name} based on \refCom{tcbinputlisting}.
  Basically, |\DeclareTCBInputListing| operates like |\DeclareDocumentCommand|. This means,
  the new command \texttt{\textbackslash}\meta{name} is constructed with the given argument \meta{specification}.
  The \meta{options} are given to the underlying \refCom{tcbinputlisting}.\\
  The \meta{init options} allow setting up automatic numbering,
  see Section \ref{sec:initkeys} from page \pageref{sec:initkeys}.\\
  The new command is always created, irrespective of an already existing
  command with the same name.

\begin{dispExample}
% counter from previous example
\DeclareTCBInputListing[use counter from=pabox]{\mylisting}{ O{} O{red} m }{%
  listing file={#3},title=Listing~\thetcbcounter,
  colback=#2!5!white,colframe=#2!50!black,colbacktitle=#2!75!black,
  fonttitle=\bfseries,listing only,#1}

\mylisting[before upper=\textit{This is the included file content:}]
  [blue]{\jobname.tcbtemp}
\end{dispExample}
  \end{docCommand}

\begin{docCommand}{NewTCBInputListing}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}}
  Operates like \refCom{DeclareTCBInputListing}, but based on |\NewDocumentCommand| instead of |\DeclareDocumentCommand|.
  An error is issued if \texttt{\textbackslash}\meta{name} has already been defined.
\end{docCommand}

\begin{docCommand}{RenewTCBInputListing}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}}
  Operates like \refCom{DeclareTCBInputListing}, but based on |\RenewDocumentCommand| instead of |\DeclareDocumentCommand|.
  An existing command is redefined.
\end{docCommand}

\begin{docCommand}{ProvideTCBInputListing}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}}
  Operates like \refCom{DeclareTCBInputListing}, but based on |\ProvideDocumentCommand| instead of |\DeclareDocumentCommand|.
  The command \texttt{\textbackslash}\meta{name} is only created if it is not already defined.
\end{docCommand}


\clearpage
\subsection{Producing \texttt{tboxfit} Commands}\label{subsec:xparse_tcboxfit}
\begin{marker}
The following commands need the \mylib{fitting} library to be included.
\end{marker}

\begin{docCommand}{DeclareTCBoxFit}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}}
  Creates a new command \texttt{\textbackslash}\meta{name} based on \refCom{tcboxfit}.
  Basically, |\DeclareTCBoxFit| operates like |\DeclareDocumentCommand|. This means,
  the new command \texttt{\textbackslash}\meta{name} is constructed with the given argument \meta{specification}.
  The \meta{options} are given to the underlying \refCom{tcboxfit}.\\
  Note that \refKey{/tcb/savedelimiter} is set to the given \meta{name}
  automatically.\\
  The \meta{init options} allow setting up automatic numbering,
  see Section \ref{sec:initkeys} from page \pageref{sec:initkeys}.\\
  The new command is always created, irrespective of an already existing
  command with the same name.

\begin{dispExample*}{sbs,lefthand ratio=0.6}
% \usepackage{lipsum}

\DeclareTCBoxFit{\mybox}{ O{} m !o }
 {colback=red!5!white,
  colframe=red!75!black,
  width=#2,height=#2/3*2,
  IfValueTF={#3}{height=#3}{},
  #1}

\mybox[colback=yellow]{5cm}%
  {\lipsum[2]}

\mybox[colback=yellow]{5cm}[4cm]{\lipsum[2]}
\end{dispExample*}
\end{docCommand}

\begin{docCommand}{NewTCBoxFit}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}}
  Operates like \refCom{DeclareTCBoxFit}, but based on |\NewDocumentCommand| instead of |\DeclareDocumentCommand|.
  An error is issued if \texttt{\textbackslash}\meta{name} has already been defined.
\end{docCommand}

\begin{docCommand}{RenewTCBoxFit}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}}
  Operates like \refCom{DeclareTCBoxFit}, but based on |\RenewDocumentCommand| instead of |\DeclareDocumentCommand|.
  An existing command is redefined.
\end{docCommand}

\begin{docCommand}{ProvideTCBoxFit}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}}
  Operates like \refCom{DeclareTCBoxFit}, but based on |\ProvideDocumentCommand| instead of |\DeclareDocumentCommand|.
  The command \texttt{\textbackslash}\meta{name} is only created if it is not already defined.
\end{docCommand}

\clearpage

\begin{docCommand}{DeclareTotalTCBoxFit}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}\marg{content}}
  Creates a new command \texttt{\textbackslash}\meta{name} based on \refCom{tcboxfit}.
  In contrast to \refCom{DeclareTCBoxFit}, also the \meta{content} of the |tcboxfit| is specified.\\
  Basically, |\DeclareTotalTCBoxFit| operates like |\DeclareDocumentCommand|. This means,
  the new command \texttt{\textbackslash}\meta{name} is constructed with the given argument \meta{specification}.
  The \meta{options} are given to the underlying \refCom{tcboxfit} which is filled with
  the specified \meta{content}.\\
  Note that \refKey{/tcb/savedelimiter} is set to the given \meta{name}
  automatically.\\
  The \meta{init options} allow setting up automatic numbering,
  see Section \ref{sec:initkeys} from page \pageref{sec:initkeys}.\\
  The new command is always created, irrespective of an already existing
  command with the same name.

\begin{dispExample}
% \usepackage{lipsum}

\DeclareTotalTCBoxFit{\multibox}{ O{} m O{10} m }
 {nobeforeafter,colback=red!5!white,colframe=red!75!black,width=#2,height=#2/3*2,
  valign=center,#1}
 { \foreach \n in {1,...,#3} { #4} }

\multibox{5cm}{I shall not repeat.}
\multibox[colframe=blue!75!white]{5cm}[20]{I shall not repeat.}\\
\multibox[colback=yellow,height=5cm]{14cm}[100]{I shall not repeat.}
\end{dispExample}
\end{docCommand}

\begin{docCommand}{NewTotalTCBoxFit}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}\marg{content}}
  Operates like \refCom{DeclareTotalTCBoxFit}, but based on |\NewDocumentCommand| instead of |\DeclareDocumentCommand|.
  An error is issued if \texttt{\textbackslash}\meta{name} has already been defined.
\end{docCommand}

\begin{docCommand}{RenewTotalTCBoxFit}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}\marg{content}}
  Operates like \refCom{DeclareTotalTCBoxFit}, but based on |\RenewDocumentCommand| instead of |\DeclareDocumentCommand|.
  An existing command is redefined.
\end{docCommand}

\begin{docCommand}{ProvideTotalTCBoxFit}{\oarg{init options}\brackets{\texttt{\textbackslash}\meta{name}}\marg{specification}\marg{options}\marg{content}}
  Operates like \refCom{DeclareTotalTCBoxFit}, but based on |\ProvideDocumentCommand| instead of |\DeclareDocumentCommand|.
  The command \texttt{\textbackslash}\meta{name} is only created if it is not already defined.
\end{docCommand}

